Existence of spiral strategies for blocking fire spreading

In this paper we address the problem for blocking fire by constructing a wall $\zeta$ whose shape is spiral-like. This is supposed to be the best strategy when a single firefighter is constructing the wall with a finite construction speed $\sigma$: the barriers which satisfy this bound on the construction speed are called admissible. We prove a sharp version of Bressan's Fire Conjecture in this case, i.e. when admissible barriers are spiral-like curves: namely, there exists a spiral-like barrier confining the fire in a bounded region of $\mathbb R^2$ if and only if the speed of construction of the barrier $\sigma$ is strictly larger than a critical speed $\bar \sigma = 2.614...$. The existence of confining spiral barriers for $\sigma > \bar \sigma$ is already known [Bressan A. et al., 2008, Klein R. et al., 2019], while we concentrate on the negative side, i.e. if $\sigma \leq \bar \sigma$ no admissible spiral blocks the fire. The proof of these results relies on: 1) the precise definition of spiral barrier and its representation; 2) the analysis of saturated spiral barriers as a Retarded Differential Equation (RDE) in the spirit of [Klein R. et al., 2019]; 3) the equivalent reformulation of the conjecture as a minimum problem for a prescribed functional; 4) the construction of the optimal closing spiral; 5) the analysis of a differentiable path of admissible spirals along which the functional is differentiable, and in particular increasing when moving from the optimal spiral to any other one (homotopy argument). Due to the complexity of the solution, the evaluation of the quantities needed to prove that the functional is increasing is performed numerically.

==> Martina_Correzioni/intro__edited_.tex <==
\section{Introduction}
\label{S:intro}


We study a dynamic blocking problem first proposed by A. Bressan in \cite{Bressan_2007}. The problem is concerned with the model of wild fire spreading in a region of the plane $\R^2$ and the possibility to block it by constructing \emph{barriers}, i.e. rectifiable curves which cannot be crossed by the fire. The local fire spreading is described by giving a set valued function
$$
F : \R^2 \to \big\{ K \subset \R^2 \ \text{compact, closed} \big\}.
$$
such that
\begin{enumerate}
\item there exists $r>0$ such that $B_r(0)\subset F(x)\quad\forall x\in\R^2$;
%\item $F(x)$ is compact and convex $\forall x   \in\R^2$;
\item $x\rightarrow F(x)$ is Lipschitz-continuous in the Hausdorff topology.
\end{enumerate}
This function represents the infinitesimal fire evolution when barriers are not present, i.e. $x + \delta t F(x)$ are the points reached by the fire in the infinitesimal time $\delta t$. In other words, if barriers are not present, the \emph{reachable set $R(t)$} is the solution to the differential inclusion
\begin{equation*}
R(t) = \Big\lbrace x(t), \quad x(\cdot) \text{ abs. cont.},\ x(0) \in R_0,\ \dot x(\tau)\in F(x(\tau))\text{ for a.e. }\tau\in[0,t] \Big\rbrace,
\end{equation*}
where the set $R_0\subset\R^2$ is the open region burnt by the fire at the initial time $t=0$.

%
%
%representing the local speed of the fire at the point $x$
%
%If we denote by $R(t)\subset\R^2$ the region burned by the fire at time $t$, then we can describe it as the reachable set for a differential inclusion. More precisely, one considers the Cauchy Problem
%\begin{equation*}
%    \dot{x}\in F(x),\qquad x(0)\in R_0,
%\end{equation*}
%, while the function $F$ describes the speed of spreading of the fire. The set $R_0\subset\R^2$ is assumed to be open, bounded, non-empty and connected with Lipschitz boundary, whereas the standard assumptions on $F:\R^2\rightarrow \R^2$, which is a Lipschitz-continuous multifunction, are:
%\begin{enumerate}
%    \item there exists $r>0$ such that $B_r(0)\subset F(x)\quad\forall x\in\R^2$;
%    \item $F(x)$ is compact and convex $\forall x   \in\R^2$;
%    \item $x\rightarrow F(x)$ is Lipschitz-continuous in the Hausdorff topology. 
%\end{enumerate}
%\noindent If no barriers are present 

When the fire starts spreading, a fireman can construct some barriers, modeled by a one-dimensional rectifiable set $\zeta\subset\R^2$, in order to block the fire. More in detail, we consider a continuous function $\psi: \R^2 \rightarrow \R^+$ together with a positive constant $\psi_0>0$ such that $\psi\geq\psi_0$. If we denote by $\zeta(t)\subset\R^2$ the portion of the barrier constructed within the time $t\geq 0$, we say that  $\zeta$ is an admissible barrier (or admissible strategy) if
\begin{enumerate}
\item{(H1)}\label{admissibility:con:1} $\zeta(t_1)\subset \zeta(t_2)$, $\forall  t_1\leq t_2$;
\item{(H2)}\label{admissibility:con:2} $\int_{\zeta(t)}\psi d\H^1\leq t,\quad \forall t\geq 0$,
\end{enumerate}
where $\H^1$ denotes the one-dimensional Hausdorff measure. Once we have an admissible strategy $\zeta$, then we define the reachable set for $\zeta$ at time $t$ the set
\begin{equation}\label{def:reach:set}
R^\zeta(t) = \Big\lbrace x(t): x\text{ abs. cont.},\ x(0) \in R_0, \ \dot x(\tau)\in F(x(\tau))\text{ for a.e. } \tau\in[0,t],\ x(\tau)\not\in\zeta(\tau) \ \forall\tau\in[0,t] \Big\rbrace.
\end{equation}

\begin{definition}
Let $t\rightarrow\zeta(t)$ be an admissible strategy. We say that it is a \emph{blocking} strategy if
\begin{equation*}
R^\zeta_\infty\doteq\bigcup_{t\geq 0} R^\zeta(t)
\end{equation*}
is a bounded set.
\end{definition}

We call \emph{isotropic} the case in which the fire is assumed to propagate with unit speed in all directions, while the barrier is constructed at a constant speed $\sigma>0$, namely
\begin{equation}
\label{isotropic case}
F \equiv \overline{B_1(0)},\quad R_0=B_1(0), \quad \psi\equiv\frac{1}{\sigma},
\end{equation}
where $\overline{B_1(0)}$ denotes the closure of the unit ball of the plane centered at the origin. We remark that in \cite{Bressan_friends} there are comparison results between more general choices of the data $R_0$ and $F$ and the isotropic problem for the study of the fire problem in a more general setting. 

The existence of admissible blocking (or winning) strategies for the isotropic blocking problem is a very challenging open problem and it has been addressed mainly in \cite{Bressan_2007},\cite{Bressan_friends}.\footnote{One can prove that the existence of blocking strategy does not depend on the starting set $R_0$ but only on the speed $\sigma$ \cite{Bressan_survey}. {\color{red} This is one of the main motivations for which the problem has been mainly studied in the isotropic case.} In particular, the following theorems hold:

\begin{theorem}
\label{thm:existence:2}
Assume that \eqref{isotropic case} hold. Then if $\sigma>2$ there exists an admissible blocking strategy.
\end{theorem}

\begin{theorem}
\label{thm:nonexistence:1}
Assume that \eqref{isotropic case} hold. Then if $\sigma\leq 1$ no admissible blocking strategy exists.
\end{theorem}

 The two theorems are proved in  \cite{Bressan_2007} and they motivate the following Fire Conjecture \cite{Bressan_conj}:
\begin{conjecture}
\label{conj:bressan}
Let \eqref{isotropic case} hold. Then if $\sigma\leq 2$ no admissible blocking strategy exists.
\end{conjecture}
For a survey of results related to the previous conjecture, see \cite{Bressan_survey}.

\medskip

\textbf{Equivalent formulation.} Throughout the paper we will use the following equivalent formulation of the dynamic blocking problem for the isotropic case (for a proof of the equivalence, see \cite{Bressan_equivalent}): let $Z\subset\R^2$ be a rectifiable set. We denote by
\begin{equation}
\label{eq:burned:region_intro}
R^Z(t) = \Big\lbrace  x(t): x\text{ abs. cont.},\ \dot x(\tau) \in \overline{B_1(0)} \text{ for a.e. } \tau \in [0,t],\ x(\tau)\not\in Z \ \forall \tau \in[0,t] \Big\rbrace.
\end{equation}
We say that the strategy $Z$ is \emph{admissible} if $\forall t\geq 0$
\begin{equation}
\H^1(Z\cap\overline{R^Z(t)})\leq\sigma t.
\end{equation}
Similarly to the previous formulation we denote by
\begin{equation}
\label{eq:burned:region}
R^Z_\infty = \bigcup_{t\geq 0} R^Z(t)
\end{equation}
the burned region and we say that $Z$ is an admissible blocking strategy if $R^Z_\infty$ is bounded. The advantage of this description is that the barrier is fixed and it does not grow while the time evolves. Here we can interpret $Z \cap \overline{R^Z(t)}$ as the amount of barrier $Z$ burned by the fire within the time $t$.

\medskip

 \textbf{Minimum time function and Hamilton-Jacobi formulation.} The propagation of fire can be described also in terms of the minimum time function
\begin{equation}\label{eq:min:time:function}
u(x) \doteq \inf \big\lbrace t \geq 0:\ x \in \overline{R^Z(t)} \big\rbrace.
\end{equation}
The function $u$ is the time needed for the fire to reach the point $x$ in the burned region, without crossing the barrier. The minimum time function can be computed by solving an Hamilton-Jacobi equation with obstacles, namely
\begin{equation}
\label{eq:hamilton:jacobi}
\begin{cases}
|\nabla u(x)|\leq 1 \qquad x\not\in Z, \\
u(x)=0 \qquad x\in R_0.
\end{cases}
\end{equation}
For the properties of the solution of \eqref{eq:hamilton:jacobi} we refer to \cite{delellisrobyr}. We conjecture that $|\nabla u(x)|=1$ for every $x\not\in Z$ as in the classic case of Eikonal equation without obstacle{\color{red}s}. Given the minimum time function $u$, and an admissible barrier $Z$, one defines the following \emph{Admissibility Functional}
\begin{equation*}
\mathcal A(x) = u(x) - \frac{1}{\sigma} \H^1 \big( Z\cap\overline{R^Z(u(x))} \big) \geq 0, \quad \forall x \in Z.
\end{equation*}
The inequality follows by the admissibility of the barrier $Z$.
In particular, one defines the \emph{saturated set} as
\begin{equation*}
\mathcal{S} = \big\lbrace x \in Z:\ \mathcal A(x) = 0 \big\rbrace,
\end{equation*}
corresponding to those points on the barrier where the firefighters are using all the barrier available in order to block the fire.

One can easily prove that if the strategy $Z$ consists of a simple closed curve, then it is not admissible for $\sigma\leq 2$ \cite{Bressan_2007} (the key idea is taking the last point $P$ on the curve reached by the fire and observing that $\mathcal{A}(P)<0$), but {\color{red} there are} only partial results are {\color{red}togli present}present in the literature if the strategy has more complicated structures, as for example the presence of internal barriers that slow down the fire.
\medskip

%One possible idea to prove the conjecture would be to investigate the shape of a strategy which is \emph{optimal} among admissible strategies, allowing for the presence of some internal barriers. 
 \textbf{Optimization problem}. {\color{red} A possible approach to attack Bressan's Fire Conjecture \eqref{conj:bressan} would be to look at optimal strategies for a given minimization problem and prove that they can not be admissible blocking strategies, reducing the analysis to concrete cases. In this spirit, one  can give an optimization problem among blocking barriers as follows:} one introduces the following cost functional
\begin{equation}\label{eq:opt:problem}
    J(Z)=\int_{R^Z_\infty} \kappa_1 d\mathcal{L}^2 +\int_{Z}\kappa_2 d\H^1,
\end{equation}
among all possible admissible blocking strategies, where $\kappa_1,\kappa_2:\R^2\rightarrow \R^+$ are two non-negative continuous functions. In \cite{Bressan_deLellis} it is proved that, if the class of admissible blocking strategies is non-empty, then there exists an optimal strategy. Moreover, there exists an optimal strategy $Z^*$ which is \emph{complete}:
\begin{definition}
Let $Z\subset\R^2$ be a rectifiable set. $Z$ is complete if it contains all its points of positive upper density,  that is, let $x\in\R^2$ such that
\begin{equation*}
\limsup_{r\to 0^+} \frac{\H^1(Z\cap B_r(x))}{2r}>0 \Longrightarrow x\in Z.
\end{equation*}
\end{definition}
 The following corollary also holds \cite{Bressan_equivalent}:
\begin{corollary}
If there exists an admissible blocking strategy $Z$ with $\H^1(Z)<\infty$, then there exists an optimal blocking strategy $Z^*$ such that
\begin{equation*}
Z^* = \bigg( \bigcup_i Z_i \bigg) \cup \mathcal{N},
\end{equation*}
where $Z_i$ are countably many compact rectifiable connected components and $\H^1(\mathcal{N})=0$.
\end{corollary}
We mention also the recent result in \cite{Bressan_Chiri} where it is proved that the optimal strategy is nowhere dense.  
What really makes the optimization problem hard is that the class of admissible strategy could be empty (and it is conjectured to be empty if $\sigma\leq 2${\color{red}, Conjecture }\ref{conj:bressan}).

Giving necessary conditions for optimality is a hard open problem. Some necessary optimality conditions are derived in \cite{Bressan_optnec} assuming further regularity on the optimal strategy. In \cite{FireSegment} some necessary optimality condition {\color{red} are given in order to} characterize the boundary $\partial R^Z_\infty$ in the case $Z$ is an optimal strategy (for the problem $\kappa_1=0$, $\kappa_2=1$) without assuming any regularity assumption on the barrier. There, some properties of the optimal barrier are derived, as the connectedness in the case the $Z=Z^2\cup Z^1$ where $Z^2=\partial R^Z_\infty$ and $Z^1$ is a single internal curve, and some concrete cases are analyzed. The major issue, however, remains deriving necessary conditions for internal barriers.


\subsection{Non admissibility of spiral-like strategies}
\label{Ss:spiral_intro}


In this paper we study spiral-like strategies: namely, admissible barriers that are constructed putting all the effort on a single curve. The study of {\color{red} spiral} strategies is of key importance in the  complete solution of Bressan's Fire conjecture, indeed {\color{red} it is conjectured} that these strategies are the "best" possible barriers that can be constructed when $\sigma\leq 2$. The heuristic reason is that, if $\sigma\leq 2$, then we can not have two firefighters (constructing {\color{red}simultaneously} two branches of {\color{red}the} strategy) with speed strictly greater than the speed of the fire{\color{red},} so that they will be engulfed by the fire: thus the best strategy should be a single curve. The case $\sigma>2$ is different, indeed we expect that the optimal strategies in this case are simple closed curves. In \cite{Bressan_isotropic} the authors construct the best strategy for the optimization problem \ref{eq:opt:problem} among simple closed curves.

\medskip

We start giving the definition of spiral strategies.

\begin{definition}[Spiral strategies]
\label{Def:spiral_barrier_intro}
Let $Z = \zeta([0,S]) \subset \R^2$ be a strategy, where $\zeta$ is a Lipschitz curve parametrized by arc-length. We say that it is a \emph{spiral strategy} if it satisfies:
\begin{enumerate}
\item $\zeta(0) = (1,0)$ and $\zeta \rest_{[0,S)}$ is simple,
\item $s \mapsto u \circ \zeta(s)$ is increasing,
\item $\zeta$ is locally convex, i.e. locally it is the graph of a convex function,
\item \label{Point:4_intro_def_spiral} it holds
\begin{equation*}
%\text {(A1)} \qquad 
0 \leq \angle (\textbf{t}^+(0),\textbf{e}_2)\leq \frac{\pi}{2},
\end{equation*}
{\color{red} $\zeta$ is rotating counterclockwise about $0$. For a precise definition, see Section \ref{Ss:spiral_barriers}.}
\end{enumerate}
The spiral $\zeta$ is \emph{admissible} if it is also an admissible barrier.
\end{definition}

The assumptions that $\zeta$ is locally convex yields a direction of rotation to the curve, and then Point \eqref{Point:4_intro_def_spiral} {\color{red} selects a direction of rotation} (Proposition \ref{thm:param_1}).

%
%Finally, we say that $Z$ is an admissible spiral if it is a spiral-like strategy,   the curve is locally convex, in the sense of Definition \ref{def:convexity:spiral} and moreover it satisfies the following assumption
%
%where $\textbf{e}_2$ is the vertical vector of the canonical base  $\mathbf t(0)$ is the tangent vector of the spiral in the starting point (commonly $(1,0)$) and $\angle$ denotes the angle between the two vectors. 

A deeper discussion is needed for the assumption %requirement
\begin{equation*}
s \rightarrow u\circ\zeta(s) \quad \text{ is increasing},
\end{equation*}
which corresponds to the fact that either a portion of the barrier lies on the level set $\lbrace u=t\rbrace$ (so that the previous function is constant), or the fire can not burn two portions of the barrier simultaneously. This means that the barrier $\zeta(\{s \geq \bar s\})$ depends only on the time function $u$ constructed with $\zeta([0,\bar s])$ is place {\color{red} che volevi dire con questa frase?}, and we do not need to compensate part{\color{red}s} of $\zeta([0,\bar s])$ which will be reached by fire at a later time: in particular, given the barrier up to time $\bar t$ (or equivalently length $\bar s$), we can ask which is the optimal barrier for a given optimization problem with the same freedom as for the initial problem. This final observation will be {\color{red} of }fundamental {\color{red} importance} in our homotopy argument {\color{red} (point $(5)$ in the abstract)}.


%We believe instead that the hypothesis of local convexity and the assumption $(A1)$ are automatically satisfied by \emph{optimal} spiral-like strategies, which is an open question. 
%\medskip
%
%In addition to the parametrization by arc-length, it is possible to parametrize any admissible spiral by $(r(\phi),\phi)$, where $\phi$ denotes the angle of rotation on the spiral, which is defined in Lemma \ref{lem:ODE:spiral}, while $r(\phi)$ represents the length of the final segment of the fire ray reaching the point $(r(\phi),\phi)$, as explained in Figure \ref{fig:param:spiral} (see Theorem \ref{thm:param}).

\medskip

The only results known on this family of barriers can be found in \cite{Bressan_friends} and \cite{firefighter}. In the two papers it is proved independently and with different techniques the following result:

\begin{theorem}
\label{bressan,klein}
Let $\sigma > 2.6144..$ (critical speed). Then there exists a spiral-like strategy which confines the fire.
\end{theorem}

The proof of this result is obtained by the study of a particular spiral, that we will call \emph{saturated spiral}. Let $Z$ be an admissible spiral. We say that $Z=Z_{\text{sat}}$ is a saturated spiral if
\begin{equation}
\label{eq:sat:spir:def}
\mathcal{S}(Z_{\text{sat}}) = \big\lbrace t \in[0,T]:\ \H^1 \big( Z_{\text{sat}} \cap \overline{R^{Z_{\text{sat}}(t)}\big) = \sigma t \big\rbrace = [0,T].
\end{equation}
In terms of the admissibility functional previously defined, every point $P\in Z$ on a saturated spiral is \emph{saturated}, that is $\mathcal{A}(P)=0$.

Saturated spirals (or {\color{red} closed and connected subsets of saturated spirals}) are thought to be building blocks for optimal strategies. Indeed, it has been proved in \cite{Bressan_isotropic} that, if $\sigma>2$, the optimal strategy (that minimizes the cost functional \eqref{eq:opt:problem}) among simple closed curves is {\color{red} the union of} an arc of circle and two branches of saturated logarithmic spirals in polar coordinates. As we will see, there are intimate relations between logarithmic spirals and saturated spirals. Also, in \cite{FireSegment}, it is proved that for $\sigma<2$, if a strategy $Z$ is optimal ($\kappa_1=0,\kappa_2=1$) and its internal barrier is a segment, then the boundary $\partial R^Z_\infty$ is the union of a segment and a branch of logarithmic spiral.

The proof of Theorem \ref{bressan,klein} relies on the following fact: a saturated spiral $Z_{\text{sat}}$ can be represented by means of polar like coordinates $(\phi,r_{\text{sat}}(\phi)) \in [0,+\infty) \times \R^+$ (see Theorem \ref{Cor:angle_preprest}), and moreover $r_{\text{sat}}(\phi)$ solves the following \emph{Retarded Differential Equation (RDE)} %satisfies the following Cauchy Problem
\begin{equation}
\label{eq:ODE:saturated:1}
\frac{d}{d\phi} r_{\text{sat}}(\phi) = \cot(\alpha) r_{\text{sat}}(\phi) - \frac{r_{\text{sat}}(\phi - (2\pi+\alpha))}{\sin(\alpha)}
\end{equation}
with initial data
\begin{equation}
\label{Equa:init_satur}
r_{\text{sat}}(\phi) = \begin{cases}
e^{\cot\alpha\phi} & \forall\phi\in[0,2\pi), \\
(e^{2\pi\cot\alpha}-1) e^{\cot\alpha(\phi-2\pi)} & \forall \phi \in [2\pi,2\pi+\alpha].
\end{cases}
\end{equation}
The angle $\alpha \in [0,\frac{\pi}{2})$ is given by
\begin{equation}\label{eq:alpha}
\alpha = \arccos \left( \frac{1}{\sigma} \right),
\end{equation}
(this is precisely the approach followed by \cite{firefighter}). {\color{red} The angle $\alpha$ is the constant angle made by the fire ray with the spiral.} Here the initial fire is the set $R_0 = B_1(0)$ and the spiral starts in a point $P=(1,0)$. Observe that for $\phi<2\pi$ the solution is an arc of the logarithmic spiral in polar coordinates $r_{\text{sat}}(\phi) = e^{\cot\alpha\phi}$.

A study of the eigenvalues of the operator associated to the previous RDE gives the proof of Theorem \ref{bressan,klein}: there is a critical value ($\bar \sigma = 2.6144...$, solution ot{\color{red}f} a trascendent{\color{red}al} equation) such that if $\sigma > \bar \sigma$ then all eigenvalues of the associated linear operator are complex conjugate: in particular the solution oscillates, and thus there is some first angle $\bar \phi$ such that $r_{\text{sat}}(\bar \phi) = 0$. This corresponds exactly to the fact that $Z_{\text{sat}}$ blocks the fire.

%(see also Subsection \ref{ss:dde}). Actually, if a player constructs any admissible spiral and at some point it decides to construct a saturated spiral, that is a branch that satisfies the length constraint of Definition \ref{eq:sat:spir:def}, then for $\sigma>2.6144$ it manages to block the fire. This is the content of Proposition \ref{prop:at:crit:speed:fire:dies} and is due to the pure complex spectrum of the operator associated to \eqref{eq:ODE:saturated:1}. 


{\color{red}However,} in \cite{Bressan_friends} it is not proved that, instead, for $\sigma \leq \bar \sigma$ the saturated spiral does not confine the fire, that is $r_{\text{sat}}(\phi) > 0$ for every angle $\phi$: this fact can be deduced from \cite{firefighter}, Theorem $3$, which gives the estimate
\begin{equation*}
\text{minimal closing angle}\sim(imaginary part of the largest eigenvalue)^{-1}.
\end{equation*}
{\color{red} Their result motivates the following conjecture for general spirals.}

\begin{conjecture}
\label{conj:spiral}
If $\sigma \leq \bar \sigma$ then no spiral-like strategy {\color{red}blocks} the fire.
\end{conjecture}

We remark here that due to the constraints on the barrier, {\color{red}the} critical speed $\bar\sigma$ is larger than the critical{\color{red}io toglierei critical qui} speed $\sigma=2$ for the original conjecture \ref{conj:bressan}.

%
%
%
%
%The proof of this result is based on the following idea: we consider the following \textbf{change of variables}
%         \begin{equation}\label{eq:change:var:1}
%       \rho(t)=r((2\pi+\bar\alpha)t)e^{-\bar c(2\pi+\bar\alpha)t},\qquad  \bar c=\cot\bar\alpha-\frac{1}{2\pi+\bar\alpha}.
%   \end{equation}
%   Then the function $\rho$ satisfies the following RDE
%   \begin{equation*}
%       \dot\rho(t)=\rho(t)-\rho(t-1).
%   \end{equation*}
%   Then we prove that $\rho(2)>\rho(t)>0$ for every $t\in [1,2)$, and since $\rho:[1,+\infty)\rightarrow\mathbb R$ is continuous, then $\rho$ is \textbf{monotonically increasing} in $[2,+\infty)$. In particular $r(\phi)>0$, for every $\phi$ (this is better explained in Proposition \ref{prop:saturated:not:closed}). This is the key idea that we will use in the later proofs: in order to show that a solution to the RDE \eqref{eq:ODE:saturated:1} is strictly positive, we need to study the monotonicity of the function $\rho$. 
%
%\medskip This collection of results inspires therefore the following 


A partial answer to this conjecture has been given in \cite{firefighter} where the authors use a geometric argument to  prove the following result:

\begin{theorem}
\label{thm:klein}
If $\sigma\leq\frac{1+\sqrt{5}}{2}$ then no spiral-like strategy is admissible. 
\end{theorem}

This bound is obtained in the assumption that only some points on the spiral are admissible, while assuming the admissibility of the whole barrier requires more effort.

The aim of this paper is to prove {\color{red} the previous conjecture}: %extend Theorem \ref{thm:klein} to higher values of $\sigma$ and to provide a general framework for the study of spirals or more complicated strategies. We will prove the following

\begin{theorem}
\label{thm:main}
No admissible spiral-like strategy confines the fire if $\sigma \leq \bar \sigma$.
\end{theorem}


\medskip

We conclude this first part of the introduction by giving a very much simplified idea of our approach. We will neglect some technical issue, which will be further addresses{\color{red}d} in the section below.

\begin{figure}
\resizebox{.75\textwidth}{!}{\input{firefigure1}}
\caption{The angle-ray parametrization $(\phi,r(\phi))$ of a spiral barrier: the optimal fire ray is red, and the red curve is the level set of the minimum time function $u$. In blue, the angle-ray coordinates.}
\label{Fig:angle_spiral_intro}
\end{figure}

First, a spiral strategy admits a polar-like representation $(\phi,r(\phi){\color{red})} \in [0,+\infty) \times \R^+$ as in Fig. \ref{Fig:angle_spiral_intro} (we will call this representation the \emph{angle-ray coordinates}):
\begin{itemize}
\item $r$ is the length of the segment starting from one point of $\zeta$ and with direction $\dot \zeta$ and ending in the next round of $\zeta$,{\color{red};}
\item $\phi$ is the rotation angle of $r$,{\color{red};}
\item $\beta(\phi)$ is the angle between $\dot \zeta$ and the direction of $r(\phi)$.
\end{itemize}
We can also think {\color{red}of} $r(\phi)$ as the last part of the optimal ray used by the time function $u$ {\color{red}better:needed to compute the minimum time function $u$} in the point $\zeta(\phi)$, where we used $\phi$ as parametrization instead of $s$.

The parameter $\beta(\phi)$ is our control parameter: once it is chosen, the RDE satisfied by $r(\phi)$ is
\begin{equation*}
\frac{d}{d\phi} r(\phi) = \cot(\beta(\phi)) r(\phi) - \frac{r(\phi^-)}{\sin(\beta(\phi^-){\color{red})}},
\end{equation*}
where the angle $\phi^-$ is given by (see Fig. \ref{Fig:angle_spiral_intro})
\begin{equation*}
\phi = \phi^- + 2\pi + \beta(\phi^-).
\end{equation*}
Using this representation, and {\color{red}observing} that $r(\bar \phi) = 0$ means that the spiral closes into itself and thus blocks the fire, we replace the closure problem with the following minimum problem:
\begin{equation}
\label{Equa:minimum_rphi_intro}
\text{{\bf Optimization Problem}: given a rotation angle $\bar \phi$, choose $\phi \mapsto \beta(\phi)$ in order to minimize $r(\bar \phi)$.}
\end{equation}
Differently from the original problem (where we have to show that the set {\color{red} of admissible strategies} is empty), we prove that the one above has an optimal solution.

We observe that while the RDE for $r$ is linear, the choice of the control parameter affects the RDE by changing the coefficients at the next round and also by varying the delay interval $2\pi + \beta(\phi^-)$: hence it seems quite difficult to find a positive lower bound for the optimization problem \eqref{Equa:minimum_rphi_intro}, or even more to prove that a choice of the control $\beta(\phi)$ is optimal. Notice also that $\beta$ depends on the angle $\bar \phi$, i.e. the optimal spiral is not the same for all angles (and in particular {\color{red} we will prove it} is not the saturated spiral).

In order to overcome these difficulties, we use a homotopy approach as follows. {\color{red} We will refer to Figure \ref{Fig:fire:intro:2}.}

\begin{figure}
\resizebox{.75\textwidth}{!}{\input{FireIntro2.png}}
\caption{The barrier $\zeta([0,\phi_0])$ is fixed. Given any angle $\phi\geq \phi_0$, we construct a new spiral $\check\zeta(\phi;\bar\zeta([0,\phi_0])$ (blue). The family of continuations of $\bar\zeta$ (black spiral) is represented in blue. The base spiral (green) is $\check\zeta(\phi;\bar\zeta(\lbrace 0\rbrace))$.}
\label{Fig:fire:intro:2}
\end{figure}


 Let $\bar \zeta(\phi)$ be a given spiral strategy, parametrized by the rotation angle: for every $\phi_0$, we construct a new spiral $\check\zeta(\phi;\bar \zeta([0,\phi_0]))$ with the following properties:
\begin{enumerate}
\item $\check\zeta(\phi;\bar \zeta([0,\phi_0])) = \bar \zeta(\phi)$ for all $\phi \in [0,\phi_0]$;
\item \label{Point:hat_spiral_2_intro} if $\check r(\phi;\bar \zeta([0,\phi_0]))$ is the representation of the spiral in the {\color{red}angle-ray} coordinates, the final value $\phi_0 \mapsto \check r(\bar \phi;\bar \zeta([0,\phi_0]))$ is differentiable and has positive derivative;
\item \label{Point:hat_spiral_3_intro} the spiral $\check \zeta (\phi)= \check \zeta(\phi;\bar \zeta(\{0\}))$ is such that $\check r(\bar \phi) > 0$.
\end{enumerate}
Since the spiral $\bar \zeta$ is fixed during the homotopy argument, we shorten the notation to $\check r(\cdot,\phi_0)$ or also $\check r(\cdot;s_0)$ when using the length parametrization for $\bar \zeta$. 

The existence of such a family for every spiral $\bar\zeta$ gives thus the expanded version of the main Theorem \ref{thm:main} (which now becomes a corollary):

\begin{theorem}
\label{Theo:main_extended}
For each spiral strategy $\bar \zeta$ and rotation angle $\bar \phi$, the spiral $\check \zeta(\cdot;\phi_0)$ is the optimal solution to the minimization problem \eqref{Equa:minimum_rphi_intro} given the initial spiral arc $\bar \zeta([0,\phi_0])$. In particular, $\check \zeta(\phi;0)$ is optimal among all spirals.
\end{theorem}

{\color{red} Given the optimality of $\check \zeta(\phi;0)$, we will refer to this spiral as $Z_{\text{opt}}=(\phi,\zeta_{\text{opt}})$.
Point \eqref{Point:hat_spiral_3_intro} {\color{red} and point \eqref{Point:hat_spiral_2_intro}}above implies that
\begin{equation*}
0 < \check r(\bar \phi;0) \leq \check r(\bar \phi;s_0) + \int_0^{\phi_0} \frac{d}{d\phi_0 {\color{red}\phi}} \check r(\bar \phi;\phi_0) d\phi_0 {\color{red}\phi}= \check r(\bar \phi;\phi_0) \leq \bar r(\bar \phi),
\end{equation*}
{\color{red}
\begin{equation*}
\check r(\bar\phi;s_0)=\check r(\bar\phi;0)+\int_0^{\phi_0} \frac{d}{d\phi} \check r(\bar \phi;\phi_0) d\phi \geq \check r(\bar\phi;0)
\end{equation*} but since this holds for every $s_0$, the previous equation is also valid for the last parameter $\bar s$, so that $\bar r(\bar\phi)\geq\check r(\bar\phi;0),
}
where we used $(\phi,\bar r(\phi))$ as the angle-ray coordinated of the fixed spiral $\bar Z$. In particular Theorem \ref{thm:main} holds.

We will also prove that the only case when the derivative $\frac{d}{d\phi_0} \check r(\bar \phi;s_0)$ is $0$ is by following exactly the spiral $\check r(\cdot;\phi_0)$, so that the above chain of inequalities become strict as soon as we perturb the spiral $Z_{\text{opt}}$. Hence we have the following

\begin{corollary}
\label{Cor:uniqueness}
The optimal spiral strategy for the angle $\bar \phi$ is $Z_{\text{opt}}$, parametrized by $\check r(\phi;0) = \check r(\phi)$.
\end{corollary}

We remark that by changing the angle $\bar \phi$, the optimal spiral changes. {\color{red} Therefore we will often refer to the optimal spiral at a fixed angle $\bar\phi$). We also remark that the optimal spiral is not regular, but only Lipschitz at the last round. This can be heuristically explained by observing that the last round is not having influence on the next evolution (being the last one!), so that the regularizing effect of the RDE is not acting.

Being able to describe the optimal spiral, it is possible to give estimates, in particular one can prove the asymptotic divergence of the optimal spiral:

\begin{corollary}
\label{Cor:divergence}
The spiral $Z_{\text{opt}}$, optimal at the angle $\bar \phi$, satisfies
\begin{equation*}
\check r(\bar \phi) \simeq {\color{red}\bar}\phi e^{\bar c {\color{red}\bar}\phi},
\end{equation*}
where $\bar c$ is the only positive eigenvalue of the RDE.
\end{corollary}

We are also able to give a precise value to the constant in front of $\phi e^{\bar c \phi}$, as we will point out in the extended introduction below.


{\color{green} io qui fare un piccolo recap del risultato, della sua importanza e di ulteriori nuovi sviluppi. Questa e' chiaramente una bozza}

{\color{red} Summarizing, we build up a new differential tool to treat spiral-like strategies. The choice of the angle-ray coordinates for a given spiral is one of the key ideas of this paper. In particular, they solve a retarded differential equation (RDE) and they allow to set up a new optimization problem, which is solvable, differently from the one proposed in \cite{Bressan_deLellis}. Given any spiral $\bar Z$, is then possible to find a family of parametrized spirals and to use an homotopy-type approach, in order to prove that any spiral-like strategy does not confine the fire for $\sigma\leq\bar\sigma=2.6144...$. Here, the main difficulty is to guess what is the right family, and to implement the computations. This will require the detailed study of Sections $6,7,8,9,10$ -qua mettere label corretto, together with the use of the Software Mathematica for the evaluation of trascendental functions. Each single building-block leads to the proof of Bressan Fire Conjecture for spirals in its sharp form. We point out that the importance of this work is not only the proof of the conjecture in the setting of spiral-like strategies, but the implementation of a framework that could be applied in order to study more general situations, hopefully leading to the full solution of the conjecture.} {\color{green} La gente se la tira per molto meno!!!}

\medskip
{\color{red} We remind that all the notations are contained in the Glossary -ci va il label-.}
\subsection{Extended introduction and collection of all principal results}
\label{Ss:extend_more_intro}


In this section we present an extended introduction to the proof of Theorem \ref{Theo:main_extended}, and all the steps required to construct the family $\check r(\cdot;\phi_0)$. Many of the results obtained along the proof are interesting on their own, and we will report their statement.


\subsubsection{Section \ref{s:admissible:barriers}}
\label{Sss:admiss_barr_intro}


This section introduces the basic objects considered in this paper: the most important ones are the set of admissible curves \gls{Gamma}, Equation \eqref{eq:admissible:curves} (recall also \eqref{eq:burned:region_intro}), the minimum time function \gls{utimefunct}, Equation \ref{eq:solution:HJ} (recall \eqref{eq:min:time:function}), the admissibility functional \gls{Acaladmisx}, Equation \ref{eq:admiss:funct}, and the saturated set \gls{Scal}, Equation \eqref{eq:sat:set}. The limit of a minimizing sequence of admissible curves in $\Gamma$ are the \emph{optimal rays}, Definition \ref{def:optimal:ray}. These Lipschitz curves are not admissible in general, but are the ones needed to compute the value of the {\color{red} minimum} time function $u(x)$.

The first result is in Section \ref{Ss:prelimnaries}, where the existence of a closing barrier for every initial burning set $R_0$ is reduced to the study when $R_0 = \{0\}$ and the barrier is constructed outside the unit ball $B_1(0)$, Proposition \ref{Prop:limit_speed}. The equivalence is not exact as stated in the proposition, but since for $\sigma \leq \bar \sigma$ we show that it is not possible to block the fire even in this situation, we conclude that in our case the equivalence is complete.

Section \ref{Ss:spiral_barrier_intro} can be though{\color{red}t} as a thoughtful {\color{red}detailed} description of the notion of spiral barrier of Definition \ref{Def:spiral_barrier_intro}: in particular Remark \ref{Rem:comment_single_curve} explains the importance of the monotonicity of $u(\zeta(s))$. Some notation for convex barriers are also introduce{\color{red}d}, like th{\color{red}e} left and right tangent vectors \gls{t-t+} , the local radius of curvature \gls{Rcurva}, the subdifferential \gls{subdiffzeta} (Definition \ref{Def:supporting_direction}). \\
The most important result of this section is that for spiral barrier one can use the angle-ray representation as considered below Theorem \ref{thm:main}. This result is obtained in two steps. First, Proposition \ref{thm:param_1} constructs this representation round-by-round, starting with the initial round about the origin $(0,0) \in \R^2$ (where it corresponds to polar coordinates), and the{\color{red}n} recursively constructing the angle at the next round. The idea is that the directions{\color{red} senza s} of $r(\phi)$ is determined by the previous round, and then the angle $\beta(\phi)$ is deduced by knowing the tangent $\mathbf t = \dot \zeta$ at that point: a look at Fig. \ref{fig:param:spiral} is probably better than any explanation. \\
A version of Proposition \ref{thm:param_1} avoiding the explicit reference to round{\color{red}s} is Theorem \ref{Cor:angle_preprest}. Together with the function \gls{rphi}, we also introduce the functions \gls{s-phi}, \gls{s+phi}, which are the length parametrization of the starting/ending point of the segment $r(\phi)$. Their regularity properties ($s^-(\phi)$ BV, $s^+(\phi)$ Lipschitz) are also proved. We conclude this section by using the angle-ray representation to rewrite the convexity of $\zeta$ in terms of the angle \gls{beta}, the admissibility functional $\mathcal A = \mathcal A(\phi)$ and the burning rate \gls{b(t)} of the barrier $\zeta$, Proposition \ref{Lem:burnign_rate}.

As a warning, because of Theorem \ref{Cor:angle_preprest} we can use indifferently the length $s$ or the angle $\phi$ as parameter for the{\color{red}togli the} a spiral barrier: in the following we will often choose the most convenient one, without underlining it, in order to simplify notation and shorten the analysis.


\subsubsection{Section \ref{S:ODE}}
\label{Sss:ODE_intro}


The first part of the section is devoted to obtain the RDE satisfied by a spiral barrier: Lemma \ref{lem:ODE:spiral} offers some differential relations among the various quantities introduced in the angle-ray description of a spiral. Equation \eqref{eq:spiral:angle} is the distributional RDE for the spiral barrier: it is nothing else than the relation
\begin{equation*}
\big\{ \text{variation of $r$} \big\} \ = \ \big\{ \text{increase due to $\beta$ at the end point} \big\} \ - \ \big\{ \text{decrease due to curvature at the base point} \big\}.
\end{equation*}
Proposition \ref{Prop:construct_spiral} is the inverse statement: assume that $r(\phi),\beta(\phi)$ satisfies the differential relations of Lemma \ref{lem:ODE:spiral}, then, up to fixing the initial point, there is a unique spiral barrier such that its angle-ray coordinates are the given ones. The proof is based on the round decomposition.

In Section \ref{Sss:equation_satur} we prove that the equation of {\color{red}t}he saturated spiral is \eqref{eq:ODE:saturated:1} with initial data \eqref{Equa:init_satur}.

The next section contains the analysis of the linear RDE
\begin{equation}
\label{Equa:satur_spiral_intro}
\frac{d}{d\phi} r(\phi) = \cot(\alpha) r(\phi) - \frac{r(\phi - 2\pi - \alpha)}{\sin(\bar {\color{red}\text{senza bar}}\alpha)}
\end{equation}
with $\alpha$ constant. This section contains many results which have already been proved in \cite{firefighter}: we present them for completeness. The main one is that there is a critical angle $\bar \alpha$ such that for $\alpha < \bar \alpha$ the characteristic equation of the above RDE has two distinct positive real eigenvalues, for $\alpha = \bar \alpha$ the two eigenvalues coincide and the geometric multiplicity is $1$, for $\alpha > \bar \alpha$ all eigenvalues are complex conjugate, Corollary \ref{Cor:eigen_angle}. This gives in particular that for $\alpha > \bar \alpha$ the saturated spiral confines the fire, Proposition \ref{prop:at:crit:speed:fire:dies}.

Section \ref{ss:subset:saturated} is concerned with the converse result for the saturated spiral. Observe that even if there are positive real eigenvalues, if the initial data is $0$ when projected on the corresponding eigenspace then the solution oscillates and thus the fire is blocked: thus the idea is to give a condition assuring {\color{red} ensuring} the exponential blow-up of the solution and checking that the saturated spiral satisfies this condition. \\
The starting point is to rescale the variables \newglossaryentry{rhotau}{name=\ensuremath{\rho(\tau)},description={rescaled variable $\rho$ with $\phi = (2\pi + \alpha) \tau$}}
\begin{equation*}
\gls{rhotau} = r((2\pi+\bar \alpha) \tau) e^{-\bar c (2\pi + \bar \alpha) \tau},
\end{equation*}
with $\bar c$ equal to the only real eigenvalue (see Corollary \ref{Cor:divergence}), and rewrite the RDE in the critical case as
\begin{equation}
\label{Equa:retarde_intro}
\dot \rho(\tau) = \rho(\tau) - \rho(\tau-1).
\end{equation}
{\color{red} We remark that in this parametrization the parameter $\tau$ represents the number of rounds of the spiral.}
Lemma \ref{lem:key} gives a simple-to-check criterion to verify if the solution diverges:

\begin{lemma}[Second part of Lemma \ref{lem:key}]
\label{lem:key_intro}
%If $\frac{a}{b} > e$ and $\rho(1) \geq \rho(\tau) > 0$ for every $\tau \in [0,1]$, then $\rho(\tau)$ diverges exponentially. 
%
{\color{red}In the critical case $\sigma=\bar\sigma$ if} $\rho(1) > \rho(\tau) > 0$, $\tau \in [0,1)$, then the solution $\rho(\tau)$ diverges linearly.
%
%If $0 < \frac{a}{b} < e$, the solution $\rho(\tau)$ oscillates.
\end{lemma} %if $\rho$ is increasing in $[0,1]$ then it remains increasing.

Even if it seems trivial, it gives immediately that the saturated spiral is diverging:

\begin{proposition}[Proposition \ref{prop:saturated:not:closed_1}]
\label{prop:not_closed_intro}
Let $Z_{\text{sat}}$ be the saturated spiral. Then it does not confine the fire for $\sigma\leq \bar \sigma$. 
\end{proposition}

The optimal solution $\check r(\cdot;\phi_0)$ and its derivatives have a more complicated structure than the saturated spiral: hence Section \ref{Sss:green_kernels} introduces the Green kernel \gls{gkernel} for the RDE \eqref{Equa:retarde_intro} (Lemma \ref{Lem:explic_kernel_RDE}), and {\color{red} there it is studied} its asymptotic behavior (Lemma \ref{Lem:aympt_g}). It is essentially standard analysis for a linear functional equation, and for completeness we write also the explicit forms of the kernel \gls{Gkernel} for the RDE of the saturated spiral \eqref{Equa:satur_spiral_intro}.

Since it will be useful to study also the evolution of the length of a spiral barrier, this section ends with some useful estimates for the primitives of $G(\phi)$ (Section \ref{Sss:length_saturated}).


\subsubsection{Section \ref{S:exist_opti_traj}}
\label{Sss:exists_opti_intro}


In this section we prove that the optimization problem \eqref{Equa:minimum_rphi_intro} has a solution in the domain of admissible spiral barriers with bounded length $\bar L$, Theorem \ref{Theo:exists_min}:

\begin{theorem}[Theorem \ref{Theo:exists_min}]
\label{Theo:exists_min_intro}
Fix a rotation angle ${\bar \phi} \geq {\phi_0}$. Then either there exists an admissible spiral in $\mathcal A_S(\bar Z,{\phi_0})$ with $\bar L \gg 1$ blocking the fire before or at ${\bar \phi}$ or there exists an admissible spiral $\zeta$ such that $r({\bar \phi})$ is minimal among all admissible spirals of length bounded by $\bar L$.
\end{theorem}

{\color{red} Here $\mathcal{A}_S(\bar Z,\phi_0)$ is the set of admissible continuations (Definition \ref{Def:continuations}), that is the set of admissible spirals that coincide with a given spiral $\bar Z$ up to the rotation angle $\phi_0$.}
Note that in the above statement we consider the more general case where a first arc of $r(\phi)$, $\phi \leq \phi_0$, is fixed, and we are allowed to choose the remaining part. This is perfectly in line with the statement of Theorem \ref{Theo:main_extended}, where the optimality is proved given the initial arc $\bar \zeta([0,\phi_0])$.

A solution means that either there is an admissible spiral blocking the fire before the angle $\bar \phi$, or there is a minimizing one, and the length ${\color{red}\bar} L$ is chosen sufficiently large {\color{red} togli in order} in order to have at least a spiral arriving at the angle $\bar \phi$ {\color{red} with length shorter than $\bar L$} {\color{blue} or rephrased $\bar L$ is sufficiently large to guarantee that the set of admissible spirals arriving at $\bar\theta$ with length shorter than $\bar L$ is not empty}. The approach is the standard one: first one proves the compactness of the set of admissible spirals, Proposition \ref{Prop:compact_curves} and Corollary \ref{Cor:convergs}, and then passes to the limit to a minimizing sequence, being the functional $\zeta \mapsto r(\bar \phi)$ continuous. We just remark that as a corollary we have that the admissibility functional is u.s.c. for {\color{red} the} Hasdorff convergence, hence giving the closure of the family of admissible spirals, and also observe that a key ingredient is the decomposition by rounds of Proposition \ref{thm:param_1}. \\
The parameter ${\color{red}\bar} L$ will not play any role in the future: indeed once we show that the spiral $\check r$ is optimal, we have an estimate for all spirals. It is {\color{red} introduced} just to assures {\color{Red}ensure} that the curves $\zeta$ lives {\color{red} senza s} in a compact set of $\R^2$.

When studying the derivative $\frac{d}{ds_0} \check r(\cdot;s_0)$ of $\check r(\phi;s_0)$ (see the discussion at the end of Section \ref{Sss:admiss_barr_intro} for the equivalence of $\phi$ and $s$), it is important to know the structure of the minimal time function $u$ generated by $\bar \zeta([0,s_0])$. Lemma \ref{Lem:convexity} and Corollary \ref{lem:C:1:1} give explicit computations of the first and second derivatives of $u$: roughly speaking, we are solving the Eikonal equation, because of the assumptions on the fire spreading speed $F(x) ={\color{red}\bar} B_1(0)$, and thus $\nabla u$ is BV and the level sets of $u$ are $C^{1,1}$-curves.

\begin{figure}
\resizebox{.75\textwidth}{!}{\input{spiral_first_round_intro.pdf_t}}
\caption{The solution to the optimization problem at the last round. The gray region is the region which cannot be reached by any admissible spiral.}
\label{Fig:optimal_last_intro}
\end{figure}

The first glimpse on the structure of the optimal solution $\check r$ is given in Section \ref{Ss:minimal_reach}: if we restrict the optimality to just one round after $\phi_0$, then $\check r$ can be explicitly constructed without further analysis. \\
To describe the structure of such a solution, we refer to Fig. \ref{Fig:optimal_last_intro}. Starting from the angle $\phi_0$, the solution is made by three components. {\color{red} In the following, we will mean by \emph{arc of the level set}, or simply \emph{arc}$, a compact and connected subset of $\lbrace u^{-1}(t)\rbrace$.}
\begin{enumerate}
\item We follow the level set of the minimal time function $u$ until the point $\zeta(\phi_1)$, which is saturated. At this point it is not possible to proceed along this level set, because the spiral would not be admissible. This arc (the magenta one between the points $\zeta(\phi_0)$ and $\zeta(\phi_1)$ in the picture) is the optimal solution for angles $\bar \phi \in [\phi_0,\phi_1]$, since the monotonicity of $s \mapsto u(\zeta(s))$ gives that we cannot cross the level set of $u(\zeta(\phi_0))$. In the case $\zeta(\bar \phi_0)$ is saturated, then this regions reduces to a point.

The optimal spiral barrier coincides {\color{red} here} with the are{\color{red}c} of {\color{red} the} level set.

\item If $\bar \phi > \phi_1$, then we consider the spirals made by a portion of the magenta arc and a segment: the segment ends in the first point it{\color{red} that} is saturated. We show that such a construction defines a convex curve (the blue one in Fig. \ref{Fig:optimal_last_intro}) starting orthogonally to the level set of $u$ and ending in a saturated point $\zeta(\phi_2)$ such that the angle formed with the direction of the optimal ray is exactly $\bar \alpha$ {\color{red} (this argument in reality holds for any $\sigma\leq\bar\sigma$, but here we prove it for the critical case)}. Also in this case, if the initial point is saturated, it holds $\phi_2 = \phi_0$.

The optimal spiral barrier is an arc of the level set and a segment ending in the blue curve.

\item For angles $\bar \phi > \phi_2$ one follows the saturated spiral starting from $\zeta(\phi_2)$ (green spiral in the picture). The optimal spiral barrier is an arc of the level set, the segment arriving in $\zeta(\phi_2)$ and an arc of a saturated spiral.
\end{enumerate}

\begin{figure}
\resizebox{\textwidth}{!}{\input{three_cases.pdf_t}}
\caption{The three cases of Theorem \ref{Cor:curve_cal_R_sat_spiral_intro}: in the first picture all level set $\xi$ is admissible, and then for every angle $\geq {\phi_0}$ the optimal solution is an arc of the level set; in the second case all curve $\mathtt R$ is admissible, and then the optimal solutions for point on $\mathtt R$ is an arc of $\xi$ and a segment; in the third case for large angles the minimal point lies on a saturated spiral, and the optimal solution is an arc of $\xi$, a segment and an arc of saturated spiral.}
\label{Fi:three_cases_intro}
\end{figure}

It is important to observe that the curve formed by the magenta arc up to $\phi_1$, the blue convex curve and the green saturated spiral is not a spiral barrier: indeed it is not convex. It gives the optimal solution for $\phi_0 \leq \bar \phi \leq \phi_0 + 2\pi + \beta^-(\phi_0)$, where $\beta^-(\phi_0) = \lim_{\phi \nearrow \phi_0} \mathbf t(\phi)$, i.e. the left tangent vector: for every angle $\bar \phi$ there exists an explicit spiral barrier ending in the corresponding point of the curve constructed above. The three situations above are drawn in Fig. \ref{Fi:three_cases_intro}. The main result is then the following

\begin{theorem}(Theorem \ref{Cor:curve_cal_R_sat_spiral})
\label{Cor:curve_cal_R_sat_spiral_intro}
The curves constructed above are the unique solution{\color{red}s} to the minimum problem considered in Theorem \ref{Theo:main_extended} for ${\bar \phi} \in [{\phi_0},{\phi_0} + 2\pi + \beta^-({\phi_0}))$.
\end{theorem}

A question which arises naturally is the following: if we proceed {\color{red} continue} the saturated spirals {\color{red} senza s} also for angles larger that $\phi_0 + 2\pi + \beta^-(\phi_0)$, is this spiral barrier optimal? The short answer is no, but the proof of this fact and the construction of the correct optimal spiral requires much more analysis and it is the central part of this work. Due to its importance, we will refer the spiral constructed by the procedure above and {\color{red} obtained by} prolonging the saturated spiral after the angle $\phi_ 0 + 2\pi + \beta^-(\phi_0)$ as the \emph{fastest saturated spiral}.


\subsubsection{Section \ref{S:case:study}}
\label{Sss:case_study_intro}


The construction above when $\phi_0 = 0$ is a particular spiral which is important for the next analysis, since the optimal one will be obtained as a perturbation of this spiral: the study of its properties is in Section \ref{S:case:study}. For the seek of generality, we consider the case where $R_0 = B_{\mathtt a}(0)$, and show explicitly the form of the fastest saturated spiral: depending on the radius $\mathtt a$, it is either a an arc + segment + saturated spiral (if $\mathtt a \in (0,\sin(\bar \alpha))$), a segment + saturated spiral (if $\mathtt a \in [\sin(\bar \alpha),1)$) or just the saturated spiral when $\mathtt a = 1$. We will use the denomination
\begin{description}
\item[Arc case] the fastest saturated spiral starts with a non-trivial arc of the level set, i.e. this arc is not just a point;
\item[Segment case] The fastest saturated spiral starts with a segment, possibly made of just a point, i.e. the initial point is saturated and the spiral coincides with the saturated one.
\end{description}
These various cases will be also encountered when considering as a starting point the spiral arc $\zeta([0,s_0])$, so that they are worth studying in this setting where the functions are explicit.

The study of the behavior of this spiral gives the following

\begin{theorem}[Theorem \ref{thm:case:a}]
\label{thm:case:a_intro}
For any value of $\mathtt a \in (0,1]$, the fastest saturated spiral $S_{\mathtt a}$ with initial burning region $B_\mathtt a(0)$ does not confine the fire: more precisely, the spiral diverges exponentially as $r(\phi) \sim \phi e^{\bar c \phi}$,
%$$
%r(\phi) \sim 2 \phi e^{\bar c \phi} \begin{cases}
%\frac{e^{-\bar c(\Delta \phi_{\mathtt a} + \frac{\pi}{2} - \bar \alpha)}}{\sin(\bar \alpha)} - e^{-\bar c(2\pi)} - \frac{e^{-\bar c(2\pi + \frac{\pi}{2})} - e^{- \bar c (2\pi + \frac{\pi}{2} + \Delta \phi_\mathtt a)}}{\bar c} - \cot(\bar \alpha) e^{-\bar c(2\pi + \frac{\pi}{2} + \Delta \phi_\mathtt a)} & 0 \leq \mathtt a < \sin(\bar \alpha), \\
%\frac{\sin(\theta_\mathtt a + \bar \alpha) e^{-\bar c \theta_\mathtt a}}{\sin(\bar \alpha)} - e^{-\bar c(2\pi)} - \frac{\sin(\theta_\mathtt a) e^{-\bar c(2\pi + \theta_\mathtt a + \bar \alpha)}}{\sin(\bar \alpha)} & \sin(\bar \alpha) \leq \mathtt a \leq 1,
%\end{cases}
%$$
being $\bar c = \ln(\frac{2\pi+\bar \alpha}{\sin(\bar \alpha)})$ the only real eigenvalue for the characteristic equation of the RDE for saturated spirals.
\end{theorem}

The proof is also interesting, because it is the prototype of the line of proof of many of the subsequence {\color{red}subsequent} statement{\color{red}s}. The explicit form of the spiral barrier in the angle-ray coordinates can be given explicitly using the kernel \gls{Gkernel}: in the segment case, where the explicit forms are simpler, the solution takes the form (see Equation \ref{Equa:expl_sol_sat})
\begin{equation*}
r(\phi) = \frac{\sin(\bar \theta_{\mathtt a})}{\sin(\bar \alpha)} G \big( \phi - \bar \phi_0(\mathtt a) \big) - G(\phi - 2\pi) - \frac{\sin(\bar \theta_{\mathtt a} - \bar \alpha)}{\sin(\bar \alpha)} G \big( \phi - \bar \phi_0(\mathtt a) - 2\pi - \bar \alpha \big),
\end{equation*}
with
\begin{equation*}
\bar \phi_0 = \bar \theta_{\mathtt a} - \bar \alpha, \quad \bar \theta_a = \arccos(\mathtt a) + \bar \alpha.
\end{equation*}
By studying the derivative w.r.t. $\mathtt a$ (Step 2 of the proof of Theorem \ref{thm:case:a}, pag. \pageref{Page:step_2_case_study_segment}), one proves that $r(\phi) = r(\phi,\mathtt a)$ is monotonically increasing w.r.t. $\mathtt a$ increases, and then that the worst case happens for $\mathtt a = \sin(\bar \alpha)$, which means $\bar \theta_a = \frac{\pi}{2}$, $\bar \phi_0 = \frac{\pi}{2} - \bar \alpha$. Then one plots numerically the rescaled function
$$
\rho(\tau) = r(\bar \phi_0 + (2\pi + \bar \alpha) \tau) e^{-\bar c (2\pi + \bar \alpha) \tau}
$$
which is explicitly given by
\begin{equation}
\label{Equa:base_sol_intro}
\rho(\tau) = \frac{1}{\sin(\bar \alpha)} g(\tau) - e^{-\bar c(2\pi + \bar \alpha - \frac{\pi}{2})} g \bigg( \tau - \frac{\frac{\pi}{2}}{2\pi + \bar \alpha} \bigg) - \cot(\bar \alpha) e^{-\bar c (2\pi + \bar \alpha)} g(\tau - 1).
\end{equation}

\begin{figure}
\resizebox{.75\textwidth}{!}{\includegraphics{base_sol_intro.png}}
\caption{Plot of the first 5 rounds of the function \eqref{Equa:base_sol_intro}.}
\label{Fig:base_sol_intro}
\end{figure}

A numerical plot of the function above is in Fig. \ref{Fig:base_sol_intro}: one observes that the function is positive, and its derivative can be numerically computed to be strictly positive for $\tau \in [4,5]$ (which corresponds to the fifth round {\color{red}of the spiral}). Then one can apply Lemma \ref{lem:key_intro} to deduce that $r(\phi)$ is positive, and actually exponentially increasing as $\phi \to \infty$. The asymptotic behavior is a consequence of the asymptotic expansion of the kernel $G(\tau)$ as $\tau \to \infty$.

The last result is{\color{red}in} this section is a{\color{red}n} estimate on the ratio between $r(\phi)$ and the length $L(\phi)$ of the spiral:

\begin{proposition}[Proposition \ref{Prop:length_compar}]
\label{Prop:length_compar_intro}
It holds for $\phi \geq \tan(\bar \alpha) + \frac{\pi}{2} - \bar \alpha$
\begin{equation*}
r(\phi) - 2.08 L(\phi - 2\pi - \bar \alpha) \geq 0.67 e^{\bar c(\phi - \tan(\bar \alpha) - \frac{\pi}{2} + \bar \alpha)}.
\end{equation*}
\end{proposition}

Besides having an interest on its own, this estimate is fundamental to show that the optimal spiral $\check r(\phi;\phi_0)$ may have an arc only for angles $\phi$ close to $\phi_0$: this m{\color{red}e}ans that there is a regularizing effect in the evolution of $\check r$, because it can be proved that one can choose the control parameter $\beta$ in order to have an arbitrarily number of arcs at arbitrarily large angles, see Remark \ref{Rem:inital_tent}. The constant $2.08$ is almost optimal, see Remark \ref{Rem:asymtp_consta_for_comp}.


\subsubsection{Section \ref{S:family}}
\label{Sss:family_intro}


This section is the core of the paper: we construct a differentiable path from the fastest saturated spiral of Section \ref{S:case:study} (Section \ref{Sss:case_study_intro}) to any admissible spiral. The construction is based on the results of Theorem \ref{Cor:curve_cal_R_sat_spiral_intro} which gives an explicit construction for the first round starting from $\zeta([0,s_0])$, and this construction is then extended to every angle by prolonging as a saturated spiral. We denote this barrier as $\tilde r(\phi) = \tilde r(\phi;s_0)$.

As we said the fastest saturated spiral $\tilde r$ is not the optimal spiral after the first round starting in $\phi_0$, and indeed the derivative w.r.t. $s_0$ will be a function with some negative regions. There re however two main advantages in studying this one-parameter family of spirals.
\begin{enumerate}
\item There are only two main cases to be considered (for the optimal case we need to work on about 20 cases): we can start with a segment or with an arc+segment. It is actually possible to reduce the analysis of the derivative $\delta \tilde r = \frac{d\tilde r}{ds_0}$ to a single case (the segment is the arc when the latter reduces to a single point, Remark \ref{Rem:same_as_segment}, yielding as a consequence that the family is actually $C^1$ in a suitable topology), but since the segment case is much easier we prefer to keep it. In Fig. \ref{Fig:segment_intro_1} the geometric situation to compute the derivative $\delta \tilde r(\phi;s_0)$ is represented.

\item The optimal solution $\check r$ will be a perturbation of the spiral $\tilde r$: this perturbation will be added to the solution computed in this section, and it will be shown that the analysis is fundamentally different only in the first round, more precisely in the regions where the derivative $\delta \tilde r$ is negative. In the other region{\color{red}s} a simple adaptation of the estimates obtained in this section is sufficient to prove the positivity of the derivative $\delta \check r = \frac{d\check r}{ds_0}$.
\end{enumerate}

The main results of this section are:
\begin{itemize}
\item Propositions \ref{Prop:equa_delta_tilde_r_segm} and \ref{Prop:equa_delta_tilde_r_arc}, which compute the RDE satisfied be the derivative $\delta \tilde r(\phi)$: for example, in the segment case this derivative satisfies

\begin{proposition}(Proposition \ref{Prop:equa_delta_tilde_r_segm})
\label{Prop:equa_delta_tilde_r_segm_intro}
For $\phi > \phi_0 + \bar \theta - \bar \alpha$, the derivative 
$$
\delta \tilde r(\phi;s_0) = \lim_{\delta s_0 \searrow 0} \frac{\tilde r(\phi;s_0 + \delta s_0) - \tilde r(\phi;s_0)}{\delta s_0}
$$
satisfies the RDE on $\R$
\begin{equation*}
\frac{d}{d\phi} \delta \tilde r(\phi;s_0) = \cot(\bar \alpha) \delta \tilde r(\phi;s_0) - \frac{\delta \tilde r(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} + S(\phi;s_0),
\end{equation*}
with source
\begin{align*}
S(\phi;s_0) &= \cot(\bar \alpha) \frac{1 - \cos(\theta)}{\sin(\bar \alpha)} \Diracd_{\phi_0 + \bar \theta - \bar \alpha} - \Diracd_{\phi_0 + 2\pi + \theta_0} \\
& \quad + \frac{\cos(\theta) - \cos(\bar \alpha)^2}{\sin(\bar \alpha)^2} \Diracd_{\phi_0 + 2\pi + \bar \theta} + \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} \Diracd'_{\phi_0 + 2\pi + \bar \theta},
\end{align*}
where $\Diracd_0$ is the Dirac-delta measure in $0$, and $\Diracd_0'$ its distributional derivative.
\end{proposition}
The angle $\theta$ is the angle formed by the tangent to the spiral $\zeta$ and the initial segment of $\tilde r$ at the angle $\phi_0$. Note the similarity with the fastest saturated spiral studied in the previous section.

\item Corollaries \ref{Cor:evolv_r_after_phi_2} and \ref{Cor:evolv_r_after_phi_2:arc}, which gives the explicit solution in terms of the kernel $G$;

\item Propositions \ref{Prop:regions_pos_neg_segm} and \ref{Prop:neg_region}, where the positivity properties and asymptotic behavior of $\delta \tilde r$ is analyzed. We present here the segment case, where we use the change of variable $\phi = \phi_0 + \bar \theta - \bar \alpha + (2\pi + \bar \alpha) \tau$, $\bar \theta$ being the angle of the ray $r(\phi_0)$ and the initial segment starting at $\zeta(\phi_0)$: using the rescaled function
\begin{equation*}
\rho(\tau) = \delta \tilde r \big( \phi_0 + \bar \theta - \bar \alpha + (2\pi + \bar \alpha) \tau \big) e^{-\bar c (2 \pi + \bar \alpha) \tau}
\end{equation*}

\begin{proposition}(Proposition \ref{Prop:regions_pos_neg_segm})
\label{Prop:regions_pos_neg_segm_intro}
The function $\rho(\tau) = \rho(\tau,\theta)$ is strictly positive outside the region
\begin{equation}
\label{Equa:neg_segmnt_666_intro}
\gls{Nsegm} := \bigg\{ 1 - \frac{\theta}{2\pi + \bar \alpha} \leq \tau \leq 1, 0 \leq \theta \leq \check \theta \bigg\} \cup \big\{ \theta = 0 \} \cup \{ \tau = 1, \theta \in [2\bar \alpha,\pi] \big\} \subset \R \times [0,\pi],
\end{equation}
where the angle \gls{thetahat} is determined by the unique solution to
\begin{equation}
\label{Equa:hat_theta_det_666_intro}
\cot(\bar \alpha) \frac{1 - \cos(\check \theta)}{\sin(\bar \alpha)} -  e^{- \cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} = 0, \qquad \hat \theta \in [0,\pi].
\end{equation}
Moreover, as $\tau \to \infty$, the function $\rho(\tau)$ diverges like
\begin{equation*}
\lim_{\tau \to \infty} \frac{\rho(\tau) e^{-\bar c \tau}}{\tau} = 2 (S_0 + S_1 + S_2 + S_3), \quad 2 (S_0 + S_1 + S_2 + S_3) \in \theta^2 (0.08,028).
\end{equation*}
\end{proposition}

The arc case is more complicated, we refer the reader to Proposition \ref{Prop:neg_region}. In Fig. \ref{Fig:segment_intro_2} we plot numerically the solution of Proposition \ref{Prop:equa_delta_tilde_r_segm_intro} with $\theta = .3$ for the first 3 rounds. Observe that there is a negative region $\tau \in [1 - \frac{{\color{red}\check}\theta}{2\pi + \bar \alpha},1]$ in the first rounds{\color{red}round}, then the solution become{\color{red}s} positive. Note that the derivative is not smooth, and this force{\color{red}s} us to study numerically the first 5 rounds in order to apply Lemma \ref{lem:key_intro}.
\end{itemize}

\begin{figure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{segment_intro.pdf_t}}
\caption{Geometric structure of the spiral $\tilde r$ and its perturbation.}
\label{Fig:segment_intro_1} \hfill
\end{subfigure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\includegraphics{rhosegm_intro_first3.png}}
\caption{Numerical plot of the function $\rho(\tau)$ for the first 3 rounds.{\color{red} Observe the negativity region for $\tau\in N_{\text{segm}}$.}
\label{Fig:segment_intro_2}
\caption{The segment case of Section \ref{Sss:family_intro}}
\label{Fig:segment_intro}
\end{subfigure}\end{figure}

The fact that there is a negative region at about the end of the first round for some angles $\theta$ means in particular that the {\color{red} fastest} saturated spiral is \emph{not optimal}: indeed, at the angle $\bar \phi - 2\pi - \bar \alpha$ by moving the barrier $\zeta$ along the direction $\bar \phi$ instead of following the spiral one obtains that $r(\bar \phi)$ is decreasing (it has negative derivative by Proposition \ref{Prop:regions_pos_neg_segm_intro}. However, since this negative region is for a relatively short interval of angles, the correction to the fastest saturated spiral $\tilde r$ will be localized only at the last round. Thus we have another argument to affirm that the fastest saturated spiral is in some sense the building block for the optimal spiral $\check r$.

For the proof of the above propositions, the approach is similar to the one used for Theorem \ref{thm:case:a_intro}: the only difference is that since the structure of the derivative is more complicate, we split the first rounds into pieces in order to avoid discontinuities. After $3$ rounds the regularizing effect of the RDE has smoothen the solution, so that we can prove the monotonicity of the solution. Numerically, we plot the function
\begin{equation*}
\frac{\delta \tilde r(\phi)}{\theta (\theta + \Delta \phi)}, \quad \Delta \phi \ \text{being the opening of the initial arc and $\theta$ as above}, 
\end{equation*}
and observe the uniform positivity or monotonicity. As observed before, we require the computer only computations on explicit functions (polynomials, exponential, trigonometric functions and their combinations), we never ask to solve a differential equation. {\color{red} We have used the Software Mathematica for the explicit evaluation of functions.}


The fact that the negativity region is limited to the first round gives that we can extended{\color{red} extend} the length estimate of Proposition \ref{Prop:length_compar_intro} to a general spiral:

\begin{proposition}(Corollary \ref{Cor:bound_length_gen})
\label{Cor:bound_length_gen_intro}
Consider the spiral $\tilde r(\phi;\phi_0)$: if
$$
\phi \geq \begin{cases}
\phi_0 + \bar \theta + 2\pi & \text{segment case}, \\
\phi_0 + \Delta \phi + \frac{\pi}{2} + 2\pi & \text{arc case},
\end{cases}
$$
then
\begin{equation*}
\tilde r(\phi) - 2.08 \tilde L(\phi - 2\pi - \bar \alpha) \geq r(\phi) - 2.08 L(\phi - 2\pi - \bar \alpha) > 0.67 e^{\bar c (\phi - \tan(\bar \alpha) - \frac{\pi}{2} + \bar \alpha)},
\end{equation*}
\end{proposition}

This is a regularity result: after one round the spirals $\tilde r$ starts to be similar to the fastest saturated spiral of the previous section. It will be used to simplify the expression of the optimal spiral $\check r(\cdot;s_0)$.


\subsubsection{Section \ref{S:optimal_solut}}
\label{Sss:optimal_solut_intro}


In this section we construct the optimal solution candidate $\check r(\cdot;s_0)$, when the spiral $\zeta([0,s_0])$ is fixed.{\color{red} We recall that we are given an angle $\bar\phi$ and we ask if, by changing the spiral at an angle $\phi_0$, corresponding to the point $\zeta(s_0)$, the ray $r(\bar\phi)$ becomes smaller (see the optimization problem \eqref{Equa:minimum_rphi_intro}). In order to avoid additional technicalities, we explain here the construction in the simple case $\zeta([0,s_0])$ is the saturated spiral, i.e. $\mathcal{A}(\zeta(\phi))=0$ and $\beta(\phi)=\bar\alpha$ for every $\phi\in[0,\phi_0]$. We will refer to Figure \ref{Fig:optimal_intro}. By the computations of the previous section, in the case of the family of fastest saturated spirals, we proved that there is a negativity region for the derivative $\delta\tilde r(\cdot;s_0)$. We also proved that this region is included in the first round (see Proposition \ref{Prop:regions_pos_neg_segm_intro} and Figure \ref{Fig:segm_intro}).} 

\medskip
Observe that
\begin{itemize}
\item {\color{red}If $\phi_0 + 2\pi + \bar \alpha < \bar \phi$, corresponding to the parameter $\tau>1$ of the previous parametrization. We are therefore outside the negativity region $N_\mathrm{segm}$ and Proposition \ref{Prop:regions_pos_neg_segm_intro} yields that any perturbation to $\zeta$ at $\phi_0$ has a positive derivative, and then the ray $r$ increases.}
\item {\color{red} If $\phi_0+2\pi+\bar\alpha=\bar\phi$, corresponding to the case of Figure \ref{Fig:optimal_intro}, then we are entering the negativity region: indeed $\tau = 1$ is the boundary of the $N_\mathrm{segm}$ for $\theta = 0$: this last condition on the angle $\theta$ means that at the angle $\phi_0$ the perturbation is tangent to the saturated spiral. Therefore, if we continue our spiral along the segment tangent to the saturated spiral at $P_0$, it follows from the computations of Section \ref{S:family} that $\theta$ is increasing ($\theta$ is the angle made by the perturbation and the segment), and then it is convenient to construct this segment up to the point $P_1$ where $\theta = \hat \theta$ (the angle constructed in Proposition \ref{Prop:regions_pos_neg_segm_intro}), i.e. we are exiting the negativity region}. {\color{red} Heuristically, the idea is clear. In order to minimize the quantity $r(\bar\phi)$ according to the optimization problem, we need to put the barrier precisely along the angle $\bar\phi$. The amount of barrier we can put is dictated by the negativity region we found from the former computations.}

From this point onward we can apply Theorem \ref{Cor:curve_cal_R_sat_spiral_intro} to specify the remaining part of the last round: it is the fastest saturated spiral starting from the point $P_1$ such that the segment originating in $P_1$ form the critical angle $\hat \theta$ with the direction $\bar \phi$.
\end{itemize}






\begin{figure}
\resizebox{.75\textwidth}{!}{\input{optimal_intro.pdf_t}}
\caption{The construction of the optimal solution for the saturated spiral.}
\label{Fig:optimal_intro}
\end{figure}


 


%
%Let $s_0 = s(\phi_0)$ be the initial point of the construction corresponding to a rotation angle $\phi_0$, i.e. the initial spiral is given for $s \in [0,s_0]$, and consider a final angle $\bar \phi$. If $\bar \phi \in \phi_0 + [0,2\pi + \beta^-(\phi_0))$, Theorem \ref{prop:best:first:Enclosure} implies that the solution $\tilde r(\phi;s_0)$ of the previous section is optimal. \\
%For $\phi \geq \phi_0 + 2\pi + \beta^-(\phi_0)$, one first follow the solution $\tilde r(\phi;s_0)$ up to an angle $\check \phi_0$ determined by $\bar \phi \in \check \phi_0 + \partial \tilde \zeta(\check \phi_0) + 2\pi$: $\tilde \zeta(s;s_0)$ is the spiral corresponding to $\tilde r(\phi;s_0)$. This angle can be either the initial angle $\phi_0$, or along the level set arc (and in this case $\bar \phi = \check \phi_0 + \frac{5}{3}\pi$) or a prolongation of the final segment $[P_1,P_2]$ ($\bar \phi = \phi_0 + \frac{\pi}{2} + \Delta \phi + 2\pi$), or in the saturated region ($\bar \phi = \check \phi_0 + 2\pi + \bar \alpha$). Let $s_1$ be the corresponding length at the angle $\check \phi_0$, $s_1 = s(\check \phi_0)$. \\
%If we repeat the construction of the previous section stating from $s_1$, and denote with $\tilde r'(\phi;s_1)$ the new fastest saturated spiral, it follows that $\tilde r'(\phi;s_1) = \tilde r(\phi;s_0)$ because both are the fastest saturated spiral. However the derivative $\delta \tilde r'$ could be negative at $\bar \phi$: indeed this happens if we are in the negativity region of the segment or the arc case. It is thus convenient for the spiral to follow a segment with direction $\bar \phi$ until the derivative $\delta \tilde r'$ becomes $0$, and at this point one closes with the fastest closing spiral. \\
%Depending on the structure of the spiral up to $s_1 = s(\check \phi)$, the segment in the direction $\bar \phi$ ends with a level set arc or with a segment: in both cases we are on the boundary of the negativity region, i.e. in the arc case the angle between the tangent to the level set and $\bar \phi$ is given by $h_1(\Delta \phi)$ (Equation \eqref{Equa:theta_Deltaphi_rel}), while in the segment case the angle between $\bar \phi$ and the segment for the fastest closing spiral is $\check \theta_0$ (Equation \eqref{Equa:hat_theta_det_666}). The various cases in the segment case are presented in Fig. \ref{fig:tent:solution}, while Fig. \ref{Fig:checkr_notation} is the most general case, and will serve as a reference for notations.
%

The first main result of this section is the definition of the optimal closing spiral $\check r(\phi;s_0)$ given the spiral arc $\zeta([0,s_0])$ and the final angle $\bar \phi$. This is the done in the first part of Section \ref{Ss:optimal_sol_def}, which contains also the proof that such a definition yields a unique spiral $\check r(\cdot;s_0)$ (Proposition \ref{Prop:unique_optimal_guess}{\color{red})}:

\begin{proposition}(Proposition \ref{Prop:unique_optimal_guess})
\label{Prop:unique_optimal_guess_intro}
Given $s_0 = s(\phi_0) \geq 0$ and an angle $\bar \phi \geq \phi_0$, there exists a unique optimal spiral candidate $\check r(\phi;s_0)$.
\end{proposition}

Such a statement is not elementary, indeed one has to rule out the possibility that when $P_1$ moves along the direction $\bar \phi$ is{\color{red}t} may enter again the negativity region. In the segment case this is easy, but in the arc case (i.e. when in the point $P_1$ the fastest saturated spiral starts with an arc) it is not, due to the more complicated structure of the negativity region \gls{Narc} for the arc perturbation.

\medskip 

The most common geometric situation for the perturbation is as in Fig. \ref{Fig:optimal_intro}: the last round starts with a segment in the direction $\bar \phi$ followed by the fastest saturated spiral starting again with a segment. We say it is the most common because the other case (i.e. the fastest saturated spiral starts with an arc in $P_1$) requires that the point $P_0$ is close to the last point of the given spiral arc $\zeta(s_0)$: roughly speaking, this is a regularity property of the fastest saturated spiral $\tilde r(\cdot;s_0)$, i.e. after less than 1 round after $s_0$ the spiral is already close to the saturated spiral. \\
We call \emph{tent} this{\color{red}these} two consecutive segments configuration. In Section \ref{Ss:comput_tent_new} we study the equations describing a spiral with a tent, obtaining the formulas which allows{\color{red}senza s} to compute how much the final tent in $\check r(\cdot;s_0)$ is going to perturb the fastest saturated spiral $\tilde r(\cdot;s_0)$ in the last round. Lemma \ref{Lem:relation_admissibility_tent} explicitly computes these formulas, and being linear relations the same formulas holds{\color{red}senza s} for the perturbation (Corollary \ref{Cor:tent_corol_for_pert}{\color{red})}. \\
Next, with these relations, we can check which condition{\color{red}s} are required in order to be not {\color{red} not to be} the admissible solution: in other words, {\color{red} when }the tent is not an admissible spiral, which in this particular case means that $s \mapsto u(\zeta(s))$ is not monotone (and then we are forced to follow an arc of the level set of $u$). It turns out that, if the the initial point $P_0$ of the tent is saturated, a necessary condition is that the length of the spiral at the previous round is much larger than the estimate of Proposition \ref{Cor:bound_length_gen_intro} (Lemma \ref{Lem:when_tent}). One thus concludes that it{\color{red}if} $P_0$ is saturated, then the optimal spiral has a tent:

\begin{proposition}(Proposition \ref{Prop:tent_admissible})
\label{Prop:tent_admissible_intro}
The tent is admissible (and then is the optimal candidate) in the saturated part of $\tilde r(\cdot;s_0)$.
%\begin{equation*}
%\tau \geq 1 - \hat \tau - \frac{\tan(\bar \alpha)}{2\pi + \bar \alpha} \ln \bigg( \frac{2.08}{\frac{e^{\cot(\bar \alpha) \hat \theta}}{K_\mathrm{tent}} - 1} \bigg) = 0.277638.
%\end{equation*}
\end{proposition}

We remark that in the non saturated part of $\tilde r(\cdot;s_0)$, i.e. when $\phi$ is close to $\phi_0$, the tent is in general not the admissible spiral solution, see the example of Remark \ref{Rem:inital_tent}.

The last result of this section is a formula based on a simple observation, Lemma \ref{Lem:final_value_satu}, which allows to prove that the derivative $\delta \check r(\bar \phi;s_0) = \frac{d}{ds_0} \check r(\bar \phi;s_0)$ is positive if $\delta \tilde r(\bar \phi;s_0) = \frac{d}{ds_0} \tilde r(\bar \phi;s_0)$ is. This formula can be applied only after 2 rounds, so that in the following we have to address what happens in these initial part of $\check r$ when $\bar \phi$ is close to $\phi_0$. One can rightly suspect that the non smoothness of $\delta \tilde r$ is the problem.


\bigskip


The last three sections address the homotopy argument starting from the optimal solution candidate and proving that the derivative $\delta \check r(\bar \phi;s_0)$ is increasing.


\subsubsection{Section \ref{S:optimal_sol_candidate}}
\label{Sss:optimal_sol_cand_intro}

\begin{figure}
\resizebox{.75\textwidth}{!}{\input{SPIRALIINTRO.png}}
\caption{In this figure, we explain the general idea of our proof and in which section the results are contained.}
\label{Fig:optimal_intro}
\end{figure}

This section is devoted to the construction of the optimal solution candidate for any given $\bar \phi$. {\color{red} The analysis carried out in this section corresponds to the one performed in Section \ref{Sss:case_study_intro} where it was proposed as a solution the fastest saturated spiral $S_a$ (Theorem \ref{thm:case:a_intro}), corresponding to the base element of the family $\tilde r(\phi;s_0)$ for $s_0=0$, or $(r(\phi),\phi)$ in angle-ray coordinates. We recall that the analysis of the positivity of $\delta \tilde r(\phi;s_0)$ was the content of Section \ref{S:family}. In Figure a summary of the results and the corresponding sections where the analysis is carried out.}  The solution \gls{roptim} will depends {\color{red}senza s} on the angle $\bar \phi$, {\color{red}therefore the analysis on the structure of $r_{\text{opt}}(\phi)$ will be more articulated than the fastest saturated spiral of Section \ref{Sss:case_study_intro}}. We refer to Fig. \ref{Fig:opt_spiral_intro} for the description of the solution $r_\mathrm{opt}$.

\begin{figure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{spiral_opt_first_intro.pdf_t}}
\caption{The optimal solution for $\bar \phi \in [0,2\pi + \frac{\pi}{2} - h_1]$.}
\label{Fig:spiral_opt_first}
\end{subfigure} \hfill
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{opt_sol_1.pdf_t}}
\caption{The optimal solution for $\bar \phi \in 2\pi + \frac{\pi}{2} + [- h_1,0]$.}
\label{Fig:spiral_opt_first_2}
\end{subfigure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{opt_sol_2.pdf_t}}
\caption{The optimal solution for $\bar \phi \in 2\pi + \frac{\pi}{2} + [0,h_2]$.}
\label{Fig:spiral_opt_first_3}
\end{subfigure} \hfill
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{opt_sol_2_tent.pdf_t}}
\caption{The optimal solution for $\bar \phi \in 2\pi + \frac{\pi}{2} + [h_2,\tan(\bar \alpha)]$.}
\label{Fig:spiral_opt_first_4}
\end{subfigure}
\caption{The optimal solution depending on the final angle $\bar \phi$ for the first round.}
\label{Fig:opt_spiral_intro}
\end{figure}

\begin{itemize}
\item The first situation is the $\bar \phi$ is the first round, more precisely $\bar \phi \in [0,2\pi + \frac{\pi}{2} - h_1]$, where the constant $h_1$ is computed explicitly by the results of Section \ref{S:family}: it is $\theta$ coordinates of the unique point on the border of the negativity region \gls{Narc} for $\Delta \phi = \tan(\bar \alpha)$. In this case the optimal solution coincides with the fastest saturated spiral of Section \ref{Sss:case_study_intro}: see Fig. \ref{Fig:spiral_opt_first}. 
\item After the angle $2\pi + \frac{\pi}{2} - h_1$, the derivative $\delta \tilde r(\bar \phi;0)$ is negative: hence the optimal solution has a initial segment of length $h$ in the direction $\bar \phi$, then it is the fastest saturated solution starting with an arc of the level set, Fig. \ref{Fig:spiral_opt_first_2}.
\item For $\bar \phi \in 2\pi + \frac{\pi}{2} + [0,h_2]$, the optimal solution candidate starts with an arc of the level set $\partial B_1(0)$, then a segment in the direction $\bar \phi$ and next the last round is the fastest saturated spiral, Fig. \ref{Fig:spiral_opt_first_3}. The value $h_2$ is computed explicitly in Section \ref{Ss:optimal_cand_3}, and corresponds to the transition from the arc case to the segment case for the fastest saturated spiral of the last round, Fig. \ref{Fig:spiral_opt_first_4}.
\item Finally, for $\bar \tau > 2\pi + \tan(\bar \alpha) + \frac{\pi}{2}$, the solution is the fastest saturated spiral up to the angle $\bar \phi - 2\pi - \bar \alpha$, followed by the tent case as described in Section \ref{Sss:optimal_solut_intro}, see Fig. \ref{Fig:opt_sol_3_tent_intro}.
\end{itemize}







\begin{figure}
\resizebox{.75\textwidth}{!}{\input{opt_sol_3_tent.pdf_t}}
\caption{The optimal candidate $r_\mathrm{opt}(\phi)$ for $\bar \phi \geq 2\pi + \tan(\bar \alpha) + \frac{\pi}{2}$.}
\label{Fig:opt_sol_3_tent_intro}
\end{figure}



The main result of this section is that this construction yields a unique spiral barrier which is positive:


\begin{proposition}[Propositions \ref{Prop:e_opt_large_phi} and \ref{Prop:postiv_aympt}]
\label{Prop:e_opt_large_phi_intro}
The optimal solution $r_\mathrm{opt}$ is positive for all $\bar \phi$ and for large angles can be estimated as %growth exponentially as
\begin{equation*}
r_\mathrm{opt}(\bar \phi) = 0.976359 r(\bar \phi) + \mathcal O(1)
\end{equation*}
where $r(\bar \phi)$ is the fastest saturated spiral
\end{proposition}

A remark is natural here: the gain of optimality is about 2.25\% w.r.t. the fastest saturated spiral, so one may suspect that there are some simpler proof{\color{red}s} of this result. Besides the fact that knowing the optimal solution is not a trivial fact, the difficulty in obtaining estimates is due to the RDE satisfied by $r(\phi)$, which makes comparisons difficult. One the other hand this method {\color{red} can be a powerful tool, since it }can be applied also for speeds which are not the critical one, and also to other geometric situations.


\subsubsection{Sections \ref{S:segment_case} and \ref{S:arc_1}}
\label{Sss:final_case_opt_intro}


At this point, having proved that for any given spiral barrier $\zeta$ the{\color{red}n} one can construct the one parameter family of spirals $\check r(\cdot;s_0)$ starting from $r_\mathrm{opt}$ and ending in $\zeta$, we are left to prove that $s_0 \mapsto \check r(\bar \phi;s_0)$ is increasing for all $\bar \phi$, thus effectively removing the negative regions of Proposition \ref{Prop:regions_pos_neg_segm_intro} (and Proposition \ref{Prop:neg_region} in the arc case) because of the additional perturbation to $\tilde r(\cdot;s_0)$. Since the structure of $\check r(\cdot;s_0)$ is more complicated, we have to consider several geometric situations, depending on the relative distance of $\bar \phi$ from $\phi_0$ and the structure of $\tilde r(\cdot;s_0)$.

\begin{figure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{segm_segm_sat_6.pdf_t}}
\caption{Segment-segment case.}
\label{Fig:deltacheckr_1}
\end{subfigure} \hfill
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_2.pdf_t}}
\caption{Segment-arc case.}
\label{Fig:deltacheckr_2}
\end{subfigure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{arc_segm_1.pdf_t}}
\caption{Arc-segment case.}
\label{Fig:deltacheckr_3}
\end{subfigure} \hfill
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_3_bis.pdf_t}}
\caption{Arc-arc case..}
\label{Fig:deltacheckr_4}
\end{subfigure}
\caption{The 4 main geometric situations for the optimal solution $\check r$.}
\label{Fig:deltacheckr}
\end{figure}

There are 4 main cases, each one with several subcases:
\begin{enumerate}
\item $\tilde r(\cdot;s_0)$ starts with a segment and its perturbation $\check r(\cdot;s_0)$ has an additional tent, Fig. \ref{Fig:deltacheckr_1}: we call it the \emph{segment-segment case};
\item $\tilde r(\cdot;s_0)$ starts with a segment and its perturbation $\check r(\cdot;s_0)$ end with an arc, Fig. \ref{Fig:deltacheckr_2}: we call it the \emph{segment-arc case};
\item $\tilde r(\cdot;s_0)$ starts with an arc and its perturbation $\check r(\cdot;s_0)$ has an additional tent, Fig. \ref{Fig:deltacheckr_3}: we call it the \emph{arc-segment case};
\item $\tilde r(\cdot;s_0)$ starts with an arc and its perturbation $\check r(\cdot;s_0)$ ends with an arc, Fig. \ref{Fig:deltacheckr_4}: we call it the \emph{arc-arc case}.
\end{enumerate}

The almost 20 subscases are due to the relative position of the final segment-arc and the initial segment-arc: referring for example to Fig. \ref{Fig:deltacheckr_1}, the tent may start inside the cone of opening $\theta$, instead that afterwards as depicted. Since this region is exactly when $\tilde r$ is discontinuous (it has also a Dirac-delta!), we did not find a general way of reducing these cases to a general situation, and we analyze{\color{red}d} them one by one.

It is important to notice that, because of Proposition \ref{Prop:tent_admissible_intro}, the segment-segment or arc-segment case are the only possibilities after some small initial angle of rotation, and this fact greatly simplif{\color{red}ies} the analysis: for example, we do not need to study the arc-arc case for large angles.

The main result{\color{red}s} are a series of lemmata, which state that the derivative $\delta \check r(\bar \phi;s_0)$ is positive: we collect their statements into the following:

\begin{proposition}
\label{Prop:deltacheckr_intro}
For a.e. every choice of $0 \leq \phi_0 < \bar \phi$ it holds $\delta \check r(\bar \phi;\phi_0) \geq 0$, with the equality only if $\dot \zeta(\phi_0+)$ is tangent to the optimal spiral $\check \zeta(\phi_0+;\phi_0)$.
\end{proposition}

This gives the proof of Theorem \ref{Theo:main_extended}, and concludes the paper.











%
%discuss here the general idea of our approach: let $Z=\zeta([0,S])$  be an admissible spiral-like strategy and let $(r(\phi),\phi)$ be its parametrization by radius (see again Theorem \ref{thm:param}). 
%Assume that for every point $\zeta(s)$ of the barrier you can assign a \emph{generalized} spiral $Z_s$ coinciding with $Z$ up to the point $\zeta(s)$ and parametrized by $(f_s(\phi),\phi)$, that is
%\begin{definition}[Family of Generalized Barriers]\label{def:fam:pert}
% We say that $f_{s}\in\text{SBV}([0,+\infty);\R)$, with $s\in[0,S]$, is an element of the family of generalized barriers $\mathcal F_Z$ if:
% \begin{itemize}
%     \item $f_0(\phi)> 0$ for $\phi\in[0,+\infty)$;
%     \item $f_s(\phi)=r(\phi)$ for every $\phi\leq\bar\phi$ whenever $\zeta(s)=(r(\bar\phi),\bar\phi)$.
%      \end{itemize}
%     Moreover, we say that it is a \emph{diverging family} if, calling \begin{equation}\label{eq:derivative:family}
%         \bar f_s(\phi)=\lim_{h\to 0}\frac{ f_{s+h}(\phi)-f_s(\phi)}{h},
%     \end{equation}
%     then $\bar f_s(\phi)\geq 0$ for every $\phi\in[0,\infty)$.
%
% \end{definition}
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{familyofspirals.png}
%     \caption{At every point an element of the family of generalized barriers is assigned.}
%     \label{fig:fam:of:spirals}
% \end{figure}
% See Figure \ref{fig:fam:of:spirals}.
%We remark that the parametrization of the optimal barrier $Z$ chosen at the beginning is an element of any family of generalized barriers, since it is $f_{S}$ accordingly to the previous notation. 
%We remark that a family of generalized barriers is NOT in general a family of admissible barriers, but it is a family of functions parametrized by the length parameter $s$. Indeed, it is not required that $Z_s$ are admissible or even that $(f_s(\phi),\phi)$ is a parametrization by angle as in the case of spirals. The family has only to satisfy all the assumptions in Definition \ref{def:fam:pert}.
%
%If a diverging family of generalized barriers exists, then no spiral-like strategy confines the fire, indeed:
%\begin{theorem}\label{thm:adm:diverg:family}
%Let $Z$ be as before and assume that there exists a family of generalized barriers $\lbrace f_s\rbrace=\mathcal F_Z$ which is diverging. Then $Z$ does not confine the fire.
%\end{theorem}
%The proof of this fact is very easy and relies on the following observation:
%by the fundamental theorem of calculus we have that
%\begin{equation*}
%    f_s(\phi)=f_0(\phi)+\int_0^s \bar f_{\eta}(\phi)d\eta.
%\end{equation*}
%By the diverging condition on the family $\mathcal F_Z$ it holds then that
%\begin{equation*}
%    f_s(\phi)\geq f_0(\phi),\quad\forall \phi\geq 0,\forall s\in[0,S], 
%\end{equation*}
%therefore
%\begin{equation*}
%    f_S(\phi)\geq f_0(\phi)> 0,
%\end{equation*}
%by the first assumption on the family. But since $f_S(\phi)$ is $r(\phi)$ one concludes that the radius of $Z$ is always positive. This also proves that $f_0(\phi)$ is the \emph{best} strategy we can do, since $r(\phi)\geq f_0(\phi)$ for every $\phi$. Here best refers to another optimization problem that we will discuss in a while (see Proposition \ref{Prop:opt:problem}).
%
%\medskip 
%Setting the framework of generalized barriers for the study of spirals has been extremely hard. One of the main issues of this procedure is that,
%in general, finding a diverging family of generalized barriers is a really difficult task. We did many attempts in order to exhibit an example of such a family, since the most reasonable failed to be correct (here the need to introduce the concept of \emph{generalized} barriers). Another important issue is that the proofs of these results are based on  numerical computations, so that it is extremely hard to take under control how the strategies evolve. The possibility to perform an analytical proof of these results is currently under investigation, but we strongly believe that the use of machine-based computations is always needed. 
%
%On the other side, we are strongly convinced that this new method to prove the non-admissibility of strategies could be promising in the study of the fire problem and could be adapted to more general cases involving internal barriers, therefore towards a proof of Bressan's Fire Conjecture in full generality.
%
%\subsection{Construction of the family of generalized barriers.}
%Summarizing, in order to prove the non-admissibility of spiral-like strategies, we need to find a diverging family of generalized barriers $\lbrace f_s\rbrace$. Let $Z$ be an admissible spiral, then for every $P\in Z$ the Admissibility Functional $\mathcal{A}$ reads as
%\begin{equation*}
%    \mathcal{A}(P)=u(P)-\frac{1}{\sigma}L(P)\geq 0,
%\end{equation*}
%where $L(P)$ is the length of the spiral from the starting point until the point $P$.
%
%We consider then the following \textbf{Optimization Problem}: fix any $\bar\phi$ angle, then the minimization problem is
%\begin{equation}\label{eq:mim:probl}
%    \min_{\tilde Z\in \mathcal A_S(Z,\bar\phi)} r_{\tilde Z}(\phi),\quad\text{ for some } \phi\geq\bar\phi,
%\end{equation}
%where $\mathcal{A}_S(Z,\bar\phi)$ denotes the class of admissible spirals (not necessarily blocking) that coincide with $Z$ up to the angle $\bar\phi$, with length uniformly bounded by a constant $N>>1$, and if $\tilde Z\in\mathcal{A}_S(Z,\bar\phi)$, then $(r_{\tilde Z}(\phi),\phi)$ will denote its parametrization by angle.
%Differently from what stated for the optimization problem \eqref{eq:opt:problem}, for which it has been proved that the minimum exists among admissible blocking strategies (therefore in a class that could be empty) \cite{Bressan_deLellis}, here the class of strategies is non-empty, since we are not assuming that they confine the fire in general. 
%
%
%
%Then we have the following geometric result (which is the content of Section \ref{S:exist_opti_traj}), that gives the minimum of the previous problem in the assumption $\phi\in[\bar\phi,\bar\phi+2\pi]$: 
%
%\begin{proposition}\label{prop:best:first:Enclosure}
%    Let $Z$ be an admissible spiral-like strategy and let $(r(\phi),\phi)$ be its parametrization by angle. Fix any $\bar\phi$ and consider the following strategy $\hat Z$ parametrized by $(\hat r(\phi),\phi)$ such that:
%    \begin{itemize}
%        \item $\hat r(\phi)=r(\phi)$ for every $\phi\leq\bar \phi$;
%        \item  $(r(\phi),\phi)\subset\lbrace u=u((r(\bar\phi),\bar\phi)\rbrace$ for $\phi\in[\bar\phi,\bar\phi+\Delta\bar\phi]$ (it is a subset of the level set of the minimum time function $u$);
%        \item $(r(\phi),\phi))$ for $\phi\in[\bar\phi+\Delta\bar\phi=\phi_1,\phi_2]$ is a segment of endpoints $P_1,P_2$ such that $P_1\in \lbrace u=u((r(\bar\phi),\bar\phi)\rbrace$ and $P_2$ is saturated, that is $\mathcal{A}(P_2)=0$. Moreover the segment $P_1P_2$ is tangent to $\lbrace u=u((r(\bar\phi),\bar\phi)\rbrace$ in $P_1$.
%        \item for every $\phi\geq \phi_2$ $\hat Z$ is a saturated spiral, that is $\mathcal{A}(r(\phi),\phi)=0$.
%    \end{itemize} Then we have that, for $\phi\in [\bar\phi,\bar\phi+2\pi]$ it holds
%    \begin{equation*}
%        r(\phi)\geq \hat r(\phi).
%    \end{equation*}
%\end{proposition}
%In Section \ref{S:exist_opti_traj} we prove that a minimizer for the problem \eqref{eq:mim:probl} always exists, but determining its exact shape for angles $\phi>>\bar\phi$ is an open problem.
%
%Since by the definition of diverging family of generalized barriers one naturally gets $r(\phi)\geq f_0(\phi)$ for every $\phi$ (so that $f_0$ is a minimizer!) we expected that the correct guess for the family was precisely the one suggested by the previous proposition. 
%
%\medskip
%At each point $P=\zeta(s)$ of the spiral the element of the family $f_s(\phi)$ is the length of the radius of a spiral-like strategy $Z_s$ (not necessarily admissible), with parametrization by angle given by $(f_s(\phi),\phi)$ with the following properties: it is a subset of the level set $\lbrace u=u(P)\rbrace$, then it continues as a segment whose last endpoint is saturated (in the sense the admissibility functional is zero at that point) and then it is a saturated spiral, in the sense that every point on the spiral is saturated. This is precisely the optimal found in Proposition \ref{prop:best:first:Enclosure}.
%
%
%
%Actually, it turned out that this construction did not produce a diverging family of generalized barriers since there was always a tiny region of parameters in which $\bar f_{s}<0$. Inspired by this (negative) result, after many attempts, we found out instead that the best strategy a player can do in order to confine the fire is to speed up the construction up to the critical value $2.144..$ (which is the maximum amount of speed we have for spirals not confining the fire, as conjectured in \ref{conj:spiral}), more precisely: from the point $\zeta(s)$, the strategy $Z_s$ is an an arc (subset of the level set of $u$), a segment (whose last point is saturated for the admissibility functional defined in \eqref{eq:sat:family}) and then it is a saturated spiral, but this time for the critical value $\sigma=2.6144...$. We underline that this is not a family of admissible barriers, since we are using a construction speed which is higher than the one available ($\leq 2.3$ in this case), but every element is a \emph{generalized} barrier. Computations show that in this case $\bar f_s>0$, therefore this family is diverging and it is the right one to consider for proving Theorem \ref{thm:main}. We remark that the value $2.3$ is 'sharp' up to numerical computations, indeed this procedure does not work for the value $2.4$. 
%
%The construction of this family gives the proof for the following 
%\begin{theorem}
%    If $\sigma\leq 2.3$ there exists a diverging family $\lbrace f_s\rbrace=\mathcal F_Z$ of generalized barriers.
%\end{theorem}
%This is the content of the last section. The main observation to carry out the proof is that, given two elements of the family $f_s$ and $f_{s+\delta s}$, then 
%$f_{s+\delta s}$ and $f_s$ for $\phi>>\bar\phi$ are the radii of saturated spirals, that is they satisfy the RDE \eqref{eq:ODE:saturated:1} for the critical speed. By linearity of the problem,  the derivative
%\begin{equation*}
%    \bar f_s(\phi)=\lim_{\delta s\to 0} \frac{f_{s+\delta s}(\phi)-f_s(\phi)}{\delta s}\qquad\text{ a.e } s,
%\end{equation*}
%satisfies the same RDE. To prove then its positivity, we need to use the \textbf{change of variables} \eqref{eq:change:var:1}. Therefore the study of the derivative $\bar f_s$ relies on a careful study of the solution of the same RDE.
%
%We conclude remarking that, even if a probably different proof is required in order to deal with the critical case $\sigma=2.6144..$, one could investigate extension of this procedure (weakening the diverging hypothesis of the family) in order to reach at least the values $2.4\sim 2.5$. We want also to underline that in this approach the presence of internal barriers seems to have no concrete role: it is a current object of investigation possible extension of the approach of generalized barriers to more general cases. 
%\subsubsection{Plan of the discussion.}
%In Section \ref{s:admissible:barriers} we give some notations and we define spiral-like strategies Definition \ref{def:adm:spirals}. We define the parametrization by angle $(r(\phi),\phi)$ Theorem \ref{thm:param}, which is motivated by the geometry of fire rays (Lemma \ref{lem:fire:rays}. In Section \ref{S:ODE} we derive the retarded differential equation associated to any admissible spiral (Lemma \ref{lem:ODE:spiral}). We study then in detail the RDE for a saturated spiral \eqref{eq:ODE:saturated} and we compute its spectrum in Subsection \ref{ss:dde}, Lemma \ref{lem:real:Eigenvalues} and Lemma \ref{lem:complex:eigenvalues}. In Subsection \ref{sss:subset:saturated} we prove that starting from any admissible spiral, if the player start constructing with speed $>2.6144..$ then it manages to confine the fire. In Subsection \ref{sss:important} we study the change of variable \eqref{eq:change:var:1} which will be of key importance for all the following results and we prove that the saturated spiral does not confine the fire for $\sigma\leq 2.6144..$ (Proposition \ref{prop:saturated:not:closed}). In Section \ref{S:exist_opti_traj} we study the optimization problem \ref{eq:mim:probl} and some properties of the minimum time function, previously defined. the results lead to the construction of the minimizer (at least for small angles) In Subsection \ref{Ss:minimal_reach}. In Section \ref{S:case:study} we focus on the first element of a family of generalized barrier $Z_0$ accordingly to the definition \ref{def:fam:pert} and we prove that $f_0(\phi)>0$ for every $\phi$, thus verifying the first condition on the family of generalized barriers. Finally, in Section \ref{c:family} we exhibit an example of a diverging family $\lbrace f_s\rbrace$ of generalized barriers and we compute the derivative $\lbrace \bar f_s\rbrace$. Here we distinguish between two cases: the first one in the assumption that the portion of strategy constructed on a level set of the minimum time function is not a single point (arc case, Subsection \ref{S:arc}), and the second one in the assumption it is a single point (segment case, Subsection \ref{S:segment}). In the Appendix \ref{S:appendix: fire} we give the numerical evaluations of functions needed for the proof of our results. 
%
%
%{\color{blue} {\bf DA SPOSTARE NELL'INTRODUZIONE} In this section we start with the construction of an optimal solution for the problem of Theorem \ref{Theo:exists_min}.
%
%More precisely, we will prove the following: given an admissible spiral $r(\phi)$, $0 \leq \phi \leq \bar \phi$, and an angle $\phi_0$, we prolong this spiral for $\phi > \phi_0$ as an admissible spiral $r(\phi;s_0)$, $s_0 = s^+(\phi_0)$, by assigning the angle of $\beta(\phi)$ for $\phi > \phi_0$. Let $\bar r(\phi) = r(\phi;0)$, which is independent of the spiral $r(\phi)$: it is indeed the unique spiral of the family starting from the point $(1,0)$.
%
%In this way we construct a continuous path
%\begin{equation*}
%    s_0 \mapsto r(\phi;s_0),
%\end{equation*}
%with the properties that
%$$
%r(\phi,0) = \bar r(\phi), \quad r(\phi;\bar \phi) = r(\phi).
%$$
%Next, we will show that for almost every $\phi$ there exists the limit
%\begin{equation*}
%    \lim_{\delta s_0 \to 0} \frac{r(\phi,s_0 + \delta s_0) - r(\phi,s_0)}{\delta s_0} = \delta r(\phi;s_0),
%\end{equation*}
%and the function $\phi \mapsto \delta r(\phi;s_0)$ satisfies an explicit RDE. In particular, we can compare the given spiral $r(\phi)$ with the spiral $\bar r(\phi)$ by
%\begin{equation}
%\label{Equa:deriv_integr_r}
%    r(\phi) = \bar r(\phi) + \int_0^{s^+(\phi)} \delta r(\phi;s) ds.
%\end{equation}
%
%The key point of the proof is the following
%
%\begin{theorem}
%    \label{Theo:optimality_check}
%    Assume that for every admissible spiral $r(\phi)$ the family $\{r(\phi;s_0)\}_{s_0 \in [0,S]}$ is a family of admissible spirals (Definition \ref{def:adm:spirals}) and for a.e. angle $\phi$ the map
%    \begin{equation*}
%        s_0 \mapsto r(\phi,s_0)
%    \end{equation*} 
%    is Lipschitz. If
%    \begin{equation*}
%        \delta r(\phi;s_0) := \lim_{\delta s \searrow 0} \frac{r(\phi,s_0 + \delta s_0) - r(\phi,s_0)}{\delta s_0} \geq 0,
%    \end{equation*}
%    for all $\phi$, then the following hold:
%    \begin{enumerate}
%        \item the spiral $r(\phi;s_0)$ is a minimum for Theorem \ref{Theo:exists_min} in the set of spirals $r'(\phi)$ such that
%        \begin{equation*}
%            r'(\phi) = r(\phi) \quad \forall \phi \leq \phi_0;
%        \end{equation*}
%        \item the base spiral $\bar r(\phi) = r(\phi;0)$ is an optimal solution of Theorem \ref{Theo:exists_min};
%        \item if moreover $\delta r(\phi;s_0) > 0$ for all $\phi >\phi(s_0)$, $s_0=s^+(\phi(s_0))$, unless
%        \begin{equation*}
%            \frac{d^+r}{ds} \rest_{s = s_0} = \frac{d^+r(s;s_0)}{ds} \rest_{s_0}, 
%        \end{equation*}
%        then $r(\phi;s_0)$ is the unique optimal solution for the closing problem starting at $\phi_0$ with a given admissible spiral $r(\phi)$ $\phi \in [0,\phi_0]$, and $\bar r(\phi)$ is the unique optimal solution for the closing problem.
%    \end{enumerate}
%\end{theorem}
%
%\begin{proof}
%    Formula \eqref{Equa:deriv_integr_r} gives the first two points. For the last one, since $s_0 \mapsto \frac{d^+r(s;s_0)}{ds} \rest_{s_0}$ is a given function, it follows that every optimal spiral has $\frac{dr}{d\phi}$ determined a.e.. In particular, being the discontinuous part only due to the curvature of the previous round, the function is uniquely determined by the construction of Theorem \ref{Prop:construct_spiral}. 
%\end{proof}
%
%Note that the uniqueness of the third point implies that if $r'(\phi;s_0')$ is the optimal spiral starting at $s_0' \geq s_0$ for the spiral $r(\phi;s_0)$, then $r'(\phi;s_0') = r(\phi;s_0)$.
%
%In order to construct the family $r(\phi;s_0)$ as required in the theorem, we need some preliminary analysis of an almost optimal candidate $\tilde r(\phi;s_0)$: the analysis of this family is the base for the construction of the optimal family $r(\phi;s_0)$. We will call this family \emph{the saturated family}, emphasizing the idea of being the fastest admissible spiral becoming saturated and remaining so.
%
%The family $\tilde r(\phi;s_0)$ is constructed in this section, while the construction of $r(\phi;s_0)$ will be studied in the next one.
%%{\color{blue} qui dobbiamo giustificare la scelta di $r$? Nono qui, metterei dopo, ma tanto lo rileggiamo}
%\begin{remark}
%    \label{Rem:more_than_one_round}
%    Note that we can assume that the optimal closing spiral is not closing for at least one round: indeed by Theorem \ref{Cor:curve_cal_R_sat_spiral} the structure of the last round is already known.
%\end{remark}
%
%\begin{comment}
%{\color{gray}
%In this section we will exhibit an example of a diverging family of generalized barriers. The computations that the construction requires rely on the evaluation of some trascendental functions, in the spirit of what has been done in Theorem \ref{thm:case:a} of the previous section, where we have analyzed concrete examples of admissible barriers and we have proved that they do not confine the fire. Here, we fix $\hat \sigma = 2.3$ and
%\begin{equation*}
%    \hat \alpha = \arccos \left( \frac{1}{\hat\sigma} \right),
%\end{equation*}
%while $\bar \sigma=2.6144..$ is the critical speed and $\bar \alpha$ denotes the corresponding angle. We consider also $Z = \zeta([0,S]) \in \mathcal{A}_S$ an admissible spiral, where $(r(\phi),\phi)$ denotes its parametrization by angle (Theorem \ref{thm:param_1}). For every point $\zeta(s)$ of the barrier we can assign an element of a family of generalized barriers, according to the following definition. (DA RIVEDERE L'INTRODUZIONE)
%
%Let $Z$ be an admissible spiral, and fix a length $\bar s$: this spiral is the one we have to evaluate, and sometimes will be referred as \emph{base spiral}.
%
%\begin{definition}[Family of Generalized spirals]
%\label{Def:fami_gene_barri_6}
%A spiral $Z_{\bar s} = \zeta_{\bar s}([0,+\infty))$ is a \emph{generalized spiral originating at $\zeta(\bar s)$} if, when represented in the fire coordinates $r_{\bar s}(\phi)$, it holds
%\begin{itemize}
%    \item $r_{\bar s}(\phi) > 0$ for $\phi \in [0,+\infty)$;
%    \item $r_{\bar s}(\phi) = r(\phi)$ for every $\phi \leq \bar \phi$, where $\bar \phi$ is the rotation angle corresponding to the length $\bar s$ for the base spiral, and $r(\phi)$ is the representation of $Z$ according to the fire coordinates (Theorem \ref{thm:param_1}). % whenever $\zeta(s)=(r(\bar\phi),\bar\phi)$.
%\end{itemize}
%
%A \emph{family of generalized spirals $\{Z_s\}_{s \in [0,S]}$} is a set of generalized spirals originating at every $s \in [0,S]$ of the domain of $\zeta$.
%
%The family of generalized spirals is a \emph{diverging family} if it is monotone w.r.t. $s$, i.e.
%\begin{equation*}
%    s \mapsto r_{s}(\phi) \quad \text{is monotone for all $\phi \in [0,\infty)$.}
%\end{equation*}
%\end{definition}
%
%The essential difference w.r.t. admissible spirals is that we do not require $\zeta_{\bar s}$ to be admissible. Looking into the proof of Theorem \ref{thm:adm:diverg:family}, one sees that this is not necessary, even if the speed of exponential growth is affected by the particular family we consider: indeed, since we will prolong $Z$ (constructed with speed $\hat \sigma = 2.3$) with spirals which are admissible for the faster speed $\bar \sigma = 2.61...$, we will obtain an exponential growth as for the critical case, which is lower than the exponential growth for the family of Section \ref{S:case:study}.
%
%In the following we will construct a family of generalized spirals which is differentiable w.r.t. $s$, and thus we will study the positivity of its derivative w.r.t. the starting point $\bar s$:
%\begin{equation}
%\label{eq:derivative:family}
%    \bar r_s(\phi) = \lim_{h \to 0} \frac{r_{s+h}(\phi) - r_s(\phi)}{h}.
%\end{equation}
%(MA SERVE QUESTA FORMULA QUI?) No però lasciamola, meglio una cosa in più
%
%%The construction of a diverging family of generalized spirals is necessary for the proof of Theorem \ref{thm:main}, whose proof follows by Theorem \ref{thm:adm:diverg:family}.
%
%The main result of this section is the following
%
%\begin{theorem}
%\label{thm:main:2}
%    If $\hat \sigma \leq 2.3$ there exists a diverging family $\lbrace r_s \rbrace_{s \in [0,S]} = \mathcal F_Z$ of generalized barriers, exponentially growing as in Theorem \ref{thm:case:a}.
%\end{theorem}
%
%Before diving into the proof, which requires several steps and some numerical evaluation of trascendental functions and it is the content of the next sections, we give a geometric intuition of the construction done below.
%
%The fundamental idea is to prolong the explicit solution for the optimal closing spiral. \\
%More precisely, for fixed angle $\bar \phi$, corresponding to a spiral length $\bar s$ for the base spiral $\zeta$, Theorem \ref{Cor:curve_cal_R_sat_spiral} gives the optimal closing barrier $\zeta_{\bar s}$ for angles $\phi \in [\bar \phi,\bar \phi + 2\pi + \beta^-(\bar \phi)]$. A first attempt is thus to continue $\zeta_{\bar s}$ as a saturated spiral for angles $\phi \geq \bar \phi + 2\pi + \beta^-(\bar \phi)$.
%%A possible candidate for the family is given following the geometric intuition of Section \ref{S:exist_opti_traj}. We recall that we have proved that, fixed any angle $\bar\phi$, the best strategy we can construct for $\phi\in[\bar\phi,\bar\phi+2\pi+\theta_0]$ where $\beta(\bar\phi)=\theta_0$ (Corollary \ref{Cor:curve_cal_R_sat_spiral}) is the one given by the union of a subset of the level set $u^{-1}(u(r(\bar\phi),\bar\phi))$, a segment tangent to it whose last point is saturated and then a saturated spiral. In Chapter  \ref{S:case:study} we have then proved that the strategy made by a circle, a segment tangent to it and a saturated spiral, does not confine the fire, which gives precisely the proof that $f_0$, which is the first element of the family of generalized barriers, is always strictly positive. 
%Even if perfectly reasonable, this family $f_s$ turned out to be non-diverging (see Definition \ref{def:fam:pert}), since in some cases $\bar r_s \leq 0$: the wrong sign of the derivative $\bar r_s$ happens already for the speed $\hat \sigma = \frac{1 + \sqrt{5}}{2}$ of Theorem \ref{thm:klein}. The explanation of this is that the continuation of the optimal closing solution of Theorem \ref{Cor:curve_cal_R_sat_spiral} as a saturated spiral is not the optimal closing solution for angles $> \bar \phi + 2\pi + \beta^-(\bar \phi)$: the idea behind this fact is that if we increase the length of a spiral of $\delta L$ about the angle $\bar \phi$, then the time function $u$ increases of $\delta L$ about the angle $\bar \phi + 2\pi + \beta^-(\bar \phi)$, and then we can build an admissible barrier of length $\hat \sigma \delta L > \delta L$, in particular a barrier which is closer that the original one.
%
%The idea to overcome this issue is to change the barrier speed $\hat \sigma \to \bar \sigma$ after the point $\bar s$: in other words, after the point $\bar s$ we construct the barrier as in the previous paragraph (i.e. the optimal closing barrier of Theorem \ref{Cor:curve_cal_R_sat_spiral} prolonged as a saturated spiral) with the critical speed $\bar \sigma$. Roughly speaking, after the time $u(\zeta(\bar s))$, the firefighters are allowed to build the barrier at a faster rate. Hence, even if these generalized spirals are not optimal for the speed $\bar \sigma$, they still form a diverging family. \\
%The new admissibility (functional which makes them admissible) is given by
%\begin{equation}
%\label{eq:new:Adm:funct}
%    \mathcal A_{\bar \sigma,\hat \sigma}(\zeta_{\bar s}(s)) = u(\zeta_{\bar s}(s)) - \frac{1}{\hat \sigma} \min\{\bar s,s\} - \frac{1}{\bar \sigma} [s - \bar s]^+ \geq 0,
%\end{equation}
%i.e. the length of the spiral is weighted by $\frac{1}{\hat \sigma}$ up to the point $\zeta(\bar s)$, then the by the smaller coefficient $\frac{1}{\bar \sigma}$ later on. This is the analytic expression of the fact that we allow a faster construction of the barrier after the base point $\zeta(\bar s)$.
%
%The exponential growth will be thus the one of the critical speed, given by Theorem \ref{thm:case:a}: indeed, Theorem \ref{thm:adm:diverg:family} yields the inequality
%\begin{equation*}
%    r(\phi) \geq r_0(\phi), \quad \forall \phi \geq 0,
%\end{equation*}
%in other words $r_0$ is the best strategy a firefighter can follow: construct a sub-optimal barrier with a faster speed. %it can decide to put some barrier on a level set, continue as a segment tangent to the level set and then it can construct a saturated spiral for the maximum speed available: the critical speed. This strategy is clearly not admissible, and this is the reason for considering \emph{generalized} barriers.
%
%The sub-optimality of $r_0$ is compensated if the speed difference is sufficiently large: this is the reason of the choice $\hat \sigma = 2.3$.
%%The idea here is that at any point $\zeta(s)=(r(\bar\phi),\bar\phi)$ of the spiral the strategy that confines better the fire is the union of a subset of the level set $u^{-1}(\zeta(s))$, a segment tangent to it and a saturated spiral for the critical speed $\bar\sigma=2.6144..$. In some sense it corresponds to slowing down the fire at the speed $\frac{\hat\sigma}{\bar\sigma}$ and then having at our disposal the construction speed $\hat \sigma\left(\frac{\bar\sigma}{\hat\sigma}\right)=\bar\sigma$. We will prove that this new family is diverging, and its explicit construction will give the proof of Theorem \ref{thm:main:2}. The heuristic motivations behind this choice of the family is not satisfactory: it is not clear while this method stops working with higher values of the speed $\hat\sigma$. Moreover, e
%Even if we strongly believe that variations of this procedure can be explored in order to increase the value of $\hat\sigma$ ($\sim 2.4-2.5$), the critical case seems to us very difficult to solve with such techniques. If we interpret our construction as the assignment of the control parameter $\beta_s(\phi)$ for each element of the generalized family $r_s$, the critical case requires a more careful choice of $\beta_s$, and probably an almost optimal choice, since every small perturbation can lead to a non diverging spiral due to the critical choice of the speed.
%
%The proof is organized as follows. In the first subsection we show that the first element $r_0$ of the family is always strictly positive and exponentially growing (Section \ref{Ss:r_0}). Then, we construct a generic element of the family $\mathcal F_Z$. As in the proof of Theorem \ref{thm:case:a}, we will consider separately the elements $r_s$ of the family made by an arc (a subset of the level set of the minimum time function $u$), a segment whose endpoint is saturated and a saturated spiral for the critical speed $\bar\sigma$ (\textbf{arc case}, Section \ref{S:arc}), and the elements $r_s$ made by a segment plus a saturated spiral (\textbf{segment case}, Section \ref{S:segment}). 
%
%The idea of the proof is very similar to the proof of Theorem \ref{thm:case:a}, when we optimize w.r.t. the parameter $a$. The derivative $\bar r_s(\phi)$ will satisfy the saturated Delay DE for angles $\phi \geq \bar \phi + 4\pi$ (the exact angle depends on the situation), so that one has to show that the initial data for this RDE verifies the condition of Lemma \ref{lem:key}: the proof of this fact is made by numerical evaluation of trascendental functions (all the plots are available in the Appendix \ref{S:appendix: fire}, done using Mathematica).% We use the software Mathematica to simply verify that all the quantities we are interested in are positive.
%
%}
%\end{comment}
%
%}


==> Martina_Correzioni/optimal_family.tex <==

\section{The optimal solution}
\label{S:optimal_solut}



In this section we construct the optimal candidate spiral for the minimization problem \eqref{Equa:minimum_rphi_intro}, \eqref{eq:min:probl_pert}. The previous section showed that the fastest saturated spiral $\tilde \zeta(\phi;s_0)$ is optimal outside a small interval of rotation angle in the first round after $\phi_0$ (for $\theta \in [0,\frac{\pi}{2}]$): we thus construct a new family of spirals $\check r$ whose structure takes into account that for some angles $\phi$ it is better not to follow the fastest saturated spiral $\tilde r$.


\subsection{Definition and construction of the optimal solution candidate}
\label{Ss:optimal_sol_def}


To describe the possible situations which can occur, depending on the relative position of $\phi_0, \bar \phi$ and the quantities \gls{thetatildeseg}, \gls{Deltaphi} {\color{red}(recall the definitions of the two quantities from Section \ref{S:family})}, we define the quantity \newglossaryentry{omegaopt}{name=\ensuremath{\omega},description={rotation angle for the unsaturated part of the fastest saturated spiral $\tilde r$}}
\begin{equation}
\label{Eq:def:omega:bar:theta}
\gls{omegaopt} = \begin{cases}
\bar \theta & \text{segment case}, \\
\frac{\pi}{2} + \Delta \phi & \text{arc case},
\end{cases} \qquad \text{so that} \ \bar \theta = \min \bigg\{ \omega, \frac{\pi}{2} \bigg\},
\end{equation}
and consider the following cases:
\begin{description}
\item[$\bar \phi -\phi_0 \in [0,2\pi +\beta^-(\phi_0))$] in this case we define
$$
\hat r(\phi;s_0) = \tilde r(\phi;s_0), \quad \phi \in [\phi_0,\bar \phi],
$$
i.e. we follow the fastest saturated spiral, which we already know it is the optimal solution for the first round by Theorem \ref{Cor:curve_cal_R_sat_spiral}.
{\color{red}Va messo come Point (2) perche' nello step successivo si fa riferimento a Point (2). }
\item[$\bar \phi - \phi_0 - 2\pi \in [\beta^-(\phi_0),\bar \theta)$] the solution $\hat r(\phi;s_0)$ will be a segment $[\check P_0,\check P^-]$ in the direction $\bar \phi - 2\pi$. We stop at a length $\ell_0 = |\check P^- - \check P_0|$ such that the fastest saturated spiral starting at the end point $\check P^-$ forms an initial angle whose value is on the boundary of the negativity region (it may happen that $\ell_0 = 0$). From this point onward, the solution is the fastest saturated spiral, which can start either with a segment or with a level set arc.

%    in the segment case, we follow the segment of direction $\bar \phi - 2\pi$ for a length $\ell_0$: this length is determined by the last point for which $\tilde r$ with perturbation in the direction $\bar \phi - 2\pi$ is in the negative region. Then we consider the almost optimal spiral $\tilde r$. 

\item[$\bar \phi - \phi_0 - 2\pi \in [\frac{\pi}{2},\omega)$] here we are in the arc case, and we follow the fastest saturated solution $\tilde r(\phi;s_0)$ in the interval
\begin{equation*}
\phi \in \bigg[ \phi_0,\bar \phi - 2\pi - \frac{\pi}{2} \bigg),
\end{equation*}
then we repeat the construction of the previous point: follow the direction $\bar \phi - 2\pi$ until we remain in the negativity region. Also in this case, after reaching the boundary of the negativity region, we close the last round starting either with a segment or with a level set arc.
%    we follow a segment of length $\ell_0$ in the direction $\bar \phi - 2\pi$ and then the fastest saturated solution $\tilde r$.

\item[$\bar \phi - \phi_0 - 2\pi - \omega \geq 0$] we follow the fastest saturated solution $\tilde \zeta$ up to the angle $\bar \phi - 2\pi - \bar \alpha$, then we repeat Point (2) above starting from a saturated point $\bar \phi - 2\pi - \bar \alpha$. Note that when $\bar \phi = \phi_0 + \omega + 2\pi$, then
\begin{equation*}
P_2 = \tilde \zeta \bigg( \phi_0 + \Delta \phi + \frac{\pi}{2} - \bar \alpha \bigg), \quad P_1 = \tilde \zeta(\phi_0 + \Delta \phi),
\end{equation*}
and then $\bar \phi - 2\pi \in \partial^- \tilde \zeta(\phi_1) \cap \partial^- \tilde \zeta(\phi_2)$, so that the two constructions above are the same. Here, we have indicated by $\phi_1=\phi_0+\Delta\phi$ and by $\phi_2=\phi_0+\Delta\phi+\frac{\pi}{2}-\bar\alpha$ as in Section \ref{S:arc}.
\end{description}

We can summarize the construction as follows, Fig. \ref{Fig:checkr_notation}: we follow the fastest saturated solution $\tilde r$ up to the angle $\check \phi_0$ such that
\begin{equation}
\label{Equa:barphi_checkphi_rel}
\bar \phi \in \check \phi_0 + 2\pi + [\beta^-(\check \phi_0),\beta^+(\check \phi_0)],
\end{equation}
then a segment of length $\ell_0 = |\check P^- - \check P_0|$ determined by requiring that it is the last point such that the derivative of the fastest saturated spiral $\tilde r'$ starting from that point satisfies $\delta \tilde r' \leq 0$, and then the fastest saturated solution for the last round.

\begin{figure}
\resizebox{.75\textwidth}{!}{\input{checkr_notation_2.pdf_t}}
\caption{The construction of the optimal closing solution: the starting spiral is $\zeta$ (black) up to the angle $\phi_0$. Then we follow the fastest saturated spiral $\tilde \zeta$ (blue) up to the angle $\check \phi_0$, determined by \eqref{Equa:barphi_checkphi_rel}. At this point we follow the segment with direction $\bar \phi$ until the angle between $\bar \phi$ and the new fastest saturated spiral $\check \zeta$ (red) is on the boundary of the negativity region. Note that while the blue spiral is inside the red one, the ray $\check r(\bar \phi;s_0)$ is smaller than $\tilde r(\bar \phi;s_0)$.}
\label{Fig:checkr_notation}
\end{figure}

Apriori, the perturbation of $\tilde r$ in the last case (i.e. on the saturated part of $\tilde r$) can be either a segment of an arc, i.e. we are exiting the negativity region in the arc or segment case. This may only happen in the first round, because afterwards the last round corresponds to the segment case (Proposition \ref{Prop:tent_admissible}): due to the particular form of the solution in this case (two consecutive segments followed by a saturated spiral), we will call this construction a \emph{tent}. In particular, Fig. \ref{Fig:checkr_notation} is correct when $\check P_1 = \check P^-$, but its purpose was just for notation.

We next fix the notation for the optimal candidate solution, see Fig. \ref{Fig:checkr_notation}.
\begin{itemize}
\item \gls{phibar} is the final angle, where we want to minimize $r(\bar \phi)$;
\item \gls{phi0} is the starting angle, with $\phi_0 \leq \bar\phi$, from which the arc/segment of the fastest saturated spiral \gls{rtildefam} starts;
\item the point \newglossaryentry{P0check}{name=\ensuremath{\check P_0},description={initial point of the segment of length $\ell_0$ in the direction $\bar \phi$}} \gls{P0check} is the point of the spiral $\tilde r(\phi;s_0)$ where a segment of length $\ell_0$ starts with direction $\bar \phi$; the corresponding angle is \newglossaryentry{phi0check}{name=\ensuremath{\check \phi_0},description={angle of the point $\check P_0$}} \gls{phi0check};
\item the segment of length \newglossaryentry{ell0}{name=\ensuremath{\ell_0},description={length of the segment $[\check P_0,P^-]$ of direction $\bar \phi$}} \gls{ell0} has endpoints \newglossaryentry{P-check}{name=\ensuremath{\check P^-},description={final point of the segment of length $\ell_0$ and direction $\bar \phi$}} $\check P_0,\gls{P-check}$, and its direction belongs to the subdifferential to the fastest saturated spiral $\tilde r(\phi;s_0),\phi)$ in the point $\check P_0$;
\item in the point $\check P^{-}$ we compute the fastest saturated spiral%, which we call \newglossaryentry{rcheck}{name=\ensuremath{\check r(\phi;s0)},description={last round of the oprimal spiral}} \gls{rcheck}
: two cases again can occur (arc and segment, see however Proposition \ref{Prop:tent_admissible});
\item if the segment case occurs in the point $\check P^{-}$ we will denote it by \newglossaryentry{P1check}{name=\ensuremath{\check P_1},description={initial point of the last segment of the fastest saturated spiral}} $\gls{P1check} = \check P^{-}$;
\item if the arc case occurs in the point $\check P^{-}$ we will denote by \gls{P1check} the second endpoint of the arc of the level set of $u$, with opening \newglossaryentry{Deltaphicheck}{name=\ensuremath{\Delta \check \phi},description={angle of the level set for the last round of the optimal solution $\check r(\bar \phi;s_0)$}} \gls{Deltaphicheck};
\item from the point $\check P_1$ the spiral is a segment of length \newglossaryentry{ell1}{name=\ensuremath{\ell_1},description={length of the last segment $[\check P_1,\check P_2]$ of the fastest saturated spiral}} \gls{ell1} and endpoints \newglossaryentry{P2check}{name=\ensuremath{\check P_2},description={final point of the last segment $[\check P_1,\check P_2]$ in the fastest saturated spiral}} $\check P_1,\gls{P2check}$;
\item the point $\check P_2$ is saturated;
\item the exterior angle between the segments $[\check P_0,\check P_1]$ and $[\check P_1,\check P_2]$ is the critical angle \gls{thetahat} in the segment case, while in the arc case the angle between $[\check P_0,\check P^-]$ and the level set arc is $\gls{h1Deltaphi} \leq \hat \theta$.
\end{itemize}

\begin{figure}
\centering
\includegraphics[scale=0.6]{tentspirals.png}
\caption{The three possible situations occurring in the construction of an element of the family, in the segment case ($\omega<\frac{\pi}{2}$). The blue curve represents the strategy $\tilde r(\phi,s_0)$ constructed in the previous section. In red the angle $\hat\theta$. {\color{blue} NON SO SE QUESTA FIGURA E' NECESSARIA}{\color{red} non perche' l'ho fatta io, ma secondo me e' piu' chiara perche' riassume punto 1,2,3. Io la terrei. Meglio una figura in piu' che una in meno}}
\label{fig:tent:solution}
\end{figure}

The first result of this section is that the above {\color{red}construction} defines a unique spiral \newglossaryentry{rcheckphis0}{name=\ensuremath{\check r(\phi;s_0)},description={optimal spiral at the angle $\bar \phi$}} \gls{rcheckphis0}.

\begin{proposition}
\label{Prop:unique_optimal_guess}
Given $s_0 = s(\phi_0) \geq 0$ and an angle $\bar \phi \geq \phi_0$, there exists a unique spiral $\check r(\phi;s_0)$ with the properties above.
\end{proposition}

We observe here that the Dirac delta part at $\tau = 1$ of $\delta \tilde r$ can be neglected having $0$ contribution to the integral {\color{red} la $\delta\tilde r$ e' calcolata in $\phi$ invece che in $\tau$, quindi secondo me scritto cosi', senza riferimenti, questo commento e' oscuro}
\begin{equation*}
\int \delta \tilde r(\bar \phi;s_0) ds_0.
\end{equation*}

\begin{proof}
The spiral $\check r(\phi;s_0)$ is defined once we know at what length $\ell_0$ of the segment starting in $\check P_0$ and pointing in the direction $\bar \phi$ has to stop, and the spiral becomes the fastest saturated afterward. This point is when the derivative $\delta \tilde r(\phi;\ell_0)$ of the fastest saturated spiral $\tilde r(\phi;\ell_0)$ starting from $\check P^-$, $|\check P^- - \check P_0| = \ell_0$, is $0$. Recall the definition of $\omega,\bar\theta$ in \eqref{Eq:def:omega:bar:theta}.

\begin{figure}
\resizebox{.75\textwidth}{!}{\input{nu_funct.pdf_t}}
\caption{The curves $\nu(\ell_0)$ of Proposition \ref{Prop:unique_optimal_guess} in blue, and the boundary of the negativity region in red.}
\label{Fig:nu_funct}
\end{figure}

If we define $\omega(\ell_0), \theta(\ell_0)$ as the values of the angles $\omega$, $\theta$ formed by the fastest saturated spiral along the segment $\ell_0 e^{\i \bar \phi}$ (recall that \gls{thetapertsegm} is the angle $\gls{thetatildeseg} -\theta_0$, where $\theta_0 = \beta^-(\check P_0)$ is the direction of the perturbation), we have defined a curve \newglossaryentry{nuell0}{name=\ensuremath{\nu(\ell_0)},description={curve representinvg the variation of the angles for the fastest saturated spiral w.r.t. the length $\ell_0$ of the segment $[\check P_0.\check P^-]$}}
\begin{equation*}
\R^+ \ni \ell_0 \mapsto \gls{nuell0} = (\theta(\ell_0),\omega(\ell_0)) \in \R^2.
\end{equation*}
The statement is proved if we show that this curve crosses the boundary of the negativity region $N = N_\mathrm{segm} \cup N_\mathrm{arc}$ (Propositions \ref{Prop:neg_region} and \ref{Prop:regions_pos_neg_segm}) only in one point: if this happens, the crossing point is a minimum for the quantity $\tilde r(\bar \phi;\ell_0)$, see Fig. \ref{Fig:nu_funct}. In the case the initial value is already outside the negativity region (i.e. $\theta > h_1(\Delta \phi)$), then we deduce that $\ell_0 = 0$. We observe that after the point $P_0$, the segment $[\check P_0,\check P^-]$ starts tangent to the spiral $\tilde \zeta$, i.e. $\theta = 0$ at the beginning $P_0$: thus we always start in the negativity region of $\delta \tilde r(\bar \phi)$ (i.e. $\ell_0 > 0$) apart from the case where $\check P_0 = P_0$. {\color{red}Cosa vuol dire questa frase? Non e' chiara}

%{\color{red} mi è venuto un dubbio: se per caso in $\bar\phi-2\pi$ sono nella regione di positività, allora $\ell_0=0$? Se sì forse vale la pena scriverlo. } {\color{blue} Si}

We can compute the derivative of the curve $\nu(\ell_0)$ by using the formulas of the previous section.

\begin{description}
\item[Segment case] we have form {\color{red}from} \eqref{Equa:delta_theta_segm_1}
\begin{equation*}
\frac{d\bar \theta}{d\ell_0} = \frac{1}{|\check P_2 - \check P_1|} \big( \sin(\theta) - \cot(\bar \alpha) \big( 1 - \cos(\theta)) \big) - \frac{\sin(\check \theta_1)}{\check r(\check \phi_1)},
\end{equation*}
\begin{equation*}
\frac{d\theta}{d\ell_0} = \frac{1}{|\check P_2 - \check P_1|} \big( \sin(\theta) - \cot(\bar \alpha) \big( 1 - \cos(\theta) \big),
\end{equation*}
where we have used Equation \eqref{Equa:delta_theta_segm_1} and where $\check r(\check \phi_1)$ is the length of the segment part of the optimal ray ending in the initial point $\check P_1$ and $\check \theta_1 = \beta^+(\check \phi_1) - \check \phi_1$. {\color{red}non ho capito che angolo e' $\check\theta_1$. Altra questione: questa derivata e' calcolata nel punto $\hat P_1$? Se si'  forse vale la pena scriverlo? Non so mi e' un po' oscuro}

 Hence, since $\frac{d\theta}{d\ell_0} > 0$ unless $\theta = 0$, the curve $\nu(\ell_0)$ {\color{red} which in the segment case is $(\theta(\ell_0),\bar\theta(\ell_0))$} can be represented as the graph of a differentiable function $\bar \theta(\theta)$, parameterized with $\theta$ increasing. Since in the segment case the boundary of the negativity region is $\theta = \hat \theta$, this curve exits the negativity region only in one point, corresponding to a unique value $\ell_0$.
 {\color{red}Altra domanda: il punto $\check P_1$ non puo' essere saturato? Il mio dubbio e' se l'espressione sopra con $\check P_2=\check P_1$ come si possa definire quella derivata? }

%{\color{red} scusa qui non mi trovo, ok la formula $\frac{d\theta}{d\ell_0}$ pero` non capisco la $\frac{d\theta_0}{d\ell_0}$... non dovrebbe essere $\delta\phi_0=-\delta\theta_0$?} {\color{blue} fissiamo l'angolo iniziale $\bar \theta_0$:  $\bar \theta$ e' l'angolo del segmento con la direzione $\theta_0$. Siccome nella nostra derivavazione noi calcoliamo la variatione $\delta \bar \theta$ di $\bar \theta$ rispetto alla direzione $\bar \theta_0$, allora il nuovo $\bar \theta$ e' $\bar \theta + \delta \bar \theta - \delta \theta_0$.}
% \medskip
% 
% {\color{red} il fatto e` che quella che scrivi tu e` vera se $\bar\theta=\frac{\pi}{2}$, in cui appunto verrebbe $\sin\theta_0$, ma cosi` onestamente non capisco.}
%
% \medskip
% {\color{red} altra domanda: perche` non basta dire che $\ell_0\rightarrow\theta({\ell_0})$ e` crescente?} {\color{blue} basta si, volevo mostrare che sappiamo calcolarlo in maniera bizantina}

\item[Arc case] here using \eqref{Equa:delta_Delta_phi} and the fact that the angle of the level set with the ray is $\frac{\pi}{2}$ to write
\begin{equation*}
\frac{d\omega}{d\ell_0} = \frac{d\Delta \check \phi}{d\ell_0} = \frac{1}{|P_2 - P_1|} \big( \sin(\theta) - \cot(\bar \alpha) (1 - \cot(\theta)) + {\color{red}\cot\bar\alpha}\sin(\theta) \Delta \check \phi \big) - \frac{\cos(\theta)}{\check r(\check \phi^-)},
\end{equation*}
{\color{red} ok ma ci ho messo un'ora per capire sto conto... forse vale la pena scrivere qualcosa in piu' o e' che sono troppo arrugginita?}
\begin{equation*}
\frac{d\theta}{d\ell_0} = \frac{\cos(\theta)}{\check r(\check \phi^-)},
\end{equation*}
with $\check r(\check \phi^-)$ the segment part of the optimal ray ending in $\check P^-$. Hence the curve can be represented again as the graph of a function $\Delta \check \phi(\theta)$, oriented along the increasing $\theta$ axis, and such that
\begin{equation*}
\frac{d\Delta \check \phi}{d\theta} = \frac{\check r(\check \phi^-)}{|P_2 - P_1|} \frac{\sin(\theta) - \cot(\bar \alpha) (1 - \cot(\theta) + \sin(\theta) \Delta \phi)}{\cos(\theta)} - 1.
\end{equation*}
The computation of Lemma \ref{Lem:study_g_1_arc} gives that the derivative of the boundary curve $h_1(\Delta \check \phi)$ is (see Equation \eqref{Equa:dh1_dDeltaphi})
\begin{equation*}
\frac{d\Delta \check \phi}{d\theta} = \bigg( \frac{dh_1}{d\Delta \check \phi} \bigg)^{-1} = - 1 - \frac{\cos(\theta) \Delta \check \phi}{\sin(\theta) - \cot(\bar \alpha) (1 - \cos(\theta) + \sin(\theta) \Delta \check \phi)},
\end{equation*}
Hence it follows that the curves are not transversal only if
\begin{equation*}
\frac{\check r(\check \phi^-)}{|P_2 - P_1|} = - \frac{\cos(\theta)^2 \Delta \check \phi}{(\sin(\theta) - \cot(\bar \alpha) (1 - \cot(\theta) + \sin(\theta) \Delta \check \phi))^2} \leq 0,
\end{equation*}
which is impossible, because the l.h.s. is strictly positive. {\color{red}Assolutamente non chiaro}
\end{description}
Thus the curves are transversal, and the crossing occurs from the negative to the positive: indeed this is clear in the segment case, while in the arc case
$$
\text{if} \quad \sin(\theta) - \cot(\bar \alpha)(1 - \cos(\theta) + \sin(\theta) \Delta \check \phi) < 0 \quad \text{then} \quad \frac{d\Delta \check \phi}{d\theta} < - 1 < \bigg( \frac{dh_1}{d\Delta \check \phi} \bigg)^{-1},
$$
$$
\text{if} \quad \sin(\theta) - \cot(\bar \alpha)(1 - \cos(\theta) + \sin(\theta) \Delta \check \phi) > 0 \quad \text{then} \quad \frac{d\Delta \check \phi}{d\theta} > -1 > \bigg( \frac{dh_1}{d\Delta \check \phi} \bigg)^{-1}. 
$$
The above inequalities yield the statement.
\end{proof}

\begin{figure}
\resizebox{.75\textwidth}{!}{\includegraphics{cross_segm_arc.png}}
\caption{Plot of the function of Remark \ref{Rem:trans_segm_arc}.}
\label{Fig:cross_segm_arc}
\end{figure}

\begin{remark}
\label{Rem:trans_segm_arc}
Observe that along the line $\Delta \check \phi = 0$, i.e. $\bar \theta = \frac{\pi}{2}$ and $\check \theta_1 = \frac{\pi}{2} - \theta$, we have
\begin{equation*}
\frac{d\omega}{d\theta} = \frac{d\bar \theta}{d\theta} = 1 - \frac{\ell_0}{\check r(\check \phi_1)} \frac{\sin(\bar \alpha) \sin(\theta)}{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}.
\end{equation*}
{\color{red}Ecco qua non si capisce. Penso che tu voglia fare separatamente il caso in cui $\hat P_0$ sia saturato, cosi' risponderesti alla mia domanda di prima, pero' va messo negli statement. E comunque non e' chiaro }
By observing that the spirals are convex and the angle at the top of the segment $\ell_0$ with the optimal ray is $\bar \alpha$, by elementary geometrical reasons we must have {\color{red}So elementary che sto qui da mezzora e ancora non ho capito come l'hai ottenuta}
\begin{equation*}
\ell_0 \leq \check r(\check \phi_1) \cot(\bar \alpha),
\end{equation*}
so that we obtain (see Fig. \ref{Fig:cross_segm_arc})
\begin{equation*}
\frac{d\omega}{d\theta} > 1 - \frac{\cos(\bar \alpha) \sin(\theta)}{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)} \geq 1 - \frac{\cos(\bar \alpha)}{\sin(\bar \alpha) - \cos(\bar \alpha)} > 0.293599 > 0.
\end{equation*}
Hence, when increasing the length $\ell_0$, we always pass from the segment case to the arc case.
\end{remark}

The previous proposition proves that construction of the spiral $\check r(\phi;s_0)$ at the beginning of the section is well defined. To prove that it is the minimizer for the minimization problem \eqref{eq:min:probl_pert}, we need to study the positivity of $\check r(\bar \phi;s_0)$ w.r.t. to perturbations. More precisely, we want to compute the derivative \newglossaryentry{deltarcheck}{name=\ensuremath{\delta \check r(\phi;s_0)},description={derivative of the candidate optimal slosing spiral w.r.t. the starting position $s_0$}}
\begin{equation}
\label{Equa:deltacheckr_def}
\gls{deltarcheck} = \frac{d}{ds_0} \check r(\phi;s_0).
\end{equation}
Similarly to the computation of $\delta \tilde r(\phi;s_0)$, depending on the structure of the solution $\check r$ several cases are possible: the initial fastest saturated part of $\check r(\phi;s_0)$ can be a segment or a level-set arc, and the segment starting in $\check P_0$ with length $\ell_0$ may be followed by a segment (tent case) or an arc.

The most important case is when the last round starts with segment (tent case), which we analyze in the next section.

%{\color{red} DA RIVEDERE
%
%
%We list the cases to be studied in the two following grids.
%
%\medskip
%First, we consider the case where at $\phi_0$ the solution $\tilde r(\phi;s_0)$ starts with a segment (Subsection \ref{S:segment}).
%
%\medskip
%
%\textbf{ The fastest saturated spiral $\tilde r(\phi;s_0)$ starts with a segment in $\phi_0$ (Segment Case), that is $\omega=\bar\theta$.}
%
%\begin{center}
%\begin{tabular}{ | m{4cm} | m{3.5cm}| m{3.5cm} | m{3.1cm}|} 
%\hline
%&$\bar \phi -\phi_0 \in [0,2\pi +\beta^-(\phi_0))$&$\bar \phi - \phi_0 - 2\pi \in [\beta^-(\phi_0),\bar \theta)$&$\bar \phi - \phi_0 - 2\pi - \omega \geq 0$\\
%  \hline
%  Tent& Content of Section \ref{S:exist_opti_traj} & Section \ref{Ss:init_segment}&Section \ref{Ss:init_segment}\\ 
%  \hline
%  Segment of length $\ell_0$+Arc & Content of Section \ref{S:exist_opti_traj} & Proposition \ref{Prop:tent_worst} &Proposition \ref{Prop:tent_worst}\\ 
%  \hline
%  
%\end{tabular}
%\end{center}
%
%We point out that the case $\bar\phi-\phi_0\in[0,2\pi+\beta^-(\phi_0))$ is the one considered in Section \ref{S:exist_opti_traj}, where the positivity is already proved. Moreover, the case where the closure is given by a segment of length $\ell_0$ and an arc can be reduced to the study of the case of the tent (two segments of lengths $\ell_0, \ell_1$ respectively) via Proposition \ref{Prop:tent_worst}, which we will prove in this subsection.
%\medskip
%
%Secondly, we consider the case where at $\phi_0$ the solution $\tilde r(\phi;s_0)$ starts with an arc (Subsection \ref{S:arc}).
%
%\medskip 
%
%\textbf{ The fastest saturated spiral $\tilde r(\phi;s_0)$ starts with an arc in $\phi_0$, that is $\omega=\frac{\pi}{2}+\Delta\phi$.}
%
%\begin{center}
%\begin{tabular}{ | m{2.5cm}| m{3.3 cm} | m{3.4cm}| m{2.9cm} | m{2.5cm}|} 
%\hline
%&$\bar \phi -\phi_0 \in [0,2\pi +\beta^-(\phi_0))$&$\bar\phi-\phi_0-2\pi\in[\beta^{-}(\phi_0),\frac{\pi}{2})$&$\bar \phi - \phi_0 - 2\pi \in [\frac{\pi}{2},\omega)$&$\bar \phi - \phi_0 - 2\pi - \omega \geq 0$\\
%  \hline
%  Tent & Content of Section \ref{S:exist_opti_traj}  & Subsection \ref{Ss:init_segment}& Subsection \ref{Ss:arc_to_segment} &\\ 
%  \hline
%  Segment $P_0P_1$+Arc & Content of Section \ref{S:exist_opti_traj} & Proposition \ref{Prop:tent_worst} &Proposition \ref{Prop:tent_worst}&Proposition \ref{Prop:tent_worst}\\ 
%  \hline
%  
%\end{tabular}
%\end{center}
%
%Again, the case $\bar\phi-\phi_0\in[0,2\pi+\beta^-(\phi_0))$ is the one considered in Section \ref{S:exist_opti_traj}, where the positivity is already proved. Moreover, the case where the closure is given by a segment of length $\ell_0$ and an arc can be reduced also in this case to the study of the tent (two segments of lengths $\ell_0$,$\ell_1$ respectively) via Proposition \ref{Prop:tent_worst}.
%}


\subsection{Formulas for the tent case}
\label{Ss:comput_tent_new}


\begin{figure}
\resizebox{.5\textwidth}{!}{\input{tent_compu.pdf_t}}
\caption{The geometry used to obtain the formulas for the tent case, Section \ref{Ss:comput_tent_new}.}
\label{Fig:tent_comput_geo}
\end{figure}

In order to study the correction to the fastest saturated spiral $\tilde r$ after the angle $\check \phi_0$, we need to study some geometric relations among the length $\ell_0$ of this segment and the underlying spiral $\tilde r$. This section is thus devoted to obtain these formulas, depending on the following quantities, which in order to distinguish from the previous ones are denoted with a hat, see Fig. \ref{Fig:tent_comput_geo}:
\begin{itemize}
\item the entrance ray \newglossaryentry{rhat0}{name=\ensuremath{\hat r_0},description={entry ray for the formulas for tent or arc perturbation}} \gls{rhat0} at angle $0$ initial position \newglossaryentry{Qhat0tent}{name=\ensuremath{\hat Q_0},description={base point for $\hat r_0$ in the tent or arc perturbation}} \gls{Qhat0tent}, the end point \newglossaryentry{Phat0}{name=\ensuremath{\hat P_0},description={initial point of the tent or arc perturbation}} \gls{Phat0} of $\hat r_0$ is saturated;
\item the exit ray \newglossaryentry{rhat2}{name=\ensuremath{\hat r_2},description={exit ray for the tent or arc computations}} \gls{rhat2} at angle $\hat \theta$ with initial position \newglossaryentry{Qhat2tent}{name=\ensuremath{\hat Q_2},description={base point for $\hat r_2$ in the tent or arc perturbation}} \gls{Qhat2tent}, the end point of $\hat r_2$ is saturated;
\item the length of segments \newglossaryentry{ellhat0}{name=\ensuremath{\hat \ell_0},description={length of the first segment in the tent or arc computations}} \newglossaryentry{ellhat1}{name=\ensuremath{\hat \ell_1},description={length of the second segment in the tent or arc computations}} \gls{ellhat0}, \gls{ellhat1};
\item the length \newglossaryentry{Lhattent}{name=\ensuremath{\hat L},description={length of the spiral between $Q_0,\hat Q_2$ in the tent or arc computations}} \gls{Lhattent} of the spiral at the base between the points $\hat Q_0, \hat Q_2$ (angle opening $[0,\hat \theta]$).
\end{itemize}
We will also give conditions to verify that it is admissible, which is equivalent to check that the angle formed by segment \newglossaryentry{Qhat1tent}{name=\ensuremath{\hat Q_1},description={point of the curve $\zeta$ where the optimal ray ending in the tip $\hat P_1$ of the ten or arc is detaching}} \newglossaryentry{Phat1tent}{name=\ensuremath{\hat P_1},description={tip of the tent or arc}} $[\gls{Qhat1tent},\gls{Phat1tent}]$ and \newglossaryentry{Phat2tent}{name=\ensuremath{\hat P_2},description={saturated final point of the tent or arc}} the second segment $[\gls{Phat1tent},\gls{Phat2tent}]$ is $\leq \frac{\pi}{2}$. %The input quantities are $\hat r_0$, $\hat Q_2 - \hat Q_0$, $\hat L$. 
{\color{red} Io scriverei che $\angle \hat Q_1\hat P_1\hat P_2\geq\frac{\pi}{2}$}

Since $\hat P_0$ is saturated, the saturation condition at the end point of the segment $\ell_1$ reads as
\begin{equation}
\label{Equa:saturation_tent}
\hat r_2 + \hat L - \hat r_0 - \cos(\bar \alpha) (\hat \ell_0 + \hat \ell_1) = 0,
\end{equation}
and the vector relation among the various points is
\begin{equation}
\label{Equa:vector_Q_1_Q_2}
\hat Q_0 + \hat r_0 (1,0) + \hat \ell_0 e^{\i \bar \alpha} + \hat \ell_1 e^{\i (\bar \alpha + \hat \theta)} = \hat Q_2 + \hat r_2 e^{\i \hat \theta}.
\end{equation}

Projecting the second equation in the direction $e^{\i \hat \theta}$ we obtain
\begin{equation*}
(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} + \hat r_2 - \hat \ell_1 \cos(\bar \alpha) - \hat \ell_0 \cos(\bar \alpha - \hat \theta) - \hat r_0 \cos(\hat \theta) = 0,
\end{equation*}
and then using the saturation condition
\begin{equation*}
(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - \hat \ell_0 \cos(\bar \alpha - \hat \theta) - \hat r_0 \cos(\hat \theta) = \hat L - \hat r_0 - \cos(\bar \alpha) \hat \ell_0,
\end{equation*}
\begin{equation*}
\begin{split}
\hat \ell_0 &= \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - {\color{red}\hat L} + \hat r_0 (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}. %\\
%&= 2.50013((\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - L) + 0.313453 \hat r_0.
\end{split}
\end{equation*}
Projecting again \eqref{Equa:vector_Q_1_Q_2} on the direction $e^{\i (\alpha + \hat \theta - \frac{\pi}{2})}$
\begin{equation*}
(\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})} + \hat r_2 \sin(\bar \alpha) - \hat \ell_0 \sin(\hat \theta) - \hat r_0 \sin(\bar \alpha + \hat \theta) = 0,
\end{equation*}
which gives
\begin{equation*}
\hat r_2 = \frac{\hat r_0 \sin(\bar \alpha + \hat \theta) + \hat \ell_0 \sin(\hat \theta) - (\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha)}.
\end{equation*}
%and using \eqref{Equa:ell_0_tent_general}
%\begin{align*}
%\hat r_2 &= \frac{\hat r_0}{\sin(\bar \alpha)} \bigg( \sin(\bar \alpha + \hat \theta) + \frac{\sin(\hat \theta) (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg) - \frac{L}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
%&\quad + \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta}}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha)} \\
%&= \hat r_0 \frac{\cos(\bar \alpha) - \cos(\bar \alpha + \hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - L}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha)}. %\\
%&= 1.23979 \hat r_0 + 1.31181 ((\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - L) - 1.0823 (\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}.
%\end{align*}
We can now compute $\hat \ell_1$ from \eqref{Equa:saturation_tent} as
\begin{equation*}
\hat \ell_1 = \frac{\hat r_2 + {\color{red}\hat L}  -\hat r_0 - \cos(\bar \alpha) \hat \ell_0}{\cos(\bar \alpha)}.
\end{equation*}
%and using \eqref{Equa:vector_Q_1_Q_2}, \eqref{Equa:r_2_tent_general}
%\begin{align*}
%\hat \ell_1 &= \frac{\hat r_0}{\cos(\bar \alpha)} \bigg[ \frac{1}{\sin(\bar \alpha)} \bigg( \sin(\bar \alpha + \hat \theta) + \frac{\sin(\hat \theta) (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg) - 1 - \cos(\bar \alpha) \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] \\
%&\quad + \frac{L}{\cos(\bar \alpha)} \bigg[ - \frac{L}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + 1 + \frac{\cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] \\
%&\quad + \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta}}{\cos(\bar \alpha)} \bigg[ \frac{1}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - \frac{\cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] - \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha) \cos(\bar \alpha)} \\
%&= \hat r_0 \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + \frac{L}{\cos(\bar \alpha)} \\
%&\quad +  \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - L}{\cos(\bar \alpha)} \bigg[ \frac{1}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} -\frac{\cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] - \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha) \cos(\bar \alpha)}. %\\
%&= 0.313453 \hat r_0 + 2.61433 L +  0.929517 ((\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - L) - 2.8296 (\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}.
%\end{align*}
Finally, the relation between $\hat L$ and $\hat Q_2 - \hat Q_0$ is given by integrating the curve \newglossaryentry{zetahattent}{name=\ensuremath{\hat \zeta},description={convex curve for computing the formulas for the tent or arc case}} \gls{zetahattent}: 
\begin{equation*}
\frac{d\hat \zeta}{d\theta} = e^{\i \theta} \hat R(\theta), \quad \hat \zeta(\theta) - \hat \zeta(\theta_0) = \int_{\theta_0}^{\theta} e^{\i \omega} \hat R(\omega) d\omega,
\end{equation*}
where \newglossaryentry{Rhatcurvsegm}{name=\ensuremath{\hat R},description={curvature of the convex curve $\hat \zeta$ for the computations of the tent or arc formulas}} \gls{Rhatcurvsegm} is the radius of curvature of $\hat \zeta$. The above formula holds also when the curvature is $\infty$, by considering $ds = \hat R d\theta$ as a measure.

We summarize the results obtained in the following lemma.

\begin{lemma}
\label{Lem:relation_admissibility_tent}
Consider the geometric configuration as in Fig. \ref{Fig:tent_comput_geo}, with $\hat P_0,\hat P_2$ saturated. Then the following geometric relations hold:
\begin{equation}
\label{Equa:DeltahatQ_tent}
\hat Q_2 - \hat Q_0 = \int_0^{\hat \theta} e^{\i \omega} \hat R(\omega) d\omega, \quad \hat R(\theta) \ \text{curvature of } \ \hat \zeta,
\end{equation}
\begin{equation*}
\hat L = \int_0^{\hat \theta} \hat R(\theta) d\theta,
\end{equation*}
\begin{equation}
\label{Equa:ell_0_tent_general}
\hat \ell_0 = \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - {\color{red}\hat L} + \hat r_0 (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation}
\begin{equation}
\label{Equa:r_2_tent_general}
\hat r_2 = \frac{\hat r_0 \sin(\bar \alpha + \hat \theta) + \hat \ell_0 \sin(\hat \theta) - (\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha)},
\end{equation}
\begin{equation*}
\hat \ell_1 = \frac{\hat r_2 + {\color{red}\hat L} -\hat r_0 - \cos(\bar \alpha) \hat \ell_0}{\cos(\bar \alpha)}.
\end{equation*}
\end{lemma}

Since all formulas are linear, we obtain the following corollary.

\begin{corollary}
\label{Cor:tent_corol_for_pert}
The same formula{\color{red}s} of Lemma \ref{Lem:relation_admissibility_tent} holds {\color{red}hold} for the perturbation $\delta \check r(\phi;s_0)$.
\end{corollary}

For future use, define the angle shift $\hat \theta$ in the $\tau$  ${\color{red}\hat\tau}$ variable: \newglossaryentry{tauhat}{name=\ensuremath{\hat \tau},description={angle shift \gls{thetahat} in the $\tau$ coordinates}}
\begin{equation}
\label{Equa:hattau_def}
\hat \tau = \frac{\hat \theta}{2\pi + \bar \alpha}.
\end{equation}

\subsubsection{Estimates for the admissibility of the tent}
\label{Sss:having_tent_check}


 The next series of lemmas give sufficient conditions which assure {\color{red}ensure} that the construction above is admissible, i.e. the angle between the segments $[\hat Q_1,\hat P_1]$ and $[\hat P_1,\hat P_2]$ is $\leq \frac{\pi}{2}$. If \newglossaryentry{phihat}{name=\ensuremath{\hat \phi},description={angular coordinate correponding to $\hat Q_1 = \hat \zeta(\hat \phi)$ for the tent or arc case}} $\hat Q_1 = \zeta(\gls{phihat})$, then we must require {\color{red}Questa $\zeta$ e' ausiliaria per indicare quel tratto li'. Non e' $\hat\zeta?$..?}
\begin{equation*}
\bar \alpha + \hat \theta - \hat \phi < \frac{\pi}{2}, \quad \hat \phi \geq 0,113642.
\end{equation*}

\begin{lemma}
\label{Lem:when_tent}
Assume that we are in the configuration of Fig. \ref{Fig:tent_comput_geo}: if \newglossaryentry{Kadmis}{name=\ensuremath{K_\mathrm{tent}},description={constant for verifying whether the tent is admissible}}
\begin{equation*}
\frac{\hat L}{\hat r_0} \leq \gls{Kadmis} = \frac{\sin(\bar \alpha) (\sin(\bar \alpha + \hat \theta) - \sin(\bar \alpha))}{\cos(\hat \theta) (1 - \sin(\bar \alpha))} < 0.966795,
\end{equation*}
then the tent is admissible.
\end{lemma}

%Observe that this is exactly the functional $AT(\tau)$ defined in \eqref{Equa:AT_tau}.

\begin{proof}
One sees geometrically that the worst case is when $\hat L = |\hat Q_2 - \hat Q_0|$ and $\hat Q_2 - \hat Q_1 {\color{red}\hat Q_0 } = \hat L e^{\i \hat \phi}$: indeed, from \eqref{Equa:ell_0_tent_general} one sees that by increasing $\hat L$ and keeping $\hat Q_0,\hat Q_1,\hat Q_2$ fixed, then length $\hat \ell_0$ increases {\color{red}decreases}, so that the worst situation is when $\hat \zeta$ is made of 2 segments, namely
\begin{equation*}
\hat \zeta = [\hat Q_0,\hat Q_1] e^{\i \bar \phi} \cup [\hat Q_1,\hat Q_2] e^{\i \hat \theta}.
\end{equation*}
{\color{red}Non e' $\bar\phi$.. a che angolo ti riferisci? }
At this point, the length of the segment $[\hat Q_1,\hat Q_2]$ does not enter into the computation of $\hat \ell_0$, while the first segment $[\hat Q_0,\hat Q_1]$ enters with the factor
\begin{equation*}
(\hat Q_1 - \hat Q_0) \cdot e^{\i \hat \theta} - |\hat Q_1 - \hat Q_0| = (\cos(\hat \theta - \hat \phi) - 1) |\hat Q_1 - \hat Q_0|.
\end{equation*}
Hence the worst case is when $\hat Q_2 = \hat Q_1$ (Fig. \ref{Fig:worst_tent_case}), maximizing the above negative term.

%if $Q$ is the point with the direction of $P_1$ in the subdifferential
%\begin{enumerate}
%    \item by taking the segment $Q - Q_0$ the angle of the optimal ray at $P_1$ increases,
%    \item by taking the largest $L$ after $Q$ the length of $\ell_0$ decreases, so that the angle increases.
%\end{enumerate}
%and the angle is $\phi$ where
%\begin{equation*}
%    \frac{\hat \ell_0}{\sin(\phi)} = \frac{\hat r_0}{\sin(\bar \alpha - \phi)},
%\end{equation*}
%i.e. the ray for the end point of $\hat r_0$ starts in the initial point of $\hat r_0$, and $Q_2$ is on the segment connecting these two points.
%
%This is because for $L$ and $Q_2 - Q_0$ fixed, the angle increases by packing the curve an close to $Q_ - Q_0$ as possible, and then increasing $L$ as much as we can so that $\hat \ell_0$ decreases.

\begin{figure}
\begin{subfigure}{.32\textwidth}
\resizebox{\linewidth}{!}{\input{worst_case_tent.pdf_t}}
\caption{The worst scenario of Lemma \ref{Lem:when_tent}.}
\label{Fig:worst_tent_case}
\end{subfigure}
\hfill
\begin{subfigure}{.32\linewidth}
\includegraphics[width=\linewidth]{admissi_tent_cond1.png}
\caption{Plot of the function (\ref{Equa:Loverr0_tent}) in blue, in orange the value of $\frac{\hat L}{\hat r_0}$ for the critical angle $\hat \phi = \bar \alpha + \hat \theta - \frac{\pi}{2}$.}
\label{Fig:Loverr0_tent}
\end{subfigure}
\hfill
\begin{subfigure}{.32\linewidth}
\resizebox{\linewidth}{!}{\input{worst_case_tent_L.pdf_t}}
\caption{The geometric situation to estimate the tent.}
\label{Fig:worst_case_tent_L}
\end{subfigure}
\caption{Analysis of Lemma \ref{Lem:when_tent}.}
\label{Fig:tent_2_case}
\end{figure}

For this configuration, elementary geometry gives %At this point the relation ($\hat \phi$ is the direction of the ray at $\hat P_1$)
\begin{equation*}
\hat r_0 \frac{\sin(\hat \phi)}{\sin(\bar \alpha - \hat \phi)} = \hat \ell_0 = \frac{\hat r_0 (1 - \cos(\hat \theta)) - \hat L (1 - \cos(\hat \theta - \hat \phi))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
{\color{red}where we have used Equation \eqref{Equa:ell_0_tent_general}},
i.e.
\begin{equation*}
\frac{{\color{red}{\hat L}}}{\hat r_0} = \frac{\sin(\bar \alpha - \hat \phi)(1 - \cos(\hat \theta)) - \sin(\hat \phi) (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha))}{\sin(\bar \alpha - \hat \phi)(1 - \cos(\hat \theta - \hat \phi))} = \frac{\sin(\bar \alpha) (\cos(\hat \phi) - \cos(\hat \theta - \hat \phi))}{\sin(\bar \alpha - \hat \phi) (1 - \cos(\hat \theta - \hat \phi))}.
\end{equation*}
The function
\begin{equation}
\label{Equa:Loverr0_tent}
\hat \phi \mapsto \frac{\sin(\bar \alpha) (\cos(\hat \phi) - \cos(\hat \theta - \hat \phi))}{\sin(\bar \alpha - \hat \phi) (1 - \cos(\hat \theta - \hat \phi))}
\end{equation}
is decreasing after $\bar \alpha + \hat \theta - \frac{\pi}{2}$, and its value at that angle is $0.966795$, see Fig. \ref{Fig:Loverr0_tent}: hence only for $\hat L \geq 0.966795 \hat r_0$ the tent may not be admissible.
\end{proof}

Consider finally the spiral $\tilde r(\phi;\phi_0)$, and let $\hat \phi_0$ {\color{red}be} the initial angle for the tent and $\hat \phi_2 = \hat \phi_0 + \hat \theta$ the final angle, and let \newglossaryentry{phihat3}{name=\ensuremath{\hat \phi_3},description={maximal angle for using the length bound as admissibility criterion for the tent}} $\gls{phihat3} \geq \hat \phi_0$. By considering the fastest growing spiral
\begin{equation*}
\dot r = \cot(\bar \alpha) r,
\end{equation*}
and observing that the worst situation is the one of the previous lemma (because it is the minimal length needed and applied at the last possible time), we obtain that if the tent is not admissible
\begin{equation}
\label{Equa:eastima_hat_r_2}
\begin{split}
\tilde r(\hat \phi_3) &\leq \tilde r(\hat \phi_0) e^{\cot(\bar \alpha)(\hat \phi_3 - \hat \phi_0)} - (\tilde L(\hat \phi_0 + \hat \theta) - \tilde L(\hat \phi_0)) e^{\cot(\bar \alpha)(\hat \phi_3 - \hat \phi_0 + \frac{\pi}{2} - \bar \alpha - \hat \theta)} \\
&\leq (\tilde L(\hat \phi_0 + \hat \theta) - \tilde L(\hat \phi_0)) \bigg( \frac{e^{\cot(\bar \alpha) (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{K_\mathrm{tent}} - 1 \bigg) e^{\cot(\bar \alpha) (\hat \phi_3 - \hat \phi_0 + \frac{\pi}{2} - \bar \alpha - \hat \theta)} \\
&\leq \tilde L(\hat \phi_3) \bigg( \frac{e^{\cot(\bar \alpha) (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{K_\mathrm{tent}} - 1 \bigg) e^{\cot(\bar \alpha) (\hat \phi_3 - \hat \phi_0 + \frac{\pi}{2} - \bar \alpha - \hat \theta)}.
\end{split}
\end{equation}
Hence by Corollary \ref{Cor:bound_length_gen} if
\begin{equation*}
\hat \phi_3 > \phi_0 + \omega \quad \text{and} \quad \bigg( \frac{e^{\cot(\bar \alpha) (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{K_\mathrm{tent}} - 1 \bigg) e^{\cot(\bar \alpha) (\hat \phi_3 - \hat \phi_0 + \frac{\pi}{2} - \bar \alpha - \hat \theta))} \leq 2.08
\end{equation*}
the tent is admissible. Numerically one obtains
\begin{equation*}
\hat \phi_3 - \hat \phi_0 \leq \bar \alpha + \hat \theta - \frac{\pi}{2} + \tan(\bar \alpha) \ln \bigg( \frac{2.08}{\frac{e^{\cot(\bar \alpha) (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{K_\mathrm{tent}} - 1} \bigg) = 7.86127,
\end{equation*}
which in the $\tau$ coordinates corresponds to
\begin{equation}
\label{Equa:hattau3_cond}
\hat \tau_3 - \hat \tau_0 \leq 1.05358.
\end{equation}
We thus have the following

\begin{proposition}
\label{Prop:tent_admissible}
The tent is admissible for $\tau \geq 0$.
%\begin{equation*}
%\tau \geq 1 - \hat \tau - \frac{\tan(\bar \alpha)}{2\pi + \bar \alpha} \ln \bigg( \frac{2.08}{\frac{e^{\cot(\bar \alpha) \hat \theta}}{K_\mathrm{tent}} - 1} \bigg) = 0.277638.
%\end{equation*}
\end{proposition}

\begin{proof}
The estimate \eqref{Equa:hattau3_cond} gives that if the tent starting in $\tau > 0$ is not admissible, then at $\tau + 1.05258 > 1$ the length $\tilde L$ does not satisfy Corollary \ref{Cor:bound_length_gen}, which is a contradiction.
\end{proof}

\begin{remark}
\label{Rem:inital_tent}
%Note that we cannot deduce that the tent is always admissible for $\tau \geq 0$ (i.e. in the saturated part) as we will see in the next section: we have only proved that after $\frac{1}{4}$ round the spiral $\tilde r$ has settled enough so that the tent become admissible.
%
It is easy to see that the tent is not always admissible: if we assume that the spiral $\zeta$ has a very long segment, $\zeta$ asymptotically becomes by scaling
\begin{equation*}
\Omega_0 = B_{\cos(\bar \alpha)}(0), \quad \zeta = [0,1],
\end{equation*}
for which the fastest saturated is an arc. Indeed, in this situation the saturation condition for the tent reads as
\begin{align*}
0 &= \hat \ell_1 \cos(\bar \alpha) + \hat \ell_0 \cos(\bar \alpha - \hat \theta) + \cos(\hat \theta) - \cos(\bar \alpha) - \cos(\bar \alpha) (1 + \hat \ell_0 + \hat \ell_1) \\
&= \hat \ell_0 (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)) - 2 \cos(\bar \alpha) + \cos(\hat \theta).
\end{align*}
Being
\begin{equation*}
2 \cos(\bar \alpha) - \cos(\hat \theta) = - 0.10964 < 0,
\end{equation*}
the tent is not admissible.
\end{remark}

\begin{remark}
\label{Rem:tent_admis_optim}
We end this section with the observation that if the tent is admissible it is the optimal solution. This fact is clearly implied by the uniqueness of Proposition \ref{Prop:unique_optimal_guess}, and moreover by Remark \ref{Rem:trans_segm_arc} we can only transition from the segment case to the arc case, not the opposite.
\end{remark}


\subsubsection{An estimate on the final value $\hat r(\bar \phi)$}
\label{Sss:estima_final_value}


To conclude this section, we give a simplified formula for estimating the final value of $\hat r$ and the angle $\bar \phi = \hat \phi_0 + 2\pi + \bar \alpha$.

\begin{lemma}
\label{Lem:final_value_satu}
Assume that base of the tent is a convex curve, $\hat r_0$ is saturated and that $\tilde r$ is the saturated spiral starting from $\hat \phi_0$. Then it holds
\begin{equation*}
\hat r(\bar \phi) \geq \tilde r(\bar \phi) - \hat \ell_0 \geq \tilde r(\bar \phi) - \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \hat r_0.
\end{equation*}
\end{lemma}

\begin{proof}
Since the base of the spiral is a convex curve, then
\begin{equation*}
|\hat Q_2 - \hat Q_0| \leq \hat L,
\end{equation*}
and then
\begin{equation*}
\hat \ell_0 \leq \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \hat r_0.
\end{equation*}
By Theorem \ref{Cor:curve_cal_R_sat_spiral} it holds also
\begin{equation*}
\hat r_2 \geq \tilde r(\hat \phi_2) = \tilde r(\hat \phi_0 + \hat \theta).
\end{equation*}
Hence we conclude that
\begin{align*}
\hat r(\bar \phi) &= (\hat r_2 - \tilde r(\hat \phi_2)) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} + \tilde r(\bar \phi) - \hat \ell_0 \\
&\geq \tilde r(\bar \phi) - \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \hat r_0. \qedhere
\end{align*}
\end{proof}


%
%{\color{blue} NON SERVE?
%
%\begin{corollary}
%\label{Cor:r_2tent_criterion}
%Let $\gls{phihat3} > \phi_0$: then if the solution of the saturated spiral satisfies
%$$
%r(\hat \phi_3) \geq \hat L (\frac{e^{\cot(\bar \alpha)\hat \theta}}{K_\mathrm{tent}} - e^{\cot(\bar \alpha)(\frac{\pi}{2} - \bar \alpha)}) = 0.0990184 \hat L,
%$$
%then the tent is admissible.
%\end{corollary}
%
%\begin{proof}
%The worst configuration is again the one in the previous lemma: indeed it is convenient to have the initial ray starting from $0$, and in order to maximize $\hat r_2$ one does not take additional base length. Then we compute for the saturated spiral
%\begin{align*}
%\hat r_2 &\leq \hat r_0 e^{\cot(\bar \alpha) \hat \theta} - \hat L e^{\cot(\bar \alpha)(\frac{\pi}{2} - \bar \alpha)} \\
%&\leq \hat L \bigg( \frac{e^{\cot(\bar \alpha) \hat \theta}}{K_\mathrm{tent}} - e^{\cot(\bar \alpha)(\frac{\pi}{2} - \bar \alpha)} \bigg) = 0.0990184 \hat L. \qedhere
%\end{align*}
%\end{proof}
%
%
%
%
%
%\newglossaryentry{phihat00}{name=\ensuremath{\hat \phi_{00}},description={maximal angle for using the length bound as admissibility criterion for the tent}}
%\begin{align*}
%\tilde r(\hat \phi_2) - \hat L \bigg( \frac{e^{\cot(\bar \alpha)\hat \theta}}{K_\mathrm{tent}} - e^{\cot(\bar \alpha)(\frac{\pi}{2} - \bar \alpha)} \bigg) &\geq \tilde r(\hat \phi_2) - \tilde L(\hat \phi_2 - 2\pi - \bar \alpha) \bigg( \frac{e^{\cot(\bar \alpha)\hat \theta}}{K_\mathrm{tent}} - e^{\cot(\bar \alpha)(\frac{\pi}{2} - \bar \alpha)} \bigg) \\
%&\geq \tilde L(\hat \phi_2 - \gls{phihat00}) \bigg( \frac{e^{\cot(\bar \alpha)\hat \theta}}{K_\mathrm{tent}} - e^{\cot(\bar \alpha)(\frac{\pi}{2} - \bar \alpha)} \bigg)
%\end{align*}
%if $\hat \phi_{00} \geq \hat \phi_2 - 2\pi - \bar \alpha$.
%
%
%
%If we let the the evolution run up tp the angle such that we are outside the non saturated zone + one rotation this angle is such that the final point is at most
%\begin{equation*}
%\tan(\bar \alpha) + \frac{\pi}{2} - \bar \alpha = 2.80812,
%\end{equation*}
%so that its final value is at most
%\begin{equation*}
%e^{\cot(\bar \alpha)(\tan(\bar \alpha) + \frac{\pi}{2} - \bar  \alpha)} r_2 \leq \hat L e^{\cot(\bar \alpha)(\tan(\bar \alpha) + \frac{\pi}{2} - \bar  \alpha)} \bigg( \frac{e^{\cot(\bar \alpha)\hat \theta}}{K_\mathrm{tent}} - e^{\cot(\bar \alpha)(\frac{\pi}{2} - \bar \alpha)} \bigg) = 0.316647.
%\end{equation*}
%
%
%
%
%
%{\bf DA VEDERE DOPO LE STIME}
%
%We will now give a second functional whose positivity implies the positivity of $K_\mathrm{tent} \hat r_0 - \hat L$. The idea is to allow the base of the tent to be convex but not necessarily part of an admissible spiral.
%
%Assume that the base of the spiral $\hat Q$ is saturated in $\hat Q_0$. The best perturbation in order to have that the length $\hat L$ is maximal and $\hat r_0$ is minimal is in Fig. \ref{Fig:Loverr0_tent}. Indeed, by convexity the maximal length is when the base is a tent, and the angle $\hat \theta$ at $\hat Q_1$ is the critical angle for which $\hat r_0$ is minimal when the spiral after $\hat Q_1$ is the fastest saturated spiral of Section \ref{S:segment}.
%
%Since the derivative $\delta \tilde r$ of Proposition \ref{Prop:regions_pos_neg_segm} is independent on the admissibility, the above analysis holds also for the non-admissible spiral, and as observed before the formulas of Lemma \ref{Lem:relation_admissibility_tent} are linear so that they holds also for the non-admissible spiral.
%
%For a more precise definition, let $\zeta$ be a spiral and an angle $\phi_{00}$ such that $\phi_0 \in \phi_{00} + 2\pi + [\beta^-(\phi_{00},\beta^+(\phi_{00}]$, and let $\hat r$ be the convex spiral defined by:
%\begin{itemize}
%\item a segment $[\hat Q_0,\hat Q_1]$ with direction $\phi_0$ of length $\hat \ell_0'$,
%\item a segment $[\hat Q_1,\hat Q_2]$ with direction $\phi_0 + \hat \theta$ of length $\hat \ell'_1$, and such that $\hat Q_2$ is saturated,
%\item the saturated spiral from $\hat Q_2$ (corresponding angle $\phi_{00} + \hat \theta$)
%\end{itemize}
%
%Define thus
%\begin{equation}
%\label{Equa:AT2_def}
%AT2(\phi_0) = K_\mathrm{tent} \hat r_0 - (\hat \ell_0' + \hat \ell_1').
%\end{equation}
%Clearly
%\begin{equation*}
%AT2(\phi_0) \leq AT(\phi_0),
%\end{equation*}
%so that the positivity of the $AT2$ is sufficient. We will thus proceed as follows: we will analyze the positivity of $r(\bar \phi)$ together with the positivity of
%\begin{equation*}
%K_\mathrm{tent} \hat r(\bar \phi) - (\hat \ell_0 + \hat \ell_1).
%\end{equation*}
%Actually we will work with the perturbations,
%\begin{equation*}
%K_\mathrm{tent} \delta \hat r(\bar \phi) - (\delta \hat \ell_0 + \delta \hat \ell_1).
%\end{equation*}
%
%
%%
%%procedure to have an upper estimate on the length of the base of the spiral: by geometric consideration the worst case is when the base is a tent itself, indeed it is the longest convex curve with slopes $0,\hat \theta$ at the boundary. Moreover, $r_0$ is minimal, so that
%%\begin{equation}
%%\label{Equa:simply_tent_verification}
%%\frac{\sin(\bar \alpha) (\sin(\bar \alpha + \hat \theta) - \sin(\bar \alpha))}{\cos(\hat \theta) (1 - \sin(\bar \alpha))} \hat r_0 - \hat L \geq \frac{\sin(\bar \alpha) (\sin(\bar \alpha + \hat \theta) - \sin(\bar \alpha))}{\cos(\hat \theta) (1 - \sin(\bar \alpha))} \hat r_0 - (\hat \ell_0' + \hat \ell_1'),
%%\end{equation}
%%see Fig. \ref{Fig:worst_case_tent_L}. We will show that the above functional is positive for the base solution and remains positive for the perturbation.
%%
%%\begin{remark}
%%\label{Rem:non_admis}
%%We note that here we do not require to be admissible, in the sense that the angle made by the optimal ray ending at the tip $\hat Q_1$ with the segment $[\hat P_1,\hat P_2]$ is larger than $\frac{\pi}{2}$: however the formula of Lemma \ref{Lem:relation_admissibility_tent} holds independently from the admissibility, and thus we will use these formulas.
%%\end{remark}
%%
%%
%
%
%
%
%\subsubsection{Estimates of $\hat r_2$}
%\label{Sss:estima_hat_r_2}
%
%
%{\color{red} DA AGGIUNGERE QUALCOSA}
%
%
%In this final section we give a condition which implies immediately that the perturbation $\delta \check r(\bar \phi;s_0)$ is positive. This condition, as well as the condition above, yields that after 1 rounds the positivity of $\delta \check r$ is assured, so that we are left to study only the first rounds for $\delta \check r$.
%
%The idea is to compare $\delta \check r$ with $\delta \tilde r$: indeed, if $\check \phi_2$ is the rotation angle of $\check P_2$ (the last point of the tent, see Fig. \ref{Fig:checkr_notation}) and %$\check \phi_0 + \hat \theta$ is the rotation angle correspondin
%\begin{equation*}
%\delta \tilde r(\check \phi_2;s_0) \leq \delta \check r(\check \phi_2,s_0),
%\end{equation*}
%being the RDE linear and since we do only a partial rotation $\bar \phi = \check \phi_2 + 2\pi + \bar \alpha - \hat \theta$, we have (see Fig. \ref{fig:comparison:saturated})
%\begin{equation}
%\label{eq:comp:sat}
%\check r(\bar \phi;s_0) - \tilde r(\bar \phi;s_0) = e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} \big( \check r(\check \phi_2;s_0) - \tilde r(\check \phi_2,s_0) \big) - \check \ell_0.
%\end{equation}
%The above formula is written for the derivative, but being linear holds also for the original solution, i.e
%\begin{equation*}
%\delta \check r(\bar \phi;s_0) - \delta \tilde r(\bar \phi;s_0) = e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} \big( \delta \check r(\check \phi_2;s_0) - \delta \tilde r(\check \phi_2,s_0) \big) - \delta \check \ell_0.
%\end{equation*}
%
%\begin{figure}
%\centering\includegraphics[scale=0.5]{comparisonwithsaturated.png}
%\caption{To quantify the quantity $\hat r(\bar\phi;s_0)$ we compare the black spiral with the saturated spiral (red curve). This motivates Equation \eqref{eq:comp:sat}, where the length $\overline{AB}=\hat r(\bar\phi-2\pi-\bar\theta)-\bar r(\bar\phi-2\pi-\bar\theta)$ is propagated in the angle $\bar\phi$ via the RDE of Saturated Spirals.}
%\label{fig:comparison:saturated}
%\end{figure}
%
%\begin{lemma}
%\label{Lem:estima_tent}
%Assume that the base of the tent $\hat \zeta$ of Fig. \ref{Fig:tent_comput_geo} is in the region where $\tilde r$ is saturated. Then
%\begin{equation*}
%\tilde r(\check \phi_2;s_0) < \hat r(\check \phi_2;s_0), \quad \hat \ell_0 \leq \hat r(\check \phi_0;s_0) \frac{1- \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} < 0.313454 \hat r(\check \phi_0;s_0).
%\end{equation*}
%The same holds for the perturbation $\delta r$, i.e.
%\begin{equation*}
%\delta \tilde r(\check \phi_2;s_0) < \delta \hat r(\check \phi_2;s_0), \quad \delta \hat \ell_0 \leq \hat r(\check \phi_0;s_0) \frac{1- \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} < 0.313454 \delta \hat r(\check \phi_0;s_0).
%\end{equation*}
%\end{lemma}
%
%\begin{proof}
%We use the saturation condition for the solution $\tilde r$,
%\begin{equation*}
%\tilde r(\check \phi_2;s_0) + L - \tilde r(\check \phi_0;s_0) + \cos(\bar\alpha)) \int \frac{\tilde r(\phi;s_0)}{\sin(\bar \alpha)} d\phi = 0,
%\end{equation*}
%and the same for the tent,
%\begin{equation*}
%\hat r(\check \phi_2;s_0) + L - \tilde r(\check \phi_0;s_0) + \cos(\bar\alpha)) (\ell_0 + \ell_1) = 0.
%\end{equation*}
%Since by convexity
%\begin{equation*}
%\int \frac{\tilde r(\phi;s_0)}{\sin(\bar \alpha)} d\phi < \ell_0 + \ell_1,
%\end{equation*}
%unless $\tilde r = 0$, we obtain the first inequality
%\begin{equation*}
%\tilde r(\check \phi_2;s_0) \leq \hat r_2(\phi;s_0).
%\end{equation*}
%The second follows from the formula \eqref{Equa:ell_0_tent_general}, 
%\begin{equation*}
%\begin{split}
%\hat \ell_0 &= \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - L + \hat r_0 (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
%\big[ |\hat Q2 - \hat Q_0| \leq L \big] \quad &\leq \frac{\hat r_0 (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}.
%\end{split}
%\end{equation*}
%We used that for continuous curves
%\begin{equation*}
%|\hat Q2 - \hat Q_0| \leq L.
%\end{equation*}
%
%The same formulas holds for the perturbations $\delta r_2,\hat r_2$, provided that
%\begin{equation*}
%\int \frac{\delta \tilde r(\phi;s_0)}{\sin(\bar \alpha)} d\phi \leq \delta \ell_0 + \delta \ell_1,
%\end{equation*}
%The picture of Fig. \ref{Fig:tent_comput_geo} is the same for the perturbation $\delta \tilde r,\delta \hat r$ provided that the base $\check \zeta$ is a convex spiral. Using \eqref{Equa:DeltahatQ_tent}, this occurs when $\tilde r \geq 0$ in the region at the base of the tent, i.e. for the angles $[\hat \phi_0,\hat \phi_2] - 2 \pi - \bar \alpha$ (recall that we are in the saturated region).
%%
%%
%%Observe that by
%%\begin{equation*}
%%L \geq |\Delta Q|,
%%\end{equation*}
%%it follows immediately
%%\begin{equation*}
%%\hat \ell_0 \leq \hat r_0 \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}.
%%\end{equation*}
%%Considering now the curve with radius of curvature given by $\tilde r$: then this curve is saturated, and thus it is impossible that $\hat r_2 = r_2$ is some point for any admissible curve, because the length of the tent is larger than the one of the saturated spiral.
%\end{proof}
%
%
%
%\subsubsection{A comparison for the tent case and the arc case}
%\label{Sss:comparison_tent_arc}
%
%
%In order to simplify the verification that the optimal solution is a generically a tent, we compare the arc case with a non admissible tent: this means that the angle \gls{thetatildeseg} (made by the optimal ray $r(\phi_0)$ and the segment $[P_1,P_2]$) is greater than $\frac{\pi}{2}$. For a given angle $\bar \phi$, let $r(\bar \phi)$ be the solution obtained by closing the last round with an arc (i.e. the arc is the only admissible solution here), and let $r_\mathrm{tent,n.a.}(\bar \phi)$ the solution obtained by closing with a segment even if $\bar \theta > \frac{\pi}{2}$ (i.e. it is not admissible (n.a.)).
%
%\begin{proposition}
%\label{Prop:tent_worst}
%It holds $r_\mathrm{tent,n.a.}(\bar \phi) < r(\bar \phi)$.
%\end{proposition}
%
%\begin{proof}
%First observe that we can reconstruct the arc solution by considering the non admissible segment solution and following the arc, i.e.
%\begin{equation*}
%r(\bar \phi) = \int \delta r_\mathrm{tent}(\bar \phi;s_0) ds_0.
%\end{equation*}
%It is thus enough to show that the derivative is $0$ in the arc region, because after it coincides with the segment solution.
%
%In this region for the non admissible tent the angles are as follows:
%\begin{equation*}
%\theta = \bar \theta - \frac{\pi}{2} > 0,
%\end{equation*}
%and since the derivative in the segment case depends only on $\theta$, if follows that the integral is strictly positive.
%\end{proof}
%
%
%
%
%
%%
%%In order to estimate the value $\hat r(\bar \phi;s_0)$, the idea will be to compare $\hat r_2(\bar \phi - 2\pi + \hat \theta;s_0)$ with $\tilde r_2(\bar \phi - 2\pi + \hat \theta;s_0)$, and then write
%%\begin{align}\label{eq:comp:sat}
%%    \notag\hat r(\bar \phi;s_0) &= e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} \big( \hat r_2(\bar \phi - 2\pi + \hat \theta;s_0) - \tilde r_2(\bar \phi - 2\pi + \hat \theta;s_0) \big) \\
%%    & \quad + \tilde r_2(\bar \phi;s_0) - \hat \ell_0.
%%\end{align}
%%{\color{red} non ho capito perchè hai messo il pedice $2$, non sono le soluzioni della spirale saturata $\bar r(\phi,s_0)$ della sezione $6$? No, lo so la notazione fa schifo}
%%
%%We next give some condition on $\hat r_0,L,Q_2-Q_1$ which assures that the above quantity is positive. The statements are based on the RDE, so that they hold also in the case of the perturbation.
%%
%%
%%
%%
%%\subsection{Formulas for the arc case}
%%\label{Ss:formulas_arc}
%%
%%
%%The geometric situation is in Fig. \ref{Fig:arc_comnpu}.
%%
%%\begin{figure}
%%\resizebox{.75\textwidth}{!}{\input{arc_compu.pdf_t}}
%%\caption{Geometric setting for the arc perturbation.}
%%\label{Fig:arc_comnpu}
%%\end{figure}
%%
%%The relations among points are \newglossaryentry{Phat-}{name=\ensuremath{\hat P^-},description={beginning of the arc in the arc perturbation}} \newglossaryentry{Qhat-}{name=\ensuremath{\hat Q^-},description={initial point of the optimal ray ending in $\hat P^-$ in the arc perturbation}} \newglossaryentry{rhat-}{name=\ensuremath{\hat r^-},description={optamal ray ening in $\hat P^-$ for the arc perturbation}} \newglossaryentry{rhat1}{name=\ensuremath{\hat r_1},description={optamal ray ening in $\hat P_1$ for the tent or arc perturbation}} \newglossaryentry{Deltaphicheck}{name=\ensuremath{\Delta \check \phi},description={opening angle of the arc for the arc perturbation}} \newglossaryentry{omegacheck}{name=\ensuremath{\check \omega},description={angle given by $\check \omega = \check \theta + \Delta \check \phi$ for the arc perturbation}} \newglossaryentry{thetacheck}{name=\ensuremath{\check \theta},description={angle formed by the arc and the segment $\hat \ell_0$ for the arc perturbation}} \newglossaryentry{Lhat1}{name=\ensuremath{\hat L_1},description={length of the arc $\overset{\frown}{\hat Q^- \hat Q_1}$ for the arc perturbation}}
%%\begin{equation}
%%\label{Equa:hatP0P-_arc}
%%\gls{Phat0} = \gls{Qhat0tent} + \gls{rhat0} e^{\i 0}, \quad \ \gls{Phat-} = \hat P_0 + \gls{ellhat0} e^{\i \bar \alpha} = \gls{Qhat-} + \gls{rhat-} e^{i (\bar \alpha + \gls{thetacheck} - \frac{\pi}{2})},
%%\end{equation}
%%\begin{equation}
%%\label{Equa:hatP1_arc}
%%\gls{Phat1tent} = \gls{Qhat1tent} + \gls{rhat1} e^{\i (\bar \alpha + \gls{omegacheck} - \frac{\pi}{2})}, \quad \gls{omegacheck} = \gls{thetacheck} + \gls{Deltaphicheck}, \quad \gls{rhat1} + \gls{Lhat1} = \check r^-,
%%\end{equation}
%%\begin{equation}
%%\label{Equa:hatP2_arc}
%%\gls{Phat2tent} = \gls{Phat1tent} + \gls{ellhat1} e^{\i (\bar \alpha + \gls{omegacheck})} = \gls{Qhat1tent} + \gls{rhat1} e^{i (\gls{omegacheck} + \bar \alpha - \frac{\pi}{2})} + \gls{ellhat1} e^{\i (\bar \alpha + \gls{omegacheck})} = \gls{Qhat2tent} + \gls{rhat2} e^{\i \gls{omegacheck}}.
%%\end{equation}
%%The relation among the angles is by
%%\begin{equation*}
%%\check \theta = h_1(\Delta \check \phi),
%%\end{equation*}
%%where $h_1$ is given by Lemma \ref{Lem:study_g_1_arc}, and the saturation condition is \newglossaryentry{Lcheckprime}{name=\ensuremath{\check L'},description={length of the arc $\overset{\frown}{\hat P^- \hat P_1}$ for the arc perturbation}}
%%\begin{equation*}
%%\hat r_2 + \gls{Lhattent} - \hat r_0 - \cos(\bar \alpha) \big( \hat \ell_0 + \gls{Lcheckprime} + \hat \ell_1 \big) = 0,
%%\end{equation*}
%%where $\check L'$ is the arc length $\overset{\frown}{\check P^- \check P_1}$. 
%%
%%We are interested in the perturbation of the above equation: we thus have
%%\begin{equation}
%%\label{Equa:saturation_arc_gen}
%%\begin{split}
%%0 &= \delta \hat r_2 + \delta \hat L - \delta \hat r_0 - \cos(\bar \alpha) \big( \delta \hat \ell_0 + \delta \check L' + \delta \ell_1 \big) \\
%%\big[(\ref{Equa:hatP2_arc})\big] \quad &= (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i \check \omega} + (\delta \hat r_1 - \hat \ell_1 \delta \check \omega) \sin(\bar \alpha) + \delta \hat L - \delta \hat r_0- \cos(\bar \alpha) \bigg( \delta \hat \ell_0 - \hat r^- \delta \check \theta + \int_{\check \theta}^{\check \omega} \delta \hat r(\phi) d\phi \bigg),
%%%\big[(\ref{Equa:hatP1_arc})\big] \quad &= (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i \check \omega} + \delta \hat r_1 \sin(\bar \alpha) + \hat r_1 \delta \check \omega \cos(\bar \alpha) - \hat \ell_1  \delta \check \omega \sin(\bar \alpha) + \delta \hat L - \delta \hat r(\check \phi_0) - \cos(\bar \alpha) \Bigg[ \delta \hat \ell_0 - \hat r^- \delta \check \theta + \int_{\check \theta}^{\check \omega} \delta r(\phi) d\phi + \hat r_1 \delta \check \omega \Bigg] \\
%%\end{split}
%%\end{equation}
%%where we have used
%%\begin{equation*}
%%\delta \hat r_2 = (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i \check \omega} + (\delta \hat r_1 - \hat \ell_1 \delta \check \omega) \sin(\bar \alpha) + (\hat r_1 \delta \check \omega + \delta \ell_1) \cos(\bar \alpha), \quad \delta \check L' = - \hat r^- \delta \check \theta + \int_{\check \theta}^{\check \omega} \delta \hat r(\phi) d\phi + \hat r_1 \delta \check \omega.
%%\end{equation*}
%%
%%Since the perturbation has initial data
%%\begin{equation}
%%\label{Equa:delta_hatr2}
%%\hat r(\check \omega + \phi) = \hat r_2 (1 + \cot(\bar \alpha) (\phi - \check \omega)) - L(\phi) + L(\check \omega), \quad \delta \hat r(\check \omega) = \delta \hat r_2 - \hat r_2 \cot(\bar \alpha) \delta \check \omega - \hat R_2 \delta \check \omega,
%%\end{equation}
%%where $R_2$ is the radius of curvature at $\hat Q_2$, by \eqref{Equa:hatP2_arc} we have
%%\begin{equation*}
%%\delta \hat r_2 - \cot(\bar \alpha) \hat r_2 \delta \check \omega = \frac{1}{\sin(\bar \alpha)} \big[ (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i (\check \omega + \bar \alpha - \frac{\pi}{2})} + (\delta \hat r_1 - \hat \ell_1 \delta \check \omega) \big],
%%\end{equation*}
%%and we rewrite \eqref{Equa:saturation_arc_gen} as
%%\begin{equation}
%%\label{Equa:initla_arc_gen}
%%\begin{split}
%%\delta \hat r_2 - \cot(\bar \alpha) \hat r_2 &= \frac{1}{\sin(\bar \alpha)^2} \bigg[ (\delta \hat Q_1 - \delta \hat Q_2) \cdot \big( \sin(\bar \alpha) e^{\i (\check \omega + \bar \alpha - \frac{\pi}{2})} - e^{\i \check \omega} \big) - \delta \hat L + \delta \hat r_0 + \cos(\bar \alpha) \bigg( \delta \hat \ell_0 - \hat r^- \delta \check \theta + \int_{\check \theta}^{\check \omega} \delta \hat r(\phi) d\phi \bigg) \bigg] \\
%%&= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \bigg[ - (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i (\check \omega + \bar \alpha)} + \delta \hat \ell_0 - \hat r^- \delta \check \theta + \int_{\check \theta}^{\check \omega} \delta \hat r(\phi) d\phi \bigg] + \frac{- \delta \hat L + \delta \hat r_0}{\sin(\bar \alpha)^2}.
%%\end{split}
%%\end{equation}
%%Using \eqref{Equa:hatP0P-_arc} we can write
%%\begin{equation*}
%%\hat r^- \delta \check \theta = (\delta \hat Q_0 - \delta \hat Q_1) \cdot e^{i(\check \theta + \bar \alpha)} + \delta \hat r_0 \cos(\bar \alpha + \check \theta) + \delta \hat \ell_0 \cos(\check \theta),
%%\end{equation*}
%%\begin{equation*}
%%\delta r^- = (\delta \hat Q_0 - \delta \hat Q^-) \cdot e^{i(\bar \alpha + \check \theta - \frac{\pi}{2})} + \delta \hat r_0 \sin(\bar \alpha + \check \theta) + \delta \hat \ell_0 \sin(\check \theta).
%%\end{equation*}
%%and since for $\phi \in [\check \theta,\check \omega]$
%%\begin{equation*}
%%\hat r(\phi) = \hat r^- - \hat L(\phi) + \hat L(\check \theta),
%%\end{equation*}
%%we also have
%%\begin{equation*}
%%\delta \hat r(\phi) = \delta \hat r^- - \delta \hat L(\phi) + \delta \hat L(\check \theta),
%%\end{equation*}
%%\begin{align*}
%%\int_{\check \theta}^{\check \omega} \delta \hat r &= \delta \hat r^- \Delta \check \phi - \int_{\check \theta}^{\check \omega} ( \delta \hat L(\phi) - \delta \hat L(\check \theta) ) d\phi \\
%%&= \Big[ (\delta \hat Q_0 - \delta \hat Q^-) \cdot e^{i(\bar \alpha + \check \theta - \frac{\pi}{2})} + \delta \hat r_0 \sin(\bar \alpha + \check \theta) + \delta \hat \ell_0 \sin(\check \theta) \Big] \Delta \check \phi - \int_{\check \theta}^{\check \omega} ( \delta \hat L(\phi) - \delta \hat L(\check \theta) ) d\phi.
%%\end{align*}
%%Substituting into \eqref{Equa:initla_arc_gen} we obtain
%%\begin{equation}
%%\label{Equa:2_initla_arc_gen}
%%\begin{split}
%%\delta \hat r_2 - \cot(\bar \alpha) \hat r_2 &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \bigg[ - (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i (\check \omega + \bar \alpha)} - (\delta \hat Q_0 - \delta \hat Q_1) \cdot e^{i(\check \theta + \bar \alpha)} + (\delta \hat Q_0 - \delta \hat Q^-) \cdot e^{i(\bar \alpha + \check \theta - \frac{\pi}{2})} \Delta \check \phi \bigg] \\
%%& \quad - \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \int_{\check \theta}^{\check \omega} ( \delta \hat L(\phi) - \delta \hat L(\check \theta) ) d\phi - \frac{\delta \hat L(\check \omega)}{\sin(\bar \alpha)^2} \\
%%&\quad + \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \bigg( \frac{1}{\cos(\bar \alpha)} - \cos(\bar \alpha + \check \theta) + \sin(\bar \alpha + \check \theta) \Delta \check \phi \bigg) \bigg] \delta \hat r_0 \\
%%& \quad + \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\check \theta) + \sin(\check \theta) \delta \Delta \check \phi) \bigg] \delta \hat \ell_0.
%%\end{split}
%%\end{equation}
%%The final value is then computed by
%%\begin{equation}
%%\label{Equa:final_arc_gen}
%%\begin{split}
%%\delta \hat r(\bar \phi) &= \bigg[ \delta \hat r_2 - \cot(\bar \alpha) \hat r_2 \delta \check \omega - \delta \tilde r_2 \bigg] e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \check \theta - \Delta \check \phi)} + \delta \tilde r(\bar \phi) - \delta \check \ell_0 \\
%%[(\ref{Equa:thetaDeltaphi_def}] \quad &= \Bigg\{ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \bigg[ - (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i (\check \omega + \bar \alpha)} - (\delta \hat Q_0 - \delta \hat Q_1) \cdot e^{i(\check \theta + \bar \alpha)} + (\delta \hat Q_0 - \delta \hat Q^-) \cdot e^{i(\bar \alpha + \check \theta - \frac{\pi}{2})} \Delta \check \phi \bigg] \\
%%& \qquad - \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \int_{\check \theta}^{\check \omega} ( \delta \hat L(\phi) - \delta \hat L(\check \theta) ) d\phi - \frac{\delta \hat L(\check \omega)}{\sin(\bar \alpha)^2} \\
%%& \qquad + \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \bigg[ \frac{1}{\cos(\bar \alpha)} - \cos(\bar \alpha + \check \theta) + \sin(\bar \alpha + \check \theta) \Delta \check \phi \bigg] \delta \hat r_0 - \delta \tilde r_2 \Bigg\} e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \check \theta - \Delta \check \phi)} + \delta \tilde r(\bar \phi) \\
%%&= \frac{\cot(\bar \alpha) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \check \theta - \Delta \check \phi)}}{\sin(\bar \alpha)} \\
%%& \quad \cdot \Bigg\{ \bigg[ - (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i (\check \omega + \bar \alpha)} - (\delta \hat Q_0 - \delta \hat Q_1) \cdot e^{i(\check \theta + \bar \alpha)} + (\delta \hat Q_0 - \delta \hat Q^-) \cdot e^{i(\bar \alpha + \check \theta - \frac{\pi}{2})} \Delta \check \phi \bigg] \\
%%& \qquad - \int_{\check \theta}^{\check \omega} ( \delta \hat L(\phi) - \delta \hat L(\check \theta) ) d\phi - \frac{\delta \hat L(\check \omega)}{\cos(\bar \alpha)} \\
%%& \qquad + \bigg[ \frac{1}{\cos(\bar \alpha)} - \cos(\bar \alpha + \check \theta) + \sin(\bar \alpha + \check \theta) \Delta \check \phi \bigg] \delta \hat r_0 - \frac{\sin(\bar \alpha)}{\cot(\bar \alpha)} \delta \tilde r_2 + \big( 1 - \cos(\check \theta) + \sin(\check \theta) \Delta \check \phi \big) \delta \tilde r(\bar \phi) \Bigg\},
%%\end{split}
%%\end{equation}
%%where $\delta \tilde r$ is the evolution for the perturbation of the saturated spiral. We remark that the critical relation $\check \theta = h_1(\Delta \check \phi)$ gives that $\delta \hat \ell_0$ disappears in the above formula.
%%
%%\begin{remark}
%%\label{Rem:different_der}
%%Note that the derivative is different, perhaps due to the fact that the angle for the segment case are fixed, while here they may change because we are on the critical curve $\check \theta = h_1(\Delta \check \phi)$.
%%\end{remark}
%}


==> appunti.tex <==
 \subsection{Base case: Segment}\label{ss:base:case:segment}
    We study first the segment case then the arc case (whose analysis is identical).  We write explicitly $f_0(\phi)=r(\phi)$: we have that
    \begin{itemize}
        \item $P_1=(1,0)$;
        \item for $\phi\in[0,\bar\theta-\alpha)$ we have that
        \begin{equation*}
            r(\phi)=\frac{\sin\bar\theta}{\sin(\bar\theta-\phi)};
        \end{equation*}
        \item for $\phi\in [\bar\theta-\alpha,2\pi)$ it holds
        \begin{equation*}
            \frac{d}{d\phi}r(\phi)=\cot\alpha r(\phi),
        \end{equation*}
        that is 
        \begin{equation*}
            r(\phi)=\frac{\sin\bar\theta}{\sin\alpha}e^{\cot\alpha(\phi-\bar\theta+\alpha)};
        \end{equation*}
        \item there is a jump at $\phi=2\pi$, that is
        \begin{equation*}
            r(2\pi+)-r(2\pi)=-1;
        \end{equation*}
        \item for $\phi\in [2\pi,2\pi+\bar\theta)$ it holds
        \begin{equation*}
            \frac{dr}{d\phi}=\cot\alpha r(\phi),
        \end{equation*}
        that is
        \begin{equation*}
            r(\phi)=\left[\frac{\sin\bar\theta}{\sin\alpha} e^{\cot\alpha(2\pi-\bar\theta+\alpha)}-1\right]e^{\cot\alpha(\phi-2\pi)};
        \end{equation*}
        \item in $\phi=2\pi+\bar\theta$ there is a jump, that is
        \begin{equation*}
            r(2\pi+\bar\theta+)-r(2\pi+\bar\theta)=-\frac{\sin(\bar\theta-\alpha)}{\sin\alpha};
        \end{equation*}
        \item for $\phi\geq 2\pi+\bar\theta$ the function solves
        \begin{equation*}
            \frac{d}{d\phi}r(\phi)=\cot\alpha r(\phi)-\frac{r(\phi-2\pi-\alpha)}{\sin\alpha}.
        \end{equation*}
    \end{itemize}
    
    Again, we compute the solution in the interval $\phi\in[2\pi+\bar\theta,4\pi+\alpha+\bar\theta]$ and the corresponding function $\rho(t)$ (see again Subsection \ref{sss:important}). We first observe that $\frac{\sin\bar\theta}{\sin\alpha}\geq 0$ and that $\frac{\sin\bar\theta}{\sin\alpha}e^{\cot\alpha(2\pi-\bar\theta+\alpha)}-1\geq 0$. Then we compute again
    \begin{equation*}
        \frac{d}{d\phi}r(\phi)e^{-c\phi}.
    \end{equation*}
    As in the previous discussion we call
    \begin{equation*}
        \kappa_1(\bar\theta)=\frac{\sin\bar\theta}{\sin\alpha};\qquad \kappa_2(\bar\theta)=\left(\kappa_1(\bar\theta)e^{\cot(\alpha)(2\pi-\bar\theta+\alpha)}-1\right);
    \end{equation*}
    \begin{equation*}
        \kappa_3(\bar\theta)=\kappa_2(\bar\theta)e^{\cot\alpha(\bar\theta)}-\frac{\sin(\bar\theta-\alpha)}{\sin\alpha}.
    \end{equation*}
    Here $\kappa_1,\kappa_2\geq 0$.
    In the interval $\phi\in [2\pi+\bar\theta+\alpha,4\pi+\alpha]$ one gets
        \begin{equation*}
            r(\phi)=\left(\kappa_3(\bar\theta)-\frac{\kappa_1(\bar\theta)}{\sin\alpha}(\phi-2\pi-\bar\theta)\right)e^{\cot\alpha(\phi-2\pi-\bar\theta)},
        \end{equation*}
        and calling 
        \begin{equation*}
            \kappa_4(\bar\theta)=r(4\pi+\alpha),
        \end{equation*}
        finally for $\phi\in[4\pi+\alpha,4\pi+\bar\theta+\alpha]$ one gets
        \begin{equation*}
    r(\phi)=\left(\kappa_4(\bar\theta)-\frac{\kappa_2(\bar\theta)}{\sin\alpha}(\phi-4\pi-\alpha)\right)e^{\cot\alpha(\phi-4\pi-\alpha)}.
        \end{equation*}
        We prove that both $\kappa_3,\kappa_4$ are positive. 
        
        \textbf{Computations for $\kappa_3$}
        We compute the second derivative of $\kappa_3$ and we find
        \begin{align*}
            \frac{d^2}{d\theta^2} \kappa_3&=-\frac{\sin\bar\theta}{\sin\alpha}e^{\cot\alpha(2\pi+\alpha)}-\cot^2\alpha e^{\cot\alpha\bar\theta}+\frac{\sin\bar\theta}{\sin\alpha}\\&\leq \frac{\sin\bar\theta}{\sin\alpha}(1-e^{\cot\alpha(2\pi+\alpha)})\leq 0.
        \end{align*}
        In particular the minimum is at the boundary (for $\bar\theta=\alpha$ or $\bar\theta=\frac{\pi}{2}$). One can easily prove that at both values $\kappa_3\geq 0$. 
        
        \textbf{Computations for $\kappa_4$}
         \begin{align*}
            \kappa_4&\geq\kappa_3-\frac{\kappa_1}{\sin\alpha}2\pi \\ & \geq \kappa_3(\alpha)-\frac{1}{\sin\alpha}2\pi\geq 0.
        \end{align*}
         
   Doing similar computations as in Theorem \ref{thm:div:arc} one finds that in order to conclude one has to prove the positivity of the two quantities
  \begin{equation*}
         Q'_3=\left(\kappa_3(\bar\theta,\theta_0)-\frac{\kappa_1(\bar\theta,\theta_0)}{\sin\alpha}\left((2\pi+\alpha)+(\phi-2\pi-\bar\theta)\right)\right)\llcorner_{\phi=4\pi+\alpha},
         \end{equation*}
 \begin{equation*}
         Q'_4=\left(\kappa_4(\bar\theta,\theta_0)-\frac{\kappa_2(\bar\theta,\theta_0)}{\sin\alpha}\left(2\pi+\alpha+(\phi-4\pi-\alpha)\right)\right)\llcorner_{\phi=4\pi+\alpha+\bar\theta},
         \end{equation*}
  which are still positive. The plots of the previous relevant quantities can be found in the Appendix Section

   Again, we compute the solution in the interval $\phi\in[2\pi+\bar\theta_a,4\pi+\alpha+\bar\theta_a]$ and the corresponding function $\rho(t)$ (see again Subsection \ref{sss:important}). We first observe that $\frac{\sin\bar\theta_a}{\sin\alpha}\geq 0$ and that $\frac{\sin\bar\theta_a}{\sin\alpha}e^{\cot\alpha(2\pi-\bar\theta_a+\alpha)}-1\geq 0$. Then we compute again
    \begin{equation*}
        \frac{d}{d\phi}r(\phi)e^{-c\phi}.
    \end{equation*}
    
    Here $\kappa_1,\kappa_2\geq 0$.
    In the interval $\phi\in [2\pi+\bar\theta_a+\alpha,4\pi+\alpha]$ one gets
        \begin{equation*}
            r(\phi)=\left(\kappa_3(\bar\theta_a)-\frac{\kappa_1(\bar\theta_a)}{\sin\alpha}(\phi-2\pi-\bar\theta_a)\right)e^{\cot\alpha(\phi-2\pi-\bar\theta_a)},
        \end{equation*}
        and calling 
        \begin{equation*}
            \kappa_4(\bar\theta_a)=r(4\pi+\alpha),
        \end{equation*}
        finally for $\phi\in[4\pi+\alpha,4\pi+\bar\theta_a+\alpha]$ one gets
        \begin{equation*}
    r(\phi)=\left(\kappa_4(\bar\theta_a)-\frac{\kappa_2(\bar\theta_a)}{\sin\alpha}(\phi-4\pi-\alpha)\right)e^{\cot\alpha(\phi-4\pi-\alpha)}.
        \end{equation*}
        We prove that both $\kappa_3,\kappa_4$ are positive. 
        
        \textbf{Computations for $\kappa_3$}
        We compute the second derivative of $\kappa_3$ and we find
        \begin{align*}
            \frac{d^2}{d\theta^2} \kappa_3&=-\frac{\sin\bar\theta_a}{\sin\alpha}e^{\cot\alpha(2\pi+\alpha)}-\cot^2\alpha e^{\cot\alpha\bar\theta_a}+\frac{\sin\bar\theta_a}{\sin\alpha}\\&\leq \frac{\sin\bar\theta_a}{\sin\alpha}(1-e^{\cot\alpha(2\pi+\alpha)})\leq 0.
        \end{align*}
        In particular the minimum is at the boundary (for $\bar\theta_a=\alpha$ or $\bar\theta_a=\frac{\pi}{2}$). One can easily prove that at both values $\kappa_3\geq 0$. 
        
        \textbf{Computations for $\kappa_4$}
         \begin{align*}
            \kappa_4&\geq\kappa_3-\frac{\kappa_1}{\sin\alpha}2\pi \\ & \geq \kappa_3(\alpha)-\frac{1}{\sin\alpha}2\pi\geq 0.
        \end{align*}
         
   Doing similar computations as in Theorem \ref{thm:div:arc} one finds that in order to conclude one has to prove the positivity of the two quantities
  \begin{equation*}
         Q'_3=\left(\kappa_3(\bar\theta_a,\theta_0)-\frac{\kappa_1(\bar\theta_a,\theta_0)}{\sin\alpha}\left((2\pi+\alpha)+(\phi-2\pi-\bar\theta_a)\right)\right)\llcorner_{\phi=4\pi+\alpha},
         \end{equation*}
 \begin{equation*}
         Q'_4=\left(\kappa_4(\bar\theta_a,\theta_0)-\frac{\kappa_2(\bar\theta_a,\theta_0)}{\sin\alpha}\left(2\pi+\alpha+(\phi-4\pi-\alpha)\right)\right)\llcorner_{\phi=4\pi+\alpha+\bar\theta_a},
         \end{equation*}
  which are still positive. The plots of the previous relevant quantities can be found in the Appendix Section
 \newpage
\subsection{Computations for the base case: segment}\label{s:base:segment}
This computations refer to Section \ref{s:base:segment}. The orange line corresponds to $y=0$.
\begin{figure}[H]
    \centering \includegraphics{basecasesegment_gr1.eps}
     \caption{Computations for the base case $f_0$ in the case of the segment: $\kappa_1$.}
\end{figure}

\begin{figure}[H]
    \centering 
    \includegraphics{basecasesegment_gr2.eps}
    \caption{Computations for the base case $f_0$ in the case of the segment: $\kappa_2$.}
\end{figure}
\begin{figure}[H]
    \centering \includegraphics{basecasesegment_gr3.eps}
     \caption{Computations for the base case $f_0$ in the case of the segment: $\kappa_3$.}
\end{figure}
\begin{figure}[H]
    \centering \includegraphics{basecasesegment_gr4.eps}
     \caption{Computations for the base case $f_0$ in the case of the segment: $\kappa_4$.}
\end{figure}
\begin{figure}[H]
    \centering \includegraphics{basecasesegment_gr5.eps}
     \caption{Computations for the base case $f_0$ in the case of the segment: $Q'_3$.}
\end{figure}
\begin{figure}[H]
    \centering \includegraphics{basecasesegment_gr6.eps}
    \caption{Computations for the base case $f_0$ in the case of the segment: $Q'_4$.}
\end{figure}


APPUNTI PAG 58 E SS
{\color{red} ma sei sicuro?}
{\color{red} quando calcolo l'espansione al primo ordine mi trovo
\begin{align*}
    \rho(\tau,\theta)=\left(-\frac{\sin\bar\alpha}{2\pi+\bar\alpha}-\frac{\cos\bar\alpha\theta}{2\pi+\bar\alpha}+\frac{\sin\bar\alpha\theta}{(2\pi+\bar\alpha)^2}\right)\left(e^{\tau-1}-\frac{e^{\tau-1}\theta}{2\pi+\bar\alpha}+\dots\right)+\left(\frac{\sin\bar\alpha}{2\pi+\bar\alpha}+\frac{\cos\bar\alpha}{2\pi+\bar\alpha}\theta\right)(e^{\tau-1}+\dots)=\frac{2\sin\bar\alpha\theta}{(2\pi+\bar\alpha)^2}e^{\tau-1}+\dots
\end{align*}
}

\begin{proposition}
    \label{Prop:tent_worst}
    The tent closure is the minimal solution.{\color{red} non lo scriverei così perchè potrebbe essere l'arco. Qui tenda potrebbe anche non essere ammissibile.}
\end{proposition}

\begin{proof}
We are in the case where the tent/arc is in the saturated region, {\color{red} in the sense that $\bar\phi-\phi_0-2\pi\geq \omega$ ?}. {\color{red}We assume that the minimal solution in the point $P^{-}$ is an arc of endpoints $P^{-}P_1$}.

We construct a path as follows: we connect the initial point $P^-$ of the final arc with another point $Q$ of the arc by a segment, then we follow the level set of the fire (arc) up to $P_1$ and then the segment of endpoints $P_1P_2$: we require that the last point $P_2$ is saturated. Such a solution is not a spiral because the initial segment is inside the level set of the fire, in particular it is not an admissible strategy (Figure \ref{fig:prop72}).
\begin{figure}
    \centering
    \includegraphics[scale=0.45]{prop72.png}
    \caption{In the point $P^{-}$ the arc solution starts. We replace it with the a segment of endpoints $P^{-},Q$ (red segment).}
    \label{fig:prop72}
\end{figure}

We compute now the derivative of this family of solutions as in the previous section. Using Equation \eqref{eq:sec6:imp} as a reference, and setting $0$ at the angle corresponding to the point $P_0$ we have that
\begin{equation*}
    \delta P_0 = r_0 \delta \phi_{P_0} e^{i\frac{\pi}{2}},
\end{equation*}
where we have indicated by $r_0=\tilde r(\phi_{P_0};s_0)$ {\color{red}(here, the point $P_0+\delta P_0$ is along the segment starting in $P_0$)}; {\color{blue} ma qui intendi invece $\delta P^{-}$ perchè se no non capisco};{\color{green} Finire di correggere domani!!}
moreover,
\begin{equation*}
    \delta Q = r_Q \delta \phi_Q e^{i(\delta\phi_Q + \frac{\pi}{2})}
\end{equation*}
(see as a reference Equation \eqref{eq:P:1:arc}) and 
\begin{equation*}
    \delta P_2 = \delta Q + \delta |P_2-Q| e^{i(\phi_Q + \frac{\pi}{2})} - |P_2-Q| \delta \phi_Q e^{i \phi_Q},
\end{equation*}
which holds similarly to Equation \eqref{eq:P:2:arc}. The saturation condition becomes 
\begin{align*}
    0 &= \delta P_2 \cdot e^{i(\phi_1 + \frac{\pi}{2} - \bar \alpha)} - \cos(\bar \alpha) \big( \delta \Delta P + r_1 \delta \phi_1 - h \big) \\
    &= (r_1 \delta \phi_1 + \delta \Delta P) \cos(\bar \alpha) - \Delta P \delta \phi_1 \sin(\bar \alpha) - \cos(\bar \alpha) \big( \delta \Delta P + r_1 \delta \phi_1 - h \big) \\
    &= - \Delta P \delta \phi_1 \sin(\bar \alpha) + \cos(\bar \alpha) h.
\end{align*}
{\color{blue} io mi trovo}
\begin{align*}
    0 &= \delta P_2 \cdot e^{i(\phi_1 {\color{red}\Delta\phi}+ \frac{\pi}{2} - \bar \alpha)} - \cos(\bar \alpha) \big( \delta \Delta P + r_1 \delta \phi_1 - h \big) \\
    &= (r_1 \delta \phi_1 + \delta \Delta P) \cos(\bar \alpha) - \Delta P \delta \phi_1 \sin(\bar \alpha) - \cos(\bar \alpha) \big( \delta \Delta P + r_1 \delta \phi_1 - h \big) \\
    &= - \Delta P \delta \phi_1 \sin(\bar \alpha) + \cos(\bar \alpha) h.
\end{align*}

\medskip

The final length is
\begin{equation*}
    \delta r_2 = - \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} h.
\end{equation*}
The variation at the final angle is hence (some geometric relations)
\begin{equation*}
    \delta r(\bar \phi) = \delta r_2 e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \theta)}, \quad h = 1 - \cos(\theta')....
\end{equation*}
The relation is linear and negative. Hence also for the derivative the relation is negative, so that by increasing the segment the length $\delta r(\bar \phi)$ decreases.

Hence we can prolong the segment up to the point that the arc disappears. In this case, we move the initial point up towards the angle $\hat \theta$: we have already proved that in this case the solution decreases.
\end{proof}

We thus have to study only the tent in the forth case.

The case $\bar \tau \in [0,1]$ (the tent is at $0$) is in the next section, the case $\bar \tau \in [1,2]$ (the tent is in $[0,1]$ and the base is at $0$) is in Section \ref{Ss:small_bar_phi}, the case $\bar \tau \geq 2$ is in Section \ref{Ss:phi_large_optimal}. For $\bar \phi \geq 3$ we can use the Lemma.





==> arc.tex <==
\subsection{Arc case}
\label{Ss:arc-arc}


This can happen only when the segment in the direction $\bar \phi$ is is the end points of an arc.


%\subsubsection{Segment-arc with $\bar \phi < \phi_0 + \bar \theta + 2\pi - \hat \theta$: see Fig. \ref{Fig:segm_arc_1}}
%\label{Sss:segm_arc_1}
%
%
%In this case $\check r = \tilde r$, and the optimality follows from the fact that we are outside the region $N_\mathrm{segm}$, as in the segment-segment case of Section \ref{Sss:segm-segm_low}.
%
%\begin{lemma}
%\label{Lem:segm_arc_1}
%If $\bar \phi \in \phi_0 + [\beta^-(\phi_0),\bar \theta + 2\pi - \hat \theta)$, then $\delta \check r(\bar \phi) \geq 0$.
%\end{lemma}
%
%Note that the angle between the level set and the direction $e^{\i \bar \phi}$ is increasing when we move from $P_0$ towards $\check \phi$, and then the arc case cannot be optimal here: indeed by Proposition \ref{Prop:unique_optimal_guess} the we are in the negativity zone for the derivative $\delta \tilde r(\bar \phi;s_0)$.


\subsubsection{Segment-arc or arc-arc with $\bar \phi \in \phi_0 + 2\pi + [\bar \theta - \theta,\bar \theta)$: see Fig. \ref{Fig:segm_arc_2}}
\label{Sss:segm_arc_2}


\begin{figure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_2.pdf_t}}
\caption{The geometric situation of Section \ref{Sss:segm_arc_2}.}
\label{Fig:segm_arc_2}
\end{subfigure}
\hfill
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_2_2.pdf_t}}
\caption{The geometry to compute the variations of the points in the arc case.}
\label{Fig:segm_arc_2_2}
\end{subfigure}
\end{figure}

Setting for simplicity $\bar \phi = 0$ and with $\theta$ the angle of the perturbation of the point $P_0$, the  variations of the positions of the points is (see Fig. \ref{Fig:segm_arc_2_2}):
\begin{equation*}
\delta P_0 = e^{- \i \theta}, \quad \delta \check P^- = \delta P_0 + \delta \check \ell_0 e^{\i 0}, \quad \delta \check \phi^- = \frac{\delta \check P^- \cdot e^{\i \check \theta}}{\check r(\check \phi^-)},
\end{equation*}
\begin{equation*}
\delta \check P_1 = \big[ \delta \check P^- \cdot e^{\i (\check \theta - \frac{\pi}{2})} \big] e^{\i (\check \theta + \Delta \check \phi - \frac{\pi}{2})} + \check r(\check \phi_1) \delta \check \phi_1 e^{\i (\check \theta + \Delta \check \phi)}, \quad \delta \check \phi_1 = \frac{\delta \check P^- \cdot e^{\i \check \theta}}{\check r(\check \phi^-)} + \delta \Delta \check \phi,
\end{equation*}
where the first term is the variation of the level set and the second is the variation of the angle along the level set,
\begin{equation*}
\delta \check P_2 = \delta \check P_1 + \delta \check \ell_1 e^{\i (\check \theta + \Delta \check \phi)} + \delta \check \phi_1 \check \ell_1 e^{i (\check \theta + \Delta \check \phi + \frac{\pi}{2})}.
\end{equation*}
The optimality condition requires by Lemma \ref{Lem:study_g_1_arc} that
\begin{equation*}
\check \theta = h_1(\Delta \check \phi), \quad \delta \check \theta = \delta \check \phi^- = \frac{dh_1(\Delta \check \phi)}{d\Delta \phi} \delta \Delta \check \phi,
\end{equation*}
and the saturation condition reads are
\begin{equation}
\label{Equa:segm_arc_2_satu}
\begin{split}
\delta \check P_2 \cdot e^{\i (\check \theta + \Delta \check \phi - \bar \alpha)} - \cos(\bar \alpha) \bigg( 1 + \delta \check \ell_0 - \check r(\check \phi^-) \delta \check \phi^- + \Delta \check \phi \big( \delta \check P^- \cdot e^{\i (\check \theta - \frac{\pi}{2})} \big) + \check r(\check \phi_1) \delta \check \phi_1 + \delta \check \ell_1 \bigg) & \\
\delta \check P_2 \cdot e^{\i (\check \theta + \Delta \check \phi - \frac{\pi}{2})} \sin(\bar \alpha) - \cos(\bar \alpha) \bigg( 1 + \delta \check \ell_0 - \check r(\check \phi^-) \delta \check \phi^- + \Delta \check \phi \big( \delta \check P^- \cdot e^{\i (\check \theta - \frac{\pi}{2})} \big) \bigg) &= 0.
\end{split}
\end{equation}
The final values is computed by
\begin{equation}
\label{Equa:segm_arc_2_final}
\begin{split}
\delta \hat r(\bar \phi) &= \frac{\delta \check P_2 \cdot e^{\i (\check \theta + \Delta \check \phi - \frac{\pi}{2})}}{\sin(\bar \alpha)} e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \check \theta - \Delta \check \phi)} - e^{\cot(\bar \alpha) \theta} - \delta \ell_0 \\
&= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \bigg( 1 + \delta \check \ell_0 - \big( \cos(\theta + \check \theta) + \delta \check \ell_0 \cos(\check \theta) \big) + \Delta \check \phi \big( \sin(\theta + \check \theta) + \delta \check \ell_0 \sin(\check \theta) \big) \bigg) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \check \theta - \Delta \check \phi)} - e^{\cot(\bar \alpha) \theta} - \delta \ell_0.
\end{split}
\end{equation}
Using \eqref{Equa:theta_Deltaphi_rel} we simplify into
\begin{equation*}
\begin{split}
\delta \hat r(\bar \phi) &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\theta + \check \theta) + \Delta \check \phi  \sin(\theta + \check \theta) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \check \theta - \Delta \check \phi)} - e^{\cot(\bar \alpha) \theta} \\
&= e^{\cot(\bar \alpha) \theta} \bigg( \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\theta + \check \theta) + \Delta \check \phi \sin(\theta + \check \theta) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - (\check \theta + \theta) - \Delta \check \phi)} - 1 \bigg),
\end{split}
\end{equation*}
which is $\geq 0$ unless $\theta = 0$ by Lemma \ref{Lem:study_g_1_arc}.

We thus have the following result.

\begin{lemma}
\label{Lem:segm_arc_2}
If $\bar \phi \in \phi_0 + 2\pi + [\bar \theta - \theta,\bar \theta)$, then $\delta \check r(\bar \phi) \geq 0$.
\end{lemma}


\subsubsection{Arc-arc with $\bar \phi \geq \phi_0 + 4\pi + \bar \alpha + \bar \theta, \bar \phi + \hat \theta + \Delta \phi \leq \phi_0 + 4\pi + \bar \alpha + \bar \theta - \theta$: see Fig. \ref{Fig:segm_arc_3}}
\label{Sss:segm_arc_3}


\begin{figure}
\resizebox{.75\textwidth}{!}{\input{segm_arc_3_bis.pdf_t}}
\caption{The geometric situation of Section \ref{Sss:segm_arc_3}.}
\label{Fig:segm_arc_3}
\end{figure}

We have
\begin{equation*}
\delta P_0 = e^{\i (\Delta \phi - \theta)}, \quad \delta \check P_0 = - \sin(\theta) e^{\i \frac{\pi}{2}},
\end{equation*}
\begin{equation*}
\delta \check P^- = \delta \ell_0 e^{\i 0} - \sin(\theta) e^{\i \frac{\pi}{2}}, \quad \delta \check P_1 = \check r_1 \delta \check \omega e^{\i \check \omega} +  \delta \check P^- \cdot e^{\i (\check \theta - \frac{\pi}{2})} e^{\i (\check \omega - \frac{\pi}{2})}
\end{equation*}
\begin{equation*}
\delta \check P_2 = \delta \check P_1 + \delta \check \ell_1 e^{\i \check \omega} - \check \ell_1 \delta \check \omega e^{\i (\check \omega - \frac{\pi}{2})}.
\end{equation*}
The saturation is
\begin{align*}
0 &= \delta \check P_2 \cdot e^{\i(\check \omega - \bar \alpha)} - \cos(\bar \alpha) \Big( (1 - \cos(\theta) + \sin(\theta) \Delta \phi) + \delta \check \ell_0 - \check r^- \delta \check \phi^- + \delta \check P^- \cdot e^{\i (\check \theta - \frac{\pi}{2})} \Delta \check \phi + \check r_1 \delta \check \phi_1 + \delta \ell_1 \Big) \\
&= \delta \check P_1 \cdot e^{\i (\check \omega - \bar \alpha)} - \check \ell_1 \delta \check \omega \sin(\bar \alpha) - \cos(\bar \alpha) \Big( (1 - \cos(\theta) + \sin(\theta) \Delta \phi) + \delta \check \ell_0 - \delta \check P^- \cdot e^{i \check \theta} + \delta \check P^- \cdot e^{\i (\check \theta - \frac{\pi}{2})} \Delta \check \phi + \delta \check P_1 \cdot e^{i \check \omega} \Big) \\
&= \delta \check P^- \cdot e^{\i (\check \theta - \frac{\pi}{2})} \sin(\bar \alpha) - \check \ell_1 \delta \check \omega \sin(\bar \alpha) \\
&\quad - \cos(\bar \alpha) \Big( (1 - \cos(\theta) + \sin(\theta) \Delta \phi) + \sin(\theta) \sin(\check \theta) + \sin(\theta) \cos(\check \theta) \Delta \check \phi + \delta \check \ell_0 (1 - \cos(\check \theta) + \sin(\check \theta) \Delta \check \phi \Big) \\
\end{align*}
The final value is
\begin{align*}
\delta \check r(\bar \phi) &= \frac{\delta \check P_2 \cdot e^{\i \check \omega - \frac{\pi}{2})}}{\sin(\bar \alpha)} e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \check \omega)} - e^{\cot(\bar \alpha)(\Delta \phi + \theta)} + \cos(\theta) e^{\cot(\bar \alpha) \Delta \phi} - \sin(\theta) \frac{e^{\cot(\bar \alpha) \Delta \phi} - 1}{\cot(\bar \alpha)} - \delta \check \ell_0 \\
&= \frac{\delta \check P^- \cdot e^{\i (\check \theta - \frac{\pi}{2})} - \check \ell_1 \delta \check \omega}{\sin(\bar \alpha)} e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \check \omega)} - e^{\cot(\bar \alpha)(\Delta \phi + \theta)} + \cos(\theta) e^{\cot(\bar \alpha) \Delta \phi} - \sin(\theta) \frac{e^{\cot(\bar \alpha) \Delta \phi} - 1}{\cot(\bar \alpha)} - \delta \check \ell_0 \\
&= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \check \omega)} \Big( (1 - \cos(\theta) + \sin(\theta) \Delta \phi) + \delta \check \ell_0 - \delta \check P^- \cdot e^{i \check \theta} + \delta \check P^- \cdot e^{\i (\check \theta - \frac{\pi}{2})} \Delta \check \phi\Big) \\
& \quad - e^{\cot(\bar \alpha)(\Delta \phi + \theta)} + \cos(\theta) e^{\cot(\bar \alpha) \Delta \phi} - \sin(\theta) \frac{e^{\cot(\bar \alpha) \Delta \phi} - 1}{\cot(\bar \alpha)} - \delta \check \ell_0 \\
&= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \check \omega)} \Big( (1 - \cos(\theta) + \sin(\theta) \Delta \phi) + \sin(\theta) \sin(\check \theta) + \sin(\theta) \cos(\check \theta) \Delta \check \phi + \delta \check \ell_0 (1 - \cos(\check \theta) + \sin(\check \theta) \Delta \check \phi) \Big) \\
& \quad - e^{\cot(\bar \alpha)(\Delta \phi + \theta)} + \cos(\theta) e^{\cot(\bar \alpha) \Delta \phi} - \sin(\theta) \frac{e^{\cot(\bar \alpha) \Delta \phi} - 1}{\cot(\bar \alpha)} - \delta \check \ell_0 \\
&= \frac{1 - \cos(\theta + \check \theta) + \sin(\theta + \check \theta) \Delta \check \phi + \sin(\theta) \Delta \phi}{1 - \cos(\check \theta) + \sin(\check \theta) \Delta \check \phi} - e^{\cot(\bar \alpha)(\Delta \phi + \theta)} + \cos(\theta) (e^{\cot(\bar \alpha) \Delta \phi} - 1) - \sin(\theta) \frac{e^{\cot(\bar \alpha) \Delta \phi} - 1}{\cot(\bar \alpha)} \\
&= \frac{1 - \cos(\theta + \check \theta) + \sin(\theta + \check \theta) \Delta \check \phi + \sin(\theta) \Delta \phi}{1 - \cos(\check \theta) + \sin(\check \theta) \Delta \check \phi} - e^{\cot(\bar \alpha)(\Delta \phi + \theta)} + \cos(\theta + \bar \alpha) \frac{e^{\cot(\bar \alpha) \Delta \phi} - 1}{\cos(\bar \alpha)}.
\end{align*}
The second derivative w.r.t. $\Delta \phi$ is
\begin{equation*}
\partial^2_{\Delta \phi} \delta \check r(\bar \phi) = - \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} e^{\cot(\bar \alpha)(\Delta \phi + \theta)} \big( \cos(\bar \alpha) -
\cos(\bar \alpha + \theta) e^{-\cot(\bar \alpha) \theta} \big) \leq 0,
\end{equation*}
so that the minimal values are for $\Delta \phi = 0 ,\tan(\bar \alpha)$. The first case corresponds to the previous section, while for $\Delta \phi = \tan(\bar \alpha)$ we plot the function and its $\theta$ derivative
\begin{equation}
\label{Equa:deriva_r_arcarc}
\partial_\theta \bigg[ 1 - \cos(\theta + \check \theta) + \sin(\theta + \check \theta) \Delta \check \phi + \sin(\theta) \tan(\bar \alpha) + (1 - \cos(\check \theta) + \sin(\check \theta) \Delta \check \phi) \bigg( - e^{1 + \cot(\bar \alpha)\theta} + \frac{\cos(\theta + \bar \alpha)}{\cos(\bar \alpha)}(e - 1) \bigg) \bigg]
\end{equation}
in a region containing the graph $\check \theta = h_1(\Delta \check \phi)$: the derivative is positive for $\theta \in [0,1]$, and the function is $0$ for $\theta = 0$ and positive for $\theta \in [1,\pi/2]$ (Fig. \ref{Fig:arcarc_2}).

\begin{figure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\includegraphics{arcarc_2_1.png}}
\caption{The $\theta$-derivative of \eqref{Equa:deriva_r_arcarc} for various values of $\theta \in [0,1]$.}
\label{Fig:arcarc_2_1}
\end{subfigure} \hfill
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\includegraphics{arcarc_2_2.png}}
\caption{The function of \eqref{Equa:deriva_r_arcarc} for various values of $\theta \in [1,\pi/2]$.}
\label{Fig:arcarc_2_2}
\end{subfigure}
\caption{In both figures, the orange set is the null function.}
\label{Fig:arcarc_2}
\end{figure}

\begin{lemma}
\label{Lem:segm_arc_3}
In the above case $\delta \check r(\bar \phi) \geq 0$.
\end{lemma}


\subsection{Arc-segment case}
\label{Ss:arc_segment}


The situation is when the initial closing set is an arc, and later it is a segment. This is the unique situation in the saturated region. There are several case depending on the position of the segment w.r.t. the arc.


\subsubsection{The tent starts inside the arc: Fig. \ref{Fig:arc_segm_1}}
\label{Sss:arc_segm_1}


\begin{figure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{arc_segm_1.pdf_t}}
\caption{The geometric situation of Section \ref{Sss:arc_segm_1}.}
\label{Fig:arc_segm_1}
\end{subfigure} \hfill
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\includegraphics{arc_segm_1.png}}
\caption{The plot of the function \eqref{Equa:arc_segm_1}.}
\label{Fig:arc_segm_1_1}
\end{subfigure}\end{figure}

In this case the analysis is the same as in the arc-arc case, by setting $\Delta \check \phi = 0$ and $\check \theta = \hat \theta$: as before we are left with the case $\Delta \phi = \tan(\bar \alpha)$, thus the final value is
\begin{align}
\label{Equa:arc_segm_1}
\delta \check r(\bar \phi) &= \frac{1 - \cos(\theta + \hat \theta) + \sin(\theta) \tan(\bar \alpha)}{1 - \cos(\hat \theta)} - e^{1 + \cot(\bar \alpha) \theta} + \frac{\cos(\theta + \bar \alpha)}{\cos(\bar \alpha)} (e-1).
\end{align}
The plot of this function is in Fig. \ref{Fig:arc_segm_1_1}.

\begin{lemma}
\label{Lem:arc_segm_1}
In the above situation the perturbation is positive.
\end{lemma}


\subsubsection{Arc-tent case in the saturated region}
\label{Sss:arc_tent_satur}


The 10 cases representing the relative positions of the arc angles and the tent are represented in Fig. \ref{Fig:arcarc_2}.

\begin{figure}
\resizebox{.75\textwidth}{!}{\input{arc_segm_2.pdf_t}}
\caption{The 10 possible relative positions of the arc and the tent in the saturated region: in green the number of the case considered in Section \ref{Sss:arc_tent_satur}.}
\label{Fig:arc_segm_2}
\end{figure}

We will use the tent formulas of Section \ref{Ss:comput_tent_new}.

\begin{description}
\item[Case 1] in this case $\hat Q = 0, \hat L = 0$, so that
\begin{equation*}
\hat \ell_0 = \delta \tilde r_0 \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
\begin{equation*}
\delta \hat r_2 - \delta \tilde r_2 = \delta \tilde r_0 \bigg( \frac{\cos(\bar \alpha) - \cos(\bar \alpha + \hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - e^{\\cot(\bar \alpha) \hat \theta)} > 0.00669 \delta \tilde r_0 > 0,
\end{equation*}
and we thus just estimate
\begin{align*}
\delta \hat r(\bar \phi) &= \big( \delta \hat r_2 - \delta \tilde r_2) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} + \delta \tilde r(\bar \phi) - \hat \ell_0 \\
&> \delta \tilde r(\bar \phi) - \delta \tilde r_0 \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}.
\end{align*}


\end{description}




\newpage


\subsection{Segment-arc case}
\label{Ss:segm_arc_1}


Because of the previous remark, we need to study this case only for $\bar \phi$ not in the saturated region.: this case cannot happen because either we are in the positive region or we are in the segment case. % \leq \phi_0 + \bar \theta + 4\pi + \bar \alpha$, i.e. $\bar \tau < 2$.




\begin{figure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_4.pdf_t}}
\caption{Section \ref{Sss:segm_arc_4}.}
\label{Fig:segm_arc_4}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_5.pdf_t}}
\caption{Section \ref{Sss:segm_arc_5}.}
\label{Fig:segm_arc_5}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_6.pdf_t}}
\caption{Section \ref{Sss:segm_arc_6}.}
\label{Fig:segm_arc_6}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_7.pdf_t}}
\caption{Section \ref{Sss:segm_arc_7}.}
\label{Fig:segm_arc_7}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_8.pdf_t}}
\caption{Section \ref{Sss:segm_arc_8}.}
\label{Fig:segm_arc_8}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_10.pdf_t}}
\caption{Section \ref{Sss:segm_arc_9}.}
\label{Fig:segm_arc_9}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_9.pdf_t}}
\caption{Section \ref{Sss:segm_arc_10}.}
\label{Fig:segm_arc_10}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_11.pdf_t}}
\caption{Section \ref{Sss:segm_arc_11}.}
\label{Fig:segm_arc_11}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_12.pdf_t}}
\caption{Section \ref{Sss:segm_arc_12}.}
\label{Fig:segm_arc_12}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_13.pdf_t}}
\caption{Section \ref{Sss:segm_arc_13}.}
\label{Fig:segm_arc_13}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_14.pdf_t}}
\caption{Section \ref{Sss:segm_arc_14}.}
\label{Fig:segm_arc_14}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_15.pdf_t}}
\caption{Section \ref{Sss:segm_arc_15}.}
\label{Fig:segm_arc_15}
\end{subfigure}
%\begin{subfigure}{.33\textwidth}
%\resizebox{\textwidth}{!}{\input{segm_arc_16.pdf_t}}
%\end{subfigure}
%\begin{subfigure}{.33\textwidth}
%\resizebox{\textwidth}{!}{\input{segm_arc_17.pdf_t}}
%\end{subfigure} \hfill
\end{figure}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_4}}
\label{Sss:segm_arc_4}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_5}}
\label{Sss:segm_arc_5}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_6}}
\label{Sss:segm_arc_6}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_7}}
\label{Sss:segm_arc_7}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_8}}
\label{Sss:segm_arc_8}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_9}}
\label{Sss:segm_arc_9}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_10}}
\label{Sss:segm_arc_10}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_11}}
\label{Sss:segm_arc_11}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_12}}
\label{Sss:segm_arc_12}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_13}}
\label{Sss:segm_arc_13}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_14}}
\label{Sss:segm_arc_14}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_15}}
\label{Sss:segm_arc_15}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_16}}
\label{Sss:segm_arc_16}



\begin{figure}
\resizebox{.5\textwidth}{!}{\input{segm_arc_17.pdf_t}}
\caption{Section \ref{Sss:segm_arc_16}.}
\label{Fig:segm_arc_16}
\end{figure}




\subsection{The arc starts at $\phi_0$ and ends with an arc}
\label{Ss:arc_to_arc}

{\it Probably this can be removed because we can assume it ends with a tent.}

In this case, the segment with direction $\bar \phi - 2\pi$ starts along the arc of the level set of the fastest saturated spiral $\tilde r(\phi;s_0)$: hence we have that the closing solution is made of a level set arc of opening $\Delta \phi^-$, a segment of length $\ell_0$, another arc of opening $\Delta \phi$, a final segment of length $\ell_1$ and a saturated spiral.

The perturbations are (see Fig. ??)
\begin{equation*}
    \delta P^{--} = \delta s_ 0e^{\i (\frac{\pi}{2} - \theta^-)},
\end{equation*}
\begin{equation*}
    \delta P^- = \delta s_0 \sin(\theta^-) e^{\i \Delta \phi^-} = h_0 e^{\i \Delta \phi^-}, \quad h_0 = \delta s \sin(\theta^-),
\end{equation*}
\begin{equation*}
    \delta P_0 = h_0 e^{- \Delta \phi^-} + \delta \ell_0 e^{\i (\Delta \phi^- + \frac{\pi}{2})},
\end{equation*}
%\begin{equation*}
%    \delta L^- = h_0 \Delta \phi^- + \delta \ell_0,
%\end{equation*}
\begin{equation*}
    \delta \phi_0 = \frac{\delta \ell_0 \cos(\theta) - h_0 \sin(\theta)}{r_0},
\end{equation*}
\begin{equation*}
    \delta P_1 = (\delta \ell_0 \sin(\theta) + h_0 \cos(\theta)) e^{\i \phi_1} + r_1 \delta \phi_1 e^{\i (\phi_1 + \frac{\pi}{2})} = h_1 e^{\i \phi_1} + r_1 \delta \phi_1 e^{\i (\phi_1 + \frac{\pi}{2})},
\end{equation*}
\begin{equation*}
     h_1 = \delta \ell_0 \sin(\theta) + h_0 \cos(\theta), \quad \phi_1 = \Delta \phi^- + \theta + \Delta \phi,
\end{equation*}
\begin{equation*}
    \delta P_2 = \delta P_1 + \delta \ell_1 e^{\i (\phi_1 + \frac{\pi}{2})} - \ell_1 \delta \phi_1 e^{\i \phi_1}.
\end{equation*}

The vector constraint is that
\begin{equation*}
    \delta r_2 e^{\i (\phi_1 + \frac{\pi}{2} - \bar \alpha)} - r_2 \delta \phi_1 e^{\i (\phi_1 - \bar \alpha)} = \delta P_2,
\end{equation*}
and projecting on $e^{\i (\phi_1 + \frac{\pi}{2} - \bar \alpha)}, e^{\i (\phi_1 - \bar \alpha)}$ we obtain
\begin{equation*}
    \delta r_2 = (\delta \ell_1 + r_1 \delta \phi_1) \cos(\bar \alpha) + (h_1 - \ell_1 \delta \phi_1) \sin(\bar \alpha), 
\end{equation*}
\begin{equation*}
    - r_2 \delta \phi_1 = - (\delta \ell_1 + r_1 \delta \phi_1) \sin(\bar \alpha) + (h_1 - \ell_1 \delta \phi_1) \cos(\bar \alpha).
\end{equation*}

The saturation condition is
\begin{align*}
    0 &= \delta r_2 - \cos(\bar \alpha) \big( \delta s (1 - \cos(\theta^-)) + h_0 \Delta \phi^- + \delta \ell_0 - r_0 \delta \phi_0 + h_1 \Delta \phi + r_1 \delta \phi_1 + \delta \ell_1 \big) \\
    &= (h_1 - \ell_1 \delta \phi_1) \sin(\bar \alpha) - \cos(\bar \alpha) \big( \delta s (1 - \cos(\theta^-)) + h_0 \Delta \phi^- + \delta \ell_0 - r_0 \delta \phi_0 + h_1 \Delta \phi \big),
\end{align*}
where we have used the first projection of the vector relation, and then we get
\begin{equation*}
    \ell_1 \delta \phi_1 = h_1 - \cot(\bar \alpha) \big( \delta s (1 - \cos(\theta^-)) + h_0 \Delta \phi^- + \delta \ell_0 - r_0 \delta \phi_0 + h_1 \Delta \phi \big).
\end{equation*}
The second vector relation reads as
\begin{align*}
    \delta \ell_1 + r_1 \delta \phi_1 - \frac{r_2 \delta \phi_1}{\sin(\bar \alpha)} = \cot(\bar \alpha) (h_1 - \ell_1 \delta \phi_1).
\end{align*}

The value of $\delta r_2(\phi_2+)$ is then initial data
\begin{align*}
    \delta r_2 - \cot(\bar \alpha) r_2 \delta \phi_1 = \frac{h_1 - \ell_1 \delta \phi_1}{\sin(\bar \alpha)} = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( \delta s (1 - \cos(\theta) + h_0 \Delta \phi^- + \delta \ell_0 - r_0 \delta \phi_0 + h_1 \Delta \phi \big).
\end{align*}
So far the functions depend on the angle $\theta^-$ and the length $\delta \ell_0$, and the quantities $\Delta \phi^-,\theta,\Delta \phi,r_0,r_1,r_2$ are parameters, given by the base solution $\tilde r(\phi_0)$.

Using the same approach as in the arc case, the solution is written as
\begin{align*}
    \delta r(\bar \phi + 2\pi) &= (\delta r_2 - \cot(\bar \alpha) r_2 \delta \phi_1) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \theta)} - e^{\cot(\bar \alpha)(\Delta \phi^- + \theta^-)} + \cos(\theta^-) e^{\cot(\bar \alpha) \Delta \phi^-} - \sin(\theta^-) \int_0^{\Delta \phi^-} e^{\cot(\bar \alpha)(\Delta \phi^- - \phi)} d\phi - \delta \ell_0 \\
    &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( \delta s (1 - \cos(\theta^-)) + h_0 \Delta \phi^- + \delta \ell_0 - r_0 \delta \phi_0 + h_1 \Delta \phi \big) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \theta)} \\
    &\quad - e^{\cot(\bar \alpha)(\Delta \phi^- + \theta^-)} + \cos(\theta^-) e^{\cot(\bar \alpha) \Delta \phi^-} - \sin(\theta^-) \frac{e^{\cot(\bar \alpha) \Delta \phi^-} - 1}{\cot(\bar \alpha)} - \delta \ell_0 \\
    &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big[ (1 - \cos(\theta^-)) + \sin(\theta^-) \Delta \phi^- + \delta \ell_0 - (\delta \ell_0 \cos(\theta) - \sin(\theta^-) \sin(\theta))  + \big( \delta \ell_0 \sin(\theta) \\
    & \quad \qquad \qquad + \sin(\theta^-) \cos(\theta) \big) \Delta \phi \big] e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \theta)} \\
    &\quad - e^{\cot(\bar \alpha)(\Delta \phi^- + \theta^-)} + \cos(\theta^-) e^{\cot(\bar \alpha) \Delta \phi^-} - \sin(\theta^-) \frac{e^{\cot(\bar \alpha) \Delta \phi^-} - 1}{\cot(\bar \alpha)} - \delta \ell_0 \\
    &= \delta \ell_0 \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) + \Delta \phi \sin(\theta)) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \theta)} - 1 \bigg] \\
    &\quad + \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)}\big[ (1 - \cos(\theta^-)) +  \sin(\theta^-) \big( \Delta \phi^- + \sin(\theta) + \cos(\theta) \Delta \phi \big) \big] e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \theta)} \\
    &\quad - e^{\cot(\bar \alpha)(\Delta \phi^- + \theta^-)} + \cos(\theta^-) e^{\cot(\bar \alpha) \Delta \phi^-} - \sin(\theta^-) \frac{e^{\cot(\bar \alpha) \Delta \phi^-} - 1}{\cot(\bar \alpha)}. 
\end{align*}
Recall that $\theta,\Delta \phi$ are related by being on the critical curve,
\begin{align*}
\frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\theta) + \sin(\theta) \Delta \phi \big) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \theta)} - 1 = 0,
\end{align*}
so that the perturbation becomes
\begin{align*}
    \delta r(\bar \phi + 2\pi)
    &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big[ (1 - \cos(\theta^-)) + \sin(\theta^-) \big( \Delta \phi^- + \sin(\theta) + \cos(\theta) \Delta \phi \big) \big] e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \theta)} \\
    &\quad - e^{\cot(\bar \alpha)(\Delta \phi^- + \theta^-)} + \cos(\theta^-) e^{\cot(\bar \alpha) \Delta \phi^-} - \sin(\theta^-) \frac{e^{\cot(\bar \alpha) \Delta \phi^-} - 1}{\cot(\bar \alpha)} \\
    &= \frac{1 - \cos(\theta^-) + \sin(\theta^-) (\Delta \phi^- + \sin(\theta) + \cos(\theta) \Delta \phi)}{1 - \cos(\theta) + \sin(\theta) \Delta \phi} \\
    & \quad - e^{\cot(\bar \alpha)(\Delta \phi^- + \theta^-)} + \cos(\theta^-) e^{\cot(\bar \alpha) \Delta \phi^-} - \sin(\theta^-) \frac{e^{\cot(\bar \alpha) \Delta \phi^-} - 1}{\cot(\bar \alpha)},
\end{align*}
with $\theta = \hat \theta(\Delta \phi)$ on the null curve.

Computing the derivative w.r.t. $\Delta \phi^-$ one gets
\begin{equation*}
    \partial_{\Delta \phi^-} \delta r_2(\bar \phi + 2\pi) = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \sin(\theta^-) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \theta)} - \cot(\bar \alpha) e^{\cot(\bar \alpha)(\Delta \phi^- + \theta^-)} + \cos(\theta^-) \cot(\bar \alpha) e^{\cot(\bar \alpha) \Delta \phi^-} - \sin(\theta^-) e^{\cot(\bar \alpha) \Delta \phi^-},
\end{equation*}
and numerically this derivative is larger than $0.935714 \theta$. Thus the worst case is for $\Delta \phi^- = 0$, which is the case segment-arc considered in Section \ref{Ss:tent_arc}.

%As in the previous section, the minimal value happens for $\Delta \phi = 0, \theta = \hat \theta$, so that
%\begin{align*}
%    \delta r(\bar \phi + 2\pi) &= \frac{\sin(\theta^-)(\Delta \phi^- + \sin(\hat \theta))}{1 - \cos(\hat \theta)} - e^{\cot(\bar \alpha)(\Delta \phi^- + \theta^-)} + \cos(\theta^-) e^{\cot(\bar \alpha) \Delta \phi^-} - \sin(\theta^-) \tan(\bar \alpha) (e^{\cot(\bar \alpha) \Delta \phi^-} - 1).
%\end{align*}
%Numerically one sees that the function is positive but at $\theta^- = 0$, where the expansion is
%
%\begin{equation*}
%    \delta r(\bar \phi) = \theta^- \bigg[ \frac{\Delta \phi^- + \sin(\hat \theta)}{1 - \cos(\hat \theta)} - \cot(\bar \alpha) e^{\cot(\bar \alpha) \Delta \phi^-} - \tan(\bar \alpha) (e^{\cot(\bar \alpha) \Delta \phi^-} - 1) \bigg] + \mathcal O((\theta^-)^2) \geq 3.45 \theta + \mathcal O((\theta^-)^2).
%\end{equation*}

\begin{lemma}
    \label{Lem:positive_deriva_arc_arc}
    Under the assumptions above, the perturbation is positive unless we follow the optimal solution.
\end{lemma}

\begin{comment}
    \subsubsection{Arc case with $\Delta \phi^- = 0$}
\label{Sss:arc_case_Delta_phi^-_0}


When we start in a part on the arc with an initial angle of $\Delta \phi^- = 0$, then the variations are
\begin{equation*}
    \delta P^{-} = \delta s e^{\i (\frac{\pi}{2} - \theta^-)}, \quad h_0 = \delta s \sin(\theta^-),
\end{equation*}
\begin{equation*}
    \delta P_0 = \delta P^- + \delta \ell_0 e^{\i \frac{\pi}{2})},
\end{equation*}
%\begin{equation*}
%    \delta L^- = h_0 \Delta \phi^- + \delta \ell_0,
%\end{equation*}
\begin{equation*}
    \delta \phi_0 = \frac{\delta \ell_0 \cos(\theta) + \delta s \cos(\theta + \theta^-)}{r_0},
\end{equation*}
\begin{equation*}
    \delta P_1 = (\delta \ell_0 \sin(\theta) + \delta s \sin(\theta + \theta^-)) e^{\i \phi_1} + r_1 \delta \phi_1 e^{\i (\phi_1 + \frac{\pi}{2})} = h_1 e^{\i \phi_1} + r_1 \delta \phi_1 e^{\i (\phi_1 + \frac{\pi}{2})},
\end{equation*}
\begin{equation*}
     h_1 = \delta \ell_0 \sin(\theta) + \delta s \sin(\theta + \theta^-), \quad \phi_1 = \theta + \Delta \phi,
\end{equation*}
\begin{equation*}
    \delta P_2 = \delta P_1 + \delta \Delta P e^{\i (\phi_1 + \frac{\pi}{2})} - \Delta P \delta \phi_! e^{\i \phi_1},
\end{equation*}
vector relation
\begin{equation*}
    \delta r_2 e^{\i (\phi_1 + \frac{\pi}{2} - \bar \alpha)} - r_2 \delta \phi_1 e^{\i (\phi_1 - \bar \alpha)} = \delta P_2,
\end{equation*}
\begin{equation*}
    \delta r_2 = (\delta \Delta P + r_1 \delta \phi_1) \cos(\bar \alpha) + (h_1 - \Delta P \delta \phi_1) \sin(\bar \alpha), 
\end{equation*}
\begin{equation*}
    - r_2 \delta \phi_1 = - (\delta \Delta P + r_1 \delta \phi_1) \sin(\bar \alpha) + (h_1 - \Delta P \delta \phi_1) \cos(\bar \alpha),
\end{equation*}
saturation
\begin{align*}
    0 &= \delta r_2 - \cos(\bar \alpha) \big( \delta s + \delta \ell_0 - r_0 \delta \phi_0 + h_1 \Delta \phi + r_1 \delta \phi_1 + \delta \Delta P \big) \\
    &= (h_1 - \Delta P \delta \phi_1) \sin(\bar \alpha) - \cos(\bar \alpha) \big( \delta s + \delta \ell_0 - r_0 \delta \phi_0 + h_1 \Delta \phi \big),
\end{align*}
\begin{equation*}
    \Delta P \delta \phi_1 = h_1 - \cot(\bar \alpha) \big( \delta s + \delta \ell_0 - r_0 \delta \phi_0 + h_1 \Delta \phi \big),
\end{equation*}
\begin{align*}
    \delta \Delta P + r_1 \delta \phi_1 - \frac{r_2 \delta \phi_1}{\sin(\bar \alpha)} = \cot(\bar \alpha) (h_1 - \Delta P \delta \phi_1),
\end{align*}
initial data
\begin{align*}
    \delta r_2 - \cot(\bar \alpha) r_2 \delta \phi_1 = \frac{h_1 - \Delta P \delta \phi_1}{\sin(\bar \alpha)} = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 + \delta \ell_0 - r_0 \delta \phi_0 + h_1 \Delta \phi \big).
\end{align*}

The solution is written as
\begin{align*}
    \delta \bar r &= \delta r_2 e^{\cot(\bar \alpha) (2 \pi + \bar \alpha - \Delta \phi - \theta)} - e^{\cot(\bar \alpha) \theta^-} - (\cos(\theta^-) + \delta \ell_0) \\
    &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 + \delta \ell_0 - (\delta \ell_0 \cos(\theta^-) + \cos(\theta + \theta^-)) + (\delta \ell_0 \sin(\theta) + \sin(\theta + \theta^-)) \Delta \phi \big) e^{\cot(\bar \alpha) (2 \pi + \bar \alpha - \Delta \phi - \theta)} \\
    & \quad - e^{\cot(\bar \alpha) \theta^-} - (\cos(\theta^-) + \delta \ell_0).
\end{align*}
The derivative w.r.t. $\delta \ell_0$ is
\begin{align*}
    \partial_{\delta \ell_0} \delta \bar r &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\theta) + \sin(\theta) \Delta \phi \big) e^{\cot(\bar \alpha) (2 \pi + \bar \alpha - \Delta \phi - \theta)} - 1 = 0
\end{align*}
by criticality so that
\begin{align*}
    \delta \bar r &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\theta + \theta^-) + \sin(\theta + \theta^-) \Delta \phi \big) e^{\cot(\bar \alpha) (2 \pi + \bar \alpha - \Delta \phi - \theta)} - e^{\cot(\bar \alpha) \theta^-} - \cos(\theta^-) \\
    &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\theta^-) + \sin(\theta^-) (\sin(\theta) + \cos(\theta) \Delta \phi) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta - \theta)} - e^{\cot(\bar \alpha) \theta^-},
\end{align*}
where we used the criticality again.

Differentiating w.r.t. $\theta^-$
\begin{align*}
    \partial_{\theta^-} \bar r &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( \sin(\theta^-) + \cos(\theta^-) (\sin(\theta) + \cos(\theta) \Delta \phi) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta - \theta)} - \cot(\bar \alpha) e^{\cot(\bar \alpha) \theta^-} \\
    &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \Big[ \big( \sin(\theta^-) + \cos(\theta^-) (\sin(\theta) + \cos(\theta) \Delta \phi) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta - \theta)} - \sin(\bar \alpha) e^{\cot(\bar \alpha) \theta^-} \Big].
\end{align*}
The minimal value of
\begin{equation*}
    \sin(\theta) + \cos(\theta) \Delta \phi \geq \sin(\hat \theta)
\end{equation*}
on the critical curve, and numerically one obtains that the derivative is positive.

Thus the minimum is for $\theta^- = 0$, where the solution is $0$.


\subsubsection{Arc with final tent}
\label{Sss:arc_final_tent}


The last remaining case is when we have an arc but the optimal closing solution is a tent.

\begin{equation*}
    \delta P^{--} = \delta s e^{\i (\frac{\pi}{2} - \theta^-)},
\end{equation*}
\begin{equation*}
    \delta P^- = \delta s \sin(\theta^-) e^{\i \Delta \phi^-} = h_0 e^{\i \Delta \phi^-}, \quad h_0 = \delta s \sin(\theta^-),
\end{equation*}
\begin{equation*}
    \delta P_0 = h_0 e^{\i \Delta \phi^-} + \delta \ell_0 e^{\i (\Delta \phi^- + \frac{\pi}{2})}, \quad \bar \theta = \Delta \phi^- + \frac{\pi}{2},
\end{equation*}
%\begin{equation*}
%    \delta L^- = h_0 \Delta \phi^- + \delta \ell_0,
%\end{equation*}
%\begin{equation*}
%    \delta \phi_0 = \frac{\delta \ell_0 \cos(\theta) - h_0 \sin(\theta)}{r_0},
%\end{equation*}
\begin{equation*}
    \delta P_2 = \delta P_0 + \delta \Delta P e^{\i (\Delta \phi^- + \frac{\pi}{2} + \hat \theta)},
\end{equation*}
vector relation
\begin{equation*}
    \delta r_2 e^{\i (\Delta \phi^- + \frac{\pi}{2} + \hat \theta - \bar \alpha)} = \delta P_2,
\end{equation*}
\begin{equation*}
    \delta r_2 = \delta \Delta P \cos(\bar \alpha) + \delta \ell_0 \cos(\bar \alpha - \hat \theta) + h_0 \sin(\bar \alpha - \hat \theta), 
\end{equation*}
\begin{equation*}
    0 = - \delta \Delta P \sin(\bar \alpha) - \delta \ell_0 \sin(\bar \alpha - \hat \theta) + h_0 \cos(\bar \alpha - \hat \theta),
\end{equation*}
saturation
\begin{align*}
    0 &= \delta r_2 - \cos(\bar \alpha) \big( \delta s + h_0 \Delta \phi^- - \delta s \sin(\theta^-) + \delta \ell_0 + \delta \Delta P \big) \\
    &= \delta \ell_0 (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)) - \cos(\bar \alpha) (1 - \cos(\theta^-)) + h_0 (\sin(\bar \alpha - \hat \theta) - \cos(\bar \alpha) \Delta \phi^-),
\end{align*}
\begin{align*}
    \delta \ell_0 &= \frac{\cos(\bar \alpha) (1 - \cos(\theta^-)) - \sin(\theta^-) (\sin(\bar \alpha - \hat \theta) - \cos(\bar \alpha) \Delta \phi^-)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
    &= \cos(\theta^-) + \frac{\sin(\theta^-) \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \Delta \phi^- - \frac{\cos(\bar \alpha - \hat \theta - \theta^-) - \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{align*}
\begin{align*}
    \delta \Delta P = \frac{...}{\sin(\bar \alpha)},
\end{align*}
initial data
\begin{align*}
    \delta r_2 &= \delta \ell_0 (\cos(\bar \alpha - \hat \theta) - \cot(\bar \alpha) \sin(\bar \alpha - \hat \theta)) + h_0 (\sin(\bar \alpha - \hat \theta) + \cot(\bar \alpha) \cos(\bar \alpha - \hat \theta)) \\
    &= \frac{\delta \ell_0 \sin(\hat \theta)}{\sin(\bar \alpha)} + \frac{\sin(\theta^-) \cos(\hat \theta)}{\sin(\bar \alpha)}.
\end{align*}

Hence
\begin{align*}
    \delta \bar r &= \delta r_2 e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} - e^{\cot(\bar \alpha)(\Delta \phi^- + \theta-} + \cos(\theta) e^{\cot(\bar \alpha) \Delta \phi^-} - \sin(\theta)  \tan(\bar \alpha) (e^{\cot(\bar \alpha) \Delta \phi^-} - 1) - \delta \ell_0.
\end{align*}
This functions depends only on $\theta^-,\Delta \phi^-$.

Taking the derivative w.r.t. $\Delta \phi^-$ we obtain
\begin{align*}
    \partial_{\Delta \phi^-} \bar r &= \frac{\cot(\bar \alpha) \sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \sin(\theta^-) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} - \cot(\bar \alpha) e^{\cot(\bar \alpha) (\Delta \phi^- + \theta^-)} \\
    &\quad + \cot(\bar \alpha) \cos(\theta^-) e^{\cot(\bar \alpha) \Delta \phi^-} - \sin(\theta^-) e^{\cot(\bar \alpha) \Delta \phi^-} - \frac{\cos(\bar \alpha) \sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \sin(\theta^-),
\end{align*}
\begin{align*}
    \partial^2_{\Delta \phi^-} \bar r &= - \cot(\bar \alpha)^2 e^{\cot(\bar \alpha) (\Delta \phi^- + \theta^-)} + \cot(\bar \alpha)^2 \cos(\theta^-) e^{\cot(\bar \alpha) \Delta \phi^-} - \cot(\bar \alpha) \sin(\theta^-) e^{\cot(\bar \alpha) \Delta \phi^-} \\
    &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} e^{\cot(\bar \alpha) \Delta \phi^-} \big( - \cos(\bar \alpha) e^{\cot(\bar \alpha) \theta^-} + \cos(\bar \alpha + \theta^-) \big),
\end{align*}
which is negative. Hence the minima are for $\Delta \phi^- = 0,\tan(\bar \alpha)$.




\newpage








We have
\begin{equation*}
    \delta \omega = \frac{\cot(\bar \alpha)}{|P_2 - P_1} \bigg( \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha) + \theta \cos(\bar \alpha) \sin(\theta)}{\sin(\bar \alpha)} - \omega \sin(\theta) \bigg), \quad \delta \theta = \frac{\sin(\theta)}{r_0},
\end{equation*}
so that
\begin{equation*}
    \frac{\delta \omega}{\delta \theta} = \frac{\cot(\bar \alpha) r_0}{|P_2 - P_1} \bigg( \frac{\frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\theta)} + \theta \cos(\bar \alpha)}{\sin(\bar \alpha)} - \omega \bigg).
\end{equation*}
This should be equal (up to a sign) to
\begin{equation*}
    \frac{d\omega}{d\hat \theta} = - \frac{\cot(\bar \alpha) r_0}{\Delta P} \frac{\cot(\bar \alpha) + \omega}{\frac{\delta \omega}{\delta \theta}}.
\end{equation*}
We thus obtain





\newpage

{\color{gray}

\subsection{Perturbations in the saturated region}


We assume that in the saturated region of $\tilde r(\phi,\phi_0)$ the solution is a tent: we compute then the perturbation.

For angles
\begin{equation*}
    \phi \leq \bar \phi - 2\pi - \bar \alpha,
\end{equation*}
the solution is equal to the previous $\tilde r$, for angle
\begin{equation*}
    \bar \phi - 2\pi - \bar \alpha \leq \phi \leq \bar \phi - 2\pi - \bar \alpha + \hat \theta
\end{equation*}
the solution is a tent (determined by the saturation condition), and for angles
\begin{equation*}
    \bar \phi - 2\pi - \bar \alpha + \hat \theta \leq \phi \leq \bar \phi
\end{equation*}
the solution is the saturated spiral.


\subsubsection{Computation for the tent - perturbation}
\label{Sss:tent_perturbation}


We denote with a check the points, angles, lengths of the tent.


Since the angles are fixed, then for the tent the variation is:
\begin{itemize}
    \item the initial point
    \begin{equation*}
        \check P_0 + \delta \check P_0 = \check P_0 + \delta \tilde r(\check \phi_0) e^{\i \check \phi_0}
    \end{equation*}
    \item the intermediate point
    \begin{equation*}
        \delta \check P_1 = \delta \check P_0 + \delta \check \ell_1 e^{\i (\check \phi_0 + \bar \alpha)}
    \end{equation*}
    \item the final point
    \begin{equation*}
        \delta \check P_2 = \delta \check P_1 + \delta \check \ell_2 e^{\i (\phi_0 + \bar \alpha + \hat \theta)}
    \end{equation*}
    \item the variation of length
    $$
    \delta \check L = \int_{\check \phi_0}^{\check \phi_2} d\delta s^-
    $$
\end{itemize}
The initial quantity $\delta \check P_0$ is known.

The saturation gives
\begin{align*}
    0 &= \delta \check L + e^{\i (\phi_0 + \hat \theta)} \cdot \delta \check P_2 - e^{\i \phi_0} \cdot \delta \check P_0 - \cos(\bar \alpha) \big( \delta \check \ell_1 + \delta \check \ell_2 \big) \\
    &= \delta \check L + \delta \tilde r(\check \phi_0) (\cos(\hat \theta) - 1) + (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)) \delta \check \ell_1,
\end{align*}
and the angle condition
\begin{align*}
    0 &= e^{\i (\phi_0 + \hat \theta + \frac{\pi}{2}} \cdot \delta P_2 \\
    &= - \delta \tilde r(\check \phi_0) \sin(\hat \theta) + \delta \check \ell_1 \sin(\bar \alpha - \hat \theta) + \delta \ell_2 \sin(\bar \alpha). 
\end{align*}
These are the same conditions for the free spiral. {\bf OF COURSE, THE CONDITIONS ARE LINEAR! QUESTO DOVREBBE IN QUALCHE MODO IMPLICARE CHE LA SOLUZIONE E' LA TENDA E NON UN PEZZO DI ARCO}

\begin{lemma}
    \label{Lem:condit_prt_tent}
    The perturbation of the optimal solution in the saturated region is the same as the free solution with the initial data for $\delta \tilde r$.
\end{lemma}

The value of the perturbation at the angle $\bar \phi$ is estimated as
\begin{align*}
    \delta \check r(\bar \phi) &= \delta \check r(\bar \phi-) - \delta \check \ell_0 \\
    &\geq \delta \tilde r(\bar \phi) - \delta \tilde r(\phi_0) (1 - \cos(\hat \theta)).
\end{align*}
In the region where $\delta \tilde r$ is increasing, it follows that this quantity is positive. 




\newpage


\subsubsection{The second round - tent perturbation}
\label{Sss:second_round_tent}


Here we expect that the condition are for a tent configuration and that the positivity holds the same. {\bf DAVERIFICARE A PARTE}

\newpage


\subsection{The basic computation - first round}
\label{Sss:first_round_pert}


We assume that we are in the situation where, setting $P_{-1}$ as the initial point at angle $\phi_{-1} = 0$ where the tent starts, we have
\begin{equation*}
    0 \leq \bar \phi - 2\pi \leq \bar \theta_{-1},
\end{equation*}
with $\bar \theta_{-1} = \frac{\pi}{2}$ in the arc case.

The initial perturbation occurs in the point $P_{-1}$ for an infinitesimal length $\delta s_{-1}$ at an angle $\theta_{-1}$
\begin{equation*}
    \delta P_{-1} = \delta s_{-1} e^{\i \theta_{-1}}.
\end{equation*}
We observe that the monotonicity assumption implies that
\begin{equation*}
    0 \leq \theta_{-1},
\end{equation*}
while the convexity assumption gives
\begin{equation*}
    \theta_{-1} \leq \bar \phi - 2\pi.
\end{equation*}
If $\theta_{-1} \in [\bar \phi - 2\pi, \frac{\pi}{2}]$, then the fastest closing solution is the optimal solution which is positive: this case is a subset of what follows when $\ell_0 = 0$.

Form $P_{-1}$ we then follow a segment of direction $\bar \phi$ for a length $\ell_0$, corresponding to the angle $\phi_0$ and a point $P_0$ where the fastest closing solution occurs:
\begin{equation*}
    \delta P_0 = \delta P_{-1} + \delta \ell_0 e^{\i \bar \phi}.
\end{equation*}

Next, we can apply the computations for the segment/arc case for the perturbation of the point $P_0$: the new perturbation in the base of $P_0$ is
\begin{equation*}
    \delta P_0 = \delta s_0 e^{\i (\theta_{-1} - \phi_0)} + \delta \ell_0 e^{\i (\bar \phi - \phi_0)}. 
\end{equation*}


\subsubsection{Segment case - tent}
\label{Sss:tent_segment}


The segment case is when the fastest closing solution is a segment: in this case we can apply the previous computations for the perturbation above, obtaining that at the angle $\bar \phi$ the solution is
\begin{align*}
    \delta r(\bar \phi) &= \delta s_0 \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\bar \theta + \bar \phi - \theta_{-1}) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - (\bar \theta + \bar \phi - \theta_{-1}))} - 1 \bigg] e^{\cot(\bar \alpha) (\bar \phi - \theta_{-1})} \\
    & \quad + \delta \ell_0 \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\bar \theta) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \bar \theta)} - 1 \bigg].
\end{align*}
The perturbation are considered independent.

In order to have that the length is the optimal one, we require that the length $\ell_0$ is such that
\begin{equation*}
    \bar \theta = \hat \theta.
\end{equation*}
In this case the last term has derivative $0$, and it is actually a minimum being the only $0$. It is not possible, this means that $\bar \phi < \bar \theta_{-1} - \hat \theta$, and then $\ell_0 = 0$ and the fastest closing solution is already positive.

For such a choice of $\bar \theta$, the angle
\begin{equation*}
    \hat \theta \leq \hat \theta + \bar \phi - \theta_{-1} \leq \hat \theta + \bar \theta - \hat \theta \leq \frac{\pi}{2},
\end{equation*}
and the computation for the segment gives that the first term is positive unless $\delta s_0 = 0$: this under the assumption that $\delta s_0 \geq 0$, while for $\delta \ell_0$ no assumptions on the sign.


\subsubsection{The arc case - tent}
\label{Sss:arc_case_tent}


Here the fastest closing solution at $P_0$ is an arc. We use the same computations of the arc case obtaining
\begin{equation*}
    \omega = \frac{\pi}{2} - \bar \phi + \phi_0,
\end{equation*}
\begin{align*}
    \delta r(\bar \phi) &= \delta s_0 \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\omega + \bar \phi - \theta_{-1}) + \Delta \phi \sin(\omega + \bar \phi - \theta_{-1} \big) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \omega - \bar \phi + \theta_{-1})} - 1 \bigg] e^{\cot(\bar \alpha)(\bar \phi - \theta_{-1}} \\
    &\quad + \delta \ell_0 \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\omega) + \Delta \phi \sin(\omega) \big) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \omega)} - 1 \bigg]. 
\end{align*}
For the second one we choose {\bf to be proved!} the angle such that it is the unique point with $0$ derivative, and it is a single point minimum. Since as before $\bar \phi - \theta_{-1} \geq 0$, it follows that the derivative is positive unless $\delta s_0 = 0$.

}


\newpage


\end{comment}


\subsection{Formulas for the tent}
\label{Ss:comput_tent}
%
%
%In order to study the correction to the fastest saturated spiral after the angle $\phi_2$ (which is a segment of direction $\bar \phi - 2\pi$ up to a the critical angle, followed by the fastest saturated spiral for the last round), we need to study some geometric relations among the length $\ell_0$ of this segment and the underlying spiral $\tilde r$.
%
%This section is thus devoted to obtain these formulas assuming that the perturbation to $\tilde r$ is a tent, i.e. it is made of two segments with angle $\hat \theta$. The construction depends on the following quantities
%\begin{itemize}
%    \item entrance ray $\hat r_0$ at angle $0$ initial position $Q_0$,
%    \item exit ray $\hat r_2$ at angle $\hat \theta$ initial position $Q_2$,
%    \item length of segments $\hat \ell_0,\hat \ell_1$,
%    \item length of spiral at the base $\hat L$.
%\end{itemize}
%We need also to verify that it is admissible, which means that the angle of the ray at the endpoint of $\hat 
%\ell_0$ is $\leq \frac{\pi}{2}$. The input quantities are $\hat r_0$, $Q_2 - Q_1$, $\hat L$.
%
%The saturation assumptions is
%\begin{equation*}
%    \hat r_2 + L - \hat r_0 - \cos(\bar \alpha) (\hat \ell_0 + \hat \ell_1) = 0,
%\end{equation*}
%the vector condition is
%\begin{equation*}
%    Q_0 + \hat r_0 e^{\i 0} + \hat \ell_0 e^{\i \bar \alpha} + \hat \ell_1 e^{\i (\bar \alpha + \hat \theta)} = Q_2 + \hat r_2 e^{\i \hat \theta}.
%\end{equation*}
%
%Projecting the second equation in the direction $e^{\i \hat \theta}$ we obtain
%\begin{equation*}
%    (Q_2 - Q_0) \cdot e^{\i \hat \theta} + \hat r_2 - \hat \ell_1 \cos(\bar \alpha) - \hat \ell_0 \cos(\bar \alpha - \hat \theta) - \hat r_0 \cos(\hat \theta) = 0,
%\end{equation*}
%and then
%\begin{equation*}
%    (Q_2 - Q_1) \cdot e^{\i \hat \theta} - \hat \ell_0 \cos(\bar \alpha - \hat \theta) - \hat r_0 \cos(\hat \theta) = L - \hat r_0 - \cos(\bar \alpha) \hat \ell_0,
%\end{equation*}
%\begin{align*}
%    \hat \ell_0 &= \frac{(Q_2 - Q_1) \cdot e^{\i \hat \theta} - L + \hat r_0 (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
%    &= 2.50013((Q_2 - Q_0) \cdot e^{\i \hat \theta} - L) + .313453 \hat r_0.
%\end{align*}
%Projecting on the direction $e^{\i (\alpha + \hat \theta - \frac{\pi}{2})}$
%\begin{equation*}
%    (Q_2 - Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})} + \hat r_2 \sin(\bar \alpha) - \hat \ell_0 \sin(\hat \theta) - \hat r_0 \sin(\bar \alpha + \hat \theta) = 0,
%\end{equation*}
%\begin{equation*}
%    \hat r_2 = \frac{\hat r_0 \sin(\bar \alpha + \hat \theta) + \hat \ell_0 \sin(\hat \theta) - (Q_2 - Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha)},
%\end{equation*}
%\begin{align*}
%    \hat r_2 &= \frac{\hat r_0}{\sin(\bar \alpha)} \bigg( \sin(\bar \alpha + \hat \theta) + \frac{\sin(\hat \theta) (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg) - \frac{L}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
%    &\quad + \frac{(Q_2 - Q_1) \cdot e^{\i \hat \theta}}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - \frac{(Q_2 - Q_1) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha)} \\
%    &= \hat r_0 \frac{\cos(\bar \alpha) - \cos(\bar \alpha + \hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + \frac{(Q_2 - Q_1) \cdot e^{\i \hat \theta} - L}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - \frac{(Q_2 - Q_1) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha)} \\
%    &= 1.23979 \hat r_0 + 1.31181 ((Q_2 - Q_0) \cdot e^{\i \hat \theta} - L) - 1.0823 (Q_2 - Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}, 
%\end{align*}
%\begin{equation*}
%    \hat \ell_1 = \frac{\hat r_2 + L -\hat r_0 - \cos(\bar \alpha) \hat \ell_0}{\cos(\bar \alpha)},
%\end{equation*}
%\begin{align*}
%    \hat \ell_1 &= \frac{\hat r_0}{\cos(\bar \alpha)} \bigg[ \frac{1}{\sin(\bar \alpha)} \bigg( \sin(\bar \alpha + \hat \theta) + \frac{\sin(\hat \theta) (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg) - 1 - \cos(\bar \alpha) \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] \\
%    &\quad + \frac{L}{\cos(\bar \alpha)} \bigg[ - \frac{L}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + 1 + \frac{\cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] \\
%    &\quad + \frac{(Q_2 - Q_1) \cdot e^{\i \hat \theta}}{\cos(\bar \alpha)} \bigg[ \frac{1}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - \frac{\cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] \\
%    &\quad - \frac{(Q_2 - Q_1) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha) \cos(\bar \alpha)} \\
%    &= \hat r_0 \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + \frac{L}{\cos(\bar \alpha)} \\
%    &\quad +  \frac{(Q_2 - Q_0) \cdot e^{\i \hat \theta} - L}{\cos(\bar \alpha)} \bigg[ \frac{1}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} -\frac{\cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] - \frac{(Q_2 - Q_1) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha) \cos(\bar \alpha)} \\
%    &= 0.313453 \hat r_0 + 2.61433 L +  0.929517 ((Q_2 - Q_0) \cdot e^{\i \hat \theta} - L) - 2.8296 (Q_2 - Q_1) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}.
%\end{align*}
%
%For convex curves we can write
%\begin{equation*}
%    \frac{d \dot \zeta}{d\theta} = \dot \zeta^\perp, \quad \dot \zeta = e^{\i \theta_0},
%\end{equation*}
%so that
%\begin{equation*}
%    \dot \zeta = e^{\i \theta},
%\end{equation*}
%and then
%\begin{equation*}
%    \frac{d\zeta}{d\theta} = e^{\i \theta} R(\theta), 
%\end{equation*}
%\begin{equation*}
%    \zeta(\theta) - \zeta(\theta_0) = \int_{\theta_0}^{\theta} e^{\i \theta} R(\theta) d\theta.
%\end{equation*}
%The above formula holds also when the curvature is $\infty$, by using the formula $ds = R d\theta$.
%
%We obtain
%
%\begin{lemma}
%    \label{Lem:relation_admissibility_tent}
%    Under the assumptions above the following linear formulas hold for the tent:
%    \begin{equation*}
%        \Delta Q \cdot e^{\i \hat \theta} = \int_0^{\hat \theta} \cos(\hat \theta - \omega) R(\omega) d\omega,
%    \end{equation*}
%    \begin{equation*}
%        L = \int_0^{\hat \theta} R(\theta) d\theta,
%    \end{equation*}
%\begin{equation*}
%    \hat \ell_0 = \frac{\Delta Q \cos(\hat \theta - \omega) - L + \hat r_0 (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}.
%\end{equation*}
%\begin{align*}
%    \hat r_2 &= \frac{\hat r_0}{\sin(\bar \alpha)} \bigg( \sin(\bar \alpha + \hat \theta) + \frac{\sin(\hat \theta) (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg) - \frac{L}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
%    &\quad + \frac{\Delta Q \cos(\hat \theta - \omega)}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - \frac{\Delta Q \sin(\bar \alpha + \hat \theta - \omega)}{\sin(\bar \alpha)},
%\end{align*}
%\begin{align*}
%    \hat \ell_1 &= \frac{\hat r_0}{\cos(\bar \alpha)} \bigg[ \frac{1}{\sin(\bar \alpha)} \bigg( \sin(\bar \alpha + \hat \theta) + \frac{\sin(\hat \theta) (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg) - 1 - \cos(\bar \alpha) \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] \\
%    &\quad + \frac{L}{\cos(\bar \alpha)} \bigg[ \frac{L}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + 1 + \frac{\cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] \\
%    &\quad + \frac{\Delta Q \cos(\hat \theta-\omega)}{\cos(\bar \alpha)} \bigg[ \frac{1}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - \frac{\cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] \\
%    &\quad - \frac{\Delta Q \sin(\bar \alpha + \hat \theta - \omega)}{\sin(\bar \alpha) \cos(\bar \alpha)}.
%\end{align*}
%The same computations holds for the perturbations by linearity.
%\end{lemma}
%
%\begin{remark}
%    \label{Rem:why_tent}
%    We observe that the fact that we are in the tent case (not the arc) for the perturbation is due to the solution: indeed the admissibility must be verified on the perturbation $\tilde r$. However being the relations linear the same conditions pass to the derivative.   
%\end{remark}
%
%\begin{comment}
%\newpage
%
%
%By triangular geometry, it follows that
%\begin{equation*}
%    \frac{\ell_0}{r_0} = \frac{\sin(\phi}{\sin(\bar \alpha - \phi)}, \quad \phi = \angle Q_0,
%\end{equation*}
%and then since we need $\phi \geq \geq \bar \alpha + \hat \theta - \frac{\pi}{2}$, we need
%\begin{equation*}
%    \frac{\ell_0}{r_0} \geq - \frac{\bar \alpha + \hat \theta)}{\cos(\hat \theta)}.
%\end{equation*}
%
%The functional
%\begin{equation*}
%    \ell_0 + \frac{\cos(\bar \alpha + \hat \theta)}{\cos(\theta)} r_0
%\end{equation*}
%is rewritten as
%\begin{equation*}
%    \frac{\Delta Q \cdot e^{\i \hat \theta} - L}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + r_0 \frac{\sin(\bar \alpha) (\sin(\bar \alpha + \hat \theta) - \sin(\bar \alpha))}{\cos(\hat \theta) (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}.
%\end{equation*}
%
%
%
%\newpage
%
%
%\subsubsection{Formulas}
%\label{Sss:formulas_tent}
%
%
%Since the relations above are linear, and the solution is written as
%\begin{equation*}
%    \delta r(\phi) = \sum_i S_i G(\phi - \phi_i),
%\end{equation*}
%then the solution is the sum of the three saturated spirals
%\begin{equation*}
%    \delta \zeta(\phi) = \sum_i S_i \zeta(\phi - \phi_i).
%\end{equation*}
%Thus the position is computed as
%\begin{equation*}
%    \Delta Q = \sum_i S_i (\zeta(\phi - 2\pi - \bar \alpha + \hat \theta) - \zeta(\phi - 2\pi - \bar \alpha)),
%\end{equation*}
%the length is
%\begin{equation*}
%    L = \int_0^{\hat \theta} \frac{r(\phi - 2\pi - \bar \alpha + \phi')}{\sin(\bar \alpha)} d\phi' = \sum_i S_i \bar L(\phi - \phi_i),
%\end{equation*}
%and in general the conditions becomes
%\begin{equation*}
%    \hat \ell_0 = \sum_i S_i \hat \ell_0(\phi - \phi_i)
%\end{equation*}
%etc.
%
%
%We thus need to compute these terms for a saturated spiral, and then we can use them in the general solution.
%
%
%\begin{equation*}
%    \rho(\tau) = S_0 g(\tau) + S_1 g(\tau - \tau_1) + D \delta_1 + S_2 g(\tau - 1) + S_3 g(\tau - 2)
%\end{equation*}
%we get the relations for the tent (in $\rho$ coordinates, i.e. multiplied by $e^{-\bar c \phi}$, and using the notation with the check).
%
%
%
%Let $Z(\tau)$ be the position of the saturated spiral
%\begin{equation*}
%    Z(\tau) = \zeta(\phi) e^{-\bar c \phi},
%\end{equation*}
%so that
%\begin{equation*}
%    \check \Delta Q = \sum_i S_i Z(\tau - \tau_i),
%\end{equation*}
%the length
%\begin{equation*}
%    \check L = \sum_i S_i \int_0^{\hat \theta/(2\pi + \bar \alpha)} e^{-\bar c \tau} g(\tau - 1) d\tau 
%\end{equation*}
%\begin{equation*}
%    \check \ell_0 = \frac{\Delta \check Q e^{- \bar c(1 - \tau_1)} \cdot e^{\i \hat \theta} - \hat L}{}
%\end{equation*}
%
%For the arc case, one has a distribute source, to which it corresponds an integral of the above quantities.
%
%
%\begin{lemma}
%    \label{Lem:lenght_tent}
%    It holds $\hat r_2 > \tilde r_2$.
%\end{lemma}
%
%\begin{proof}
%For the spiral in the saturated region it holds
%\begin{equation*}
%    \tilde r_2 + L - \tilde r_0 - \cos(\bar \alpha) \tilde L = 0,
%\end{equation*}
%where $\tilde L$ is the length of the spiral:
%\begin{equation*}
%    \tilde L = \int \frac{r}{\sin(\bar \alpha)} d\phi.
%\end{equation*}
%All above quantities are linear w.r.t. the perturbation, if the base of the tent it is in the saturated region.
%
%Hence we obtain the same relations also for the perturbation. By convexity, the tent thus converging to a tent, and then by saturation it follows that the end point is larger than the original end point.
%\end{proof}
%
%Since the limit is still a spiral like, the fact that $\hat r_2$ is larger than $\tilde r_2$ is verified in the remaining parts, and also the it is thus enough by convexity to verify that it is sufficiently large.
%
%
%
%
%
%
%\newpage
%
%\subsection{Computations for a saturated spiral}
%\label{Ss:caompu_sat_spira_tent}
%
%
%The solution is
%\begin{equation*}
%    G(\phi) = \sum_i \frac{e^{\cot(\bar \alpha) (\phi - (2\pi + \bar \alpha)k)}}{\sin(\bar \alpha)^k} \frac{([\phi - (2\pi + \bar \alpha)]^=)^k}{k!}.
%\end{equation*}
%Then
%
%
%\newpage
%\end{comment}
%
%
%\subsubsection{Estimates of $\hat r(\bar \phi;s_0)$}
%\label{Sss:estima_hat_r_bar_phi}
%
%
%In order to estimate the value $\hat r(\bar \phi;s_0)$, the idea will be to compare $\hat r_2(\bar \phi - 2\pi + \hat \theta;s_0)$ with $\tilde r_2(\bar \phi - 2\pi + \hat \theta;s_0)$, and then write
%\begin{align}\label{eq:comp:sat}
%    \notag\hat r(\bar \phi;s_0) &= e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} \big( \hat r_2(\bar \phi - 2\pi + \hat \theta;s_0) - \tilde r_2(\bar \phi - 2\pi + \hat \theta;s_0) \big) \\
%    & \quad + \tilde r_2(\bar \phi;s_0) - \hat \ell_0.
%\end{align}
%{\color{red} non ho capito perchè hai messo il pedice $2$, non sono le soluzioni della spirale saturata $\bar r(\phi,s_0)$ della sezione $6$? No, lo so la notazione fa schifo}
%\begin{figure}
%    \centering\includegraphics[scale=0.5]{comparisonwithsaturated.png}
%    \caption{{\color{red}To quantify the quantity $\hat r(\bar\phi;s_0)$ we compare the black spiral with the saturated spiral (red curve). This motivates Equation \eqref{eq:comp:sat}, where the length $\overline{AB}=\hat r(\bar\phi-2\pi-\bar\theta)-\bar r(\bar\phi-2\pi-\bar\theta)$ is propagated in the angle $\bar\phi$ via the RDE of Saturated Spirals. Sì fa schifo detto così lo so }}
%    \label{fig:comparison:saturated}
%\end{figure}
%
%We next give some condition on $\hat r_0,L,Q_2-Q_1$ which assures that the above quantity is positive. The statements are based on the RDE, so that they hold also in the case of the perturbation.
%
%\begin{lemma}
%    \label{Lem:estima_tent}
%    Assume that $\tilde r$ is positive in the region where the tent is constructed, and moreover $|Q_2 - Q_1| \leq L$: then
%        \begin{equation*}
%            \hat r_2 > \tilde r_2, \quad \hat \ell_0 \leq \hat r_0 \frac{1- \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} < 0.313454 \hat r_0.
%        \end{equation*}
%%\begin{equation*}         
%%\hat \ell_1 \leq \hat r_0 \frac{1- \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + \frac{L - \Delta Q \cdot e^{\i \hat \theta} 
%%\sin(\bar \alpha - \hat \theta)}{\sin(\bar \alpha) (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}.
%%        \end{equation*}
%        The same holds for the perturbation $\delta r$.
%%        and the last estimate holds if the base curve is only continuous;
%%        \item if the curve where the tent occurs is saturated and $\tilde r$ is increasing, then
%%        \begin{equation*}
%%            \hat r_2 > \tilde r_2, \quad \hat \ell_0 \leq \tilde r_2 \frac{\sin(\bar \alpha) - \sin(\bar \alpha - \hat \theta) - \cos(\bar \alpha) \hat \theta}{\sin(\bar \alpha)} < 0.116544 \tilde r_2.
%%        \end{equation*}
%%    \end{enumerate}
%\end{lemma}
%
%Note that the $|\Delta Q| \leq L$ is always verified if $\delta r \geq 0$.
%
%\begin{proof}
%Observe that by
%\begin{equation*}
%    L \geq |\Delta Q|,
%\end{equation*}
%it follows immediately
%\begin{equation*}
%    \hat \ell_0 \leq \hat r_0 \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}.
%\end{equation*}
%Considering now the curve with radius of curvature given by $\tilde r$: then this curve is saturated, and thus it is impossible that $\hat r_2 = r_2$ is some point for any admissible curve, because the length of the tent is larger than the one of the saturated spiral.
%\begin{comment}
%
%Write the two RDE as 
%\begin{equation*}
%    \dot \tilde r = \cot(\bar \alpha) \tilde r - dL, \quad \dot \hat r = \cot(\beta) \hat - dL,
%\end{equation*}
%where $\beta = \beta(\phi)$ corresponds to the angle
%\begin{equation*}
%    \beta(\phi) = \begin{cases}
%        \alpha - \phi & 0 \leq \phi \leq \hat \phi, \\
%        \alpha + \hat \theta - \phi & \hat \phi < \phi \leq \hat \theta,
%    \end{cases}
%\end{equation*}
%with $\hat \phi$ angle of the tip of the ten. Hence
%\begin{equation*}
%    \frac{d}{d\phi} (\hat r - \tilde r) = \cot(\beta) (\hat r - \tilde r) + (\cot(\beta) - \cot(\bar \alpha)) \tilde r.
%\end{equation*}
%Let $\check \phi$ be the first time where the 
%
%
%for the saturated spiral as
%\begin{equation*}
%    \tilde r(\hat \theta) = \sum_i S_i e^{\cot(\bar \alpha) (\hat \theta - \phi_i)} - \int_0^{\hat \theta} e^{\cot(\bar \alpha) (\hat \theta - \phi')} R(\phi') d\phi' = \sum_i S_i e^{\cot(\bar \alpha) (\hat \theta - \phi_i)} - \int_0^{\hat \theta} e^{\cot(\bar \alpha) (\hat \theta - \phi')} dL(\phi'),
%\end{equation*}
%where we consider the case of several sources in the interval, we observe that
%\begin{equation*}
%    e^{\cot(\bar \alpha) \hat \theta} < 1.2331 < 1.31 < \frac{\sin(\hat \theta)}{\sin(\bar \alpha)(\cos(\bar \alpha - \hat \theta) - \cos('\bar \alpha))},
%\end{equation*}
%so that by maintaining constant $Q_2 - Q_0$ the quantity
%\begin{equation*}
%    L \mapsto \hat r_2 - \tilde r_2
%\end{equation*}
%has a minimum when $L$ is maximal. This case occurs when the convex initial curve is made of two segments, one along $\hat r_0$ and the other with direction $\hat \theta$: being in this case the solution explicit, we obtain that
%\begin{equation*}
%    \hat r_2 - \tilde r_2 = \tilde r_2 \bigg( e^{-\cot(\bar \alpha) \hat \theta} \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - 1 \bigg) > 0.
%\end{equation*}
%
%For the second case, we observe that we can rewrite the saturation assumption as
%\begin{equation*}
%    \hat r_2 - \tilde r_2 - \cos(\bar \alpha) \int_0^{\hat \theta} \frac{r}{\sin(\bar \alpha)} d\phi - \cos(\bar \alpha(\ell_0 + \ell_1) = 0.
%\end{equation*}
%Then, being the curvature radius increasing, the worst case is for a circle. In this case the computations are explicit, giving the second estimate on $\hat \ell_0$. About the first, this follows from the saturation condition.
%    
%\end{comment}
%\end{proof}

We conclude with an estimate in the case we have an arc.

\begin{lemma}
    \label{Lem:length_arc_hat_ell_0}
    If the fastest closing solution is an arc, and $\hat \ell_0$ is the length up to the critical angle $\hat \theta(\Delta \phi)$, then
    \begin{equation*}
        \hat \ell_0 \leq \hat r_0 \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}.
    \end{equation*}
\end{lemma}

\begin{proof}
We imagine to extend the construction of the segment also to situations where the angle at the endpoint of $\hat \ell_0$ is above $\frac{\pi}{2}$: also in this non-admissible case the formulas for the segment hold the same, because they depend only on the geometric relations among the different quantities.

We have then to prove that the admissible arc case has an initial segment which is less than the saturated spiral.

We start observing that when computing $\delta r$ in the segment case, the negativity region depends only on the angle $\theta = \bar \theta - \theta_0$. In particular, at the end point of the segment $\hat \ell_0$ for the arc, the arc derivative $\delta r$ is $0$, while the derivative in the segmnt case is negative, because $\hat \theta(\Delta \phi) < \hat \theta$ unless $\Delta \phi = 0$. Hence the length of $\hat \ell_0$ for the segment (not-admissible) case is larger than the one for the arc case.
%
%In the formulas for the derivative of the segment, observe that the negativity depends only on the angle $\theta$, not requiring admissibility. for the arc case we have that the critical angle $\hat \theta(\Delta \phi) \leq \hat \theta(0) = \hat \theta$, so that for the segment we would increase the length $\hat \ell_0$.
%
%
%Since $\Delta \phi + \hat \theta(\Delta \phi) \geq \hat \theta$, then we follow an arc on the level set which is outside the corresponding segment starting at the end of $\hat \ell_0$. The saturation gives that if we follow the segment 
%   
\end{proof}



\subsubsection{Estimates for having a tent}
\label{Sss:having_tent_check}


The next lemma gives a sufficient condition assuring that we have a tent: the condition is that if $\hat \phi$ is the angle at the tip of the tent, then
\begin{equation*}
    \bar \alpha + \hat \theta - \hat \phi < \frac{\pi}{2}, \quad \hat \phi \geq 0,113642.
\end{equation*}

\begin{lemma}
    \label{Lem:when_tent}
    Assume that the base of the tent is a convex curve of length $L$: if
    \begin{equation*}
        \frac{L}{\hat r_0} \leq \frac{\sin(\bar \alpha) (\sin(\bar \alpha + \hat \theta) - \sin(\bar \alpha))}{\cos(\hat \theta) (1 - \sin(\bar \alpha))} < 0.966795,
    \end{equation*}
    then the tent/segment is the fastest saturated solution.
\end{lemma}

\begin{proof}
Keeping $Q_2 - Q_0$ fixed, one sees geometrically that the worst case is when $L = |\Delta Q|$ pointing exactly in the direction $\hat \phi$ of the tip of the tent: indeed, if $Q$ is the point with the direction of $P_1$ in the subdifferential
\begin{enumerate}
    \item by taking the segment $Q - Q_0$ the angle of the optimal ray at $P_1$ increases,
    \item by taking the largest $L$ after $Q$ the length of $\ell_0$ decreases, so that the angle increases.
\end{enumerate}
%and the angle is $\phi$ where
%\begin{equation*}
%    \frac{\hat \ell_0}{\sin(\phi)} = \frac{\hat r_0}{\sin(\bar \alpha - \phi)},
%\end{equation*}
%i.e. the ray for the end point of $\hat r_0$ starts in the initial point of $\hat r_0$, and $Q_2$ is on the segment connecting these two points.
%
%This is because for $L$ and $Q_2 - Q_0$ fixed, the angle increases by packing the curve an close to $Q_ - Q_0$ as possible, and then increasing $L$ as much as we can so that $\hat \ell_0$ decreases.

At this point the relation ($\hat \phi$ is the direction of the ray at $\hat P_1$)
\begin{equation*}
    \hat r_0 \frac{\sin(\hat \phi)}{\sin(\bar \alpha - \hat \phi)} = \hat \ell_0 = \frac{\hat r_0 (1 - \cos(\hat \theta)) - L (1 - \cos(\hat \theta - \hat \phi))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}
\end{equation*}
gives
\begin{equation*}
    \frac{L}{\hat r_0} = \frac{\sin(\bar \alpha - \hat \phi)(1 - \cos(\hat \theta)) - \sin(\hat \phi) (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha))}{\sin(\bar \alpha - \hat \phi)(1 - \cos(\hat \theta - \hat \phi))} = \frac{\sin(\bar \alpha) (\cos(\hat \phi) - \cos(\hat \theta - \hat \phi))}{\sin(\bar \alpha - \hat \phi) (1 - \cos(\hat \theta - \hat \phi))}.
\end{equation*}
The function
\begin{equation*}
    \hat \phi \mapsto \frac{\sin(\bar \alpha) (\cos(\hat \phi) - \cos(\hat \theta - \hat \phi))}{\sin(\bar \alpha - \hat \phi) (1 - \cos(\hat \theta - \hat \phi))}
\end{equation*}
is decreasing after $\bar \alpha + \hat \theta - \frac{\pi}{2}$, and its value at that angle is $0.966795$.
\end{proof}

It is thus enough to verify that the above ratio is not satisfied in the saturated region of $\tilde r$, and then use the previous lemma to show that it is positive.


\subsection{Analysis of the arc}
\label{Ss:arc_instead_of_tent}


For the arc-closing, the entering quantities are the initial point, the point of the ray ending the arc, the point of the ray ending the segment, the length of the base, the angle
\begin{equation*}
    Q_0, \ Q_1, \ Q_2, \ L(\phi), \ \hat r_0, \ \widehat{\Delta \phi}.
\end{equation*}
The points are
\begin{equation*}
    P_0 = \hat r_0 e^{\i 0},
\end{equation*}
\begin{equation*}
    P_1 = \hat r(\widehat{\Delta \phi}) e^{\i \widehat{\Delta \phi}}, \quad \hat r(\phi) = \hat r_0 - L(\phi),
\end{equation*}
\begin{equation*}
    P_2 = P_1 + \widehat{\Delta P} e^{\i (\widehat{\Delta \phi} + \frac{\pi}{2})} = Q_2 + \hat r_2 e^{\i (\widehat{\Delta \phi} + \frac{\pi}{2} - \bar \alpha)},
\end{equation*}
The saturation is
\begin{equation*}
    \hat r_2 + L \bigg( \widehat{\Delta \phi} + \frac{\pi}{2} - \bar \alpha \bigg) - \hat r_0 - \cos(\bar \alpha) \bigg( \int_0^{\widehat{\Delta \phi}} \hat r(\phi) d\phi + \widehat{\Delta P} \bigg) = 0. 
\end{equation*}

We have the following result.

\begin{proposition}
    \label{Prop:non_admi_tent}
    The optimal solution $r(\bar \phi)$ is larger than the solution when we close with the tent, also in the non admissible case.
\end{proposition}

\begin{proof}
Indeed, the derivative $\delta (\bar \phi)$ is still negative for the tent, only we are not allowed to use this solution.
\end{proof}

In particular we deduce

\begin{corollary}
    \label{Cor:not_admis_tent_to_arc}
    If the closure with the not admissible tent is positive, so it is for the arc.
\end{corollary}

In particular, we will consider the not admissible optimal solution closing with the tent. Hence we do not need to check if the solution is a tent. 

{\bf But to verify which is the optimal solution we need!}

In general we have to compute the tent is specific cases, i.e. its initial point is only in the part where we cannot prove we have a tent.

The opening of the arc is nevertheless not too large: indeed we mast have that the angle at the beginning of the arc
\begin{equation*}
    0 \leq \phi_1 = \bar \alpha + \theta(\Delta \phi) - \frac{\pi}{2},
\end{equation*}
so that
\begin{equation*}
    \theta(\Delta \phi) \geq \frac{\pi}{2} - \bar \alpha.
\end{equation*}
This gives
\begin{equation*}
    \Delta \phi \leq 0.131397.
\end{equation*}


\subsection{Analysis of the optimal solution for $\bar \phi - 2\pi \geq \phi_2 + 2\pi + \bar \alpha$}
\label{Ss:phi_large_optimal}


This means that we are evaluating the optimal solution for $\tau \geq 2$.

The first result is that the tent is the optimal closing solution.


\subsubsection{Segment case}
\label{Sss:segment_in_tent_case}


We start with the analysis of the segment case, i.e. the solution is the fastest saturated spiral up to the angle $\bar \phi - 2\pi$.

\begin{proposition}
    \label{Prop:large_bar_phi_optimnal}
    For the solution $\tilde r$ the above lemma gives that it is a tent.
\end{proposition}

Here $\bar \tau$ is the initial angle of the base of the tent.

\begin{proof}
    Consider the functional for $\check \phi$ fixed
    \begin{equation*}
        \mathcal F(\check \phi,K) = \tilde r(\check \phi + 2\pi + \bar \alpha;s_0) - K \tilde L(\check \phi,\check \phi + \hat \theta) = \tilde r(\check \phi + 2\pi + \bar \alpha;s_0) - K \int_{\check \phi}^{\check \phi + \hat \theta} \frac{\tilde r(\phi';s_0)}{\sin(\bar \alpha)} d\phi',
    \end{equation*}
    where we have used that we are in the saturated zone so that $\beta(\check \phi) = \check \phi + \bar \alpha)$, with $K$ to be determined: from the above lemma, it is enough to have $K = 1.03435 = \frac{1}{0.966795}$.

Being linear, its derivative w.r.t. $s_0$ is
\begin{equation*}
    \delta \mathcal F(\check \phi,K) = \delta \tilde r(\check \phi + 2\pi + \bar \alpha;s_0) - K \int_{\check \phi}^{\check \phi + \hat \theta} \frac{\delta \tilde r(\phi';s_0)}{\sin(\bar \alpha)} d\phi',
\end{equation*}
so that an estimate on the maximal value of $K$ can be based on the perturbation analysis of the previous section, with $\check \phi \geq \phi_2 + 2\pi + \bar \alpha$. We rewrite this is terms of $\rho$,
\begin{equation*}
    \mathcal G(\check \tau) = \rho(\check \tau + 1) - K \int_0^{\frac{\hat \theta}{2\pi + \bar \alpha}} e^{\bar c (2\pi + \bar \alpha) \tau'} \rho(\check \tau + \tau') d\tau', \quad \check \tau \geq 1.
\end{equation*}

\medskip

{\it Case 1: $\check \tau \geq 3$.}

\smallskip

\noindent In this region the function $\rho(\tau)$ is increasing, so that
\begin{align*}
    \mathcal G(\tau) &\geq \rho(\check \tau + 1) \bigg( 1 - K \int_0^{\frac{\hat \theta}{2\pi + \bar \alpha}} e^{\bar c (2\pi + \bar \alpha) \tau'} d\tau' \bigg) \\
    &= \rho(\check \tau + 1) \bigg( 1 - K \frac{e^{\bar c \hat \theta} - 1}{(2\pi + \bar \alpha) \bar c} \bigg) = 0.924623 \rho(\check \tau + 1).
\end{align*}
Hence the optimal closing solution start with a tent.

\medskip

{\it Case 2: $\check \tau \in [2,3)$.}

\smallskip

\noindent

Taking the derivative w.r.t. $\check \tau$ we obtain %setting $\kappa = \frac{K}{2\pi + \bar \alpha}$
\begin{equation*}
    \partial_{\check \tau} \mathcal G = \rho(\check \tau + 1) - K e^{\bar c \hat \theta} \rho \bigg( \check \tau + \frac{\hat \theta}{2\pi + \bar \alpha} \bigg) + (K - 1) \rho(\check \tau).
\end{equation*}
%Two cases may happen: if $\rho(\tau + \frac{\hat \theta}{2\pi + \bar \alpha}) \geq \rho(\tau)$, then it is enough to estimate
%\begin{equation*}
%    \rho(\tau + 1) - \kappa e^{\bar c \hat \theta} \rho \bigg( \tau - \frac{\hat \theta}{2\pi + \bar \alpha} \bigg),
%\end{equation*}
%otherwise
%\begin{equation*}
%    \rho(\tau + 1) - \rho(\tau).
%\end{equation*}
%
%In the region where $\rho$ is increasing, since
%\begin{equation*}
%    1.05 \hat \theta e^{\bar c \hat \theta} < 0.612339 < 1,
%\end{equation*}
%it follows that the function is increasing.
%
%Set
%\begin{equation*}
%    \hat \tau = \frac{\hat \theta}{2\pi + \bar \alpha}.
%\end{equation*}
%We will sometime use the estimate
%\begin{equation*}
%    \int \dots \leq K \hat \theta e^{\bar c \theta} \max \rho = \kappa \max \rho.
%\end{equation*}
Using the explicit formulas of the previous secion, one finds that the derivative is
\begin{equation*}
    \partial_{\check \tau} \mathcal G \geq 0.192012 \theta^2,
\end{equation*}
so that the minumum is in the interval $[1,2]$.

\medskip

{\it Case 3: $\bar \tau \in [1,2)$.}

\smallskip

\noindent For $\tau \in [1,2)$, we observe numerically that the derivative is positive in the region
\begin{equation*}
    \big\{ \theta \geq \hat \theta \big\} \cup \big\{ 1 \leq \tau \leq 1 + \tau_1 - \hat \tau \big\} \cup \big\{ 0 \leq \theta \leq \hat \theta, 2 - \hat \tau \leq \tau \leq 2 \big\},
\end{equation*}
The choice of this region is to avoid the part where $\rho \simeq \theta$ for small angles in the term $\rho(\tau + \hat \tau)$, i.e. $\{1 + \tau_1 \leq \tau < 2\big\}$. Numerical estimates gives
\begin{equation*}
    \partial_\tau \mathcal G \geq 0.189194 \theta^2.
\end{equation*}
Since $\mathcal G$ is continuous for $\tau \geq 1$ ($\rho$ is continuous for $\tau \geq 3$ and the integral is Lipschitz continuous), we evaluate at $\tau = 1$:
\begin{align*}
    \mathcal G(1) &= \rho(1) - K \bigg[ S_0 \bigg( \frac{e^{1 + \cot(\bar \alpha) (2\pi + \bar \alpha) \hat \tau} - e}{\cot(\bar \alpha) (2\pi + \bar \alpha)} - \frac{\hat \tau e^{\cot(\bar \alpha) (2\pi + \bar \alpha) \hat \tau}}{\cot(\bar \alpha) (2\pi + \bar \alpha)} + \frac{e^{\cot(\bar \alpha) (2\pi + \bar \alpha) \hat \tau} - 1}{(\cot(\bar \alpha) (2\pi + \bar \alpha))^2} \bigg) \\
    & \quad \qquad \qquad + S_1 \frac{e^{1 -\tau_! + \cot(\bar \alpha) (2\pi + \bar \alpha) \hat \tau} - e^{1-\tau_1}}{\cot(\bar \alpha) (2\pi + \bar \alpha)} + S_2 \frac{e^{\cot(\bar \alpha) (2\pi + \bar \alpha) \hat \tau} - 1}{\cot(\bar \alpha) (2\pi + \bar \alpha)} \bigg].
\end{align*}
Numerical evaluation gives that
\begin{equation*}
    \mathcal G(1) \geq 0.581965 \theta^2.
\end{equation*}

It remains to compute the value of the functional in the other regions, i.e.
\begin{equation*}
    \{ 0 \leq \theta \leq \hat \theta \} \cap \big\{ 1 + \tau_1 - \hat \tau \leq \tau \leq 2 -\hat \tau \big\}.
\end{equation*}
Numerically one observes that for $\theta$ fixed the derivative $\partial_\tau \mathcal G$ is negative in an interval of the form $(a,2 - \hat \tau)$, so that the minimum is reached at $\tau = 2 - \hat \tau$. Numerical computations shows that
\begin{equation*}
    \mathcal G(2-\hat \tau) \geq 0.847926 \theta^2.
\end{equation*}

\medskip

{\it Case 4: $\bar \tau \in [0,1]$.}

\smallskip

\noindent The derivative is positive $\geq 0.154759 \theta^2$ outside the region
\begin{equation*}
    \big\{ 0 \leq \theta \leq \hat \theta, \tau_1 \leq \tau \leq 1 \big\}.
\end{equation*}
In that region an explicit evaluation of $\mathcal G$ gives
\begin{equation*}
    \mathcal G(\tau) \geq 0.01660 \theta,
\end{equation*}
so it is positive. %The explicit computation of the integral for...

Finally for $\tau = 0$ one obtains
\begin{equation*}
    \mathcal G(0) \geq 0.386838 \theta^2.
\end{equation*}
This concludes the proof.
%
%
%For $\theta \leq \hat \theta$, we need to use the integral because of the behavior as $\theta$ for $\theta \searrow 0$. 
%
%
%it is positive: indeed being the solution increasing, one can prove numerically that (set $\kappa = 1.05 \hat \theta^{\bar c \hat \theta}$)
%\begin{equation*}
%    \frac{\rho(3) - \kappa \rho([2,1.9+\tau_1))}{\theta^2} \geq 0.3,
%\end{equation*}
%\begin{equation*}
%    \frac{\rho(3.1) - \kappa \rho([2,2+\tau_1))}{\theta^2} \geq 0.3,
%\end{equation*}
%\begin{equation*}
%    \frac{\rho(3.5) - \rho([2+\tau_1,3))}{\theta^2} \geq 0.1.
%\end{equation*}
%Hence the functional is positive.
%
%For $\tau \in [1+\tau_1,2]$ we need to use the integral, because of the convergence like $\theta$ for $\tau \in [1+\tau_1,2)$: we have
%\begin{equation*}
%    \frac{\rho(\tau+1) - \rho(\tau)}{\theta^2}, \frac{\rho(\tau+1-\hat \tau) - K e^{\bar c \hat \theta} \rho(\tau)}{\theta^2} > 0.3,
%\end{equation*}
%and then for $\tau \in [1,1+\tau_1 - \hat \tau]$ the functional is still increasing (so it not an extremal point).
%
%For $\tau \in [1,1 + \tau_1 + \hat \tau)$, we have for $\theta > 0.3$ that
%\begin{equation*}
%    \frac{\rho(\tau+1) - \rho(\tau)}{\theta^2}, \frac{\rho(\tau+1-\hat \tau) - \rho(\tau)}{\theta^2} > 0.02.
%\end{equation*}
%For $\theta \leq 0.1$, we compute
%\begin{equation*}
%    \rho(\tau+1) - K e^{\bar c \hat \theta} \int_{\tau}^{\tau+\hat \tau} \rho(\tau') d\tau' \geq \theta^2, \quad \tau \in [1+\tau_1-\hat \tau,1+\tau_1],
%\end{equation*}
%\begin{equation*}
%    \rho(\tau+1) - K e^{\bar c \hat \theta} \int_{\tau}^{\tau+\hat \tau} \rho(\tau') d\tau' \geq \theta^2, \quad \tau \in [2-\hat \tau,1 + \tau_1],
%\end{equation*}
%\begin{equation*}
%    \rho(\tau+1) - K e^{\bar c \hat \theta} \int_{\tau}^{\tau+\hat \tau} \rho(\tau') d\tau' \geq \theta^2, \quad \tau \in [1+\tau_1,2],
%\end{equation*}
%so that also in this case the optimal solution is a segment.
\end{proof}

We can then apply the above lemma to prove that the perturbation is positive.

\begin{proposition}
    \label{Prop:pertub_positive_large_bar_phi}
    In the region under consideration ($\bar \phi - 2\pi - \bar \alpha \geq \phi_2$), the tent perturbation is positive.
\end{proposition}

\begin{proof}
We consider several cases: $\bar \tau$ is the angle at the initial ray $\hat r_0$ of the tent.

\medskip

{\it Case 1: $\bar \tau \geq 2$.}

\smallskip

\noindent If $\bar \tau \geq 2$ (the initial ray $\hat r_0$ is after the first round), then the solution $\delta r$ is positive, so that we can apply Lemma ?? to compare with the saturated solution. In the $\rho$ coordinates the functional we estimate is
\begin{equation*}
    \mathcal M(\tau) = \rho(\bar \tau + 1) - H e^{-\bar c (2\pi + \bar \alpha)} \rho(\bar \tau),
\end{equation*}
\begin{equation*}
    H = \frac{1-\cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} e^{-\bar c (2\pi + \bar \alpha)} = 0.038815.
\end{equation*}

We have
\begin{description}
    \item[$\bar \tau \geq 3$] the solution $\rho$ is increasing, so that
    \begin{equation*}
        \rho(\bar \phi + 1) - H \rho(\bar \phi) \geq (1 - H) \rho(\bar \phi + 1) \geq 0.
    \end{equation*}
We can apply the lemma, because the base of the tent is in $[2,3)$, thus positive.

    \item[$\bar \tau \in [2,3)$] it holds
    \begin{equation*}
        \mathcal M \geq 0.796496 \theta^2.
    \end{equation*}
    We can apply the lemma, because the base of the tent is in $[1,2)$, thus positive.
    
    \item[$\bar \tau \in [1,1+\tau_1-\hat \theta)$] it holds
    \begin{equation*}
        \mathcal M \geq 0.597203 \theta^2.
    \end{equation*}
We can apply the lemma, because the base of the tent is in $[0,\tau_1)$, thus positive.

    \item[$\bar \tau \in [1 + \tau_1 - \hat \theta,2), \theta \geq \hat \theta$] we can still apply the lemma, and numerically one obtains
    \begin{equation*}
        \mathcal M \geq 0.170638.
    \end{equation*}

\item[$\bar \tau \in [1,1+\tau_1-\hat \theta,2), \theta \leq \hat \theta$] we need to compute the complete form for the tent, because the base of the tent is in the negative region. 




%Numerically one obtains:
    \begin{itemize}
        \item If $\bar \tau \in [1 + \tau_1 - \hat \theta,2 - \hat \theta)$, then we compute %explicitly
        \begin{align*}
            \delta L &= \int_{\bar \phi - (2\pi + \bar \alpha)}^{\bar \phi - (2\pi + \bar \alpha - \hat \theta)} \frac{\delta r(\phi')}{\sin(\bar \alpha)} d\phi' \\
            &= \frac{1-\cos(\theta)}{\sin(\bar \alpha)^2} \big( e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \theta)} - e^{\cot(\bar \alpha) \phi} \big) - \frac{e^{\cot(\bar \alpha)(\phi + \hat \theta - (2 \pi + \bar \alpha - \theta))} - 1}{\cos(\bar \alpha)},
        \end{align*}
        \begin{align*}
            (Q_1 - Q_0) \cdot e^{\i \hat \theta} &= \int_{\bar \phi - (2\pi + \bar \alpha)}^{\bar \phi - (2\pi + \bar \alpha - \hat \theta)} \frac{\delta r(\phi')}{\sin(\bar \alpha)} \cos(\phi' - \phi - \hat \theta - \bar \alpha) d\phi' \\
            &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) \bigg( \frac{e^{\cot(\bar \alpha) (\phi + \hat \theta)} (\cot(\bar \alpha) \cos( \bar \alpha) - \sin(\bar \alpha)) - e^{\cot(\bar \alpha) \phi} (\cot(\bar \alpha) \cos( \bar \alpha + \hat \theta) - \sin(\bar \alpha + \hat \theta))}{1 + \cot(\bar \alpha)^2} \bigg) \\
            & \quad + \frac{e^{\cot(\bar \alpha) (\phi + \hat \theta - (2\pi + \bar \alpha - \theta))} (\cot(\bar \alpha) \cos( \bar \alpha) - \sin(\bar \alpha)) - (\cot(\bar \alpha) \cos( 2 \pi + \bar \alpha - \theta - \phi - \bar \alpha - \hat \theta) + \sin(2 \pi + \bar \alpha - \theta - \phi - \bar \alpha - \hat \theta))}{1 + \cot(\bar \alpha)^2},
        \end{align*}
        \begin{align*}
            (Q_1 - Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2}} &= \int_{\bar \phi - (2\pi + \bar \alpha)}^{\bar \phi - (2\pi + \bar \alpha - \hat \theta)} \frac{\delta r(\phi')}{\sin(\bar \alpha)} \cos \bigg( \phi' - \phi - \hat \theta - \bar \alpha + \frac{\pi}{2} \bigg) d\phi', %\\ 
        \end{align*}

        Numerically the solution is positive $\geq 200 \theta^2$.

        \item if $\bar \tau \in [2 - \hat \tau, 1 + \tau_1)$, then in the computation of the length we have to add the Dirac delta $D$: one obtains
        \begin{equation*}
            \delta \hat r(\bar \phi) 
        \end{equation*}


        \item if $\bar \tau \in [1 + \tau_1,2)$, again we need to consider the presence of the Dirac delta: one obtains


        
        \begin{equation*}
            \delta \hat r(\bar \phi + 2\pi + \bar \alpha) \geq  \frac{\theta}{\sin(\bar \alpha) \cos(\bar \alpha) (1 - \cos(\hat \theta))};
        \end{equation*}
    \end{itemize}   
\end{description}


\begin{comment}
In the range of $\tau$ under consideration, $\rho$ is positive, and then we have to verify that
\begin{equation*}
    \hat r(\bar \phi) \geq \tilde r(\bar \phi) \geq .313454 r(\bar \phi - 2\pi - \bar \alpha).
\end{equation*}
In terms of $\rho$ we require
\begin{equation*}
    \rho(\tau + 1) \geq .313454 e^{-\bar c(2\pi + \bar \alpha} \rho(\tau),
\end{equation*}
which is numerically verified: indeed in terms of $\rho$ we estimate
\begin{align*}
    \hat \rho(\bar \tau) &= e^{- \bar c \bar \phi} \big( \hat r(\bar \phi) - \hat \ell_0 \big) \\
    &\geq e^{-\bar c \bar \phi} (\tilde r(\bar \phi) - 0.31 \tilde r(\bar \phi - 2\pi - \bar \alpha) \big) \\
    &= \rho(\bar \tau) - e^{-\bar c (2\pi + \bar \alpha)} 0.31 \rho(\bar \tau - 1) \\
    &\geq \rho(\bar \tau) - 0.0389 \rho(\bar \tau - 1).
\end{align*}
When $\rho$ is increasing, nothing has to be proved, hence we are left to $\tau \in [1,3]$.

We have
\begin{equation*}
    \hat \rho(\tau + 1) - 0.0389 \hat \rho(\tau) \geq 0.6 \theta^2, \quad \tau \in [1,1+\tau_1],
\end{equation*}
\begin{equation*}
    \hat \rho(\tau + 1) - 0.0389 \hat \rho(\tau) \geq 0.7 \theta^2, \quad \tau \in [2,2+\tau_1],
\end{equation*}
\begin{equation*}
    \hat \rho(\tau + 1) - 0.0389 \hat \rho(\tau) \geq 0.9 \theta^2, \quad \tau \in [2+\tau_1,3].
\end{equation*}

For the interval $[1+\tau_1,2]$, we need to use the full formula for $\hat r_2$, due to the fact that $\rho(\bar \tau - 1)$ behaves like $\theta$: we first observe that since $\omega$ (the angle of $\Delta Q$) is in $[0,\hat \theta]$ then the function
\begin{equation*}
    \frac{\cos(\hat \theta - \omega) \sin(\hat \theta)}{\sin(\bar \alpha)(\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha))} - \frac{\sin(\bar \alpha + \hat \theta - \omega)}{\sin(\bar \alpha)} > 0.072,
\end{equation*}
so that we can use the estimate
\begin{equation*}
    \hat r_2 > \hat r_0 \frac{\cos(\bar \alpha) - \cos(\bar \alpha - \hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - L \frac{\sin(\hat \theta)}{\sin(\bar \alpha) (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
\begin{equation*}
    \hat \rho_2 > e^{- \bar c \hat \theta} \rho_0 \frac{\cos(\bar \alpha) - \cos(\bar \alpha - \hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - e^{\bar c \hat \theta} L \frac{\sin(\hat \theta)}{\sin(\bar \alpha) (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
We thus have to study
\begin{align*}
    \hat r(\bar \phi) &= (\hat r_2 - \tilde r_2) e^{\cot(\bar \alpha)(2\pi+ \bar \alpha - \hat \theta)} + \tilde r(\bar \phi) - \hat \ell_0.
\end{align*}
\begin{align*}
    \hat \rho(\bar \tau) &= (\hat \rho_2 - \tilde \rho_2) e^{1 - \frac{\hat \theta}{2\pi+\bar \alpha}} + \tilde \rho(\bar \tau) - 0.0389 \rho(\bar \tau - 1).
\end{align*}
Numerical computations give
\begin{equation*}
    \rho(\bar \tau) \geq 0.7 \theta^2, \quad \theta \in [0,\hat \theta], \tau \in [1+\tau_1,2],
\end{equation*}
\begin{equation*}
    \rho(\bar \tau) - 0.0389 \rho(\bar \tau - 1) \geq 0.2, \quad \theta \in [\hat \theta,Pi/2], \tau \in [1+\tau_1,2].
\end{equation*}
Thus in all cases the perturbation is positive.
\end{comment}
This concludes the proof.
\end{proof}


\subsubsection{Arc case for large angles}
\label{Sss:arc_case_large_angels_tent}


\begin{proposition}
    \label{Prop:sol_tent_arc_case}
    The solution is a tent.
\end{proposition}

\begin{proof}
    
\end{proof}



\subsection{Analysis of the optimal solution for $\bar \phi - 2\pi \in \phi_2 + [0,2\pi + \bar \alpha]$}
\label{Ss:small_bar_phi}


Here apriori we do not know if the optimal closing perturbation is a tent or an arc.

In both cases, the perturbation is positive unless
\begin{equation*}
    \bar \phi - 2\pi < \phi_2 + 2\pi + \alpha \quad \text{or} \quad \hat \phi_2 > \phi_0 + \theta_0,
\end{equation*}
where $\hat \phi_2$ is the last angle before the solution becomes saturated.

Also for the case $\theta \geq \hat \theta$, the solution $\delta r$ is positive and we can apply previous computation which assures it is a tent and the tent is positive.


\subsubsection{Segment case closing with tent}
\label{Ss:segment_erptu_optimal}


Set $\phi_2 = 0$, and recall that $\theta$ is the angle of the perturbation.

The computation of the tent functional gives that it has positive, unless the tip point of $\hat r_0$ is inside the negativity region.


\medskip

{\it Case 1: $\hat \theta_2 \in 2\pi + \bar \alpha + [-\theta,0]$}

\smallskip

\noindent In this case $Q = L$ and then we obtain (use $\omega \mapsto \hat \theta - \omega$, and some obvious notations)
\begin{equation*}
    \hat \ell_0 = \frac{\hat r_0 (1- \cos(\hat \theta)) - \delta s_0 (1 - \cos(\omega))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
\begin{equation*}
    \hat r_2 = \hat r_0 \frac{\cos(\bar \alpha) - \cos(\bar \alpha + \hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - \frac{\delta s_0}{\sin(\bar \alpha)} \bigg( \sin(\bar \alpha + \omega) + \frac{\sin(\hat \theta) (1 - \cos(\omega)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg). 
\end{equation*}
We write the solution as
\begin{align*}
    \hat \rho \bigg( 2 - \frac{\theta - \omega + \hat \theta}{2\pi + \bar \alpha} \bigg) = \rho \bigg( 2 - \frac{\theta - \omega + \hat \theta}{2\pi + \bar \alpha} \bigg) + (\hat r_2 - \tilde r_2) e^{\bar c ..} e^{1 - \frac{\theta - \omega + \hat \theta}{2\pi + \bar \alpha}} - \hat \ell_0.
\end{align*}
Numerical plots shows that this is positive and $\geq .4 \theta^2$.

Numerical plot gives
\begin{equation*}
    \hat r(\bar \phi) \geq 17.783 \theta(\theta + \omega).
\end{equation*}


\medskip

{\it Case 2: $\hat \theta_0 < \theta_0 < \bar \theta < \hat \theta_2$}.


In this case $\delta \ell_0 = 0$, and
\begin{equation*}
    \hat r_0 = \delta \tilde r(2\pi + \bar \alpha - (\hat \theta - \omega)),
\end{equation*}
\begin{equation*}
    Q_2 - Q_1 = \delta \tilde r(\omega) e^{\i (\hat \theta - \bar \alpha)},
\end{equation*}
\begin{equation*}
    \Delta Q \cdot e^{\i \hat \theta} = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta)) e^{\cot(\bar \alpha) \omega} \cos(\omega),
\end{equation*}
\begin{equation*}
    L = 1 + \delta \Delta P - \frac{r_2 \delta \theta}{\sin(\bar \alpha)} + \int_0^\omega \frac{r}{\sin(\bar \alpha)} = \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} e^{\cot(\bar \alpha) \omega}.
\end{equation*}
The solution is the written as
\begin{equation*}
    \ell_0 = \delta \tilde r \bigg( 2\pi + \bar \alpha - \frac{\hat \theta - \omega}{2\pi+\bar \alpha} \bigg)
\end{equation*}
\begin{align*}
    \hat r_2 &= ..
\end{align*}
and
\begin{align*}
    \hat r_2 = ...
\end{align*}

Numerically this function is above
$$
40 \theta^2(\theta + \check \theta).
$$

\medskip

{\it Case 3: the tent is inside the negative region.}

\smallskip

\noindent In this case $L=\Delta Q = 0$, so that the solution is positive by explicit computation:
\begin{equation*}
    \geq 13.3793.
\end{equation*}


\medskip

{\it Case 4: the tent starts inside the negative region but it exits after}


Again the solution is
\begin{equation*}
    \Delta Q = \delta \tilde r(\omega) e^{\i (\hat \theta - \bar \alpha)} - e^{\i (\theta - (\hat \theta - \omega)},
\end{equation*}
\begin{equation*}
    \hat r_0 = \delta \tilde r(2\pi + \bar \alpha - (\hat \theta - \omega)),
\end{equation*}
\begin{equation*}
    L = - 1 + \frac{1-\cos(\theta)}{\sin(\bar \alpha)^2} e^{\cot(\bar \alpha) \omega},
\end{equation*}
and then numerically one gets
\begin{equation*}
    \geq 33.5362 \theta^2.
\end{equation*}


\subsubsection{Segment case with arc closure}
\label{Sss:arc_case_small_angles}


The first case is when the end point of the arc is before the negativity region: then the formulas are
\begin{equation*}
    r_1 e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})} = r_0 e^{\i 0} + \ell_0 e^{\i \bar \alpha},
\end{equation*}
\begin{equation*}
    r_1 e^{\i (\bar \alpha + \hat \theta + \Delta \phi - \frac{\pi}{2})} + \ell_1 e^{\i (\bar \alpha + \hat \theta + \Delta \phi)} = r_2 e^{\i (\hat \theta + \Delta \phi)},
\end{equation*}
saturation
\begin{equation*}
    r_2 - r_0 - \cos(\bar \alpha) \big( \ell_0 + r_1 \Delta \phi + \ell_1 \big) = 0,
\end{equation*}
\begin{equation*}
    r_2 - \ell_1 \cos(\bar \alpha) = r_1 \sin(\bar \alpha) = \cos(\bar \alpha) (\ell_0 + r_1 \Delta \phi),
\end{equation*}
\begin{equation*}
    r_1 = r_0 \sin(\bar \alpha + \hat \theta) + \ell_0 \sin(\hat \theta),
\end{equation*}


\begin{comment}
    
\newpage


\subsection{Expansion of the solution near $\theta = 0$ for segment case}
\label{Ss:expansion_segm_0}


We first study the functional $\mathcal F$ for $\bar \tau \in [0,1]$, i.e. when the tent is constructed in the first round.

\medskip

{\it Case 1 below}

\smallskip

\noindent There is a trapezoidal negative region similar to the negativity region for the segment, only translated of $-\hat \theta$, where the functional is negative.

\medskip

In the rest it is positive.

\begin{lemma}
    \label{Lem:tent_round_01}
    In the round $[0,1]$ the optimal closing solution is a tent unless the end point is in the negativity region.
\end{lemma}

One can also compute explicitly the value of the region, i.e. the maximal value of the angle for which it is positive.


\subsubsection{Study of tent in the segment case}
\label{Sss:study_tent_bar_phi_final_segment}


Here we study the tent in the segment case when the base of the tent passes $0$, i.e. it contains parts of the non saturated region: this means that $\bar \tau \in [0,1]$, being the initial angle of the tent.

\medskip

{\it Case 1: $\phi_0 + \theta_0 \leq \bar \phi + \hat \theta \leq \phi_0 + \bar \theta$.}

\smallskip

\noindent Define the angle $\check \theta$ as the angle formed by the ray $\hat r_2$ (exiting the tent) and the perturbation $\delta s_0$. The entering solution is then 
\begin{equation*}
    \delta \hat r_0 = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta)) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - (\theta - \check \theta + \hat \theta))} = S_0' e^{\cot(\bar \alpha)(2\pi + \bar \alpha - (\theta - \check \theta + \hat \theta))},
\end{equation*}
variation of initial points (with angles w.r.t. the base of the tent) and of length (remember that $\delta s_0 \to 1$)
\begin{equation*}
    \delta Q_0 = 0, \quad \delta Q_1 = \delta s_0 e^{\i (\hat \theta - \check \theta)}, \quad \delta L = \delta s_0.
\end{equation*}
The final value is computed by
\begin{equation*}
    \delta \hat r(\bar \phi) = (\hat r_2 - \delta r(\phi_2)) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} + \delta r(\bar \phi) - \hat \ell_0,
\end{equation*}
with
\begin{equation*}
    \delta r(\hat \phi_2) = S_0' e^{\cot(\bar \alpha)(2\pi + \bar \alpha - (\theta - \check \theta))} - e^{\cot(\bar \alpha) \check \theta}, 
\end{equation*}
\begin{align*}
    \delta r(\bar \phi) &= S_0' \bigg( e^{\cot(\bar \alpha)(2(2\pi + \bar \alpha) - (\theta - \check \theta + \hat \theta))} - e^{\cot(\bar \alpha)(2\pi + \bar \alpha - (\theta - \check \theta + \hat \theta))} \frac{(2\pi + \bar \alpha - (\theta - \check \theta + \hat \theta))}{\sin(\bar \alpha)} \bigg) \\
    & \quad - e^{\cot(\bar \alpha) (2\pi + \bar \alpha - (\hat \theta - \check \theta))} \\
    & \quad + \bigg[ 1 - \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} + \cot(\bar \alpha) \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} \bigg] e^{\cot(\bar \alpha) (2\pi + \bar \alpha - (\theta - \check \theta + \hat \theta))}.
\end{align*}
Numerical evaluation show that
\begin{equation*}
    \delta \hat r(\bar \phi) \geq 19.904 \theta (\theta + \check \theta).
\end{equation*}

\medskip

{\it Case 2: $\bar \phi \leq \phi_0 < \phi_2 \leq \bar \phi + \hat \theta$.}

\smallskip

\noindent

The entering solution is the same as before, with entering angle $\phi = 2\pi + \bar \alpha - (\hat \theta - \check \theta)$, the variation of the point $Q_0$ is $0$ and
\begin{equation*}
    \delta Q_1 = r(\check \theta) e^{\i (\hat \theta - \bar \alpha)},
\end{equation*}
\begin{equation*}
    \delta L = \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} e^{\cot(\bar \alpha) \check \theta}.
\end{equation*}
It follows by direct computations that
\begin{equation*}
    \delta \ell_0 = 0,
\end{equation*}
\begin{equation*}
    \delta \hat r_2 = \frac{\delta \hat r_0 \sin(\bar \alpha + \hat \theta) - \delta r_0(\check \theta) \sin(2\bar \alpha)}{\sin(\bar \alpha)}
\end{equation*}
Numerical valuation gives
\begin{equation*}
    \delta \hat r(\bar \phi) \geq 87.5535 \theta^2 (\theta + \check \theta).
\end{equation*}

\medskip

{\it Case 3:$\phi_0 + \theta_0 \leq \bar \phi - 2\pi \leq \bar \phi - 2\pi + \hat \theta \leq \phi_0 + \bar \phi$.}

\smallskip

\noindent We have
\begin{equation*}
    \delta Q_i = 0, \quad \delta L = 0,
\end{equation*}
and choosing $\check \theta$ as the angle from $\delta s_0$ to $\hat r_0$
\begin{equation*}
    \delta \hat r_0 = S_0' e^{\cot(\bar \alpha)(2\pi + \bar \alpha - (\theta - \check \theta)} - e^{\cot(\bar \alpha) \check \theta}.
\end{equation*}
Hence numerically one obtains
\begin{equation*}
    \delta \hat r(\bar \phi) \geq 32.3172.
\end{equation*}

\medskip

{\it Case 4: $\phi_0 \leq \bar \phi \leq \phi_2 \leq \bar \phi + \hat \theta$.}

\smallskip

\noindent

Choose $\check \theta$ as the angle of $\Delta P$ and $\hat r_2$. The entering solution is the same as before, with entering angle $\phi = 2\pi + \bar \alpha - (\hat \theta - \check \theta)$,
\begin{equation*}
    \delta \hat r_0 = S_0' e^{\cot(\bar \alpha)(2\pi + \bar \alpha - (\hat \theta - \check \theta))} - e^{\cot(\bar \alpha) (\theta - (\hat \theta - \check \theta))},
\end{equation*}
the variation of initial points is
\begin{equation*}
    \Delta Q_0 = e^{-i(\theta - (\hat \theta - \check \theta))}, \quad \delta Q_1 = S_0' e^{\cot(\bar \alpha) \check \theta} e^{\i (\hat \theta - \bar \alpha)},
\end{equation*}
\begin{equation*}
    \delta L = -1 + \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} e^{\cot(\bar \alpha) \check \theta}.
\end{equation*}
It follows by direct computations that
\begin{equation*}
    \delta \hat r(\bar \phi) \geq 33.5362 \theta^2.
\end{equation*}



\newpage


\begin{proposition}
    \label{Lem:saturated_tent}
    The tent is the perturbation in the saturated part of $\tilde r$.
\end{proposition}

\begin{proof}
Let $\bar \phi$ be the first angle where the solution is not a tent in the saturate part of $\tilde r$: equivalently, it is the first angle for which we reach the angle $\frac{\pi}{2}$ on the point $P_1$ tip of the tent. The perturbations we consider are the optimal closing solution in the direction $\bar \phi$.

We want to show that the angle $\frac{\pi}{2}$ will be diminished after the perturbation. We already know that this is not possible to happens after the first saturated round.



We compute the functional
\begin{equation*}
    \delta r(\bar \phi) - K L
\end{equation*}
along the optimal solutions considered before. Since we are in the saturated part, this functional is in the original and $\tau$ coordinates
\begin{equation*}
    \mathcal G = \delta r(\bar \phi + 2\pi + \bar \alpha) - K \int_0^{\hat \theta} \frac{\delta r(\bar \alpha + \phi')}{\sin(\bar \alpha)} d\phi',
\end{equation*}
\begin{equation*}
    \mathcal G = \rho(\bar \tau + 1) - K \int_0^{\hat \tau} e^{\bar c (2\pi + \bar \alpha) \tau'} \rho(\bar \tau + \tau') d\tau', \quad \hat \tau = \frac{\hat \theta}{2\pi + \bar \alpha}.
\end{equation*}

\medskip

{\it Case 1: the final angle of the tent is before the perturbation.}

\smallskip

\noindent This means that we are in the region where the solution is a pure logarithmic spiral, and the optimal closing solution is equal to the fastest closing solution. We thus have
\begin{equation*}
    \delta r(\bar \phi + 2\pi + \bar \alpha) > 0, \quad \delta L = 0,
\end{equation*}
both in the segment and in the arc cases.

For the angle,
\begin{equation*}
    \delta \ell_0 = \frac{\delta r_0 (1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
\begin{align*}
    \delta \ell_0 \cos(\hat \theta) - \delta r_0 \cos \bigg( \bar \alpha + \hat \theta - \frac{\pi}{2}\bigg)
\end{align*}
\medskip

{\it Case 2: $\bar \phi + 2\pi + \bar \alpha \in \phi_0 + \bar \theta + [-\hat \theta,0]$.}

\smallskip

This means that the the initial angle is along the direction where in the optimal closing solution we take the segment up to the critical angle $\hat \theta$.

We have thus
\begin{equation*}
    L = \hat \ell_1 = 
\end{equation*}
\begin{align*}
    \mathcal G &= \delta r_2 - K \ell_1 \\
    &= \frac{1 - \cos(\hat \theta + \theta)}{1 - \cos(\hat \theta)} - e^{\cot(\bar \alpha) \theta} - K \ell_1,
\end{align*}



We start by using the optimality procedure we outlined above.

We want to study the minimum of the ratio $\frac{\hat r_0}{L}$. We consider as base guess the 

{\it Case 1.}

    
\end{proof}


\newpage


\subsection{Computations for the perturbations}
\label{Ss:perturb_segment}


After the angle $\bar \theta - \bar \alpha$ we use the computation for the solution, resetting the angle to $0$


\subsubsection{Angle $0 \leq \phi \leq 2\pi + \bar \alpha - \theta - \hat \theta$}
\label{Sss:first_half_round_segment}


In this case the solution is
\begin{equation*}
    \delta \tilde r(\phi) = \delta r_0 e^{\cot(\bar \alpha)}, \quad \delta r_0 = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta)),
\end{equation*}
and the above quantities are thus computed as
\begin{equation*}
    Q_1 = Q_2 = 0, \quad L = 0,
\end{equation*}
(wrong use the original formula)
\begin{equation*}
    \hat \ell_0 = \hat r_0 \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \sim .314 \hat r_0,
\end{equation*}
\begin{equation*}
    \hat r_2 = \hat r_0 \frac{\sin(\bar \alpha) ( 2 \cos(\bar \alpha) - \cos(\bar \alpha + \hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \sim 1.23979 \hat r_0 > \delta r_2 = e^{\cot(\bar \alpha) \hat \phi)} \sim 1.23309 \hat r_0.
\end{equation*}
Hence we get that the solution is greater that $\delta r$ and then
\begin{equation*}
    \hat r - \hat \ell_0 \geq \delta r - \hat \ell_0 \geq (1 - .314) \hat r_0 > 0
\end{equation*}
if $\delta r \geq \hat r_0$. This is verified by our solution. Notice that
\begin{equation*}
    (\hat r_2 - \tilde r_2) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} - \hat \ell_0 = - 0.19428 \hat r_0,
\end{equation*}
so we have verified that we have a better solution.


\subsubsection{Angle $2\pi + \bar \alpha - \theta - \hat \theta \leq \phi \leq 2\pi + \bar \alpha - \hat \theta$}
\label{Sss:negative_1_segm}


Here we consider first the case where the starting point of the tent is before $2\pi + \theta_0$ and the end point of the tent is before $2\pi + \bar \theta$. Then
\begin{equation*}
    \delta L = \delta s_0, \quad Q_2 - Q_1 = \delta s_0 e^{\i \theta_0}.
\end{equation*}
In the coordinates with $\bar \phi - \bar \alpha = 0$ we have
\begin{equation*}
    Q_2 - Q_1 = \delta s_0 e^{\i \check \theta}, \quad 0 \leq \check \theta \leq \hat \theta,
\end{equation*}
and the condition that the starting point of the tent is again $r(\phi_0)$ is that
\begin{equation*}
    \bar \theta - \theta_0 \geq \hat \theta - \phi_1.
\end{equation*}
Hence the configuration is when $L = |\Delta Q|$, with an initial angle $\check \theta$:
\begin{equation*}
    \hat r_0 = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta)) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \bar \theta - \check \theta)},
\end{equation*}
\begin{align*}
    \hat \ell_0 &= \hat r_0 \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - \frac{1 - \cos(\hat \theta - \check \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{align*}
\begin{equation*}
    \hat r_2 = \hat r_0 \frac{\cos(\bar \alpha) - \cos(\bar \alpha + \hat \theta)}{\cos(\bar \alpha - \hat \theta)) - \cos(\bar \alpha)} + \frac{1}{\sin(\bar \alpha)} \frac{\cos(\hat \theta - \check \theta) - 1}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - \frac{\cos(\bar \alpha + \check \theta)}{\sin(
    \bar \alpha)}
\end{equation*}

We next use the following lemma.

\begin{lemma}
    \label{Lem:convex_base_tent}
    Assume that the base of tent (i.e. the region between is convex): then $\hat r_2 \geq \tilde r_2$.
\end{lemma}

\begin{proof}
The solution for the saturated spiral is written as
\begin{equation*}
    \tilde r_2 = e^{\cot(\bar \alpha) \hat \theta} \hat r_0 - \int_0^{\hat \theta} e^{\cot(\bar \alpha) (\hat \theta - \phi)} dL(d\phi).
\end{equation*}
The coefficient inside the integral is
\begin{equation*}
    \leq e^{\cot(\bar \alpha) \hat \theta} = 1.23309,
\end{equation*}
while the coefficient for $L$ in front of $\hat r_2$ is $1.31181$: we conclude that the the more length we have the more $\hat r_2$ decreases comnpared to $\tilde r_2$.

Hence the worst case is for the maximal length, which corresponds to the initial point of $\hat r_2$ on $\hat r_0$. In this case it is computed before to be
\begin{equation*}
    \hat r_2 - \tilde r_2 \geq 0.0066943 \hat r_0 \geq 0. 
\end{equation*}
\end{proof}

We thus conclude that this situation is verified every time we have the solution of the perturbation can be represented as a local spiral.

In particular, at the angle $\bar \phi + w\pi + \hat \theta$ we obtain
\begin{equation*}
    \geq r(\bar \phi + 2\pi + \hat \theta) - 0.313453 \hat r_0,
\end{equation*}
and this is verified after the first round.

In general, the end point $Q_2 - Q_1$ for the tent up to $4\pi + 2 \bar \alpha - \hat \theta$ is the ray $\delta r$, which is pointing inside the tent, and the variation of length estimate of the above lemma should apply.

Another important observation is that if $r$ in the base of the tent is positive, then it corresponds locally to a convex curve, so that the previous lemma applies.

{\bf The other case for segment}


In the case
\begin{equation*}
    0 \leq \check \theta \leq \phi + \theta \leq \hat \theta,
\end{equation*}
the variation of length is
\begin{align*}
    L &= \delta s_0 + \delta |P_2 - P_1| - \frac{r_2 \delta \theta}{\sin(\bar \alpha)} + \int_{\check + \bar \theta}^{\hat \theta} \frac{\delta r}{\sin(\bar \alpha)} d\phi \\
    &= \frac{1- \cos(\theta)}{\sin(\bar \alpha)^2} + \frac{1 - \cos(\theta)}{\sin(\bar \alpha)} \big( e^{\cot(\bar \alpha) (\hat \theta - \bar \theta - \check \theta)} - 1 \big),
\end{align*}
\begin{equation*}
    \Delta Q = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta)) e^{\cot(\bar \alpha) ( \hat \theta - \bar \theta - \check \theta)} e^{\i (\hat \theta - \bar \alpha)},
\end{equation*}
\begin{equation*}
    \hat r_0 = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta)) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \theta - \check \theta)},
\end{equation*}
\begin{align*}
    \hat \ell_0 &= \frac{\frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta)) \cos(\bar \alpha) - \frac{1- \cos(\theta)}{\sin(\bar \alpha)^2} - \frac{1 - \cos(\theta)}{\sin(\bar \alpha)} \big( e^{\cot(\bar \alpha) (\hat \theta - \bar \theta - \check \theta)} - 1 \big) + \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta)) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \theta - \check \theta)} \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
    &= \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2 (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg( \cos(\bar \alpha^2 - 1 - \sin(\bar \alpha) (e^{\cot(\bar \alpha) (\hat \theta - \theta - \check \theta)} - 1) + \cos(\bar \alpha) \sin(\bar \alpha) \cos(\hat \theta) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \theta - \check \theta)} \bigg) \\
    &\leq \hat r_0 \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{align*}
\begin{align*}
    \hat r_2 &= 
\end{align*}

I think we can apply the same reasoning of increasing $L$, showing in this case that it is still below $\tilde r$.






\subsubsection{The second round - segment and tent}
\label{Sss:second_round_tent}


The part where the base of the tent is convex can still be treated as before.






\newpage





\subsubsection{It is a tent?}
\label{Sss:tent?_true?}


A previous proposition gives that the solution in the saturated zone is a tent. However in the non saturated zone the solution can be an arc: consider for example a situation where one follows the segment as much as possible. Then the limit case is a triangle starting from the origin with sides $\ell_i$, $i = 1,2,3$ such that
\begin{equation*}
    \ell_3 = \cos(\bar \alpha) (\ell_0 + \ell_1).
\end{equation*}
This is an ellipse, with minimal angle at the vertex
\begin{equation*}
    \pi - 2\bar \alpha < \frac{\pi}{2}.
\end{equation*}
Hence it is an arc.

So the distinction here is as follows:
\begin{itemize}
    \item One take the fastest closing spiral, obtaining $\bar \theta \in [0,\frac{\pi}{2}]$ and $\Delta \phi$
    \item if $\bar \phi$ is in the region of negativity, we follow the segment of direction $\bar \phi$ until we arrive at the boundary of the region
    \item the fastest closing spiral at that final points determines if we are in a segment or an arc.
\end{itemize}

\begin{proposition}
    \label{Prop:it_is_unique}
    The above procedure determines a unique length $\ell_0$ in the direction $\bar \phi$.
\end{proposition}

\begin{proof}
    The derivative of the initial angle is $\delta \bar \theta$.

    In the segment case the above derivative is positive, so that the angle $\theta$ is increasing. Either we reach $\hat \theta$ or we arrive at $\bar \theta = \frac{\pi}{2}$, where the arc start.

In the arc case, the derivative of the angle is
\begin{equation*}
    \frac{\sin(\theta_0)}{r_0} \geq \frac{\cos(\hat \theta)}{r_0} > 0,
\end{equation*}
where we have used that in any case the region of negativity for the arc is smaller than the one for the segment. From the formulas
\begin{align*}
    \delta \Delta \phi + \delta \theta = \frac{\sin(\theta)(1 - \cot(\bar \alpha) \Delta \phi) - \cot(\bar \alpha) (1 - \cos(\theta))}{|P_2 - P_1|} = \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha) - \Delta \phi \cos(\bar \alpha) \sin(\theta)}{\sin(\bar \alpha) |P_2 - P_1|}.
\end{align*}
This quantity is increasing as $\Delta \phi$ decreases, showing that the worst situation is when $\Delta \phi = \tan(\bar \alpha)$.





\end{proof}

\newpage


The previous computation settles the analysis in all cases where the fastest closing solution has positive perturbation.

It settles also the case for the initial angle where the segment $\ell_0$ starts from the $\phi_{-1}$.

The only case not covered in the arc case, in the negativity region close to $\Delta \phi = 0$.





\newpage


The previous analysis shows if $\phi_0 - \phi > 2\pi + \tan(\bar \alpha) + \frac{\pi}{2}$, then the optimal choice is the saturated spiral. 

In particular, when $\phi_0 \geq 2\pi + 2 \tan(\bar \alpha) + \pi - \bar \alpha$, the starting point of the region of negativity is a saturated point. Hence, we can continue this initial point until $\phi_0$ is the tangent to the ray.

Next, one has to continue along the segment (otherwise we are entering into the region of positivity), until we exit the region of negativity. We ask here is this final point of the segment is still in the segment case or in the arc case.

Consider the case where the fire is in the initial point of the ray $r(\phi_0)$, and no other barrier exists: then the level sets of $u$ makes a larger angle with the ones of this simplified solution.

Begin the fire faster, it follows that for the simplified solution the angle is slower, so that we arrive to the following worst case.


\subsection{Computations for the worst case}


The initial fire is the ball $B_1(0)$, the segment starts at $P_0 = (1,0)$ with angle $\bar \alpha$ up to the point $P_1$ (the variable is the angle $\theta_1 = \angle(P_0OP_1) \in (0,\bar \alpha]$), then a segment up to a point $P_2$ where it forms an angle $\bar \alpha = \angle(OP_2P_1)$ (the angle is $\theta_2 = \angle(P_2OP_1P_0) \in [0,\pi-\bar\alpha]$): setting $|P_1 - O| = \sin(\bar \alpha)$ for scaling,
\begin{equation*}
    \frac{\sin(\bar \alpha)}{\sin(\pi-\bar \alpha)} = \frac{|P_1 - P_0|}{\sin(\theta_1)} = \frac{|P_0 - O||}{\sin(\pi - (\pi - \bar \alpha) - \theta_1)},
\end{equation*}
\begin{equation*}
    \frac{\sin(\bar \alpha)}{\sin(\bar \alpha)} = \frac{|P_2 - O|}{\sin(\pi - \bar \alpha - \theta_2)} = \frac{|P_2 - P_1|}{\sin(\theta_2)}.
\end{equation*}
Saturation condition
\begin{equation*}
    \begin{split}
        0 &= |P_2 - O| - |P_0 - O| - \cos(\bar \alpha) \big( |P_1 - P_0| + |P_2 - P_1| \big) \\
        &= \sin(\theta_2+\alpha) - \sin(\alpha - \theta_1) - \cos(\bar \alpha) \big( \sin(\theta_1) + \sin(\theta_2) \big) \\
        &= \sin(\bar \alpha) \big( \cos(\theta_2) - \cos(\theta_1) \big).%\frac{\sin(\check \theta + \theta)}{\sin(\check \theta)} - 1 - \cos(\bar \alpha) \bigg( \frac{\sin(\bar \alpha - \check \theta)}{\sin(\bar \alpha)} + \frac{\sin(\theta+ \check \theta - \bar \alpha)}{\sin(\check \theta)} \bigg)
    \end{split}
\end{equation*}
Hence $\theta_1 = \theta_2 = \theta$ and the angle between the segment $P_0P_1$ and the segment $P_1P_2$ is %of the ray at $P_1$ is
\begin{equation*}
    2\theta.
\end{equation*}
So the saturation conditions implies that the angle growths until we arrive at $\theta = \frac{\hat \theta}{2}$. %The critical angle is
%\begin{equation*}
%    \theta = \frac{\hat \theta}{2} = .253,
%\end{equation*}
%and then
%\begin{equation*}
%    \bar \alpha + \frac{\hat \theta}{2} = 1.43137 < \frac{\pi}{2}. 
%\end{equation*}
We thus conclude with the following

\begin{proposition}
    \label{Prop:optima_after}
    For $\phi_0 \geq 2\pi + \frac{\pi}{2} + \tan(\bar \alpha)$, the optimal solution is a segment.
\end{proposition}

\begin{proof}
%We need to prove that the worst case is the one above.
%
Let $P_0$ be the starting point of the first segment, and $O_0$ the base point of $r(\phi_0)$, and similarly for the other points $P_1$, $O_1$ (starting point of the second segment and end point of the first segment), $P_2$, $O_2$, last point before the saturated spiral. The angles are
$$
\angle(P_1P_0O_0) = \pi - \bar \alpha, \quad \angle(O_2P_2P_1) = \bar \alpha.
$$
Let $O'$ be the intersection of the line through the points $O_2,P_2$ and the segment $O_0P_0$. Hence the angle $\theta$ is
\begin{equation*}
    \theta = \angle(P_0O'P_2),
\end{equation*}
as in the case above.

Choosing this angle as a parameter, for all previous angles (up to the critical), one construct the parallelogram and finds the saturates point $P_2$: the point $P_1$ is increasing with $\theta$, because $P_1P_2$ is in the non saturated region. Hence, taking a smaller angle, the ray with that angle will intersect $P_1P_2$ in a point $P_2'$ non saturate: in particular, coming back with a segment of angle alpha, we are still in the non saturated part, and then the saturated is closer to $P_0$.
\end{proof}
%{\bf The numerical simulation shows that it is never satisfied at the critical angle $.5$, which means that we cross to the arc case. Hence the structure is determined for large angles, while for the second round it is not clear. MI VIENE IL PRURITO DI FARLO!}


\subsection{A new parametric spiral}
\label{Ss:parametric_spiral}


Given an angle $\phi_0$, we consider the new parametric spirals as follows:
\begin{itemize}
    \item for $\phi < \phi_0 - 2\pi + \bar \alpha$, we solve the asymptotic optimal spiral;
    \item for $\phi = \phi_0 - 2\pi + \bar \alpha$, we follow the direction $\phi_0$ for a length $\ell_0$;
    \item then we follows the optimal closing spiral for $\phi > 2\pi + \bar \alpha$. 
\end{itemize}
We set
\begin{equation*}
    P_{-1} = \zeta(\phi_0-2\pi-\bar \alpha-), \quad P_0 = \zeta(\phi_0 - 2\pi - \bar \alpha),
\end{equation*}
and $P_1,P_2$ as in the previous construction.

The parameter for optimality is the lenght $\ell_0$, and the previous computation shows the following:

\begin{lemma}
\label{Lem:optima_ell_0}
The angle $\theta$ or $\Delta \phi$ is increasing when $\ell_0$ is increasing, so that there an optimal value $\hat \theta$ or $\widehat{\Delta \phi}$.
\end{lemma}

\begin{proof}
    When the starting point is saturated, the case is the one of Proposition \ref{Prop:optima_after}. Here, the angle $\bar \theta(\ell_0)$ is monotonically increasing in $\ell_0$.

In the segment case it holds (recall \eqref{Equa:delta_bar_theta_segment})
\begin{align*}
    \delta \bar \theta = \delta (\bar \theta - \theta_0) &= \frac{\delta s}{|P_2 - P_1|} \big( \cot(\bar \alpha) \cos(\bar \theta - \theta_0) - (1 - \sin(\bar \theta - \theta_0) \big) \\
    &= \frac{\delta s}{|P_2 - P_1|} \frac{\cos(\bar \alpha - (\bar \theta - \theta_0)) - \cos(\bar \alpha)}{\sin(\bar \alpha)}.
\end{align*}
Hence the angle is growing up until we arrive at the critical angle $\hat \theta \sim .5$.
\end{proof}

\begin{corollary}
    \label{Cor:optimal_ell_0}
    There exists a unique value $\ell_0$ for which the value $r(\phi_0)$ is minimal.
\end{corollary}


\subsubsection{The perturbation along the spiral}
\label{Sss:perturb_optima_along_spiral}


We study the variation of the final values for different starting points.

\begin{description}
    \item[Starting point $P_0$] the initial angle is $\phi_0$, with curvature $\frac{r(\phi_0)}{\sin(\bar \alpha)}$: then a variation of $\delta s$ on the initial point determines a variation of the tangent of an angle
    \begin{equation*}
        \delta \psi_0 = \frac{\delta s \sin(\bar \alpha)}{r(\phi_0)}, \quad \delta P_0 = \delta s \sin(\hat \theta) \mathbf e_1 + \delta s \cos(\hat \theta) \mathbf e_2.
    \end{equation*}

\item[Point $P_1$] in the coordinates with the second axis along $P_2 - P_1$, the new position of $P_1 + \delta P_1$ is
\begin{align*}
    \delta P_1 &= \Big\{ \big[ \delta s + \delta \ell_0 \big] \sin(\hat \theta) - \ell_0 \delta \psi_0 \cos(\hat \theta) \Big\} \mathbf e_1 + \Big\{ \big[ \delta s + \delta \ell_0 \big] \cos(\hat \theta) + \ell_0 \delta \psi_0 \sin(\hat \theta)\Big\} \mathbf e_2.
\end{align*}
The slope of the final point has a variation of $\delta \psi_0$.

\item[Point $P_2$] the variation of the point $P_2$ in the previous coordinates is
\begin{align*}
    \delta P_2 &= \Big\{ \big[ \delta s + \delta \ell_0 \big] \sin(\hat \theta) - \ell_0 \delta \psi_0 \cos(\hat \theta)  - |P_2 - P_1| \delta \psi_0) \Big\} \mathbf e_1 \\
    & \quad + \Big\{ \big[ \delta s + \delta \ell_0 \big] \cos(\hat \theta) + \ell_0 \delta \psi_0 \sin(\hat \theta) + \delta |P_2 - P_1|) \Big\} \mathbf e_2.
\end{align*}
In the coordinates of the fire ray at $\phi_2$ we obtain
\begin{align*}
\delta P_2 &= \Big\{ \big[ (\delta s + \delta \ell_0 \big) \sin(\hat \theta) - \ell_0 \delta \psi_0 \cos(\hat \theta)  - |P_2 - P_1| \delta \psi_0 \big] \sin(\bar \alpha) + \big[ (\delta s + \delta \ell_0) \cos(\hat \theta) + \ell_0 \delta \psi_0 \sin(\hat \theta) + \delta |P_2 - P_1| \big] \cos(\bar \alpha) \Big\} \mathbf e_1' \\
& \quad + \Big\{ - \big[ (\delta s + \delta \ell_0 \big) \sin(\hat \theta) - \ell_0 \delta \psi_0 \cos(\hat \theta)  - |P_2 - P_1| \delta \psi_0 \big] \cos(\bar \alpha) + \big[ (\delta s + \delta \ell_0) \cos(\hat \theta) + \ell_0 \delta \psi_0 \sin(\hat \theta) + \delta |P_2 - P_1| \big] \sin(\bar \alpha) \Big\} \mathbf e_2' \\
&= \Big\{ (\delta s + \delta \ell_0 \big) \cos(\bar \alpha - \hat \theta) - \ell_0 \delta \psi_0 \sin(\bar \alpha - \hat \theta) - |P_2 - P_1| \delta \psi_0 \sin(\bar \alpha) + \delta |P_2 - P_1| \cos(\bar \alpha) \Big\} \mathbf e_1' \\
& \quad + \Big\{ (\delta s + \delta \ell_0 \big) \sin(\bar \alpha - \hat \theta) + \ell_0 \delta \psi_0 \cos(\bar \alpha - \hat \theta) + |P_2 - P_1| \delta \psi_0 \cos(\bar \alpha) + \delta |P_2 - P_1| \sin(\bar \alpha) \Big\} \mathbf e_2'
\end{align*}
%At the first order
%\begin{align*}
%    \delta P_2 &= \Big\{ \big[ \delta s + \delta \ell_0 \big] \sin(\hat \theta) - \delta \ell_0  - |P_2 - P_1| \delta \psi_0) \Big\} \e_1 \\
%    & \quad + \Big\{ \big[ \delta s + \delta \ell_0 \big] \cos(\hat \theta) + \ell_0 \delta \psi_0 + \delta |P_2 - P_1| \Big\} \e_2.
%\end{align*}
The saturation is
\begin{align*}
    0 &= \sin(\bar \alpha) \Big\{ \big[ \delta s + \delta \ell_0 \big] \sin(\hat \theta) - \ell_0 \delta \psi_0 \cos(\hat \theta) - |P_2 - P_1| \delta \psi_0 \Big\} \\
    & \quad + \cos(\bar \alpha) \Big\{ \big[ \delta s + \delta \ell_0 \big] \cos(\hat \theta) + \ell_0 \delta \psi_0 \sin(\hat \theta) + \delta |P_2 - P_1| \Big\} \\
    & \quad - \cos(\bar \alpha) \big\{ \delta s + \delta \ell_0 + \delta |P_2 - P_1| \big\} \\
    &= (\delta s + \delta \ell_0) \big( \cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha) \big) - \ell_0 \delta \psi_0 \sin(\bar \alpha - \hat \theta) - |P_2 - P_1| \delta \psi_0 \sin(\bar \alpha).  
\end{align*}
Simplifying
\begin{align*}
    \delta \ell_0 \big( \cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha) \big) = \delta s \bigg[ - \big( \cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha) \big) + \big( |P_1 - P_0| \sin(\bar \alpha - \hat \theta) + |P_2 - P_1| \sin(\bar \alpha) \big) \frac{ \sin(\bar \alpha)}{r(\phi_0)} \bigg].
\end{align*}
\begin{align*}
    (\delta s + \delta \ell_0) \big( \cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha) \big) = \big( |P_1 - P_0| \sin(\bar \alpha - \hat \theta) + |P_2 - P_1| \sin(\bar \alpha) \big) \delta \psi_0.
\end{align*}
%At the first order
%\begin{align*}
%    0 &= \sin(\bar \alpha) \big[ (\delta s + \delta \ell_0) \cos(\hat \theta) - |P_2 - P_1| \delta \psi_0 \big] \sin(\bar \alpha) + \big[ \ell_0 \delta \psi_0 + \delta |P_2 - P_1| \big] \cos(\bar \alpha).
%\end{align*}
The other relation we have to use is that the angle of $P_2 - P_1 + \delta P_2 - \delta P_1$ with the fire at the end is $\bar \alpha$: the slope of the ray is
\begin{align*}
    r(\phi_2) \delta \psi_0 &= \Big\{ (\delta s + \delta \ell_0 \big) \sin(\bar \alpha - \hat \theta) + \ell_0 \delta \psi_0 \cos(\bar \alpha - \hat \theta) + |P_2 - P_1| \delta \psi_0 \cos(\bar \alpha) + \delta |P_2 - P_1| \sin(\bar \alpha) \Big\} \\
    &= \delta \psi_0 \bigg\{ \frac{|P_1 - P_0| \sin(\bar \alpha - \hat \theta) + |P_2 - P_1| \sin(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \sin(\bar \alpha - \hat \theta) + |P_1 - P_0| \cos(\bar \alpha - \hat \theta) + |P_2 - P_1| \cos(\bar \alpha) \bigg\} + \delta |P_2 - P_1| \sin(\bar \alpha) \\
    &= \delta \psi_0 \bigg\{ |P_1 - P_0| \frac{1 - \cos(\bar \alpha - \hat \theta) \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + |P_2 - P_1| \frac{\cos(\hat \theta) - \cos(\bar \alpha)^2}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg\} + \delta |P_2 - P_1| \sin(\bar \alpha)
    %- \cos(\bar \alpha) \Big\{ \big[ \delta s + \delta \ell_0 \big] \sin(\hat \theta) - \delta \ell_0  - |P_2 - P_1| \delta \psi_0) \Big\} + \sin(\bar \alpha) \Big\{ \big[ \delta s + \delta \ell_0 \big] \cos(\hat \theta) + \ell_0 \delta \psi_0 + \delta |P_2 - P_1| \Big\}.
\end{align*}
and then we must have
\begin{align*}
\delta |P_2 - P_1| \sin(\bar \alpha) &= \delta s \bigg[ - \sin(\bar \alpha - \hat \theta) + \big( r(\phi_2) - |P_1 - P_0| \cos(\bar \alpha -\hat \theta) - |P_2 - P_1| \cos(\bar \alpha) \big)\frac{\sin(\bar \alpha)}{r(\phi_0)} \bigg] - \delta \ell_0 \sin(\bar \alpha - \hat \theta) \\
&= \delta \psi_0 \bigg\{ r(\phi_2) - |P_1 - P_0| \frac{1 - \cos(\bar \alpha - \hat \theta) \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - |P_2 - P_1| \frac{\cos(\hat \theta) - \cos(\bar \alpha)^2}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg\}.
\end{align*}
Hence the sizes of the variation of the segments are determined.
\end{description}

The equation of the solution from $\phi_0$ is as follows: let $\phi_0$ be the angle for $P_0$ (before was the angle from $P_0$), $\phi_1$ the angle for $P_1$, $\phi_2$ the angle for $\phi_2$ and $\bar \phi$ the angle of the slope of the segment $P_1 - P_0$.
\begin{description}
    \item[$\phi < \phi_0$] here we have the saturated spiral
    \begin{equation*}
        \dot r(\phi) = \cot(\bar \alpha) r(\phi) - \frac{r(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)};
    \end{equation*}
    \item[$\phi \in [\phi_0,\phi_1)$] segment $[P_0,P_1)$;
    \item[$\phi \in [\phi_1,\phi_2)$] segment $[P_1,P_2)$;
    \item[$\phi \in [\phi_2,\bar \phi)$] saturated spiral as above;
    \item[$\phi = \bar \phi$] jump $- \ell_0 = |P_1 - P_0|$.
\end{description}
We need to compute the variation of $r(\bar \phi)$ when we change $\bar \phi$ of the angle $\delta \psi_0$.

The solution at $\bar \phi$ is then computed as
\begin{equation*}
    r(\bar \phi) = r(\phi_2) e^{\cot(\bar \alpha) (\bar \phi - \phi_2)} - \int_{\phi_2}^{\bar \phi} e^{\cot(\bar \alpha)(\bar \phi - \phi')} \frac{r(\phi' - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} d\phi' - \ell_0.
\end{equation*}
Notice that $\bar \phi - \phi_2 = 2\pi + \bar \alpha - \theta$ is constant, due to the relation at point $P_2$. Its derivative w.r.t. $\bar \phi$ is then
\begin{align*}
    \delta r(\bar \phi) &= \delta r(\phi_2) e^{\cot(\bar \alpha)(\bar \phi - \phi_2)} - e^{\cot(\bar \alpha)(\bar \phi - \phi_2)} \int_0^{\bar \phi - \phi_2} \frac{e^{-\cot(\bar \alpha) \phi'}}{\sin(\bar \alpha)} \dot r(\phi_2 + \phi' - 2\pi - \bar \alpha) d\phi' - \delta \ell_0 \\
    &= \delta r(\phi_2) e^{\cot(\bar \alpha)(\bar \phi - \phi_2)} - \frac{r(\bar \phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} + \frac{e^{\cot(\bar \alpha)(\bar \phi - \phi_2)} r(\phi_2 - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} \\
    & \quad - e^{\cot(\bar \alpha) (\bar \phi - \phi_2)} \cot(\bar \alpha) \int_0^{\bar \phi - \phi_2} \frac{e^{-\cot(\bar \alpha) \phi'}}{\sin(\bar \alpha)} r(\phi_2 + \phi' - 2\pi - \bar \alpha) d\phi' - \delta \ell_0 \\
    &= \delta r(\phi_2) e^{\cot(\bar \alpha)(\bar \phi - \phi_2)} - \frac{r(\bar \phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} + \frac{e^{\cot(\bar \alpha)(\bar \phi - \phi_2)} r(\phi_2 - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} \\
    & \quad - \cot(\bar \alpha) r(\phi_2) e^{\cot(\bar \alpha) (\bar \phi - \phi_2)} + \cot(\bar \alpha) r(\bar \phi-) - \delta \ell_0 \\
    &= \big( \delta r(\phi_2) - \dot r(\phi_2) \big) e^{\cot(\bar \alpha)(\bar \phi - \phi_2)} + \dot r(\bar \phi-) - \delta \ell_0.
\end{align*}
The first quantity can be estimated as
\begin{align*}
    \big( \delta r(\phi_2) - \dot r(\phi_2) \big) \sin(\bar \alpha) &= (\delta s + \delta \ell_0) \sin(\hat \theta) - \ell_0 \delta \psi_0 \cos(\hat \theta) - \ell_1 \delta \psi_0 \\
    &= \frac{\delta \psi_0}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \Big[ \ell_0 \big( \sin(\bar \alpha - \hat \theta) \sin(\hat \theta) - \cos(\hat \theta) (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)) \big) \\
    & \qquad \qquad \qquad + \ell_1 \big( \sin(\bar \alpha) \sin(\hat \theta) - (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)) \Big] \\
    &= - \delta \psi_0 \frac{\ell_1 \cos(\bar \alpha) (1 + \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}.
\end{align*}
The last two terms are
\begin{align*}
    \dot r(\bar \phi) - \delta \ell_0 &= \bigg[ r(\phi_2) e^{\cot(\bar \alpha) (2 \pi + \bar \alpha - \hat \theta)} - \frac{r(\phi_0)}{\sin(\bar \alpha)} \bigg] \delta \psi_0 + \frac{r(\phi_0) \delta \psi_0}{\sin(\bar \alpha)} - \frac{\ell_0 \sin(\bar \alpha - \hat \theta) + \ell_1 \sin(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
    &= \delta \psi_0 \bigg[ r(\phi_2) e^{\cot(\bar \alpha) (2 \pi + \bar \alpha - \hat \theta)} - \frac{\ell_0 \sin(\bar \alpha - \hat \theta) + \ell_1 \sin(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg].
\end{align*}
Hence we obtain
\begin{equation*}
    \frac{dr(\bar \phi)}{d\bar \phi} = \bigg[ r(\phi_2) - \frac{1}{\sin(\bar \alpha)} \frac{\ell_1 \cos(\bar \alpha) (1 + \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] e^{\cot(\bar \alpha) (2 \pi + \bar \alpha - \hat \theta)} - \frac{\ell_0 \sin(\bar \alpha - \hat \theta) + \ell_1 \sin(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}. 
\end{equation*}
%Since
%\begin{equation*}
%    \frac{\cot(\bar \alpha) (1 + \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} = - 8.42, \quad \frac{\sin(\bar \alpha - \hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} = - 6.75, \quad \frac{\sin(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} = - 10.02,
%\end{equation*}
%we see that the derivative is increasing $> r(\phi_2)$, so that the optimal $r(\phi)$ is increasing exponentially as $r(\phi_2)$.


\subsection{How to prove positivity: SEE THE COMPUTATION ABOVE?}
\label{Ss:positive_sol_final}


For a given $\bar \phi$ sufficiently large, we know that the spiral is saturated up to $s^-(\bar \phi-)$, and then it is a segment up to the starting point of a arc-segment because the angle exits the negative region.

We then change the speed after that point to $\sigma' > \bar \sigma$ so that the generalized spirals are diverging: one has to show that
\begin{itemize}
    \item the saturated spiral with changing speed (or more generally the base spirals) is still positive
    \item the derivative of the perturbation is always positive
\end{itemize}


\subsection{Optimal solution}
\label{Ss:optima_solut}


We first compute the optimal solution at various angles. For $\phi \in [0,2\pi + \bar \alpha + \check \theta$ the optimal solution is the saturated spiral.

We compute now the solution for a starting angle $\theta_0$ in $(1,0)$ and a segment of length $\ell_0$, and next the saturated spiral.

\begin{description}
    \item[Point $P_0$]
    \begin{equation*}
        P_0 = \big( 1 + \ell_0 \cos(\theta_0),\ell_0 \sin(\theta_0) \big), \quad (1 + \ell_0 \cos(\theta_0)) \tan(\phi_0) = \ell_0 \sin(\theta_0).
    \end{equation*}
    %The region of definition is
    %\begin{equation*}
    %    \ell_0 \leq \frac{1}{\sin(\theta_0) - \cos(\theta_0)}.
    %\end{equation*}
    \item[Point $P_1$] it follows the arc or radius $1 + \ell_0 \cos(\theta_0)$ for an angle $\Delta \phi$:
    \begin{equation*}
        P_1 = \sqrt{ 1 + \ell_0^2 + 2\ell_0 \cos(\theta_0)} e^{\i (\phi_0 + \Delta \phi)}, \quad r_0 = \sqrt{1 + \ell_0^2 + 2 \ell_0 \cos(\theta_0)}.
    \end{equation*}
    \item[Point $P_2$] this is the end of the segment, it is saturated and has angle $\bar \alpha$:
    \begin{equation*}
        \ell_1 = r_0 \cot(\bar \alpha),
    \end{equation*}
    and the saturation gives $\Delta \phi$:
    \begin{align*}
        0 &= \frac{r_0}{\sin(\bar \alpha)} - \cos(\bar \alpha) \big( \ell_1 + r_0 \Delta \phi + \ell_0 \big) \\
        &= \big( \sin(\bar \alpha) - \cos(\bar \alpha) \Delta \phi) \big) r_0 - \ell_0 \cos(\bar \alpha),
    \end{align*}
    \begin{equation*}
        \Delta \phi = \tan(\bar \alpha) - \frac{\ell_0}{r_0}.
    \end{equation*}
    \item[$\phi = 2\pi$]
    \begin{equation*}
        r(2\pi) = \frac{r_0}{\sin(\bar \alpha)} e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \phi_0 - \Delta \phi - \frac{\pi}{2})} - 1.
    \end{equation*}
    \item[$\phi = 2\pi + \theta_0$]
    \begin{equation*}
        r(2\pi + \theta_0) = \bigg[ \frac{r_0}{\sin(\bar \alpha)} e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \phi_0 - \Delta \phi - \frac{\pi}{2})} - 1 \bigg] e^{\cot(\bar \alpha) \theta_0} - \ell_0. 
    \end{equation*}
\end{description}

The derivative w.r.t. $\ell_0$ is
\begin{align*}
    \partial_{\ell_0} r(2\pi + \theta_0) &= \frac{\delta r_0 - r_0 \cot(\bar \alpha) (\delta \phi_0 + \delta \Delta \phi)}{\sin(\bar \alpha)} e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \phi_0 - \Delta \phi - \frac{\pi}{2} + \theta_0)} - 1 \\
    &= \frac{\frac{\ell_0 + \cos(\theta_0)}{r_0} - \cot(\bar \alpha) \big( \frac{\sin(\theta_0)}{r_0} - \frac{1 + \ell_0 \cos(\theta_0)}{r_0^2} \big)}{\sin(\bar \alpha)} e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \phi_0 - \Delta \phi - \frac{\pi}{2} + \theta_0)} - 1.
\end{align*}
Note that for $\ell_0$ we obtain the formula for the perturbation as in the previous section in the arc case.

This is a monotone function, with a minimum inside the admissible region $\theta_0 \in [0,\frac{\pi}{2}], \ell_0 \geq 0$ only for (numerical computations)
$$
\ell_0 \sim \bigg[ .23 + \bigg( \theta_0 - \frac{\pi}{2} \bigg]^+.
$$
Hence the optimal is up to the angle $2\pi + .1.36$ the saturated spiral, next one takes the segment up to the minimal $r(2\pi + \theta_0)$.


\subsubsection{The segment on the initial circle}
\label{Sss:segment_circle}


Next, we consider the case of a segment leaving tangentially from the initial arc at an angle $\check \phi \in [0,\tan(\bar \alpha))$. Note that
\begin{equation*}
    \check \phi = \bar \phi - 2\pi - \frac{\pi}{2}.
\end{equation*}

\begin{description}
    \item[Angle $[0,\check \phi)$]
    \begin{equation*}
        r(\phi) = 1.
    \end{equation*}
\item[Angle $\phi \in [\check \phi,\phi_0)$] it is a segment of length $\ell_0$ and slope $\check \phi + \frac{\pi}{2}$
    \begin{equation*}
        \ell_0 = \tan(\theta_0), \quad \phi_0 = \check \phi + \theta_0.
    \end{equation*}
    \item[Angle $\phi \in [\phi_0,\phi_1)$] arc of opening $\Delta \phi$
\begin{equation*}
    r(\phi) = r_1 e^{\i \phi}, \quad r_1 = \frac{1}{\cos(\theta_0)}, \quad \phi_1 = \phi_0 + \Delta \phi.
\end{equation*}
\item[$\phi \in [\phi_1,\phi_2)$] segment up to the last saturated point $P_2$ with angle $\bar \alpha$:
\begin{equation*}
    r_2 = \frac{r_1}{\sin(\bar \alpha)}, \quad \phi_2 = \phi_1 + \frac{\pi}{2} - \bar \alpha, \quad \ell_2 = \cot(\bar \alpha) r_1,
\end{equation*}
\begin{align*}
0 &= r_2 - \cos(\bar \alpha) \big( \check \phi + \ell_0 + r_1 \Delta \phi + \ell_2),
\end{align*}
\begin{equation*}
    \Delta \phi = \tan(\bar \alpha) - \cos(\theta_0) \check \theta - \sin(\theta_0).
\end{equation*}
\end{description}

The solution is computed by
\begin{equation*}
    r(\bar\phi) = \bigg[ \frac{1}{\sin(\bar \alpha) \cos(\theta_0)} e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \frac{\pi}{2} - \Delta \phi - \theta_0 - \check \phi} - 1 \bigg] e^{\cot(\bar \alpha) (\frac{\pi}{2} + \check \phi)} - \frac{e^{\cot(\bar \alpha) \check \phi} - 1}{\cot(\bar \alpha)} - \ell_0.
\end{equation*}
Its derivative w.r.t. $\ell_0$ is
\begin{align*}
    \partial r(\bar \phi) &= 
\end{align*}


\section{A new generalized family}
\label{S:new_gen_fam_2}


Fixed the final angle $\bar \phi$, and fixed the spiral up to $s_0$, we define the fastest closing spiral as:
\begin{description}
    \item[$\bar \phi > \phi + 2\pi + \beta^-(\phi)$] these are the angles before the limit angle $\bar \phi$. Here the choice is fastest closing spiral constructed before.
    \item[$\bar \phi = \phi + 2\pi + \beta(\phi)$] here we choose a segment of length $\ell_0$: this length is obtained by minimizing the length $r(\bar \phi)$ as in Section \ref{Sss:perturb_optima_along_spiral}.
    \item[$\bar \phi < \phi + 2\pi + \beta(\phi)$] here we follow again the fastest closing spiral.
\end{description}

Depending on the relative position of $\bar \phi$ and $\phi_0$ and the value of $\Delta \phi$ or $\bar \theta$, several situations may occur.


\subsection{Arc case for the new generalized family}
\label{Ss:arc_case_new_family}


\subsubsection{The starting segment $\ell_0$ is in $r(\phi_0)$}
\label{Sss:starting_phi_0}


The following are the cases when the ray starts in $r(\phi_0)$.

\begin{itemize}
    \item If
\begin{equation*}
    \bar \phi < \phi_0 + 2\pi + \beta^-(\phi_0),
\end{equation*}
then the optimal solution is the one of Section \ref{S:case:study}. This means that the optimal segment is $0$.

In this case, we already know from the optimality that the variation $\delta r$ is positive.

\item If
\begin{equation*}
    \phi_0 + 2\pi + \beta^-(\phi_0) \leq \bar \phi \leq \phi_0 + \bar \theta + 2\pi = \phi_2 + 2\pi - \bar \alpha - 
\end{equation*}
then the segment starts in $r(\phi_0)$ with direction $\bar \phi$, and with a length determined until we reach the critical angle $\bar \theta$. In particular $\ell_0 = 0$ if
\begin{equation*}
    \bar \phi \leq \phi_2 - \bar \theta + 2\pi + \bar \alpha.
\end{equation*}

We know already that before this angle the derivative is positive.

If the choice of the perturbation is after the direction $\bar \phi - 2\pi$, then it is $0$ since the spiral is not varying before $\bar \phi - 2\pi$. The variation is thus positive, since we already know that the variation along the angle $\bar \phi$ is negative.

If we choose a variation at a different angle, we have to compute the variation:
\begin{description}
    \item[Point $P_0$]
    \begin{equation*}
        \delta P_0 = \delta s e^{\i \theta_0}, \quad \delta \phi_0 = \frac{\delta s \sin(\theta_0)}{r(\phi_0)}.
    \end{equation*}
    \item[Point $P_1$]
    \begin{equation*}
        \delta P_1 = \delta P_0 + \delta \ell_0 e^{\i (\phi_0 + \bar \phi)}, \quad \delta \phi_1 = \frac{(\delta P_0 + \delta \ell_0 e^{\i \bar \phi}) \cdot e^{\i \phi_1}}{r(\phi_1)}.
    \end{equation*}
    \item[Point $P_2$]
    \begin{equation*}
        \delta P_2 = \delta P_1 + \delta \ell_1 e^{\i (\phi_0 + \bar \phi + \hat \theta)}.
    \end{equation*}
\end{description}

The angle relation is
\begin{align*}
    0 &= r(\phi_2) \delta \phi_2 = \delta P_2 \cdot e^{\i (\phi_2 + \frac{\pi}{2})} \\
    &= \delta s \cos \bigg( \phi_2 + \frac{\pi}{2} - \phi_0 - \theta_0 \bigg) + \delta \ell_0 \cos \bigg( \phi_2 + \frac{\pi}{2} - \phi_0 - \bar \phi \bigg) + \delta \ell_1 \cos \bigg( \phi_2 + \frac{\pi}{2} - \phi_0 - \bar \phi - \hat \theta \bigg) \\
[\text{taking $\phi_2 \to \phi_2 + \phi_0$}] \quad &= - \delta s \sin(\phi_2 - \theta_0) - \delta \ell_0 \sin(\phi_2 - \bar \phi) - \delta \ell_1 \sin(\phi_2 - \bar \phi - \hat \phi) \\
[\phi_2 = \bar \phi + \hat \theta - \bar \alpha] \quad &= \delta s \sin(\bar \alpha - \hat \theta - \bar \theta + \theta_0) + \delta \ell_0 \sin(\bar \alpha - \hat \theta) + \delta \ell_1 \sin(\bar \alpha).
\end{align*}
The saturation condition is
\begin{align*}
    0 &= \delta t - \cos(\bar \alpha) \delta \ell \\
    &= \delta s \cos(\bar \alpha - \hat \theta - \bar \theta + \theta_0) + \delta \ell_0 \cos(\bar \alpha - \hat \theta) + \delta \ell_1 \cos(\bar \alpha) - \cos(\bar \alpha) \big( \delta s + \delta \ell_0 + \delta \ell_1 \big) \\
    &= - \delta s (\cos(\bar \alpha) - \cos(\bar \alpha - \hat \theta - \bar \theta + \theta_0)) + \delta \ell_0 (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha))
\end{align*}
From the second one we obtain
\begin{equation*}
    \frac{\delta \ell_0}{\delta s} = - \frac{\cos(\bar \alpha - \hat \theta - \bar \theta + \theta_0) - \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
and from the first
\begin{align*}
    \frac{\delta \ell_1}{\delta s} &= - \frac{\sin(\bar \alpha - \hat \theta - \bar \theta + \theta_0) + \frac{\delta \ell_0}{\delta s} \sin(\bar \alpha - \hat \theta)}{\sin(\bar \alpha)} \\
    &= \frac{- \sin(\bar \alpha - \hat \theta - \bar \theta + \theta_0) + \sin(\bar \alpha - \hat \theta) \frac{\cos(\bar \alpha - \hat \theta - \bar \theta + \theta_0) - \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}}{\sin(\bar \alpha)}.
\end{align*} 
The variation of the initial condition is
\begin{align*}
\frac{\delta r(\phi_2)}{\delta s} &= \cos(\bar \alpha - \hat \theta - \bar \theta + \theta_0) + \frac{\delta \ell_0}{\delta s} \cos(\bar \alpha - \hat \theta) + \frac{\delta \ell_1}{\delta s} \cos(\bar \alpha) \\
&= \cos(\bar \alpha - \hat \theta - \bar \theta + \theta_0) + \cos(\bar \alpha - \hat \theta) \frac{\cos(\bar \alpha) - \cos(\bar \alpha - \hat \theta - \bar \theta + \theta_0)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
& \quad + \cot(\bar \alpha) \bigg( - \sin(\bar \alpha - \hat \theta - \bar \theta + \theta_0) - \sin(\bar \alpha - \hat \theta) \frac{\cos(\bar \alpha) - \cos(\bar \alpha - \hat \theta - \bar \theta + \theta_0)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg).
\end{align*}
Its solution at $\bar \phi$ is then
\begin{equation*}
    \frac{\delta r(\bar \phi)}{\delta s} = \bigg[ \frac{\delta r(\phi_2)}{\delta s} e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta - \bar \theta + \theta_0)} - 1 \bigg] e^{\cot(\bar \alpha)(\bar \theta - \theta_0)} - \frac{\delta \ell_0}{\delta s}.
\end{equation*}
Note that everything depends only on the quantity $\bar \theta - \theta_0 \in [0,\frac{\pi}{2}]$.

From numerical computations, the solution is positive, unless the angle is $\theta_0 = \bar \phi$. To check about $\theta_0 = 0$, one can differentiate w.r.t. $\theta_0$ at $\bar \phi - \theta_0 = 0$ obtaining
\begin{equation*}
    0 = - \cos(\bar \alpha - \hat \theta) + \frac{d}{d\theta} \frac{\delta \ell_0}{\delta s} \sin(\bar \alpha - \hat \theta) + \frac{d}{d\theta_0} \frac{\delta \ell_1}{\delta s} \sin(\bar \alpha),
\end{equation*}
\begin{equation*}
    0 = \sin(\bar \alpha - \hat \theta) + \frac{d}{d\theta} \frac{\delta \ell_0}{\delta s} (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)),
\end{equation*}
\begin{equation*}
    \frac{d}{d\theta} \frac{\delta \ell_0}{\delta s} = - \frac{\sin(\bar \alpha - \hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
\begin{equation*}
    \frac{d}{d\theta} \frac{\delta \ell_1}{\delta s} = \frac{\cos(\bar \alpha - \hat \theta) - \frac{d}{d\theta} \frac{\delta \ell_0}{\delta s} \sin(\bar \alpha - \hat \theta)}{\sin(\bar \alpha)},
\end{equation*}
\begin{equation*}
    \frac{d}{d\theta} \frac{\delta r(\phi_2)}{\delta s} = \sin(\bar \alpha - \hat \theta) + \cos(\bar \alpha - \hat \theta) \frac{d}{d\theta} \frac{\delta \ell_0}{\delta s} + \cos(\bar \alpha) \frac{d}{d\theta} \frac{\delta \ell_1}{\delta s},
\end{equation*}
\begin{equation*}
    \frac{d}{d\theta} \frac{\delta r(\bar \phi)}{\delta s} = \frac{d}{d\theta} \frac{\delta r(\phi_2)}{\delta s} e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} - \cos(\bar \alpha) - \frac{d}{d\theta} \frac{\delta \ell_0}{\delta s}.
\end{equation*}
Numerical computations shows that it is always larger that $3$.

\item If the angle $\bar \phi$ is after the angle $\bar \theta$ in the segment case, then we add the tent at the angle $\bar \phi$ later.

More precisely
\begin{itemize}
    \item we follow the segment for the fastest closing spiral up to the angle $\phi_2$. The angle of the corner in $\phi_0$ is $\bar \theta$, which is computed before. the angles are (as usual $\phi_0 = 0$)
    \begin{equation*}
        \phi_2 = \bar \theta - \bar \alpha.
    \end{equation*}
\item we follow the saturated spiral for an angle $\Delta \phi$, so that (the final angle is $\bar \phi + 2\pi$)
\begin{equation*}
    \phi_3 = \phi_2 + \Delta \phi = \bar \phi - \bar \alpha;
\end{equation*}
\item we follow the segment long $\bar \phi$ until we reach the critical angle $\hat \phi$, then we close with the fastest spiral,
\begin{equation*}
    \phi_4 = \phi_3 + \hat \theta;
\end{equation*}
\item next it is a saturated spiral.
\end{itemize}

We compute the perturbation. The first part with angle $\bar \theta$ is compute as before, obtaining
\begin{equation*}
    \delta r_2 = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\bar \theta - \theta_0)).
\end{equation*}
Then the value at $\phi_3 = \bar \phi - \bar \alpha$ is
\begin{equation*}
    \delta r_3 = \delta r_2 e^{\cot(\bar \alpha)(\bar \phi - \phi_2)}.
\end{equation*}
Then the computations are as above with the starting point (recall that the base angle here is $\bar \phi - \bar \alpha$
\begin{equation*}
    \delta P_2 = \delta r_3 e^{\i (\bar \phi - \bar \alpha)}.
\end{equation*}
Thus the variation at the angle $\phi_4 = \phi_3 + \hat \theta$ is
\begin{align*}
    \delta r_4 &= \delta r_3 \frac{\delta r(\phi_2)}{\delta s}(\bar \theta - \theta_0 = \bar \alpha) \\
    &= \delta r_3 \bigg[ \cos(\hat \theta) + \cot(\bar \alpha) \sin(\hat \theta) + \big( \cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha) \sin(\bar \alpha - \hat \theta) \big) \frac{\cos(\bar \alpha) - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg].
\end{align*}
Next it is the saturated spiral up to $\phi_5 = 2\pi + \phi_0 + \theta_0$, where it has a jump of $-1$
\begin{equation*}
    \delta r_5 = \delta r_4 e^{\cot(\bar \alpha) (\phi_5 - \phi_4)} - 1.
\end{equation*}
Then again the saturated spiral up to the second angle $\phi_6 = 2\pi + \bar \alpha + \phi_2$ where there is a jump
\begin{equation*}
    \delta r_6 = \delta r_5 e^{\cot(\bar \alpha)(\phi_6 - \phi_5)} - \sin(\bar \theta - \theta_0) \cot(\bar \alpha) + \cos(\theta - \theta_0) (1 + 2 \cot(\bar \alpha)^2) - 2 \cot(\bar \alpha)^2.
\end{equation*}
Next it is the saturated spiral
\begin{equation*}
    \delta r(\bar \phi + 2\pi) = \delta r_6 e^{\cot(\bar \alpha) (2\pi + \bar \phi - \phi_6)}.
\end{equation*}

We differentiate w.r.t. the initial angle $\bar \phi$: keeping $\theta_0$ fixed, the variations occur at $\phi_3$
\begin{equation*}
    \frac{d\delta r_3}{d\bar \phi} = \cot(\bar \alpha) \delta r_3,
\end{equation*}
at $\phi_4$
\begin{equation*}
    \frac{d\delta r_4}{d\bar \phi} = \cot(\bar \alpha) \delta r_4,
\end{equation*}
the jumps and the angle being the same are not influencing the evolution as a saturated spiral, so that we arrive at $\bar \phi + 2\pi$ as
\begin{equation*}
    \frac{d}{d\bar \phi} \delta r(\bar \phi + 2\pi) = \frac{d\delta r_4}{d\bar \phi} e^{\cot(\bar \alpha) (2\pi - \hat \theta)}.
\end{equation*}
This derivative is positive, and it holds also for perturbations longer than the upper bound. Thus it is increasing, with minimal value at $\bar \phi = \bar \theta - \bar \alpha$.

Just for verification, the computations above (for the first case) with $\bar \phi = \phi_2 + \hat \theta$, becomes
\begin{equation*}
    \delta r_2 = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\bar \theta - \theta_0)),
\end{equation*}
\begin{equation*}
    \delta r_4 = \delta r_2 \bigg[ \cos(\hat \theta) + \cot(\bar \alpha) \sin(\hat \theta) + \big( \cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha) \sin(\bar \alpha - \hat \theta) \big) \frac{\cos(\bar \alpha) - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg],
\end{equation*}
\begin{equation*}
    \delta r_5 = \delta r_4 e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta - \bar \theta + \theta_0)},
\end{equation*}
The numerical computations shows that is it positive. Note that it is discontinuous w.r.t. $\bar \phi$ across the value $\bar \phi = \bar \theta$: indeed in one case the angle $\delta \theta = 0$, while in the other $\delta \theta \not= 0$.



\end{itemize}



\subsection{The final tent}
\label{Ss:final_tent_666}


This is the final tent starting with an initial data $r$ saturated. The relation for saturation with angle $\hat \theta$ is
\begin{equation*}
    P_0' = P_0 + \frac{r(\phi_0)}{\sin(\bar \alpha)} \delta \bar \phi e^{\i \bar \alpha},
\end{equation*}
\begin{equation*}
    P_1' = P_1 + \bigg( \frac{r(\phi_0)}{ \sin(\bar \alpha)} \delta \bar \phi + \delta \ell_0 \bigg) e^{\i \bar \alpha} + \ell_0 \delta \bar \phi e^{\i (\bar \alpha + \frac{\pi}{2})},
\end{equation*}
\begin{equation*}
    P_2' = P_2 + \bigg( \frac{r(\phi_0)}{ \sin(\bar \alpha)} \delta \bar \phi + \delta \ell_0 \bigg) e^{\i \bar \alpha} + \ell_0 \delta \bar \phi e^{\i (\bar \alpha + \frac{\pi}{2})} + \delta \ell_1 e^{\i (\bar \alpha + \hat \theta)} + \ell_1 \delta \bar \theta e^{\i (\bar \alpha + \hat \theta + \frac{\pi}{2})}, 
\end{equation*}
saturation condition
\begin{align*}
    0 &= e^{\i \hat \theta} \cdot \delta P_2 - \cos(\bar \alpha) \bigg( \frac{r_0}{\sin(\bar \alpha)} \delta \bar \phi + \delta \ell_0 + \delta \ell_1 \bigg) \\
    &= \bigg( \frac{r(\phi_0)}{\sin(\bar \alpha)} \delta \bar \phi + \delta \ell_0 \bigg) \big( \cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha) \big) - \ell_0 \delta \bar \phi \sin(\bar \alpha - \hat \theta) - \ell_1 \delta \bar \phi \sin(\bar \alpha),
\end{align*}
\begin{equation*}
    \frac{r_0}{\sin(\bar \alpha)} + \delta \ell_0 = \frac{\ell_0 \sin(\bar \alpha - \hat \theta) + \ell_1 \sin(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
angle relation:
\begin{align*}
    0 &= e^{\i (\bar \theta + \frac{\pi}{2})} \cdot \delta P_2 - r(\phi_2) \delta \bar \phi \\
    &= \bigg( \frac{r(\phi_0)}{\sin(\bar \alpha)} \delta \bar \phi + \delta \ell_0 \bigg) \sin(\bar \alpha - \hat \theta) + \ell_0 \delta \phi \cos(\bar \alpha - \hat \theta) + \delta \ell_1 \sin(\bar \alpha) + \ell_1 \delta \bar \phi \cos(\bar \alpha) - r(\phi_2) \delta \bar \phi \\
    &= \frac{\ell_0 \sin(\bar \alpha - \hat \theta) + \ell_1 \sin(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \sin(\bar \alpha - \hat \theta) \delta \bar \phi + \ell_0 \delta \bar \phi \cos(\bar \alpha - \hat \theta) + \delta \ell_1 \sin(\bar \alpha) + \ell_1 \delta \bar \phi \cos(\bar \alpha) - r(\phi_2) \delta \bar \phi,
\end{align*}
\begin{equation*}
    r(\phi_2) - \delta \ell_1 \sin(\bar \alpha) = \ell_0 \frac{1 - \cos(\bar \alpha - \hat \theta) \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + \ell_1 \frac{\cos(\hat \theta) - \cos^2(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\hat \theta)},
\end{equation*}
variation at the initial angle $\phi_2 = \phi_0 + \hat \theta$:
\begin{align*}
    &= e^{\i \hat \theta} \cdot \delta P_2 - r(\phi_2) \cot(\bar \alpha) \delta \bar \phi \\
    &= \cos(\bar \alpha) \bigg( \frac{r_0}{\sin(\bar \alpha)} \delta \bar \phi + \delta \ell_0 + \delta \ell_1 \bigg) - r(\phi_2) \cot(\bar \alpha) \delta \bar \phi \\
    &= \cot(\bar \alpha) (\ell_1 - \ell_0) \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - \cot(\bar \alpha) r_0 \delta \bar \phi, 
\end{align*}
variation at the final angle $\phi_0 + 2\pi + \bar \alpha$:
\begin{align*}
    &= (r(\bar \phi + 2\pi +  \bar \alpha) + \delta r(\bar \phi + 2\pi + \bar \alpha))(1 + \cos(\bar \alpha) \delta \bar \phi) - \frac{r(\phi_0)}{\sin(\bar \alpha)} \delta \phi - (\ell_0 + \delta \ell_0) - \big[ r(\bar \phi + 2\pi + \bar \alpha) - \ell_0 \big] \\
    &= r(\bar \phi + 2\pi + \bar \alpha) \cot(\bar \alpha) \delta \phi + \delta r(\bar \phi + 2\pi + \bar \alpha) - \delta \ell_0 - \frac{r(\phi_0)}{\sin(\bar \alpha)} \delta \bar \phi,
\end{align*}
final value $\phi_3 = \bar \phi + 2\pi + \bar \alpha$
\begin{align*}
    &r_3 \cot(\bar \alpha) - \frac{r_0}{\sin(\bar \alpha)} + \big[ (\cos(\bar \alpha) (\delta \ell_0 + \delta \ell_1) - r(\phi_2) \cot(\bar \alpha) \big] e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} - \delta \ell_0 \\
    &= \cot(\bar \alpha) r(\phi_3) - \frac{r(\bar \phi)}{\sin(\bar \alpha)} + \Big[ \cot(\bar \alpha) (\ell_1 - \ell_0) \frac{1 - \cos(\hat \theta)}{\cot(\bar \alpha) - \hat \theta) - \cos(\bar \alpha)} - \cot(\bar \alpha) r_0 \Big] e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} -  \frac{\ell_0 \sin(\bar \alpha - \hat \theta) + \ell_1 \sin(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + \frac{r_0}{\sin(\bar \alpha)} \\
    &= \cot(\bar \alpha) r(\phi_3) + \Big[ \cot(\bar \alpha) (\ell_1 - \ell_0) \frac{1 - \cos(\hat \theta)}{\cot(\bar \alpha) - \hat \theta) - \cos(\bar \alpha)} - \cot(\bar \alpha) r_0 \Big] e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} -  \frac{\ell_0 \sin(\bar \alpha - \hat \theta) + \ell_1 \sin(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{align*}
difference of length
\begin{align*}
    \delta \ell_1 - \delta \ell_0 = 
\end{align*}


\subsection{Solution for tent}
\label{Ss:sol_tent}


Assume that we are in the saturated spiral: let
\begin{itemize}
    \item $r_0$ be the initial ray of the first point $P_0$ of the tent at angle $\bar \phi$,
    \item $\bar \phi + \hat \theta_1$ be the angle of $P_1$, the tip of the tent
    \item $\ell_0 = |P_1 - P_0|$, $\ell_1 = |P_2 - P_1|$,
\item $r_2$ be the final ray of lat point $P_2$ of the tent, at angle $\bar \phi + \bar \alpha + \hat \theta$,
\item $\hat P_0$ be the intersection of the line through $P_2$ with slope $e^{\i \hat \theta}$, and $\hat r_0 = |P_0 - \hat P_0|$,
\item $S$ be the length of the saturated spiral between the initial point of $r_0$ and the initial point $\hat P_2$ of $r_2$,
\item $D = |\hat P_2 - \hat P_0|$. 
\end{itemize}

Being saturated after $\phi_2$, the solution can be computed as
\begin{equation*}
    r_2 e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} - \int_{\phi_2}^{\bar \phi + 2\pi + \bar \alpha} e^{\cot(\bar \alpha) (\bar \phi + 2\pi + \bar \alpha - \phi'} R(\phi') d\phi' - \ell_0,
\end{equation*}
where $R(\phi)$ is the curvature radius.

We estimate the above quantities as follows:
\begin{itemize}
    \item the sine-theorem for the quadrilater $\hat P_0 P_0 P_1 P_2$ gives
    \begin{equation*}
        \frac{|P_1 - \hat P_0|}{\sin(\bar \alpha)} = \frac{|P_1 - P_0|}{\sin(\hat \theta_1)} = \frac{|P_2 - P_1|}{\sin(\hat \theta - \hat \theta_1)} = \frac{|P_2 - \hat P_0|}{\sin(\bar \alpha + \hat \theta - \hat \theta_1)} = \frac{|P_0 - \hat P_0|}{\sin(\bar \alpha - \hat \theta_1)},
    \end{equation*}
    \item the saturation condition is
    \begin{align*}
        0 &= |P_2 - \hat P_0| - (r_0 - S + D) - \cos(\bar \alpha) (|P_1 - P_0| + |P_2 - P_1|).
    \end{align*}
\end{itemize}

The maximal value of
\begin{equation*}
    |P_1 - P_0| = |P_1 - \hat P_0| \frac{\sin(\hat \theta_1)}{\sin(\bar \alpha - \hat \theta_1)} \leq r_0 \frac{\sin(\hat \theta)}{\sin(\bar \alpha - \hat \theta)}
\end{equation*}
and being the saturated spiral less that the tent at the angle $\bar \phi_2$ we can estimate
\begin{align*}
    &r_2 e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} - \int_{\phi_2}^{\bar \phi + 2\pi + \bar \alpha} e^{\cot(\bar \alpha) (\bar \phi + 2\pi + \bar \alpha - \phi'} R(\phi') d\phi' - \ell_0 \\
    &\leq r(\bar \phi + 2\pi + \bar \alpha) - r(\bar \phi) \frac{\sin(\hat \theta)}{\sin(\bar \alpha - \hat \theta)}.
\end{align*}
In terms of $\rho$ one gets
\begin{equation*}
    \rho(\bar \tau + 1) - \rho(\bar \tau) e^{-\bar c(2\pi+ \bar \alpha)} \frac{\sin(\hat \theta)}{\sin(\bar \alpha - \hat \theta)}.
\end{equation*}
Hence if $\rho$ is increasing, the tent never closes: this solves also for the perturbation.


\subsubsection{The initial angles}
\label{Ss:initial angle}


For the segment case, the angle $\bar \phi \in [0,\bar \theta]$ one computes:
\begin{equation*}
    \delta P_0 = \delta s e^{\i \theta_0},
\end{equation*}
\begin{equation*}
    \delta P_1 = \delta s e^{\i \theta_0} + \delta \ell_0 e^{\i \bar \phi},
\end{equation*}
\begin{equation*}
    \delta P_2 = \delta s e^{\i \theta_0} + \delta \ell_0 e^{\i \bar \phi} + \delta \ell_2 e^{\i (\bar \phi + \hat \theta)},
\end{equation*}
saturation
\begin{align*}
    0 &= e^{\i (\bar \phi + \hat \theta - \bar \alpha)} \cdot \delta P_2 - \cos(\bar \alpha) (\delta s + \delta \ell_0 + \delta \ell_1) \\
    &= \delta s \big[ \cos(\bar \alpha - \hat \theta - \bar \phi + \theta_0) - \cos(\bar \alpha) \big] + \delta \ell_0 \big[ \cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha) \big],
\end{align*}
\begin{equation*}
    \delta \ell_0 = - \delta s \frac{\cos(\bar \alpha - \hat \theta - (\bar \phi - \theta_0)) - \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
angle
\begin{align*}
    0 &= e^{\i (\bar \phi + \hat \theta - \bar \alpha + \frac{\pi}{2})} \cdot \delta P_2 \\
    &= \delta s \sin(\bar \alpha - \hat \theta - \bar \phi + \theta_0) + \delta \ell_0 \sin(\bar \alpha - \hat \theta) + \delta \ell_1 \sin(\bar \alpha).
\end{align*}
\begin{equation*}
    \sin(\bar \alpha) \delta \ell_1 = \delta s \frac{\sin(\bar \phi - \theta_0) - \cos(\bar \alpha) (\sin(\bar \alpha - \hat \theta) - \sin(\bar \alpha - \hat \theta  - (\bar \phi - \theta_0))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
The value at $\bar \phi + 2\pi + \bar \alpha$ is
\begin{equation*}
    \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\hat \theta)) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} = 1,
\end{equation*}
\begin{align*}
    &e^{\i (\bar \phi + \hat \theta - \bar \alpha)} \cdot \delta P_2 e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} - \delta s e^{\cos(\bar \alpha)(\bar \phi - \theta_0)} - \delta \ell_0 \\
    &= \cos(\bar \alpha) (\delta s + \delta \ell_0 + \delta \ell_1) e^{\cos(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} - \delta s e^{\cos(\bar \alpha) (\bar \phi - \theta_0)} - \delta \ell_0 \\
    &= (\delta s + \delta \ell_0 + \delta \ell_1) \frac{\sin(\bar \alpha)^2}{1 - \cos(\hat \theta)} - \delta s e^{\cos(\bar \alpha) (\bar \phi - \theta_0)} - \delta \ell_0 \\
    &= \delta s \bigg[ \frac{\sin^2(\bar \alpha)}{1 - \cos(\hat \theta)} \bigg( 1 - \frac{\sin(\bar \alpha - \hat \theta - (\bar \phi - \theta_0))}{\sin(\bar \alpha)} \bigg) - e^{\cos(\bar \alpha)(\bar \phi - \theta_0)} \bigg] + \delta \ell_0 \bigg[ \frac{\sin^2(\bar \alpha)}{1 - \cos(\hat \theta)} \bigg( 1 - \frac{\sin(\bar \alpha - \hat \theta)}{\sin(\bar \alpha)} \bigg) - 1 \bigg].
\end{align*}
Numerically the solution is positive, with a derivative for $\bar \phi - \theta_0$ at $0$ of
\begin{align*}
    &\frac{\sin(\bar \alpha)^2}{1 - \cos(\hat \theta)} \bigg( - \frac{\sin(\bar \alpha - \hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg( 1 - \frac{\sin(\bar \alpha - \hat \theta)}{\sin(\bar \alpha)} \bigg) + \frac{\cos(\bar \alpha - \hat \theta)}{\sin(\bar \alpha)} \bigg) - \cot(\bar \alpha) + \frac{\sin(\bar \alpha - \hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
    &= \frac{1 - \cos(2\bar \alpha - \hat \theta)}{\sin(\bar \alpha)(\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha))} > 0.
\end{align*}


\subsection{Arc case for tent}
\label{Ss:arc_case_tent}


For the arc case, we follow the segment until the perturbation exits the negativity region: more precisely,
\begin{enumerate}
    \item if the angle $\bar \phi \geq \theta_0 + \delta \phi + \frac{\pi}{2}$, we apply the tent at that angle;
    \item if $\bar \phi \in \theta_0 + \frac{\pi}{2} + [0,\Delta \phi]$, we follow the direction $\bar \phi$ until we exit the negativity region for the perturbation: this as before is due to the fact that the angle between the fast closing solution and the angle $\bar \theta$ (in the arc case is $\frac{\pi}{2}$) is increasing;
    \item if $\bar \phi \in \theta_0 + [0,\frac{\pi}{2}]$ then the tent starts at $\phi_0$ and then sops when we exit the negativity region.
\end{enumerate}


\subsubsection{Case $\bar \phi \in [0,\frac{\pi}{2}]$}
\label{Sss:arc_case_tent_1}


The final angle is computed as the last angle where when we continue the perturbation becomes positive.

Variation of the points
\begin{equation*}
    \delta P_0 = \delta s e^{\i \theta_0},
\end{equation*}
\begin{equation*}
    \delta P_1 = \delta P_0 + \delta \ell_0 e^{\i \bar \phi},
\end{equation*}
and the variation of $P_1$ is the input of the solution to the arc/segment case for the previous perturbation, which is positive by the choice of the final angle.

This is the correct proof.


\subsection{The base solution}
\label{S:computation_base_solution}


For the base solution, it never happens that the tent can close since $\rho(\tau+1) > .5 \rho(\tau)$.

\subsubsection{Angle $\bar \phi \in [0,\frac{\pi}{2})$}
\label{Sss:base_spiral_tent_1}


We take as variable the length $\ell_0$:
\begin{equation*}
    r = \sqrt{1 + \ell_0^2 + 2 \ell_0 \cos(\bar \phi)}, \quad \phi_0 = \arcsin \bigg( \frac{\ell_0 \sin(\bar \phi)}{r} \bigg),
\end{equation*}
saturation
\begin{align*}
    0 &= \frac{r}{\sin(\bar \alpha)} - \cos(\bar \alpha)(\ell_0 + r \Delta \phi + r \cot(\bar \alpha)) \\
    &= \sin(\bar \alpha) r - r \cos(\bar \alpha) \Delta \phi - \cos(\bar \alpha) \ell_0,
\end{align*}
value of $\delta \phi$ (so it remains an arc)
\begin{equation*}
    \Delta \phi = \tan(\bar \alpha) - \frac{\ell_0}{r} > 0,
\end{equation*}
value at $2\pi + \bar \phi$
\begin{equation*}
    \frac{r}{\sin(\bar \alpha)} e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \frac{\pi}{2} - \Delta \phi + \bar \phi - \phi_0
)} - e^{\cot(\bar \alpha) \bar \phi} - \ell_0, %= \frac{r}{\sin(\bar \alpha)} = \frac{r}{\sin(\bar \alpha)} e^{\cot(\bar \alpha)(2\pi + \bar \alpha + \bar \phi - \frac{\pi}{2} - \tan(\bar \alpha) + \frac{\ell_0}{r})}- e^{\cot(\bar \alpha) \bar \phi} - \ell_0,
\end{equation*}
numerical value larger than 4.5 in all cases.


\subsubsection{$\bar \phi \in [\frac{\pi}{2},\tan(\bar \alpha) + \frac{\pi}{2} - \bar \alpha]$}
\label{Sss:base_spiarl_second_case}


Distance
\begin{equation*}
    r = \sqrt{1 + \ell_0^2}, \quad \Delta \phi_0 = \arctan(\ell_0)
\end{equation*}
saturation if the arc exists
\begin{align*}
    0 &= \frac{r}{\sin(\bar \alpha)} - \cos(\bar \alpha) \bigg( \bar \phi - \frac{\pi}{2} + \ell_0 + r \Delta \phi + r \cot(\bar \alpha) \bigg) \\
    &= \sin(\bar \alpha) r - \cos(\bar \alpha) r \Delta \phi - \cos(\bar \alpha) \bigg( \bar \phi - \frac{\pi}{2} + \ell_0 \bigg),
\end{align*}
\begin{equation*}
    \Delta \phi = \tan(\bar \alpha) - \frac{\ell_0}{r} - \frac{\bar \phi - \frac{\pi}{2}}{r},
\end{equation*}
is instead negative then ($\psi$ the new angle at the center)
\begin{align*}
    0 &= \frac{r \sin(\bar \alpha + \psi)}{\sin(\bar \alpha)} - \cos(\bar \alpha) \bigg( \bar \phi - \frac{\pi}{2} + \ell_0 + \frac{r \sin(\psi)}{\sin(\bar \alpha} \bigg) \\
    &= r \cos(\psi) - \cos(\bar \alpha) \bigg( \bar \phi - \frac{\pi}{2} + \ell_0 \bigg),
\end{align*}
\begin{equation*}
    \cos(\psi) = \cos(\bar \alpha) \bigg( \frac{\bar \phi - \frac{\pi}{2} + \ell_0}{r} \bigg),
\end{equation*}
final value for the arc case
%\begin{equation*}
%    \frac{r}{\sin(\bar \alpha)} e^{\cot(\bar \alpha)(2\pi + \bar \phi - \frac{\pi}{2} + \bar \alpha - \Delta \phi - \Delta \phi_0)} - e^{\cot(\bar \alpha) \bar \phi} - \ell_0 - \frac{e^{\cot(\bar \alpha)(\bar \phi - \frac{\pi}{2})} - 1}{\cot(\bar \alpha)}
%\end{equation*}
\begin{equation*}
    \frac{r}{\sin(\bar \alpha)} e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \Delta \phi_0)} - e^{\cot(\bar \alpha) \bar \phi} - \frac{e^{\cot(\bar \alpha)(\bar \phi - \frac{\pi}{2})} - 1}{\cot(\bar \alpha)} - \ell_0,
\end{equation*}
\begin{equation*}
    \frac{r}{\sin(\bar \alpha)} e^{\cot(\bar \alpha)(2\pi + \frac{\pi}{2} - \Delta \phi_0 - \psi)} - e^{\cot(\bar \alpha) \bar \phi} - \frac{e^{\cot(\bar \alpha)(\bar \phi - \frac{\pi}{2})} - 1}{\cot(\bar \alpha)} - \ell_0,
\end{equation*}
Again the value is positive with a minimum above 6.



\subsection{Asymptotic grow of the spiral}
\label{Ss:asympto_growth}


In the asymptotic case
\begin{equation*}
    \rho(\tau) = 2\tau + \frac{2}{3} + o(1), \quad r(\phi) = \bigg( \frac{2\phi}{2\pi + \bar \alpha} + \frac{2}{3} + o(1) \bigg) e^{\bar c \phi},
\end{equation*}




\section{The final optimal solution}
\label{S:final_optimal}


The initial angle is $\phi_0$, and we want to optimize at $\bar \phi$. At the initial angle $\phi_0$ we have the maximal closing spiral for the first round, which gives an initial angle $\bar \theta$; for the arc case, $\bar \theta = \frac{\pi}{2}$ and there is also the dependence w.r.t. $\Delta \phi$. In both cases, we have that the initial unperturbed situation is defined. Which ever is the situation, there is a region of angles $\bar \theta - \theta_0 = \theta(\Delta \phi)$ such that the derivative is negative.

We next proceed by defining the angles the family of angles
\begin{equation*}
    \bar \phi_k = \bar \phi - (2\pi + \alpha) k, \quad k = 0,\dots,\bar k.
\end{equation*}
The value $\bar k$ is determined as follows: it is the first value for which
$$
\bar \phi_{\bar k+1} < \phi_0 + \bar \theta - \theta(\Delta \phi).
$$
Taking $\phi_0 = 0$ (everything depends on the difference), it holds
\begin{equation*}
    \bar \theta - \theta(\Delta \phi) \leq \bar \phi_{\bar k} \leq \bar \theta \quad \text{or} \quad \bar \theta \leq \bar \phi_k \leq 2\pi + \bar \alpha + \bar \theta - \theta(\Delta \phi).
\end{equation*}

\begin{definition}
    \label{Def:optimal_solution}
    The optimal solution is defined as follows: whenever we arrive to the angle $\bar \phi_k$, we follow a segment until we exit the negativity region (computed in the previous section with final angle $\hat \theta$), and then we use the fastest closing spiral from that point onward.
\end{definition}

We describe now the situation which can occurs. For simplicity, we will write $\bar \phi$ as the angle $\bar \phi_{\bar k}$, so that the computations for the subsequent angles will be done by repeating the construction for a rotation (more details later on).

\begin{description}
    \item[$\bar \theta - \theta(\Delta \phi) \bar \phi \leq \bar \theta$] we follow the segment with direction $\bar \phi$, until the angle of the segment with the fastest closing spiral is outside the negative region; then we use the fastest closing spiral until we arrive at the angle $\bar \phi_1 = \bar \phi + 2\pi + \bar \alpha$, to which we use again the segment, and so on until we are at $\bar \phi_k$.
    \item[$\bar \theta \leq \bar \phi \leq \bar \theta - \theta(\Delta \phi) + 2\pi + \bar \alpha)$] we use the fastest closing spiral until the angle $\bar \phi$, then the segment until we are in the negative region, and then the fastest closing spiral, then the segment at $\bar \phi_1$, etc until $\bar \phi_k$.
\end{description}


\subsection{Equation for the fastest closing spiral}
\label{Ss:fastest_closing_eq}


We have the base spiral $r(\phi)$, $\phi \in [0,\phi_0]$, and we are given the angle $\bar \phi$. By the previous computations we have that the fastest closing solution at the first round is either and arc of a segment.

We consider separately the various cases above: we set $\phi_0 = 0$ by translation. The angle we take as $\bar \phi_1$ is the angle of the first segment in the tent. The first value is when
$$
\phi_0 + \bar \theta - \hat \theta \leq \bar \phi_1,
$$
otherwise it is $0$, and then it proceed up to
$$
\bar \phi_1 < \phi_0 + \bar \theta - \hat \theta + 2\pi + \bar \alpha.
$$
Note that in the last case the last point of the first tent has angle
\begin{equation*}
    \bar \phi_1 + \hat \theta + 2\pi \leq \bar \theta + 2\pi,
\end{equation*}
so that the tent is in the smooth part of the spiral (no jump of $r$, and it can have jumps due to the fixed part before $\phi_0$).


\subsubsection{Fastest closing is a segment with angle $\bar \theta$ and $\bar \phi_0 \in [\bar \alpha - \hat \theta, 2\pi + \bar \theta - \hat \theta)$}
\label{Ss:case_1_optimal}


In this case, the tent is after the fastest closing segment, and the solution is
\begin{description}
    \item[$\phi \in [\phi_0,\bar \theta -\bar \alpha)$] segment
    \begin{equation*}
        \dot r(\phi) = \cot(\bar \theta - \phi) r - R(\phi-), \quad \phi_1 = \bar \theta - \bar \alpha;
    \end{equation*}

\item[$\phi \in [\phi_1,\bar \phi_1)$] saturated spiral
\begin{equation*}
    \dot r(\phi) = \cos(\bar \alpha) r - R(\phi-);
\end{equation*}

\item[$\phi \in [\bar \phi_1,\bar \phi_1 + \hat \theta)$] tent, determined uniquely by the angles and the saturation;

\item[$\phi \in [\bar \phi_1 + \hat \theta,2\pi + \beta(\phi_0))$] saturated spiral
\begin{equation*}
    \dot r  = \cot(\bar \alpha) r - R(\phi-);
\end{equation*}

\item[$\phi \in [2\pi + \beta(\phi_0),2\pi + \hat \theta)$] saturated spiral
\begin{equation*}
    \dot r = \cot(\bar \alpha) r;
\end{equation*}

\item[$\phi \in [2\pi + \hat \theta,\bar \phi_2)$] saturated spiral
\begin{equation*}
    \dot r = \cot(\bar \alpha) r - \frac{r(\phi-)}{\sin(\bar \alpha)};
\end{equation*}

\item[$\phi \in [\bar \phi_k,\bar \phi_k + \hat \theta)$] tent;

\item[$\phi \in [\bar \phi_k + \hat \theta,\bar \phi_{k+1})$] saturated spirals.
\end{description}

We differentiate w.r.t. $\bar \theta$, the initial position of the tent: we notice that at every next tent the geometric relation with the previous one is fixed.

\begin{description}
    \item[$\phi \leq [\phi_0,\bar \phi_1)$] no variation,
\begin{equation*}
    r(\phi) = 0;
\end{equation*}

\item[$\phi \in [\bar \phi_1,\bar \phi_1 + \hat \theta)$] derivative of the tent, determined uniquely by the angles and the saturation: we repeat the computations for verification
\begin{equation*}
    \delta P_0 = \delta s e^{\i \bar \phi_1}, \quad \delta s \sin(\bar \alpha) = r(\bar \phi_1 - 2\pi - \bar \alpha) \delta \bar \phi,
\end{equation*}
\begin{equation*}
    \frac{\delta r(\bar \phi_1 - 2\pi - \bar \alpha)}{\delta \bar \phi_1} = \delta s \cos(\bar \alpha) - R(-) = r(\bar \phi_1 - 2\pi - \bar \alpha) \cot(\bar \alpha) - R(\bar \phi_1 - 2\pi - \bar \alpha-) = \dot r_0,
\end{equation*}
\begin{equation*}
    \delta P_1 = (\delta s + \delta \ell_0) e^{\i \bar \phi_1} + \delta \bar \phi_1 \ell_0 e^{\i (\bar \phi_1 + \frac{\pi}{2})},
\end{equation*}
\begin{equation*}
    \delta P_2 = (\delta s + \delta \ell_0) e^{\i \bar \phi_1} + \delta \bar \phi_1 \ell_0 e^{\i (\bar \phi_1 + \frac{\pi}{2})} + \delta \ell_1 e^{\i (\bar \phi + \hat \theta)} + \ell_1 \delta \bar \phi_1 e^{\i (\bar \phi_1 + \hat \theta + \frac{\pi}{2})},
\end{equation*}
\begin{align*}
    0 &= \delta P_2 \cdot e^{\i (\bar \phi_1 + \hat \theta - \bar \alpha)} - \cos(\bar \alpha) (\delta s + \delta \ell_0 + \delta \ell_1) \\
    &= (\delta s + \delta \ell_0) \cos(\bar \alpha - \hat \theta) - \ell_0 \delta \bar \phi_1 \sin(\bar \alpha - \hat \theta) + \delta \ell_1 \cos(\bar \alpha) - \ell_1 \delta \bar \phi_1 \sin(\bar \alpha) - \cos(\bar \alpha) (\delta s + \delta \ell_0 + \delta \ell_1) \\
    &= (\delta s + \delta \ell_0) (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)) - \ell_0 \delta \bar \phi_1 \sin(\bar \alpha - \hat \theta) - \ell_1 \delta \bar \phi_1 \sin(\bar \alpha), 
\end{align*}
\begin{equation*}
    \delta \ell_0 + \delta s = \frac{\ell_0 \sin(\bar \alpha - \hat \theta) + \ell_1 \sin(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \delta \bar \phi_1,
\end{equation*}
\begin{align*}
    r(\bar \phi_1 - 2\pi - \bar \alpha + \hat \theta) \delta \phi &= \delta P_2 \cdot e^{\i (\bar \phi_1 + \hat \theta - \bar \alpha + \frac{\pi}{2})} \\
    &= (\delta s + \delta \ell_0) \sin(\bar \alpha - \hat \theta) + \ell_0 \delta \bar \phi_1 \cos(\bar \alpha - \hat \theta) + \delta \ell_1 \sin(\bar \alpha) + \ell_1 \delta \bar \phi_1 \cos(\bar \alpha) \\
    &= \bigg( \ell_0 \frac{1 - \cos(\bar \alpha - \hat \theta) \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + \ell_1 \frac{\cos(\hat \theta) - \cos(\bar \alpha)^2}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg) \delta \bar \phi_1 + \delta \ell_1 \sin(\bar \alpha),
\end{align*}
\begin{equation*}
    \delta \ell_1 = \frac{1}{\sin(\bar \alpha)} \bigg[ r(\bar \phi_1 - 2\pi - \bar \alpha + \hat \theta) - \bigg( \ell_0 \frac{1 - \cos(\bar \alpha - \hat \theta) \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + \ell_1 \frac{\cos(\hat \theta) - \cos(\bar \alpha)^2}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg) \bigg] \delta \bar \phi_1,
\end{equation*}
\begin{align*}
    \frac{\delta r(\bar \phi_1 - 2\pi - \bar \alpha + \hat \theta)}{\delta \bar \phi_1} &= \delta P_2 \cdot e^{\i (\bar \phi_1 + \hat \theta - \bar \alpha)} - R(\bar \phi_1 - 2\pi - \bar \alpha + \hat \theta -) \\
    &= (\delta s + \delta \ell_0) \cos(\bar \alpha - \hat \theta) - \ell_0 \delta \bar \phi_1 \sin(\bar \alpha - \hat \theta) + \delta \ell_1 \cos(\bar \alpha) - \ell_1 \delta \bar \phi_1 \sin(\bar \alpha) - R(\bar \phi_1 - 2\pi - \bar \alpha + \hat \theta -) \\
    &= \ell_0 \frac{\cot(\bar \alpha)(-1 + \cos(\theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + \ell_1 \frac{\cot(\bar \alpha)(1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + r(\bar \phi_1 - 2\pi - \bar \alpha + \hat \theta) \cot(\bar \alpha) - R(\bar \phi_1 - 2\pi - \bar \alpha + \hat \theta -) \\
    &= (\ell_1 - \ell_0) \frac{\cot(\bar \alpha)(1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + \dot r_2;
\end{align*}

\item[$\phi \in [\bar \phi_1 + \hat \theta,\bar \phi_2)$] saturated spiral, with $0$ as curvature term because it is unperturbed
\begin{equation*}
    \dot{\delta r}  = \cot(\bar \alpha) \delta r;
\end{equation*}

\item[$\phi \in [\bar \phi_2,\bar \phi_2 + \hat \theta)$] tent: now the angle are fixed, so that one can compute the transformation as before (below), with entering data the previous tent and $r(\bar \phi_2 -)$
\begin{equation*}
    r(\bar \phi_2) = r(\bar \phi_2-) - \ell_0,
\end{equation*}
\begin{equation*}
    r(\bar \phi_2 + \hat \theta) = r(\bar \phi_2) \frac{\sin(\bar \alpha + \frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\hat \theta}{2})} - \ell_1,
\end{equation*}
hence the variation is
\begin{equation*}
    \delta r(\bar \phi_2 + \hat \theta) = \delta r(\bar \phi_2) \frac{\sin(\bar \alpha + \frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\hat \theta}{2})} - \delta \ell_1;
\end{equation*}

\item[$\phi \in [\bar \phi_2 + \hat \theta,\bar \phi_3)$] saturated spiral
\begin{equation*}
    \dot{\delta r} = \cos(\bar \alpha) \delta r - \frac{\delta r(-)}{\sin(\bar \alpha)},
\end{equation*}

\item[$\phi \in [\bar \phi_3,\bar \phi_3+\hat \theta)$] tent: keeping into account that $r_1^2$ 
\begin{equation*}
    r_0^2 = r(\bar \phi_2-) - \ell_0,
\end{equation*}
\begin{equation*}
    \ell_0^2 = \ell_1^2 = r_0^2 \frac{\sin(\frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\hat \theta}{2})},
\end{equation*}
saturation verification
\begin{align*}
    &r_0^2 \frac{\sin(\bar \alpha + \frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\hat \theta}{2})} - r_0^2 - \cos(\bar \alpha) (\ell_0^2 + \ell_1^2) \\
    &= \frac{r_0^2}{\sin(\bar \alpha - \frac{\hat \theta}{2})} \bigg( \sin \bigg( \bar \alpha + \frac{\hat \theta}{2} \bigg) - \sin \bigg( \bar \alpha - \frac{\hat \theta}{2} \bigg) - 2 \cos(\bar \alpha \sin \bigg( \frac{\hat \theta}{2} \bigg) \bigg) = 0,
\end{align*}
\begin{equation*}
    r_2^2 = r(\bar \phi_2 + \hat \theta) = r(\bar \phi_2) \frac{\sin(\bar \alpha + \frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\hat \theta}{2})} - \ell_1,
\end{equation*}
so that the variations satisfies the same relations, being the coefficients constant:
\begin{equation*}
    \delta r_0^2 = \delta r_2^1 e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} - \delta \ell_0,
\end{equation*}
\begin{equation*}
    \delta \ell_0^2 = \delta \ell_1^2 = \delta r_0^2 \frac{\sin(\frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\hat \theta}{2})},
\end{equation*}
\begin{equation*}
    \delta r_2^2 = (\delta r(\bar \phi_2) - \delta \ell_0^2) \frac{\sin(\bar \alpha + \frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\hat \theta}{2})} - \delta \ell_1^2;
\end{equation*}

\item[$\phi \in [2\pi + \hat \theta,\bar \phi_2)$] saturated spiral
\begin{equation*}
    \dot{\delta r} = \cot(\bar \alpha) \delta r - \frac{\delta r(\phi-)}{\sin(\bar \alpha)};
\end{equation*}

\item[$\phi \in [\bar \phi_k,\bar \phi_k + \hat \theta)$] tent perturbation;

\item[$\phi \in [\bar \phi_k + \hat \theta,\bar \phi_{k+1})$] saturated spirals.
\end{description}

The initial data for this construction depends on the base spiral $r$: in order to determine them, we differentiate according to the initial angle $\phi_0$. In this case the initial data are computed according to the fast closing solution, because the tent is after the segment.

These computations do not change much for the arc case, the only difference being that the initial data for the base tent-solution is different.



\subsubsection{Base solution}
\label{Sss:base_solution}


The base solution is the tent solution with initial data for the first tent
\begin{equation*}
    r_0(1), \quad \ell_0(1), \quad \ell_1(1), \quad r_2(1), \quad \bar \phi_1 = 0,
\end{equation*}
Then one defines the solution
\begin{equation*}
    r(1,\phi) = r_2(1) e^{\cot(\bar \alpha) (\phi - \hat \theta)}, \quad \phi \in [\hat \theta,\bar \phi_2 = \bar \phi_1 + 2\pi + \bar \alpha)
\end{equation*}

Then the iterative procedure is: given $r_0(k),\ell_0(k),\ell_1(k),r_2(k)$ and the function $r(k-1,\phi)$, $\phi \in [\bar \phi_{k-1} + \hat \theta,\bar \phi_k = \bar \phi_{k-1} + 2\pi + \bar \alpha)$, we compute
\begin{equation*}
    \dot r(k,\phi) = \cot(\bar \alpha) r(k,\phi) - \frac{r(k-1,\phi - 2\pi-\bar \alpha)}{\sin(\bar \alpha)}, \quad \phi \in [\bar \phi_k+\hat \theta,\bar \phi_{k+1}), 
\end{equation*}
and
\begin{equation*}
    r_0(k+1) = r(k,\bar \phi_{k+1}) - \ell_0(k), \quad \ell_0(k+1) = \ell_1(k+1) = r_0(k+1) \frac{\sin(\frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\hat \theta}{2})}, \quad r_2(k+1) = r_0(k+1) \frac{\sin(\bar \alpha + \frac{\theta}{2})}{\sin(\bar \alpha - \frac{\theta}{2})} - \ell_1(k).
\end{equation*}
{\color{red} We can also write

}

To get rid of the various constants, we change coordinates passing to
\begin{equation*}
    \rho(\tau) = r((2\pi + \bar \alpha) \tau) e^{-c (2\pi + \bar \alpha) \tau}, \quad \tau \in k + \bigg[ 0, 1 - \frac{\hat \theta}{2\pi + \bar \alpha} \bigg),
\end{equation*}
so that we get
\begin{equation*}
    \dot \rho(\tau) = \rho(\tau) - \rho(\tau - 1).
\end{equation*}
\begin{equation*}
    e^{\bar c(2\pi + \bar \alpha) (k+1)} \rho(k+1) = e^{\bar c(2\pi + \bar \alpha) (k+1)} \rho(k+1-) - e^{\bar c(2\pi + \bar \alpha) k} l_0(k),
\end{equation*}
\begin{equation*}
     e^{\bar c(2\pi + \bar \alpha) (k+1)} l_0(k+1) = e^{\bar c(2\pi + \bar \alpha) (k+1)} l_1(k+1) = e^{\bar c(2\pi + \bar \alpha) (k+1)} \rho(k+1) \frac{\sin(\frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\hat \theta}{2})},
\end{equation*}
\begin{equation*}
      e^{\bar c(2\pi + \bar \alpha) (k+1+\hat \tau)} \rho(k+1+\hat \tau) = e^{\bar c(2\pi + \bar \alpha) (k+1)} \rho(k+1) \frac{\sin(\bar \alpha + \frac{\theta}{2})}{\sin(\bar \alpha - \frac{\theta}{2})} - e^{\bar c(2\pi + \bar \alpha) k} l_1(k),
\end{equation*}
which rewritten are
\begin{equation*}
    \rho(k+1) = \rho(k+1-) - e^{- \bar c(2\pi + \bar \alpha)} l_0(k), \quad l_0(k+1) = l_1(k+1) = \rho(k+1) \frac{\sin(\frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\hat \theta}{2})}, \quad e^{\bar c(2\pi + \bar \alpha) \hat \tau} \rho(k + 1 + \hat \tau) = \rho(k+1) \frac{\sin(\bar \alpha + \frac{\theta}{2})}{\sin(\bar \alpha - \frac{\theta}{2})} - e^{- \bar c(2\pi + \bar \alpha)} l_1(k).
\end{equation*}

Then scaling time by
\begin{equation*}
    k + \bigg[ 0, 1 - \frac{\hat \theta}{2\pi + \bar \alpha} \bigg) \ni \tau \mapsto k + \frac{\tau - k}{1 - \frac{\hat \theta}{2\pi + \bar \alpha}} \in k + [0,1],
\end{equation*}
we get
\begin{equation*}
    \dot \rho = \bigg( 1 - \frac{\hat \theta}{2\pi + \bar \alpha} \bigg) \big( \rho(\tau) - \rho(\tau - 1) \big), \quad \hat \tau = \frac{\hat \theta}{2\pi + \bar \alpha},
\end{equation*}
\begin{equation*}
l_0(k+1) = \big( \rho(k+1-) - e^{- \bar c(2\pi + \bar \alpha)} l_0(k) \big) \frac{\sin(\frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\hat \theta}{2})}, \quad e^{\bar c(2\pi + \bar \alpha) \hat \tau} \rho(k+1) = \big( \rho(k+1-) - e^{- \bar c(2\pi + \bar \alpha)} l_0(k) \big) \frac{\sin(\bar \alpha + \frac{\theta}{2})}{\sin(\bar \alpha - \frac{\theta}{2})} - e^{- \bar c(2\pi + \bar \alpha)} l_0(k).
\end{equation*}
Scaling again
\begin{equation*}
    \rho \mapsto \rho e^{d \tau}, \quad d = - \log \bigg( 1 - \frac{\hat \theta}{2\pi + \bar \alpha} \bigg),
\end{equation*}
we obtain
\begin{equation*}
    \dot \rho(\tau) = \alpha \rho(\tau) - \rho(\tau - 1), \quad \alpha = \bigg( 1 - \frac{\hat \theta}{2\pi + \bar \alpha} \bigg) - \log \bigg( 1 - \frac{\hat \theta}{2\pi + \bar \alpha} \bigg) \geq 1.
\end{equation*}
Hence the base solution is obtained by adding to the previous RDE the discontinuities
\begin{equation*}
l_0(k) = \frac{\sin(\frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\hat \theta}{2})} \big( \rho(k-) - e^{- \bar c(2\pi + \bar \alpha) + d} l_0(k-1) \big),
\end{equation*}
\begin{equation*}
    \rho(k) = \frac{\sin(\bar \alpha + \frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\hat \theta}{2})} e^{- \bar c(2\pi + \bar \alpha) \hat \tau} \big( \rho(k-) - e^{- \bar c(2\pi + \bar \alpha) + d} l_0(k-1) \big) - e^{- \bar c(2\pi + \bar \alpha)(1 - \hat \tau) + d} l_0(k-1).
\end{equation*}

{\bf COME MOSTRARE CHE CRESCE SE I DATI INIZIALI SONO BUONI?}


\begin{remark}
    \label{Rem:verification_tent}
    The map for the time is
    \begin{equation*}
        \tau \mapsto t = (2\pi + \bar \alpha - \hat \theta) \tau + \hat \theta [\tau],
    \end{equation*}
the change is
\begin{equation*}
    r(t(\tau)) = \rho(\tau) e^{\bar c t(\tau) - \bar d \tau}, \quad \rho(\tau) = r(t(\tau)) e^{-\bar c t(\tau) + d \tau},
\end{equation*}
the RDE is then
\begin{align*}
    \dot \rho &= (2\pi + \bar \alpha - \hat \theta) (\cot(\bar \alpha) - c) r e^{-\bar c t(\tau) + d \tau} + d r e^{-\bar c t(\tau) + d \tau} - (2\pi + \bar \alpha - \hat \theta) \frac{r(t(\tau - 1)) e^{-\bar c t(\tau) + d \tau}}{\sin(\bar \alpha)} \\
    &= (1 - \hat \tau + d) \rho(\tau) + \frac{(2\pi + \bar \alpha - \hat \theta) e^{-\bar c (2\pi + \alpha) + d}}{\sin(\bar \alpha)} \rho(\tau - 1) \\
    &= \alpha \rho(\tau) - \rho(\tau-1),
\end{align*}
and scaling also
\begin{equation*}
    \ell_0(k) = l(k) e^{-\bar c t(k+1) + d (k+1)},
\end{equation*}
the jump relations become
\begin{equation*}
    l_0(k) = \frac{e^{-\bar c(2\pi+\bar \alpha) + d - \bar c \hat \theta} \sin(\hat \theta/2)}{\sin(\bar \alpha - \hat \theta/2)} \rho(k-) - \frac{e^{-\bar c(2\pi + \bar \alpha) + d} \sin(\hat \theta/2)}{\sin(\bar \alpha - \hat \theta/2)} l_0(k-1),
\end{equation*}
\begin{equation*}
    \rho(k) = \frac{e^{-\bar c \hat \theta} \sin(\bar \alpha + \hat \theta/2)}{\sin(\bar \alpha - \hat \theta/2)} \rho(k-) - \bigg( \frac{e^{-\bar c(2\pi+\bar \alpha) + d} \sin(\bar \alpha + \hat \theta/2)}{\sin(\bar \alpha - \hat \theta/2)} + 1 \bigg) l_0(k-1).
\end{equation*}
Taking into account
\begin{equation*}
    e^{- \bar c(2\pi + \bar \alpha) + d} = \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha - \hat \theta},
\end{equation*}
we conclude that the equations are as above:
\begin{equation*}
    \dot \rho(\tau) = \alpha(\hat \theta) \rho(\tau) - \rho(\tau-1), \quad \alpha(\hat \theta) = 1 - \frac{\hat \theta}{2\pi + \bar \alpha} - \ln \bigg( 1 - \frac{\hat \theta}{2\pi + \bar \alpha} \bigg),
\end{equation*}
\begin{equation*}
    l_0(k) = \frac{\sin(\bar \alpha) \sin(\hat \theta/2)}{(2\pi + \bar \alpha - \hat \theta) \sin(\bar \alpha - \hat \theta/2)} \rho(k-) - \frac{\sin(\bar \alpha) \sin(\hat \theta/2)}{(2\pi + \bar \alpha - \hat \theta) \sin(\bar \alpha - \hat \theta/2)} l_0(k-1),
\end{equation*}
\begin{equation*}
    \rho(k) = \frac{e^{-\bar c \hat \theta} \sin(\bar \alpha + \hat \theta/2)}{\sin(\bar \alpha - \hat \theta/2)} \rho(k-) - \bigg( 1 + \frac{\sin(\bar \alpha) \sin(\bar \alpha + \hat \theta/2)}{(2\pi + \bar \alpha - \hat \theta) \sin(\bar \alpha - \hat \theta/2)} \bigg) l_0(k-1).
\end{equation*}
The first can be written as
\begin{equation*}
    l_0(k) = \sum_{j=0}^{k-1} (-1)^j \bigg( \frac{\sin(\bar \alpha) \sin(\hat \theta/2)}{(2\pi + \bar \alpha - \hat \theta) \sin(\bar \alpha - \hat \theta/2)} \bigg)^{1+j} \rho(k-j-),
\end{equation*}
and then
\begin{equation*}
    \rho(k) = \frac{e^{-\bar c \hat \theta} \sin(\bar \alpha + \hat \theta/2)}{\sin(\bar \alpha - \hat \theta/2)} \rho(k-) - \bigg( 1 + \frac{\sin(\bar \alpha) \sin(\bar \alpha + \hat \theta/2)}{(2\pi + \bar \alpha - \hat \theta) \sin(\bar \alpha - \hat \theta/2)} \bigg) \sum_{j=0}^{k-2} (-1)^j \bigg( \frac{\sin(\bar \alpha) \sin(\hat \theta/2)}{(2\pi + \bar \alpha - \hat \theta) \sin(\bar \alpha - \hat \theta/2)} \bigg)^{1+j} \rho(k-1-j-)
\end{equation*}
\end{remark}


The numerical computation gives
\begin{equation*}
    \alpha = 1.00241, \quad C_1 = \frac{e^{-\bar c \hat \theta} \sin(\bar \alpha + \hat \theta/2)}{\sin(\bar \alpha - \hat \theta/2)} = 1.076, \quad C_2 = \frac{\sin(\bar \alpha) \sin(\hat \theta/2)}{(2\pi + \bar \alpha - \hat \theta) \sin(\bar \alpha - \hat \theta/2)} = 0.0416395,
\end{equation*}
and the evolution is written as
\begin{equation*}
    \dot \rho(\tau) = \alpha \rho(\tau) - \rho(\tau-1),
\end{equation*}
\begin{equation*}
    \rho(k) = C_1 \rho(k-) - C_2 (1 + C_2) \sum_{j=0}^{k-2} (- C_2)^j \rho(k-1-j-).
\end{equation*}

\begin{lemma}
    \label{Lem:increasing_good_optima}
    If $\rho$ is increasing in $[0,k+1)$, then it is increasing in $[0,k+2)$.
\end{lemma}

\begin{proof}
    Because of a previous lemma {\bf ???}, it is enough to prove that the jump in $k$ is positive. Writing
    \begin{align*}
        \rho(k) &= C_1 \rho(k-) - C_2 (1 + C_2) \sum_{j=0}^{k-2} (- C_2)^j \rho(k-1-j-) \\
        &\geq \bigg( C_1 - C_2 (1+C_2) \sum_j C_2^j \bigg) \rho(k-) \\
        &= \bigg( C_1 - \frac{C_2(1+C_2)}{1-C_2} \bigg) \rho(k-),
    \end{align*}
    and numerical computations gives
    \begin{equation*}
        C_1 - \frac{C_2(1+C_2)}{1-C_2} = 1.03074 > 1. \qedhere
    \end{equation*}
\end{proof}

We next compute the eigenvalues of the compact operator
\begin{equation*}
    C([0,1],\R) \times \R \ni (\rho,l_0) \mapsto T(\rho,l_0)(\tau) = \bigg( e^{\alpha \tau} (C_1 \rho(1) - (1+C_2) \ell_0) - \int_0^\tau e^{\alpha(\tau-\tau')} \rho(\tau') d\tau', C_2(\rho(1) - \ell_0) \bigg).
\end{equation*}
It holds
\begin{equation*}
    \ell_0 = \frac{C_2}{\lambda + C_2} \rho(1),
\end{equation*}
\begin{equation*}
    \lambda \rho(\tau) = e^{\alpha \tau} \bigg( C_1 - \frac{C_2 (1+C_2)}{\lambda + C_2} \bigg) \rho(1) - \int_0^\tau e^{\alpha (\tau-\tau')} \rho(\tau') d\tau',
\end{equation*}
\begin{equation*}
    \lambda \dot \rho = (\alpha \lambda - 1) \rho, \quad \rho(\tau) = \rho(1) e^{\frac{\alpha \lambda - 1}{\lambda}(\tau-1)},
\end{equation*}
\begin{align*}
    \lambda e^{\frac{\alpha \lambda - 1}{\lambda} (\tau-1)} &= e^{\alpha \tau} \bigg( C_1 - \frac{C_2 (1+C_2)}{\lambda + C_2} \bigg) - \int_0^\tau e^{\alpha (\tau-\tau') + \frac{\alpha \lambda - 1}{\lambda} (\tau'-1)} d\tau' \\
    &= e^{\alpha \tau} \bigg( C_1 - \frac{C_2 (1+C_2)}{\lambda + C_2} \bigg) 
    + \lambda \big( e^{\frac{\alpha - 1}{\lambda} (\tau-1)} - e^{\alpha \tau -\frac{\alpha \lambda - 1}{\lambda}} \big).
\end{align*}
The eigenvalues satisfy
\begin{equation*}
    C_1 - \frac{C_2 (1+C_2)}{\lambda + C_2} = \lambda e^{- \alpha + \frac{1}{\lambda}}.
\end{equation*}
The only real eigenvalues are the splitting of the double eigenvalue for $\hat \theta = 0$, and the maximal one is
\begin{equation*}
    \bar \lambda = 1.38096.
\end{equation*}
We should also verify that the others have modulus $<1$ and that these are simple.

In the original coordinates, the solution thus evolves with exponent
\begin{equation*}
    \bar c - \frac{d}{2\pi+\alpha} + \frac{\ln(\bar \lambda)}{2\pi + \alpha} = \bar c + .252535 > \bar c.
\end{equation*}
{\bf HENCE IT IS NOT THE OPTIMAL SOLUTION: THE PROBLEM IS THAT THE ANGLE OF THE TENT DIMINISHES AS WE GET FAR FROM THE LAST ROUND!}.



{\bf This part is used before and copied above too.}

We ask how the solution changes when differentiating w.r.t. $\bar \phi$.

If the spiral is saturated at $\bar \phi$, then at $\bar \phi$
\begin{equation*}
    \delta P_0 = \delta s e^{\i (\bar \phi + \bar \alpha)}, \quad \delta s \sin(\bar \alpha) = \delta \bar \phi r(\bar \phi),
\end{equation*}
\begin{equation*}
    \delta P_1 = \delta P_0 + \ell_0 \delta \bar \phi e^{\i (\bar \phi + \bar \alpha + \frac{\pi}{2})} + \delta \ell_0 e^{\i (\bar \phi + \bar \alpha)},
\end{equation*}
\begin{equation*}
    \delta P_2 = \delta P_1 + \ell_1 \delta \bar \phi  e^{\i (\bar \phi + \bar \alpha + \hat \theta + \frac{\pi}{2})} + \delta \ell_1 e^{\i (\bar \phi + \bar \alpha + \hat \theta)}.
\end{equation*}
The saturation condition is
\begin{align*}
0 &= \delta P_2 \cdot e^{\i (\bar \phi + \hat \theta)} - \cos(\bar \alpha) \big( \delta s + \delta \ell_0 + \delta \ell_1 \big) \\
&= (\delta s + \delta \ell_0) \cos(\bar \alpha - \hat \theta) - \ell_0 \delta \bar \phi \sin(\bar \alpha - \hat \phi) - \ell_1 \delta \bar \phi \sin(\bar \alpha) + \delta \ell_1 \cos(\bar \alpha) - \cos(\bar \alpha) \big( \delta s + \delta \ell_0 + \delta \ell_1 \big) \\
&= (\delta s + \delta \ell_0) \big( \cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha) \big) - \delta \bar \phi \big( \ell_0 \sin(\bar \alpha - \hat \theta) + \ell_1 \sin(\bar \alpha) \big), 
\end{align*}
and the angle relation is
\begin{align*}
    r(\phi_2) \delta \bar \theta &= \delta P_2 \cdot e^{\i (\bar \phi + \hat \theta + \frac{\pi}{2})} \\
    &= (\delta s + \delta \ell_0) \sin(\bar \alpha - \hat \theta) + \ell_0 \delta \bar \phi \cos(\bar \alpha - \hat \theta) + \ell_1 \delta \bar \phi \cos(\bar \alpha) + \delta \ell_1 \sin(\bar \alpha).
\end{align*}

At the next round, the sides are parallel: if $P_0,P_1,P_2$ are the points of the previous round, and $P_0',P_1',P_2'$ are for the next round, then
\begin{equation*}
    \angle(P_0'P_1P_2) = \hat \theta = \pi - \angle(P_2'P_1'P_0'). 
\end{equation*}
Hence by the point $P_2'$ is on the segment $P-2 - P_1$, because it has an angle of $\bar \alpha$.

By elementary geometric computations, the segment $P_1' - P_1$ splits the angle $\hat \theta = \angle(P_0'P_1P_2) = \angle(P_0'P_1P_2')$ is two equal parts, and then
\begin{equation*}
    |P_2' - P_2| = |P_0' - P_1| \frac{\sin(\bar \alpha + \frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\bar \alpha}{2})} - |P_2 - P_1|.
\end{equation*}
We can compute also
\begin{equation*}
    |P_2' - P_1'| = |P_0' - P_1| \frac{\sin(\frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\hat \theta}{2})},
\end{equation*}
At the next round we can thus compute the scale factor as
\begin{equation*}
    |P_2'' - P_2'| = \frac{|P_0'' - P_1'| \sin(\bar \alpha + \frac{\hat \theta}{2}) - |P_0' - P_1| \sin(\frac{\hat \theta}{2})}{\sin(\bar \alpha - \frac{\bar \alpha}{2})}.
\end{equation*}




The above equations determine the quantities, up to the knowledge of $r(\bar \phi)$, $\ell_0$, $\ell_1$. We are interested in their derivatives w.r.t. the perturbation $\theta_0$, because in this case the solution is explicit.



\section{Perturbed spiral}
\label{S:perturb_spiral}


We follow the base spiral up to an angle $\phi_0$, then we switch to the faster closing spiral with critical angle $\bar \alpha$ up to an angle $\bar \phi$, next we accelerate to $\hat \alpha$, $\cot(\hat \alpha) = \bar c$ for sligthly more that $2\pi + \frac{\pi}{2}$.


\subsection{Derivative w.r.t. $\bar \phi$}


We consider first the case where $\bar \phi$ is in the region where the solution satisfies
\begin{equation*}
    \dot r = \cot(\bar \alpha) r - \frac{r(-(2\pi + \bar \alpha))}{\sin(\bar \alpha)}.
\end{equation*}
Then we obtain
\begin{description}
    \item[$\phi \in [\bar \phi,\bar \phi + 2\pi + \bar \alpha)$]
    \begin{equation*}
        \dot r = \cot(\hat \alpha) r - \frac{r(-(2\pi + \bar \alpha))}{\sin(\bar \alpha)},
    \end{equation*}
    \item[$\phi \in [\bar \phi + 2\pi + \bar \alpha,\bar \phi + 2\pi + \hat \alpha)$]
    \begin{equation*}
        \dot r = \cot(\hat \alpha) r,
    \end{equation*}
    \item[$\phi \geq \bar \phi + 2\pi + \hat \alpha$]
    \begin{equation*}
        \dot r = \cot(\hat \alpha) r - \frac{r(-2\pi-\hat \alpha)}{\sin(\hat \alpha)}.
    \end{equation*}
\end{description}

We rewrite in terms of
\begin{equation*}
    \hat \rho(\tau) = r((2\pi + \hat \alpha) \tau) e^{-c(\hat \alpha)(2\pi + \hat \alpha) \tau},
\end{equation*}
with initial data
\begin{equation*}
    r(\bar \phi) = \rho \bigg( \frac{\bar \phi}{2\pi + \bar \alpha} \bigg) e^{\bar c \bar \phi},
\end{equation*}
\begin{align*}
     &- \frac{(2\pi + \hat \alpha)}{\sin(\bar \alpha)} r(\bar \phi + (2\pi + \hat \alpha) \tau - (2\pi + \bar \alpha)) e^{-c(\hat \alpha) (2\pi + \hat \alpha) \tau} \ind_{[0,\frac{2\pi + \bar \alpha}{2\pi + \hat \alpha})} \\
     &= - \frac{2\pi + \hat \alpha}{\sin(\bar \alpha)} \rho \bigg( \frac{\bar \phi}{2\pi + \bar \alpha} + \frac{2\pi + \hat \alpha}{2\pi + \bar \alpha} \tau - 1 \bigg) e^{\bar c (\bar \phi + (2\pi + \bar \alpha) \tau - (2\pi + \bar \alpha) + \bar \phi)} e^{-c(\hat \alpha) (2\pi + \hat \alpha) \tau} \ind_{[0,\frac{2\pi + \bar \alpha}{2\pi + \hat \alpha})} \\
     &= - e^{\bar c \bar \phi} \frac{2\pi + \hat \alpha}{2\pi + \bar \alpha} \rho \bigg( \frac{\bar \phi}{2\pi + \bar \alpha} + \frac{2\pi + \hat \alpha}{2\pi + \bar \alpha} \tau - 1 \bigg) e^{(\bar c - c(\hat \alpha))(2\pi + \hat \alpha) \tau} \ind_{[0,\frac{2\pi + \bar \alpha}{2\pi + \hat \alpha})},
\end{align*}
so dividing/scaling by $e^{\bar c \bar \phi}$ we get
\begin{align*}
\frac{d}{d\tau} \hat \rho(\tau) &= \log \bigg( \frac{a(\hat \alpha)}{b(\hat \alpha)} \bigg) \hat \rho(\tau) - \hat \rho(\tau - 1) + \rho \bigg( \frac{\bar \phi}{2\pi + \bar \alpha} \bigg) \delta_{\frac{\bar \phi}{2\pi + \bar \alpha}} - \frac{2\pi + \hat \alpha}{2\pi + \bar \alpha} \rho \bigg( \frac{\bar \phi}{2\pi + \bar \alpha} + \frac{2\pi + \hat \alpha}{2\pi + \bar \alpha} \tau - 1 \bigg) e^{(\bar c - c(\hat \alpha))(2\pi + \hat \alpha) \tau} \ind_{[0,\frac{2\pi + \bar \alpha}{2\pi + \hat \alpha})}.
\end{align*}
The solution is written as
\begin{equation*}
    \hat g(\tau) = \sum_{k=0}^\infty (-1)^k e^{\ln( \frac{\hat a}{\hat b}) (\tau - k)} \frac{(\tau - k)^k}{k!} \ind_{[k,+\infty)}, \quad \hat \tau = 1 - \frac{\hat \alpha - \bar \alpha}{2\pi + \hat \alpha},
\end{equation*}
\begin{align*}
    \hat \rho(\tau) &= \rho(\bar \tau) \hat g(\tau) - \int_0^{\hat \tau} \hat g(\tau - \tau') \frac{2\pi + \hat \alpha}{2\pi + \bar \alpha} \rho \bigg( \bar \tau + \frac{2\pi + \hat \alpha}{2\pi + \bar \alpha} \tau' - 1 \bigg) e^{(\bar c - c(\hat \alpha))(2\pi + \hat \alpha) \tau'} d\tau' \\
    &= \rho(\bar \tau) \sum_k (-1)^k e^{\ln( \frac{\hat a}{\hat b}) (\tau - k)} \frac{(\tau - k)^k}{k!} \ind_{[k,+\infty)}, \quad \hat \tau = 1 - \frac{\hat \alpha - \bar \alpha}{2\pi + \hat \alpha} \\
    & \quad - \frac{2\pi + \hat \alpha}{2\pi + \bar \alpha} \sum_k (-1)^k \frac{e^{\ln(\frac{a}{b}) (\tau - k)}}{k!} \int_0^{\hat \tau} e^{-\ln(\frac{\hat a}{\hat b}) \tau'} ([\tau - \tau' - k]^+)^k \rho \bigg( \bar \tau + \frac{2\pi + \hat \alpha}{2\pi + \bar \alpha} \tau' - 1 \bigg) e^{\ln(\frac{\hat a}{\hat b}) \tau'} d\tau' \\
    &= \rho(\bar \tau) \sum_k (-1)^k e^{\ln( \frac{\hat a}{\hat b}) (\tau - k)} \frac{(\tau - k)^k}{k!} \ind_{[k,+\infty)}, \quad \hat \tau = 1 - \frac{\hat \alpha - \bar \alpha}{2\pi + \hat \alpha} \\
    & \quad - \frac{2\pi + \hat \alpha}{2\pi + \bar \alpha} \sum_k (-1)^k \frac{e^{\ln(\frac{a}{b}) (\tau - k)}}{k!} \int_0^{\hat \tau} ([\tau - \tau' - k]^+)^k \rho \bigg( \bar \tau + \frac{2\pi + \hat \alpha}{2\pi + \bar \alpha} \tau' - 1 \bigg) d\tau'.
\end{align*}
The first terms are
\begin{align*}
    \hat \rho(\tau) &= \rho(\bar \tau) \Big[ e^{\ln(\frac{\hat a}{\hat b}) \tau} - e^{\ln(\frac{\hat a}{\hat b}) (\tau - 1)} [\tau - 1]^+ \Big] \\
    & \quad - \frac{2\pi + \hat \alpha}{2\pi + \bar \alpha} e^{\ln(\frac{\hat a}{\hat b}) \tau} \int_0^{\min\{\tau,\hat \tau\}}  \rho \bigg( \bar \tau + \frac{2\pi + \hat \alpha}{2\pi + \bar \alpha} \tau' - 1 \bigg) d\tau' \\
    & \quad + \frac{2\pi + \hat \alpha}{2\pi + \bar \alpha} e^{\ln(\frac{a}{b}) (\tau - 1)} [\tau - 1]^+ \int_0^{0 \vee \min\{\tau - 1,\hat \tau\}} (\tau - \tau' - 1) \rho \bigg( \bar \tau + \frac{2\pi + \hat \alpha}{2\pi + \bar \alpha} \tau' - 1 \bigg) d\tau'.
\end{align*}
At the end of the first round we value is
\begin{equation*}
    \hat \rho(\tau) = e^{\ln(\frac{\hat a}{\hat b}) \tau} \bigg[ \rho(\bar \tau) - \int_{0}^{\min\{1,\frac{2\pi+\hat \alpha}{2\pi+\bar \alpha} \tau\}} \rho(\tau') d\tau' \bigg].
\end{equation*}


Setting $\bar \phi = 0$ we obtain
\begin{description}
    \item[$\phi \in [0,2\pi + \bar \alpha)$]
    \begin{equation*}
        \dot r = \cot(\hat \alpha) r - \frac{r(-(2\pi + \bar \alpha) + \bar \phi)}{\sin(\bar \alpha)}, \quad r(0) = r(\bar \phi),
    \end{equation*}
    \item[$\phi \in [2\pi + \bar \alpha,2\pi + \hat \alpha)$]
    \begin{equation*}
        \dot r = \cot(\hat \alpha) r,
    \end{equation*}
    \item[$\phi \geq 2\pi + \hat \alpha$]
    \begin{equation*}
        \dot r = \cot(\hat \alpha) r - \frac{r(-2\pi-\hat \alpha)}{\sin(\hat \alpha)}.
    \end{equation*}
\end{description}

Differentiating w.r.t. $\bar \phi$
\begin{description}
    \item[$\phi \in [0,2\pi + \bar \alpha)$]
    \begin{equation*}
        \dot \delta r = \cot(\hat \alpha) \delta r - \frac{\dot r(-(2\pi + \bar \alpha))}{\sin(\bar \alpha)}, \quad  \delta r(0) = \dot r
        (\bar \phi),
    \end{equation*}
    \item[$\phi \in [2\pi + \bar \alpha, 2\pi + \hat \alpha)$]
    \begin{equation*}
        \dot \delta r = \cot(\hat \alpha) \delta r,
    \end{equation*}
    \item[$\phi \geq 2\pi + \hat \alpha$]
    \begin{equation*}
        \dot \delta r = \cot(\hat \alpha) \delta r - \frac{\delta r(-2\pi-\hat \alpha)}{\sin(\hat \alpha)}.
    \end{equation*}
\end{description}

The kernel for the equation is for the first 2 rounds (it closes at the beginning of the third):
\begin{equation*}
    G(\phi) = e^{\cot(\hat \alpha) \phi} - \frac{[\phi - 2 \pi - \hat \alpha]^+}{\sin(\hat \alpha)} e^{\cot(\hat \alpha)(\phi - 2\pi - \hat \alpha)}.
\end{equation*}
Using as source terms
\begin{equation*}
    \dot \phi(\bar \phi), \quad - \frac{\dot r(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} \ind_{[0,2\pi + \bar \alpha)},
\end{equation*}
we thus obtain for the first two rounds
\begin{align*}
    \delta r(\phi) &= G(\phi) \dot r(\bar \phi) - \int_0^{2\pi + \bar \alpha} G(\phi - \phi') \frac{r(\phi' - 2\pi - \alpha)}{\sin(\bar \alpha)} d\phi'.
\end{align*}
If $\dot r - \bar c r \geq $ (which we write as $\dot r(\bar \phi) \geq e^{\bar c (\bar \phi - \phi)} \dot r(\phi)$, $\phi \leq \bar \phi$), then being $G([0,2(2\pi + \hat \alpha)]) \geq 0$ we can estimate
\begin{align*}
    \delta r(\phi) &\geq \dot r(\bar \phi) \bigg[ G(\phi) - \int_0^{2\pi + \bar \alpha} \frac{G(\phi - \phi')}{\sin(\bar \alpha)} e^{\bar c(\phi' - 2\pi - \bar \alpha)} d\phi' \bigg] \\
    &= \dot r(\bar \phi) \bigg[ e^{\cot(\hat \alpha) \phi} - \frac{[\phi - 2 \pi - \hat \alpha]^+}{\sin(\hat \alpha)} e^{\cot(\hat \alpha)(\phi - 2\pi - \hat \alpha)} \\
    & \quad \quad - \frac{1}{\sin(\bar \alpha)} \int_0^{2\pi + \bar \alpha} \bigg( e^{\cot(\hat \alpha) (\phi - \phi')} - \frac{[\phi - \phi' - 2 \pi - \hat \alpha]^+}{\sin(\hat \alpha)} e^{\cot(\hat \alpha)(\phi - \phi' - 2\pi - \hat \alpha)} \bigg) e^{\bar c(\phi' - 2\pi - \bar \alpha)} d\phi' \bigg] \\
    &= e^{\cot(\hat \alpha) \phi} \dot r(\bar \phi) \bigg[ 1 - \frac{[\phi - 2 \pi - \hat \alpha]^+}{\sin(\hat \alpha)} e^{- \cot(\hat \alpha)(2\pi + \hat \alpha)} \\
    & \quad \quad - \frac{e^{-\bar c(2\pi + \bar \alpha)}}{\sin(\bar \alpha)} \int_0^{2\pi + \bar \alpha} e^{(\bar c - \cot(\hat \alpha)) \phi'} d\phi' + \frac{e^{-\bar c(2\pi + \bar \alpha) - \cot(\hat \alpha) (2\pi + \hat \alpha)}}{\sin(\bar \alpha)}  \int_0^{2\pi + \bar \alpha} \frac{[\phi - \phi' - 2 \pi - \hat \alpha]^+}{\sin(\hat \alpha)} e^{(\bar c - \cot(\hat \alpha)) \phi'} d\phi' \bigg].
\end{align*}
Thus a first approximation of the coefficient is
\begin{align*}
    & 1 - \frac{[\phi - 2 \pi - \hat \alpha]^+}{\sin(\hat \alpha)} e^{- \cot(\hat \alpha)(2\pi + \hat \alpha)} - \frac{(2 \pi + \bar \alpha) e^{-\bar c(2\pi + \bar \alpha)}}{\sin(\bar \alpha)}.
\end{align*}
{\color{blue} Since $\phi\leq 2\pi+\frac{\pi}{2}+0.05$ we find that
\begin{align*}
    & 1 - \frac{[\phi - 2 \pi - \hat \alpha]^+}{\sin(\hat \alpha)} e^{- \cot(\hat \alpha)(2\pi + \hat \alpha)} \\
    & \quad \quad - \frac{1 - e^{-\cot(\hat \alpha)(2\pi + \bar \alpha)}}{\sin(\bar \alpha) \cot(\hat \alpha)} + \int_0^{2\pi + \bar \alpha} \frac{[\phi - \phi' - 2 \pi - \hat \alpha]^+}{\sin(\hat \alpha)} e^{- \cot(\hat \alpha)(\phi' + 2\pi + \hat \alpha)} d\phi' \\
    & \geq -2.42748 + \int_0^{2\pi + \bar \alpha} \frac{[\phi - \phi' - 2 \pi - \hat \alpha]^+}{\sin(\hat \alpha)} e^{- \cot(\hat \alpha)(\phi' + 2\pi + \hat \alpha)} d\phi'
\end{align*}}




\subsection{The critical $\hat \alpha$}
\label{Ss:critical_hat_alpha}


The critical $\hat \alpha$ is computed by considering the solution to the segment case increasing the angle from $\bar \alpha$ to $\hat \alpha$ such that the solution is always positive.

The function to be positive is
\begin{equation*}
    e^{\cot(\hat \alpha)(2\pi + \hat \alpha - (\bar \theta - \theta_0)} \frac{\cos(\bar \alpha) - \cos(\hat \alpha) \cos(\bar \theta - \theta_0)}{\sin(\hat \alpha)^2} - 1.
\end{equation*}
Taking the derivative w.r.t. $\bar \theta - \theta_0$ in order to have the minimum
\begin{align*}
    &e^{\cot(\hat \alpha)(2\pi + \hat \alpha-(\bar \theta - \theta_0)} \bigg( \frac{\cos(\hat \alpha) \sin(\bar \theta - \theta_0)}{\sin(\hat \alpha)^2} - \cos(\hat \alpha) \frac{\cos(\bar \alpha) - \cos(\hat \alpha) \cos(\bar \theta - \theta_0)}{\sin(\hat \alpha)^2} \bigg) \\
    &= e^{\cot(\hat \alpha)(2\pi + \hat \alpha-(\bar \theta - \theta_0)} \frac{\cot(\hat \alpha)}{\sin(\hat \alpha)} \big( \cos(\hat \alpha - (\bar \theta - \theta_0)) - \cos(\bar \alpha) \big) = 0.
\end{align*}
Hence the worst case is
\begin{equation*}
    \theta - \theta_0 = \hat \alpha - \bar \alpha,
\end{equation*}
and the function becomes
\begin{equation*}
    e^{\cot(\hat \alpha)(2\pi + \bar \alpha)} \frac{\cos(\bar \alpha) - \cos(\hat \alpha) \cos(\hat \alpha - \bar \alpha)}{\sin(\hat \alpha)^2} - 1 = e^{\cot(\hat \alpha) (2\pi + \bar \alpha)} \big( \cos(\bar \alpha) - \sin(\bar \alpha) \cot(\hat \alpha) \big) - 1.
\end{equation*}
Its derivative w.r.t. $\cot(\bar \alpha)$ is
\begin{equation*}
    \big( (2\pi + \bar \alpha) (\cos(\bar \alpha) - \sin(\bar \alpha) \cot(\hat \alpha)) - \sin(\bar \alpha) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha)} = 0,
\end{equation*}
which gives
\begin{equation*}
    \cot(\hat \alpha) = \cot(\bar \alpha) - \frac{1}{2\pi + \bar \alpha} = \bar c.
\end{equation*}


\section{Computations of the perturbation - at last!}
\label{S:comput_pertu}


We can now write the solution as
\begin{equation*}
    r(\bar \phi) = \bar r(\bar \phi) + \int_0^{\bar \phi} \delta r(\bar \phi,\phi_0) ds_0 = \bar r(\bar \phi) + \bigg( \int_{A^-} + \int_{A^+} \bigg) \delta r(\bar \phi,\phi_0) ds_0,
\end{equation*}
where
\begin{equation*}
    A^- = \big\{ \phi_0 : \delta r(\bar \phi,\phi_0) < 0 \big\}, \quad A^+ = [0,\bar \phi] \setminus A^-.
\end{equation*}
We write
\begin{align*}
    \int_{A^-} \delta r(\bar \phi,\phi_0) ds_0 &= \int_{A^-} \delta r(\bar \phi,\phi_0) \frac{r(\phi_0)}{\sin(\theta_0)} d\phi_0 \\
    &= \int_{A^-} \frac{\delta r(\bar \phi,\phi_0)}{\sin(\theta_0)} \bigg[ \bar r(\phi_0) + \int_0^{\phi_0} \delta r(\phi_0,\phi_1) ds_1 \bigg] d\phi_0 \\
    &= \int_{A^-} \frac{\delta r(\bar \phi,\phi_0)}{\sin(\theta_0)} \bar r(\phi_0) d\phi_0 + \int_0^{\bar \phi} \bigg[ \int_{A^- \cap \{\phi_0 \geq \phi_1\}} \frac{\delta r(\bar \phi,\phi_0)}{\sin(\theta_0)} \delta r(\phi_0,\phi_1) d\phi_0 \bigg] ds_1.
\end{align*}
Substituting we get
\begin{align*}
    r(\bar \phi) &= \bar r(\bar \phi) + \int_{A^-} \frac{\delta r(\bar \phi,\phi_0)}{\sin(\theta_0)} \bar r(\phi_0) d\phi_0 \\
    & \quad + \int_{A^+} \bigg[ \delta r(\bar \phi,\phi_1) + \int_{A^- \cap \{\phi_0 \geq \phi_1\}} \frac{\delta r(\bar \phi,\phi_0)}{\sin(\theta_0)} \delta r(\phi_0,\phi_1) d\phi_0 \bigg] ds_1 \\
    & \quad + \int_{A^-} \int_{A^- \cap \{\phi_0 \geq \phi_1\}} \frac{\delta r(\bar \phi,\phi_0)}{\sin(\theta_0)} \delta r(\phi_0,\phi_1) d\phi_0 ds_1.
\end{align*}

We pass to the $\rho(\tau)$ function so that the terms are:
\begin{align*}
    \bar r(\bar \phi) + \int_{A^-} \frac{\delta r(\bar \phi,\phi_0)}{\sin(\theta_0)} \bar r(\phi_0) d\phi_0 &= \bar \rho(\bar \tau) e^{\bar c(2\pi + \bar \alpha) \bar \tau} + \int_{A^-} \frac{\delta \rho(\bar \tau,\tau_0) e^{\bar c(2\pi + \bar \alpha) (\tau - \tau_0)}}{\sin(\theta_0)} \bar \rho(\phi_0) e^{\bar c(2\pi + \bar \alpha) \tau_0} d\tau_0 (2\pi + \bar \alpha) \\
    &= e^{\bar c(2\pi + \bar \alpha) \bar \tau} \bigg[ \bar \rho(\bar \tau) + \int_{A^-} \frac{\delta \rho(\bar \tau,\tau_0)}{\sin(\theta_0)} \bar \rho(\tau_0) d\tau_0 (2\pi + \bar \alpha) \bigg],
\end{align*}
\begin{align*}
    \delta r(\bar \phi,\phi_1) + \int_{A^- \cap \{\phi_0 \geq \phi_1\}} \frac{\delta r(\bar \phi,\phi_0)}{\sin(\theta_0)} \delta r(\phi_0,\phi_1) d\phi_0 &= e^{\bar c(2\pi + \bar \alpha) (\bar \tau - \tau_1)} \bigg[ \delta \rho(\bar \tau,\tau_1) + \int_{A^- \cap \{\tau_0 \geq \tau_1\}} \frac{\delta \rho(\bar \tau,\tau_0)}{\sin(\theta_0)} \delta \rho(\tau_0,\tau_1) d\tau_0 (2\pi + \bar \alpha) \bigg]
\end{align*}
\begin{align*}
    \int_{A^-} \int_{A^- \cap \{\phi_0 \geq \phi_1\}} \frac{\delta r(\bar \phi,\phi_0)}{\sin(\theta_0)} \delta r(\phi_0,\phi_1) d\phi_0 ds_1 &= \int_{A^- \times A^- \cap \{\tau_1 \leq \tau_0\}} e^{\bar c(2\pi + \bar \alpha) (\bar \tau - \tau_1)} \frac{\delta \rho(\bar \tau,\tau_0) \delta \rho(\tau_0,\tau_1)}{\sin(\theta_0)} d\tau_0 ds_1 (2\pi + \bar \alpha).
\end{align*}


\subsection{Negativity region}
\label{Ss:nega_region_deriv}


PLOT OF NEGATIVITY REGION

We estimate the minimum
\begin{equation*}
    \min \frac{\delta r(\bar \tau,\tau_0)}{\sin(\theta_0)(2\pi + \bar \alpha)} \geq - 1.105.
\end{equation*}
The negativity region is contained in the region
\begin{equation*}
\max \big\{ 2 \bar \alpha - \bar \theta,\bar \theta - \hat \theta \big\} \leq \theta_0 \leq \bar \theta, \quad 
    \frac{2\pi + \theta_0}{2\pi + \bar \alpha} \leq \tau \leq \frac{2\pi + \bar \theta}{2\pi + \bar \alpha},
\end{equation*}
\begin{equation*}
    f(\Delta \phi) \leq \theta_0 \leq \frac{\pi}{2}, \quad \frac{2 \pi + \theta_0}{2\pi + \bar \alpha} \leq \tau \leq \frac{2\pi + \frac{\pi}{2}}{2\pi + \bar \alpha},
\end{equation*}
plus a small region for $\Delta \phi \leq 0.06$ and
\begin{equation*}
    \frac{2\pi + \frac{\pi}{2}}{2\pi + \bar \alpha} \leq \tau \leq \frac{2\pi + \frac{\pi}{2} + \Delta \phi}{2\pi + \bar \alpha}.
\end{equation*}

A rough estimate gives that
\begin{equation*}
    1 - \frac{\frac{\hat \theta}{2}}{2\pi + \bar \alpha} \leq \tau - \tau_0 \leq 1 + \frac{\frac{\pi}{2} - \bar \alpha +.06}{2\pi + \bar \alpha},
\end{equation*}
and we need to estimate (for $\bar \rho$, the same for the other cases)
\begin{align*}
    \bar \rho(\bar \tau) + (2\pi + \bar \alpha) \int_{A^-} \frac{\delta \rho(\bar \tau,\tau_0)}{\sin(\theta_0)} \bar \rho(\tau_0) d\tau_0 &\geq \bar \rho(\bar \tau) - (2\pi + \bar \alpha) 1.105 \int_{\bar \tau - 1 -\frac{\frac{\pi}{2} - \bar \alpha + .06}{2\pi + \bar \alpha}}^{\bar \tau - 1 + \frac{\frac{\hat \theta}{2}}{2\pi + \bar \alpha}} \bar \rho(\bar \tau,\tau_0) d\tau_0.
\end{align*}
If $\bar \rho$ is increasing, we get
\begin{align*}
    &\geq \bar \rho(\bar \tau) - 1.105 \bigg( \frac{\hat \theta}{2} + \frac{\pi}{2} - \bar \alpha + .06 \bigg) \bar \rho \bigg( \bar \tau - 1 + \frac{\frac{\hat \theta}{2}}{2\pi + \bar \alpha} \bigg) \\
    &\geq \bar \rho(\bar \tau) (1 - .78) = .22 \bar \rho(\bar \tau).
\end{align*}



==> casestudy_martina.tex <==
\section{A case study: the fastest saturated spiral}
\label{S:case:study}


In this section we consider as initial data for the saturated spiral the solution considered in Theorem \ref{Cor:curve_cal_R_sat_spiral}, namely an arc of the level set of $u$, a segment and the saturated spiral, where the initial fire set is the ball $\newglossaryentry{att}{name=\ensuremath{\mathtt a},description={initial radius for the case study of Section \ref{S:case:study}}} B_{\gls{att}}(0)$, $\gls{att} \in (0,1)$. The case $\mathtt a =1$ is the previous case of Section \ref{Sss:equation_satur}.

The aim of this analysis is twofold: on the one hand it is not clear if with this "optimized" initial data the spiral will close after some time, on the other hand the solution constructed here will be the fundamental block for the analysis of the general case. Since the spiral we construct is the spiral which becomes saturated before any other spiral, we call it the \emph{fastest saturated spiral}. We are not asking the question of its optimality here.

The construction speed we consider in this situation is the critical speed $\bar\sigma = \frac{1}{\cos(\bar \alpha)} = 2.6144..$ (Corollary \ref{Cor:eigen_angle}). The results proved here will be valid also for any other $\sigma \leq \bar\sigma$: more precisely, in the critical case the spirals diverges exponentially like $\phi e^{\lambda \phi}$, being $\lambda = \ln (\frac{2\pi + \bar 
\alpha}{\sin(\bar \alpha)}) = 0.27995...$ the only real eigenvalue of the RDE, and above {\color{red}below?} the critical case it diverges like $e^{\lambda_1 \phi}$, being $\lambda_1$ the greater real eigenvalue. 

According to Cases 1,2,3 above Theorem \ref{Cor:curve_cal_R_sat_spiral} with $\hat \phi = 0$, the firefighter constructs a spiral $S_\mathtt a$ ($\mathtt a$ being the radius of the initial burning region $B_\mathtt a(0)$) starting from a point $P_0 = (1,0)$ with the following structure: it is the union of
\begin{enumerate}
\item a circle (the arc of the level set of $u$, in some cases consisting of a single point),
\item a segment of endpoints $P_1(\mathtt a),P_2(\mathtt a)$ tangent to the circle in $P_1(\mathtt a)$ such that the point $P_2(\mathtt a)$ is saturated,
\begin{equation*}
\mathcal{A}(P_2(\mathtt a)) = u(P_2(\mathtt a)) - \frac{1}{\bar\sigma} L(P_2(\mathtt a)) = 0,
\end{equation*}
where $L(P_2(\mathtt a))$ is the length of the spiral $S_{\mathtt a}$ up to the point $P_2(\mathtt a)$,
\item a saturated spiral starting in $P_2(\mathtt a)$.
\end{enumerate}
The relevant quantities determining the exact structure of the spiral barrier are the following:
\begin{itemize}
\item the length of the arc of circle \newglossaryentry{Deltaphia}{name=\ensuremath{\Delta \phi_{\mathtt a}},description={opening angle of the initial starting in $(1,0)$}}
$$
P_0 P_1(\mathtt a) = \gls{Deltaphia},
$$
where $\Delta \phi_{\mathtt a}$ is the angle opening (remember that the level set $u$ passing by $(1,0)$ is $\partial B_1(0)$);
\item the length of the segment
$$
|P_2(\mathtt a) - P_1(\mathtt a)| = \frac{1}{\sin\bar\alpha},
$$
where we have used that by convexity and admissibility the segment is tangent to the saturated spiral in $P_2(\mathtt a)$, i.e. $\angle(P_2(\mathtt a),P_2(\mathtt a) - P_1(\mathtt a)) = \bar \alpha$;
\item the saturation condition at $P_2(\mathtt a)$, which can be written now as
\begin{align*}
&u(P_2(\mathtt a)) - \frac{1}{\bar \sigma} L(P_2(\mathtt a)) = \left( \frac{1}{\sin(\bar \alpha)} - \mathtt a \right) - \frac{1}{\bar \sigma} \left( \Delta \phi_{\mathtt a} + \frac{\cos(\bar \alpha)}{\sin(\bar \alpha)} \right) = 0.
\end{align*}
\end{itemize}

Using $\bar \sigma = \frac{1}{\cos(\bar \alpha)}$, the last equation becomes
\begin{equation}
\label{eq:Delta:phi:a}
\Delta \phi_{\mathtt a} = \bar \sigma \left( \frac{1}{\sin(\bar \alpha)} - \mathtt a \right) - \frac{\cos(\bar \alpha)}{\sin(\bar \alpha)} = \tan(\bar \alpha) - \frac{\mathtt a}{\cos(\bar \alpha)}.
\end{equation}
Depending on the value of the initial radius $\mathtt a$ of the fire initial position, we have the following situations (see Fig. \ref{fig:two:cases}).

\begin{description}
\item[Arc case, $\mathtt a < \sin(\bar \alpha)$, i.e. $\Delta\phi_{\mathtt a} > 0$] then the angle at the origin corresponding to the segment $[P_1,P_2]$ is $\theta_{\mathtt a} = \frac{\pi}{2} - \bar\alpha$.
\item[Segment case, $\mathtt a \geq \sin(\bar \alpha)$, i.e. $\Delta \phi_{\mathtt a} \leq 0$] then $P_1(\mathtt a) = P_0 = (1,0)$, and the tangency and saturation conditions for $P_2(\mathtt a)$ give
\begin{equation}
\label{eq:relation:theta:a}
(|P_2(\mathtt a)| -  \mathtt a) - \frac{1}{\bar \sigma} |P_1(\mathtt a) - P_2(\mathtt a)| = \frac{\sin(\theta_{\mathtt a} + \bar \alpha)}{\sin(\bar \alpha)} -  \mathtt a - \frac{1}{\bar \sigma} \frac{\sin(\theta_{\mathtt a})}{\sin(\bar \alpha)} = 0.
\end{equation}
Using again $\frac{1}{\bar \sigma} = \cos(\bar \alpha)$ we obtain
\begin{equation*}
\cos(\theta_{\mathtt a}) = \mathtt a, \quad \theta_{\mathtt a} \in \bigg[ 0 , \frac{\pi}{2} - \bar \alpha \bigg],
\end{equation*}
because $\mathtt a \in [\sin(\bar \alpha),1]$.
\end{description}

\begin{figure}
\centering
\includegraphics[scale=0.6]{twositcasestudy.png}
\caption{The two cases with $ \mathtt a \in (0,\sin(\bar \alpha))$ and $ \mathtt a \in [\sin(\bar \alpha),1]$.}
\label{fig:two:cases}.
\end{figure}

The main result of this section is the following

\begin{theorem}
\label{thm:case:a}
For any value of $\mathtt a \in (0,1]$, the spiral \newglossaryentry{Stta}{name=\ensuremath{S_{\mathtt a}},description={a particular spiral which is optimal for the first round, with the initial burning region $B_\mathtt{a}(0)$}} \gls{Stta} does not confine the fire: more precisely, the spiral diverges exponentially as
$$
r{\color{red}_a}(\phi) \sim 2 \phi e^{\bar c \phi} \begin{cases}
\frac{e^{-\bar c(\Delta \phi_{\mathtt a} + \frac{\pi}{2} - \bar \alpha)}}{\sin(\bar \alpha)} - e^{-\bar c(2\pi)} - \frac{e^{-\bar c(2\pi + \frac{\pi}{2})} - e^{- \bar c (2\pi + \frac{\pi}{2} + \Delta \phi_\mathtt a)}}{\bar c} - \cot(\bar \alpha) e^{-\bar c(2\pi + \frac{\pi}{2} + \Delta \phi_\mathtt a)} & 0 \leq \mathtt a < \sin(\bar \alpha), \\
\frac{\sin(\theta_\mathtt a + \bar \alpha) e^{-\bar c \theta_\mathtt a}}{\sin(\bar \alpha)} - e^{-\bar c(2\pi)} - \frac{\sin(\theta_\mathtt a) e^{-\bar c(2\pi + \theta_\mathtt a + \bar \alpha)}}{\sin(\bar \alpha)} & \sin(\bar \alpha) \leq \mathtt a \leq 1,
\end{cases} 
$$
being $\bar c = \ln(\frac{2\pi+\bar \alpha}{\sin(\bar \alpha)})$ given by \eqref{Equa:c_gene_defi}.
\end{theorem}

The proof of this theorem relies on a careful application of Lemma \ref{lem:key}. %Before proving the previous theorem, we state the following two lemmas on elementary properties of the solution of RDEs.
%
%\begin{lemma}
%\label{lem:conti:uguali}
%Let $r(\phi)$ such that
%\begin{equation*}
%\frac{d}{d\phi}r(\phi)=\lambda r(\phi)-\gamma r(\phi-\phi_0),
%\end{equation*}
%for some $\lambda,\gamma,\phi_0>0$, and, given $\phi_0\leq\phi_1\leq\phi_2$, assume that
%\begin{equation*}
%r(\phi)=\kappa e^{\lambda (\phi -\phi_1+\phi_0)}, \quad \forall\phi\in[\phi_1-\phi_0,\phi_2-\phi_0),
%\end{equation*}
%for some constant $\kappa$. Then
%\begin{equation*}
%r(\phi)=\left(r(\phi_1)-\gamma r(\phi_1-\phi_0)(\phi-\phi_1)\right)e^{\lambda (\phi-\phi_1)},\quad\forall\phi\in[\phi_1,\phi_2].
%\end{equation*}
%\end{lemma}
%
%\begin{proof}
%The proof follows easily by Duhamel's formula for the ODE:
%\begin{align*}
%r(\phi) &= e^{\lambda(\phi-\phi_1)} r(\phi_1) - \gamma \int_{\phi_1}^{\phi} e^{\lambda(\phi-\eta)} r(\eta-\phi_0)d\eta \\
%&= e^{\lambda(\phi-\phi_1)} r(\phi_1) - \gamma \int_{\phi_1-\phi_0}^{\phi-\phi_0} e^{\lambda(\phi-z-\phi_0)} \kappa e^{\lambda(z-\phi_1+\phi_0)} dz \\
%&= \left(r(\phi_1) - \gamma\kappa(\phi-\phi_1)\right) e^{\lambda(\phi-\phi_1)},
%\end{align*}
%which is the statement.
%\end{proof}
%
%\begin{lemma}
%\label{lem:conti:uguali:2:che:palle}
%Let $r(\phi)$ such that
%\begin{equation*}
%\frac{d}{d\phi}r(\phi)=\lambda r(\phi)-\gamma r(\phi-\phi_0),
%\end{equation*}
%for some $\lambda,\gamma,\phi_0>0$, and, given $\phi_0\leq\phi_1\leq\phi_2$, assume that
%\begin{equation*}
%r(\phi) = \left( r(\phi_1) - \gamma r(\phi_1-\phi_0) (\phi-\phi_1) \right) e^{\lambda (\phi-\phi_1)}, \quad \forall \phi \in [\phi_1,\phi_2].
%\end{equation*}
%Call
%\begin{equation*}
%\bar d = \lambda-\frac{1}{\phi_0}.
%\end{equation*}
%Then if $r(\phi_1),r(\phi_1-\phi_0)\geq 0$ the function
%\begin{equation*}
%\rho(\phi)=r(\phi)e^{-\bar d\phi}
%\end{equation*}
%is monotonically increasing in $[\phi_1,\phi_2]$ if
%\begin{equation}\label{rho:mon:incr}
%r(\phi_1)-\gamma r(\phi_1-\phi_0) (\phi_2-\phi_1+\phi_0) \geq 0. 
%\end{equation}
%\end{lemma}
%
%\begin{proof}
%The computation of the derivative of $\rho(\phi)$ is straightforward, in particular 
%\begin{equation*}
%\text{sign}(\rho'(\phi)) = \text{sign}\left( \frac{r(\phi_1)}{\phi_0} - \gamma \left( r(\phi_1-\phi_0) + \frac{1}{\phi_0} r(\phi_1-\phi_0) (\phi-\phi_1) \right) \right),
%\end{equation*}
%and the conclusion follows observing that $r(\phi_1),r(\phi_1-\phi_0)\geq 0$.
%\end{proof}

\begin{figure}
\centering
\includegraphics[scale=0.6]{basecasearc.png}
\caption{Here {\color{red} the fastest saturated spiral $S_a$} is {\color{red} the union of} an arc {\color{red} of circle}, a segment and a saturated spiral.}
\label{fig:base:case:Arc}
\end{figure}

\begin{proof}[Proof of Theorem \ref{thm:case:a}]
We analyze separately the two cases $\Delta\phi_{\mathtt a}>0$ and $\Delta\phi_{\mathtt a}\leq 0$.

\medskip

\noindent{\bf Case $\Delta\phi_{\mathtt a}>0$.} This case is described in Figure \ref{fig:base:case:Arc}. We remark that from \eqref{eq:Delta:phi:a} we find that $\Delta \phi_{\mathtt a} \in (0,\tan(\bar \alpha)]$, the largest possible arc-length being
\begin{equation}
\label{eq:Delta:case:study:section:5}
\Delta \phi_0 = \tan(\bar \alpha)
\end{equation}
corresponding to $\mathtt a = 0$. We will denote by $r_{\mathtt a}$ the radius of the spiral $S_{\mathtt a}$ in the fire coordinates of Theorem \ref{thm:param_1}, to underline the dependence w.r.t. $\mathtt a$. {\color{red}Scritto qui o spostato sopra?}

\medskip

\noindent{\it Step 1.} We compute the first rounds:
\begin{itemize}
\item for $\phi \in [0,\Delta \phi_{\mathtt a})$ we have
\begin{equation*}
r_1{\color{red}_a?}(\phi) = 1;
\end{equation*}
\item for $\phi \in [\Delta \phi_{\mathtt a}, \Delta \phi_{\mathtt a} + \frac{\pi}{2} -\bar \alpha)$ we have that
\begin{equation*}
r_{\mathtt a}(\phi) = \frac{1}{\cos(\phi - \Delta\phi_{\mathtt a})},
\end{equation*}
in particular we call
\begin{equation*}
\kappa_1(\mathtt a) = r_{\mathtt a} \left( \Delta \phi_{\mathtt a} + \frac{\pi}{2} -\bar \alpha \right) = \frac{1}{\sin(\bar\alpha)}
\end{equation*}
the final distance for $0$;
\item for $\phi \in [\Delta \phi_{\mathtt a} + \frac{\pi}{2} - \bar \alpha, 2\pi)$ it holds
\begin{equation*}
\frac{d}{d\phi} r_{\mathtt a}(\phi) = \cot(\bar\alpha) r_{\mathtt a}(\phi),
\end{equation*}
since the spiral is saturated, giving
\begin{equation*}
r_{\mathtt a}(\phi) = \kappa_1(\mathtt a) e^{\cot(\bar\alpha)(\phi - \frac{\pi}{2} + \bar\alpha - \Delta \phi_{\mathtt a})};
\end{equation*}
\item the radius $r_{\mathtt a}$ has a jump at $\phi = 2\pi$,
\begin{equation*}
r_{\mathtt a}(2\pi)-r_{\mathtt a}(2\pi-)=-1,
\end{equation*}
in particular we denote by
\begin{equation*}
\kappa_2(\mathtt a) = r_{\mathtt a}(2\pi) = \kappa_1(\mathtt a) e^{\cot(\bar \alpha) (2\pi - \frac{\pi}{2} + \bar \alpha-\Delta \phi_{\mathtt a})}-1;
\end{equation*}
\item for $\phi \in [2\pi,2\pi+\frac{\pi}{2})$ it holds
\begin{equation*}
\frac{d}{d\phi} r_{\mathtt a}(\phi) = \cot(\bar\alpha) r_{\mathtt a}(\phi),
\end{equation*}
therefore
\begin{equation}
\label{eq:r:2pi:etc}
r_{\mathtt a}(\phi) = \kappa_2(\mathtt a) e^{\cot(\bar\alpha)(\phi - 2\pi)} = \left[ \kappa_1(\mathtt a) e^{\cot(\bar \alpha) (2\pi - \frac{\pi}{2} + \bar \alpha - \Delta \phi_{\mathtt a})} - 1 \right] e^{\cot(\bar\alpha)(\phi - 2\pi)};
\end{equation}
\item define
$$
\kappa_3(\mathtt a) = r_{\mathtt a} \left( 2\pi + \frac{\pi}{2} \right) = \kappa_2(\mathtt a) e^{\frac{\pi}{2}\cot(\bar\alpha)};
$$
\item for $\phi \in \left[ 2\pi + \frac{\pi}{2}, 2\pi + \frac{\pi}{2} + \Delta\phi_{\mathtt a} \right]$ the radius $r_{\mathtt a}(\phi)$ satisfies
\begin{equation*}
\frac{d}{d\phi} r_{\mathtt a}(\phi) = \cot(\bar\alpha) r_{\mathtt a}(\phi) - 1,
\end{equation*}
whose solution is
\begin{equation*}
r_{\mathtt a}(\phi) = \kappa_3(\mathtt a) e^{\cot(\bar \alpha)(\phi - 2\pi - \frac{\pi}{2})} + \tan(\bar \alpha) \big( 1 - e^{\cot(\bar \alpha)(\phi - 2\pi - \frac{\pi}{2})} \big);
\end{equation*}
\item the radius $r_{\mathtt a}$ has a jump in $\phi = 2\pi + \frac{\pi}{2} + \Delta\phi_{\mathtt a}$: 
\begin{equation*}
r_{\mathtt a} \left( 2\pi + \frac{\pi}{2} + \Delta \phi_{\mathtt a} \right) -r_{\mathtt a} \left( 2\pi + \frac{\pi}{2} + \Delta \phi_{\mathtt a} - \right) = - \cot(\bar \alpha),
\end{equation*}
and also here we will introduce the quantity
\begin{equation*}
\kappa_4(\mathtt a) = r_{\mathtt a} \left(2\pi+\frac{\pi}{2}+\Delta\phi_{\mathtt a} \right) = e^{\cot(\bar \alpha) \Delta \phi_{\mathtt a}} \kappa_3(\mathtt a) + \tan(\bar \alpha) \left( 1 - e^{\cot(\bar \alpha)\Delta \phi_{\mathtt a}} \right) - \cot(\bar \alpha);
\end{equation*}
\item finally, for $\phi \geq 2\pi + \frac{\pi}{2} + \Delta \phi$ the function solves
\begin{equation*}
\frac{d}{d\phi} r_{\mathtt a}(\phi) = \cot(\bar \alpha) r_{\mathtt a}(\phi) -\frac{r_{\mathtt a}(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)}.
\end{equation*}
\end{itemize}

Using the kernel $G(\phi),M(\phi,\phi_1,\phi_2)$ of Remark \ref{Rem:oringal_phi_kernel} {\color{red} and the expressions computed in Section \ref{Sss:green_kernels}}, the solution can be written for $\phi \geq \Delta \phi_\mathtt a + \frac{\pi}{2} - \bar \alpha$ as
\begin{equation}
\label{Equa:expl_sol_sat_or}
r{\color{red}_a}(\phi) = \frac{1}{\sin(\bar \alpha)} G(\phi - \bar \phi_0(\mathtt a)) - G(\phi - 2\pi) - M(\phi,\bar \phi_1(\mathtt a),\bar \phi_2(\mathtt a)) - \cot(\bar \alpha) G(\phi - \bar\phi_0(\mathtt a) - 2\pi - \bar \alpha),
\end{equation}
where the angles are given by
\begin{equation*}
%\label{Equa:time_case_st}
\bar \phi_0(\mathtt a) = \Delta \phi_\mathtt a + \frac{\pi}{2} - \bar \alpha, \quad \bar \phi_1(\mathtt a) = 2\pi + \frac{\pi}{2}, \quad \bar \phi_2(\mathtt a) = \bar \phi_0(\mathtt a) + 2\pi + \bar \alpha = \Delta \phi_a + 2\pi + \frac{\pi}{2}.
\end{equation*}
We can translate the solution by $\varphi = \phi - \bar \phi_0(\mathtt a)$ obtaining
\begin{equation}
\label{Equa:expl_sol_sat}
r{\color{red}_a}(\varphi) = \frac{1}{\sin(\bar \alpha)} G(\varphi) - G \bigg( \varphi + \frac{\pi}{2} - \bar \varphi_1(\mathtt a) \bigg) - M(\varphi,\bar \varphi_1(\mathtt a),2\pi + \bar \alpha) - \cot(\bar \alpha) G(\varphi - 2\pi - \bar \alpha),
\end{equation}
with
\begin{equation}
\label{Equa:time_case_st}
\bar \varphi_1(\mathtt a) = 2\pi + \frac{\pi}{2} - \bar \varphi_0 = 2\pi + \bar \alpha - \Delta \phi_\mathtt a.
\end{equation}

\medskip

\noindent{\it Step 2.}
The next step is to optimize the solution w.r.t. $\mathtt a$: this is done by taking the derivative w.r.t. $\mathtt a$ of the solution and using the linearity of the Delay ODE. We use the relations \eqref{Equa:ker_der_G}, \eqref{Equa:der_M_phi1} and
\begin{equation*}
\frac{d}{d\mathtt a} \bar \varphi_1 = \frac{1}{\cos(\bar \alpha)} \quad \text{because of (\ref{eq:Delta:phi:a})},
\end{equation*}
we obtain that
\begin{align*}
\partial_{\mathtt a} r(\varphi) &= \frac{1}{\cos(\bar \alpha)} \bigg[ - \Diracd_{- \frac{\pi}{2} + \bar \varphi_1} - \cot(\bar \alpha) G \bigg( \varphi + \frac{\pi}{2} - \bar \varphi_1 \bigg) + \frac{G \big( \varphi + \frac{\pi}{2} - \bar \varphi_1 - 2\pi - \bar \alpha) \big)}{\sin(\bar \alpha)} + G(\varphi - \bar \varphi_1) \bigg].
\end{align*}
We have thus to study the function
\begin{equation*}
\check r(\psi) = \cot(\bar \alpha) G(\psi) - \frac{G(\psi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} - G \bigg( \psi - \frac{\pi}{2} \bigg), \quad \psi = \varphi + \frac{\pi}{2} - \bar \varphi_1,
\end{equation*}
which is the solution to the RDE for the saturated spiral
\begin{equation*}
\frac{d}{d\psi} \check r(\psi) = \cot(\bar \alpha) \check r(\psi) - \frac{\check r(\psi- 2\pi - \bar \alpha)}{\sin(\bar \alpha)} + \cot(\bar \alpha) \Diracd_0 - \Diracd_{\frac{\pi}{2}} - \frac{\Diracd_{2\pi + \bar \alpha}}{\sin(\bar \alpha)}. 
\end{equation*}
In terms the function $\check \rho(\tau) = \check r((2\pi+\bar \alpha) \tau) e^{- \bar c (2\pi + \bar \alpha) \tau}$ the RDE becomes
\begin{equation}
\label{Equa:ckrho_delph_casest}
\check \rho(\tau) = \cot(\bar \alpha) g(\tau) - \frac{e^{-\bar c (2\pi + \bar \alpha)} g(\tau - 1)}{\sin(\bar \alpha)} - e^{-\bar c \frac{\pi}{2}} g \bigg( \tau - \frac{\frac{\pi}{2}}{2\pi + \bar \alpha} \bigg),
\end{equation}
which is the solution to the RDE for the saturated spiral
\begin{equation*}
\frac{d}{d\psi} \check \rho(\tau) = \check \rho(\tau) - \check \rho(\tau-1) + \cot(\bar \alpha) \Diracd_0 - e^{-\bar c \frac{\pi}{2}} \Diracd_{\frac{\pi}{2(2\pi+\bar \alpha)}} - \frac{e^{-\bar c(2\pi+\bar \alpha)} \Diracd_{1}}{\sin(\bar \alpha)}. 
\end{equation*}

\begin{figure}
\includegraphics[scale=.6]{case_study_deltaphi1.png}\hfill\includegraphics[scale=.6]{case_study_a01.png}
\caption{Plot of the function \eqref{Equa:ckrho_delph_casest} for $\tau \in [1,2]$ on the left and of the function $r(\phi)$ of Equation \eqref{Equa:expl_sol_sat_or} (multiplied by $e^{-\bar c \phi}$) for $\mathtt a = 0$.}
\label{Fig:ckrho_delph_casst}
\end{figure}

A numerical plot of the solution for $\tau \in [1,2]$ is in Fig. \ref{Fig:ckrho_delph_casst}: we notice that it is strictly negative together with its derivative, and from Lemma \ref{lem:key} we deduce that $\check \rho < 0$ for all $\tau \geq 1$, corresponding to the angle
\begin{equation*}
\phi = 4\pi + \bar \alpha, \quad \text{because of the map} \ \tau \mapsto \phi = (2\pi + \bar \alpha) \tau + 2\pi.
\end{equation*}
For the first two rounds, a numerical plot of $r(\phi)$ as function for $(\phi,\Delta \phi) \in [\Delta \phi + \frac{\pi}{2} - \bar \alpha] \times [0,\tan(\bar \alpha)]$ shows that the solution is strictly positive (and actually decreasing w.r.t. $\Delta \phi_\mathtt a$, i.e. increasing w.r.t. $\mathtt a$), see Fig. \ref{Fig:ckrho_delph_casst}.

\medskip

\begin{figure}
\includegraphics[scale=.8]{case_study_a01.png}
\caption{The first 2 rounds of the function $r(\phi)$ of \eqref{Equa:expl_sol_sat_or} (multiplied by $e^{-\bar c \phi}$) for $\mathtt a = 0$.}
\label{Fig:casr_a=0}
\end{figure}

\noindent{\it Step 3.} From now on we will assume $\mathtt a = 0$, therefore $\Delta \phi_0 = \tan(\bar \alpha)$: a numerical plot of the function $r(\phi) e^{-\bar c \phi}$ is in Fig. \ref{Fig:casr_a=0}. We observe that the function is strictly positive and increasing in an interval larger than $2\pi+\bar \alpha$, and then by Lemma \ref{lem:key} we deduce that the solution is positive for all $\phi$.

\medskip

\noindent{\it Case $\Delta\phi_{\mathtt a}\leq 0$.} This case is described in Figure \ref{fig:base:case:185}. We will prove that the worst case is for $\mathtt a = \sin(\bar \alpha)$, which corresponds to $\Delta \phi_{\mathtt a} = 0$ in the previous analysis: hence again the worst case is for $\mathtt a = 0$, as shown above, and the spiral does not close.

The approach is completely similar, the only variation being the missing initial arc.

{\it Step 1.} We compute $r_{\mathtt a}(\phi)$ explicitly for the first rounds. We call $\bar \theta_{\mathtt a} = \theta_{\mathtt a} + \bar\alpha \in [0,\frac{\pi}{2}]$ as the slope of the segment $[P_1(\mathtt a),P_2(\mathtt a)]$:

\begin{figure}
\centering
\includegraphics[scale=0.75]{base.case.185.png}
\caption{The function $\phi\rightarrow f_0(\phi)$.}
\label{fig:base:case:185}
\end{figure}

\begin{itemize}
\item for $\phi \in[0,\bar \theta_{\mathtt a} - \bar \alpha]$ we have that
\begin{equation*}
r_{\mathtt a}(\phi) = \frac{\sin(\bar \theta_{\mathtt a})}{\sin(\bar \theta_{\mathtt a} - \phi)},
\end{equation*}
and we call
\begin{equation*}
\kappa'_1(\mathtt a) = r_{\mathtt a}(\bar \theta_{\mathtt a} - \bar \alpha) = \frac{\sin(\bar \theta_{\mathtt a})}{\sin(\bar \alpha)};
\end{equation*}
\item for $\phi \in [\bar \theta_{\mathtt a} - \bar \alpha, 2\pi)$ it holds
\begin{equation*}
\frac{d}{d\phi} r_{\mathtt a}(\phi) = \cot(\bar \alpha) r_{\mathtt a}(\phi),
\end{equation*}
which gives
\begin{equation*}
r_{\mathtt a}(\phi) = \kappa'_1(\mathtt a) e^{\cot(\bar \alpha) (\phi - \bar \theta_{\mathtt a} + \bar \alpha)};
\end{equation*}
\item the function $r_{\mathtt a}(\phi)$ has a jump at $\phi = 2\pi$, %indeed
\begin{equation*}
r_{\mathtt a}(2\pi) - r_{\mathtt a}(2\pi-) = - 1,
\end{equation*}
and we set
$$
\kappa'_2(\mathtt a) = r_{\mathtt a}(2\pi) = \frac{\sin(\bar \theta_{\mathtt a})}{\sin(\bar \alpha)} e^{\cot(\bar \alpha) (2\pi - \bar \theta_{\mathtt a} + \bar \alpha)} - 1;
$$
\item for $\phi \in [2\pi,2\pi + \bar \theta_{\mathtt a})$ it holds
\begin{equation*}
\frac{d}{d\phi} r_{\mathtt a}(\phi) = \cot(\bar\alpha) r_{\mathtt a}(\phi),
\end{equation*}
so that
\begin{equation*}
r_{\mathtt a}(\phi) = \kappa'_2(\mathtt a) e^{\cot(\bar\alpha) (\phi - 2\pi)};
\end{equation*}
\item in $\phi=2\pi+\bar\theta_{\mathtt a}$ the function $r_{\mathtt a}$ has a jump, computed as
\begin{equation*}
r_{\mathtt a}(2\pi + \bar \theta_{\mathtt a}) - r_{\mathtt a}(2\pi + \bar \theta_{\mathtt a}-) = - \frac{\sin(\bar\theta_{\mathtt a} - \bar \alpha)}{\sin(\bar \alpha)},
\end{equation*}
and we call
$$
\kappa_3'(\mathtt a) = r_{\mathtt a}(2\pi + \bar \theta_{\mathtt a}) = \kappa'_2(\mathtt a) e^{\cot(\bar \alpha) \bar \theta_{\mathtt a}} - \frac{\sin(\bar \theta_{\mathtt a} - \bar \alpha)}{\sin(\bar \alpha)};
$$
\item finally, for $\phi \geq 2\pi+\bar\theta_{\mathtt a}$ the function solves
\begin{equation*}
\frac{d}{d\phi} r_{\mathtt a}(\phi) = \cot(\bar \alpha) r_{\mathtt a}(\phi) - \frac{r_{\mathtt a}(\phi - 2\pi - \bar \alpha)}{\sin(\bar\alpha)}.
\end{equation*}
\end{itemize}

As before, by using the kernel $G(\phi),M(\phi,\phi_1,\phi_2)$ of Remark \ref{Rem:oringal_phi_kernel}, the solution can be written for $\phi \geq \bar \theta_\mathtt a - \bar \alpha$ as
\begin{equation}
\label{Equa:expl_sol_sat_or2}
r(\phi) = \frac{\sin(\bar \theta_\mathtt a)}{\sin(\bar \alpha)} G(\phi - \bar \phi_0(\mathtt a)) - G(\phi - 2\pi) - \frac{\sin(\bar \theta_\mathtt a - \bar \alpha)}{\sin(\bar \alpha)} G(\phi - \bar \phi_0(\mathtt a) - 2\pi - \bar \alpha),
\end{equation}
where the angle $\bar \phi_0(\mathtt a)$ given by
\begin{equation*}
\bar \phi_0(\mathtt a) = \bar \theta_\mathtt a - \bar \alpha.
\end{equation*}

\medskip

\noindent{\it Step 2.} \label{Page:step_2_case_study_segment} Taking the derivative w.r.t. $\bar \theta_\mathtt a$ and using \eqref{Equa:ker_der_G} we get
\begin{align*}
\check r(\phi) &= \frac{d}{d\bar \theta_\mathtt a} r(\phi) \\
&= \bigg( \frac{\cos(\theta_\mathtt a)}{\sin(\bar \alpha)} - \frac{\sin(\theta_\mathtt a)}{\sin(\bar \alpha)} \cot(\bar \alpha) \bigg) G(\phi - \phi_0) \\
& \quad + \bigg( \frac{\sin(\theta_\mathtt a)}{\sin(\bar \alpha)^2} - \frac{\cos(\theta_\mathtt a - \bar \alpha)}{\sin(\bar \alpha)} + \frac{\sin(\theta_\mathtt a - \bar \alpha)}{\sin(\bar \alpha)} \cot(\bar \alpha) \bigg) G(\phi - \phi_0 - (2\pi + \bar \alpha)) \\
& \quad  - \frac{\sin(\theta_\mathtt a - \bar \alpha)}{\sin(\bar \alpha)^2} G(\phi - \phi_0 - 2(2\pi + \bar \alpha)) \\
&= - \frac{\sin(\theta_\mathtt a - \bar \alpha)}{\sin(\bar \alpha)^2} \Big( G(\phi - \phi_0) - 2 \cos(\bar \alpha) G(\phi - \phi_0 - (2\pi + \bar \alpha)) + G(\phi - \phi_0 - 2(2\pi + \bar \alpha)) \Big).
\end{align*}
The latter function, when rescaled by $\rho(\tau) = r(\phi_0 + (2\pi + \bar \alpha) \tau) e^{-\bar c(2\pi + \bar \alpha) \tau}$ is proportional to
\begin{equation}
\label{Equa:case_study_thetader2}
g(\tau) - 2 \cos(\bar \alpha) e^{- \bar c (2\pi +\bar \alpha)} g(\tau - 1) + e^{- 2 \bar c (2 \pi + \bar \alpha)} g(\tau - 2),
\end{equation}
The numerical plot (Fig. \ref{Fig:ckrho_delph_case_tg}) shows that it is positive and strictly increasing, hence by Lemma \ref{lem:key} we conclude that $\frac{\delta dr}{d\bar \theta_\mathtt a} < 0$, so the worst case is $\bar \theta_\mathtt a = \frac{\pi}{2}$, which corresponds to the arc case when $\Delta \phi_\mathtt a = 0$.

\begin{figure}
\includegraphics[scale=.5]{case_study_theta2der2.png}
\caption{Plot of the function \eqref{Equa:case_study_thetader2}.}
\label{Fig:ckrho_delph_case_tg}
\end{figure}

\medskip

\noindent{\it Asymptotic behavior.} For $\mathtt a \in [0,\sin(\bar \alpha)]$ the solution is given by \eqref{Equa:expl_sol_sat_or}:
\begin{equation*}
%\label{Equa:expl_sol_sat_or}
r(\phi) = \frac{1}{\sin(\bar \alpha)} G(\phi - \bar \phi_0(\mathtt a)) - G(\phi - 2\pi) - M(\phi,\bar \phi_1(\mathtt a),\bar \phi_2(\mathtt a)) - \cot(\bar \alpha) G(\phi - \phi_0(\mathtt a) - 2\pi - \bar \alpha).
\end{equation*}
Using the asymptotic expansions of Corollary \ref{Cor:crit_G_M}, we obtain that the coefficient in front of the principal term $\phi e^{\bar c \phi}$ is
\begin{align*}
\frac{2 e^{-\bar c \bar \phi_0}}{\sin(\bar \alpha)} - 2 e^{-\bar c (2\pi)} - \int_{\bar \phi_1}^{\bar \phi_2} 2 e^{- \bar c \phi_0} d\phi_0 - 2 \cot(\bar \alpha) e^{-\bar c \bar \phi_2},
\end{align*}
which is the first case of the asymptotic expansion. The other case is completely similar.
\end{proof}


\subsection{An estimate on the length of the fastest saturated spiral}
\label{Ss:length_spiral_est}


We conclude this section with an estimate on the length $L$ of the fastest saturated spiral when $\mathtt a = 0$. Writing the solution \eqref{Equa:expl_sol_sat} with $\Delta \phi_{\mathtt a = 0} = \tan(\bar \alpha)$ in the variable
\begin{equation}
\label{Equa:rhobase_01}
\rho(\tau) = r_{\mathtt a = 0}(\phi_0 + (2\pi + \bar \alpha) \tau) e^{- \bar c (2\pi + \bar \alpha) \tau}, \quad \phi_0(0) {\color{red}=\phi_0} = \tan(\bar \alpha) + \frac{\pi}{2} - \bar \alpha,
\end{equation}
we obtain
\begin{equation*}
\rho(\tau) = \frac{1}{\sin(\bar \alpha)} g(\tau) - e^{-\bar c(2\pi + \bar \alpha - \frac{\pi}{2} - \tan(\bar \alpha))} g(\tau - \tau_1) - m(\tau,\tau_2,1) - \cot(\bar \alpha) e^{-\bar c(2\pi + \bar \alpha)} g(\tau - 1),
\end{equation*}
where
\begin{equation*}
\tau_1 = 1 - \frac{\frac{\pi}{2} + \tan(\bar \alpha)}{2\pi + \bar \alpha}, \quad \tau_2 = 1 - \frac{\tan(\bar \alpha)}{2\pi + \bar \alpha}.
\end{equation*}
Using the definitions of \gls{gfrak} and \gls{Gfrak} and that $L = \int \frac{r}{\sin(\bar \alpha)}$, we thus have that the length of the spiral is {\color{red}Domanda: perche' gli intervalli temporali qui sono negativi? Forse c'e' un $1-$?}
\begin{equation}
\label{Equa:Lbase_01}
L(\tau) = \begin{cases}
0 & \tau < - \frac{\frac{\pi}{2} - \bar \alpha + \tan(\bar \alpha)}{2\pi + \bar \alpha}, \\
(2\pi + \bar \alpha) \tau + \frac{\pi}{2} - \bar \alpha + \tan(\bar \alpha) & - \frac{\frac{\pi}{2} - \bar \alpha + \tan(\bar \alpha)}{2\pi + \bar \alpha} \leq \tau < - \frac{\frac{\pi}{2} - \bar \alpha}{2\pi + \bar \alpha}, \\
\tan(\bar \alpha) + \cot(\bar \alpha - (2\pi + \bar \alpha) \tau) & - \frac{\frac{\pi}{2} - \bar \alpha}{2\pi + \bar \alpha} \leq \tau < 0, \\
\tan(\bar \alpha) + \cot(\bar \alpha) + \frac{\mathfrak g(\tau)}{\sin(\bar \alpha)} - \mathfrak g(\tau - \tau_1) - (2\pi + \bar \alpha) (\mathfrak G(\tau - \tau_2) - \mathfrak G(\tau - 1)) - \cot(\bar \alpha) \mathfrak g(\tau - 1) & \tau \geq 0.
\end{cases}
\end{equation}
The first terms take into account the initial arc and the initial segment.

\begin{proposition}
\label{Prop:length_compar}
It holds for $\phi \geq \tan(\bar \alpha) + \frac{\pi}{2} - \bar \alpha$
\begin{equation*}
r(\phi) - 2.08 L(\phi - 2\pi - \bar \alpha) \geq 0.67 e^{\bar c(\phi - \tan(\bar \alpha) - \frac{\pi}{2} + \bar \alpha)}.
\end{equation*}
\end{proposition}

\begin{figure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\includegraphics{rhobase_Lbase.png}}
\end{subfigure} \hfill
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\includegraphics{rhobase_Lbase_1.png}}
\end{subfigure}
\caption{Numerical computations of the function \eqref{Equa:rhobase_Lbase_comp}, with a blow-up about the minimum.}
\label{Fig:rhobase_Lbase_comp}
\end{figure}

\begin{proof}
We numerically compute the function
\begin{equation}
\label{Equa:rhobase_Lbase_comp}
\tau \mapsto \rho(\tau) - 2.08 e^{-\bar c (2\pi + \bar \alpha) \tau} L(\tau - 1),
\end{equation}
which is the rescaling of the function in the statement: Fig. \ref{Fig:rhobase_Lbase_comp} shows that the function has a minimum $>0.67$ for $\tau \in [3,4]$ and it is increasing for $\tau \in [4,5]$.

In order to apply Lemma \ref{lem:key}, we write the equation for $r - 2.08 L$. By using the equation for $\mathcal G$ \eqref{Equa:eq_for_calG} we have
\begin{align*}
\dot L(\phi) &= \cot(\bar \alpha) L(\phi) - \frac{L(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} \\
& \quad + (\tan(\bar \alpha) + \cot(\bar \alpha) \delta_{\frac{\pi}{2} - \bar \alpha + \tan(\bar \alpha)} + \frac{H(\phi - \tan(\bar \alpha) - \frac{\pi}{2} + \bar \alpha)}{\sin(\bar \alpha)} - H(\phi - 2\pi) - \cot(\bar \alpha) H \bigg( \phi - \frac{5\pi}{2} \bigg).
\end{align*}
Recall that \gls{Heavyside} is the Heavyside function. Hence for $\phi \geq \frac{5\pi}{2}$ we have \newglossaryentry{SL}{name=\ensuremath{S_L},description={source term for the length $L$ of a spiral}}
\begin{equation*}
\frac{d}{d\phi} L(\phi) = \cot(\bar \alpha) L(\phi) - \frac{L(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} + \gls{SL},
\end{equation*}
where
\begin{equation*}
\gls{SL} = \frac{1}{\sin(\bar \alpha)} - 1 - \cot(\bar \alpha) = -0.331672 < 0.
\end{equation*}
Hence for $\phi \geq \tan(\bar \alpha) + \frac{\pi}{2} - \bar \alpha + 2(2\pi + \bar \alpha)$ we have
\begin{align*}
\frac{d}{d\phi} (r(\phi) - 2.08 L(\phi - 2\pi - \bar \alpha)) &= \cot(\bar \alpha) (r(\phi) - 2.08 L(\phi - 2\pi - \bar \alpha)) - \frac{r(\phi - 2\pi - \bar \alpha) - 2.08 L(\phi - 2(2\pi + \bar \alpha))}{\sin(\bar \alpha)} - S_L \\
&\geq \cot(\bar \alpha) (r(\phi) - 2.08 L(\phi - 2\pi - \bar \alpha)) - \frac{r(\phi - 2\pi - \bar \alpha) - 2.08 L(\phi - 2(2\pi + \bar \alpha))}{\sin(\bar \alpha)}.
\end{align*}
Therefore in therms of $\tau$ we obtain
\begin{equation*}
\frac{d}{d\tau} (\rho(\tau) - 2.08 e^{-\bar c(2\pi + \bar \alpha) \tau} L(\tau-1)) \geq (\rho(\tau) - 2.08 e^{-\bar c(2\pi + \bar \alpha) \tau} L(\tau-1)) - (\rho(\tau-1) - 2.08 e^{-\bar c(2\pi + \bar \alpha) (\tau-1)} L(\tau-2)),
\end{equation*}
so that Lemma \ref{lem:key} and Remark {\color{red}A quale remark ti riferisci?} \ref{rmk:exponentially:explod} may be applied.
\end{proof}

\begin{remark}
\label{Rem:asymtp_consta_for_comp}
The asymptotic constant for the length should be
\begin{equation*}
\frac{r(\phi)}{L(\phi-2\pi-\bar \alpha)} \sim e^{\bar c} \bar c \sin(\bar \alpha) = 2.08884,
\end{equation*}
obtained by using $r(\phi) \sim \phi e^{\bar c \phi}$. However for this exact value we cannot use Lemma \ref{lem:key}, obviously.
\end{remark}

%We conclude with an additional estimate, which will be helpful when estimating the positivity of the optimal solution. Define the functional 

==> familydiv__1_.tex <==

\section{A differentiable path of spirals}
\label{S:family}


Let $\zeta(s)$, $s \in [0,L]$, be a given admissible spiral {\color{red}L'abbiamo chiamata $\bar \zeta$?}. In this section we construct a family of admissible spirals \newglossaryentry{zetatildefam}{name=\ensuremath{\tilde \zeta(s;s_0)},description={family of admissible spirals, parametrized by $s_0$}} \gls{zetatildefam} with the following properties:
\begin{enumerate}
\item for $s \in [0,s_0]$ it holds $\tilde \zeta(s;s_0) = \zeta(s)$;
\item in the first round starting from $\zeta(s_0)$, the spiral $\tilde \zeta(s;s_0)$ is the fastest closing spiral;
\item after the first round, the spiral $\tilde \zeta(s;s_0)$ is the saturated spiral.
\end{enumerate}
We call each spiral \newglossaryentry{Ztildes0}{name=\ensuremath{\tilde Z(s_0)},description={fastest saturated spiral starting from $s_0$}} $\gls{Ztildes0} = \tilde \zeta([0,L];s_0)$ the \emph{fastest saturated spiral starting from $s_0$}. The map $s_0 \mapsto \tilde Z(s_0)$ defines a path in the space of admissible spirals, connecting the fastest saturated spiral of the previous section (corresponding to $\tilde \zeta(s;0)$) with the given spiral $Z = \zeta([0,s])$.

If we denote by \newglossaryentry{phi0initangle}{name=\ensuremath{\phi_0 = (s^+)^{-1}(s_0)},description={initial angle for the admissible family of spiral $\tilde \zeta(s,;s_0)$}} \gls{phi0initangle} the initial angle of the above construction, then the first round is determined by
\begin{equation*}
\phi_0 \leq \phi \leq \phi_0 + \beta^-(\phi_0),
\end{equation*}
In the following we will write both $\tilde \zeta(\cdot;s_0),\tilde r(\cdot;s_0)$ and $\tilde \zeta(\cdot;\phi_0),\tilde r(\cdot;\phi_0)$ to denote this admissible family of spirals, and the argument $\cdot$ can be either the arc length $s$ or the rotation angle $\phi$.

It is immediate to deduce the following lemma.

\begin{lemma}
\label{Lem:tilde_zeta_prop}
The family of spirals $\tilde \zeta(s;s_0)$ satisfies the following properties:
\begin{enumerate}
\item $\tilde \zeta(s;L) = \zeta(s)$;
\item $\tilde \zeta(s;0)$ is the fastest saturated spiral constructed in Section \ref{S:case:study};
\item if $s$ belongs to the first round starting from $\zeta(s_0)$, then the solution is given by Theorem \ref{Cor:curve_cal_R_sat_spiral};
\item after the first round, denoting with \newglossaryentry{rtildefam}{name=\ensuremath{\tilde r(\phi;s_0)},description={family of admissible spirals in the rotation angle coordinate $\phi$, parametrized by $s_0$}} \gls{rtildefam} the representation in the rotation angle coordinates, we have
\begin{equation*}
\frac{d}{d\phi} \tilde r(\phi;s_0) = \cot(\bar \alpha) \tilde r(\phi;s_0) - \frac{\tilde r(\phi - 2\pi + \bar \alpha;s_0)}{\sin(\bar \alpha)}.
\end{equation*}
\end{enumerate}
\end{lemma}

Since the construction of Theorem \ref{Cor:curve_cal_R_sat_spiral} is explicit, the last point above yields that the family is completely determined, up to computing the solution in the first round after $s_0$ and solving the saturated RDE.

The main result of this section is to prove that this family is $C^1$-w.r.t. the parameter $s_0$: more precisely, we will show that the limit of the incremental ratio \newglossaryentry{deltartildefam}{name=\ensuremath{\delta \tilde r(\phi;s_0)},description={derivative of the family $\tilde r(s;s_0)$ w.r.t. $s_0$}}
\begin{equation*}
\gls{deltartildefam} := \lim_{\delta s_0 \searrow 0} \frac{\tilde r(\phi;s_0 + \delta s_0) - \tilde r(\phi;s_0)}{\delta s_0}
\end{equation*}
exists outside a finite number of angles $\phi$, and it satisfies a precise RDE, which allows the explicit computation of the $\delta \tilde r$. The dependence on the base spiral $\zeta$ enters only in two real parameters of the initial data of $\delta \tilde r$, allowing to write its explicit form with similar computations: indeed, the form of the RDE satisfied by the perturbation is very similar to the RDE satisfied by the solution $r(\phi)$ or its derivative $\frac{d}{d\mathtt a} r(\phi)$ {\color{red} qui e' giusta la derivata rispetto al parametro $a$?} considered in Section \ref{S:case:study}, and will be studied with similar techniques. In particular, depending whether the non-saturated part of the fastest closing spiral at the first round is a segment or is an arc+segment, the derivative takes different form, and we will study them separately in two different subsections, Subsections \ref{S:segment} and \ref{S:arc}.

\begin{remark}
\label{Rem:segmet_sub_arc0}
We remark that the segment case can be recovered from the arc case when the initial level set is just one point: however we believe that it is simpler and very instructive to perform the analysis in the segment case.

We anticipate also that  $\delta \tilde r(\phi;s_0)$ is not positive in an interval of the second round, and thus it cannot be optimal for some angles. Hence to prove the {\color{blue} main theorem} we will need an additional perturbation of the last round: we address this fact in Section \ref{S:optimal_sol_candidate}.
\end{remark}

Since in the last round we have already the explicit form of the optimal closing solution, we can assume that $\zeta$ makes at least one round after $\phi_0$, so that there will always be a saturated part.


\subsection{Analysis of $\tilde \zeta(s;s_0)$ - Segment Case}
\label{S:segment}


The assumption on $\tilde \zeta(\phi;s_0)$ is that for $\phi \in \phi_0 + [0,2\pi + \beta^-(\phi_0))$ it is made of
\begin{itemize}
\item a segment $[P_1,P_2]$ where $P_1 = \zeta(s_0) = \zeta(s^+_0(\phi_0))$, followed by
\item a saturated spiral with $\beta(\phi) = \bar \alpha$.
\end{itemize}
The spiral $\tilde r(\phi,s_0)$ will then proceed for all angles $\phi \geq \phi_0 + 2\pi + \beta^-(\phi_0)$ as a saturated spiral, i.e. $\beta(\phi) = \bar \alpha$ constant. Following the notation of Step 1 in Case $\Delta \phi_\mathtt a = 0$ of the proof of Theorem \ref{thm:case:a}, we will denote by $\bar \theta$ the angle \newglossaryentry{thetatildeseg}{name=\ensuremath{\bar \theta},description={angle of the initial segment $[P_1,P_2]$ for the family $\tilde \zeta(\cdot;s_0)$}}
\begin{equation}
\label{eq:ba:theta}
\gls{thetatildeseg} = \angle(e^{i\phi_0},[P_1,P_2]).
\end{equation}

The same structure (i.e. an initial segment followed by a saturated spiral) holds for the spiral $\tilde r(\phi;s_0 + \delta s_0)$, starting from the point $\zeta(s_0 + \delta s_0)$ if $\delta s_0 \ll 1$ and $\bar \theta < \frac{\pi}{2}$, i.e. there will be an initial segment
$$
[P_1',P_2'] = [P_1 + \delta P_1, P_2 + \delta P_2],
$$
with the angles
$$
s^+(\phi_0') = s_0^+(\phi_0 + \delta \phi_0) = s_0 + \delta s_0, \quad \bar \theta' = \bar \theta + \delta \bar \theta = \angle(e^{i\phi_0},[P_1',P_2']),
$$
followed by a saturated spiral. The analysis of this section refers to Figure \ref{segm:per}. 

\begin{figure}
\centering
\includegraphics[scale=0.7]{segment_pert.png}
\caption{Analysis of perturbations for the segment case.}
\label{segm:per}
\end{figure}

The fact that the spirals are convex and there are no smaller admissible convex spirals for the first round $[\phi_0,\phi_0 + 2\pi + \beta^-(\phi_0))$ by Proposition \ref{Prop:der_calR} implies that \newglossaryentry{theta0pertsegm}{name=\ensuremath{\theta_0 = \beta^+(s_0)},description={minimal initial angle for the segment in the segment case, Section \ref{S:segment}}}
\begin{equation*}
0 < \gls{theta0pertsegm} \leq \bar \theta, \quad \bar \alpha \leq \bar \theta,
\end{equation*}
where the second is due to the fact that the point $\zeta(s_0)$ is not saturated if $P_1 \not= P_2$. We will denote by $\theta$ the angle \newglossaryentry{thetapertsegm}{name=\ensuremath{\theta},description={variation of the direction of the spiral at $s_0$}}
\begin{equation*}
\gls{thetapertsegm} = \bar \theta - \theta_0.
\end{equation*}

We compute now the variations up to second order terms w.r.t. $\delta s_0$:
\begin{equation}\label{eq:sec6:imp}
\delta P_1 = \delta s_0 e^{\i (\phi_0 + \theta_0)}, \quad \delta \phi_0 = \frac{\delta s_0 \sin(\theta_0)}{r(\phi_0)},
\end{equation}
\begin{align}\label{delta:p2:segment}
\delta P_2 &= \delta P_1 + \delta |P_2 - P_1| e^{\i (\phi_0 + \bar \theta)} + |P_2 - P_1| \delta \bar \theta e^{\i (\phi_0 + \bar \theta + \frac{\pi}{2})} \\
\notag &= \delta s_0 e^{\i (\phi_0 + \theta_0)} + \delta |P_2 - P_1| e^{\i (\phi_0 + \bar \theta)} + |P_2 - P_1| \delta \bar \theta e^{\i (\phi_0 + \bar \theta + \frac{\pi}{2})}.
\end{align}
Since the point $P_2'$ is saturated, we obtain
\begin{equation*}
0 = u(P_2') - \cos(\bar \alpha) (\delta s_0 + |P_2' - P_1'|+L(P_0)),
\end{equation*}
where $L(P_0)$ is the length of the spiral up to the angle $\phi_0$. In particular, observing that $\nabla u = e^{\i (\phi_0 + \bar \theta - \bar \alpha)}$,
\begin{align*}
 0 &= e^{\i (\phi_0 + \bar \theta - \bar \alpha)} \cdot \delta P_2 - \cos(\bar \alpha) (\delta s_0 + \delta |P_2 - P_1|) \\
&= \delta s_0 \cos(\bar \theta - \theta_0 - \bar \alpha) + \delta |P_2 - P_1| \cos(\bar \alpha) - |P_2 - P_1| \delta \theta \sin(\bar \alpha) - \cos(\bar \alpha) (\delta s_0 + \delta |P_2 - P_1|) \\
&= \delta s_0 \cos(\bar \alpha - \theta) + \delta |P_2 - P_1| \cos(\bar \alpha) - |P_2 - P_1| \delta \theta \sin(\bar \alpha) - \cos(\bar \alpha) (\delta s_0 + \delta |P_2 - P_1|)
\end{align*}
where we recall that $\cdot$ denotes the scalar product in $\R^2$. We thus deduce that
\begin{equation}
\label{Equa:delta_theta_segm_1}
\frac{|P_2 - P_1| \delta \theta}{\delta s_0} = \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)}.
\end{equation}
Imposing that the angle at $P_2'$ with the fire ray is the critical angle $\bar \alpha$, we deduce that $P_2'$ corresponds to the angle $\phi_2 + \delta \theta$, where $\phi_2 = \phi_0 + \bar \theta - \bar \alpha$ is the angle corresponding to $P_2$ in the fire representation for $\tilde r(\phi;s_0)$. Hence, imposing this relation we obtain
\begin{align*}
    r(\phi_2) \delta \theta &= e^{\i (\phi_0 + \bar \theta - \bar \alpha + \frac{\pi}{2})} \cdot \delta P_2 \\
    &= \delta s_0 \sin(\bar \alpha - \theta) + \delta |P_2 - P_1| \sin(\bar \alpha) + |P_2 - P_1| \delta \theta \cos(\bar \alpha),
\end{align*}
so that using \eqref{Equa:delta_theta_segm_1} we conclude that
\begin{equation}
\label{Equa:delta_P_2P_1_segm}
\begin{split}
\frac{\delta |P_2 - P_1|}{\delta s_0} - \frac{r(\phi_2)}{\sin(\bar \alpha)} \frac{\delta \theta}{\delta s_0} &= \cot(\bar \alpha) \frac{\cos(\bar \alpha) - \cos(\bar \alpha - \theta)}{\sin(\bar \alpha)} + \frac{\sin(\theta - \bar \alpha)}{\sin(\bar \alpha)} \\
&= \frac{\cos(\bar \alpha)^2 - \cos(\theta)}{\sin(\bar \alpha)^2} = - 1 + \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2}.
\end{split}
\end{equation}

To compute the perturbation $\delta \tilde r(\phi;s_0)$ for $\phi \geq \phi_2$, we observe that $\beta(\phi) = \bar \alpha$ in this region, so that, denoting with $R(\phi)$ the radius of curvature of the base spiral $r(\phi)$, one obtains

\begin{lemma}
\label{Lem:equation_segment_tilde_r}
The RDE satisfied by $\tilde r$ for $\phi \geq \phi_0 + \bar \theta - \bar \alpha$ is
\begin{equation}
\label{Equa:segm_equ_tilde_r}
\frac{d}{d\phi} \tilde r(\phi;s_0) = \cot(\bar \alpha) \tilde r(\phi;s_0) - \begin{cases}
R(\phi) & \phi_0 + \bar \theta - \bar \alpha \leq \phi < \phi_0 + 2\pi + \beta^-(\phi_0), \\
0 & \phi_0 + 2\pi + \beta^-(\phi_0) \leq \phi < \phi_0 + 2\pi + \bar \theta, \\
|P_2 - P_1| \Diracd_{\phi_0 + 2\pi + \bar \theta} + \frac{\tilde r(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} & \phi \geq \phi_0 + 2\pi + \bar\theta.
\end{cases}
\end{equation}
\end{lemma}

\begin{proof}
We have just to compute the radius of curvature, since $\beta = \bar \alpha$ fixed. Formula \eqref{Equa:segm_equ_tilde_r} follows easily, observing that if $\beta^-(s_0) < \bar \theta$ then there is corner in the spiral $\tilde r(\phi;s_0)$ whose subdifferential is
\begin{equation*}
\partial^- \tilde r(\phi_0;s_0) = \big\{ e^{i\phi}, \phi \in \phi_0 + [\beta^-(\phi_0),\bar \theta] \big\}.
\end{equation*}
The jump at $\phi_0 + 2\pi + \bar \theta$ is due to the segment $[P_1,P_2]$, corresponding in a jump in $s^-(\phi)$ at that angle.
\end{proof}

In the next proposition we compute the RDE satisfied by the derivative $\delta \tilde r(\phi;s_0)$ w.r.t. $s_0$, for angles $\phi > \phi_0 + \bar \theta - \bar \alpha$.

\begin{proposition}
\label{Prop:equa_delta_tilde_r_segm}
For $\phi > \phi_0 + \bar \theta - \bar \alpha$, the derivative 
$$
\delta \tilde r(\phi;s_0) = \lim_{\delta s_0 \searrow 0} \frac{\tilde r(\phi;s_0 + \delta s_0) - \tilde r(\phi;s_0)}{\delta s_0}
$$
satisfies the RDE on $\R$
\begin{equation*}
\frac{d}{d\phi} \delta \tilde r(\phi;s_0) = \cot(\bar \alpha) \delta \tilde r(\phi;s_0) - \frac{\delta \tilde r(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} + S(\phi;s_0),
\end{equation*}
with source
\begin{align*}
S(\phi;s_0) &= \cot(\bar \alpha) \frac{1 - \cos(\theta)}{\sin(\bar \alpha)} \Diracd_{\phi_0 + \bar \theta - \bar \alpha} - \Diracd_{\phi_0 + 2\pi + \theta_0} \\
& \quad + \frac{\cos(\theta) - \cos(\bar \alpha)^2}{\sin(\bar \alpha)^2} \Diracd_{\phi_0 + 2\pi + \bar \theta} + \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} \Diracd'_{\phi_0 + 2\pi + \bar \theta}.
\end{align*}
\end{proposition}

\begin{proof}
For shortness denote by $\phi_2$ the angle $\phi_0 + \bar \theta - \bar \alpha$.

We compute first the variation of the initial data of \eqref{Equa:segm_equ_tilde_r}: observing that the spiral $\tilde r(\phi;s_0)$ is saturated at $\phi_2$ and hence its tangent vector is $e^{\i (\phi_0 + \bar \theta)}$, one has up to second order terms for $\phi$ close to $\phi_2$ 
\begin{align*}
\tilde r(\phi;s_0 + \delta s_0) - \tilde r(\phi;s_0) &= \frac{e^{\i (\phi_0 + \bar \theta - \frac{\pi}{2})} \cdot \delta P_2}{\sin(\bar \alpha)} \\
&= \delta s_0 \frac{\sin(\theta)}{\sin(\bar \alpha)} - \frac{|P_2 - P_1| \delta \theta}{\sin(\bar \alpha)} \\
&= \delta s_0 \cot(\bar \alpha) \frac{1 - \cos(\theta)}{\sin(\bar \alpha)},
\end{align*}
which gives the first jump at $\phi_0 + \bar \theta - \bar \alpha$.

Being $R(\phi)$ the same up to $\phi_0 + 2\pi + \theta_0$, the RDE for $\delta \tilde r$ is actually the ODE
\begin{equation*}
\frac{d}{d\phi} \delta \tilde r(\phi) = \cot(\bar \alpha) \delta \tilde r(\phi)
\end{equation*}
for $\phi_0 + \bar \theta - \bar\alpha \leq \phi < \phi_0 + 2\pi + \theta_0$.

Using $R = Ds^-$, the variation at $\phi_0 + 2\pi + \theta_0$ is
\begin{align*}
\tilde r(\phi;s_0 + \delta s_0) - \tilde r(\phi;s_0) &= \cot(\bar \alpha) \big( \tilde r(\phi;s_0 + \delta s_0) - \tilde r(\phi;s_0) \big) - \big( s^-(\phi) - s^-(\phi_0 + 2\pi + \theta_0) \big) \\
&= \cot(\bar \alpha) \big( \tilde r(\phi;s_0 + \delta s_0) - \tilde r(\phi;s_0) \big) - \delta s_0.
\end{align*}
Hence $\delta \tilde r(\phi;s_0)$ has a jump of size $-1$ at the angle $\phi_0 + 2\pi + \theta_0$, due to the change of slope at the corner $P_1$.

From \eqref{Equa:segm_equ_tilde_r} it follows that
\begin{equation*}
\frac{d}{d\phi} \delta \tilde r(\phi) = \cot(\bar \alpha) \delta \tilde r(\phi)
\end{equation*}
for $\phi_0 + 2\pi + \theta_0 < \phi < \phi_0 + 2\pi + \bar \theta$.

At the angle $\phi_0 + 2\pi + \bar \theta$, computing the first order approximations for $0 \leq \phi - \phi_0 + 2\pi + \bar \theta \ll 1$ one gets up to second order terms
\begin{align*}
\tilde r(\phi;s_0 + \delta s_0) - \tilde r(\phi;s_0) &= \bigg[ \tilde r(\phi_0 + 2\pi + \bar\theta; s_0 + \delta s_0) + \cot(\bar \alpha) \tilde r(\phi_0 + 2\pi + \bar\theta;s_0 + \delta s_0) (\phi - \phi_0 - 2\pi - \bar \theta) \\
& \quad \quad - |P_2' - P_1'| \big( 1 + \cot(\bar \alpha) (\phi - \phi_0 - 2\pi - \bar \theta - \delta \bar \theta) \big) \ind_{\phi \geq \phi_0 + 2\pi + \bar \theta + \delta \bar \theta} \\
& \quad \quad - \frac{\tilde r(\phi_0 + \bar \theta - \bar \alpha;s_0 + \delta s_0)}{\sin(\bar \alpha)} (\phi - \phi_0 - 2\pi - \bar \theta - \delta \bar \theta) \bigg] \\
& \quad - \bigg[ \tilde r(\phi_0 + 2\pi + \theta-;s_0) + \cot(\bar \alpha) \tilde r(\phi_0 + 2\pi +\theta;s_0) (\phi - \phi_0 - 2\pi - \bar \theta) \\
& \quad \quad - |P_2 - P_1| \big( 1 + \cot(\bar \alpha) (\phi - \phi_0 - 2\pi - \bar \theta) \big) \ind_{\phi \geq \phi_0 + 2\pi + \bar \theta}  \\
& \quad \quad - \frac{\tilde r(\phi_0 + \bar \theta - \bar \alpha;s_0)}{\sin(\bar \alpha)} (\phi - \phi_0 - 2\pi - \bar \theta) \bigg] \\
&= \big( \tilde r(\phi_0 + 2\pi + \bar\theta;s_0 + \delta s_0) - \tilde r(\phi_0 + 2\pi + \bar\theta;s_0) \big) \big( 1 + \cot(\bar \alpha) (\phi - \phi_0 - 2\pi - \bar \theta) \big) \\
& \quad - \frac{\tilde r(\phi_0 + \bar \theta - \bar \alpha;s_0 + \delta s_0) - \tilde r(\phi_0 + \bar \theta - \bar \alpha;s_0)}{\sin(\bar \alpha)} (\phi - \phi_0 - 2\pi - \bar \theta) \\
& \quad + \bigg( - \delta |P_2 - P_1| + \frac{\tilde r(\phi_0 + \bar \theta - \bar \alpha;s_0)}{\sin(\bar \alpha)} \bigg) \ind_{\phi \geq \phi_0 + 2\pi + \bar \theta} + |P_2 - P_1| \ind_{[\phi_0 + 2\pi + \bar \theta,\phi_0 + 2\pi + \bar \theta + \delta \theta)}.
\end{align*}
For the above formula, we have used that the jumps $|P_2 - P_1|$ are in different angles and that the curvature term $- \frac{\tilde r(\phi_0+\bar \theta -\bar \alpha;s_0)}{\sin(\bar \alpha)}$ is applied starting from different angles. \\
Passing to the limit $\delta s_0 \searrow 0$ we obtain
\begin{align*}
\delta \tilde r(\phi;s_0) &= \delta \tilde r(\phi_0 + 2\pi + \bar\theta;s_0) \big( 1 + \cot(\bar \alpha) (\phi - \phi_0 - 2\pi - \bar \theta) \big) - \frac{\delta \tilde r(\phi_0 + \bar \theta - \bar \alpha;s_0)}{\sin(\bar \alpha)} (\phi - \phi_0 - 2\pi - \bar \theta) \\
& \quad + \bigg( - \frac{\delta |P_2 - P_1|}{\delta s_0} + \frac{\tilde r(\phi_0 + \bar \theta - \bar \alpha;s_0)}{\sin(\bar \alpha)} \frac{\delta \theta}{\delta s_0} \bigg) \ind_{\phi \geq \phi_0 + 2\pi + \bar \theta} + |P_2 - P_1| \frac{\delta \theta}{\delta s_0} \Diracd_{\phi_0 + 2\pi + \bar \theta}.
\end{align*}
Hence its derivative w.r.t. $\phi$ satisfies
\begin{align*}
\frac{d}{d\phi} \delta \tilde r(\phi;s_0) &= \cot(\bar \alpha) \delta \tilde r(\phi;s_0) - \frac{\delta \tilde r(\phi - 2\pi - \bar \alpha;s_0)}{\sin(\bar \alpha)} \\
& \quad + \bigg( - \frac{\delta |P_2 - P_1|}{\delta s_0} + \frac{\tilde r(\phi_0 + \bar \theta - \bar \alpha;s_0)}{\sin(\bar \alpha)} \frac{\delta \theta}{\delta s_0}  \bigg) \Diracd_{\phi_0 + 2\pi + \bar\theta} + |P_2 - P_1| \frac{\delta \theta}{\delta s_0} \Diracd'_{\phi_0 + 2\pi + \bar \theta},
\end{align*}
where $\Diracd'$ is the derivative of the Dirac's delta:
\begin{equation*}
\langle \Diracd'_x, f \rangle = - \frac{df(x)}{dx}.
\end{equation*}
Using \eqref{Equa:delta_theta_segm_1} and \eqref{Equa:delta_P_2P_1_segm} we obtain
\begin{align*}
- \frac{\delta |P_2 - P_1|}{\delta s_0} + \frac{\bar r(\phi_0 + \bar \theta - \bar \alpha;s_0)}{\sin(\bar \alpha)} \frac{\delta \theta}{\delta s_0} &= \cot(\bar \alpha) \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} - \frac{\sin(\theta - \bar \alpha)}{\sin(\bar \alpha)} \\
&= \frac{\cos(\theta - \theta_0) - \cos(\bar \alpha)^2}{\sin(\bar \alpha)^2},
\end{align*}
\begin{equation*}
|P_2 - P_1| \frac{\delta \theta}{\delta s_0} = \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)}.
\end{equation*}
It is now easy to verify that the derivative $\delta \tilde r(\phi;s_0) \rest_{\phi_0 + \bar \theta - \bar \alpha}$ satisfies the RDE in the statement, since in the remaining part it solves a linear RDE.
\end{proof}

Since
\begin{equation}
\label{Equa:segm_part_of_segm}
\sin(\theta) - \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} = \cot(\bar \alpha) (1 - \cos(\bar \theta)) \geq 0,
\end{equation}
it follows that the perturbation is positive for $\phi \in [\phi_0,\phi_0+\bar \theta - \bar \alpha]$, and it is given explicitly by
\begin{equation*}
\delta \tilde r(\phi;s_0) = \frac{1}{\sin(\phi_0 + \bar \theta - \phi)} \bigg( \sin(\theta) - \frac{|P(\phi) - P_1|}{|P_2 - P_1|} \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} \bigg),
\end{equation*}
where $P(\phi)$ is the position of the point on $[P_1,P_2]$ corresponding to the angle $\phi \in [\theta_0,\theta_0 + \bar \theta - \bar \alpha]$.

\begin{corollary}
\label{Cor:evolv_r_after_phi_2}
The solution $\delta \tilde r(\phi)$ for $\phi \geq \phi_2 = \phi_0 + \bar \theta - \bar \alpha$ is explicitly given by
\begin{equation}
\label{Equa:evolv_r_after_phi_2}
\begin{split}
\delta \tilde r(\phi) &= \cot(\bar \alpha) \frac{1 - \cos(\theta)}{\sin(\bar \alpha)} G(\phi - \phi_0 - \bar \theta + \bar \alpha) - G(\phi - \phi_0 - 2\pi - \theta_0) \\
&\quad + \bigg( 1 - \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} + \cot(\bar \alpha) \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} \bigg) G(\phi - 2\pi - \phi_0 - \bar \theta) \\
& \quad + \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} \Diracd_{\phi - 2\pi - \phi_0 - \bar \theta} - \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)^2} G(\phi - 4\pi - \bar \theta - \bar \alpha),
\end{split}
\end{equation}
where $G(\phi)$ is the Green kernel for the RDE.
\end{corollary}

\begin{proof}
The formula follows from Remark \ref{Rem:oringal_phi_kernel}.
\end{proof}

To proceed further, we rewrite the RDE translating $\phi_0 + \bar \theta - \bar \alpha$ to $0$ and then use the new variable
\begin{equation}
\label{Equa:rho_segm_r}
\rho(\tau) = \delta \tilde r(\phi_0 + \bar \theta - \bar \alpha + (2\pi + \bar \alpha) \tau;s_0) e^{- \bar c (2\pi + \bar \alpha) \tau}.
\end{equation}

\begin{corollary}
\label{Cor:equation}
The values of the perturbation $\delta r(s;s_0)$ depend uniquely on the angle $\theta = \bar \theta - \theta_0 \in [0,\frac{\pi}{2}]$, and the function $\rho(\tau)$ of Equation \eqref{Equa:rho_segm_r} is given explicitly by the formula \newglossaryentry{tau1}{name=\ensuremath{\tau_1},description={time of the first discontinuity for the perturbation in the segment and arc case}}
\begin{equation}
\label{Equa:equa_rho_segm_666}
\rho(\tau) = S_0 g(\tau) + S_1 g(\tau - \tau_1) + S_2 g(\tau-1) + D \Diracd_1 + S_3 g(\tau - 2), \quad \gls{tau1} = 1 - \frac{\theta}{2\pi + \bar \alpha},
\end{equation}
with
\begin{subequations}
\label{Equa:source_segmnt_pert}
\begin{equation}
\label{Equa:S0_segment_pert}
S_0(\theta) = \cot(\bar \alpha) \frac{1 - \cos(\theta)}{\sin(\bar \alpha)},
\end{equation}
\begin{equation}
\label{Equa:S1_segment_pert}
S_1(\theta) = - e^{- \bar c (2\pi + \bar \alpha - \theta)} = - \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} e^{\bar c \theta},
\end{equation}
\begin{equation}
\label{Equa:S2_segment_pert}
\begin{split}
S_2(\theta) &= \bigg( 1 - \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} + \cot(\bar \alpha) \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} \bigg) e^{-\bar c (2\pi + \bar \alpha)} \\
&= \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} - \frac{1 - \cos(\theta)}{(2\pi + \bar \alpha) \sin(\bar \alpha)} + \frac{\cot(\bar \alpha)}{2\pi + \bar \alpha} \big( \cos(\bar \alpha - \theta) - \cos(\bar \alpha) \big),
\end{split}
\end{equation}
\begin{equation}
\label{Equa:D_source_segme}
D(\theta) = \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} e^{-\bar c (2\pi + \bar \alpha)} = \frac{\cos(\bar \alpha -\theta) - \cos(\bar \alpha)}{2\pi + \bar \alpha},
\end{equation}
\begin{equation}
\label{Equa:S3_segment_pert}
S_3(\theta) = - \frac{\cos(\bar \alpha -\theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)^2} e^{-\bar c (4\pi + 2 \bar \alpha)} = - \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{(2\pi + \bar \alpha)^2}.
\end{equation}
\end{subequations}
\end{corollary}

We remark that we have used Equation \eqref{Equa:c_gene_defi} to replace $e^{- \bar c(2\pi + \bar \alpha)}$ with $\frac{\sin(\bar \alpha)}{2\pi + \bar \alpha}$.

The study of the sign of $\rho$ given by \eqref{Equa:equa_rho_segm_666} is done in the next proposition, which is the main statement of this section concerning the segment case. For some future needs, we let $\theta$ to vary in $[0,\pi]$.

\begin{proposition}
\label{Prop:regions_pos_neg_segm}
The function $\rho(\tau) = \rho(\tau,\theta)$ is strictly positive outside the region \newglossaryentry{Nsegm}{name=\ensuremath{N_\mathrm{segm}},description={negative region for the perturbation of the segment case}}
\begin{equation}
\label{Equa:neg_segmnt_666}
\gls{Nsegm} := \bigg\{ 1 - \frac{\theta}{2\pi + \bar \alpha} \leq \tau \leq 1, 0 \leq \theta \leq \hat \theta \bigg\} \cup \big\{ \theta = 0 \} \cup \{ \tau = 1, \theta \in [2\bar \alpha,\pi] \big\} \subset \R \times [0,\pi],
\end{equation}
where the angle \newglossaryentry{thetahat}{name=\ensuremath{\hat \theta},description={angle corresponding to the boundary of the negativity region of the perturbation in the segment case, Equation (\ref{Equa:hat_theta_det_666})}} \gls{thetahat} is determined by the unique solution to
\begin{equation}
\label{Equa:hat_theta_det_666}
\cot(\bar \alpha) \frac{1 - \cos(\hat \theta)}{\sin(\bar \alpha)} -  e^{- \cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} = 0, \qquad \hat \theta \in [0,\pi].
\end{equation}
Moreover, as $\tau \to \infty$, the function $\rho(\tau)$ diverges like
\begin{equation*}
\lim_{\tau \to \infty} \frac{\rho(\tau) e^{-\bar c \tau}}{\tau} = 2 (S_0 + S_1 + S_2 + S_3), \quad 2 (S_0 + S_1 + S_2 + S_3) \in \theta^2 (0.08,028).
\end{equation*}
\end{proposition}

\begin{figure}
\includegraphics[scale=.6]{hattheta_comput2.png}\hfill\includegraphics[scale=.6]{first_round.rhosegm1.png}
\caption{Plot of the function (\ref{Equa:hat_theta_det_666}) on the left side, and of the solution (\ref{Equa:rho_segm_first}) on the right side.}
\label{Fig:hattheta_comput}
\end{figure}

A numerical computation gives the value (see Fig. \ref{Fig:hattheta_comput})
\begin{equation}
\label{Equa:hat_theta_value}
\hat \theta = 0.506134.
\end{equation}

\begin{proof}
We start by observing that for $\theta = 0$ the coefficients \eqref{Equa:source_segmnt_pert} are all $0$, so that the solution \eqref{Equa:equa_rho_segm_666} is $0$. Hence $\{\theta = 0\} \subset N_\mathrm{segm}$.

\medskip

{\it Step 1: computation of the first round.}

\noindent For $\tau \in [0,1)$ the solution is explicitly computed as
\begin{equation}
\label{Equa:rho_segm_first}
\rho(\tau) = S_0 e^\tau + S_1 e^{\tau - \tau_1} \ind_{\tau \geq \tau_1} = e^{\tau} (S_0 + S_1 e^{-\tau_1} \ind_{\tau \geq \tau_1}).
\end{equation}
The solution $\rho$ is thus negative only when $\tau_1 \leq \tau < 1$  and iff
\begin{equation*}
S_0 + S_1 e^{-\tau_1} = \cot(\bar \alpha) \frac{1- \cos(\theta)}{\sin(\bar \alpha)} - \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} e^{(\bar c + \frac{1}{2\pi + \bar \alpha})  \theta - 1} \leq 0,
\end{equation*}
which is \eqref{Equa:hat_theta_det_666}. This gives the angle $\hat \theta$: indeed
the function
\begin{equation*}
\theta \mapsto f(\theta) = (1 - \cos(\theta)) e^{- (\bar c + \frac{1}{2\pi + \bar \alpha}) \theta} = (1 - \cos(\theta)) e^{- \cot(\bar \alpha) \theta}
\end{equation*}
has first derivative
\begin{align*}
f'(\theta) &= \big( \sin(\theta) - \cos(\bar \alpha) (1 - \cos(\theta)) \big) e^{-\cot(\bar \alpha) \theta} = \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} e^{- \cot(\bar \alpha) \theta} > 0 \quad \text{if} \ \theta > 0,
\end{align*}
because $\bar \alpha > \frac{\pi}{4}$, and
$$
f(0) = -1, \quad f \bigg( \frac{\pi}{2} \bigg) = e^{-\cot(\bar \alpha) \frac{\pi}{2}} > 0.
$$
Hence there is only one zero for $f$, and numerically one obtains the value $\hat \theta = 0.506134$, see Figure \ref{Fig:hattheta_comput}.

\medskip

\begin{figure}
\includegraphics[scale=.6]{second_round.rhosegm_orig1.png}\hfill\includegraphics[scale=.6]{second_round.rhosegm1.png}
\caption{Plot of the solution $\rho(\tau;\theta)$ and of $\frac{\rho(\tau;\theta)}{\theta^2}$ in the segment case for $\tau \in [1,2)$. Notice that the discontinuity for $\tau = \tau_1$ becomes here a discontinuity in the derivative in $1 + \tau_1$, and this is the reason why $\rho \sim \theta$ as $\theta \in [1+\tau_1,2)$. In the next step we will have $\rho \sim \theta^2$ in $[2 + \tau_1,3)$.}
\label{Fig:segm_round_2}
\end{figure}

{\it Step 2: the function $\frac{\rho(\tau,\theta)}{\theta^2}$ is strictly positive for $\tau \in [1,1+\tau_1)$ and increasing w.r.t. $\tau$.}

\noindent For $\tau = [1,1+\tau_1)$ it holds
\begin{align*}
\rho(\tau) &= D \Diracd_1 + S_0 \big( e^\tau - e^{\tau - 1} (\tau - 1) \big) + S_1 e^{\tau - \tau_1} + S_2 e^{\tau - 1}.
\end{align*}
Elementary computations show as before that since $\bar \alpha > \frac{\pi}{4}$
$$
D = \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{2\pi + \bar \alpha} \leq 0 \quad \Longleftrightarrow \quad \theta \in \{0\} \cup [2\bar \alpha,\pi],
$$
and in the interval $\theta \in [0,\pi]$ the only $0$ is for $\theta = 0$ which corresponds to $D = 0$.

When $1 < \tau < 1 + \tau_1$ the positivity of $\rho$ depends on
\begin{align*}
f(\theta) &= S_0 (e - \tau + 1) + S_1 e^{1 - \tau_1} + S_2,
\end{align*}
whose worst case is for $\tau = 1 + \tau_1$:
\begin{equation*}
f(\theta) = S_0 (e - \tau_1) + S_1 e^{1-\tau_1} + S_2.
\end{equation*}
Near $\bar \theta = \theta_0$ we have the expansion
\begin{equation}
\label{Equa:first_round_exp_segm}
\begin{split}
f(\theta) &= \bigg( \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (e-1) - \frac{1}{(2\pi + \bar \alpha) \sin(\bar \alpha)} - 2 \frac{\cot(\bar \alpha) \cos(\bar \alpha)}{2\pi + \bar \alpha} \bigg) \frac{(\bar \theta - \theta_0)^2}{2} + \mathcal O((\bar \theta - \theta_0)^3) \\
&\sim 0.582367 \frac{(\bar \theta - \theta_0)^2}{2} + \mathcal O((\bar \theta - \theta_0)^3),
\end{split}
\end{equation}
so that we consider the function
\begin{equation*}
f'(\theta) = \frac{\rho(\tau,\theta)}{\theta^2}, \quad 0 \leq \theta \leq \frac{\pi}{2}, 1 \leq \tau \leq 1 + \tau_1. 
\end{equation*}
A numerical plot shows that this function is increasing w.r.t. $\tau$ for all fixed $\theta$, and its minimal value is
\begin{equation*}
f'(1,\pi) = 0.17959.
\end{equation*}

\medskip

{\it Step 3: the function $\frac{\rho(\tau,\theta)}{\theta^2}$ is strictly positive and increasing for $\tau \in [1+\tau_1(\theta),2)$, and diverging near $\theta = 0$.}

\noindent For $\tau \in [1+\tau_1,2)$ the solution is
\begin{align*}
\rho(\tau) &= S_0 \big( e^\tau - e^{\tau - 1} (\tau - 1) \big) + S_1 \big( e^{\tau - \tau_1} - e^{\tau - 1 - \tau_1} (\tau - 1 - \tau_1) \big) + S_2 e^{\tau - 1}.
\end{align*}
Again numerically the function
\begin{equation*}
f(\tau,\theta) = \frac{\rho(\tau,\theta)}{\theta^2}
\end{equation*}
has a strictly positive derivative w.r.t. $\tau$, and it is strictly positive, with minimal value at 
$$
f(1+\tau_1,\pi) = 0.226635.
$$

We compute the expansion at $\theta = 0$ finding
\begin{align*}
\rho(\tau,\theta) &= \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} \bigg( \tau - 2 + \frac{\theta}{2\pi + \bar \alpha} \bigg),
\end{align*}
so that $g$ is diverging as $\frac{\sin(\bar \alpha) (1-\xi)}{(2\pi + \bar \alpha)^2 \theta}$ as $\theta \to 0$ and $\tau = 2 - \xi \frac{\theta}{2\pi + \bar \alpha}$.

\medskip

\begin{figure}
\includegraphics[scale=.6]{third_round.rhosegm_orig1.png}\hfill\includegraphics[scale=.6]{third_round.rhosegm1.png}
\caption{Plot of the function $\rho(\tau;\theta)$ (Equation (\ref{Equa:rhosegm_third})) on the left side and of $\frac{\rho(\tau;\theta)}{\theta^2}$ on the right side for $\tau \in [2,3)$.}
\label{Fig:thordround_rhosegm}
\end{figure}

{\it Step 4: for $\tau \in [2,3]$ the function $\rho(\tau,\theta)/\theta^2$ is bounded and strictly positive}

\noindent The solution in this interval is written as
\begin{equation}
\label{Equa:rhosegm_third}
\begin{split}
\rho(\tau,\theta) &= S_0 \bigg( e^\tau - e^{\tau - 1} (\tau-1) + e^{\tau-2} \frac{(\tau-2)^2}{2} \bigg) \\
& \quad + S_1 \bigg( e^{\tau - \tau_1} - e^{\tau - 1 - \tau_1} (\tau - 1 - \tau_1) + e^{\tau - 2 - \tau_1} \frac{(\tau - 2 - \tau_1)^2}{2} \ind_{\tau \geq 2 + \tau_1} \bigg) \\
&\quad + S_2 \big( e^{\tau-1} - e^{\tau-2} (\tau-2) \big) + S_3 e^{\tau-2}.
\end{split}
\end{equation}
Its expansion at $\theta = 0$ is quadratic in $\theta$, 
\begin{align*}
\rho(\tau,\theta) &= \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \bigg( e^\tau - e^{\tau - 1} (\tau-1) + e^{\tau-2} \frac{(\tau-2)^2}{2} \bigg) \\
& \quad - \frac{2 \cos(\bar \alpha)^2 + 1}{(2\pi + \bar \alpha) \sin(\bar \alpha)} \big( e^{\tau - 1} - e^{\tau - 2} (\tau - 2) \big) + \frac{3 \cos(\bar \alpha)}{(2\pi + \bar \alpha)^2} e^{\tau - 2} + \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} e^{\tau -3} \frac{(\frac{\tau - 3}{\theta} - \frac{1}{2\pi + \bar \alpha})^2}{2} \ind_{0 \geq \tau - 3 \geq - \frac{\theta}{2\pi + \bar \alpha}} \bigg) \bigg] \frac{\theta^2}{2} + o(\theta^2).
\end{align*}
We can thus study numerically the function
\begin{equation*}
f(\tau,\theta) = \frac{\rho(\tau,\theta)}{\theta^2},
\end{equation*}
which shows that the minimal/maximal value are
\begin{equation*}
f(2,\pi) = 0.262163.
\end{equation*}

\medskip

\begin{figure}
\includegraphics[scale=.6]{increasing.rhosegm1.png}\hfill\includegraphics[scale=.6]{asympt_segment1.png}
\caption{Plot of the function $\frac{\rho(\tau;\theta)}{\theta^2}$ (Equation (\ref{Equa:f_increas_segm})) on the left side and of the r.h.s. of Equation (\ref{Equa:asympt_segm}) for $\tau \geq 3$.}
\label{Fig:final_growth_rhosegm}
\end{figure}

{\it Step 5: the function $\frac{\rho(\tau,\theta)}{\theta^2}$ is strictly increasing for $\tau \geq 3$.}

\noindent It is enough to study the interval $\tau \in [3,4]$ for the function
\begin{equation}
\label{Equa:f_increas_segm}
f(\tau,\theta) = \frac{\rho(\tau,\theta)}{\theta^2}
\end{equation}
and apply Lemma \ref{lem:key}. The previous point, plus the fact that $g$ satisfies
\begin{equation*}
\dot g(\tau) = g(\tau) - g(\tau -1),
\end{equation*}
implies that it is bounded, so we do not need to study the expansion about $\theta = 0$.

The solution $\rho$ is written as
\begin{align*}
\rho(\tau,\theta) &= S_0 \bigg( e^\tau - e^{\tau - 1} (\tau-1) + e^{\tau-2} \frac{(\tau-2)^2}{2} - e^{\tau-3} \frac{(\tau-3)^3}{3!} \bigg) \\
& \quad + S_1 \bigg( e^{\tau - \tau_1} - e^{\tau - 1 - \tau_1} (\tau - 1 - \tau_1) + e^{\tau - 2 - \tau_1} \frac{(\tau - 2 - \tau_1)^2}{2} - e^{\tau - 3 - \tau_1} \frac{(\tau - 3 - \tau_1)^3}{3!} \ind_{\tau \geq 3 + \tau_1} \bigg) \\
&\quad + S_2 \bigg( e^{\tau-1} - e^{\tau-2} (\tau-2) + e^{\tau-3} \frac{(\tau-3)^2}{2} \bigg) + S_3 \big( e^{\tau-2} - e^{\tau-3} (\tau-3) \big).
\end{align*}
Numerical computations show that
\begin{equation*}
\frac{\partial_\tau \rho(\tau,\theta)}{\theta^2} \geq \frac{\partial_\tau \rho(3,\pi)}{\pi^2} = 0.142304,
\end{equation*}
and since the solution is continuous in the closed interval and positive at $\tau = 3$ from the previous point, we conclude that $\frac{\rho(\tau,\theta)}{\theta^2}$ is strictly increasing in $\tau$, see Fig. \ref{Fig:final_growth_rhosegm}.

\medskip

{\it Step 6: the asymptotic behavior.} By using Lemma \ref{Lem:aympt_g}, the solution behaves
\begin{equation}
\label{Equa:asympt_segm}
\lim_{\tau \to \infty} \frac{g(\tau,\theta)}{\tau \theta^2} = 2 \frac{S_0(\theta) + S_1(\theta) + S_2(\theta) + S_3(\theta)}{\theta^2},
\end{equation}
and numerical plots gives that the function is decreasing w.r.t. $\theta$ values with (Fig. \ref{Fig:final_growth_rhosegm})
\begin{equation}
0.0816077 \leq 2 \frac{S_0 + S_1 + S_2 + S_3}{\theta^2} \leq 0.278936. \qedhere
\end{equation}
\end{proof}

%\begin{figure}
%\includegraphics[scale=.7]{rhosegm_theta04.png}
%\caption{Plot of the evolution of the perturbation $\rho(\tau)$ for $\theta = 0.4$. Note that there is a first negative region for $\tau \in [1 - \frac{.4}{2\pi + \bar \alpha},1)$, and this oscillation perturbs the solution up to the third round, where it becomes strictly increasing.}
%\label{Fig:rhosegm_theta04}
%\end{figure}
%
%
%To have an idea of how the perturbation evolves in the segment case, we plot in Fig. \ref{Fig:rhosegm_theta04} the solution for $\theta = 0.4$.


\subsubsection{Estimate on the length for the {\color{red}perturbation of the} fastest saturated spiral $\delta r(\phi;s_0)$, segment case}
\label{Sss:additional_estim_opt_segm}


In this section we study the functional
\begin{equation}
\label{Equa:Lpert_segm}
\delta \tilde r(\phi;s_0) - 2.08 \delta \tilde L(\phi - 2\pi + \bar \alpha;s_0) \quad \text{when} \quad \phi \geq 2\pi + \bar \alpha,
\end{equation}
{\color{red} domanda: non e' $\phi-\phi_0$?}
where we denote by $\delta \tilde L$ the variation of length: more precisely, for angles larger than $\phi_0 + \bar \theta - \bar \alpha$ the spirals are saturated so that
\begin{equation*}
\delta \tilde L(\phi;s_0) = \frac{1 - \cos(\theta)}{\sin(\bar \alpha){\color{red}^2}} + \int_{\phi_0 + \bar \theta - \bar \alpha}^\phi \frac{\delta \tilde r(\phi';s_0)}{\sin(\bar \alpha)} d\phi'.
\end{equation*}
The first term is the due to the computation
\begin{equation*}
1 + \delta |P_2 - P_1| - \frac{r_2}{\sin(\bar \alpha)} \delta \bar \theta = \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2}
\end{equation*}
by \eqref{Equa:delta_P_2P_1_segm}, {\color{red}obtained by computing the differences of length of $\tilde r(\phi;s_0+\delta s_0)-\tilde r(\phi;s_0)$ before the spirals become saturated.}

Using the explicit expression of $\delta \tilde r$ of Corollary \ref{Cor:evolv_r_after_phi_2}, the length $\delta \tilde L$ can be written as
\begin{equation*}
%\label{Equa:evolv_L_after_phi_2}
\begin{split}
\delta \tilde L(\phi;s_0) &= \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} + \cot(\bar \alpha) \frac{1 - \cos(\theta)}{\sin(\bar \alpha)} \mathcal G(\phi - \phi_0 - \bar \theta + \bar \alpha) - \mathcal G(\phi - \phi_0 - 2\pi - \theta_0) \\
&\quad + \bigg( 1 - \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} + \cot(\bar \alpha) \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} \bigg) \mathcal G(\phi - 2\pi - \phi_0 - \bar \theta) \\
& \quad + \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} H(\phi - 2\pi - \phi_0 - \bar \theta) - \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)^2} \mathcal G(\phi - 4\pi - \phi_0 - \bar \theta - \bar \alpha),
\end{split}
\end{equation*}
where we have used the definition of \gls{Gcal}. The equation it satisfies is
\begin{align*}
\frac{d}{dt{\color{red}\phi}} \delta \tilde L(\phi{\color{red};s_0}) &= \cot(\bar \alpha) \delta \tilde L(\phi{\color{red};s_0}) - \frac{\delta \tilde L(\phi - 2\pi - \bar \alpha{\color{red};s_0})}{\sin(\bar \alpha)} + \cot(\bar \alpha) \frac{1 - \cos(\theta)}{\sin(\bar \alpha)} H(\phi - \phi_0 - \bar \theta + \bar \alpha) - H(\phi - \phi_0 - 2\pi - \theta_0) \\
&\quad + \bigg( 1 - \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} + \cot(\bar \alpha) \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} \bigg) H(\phi - 2\pi - \phi_0 - \bar \theta) \\
& \quad + \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} \Diracd{\color{red}H?x}(\phi - 2\pi - \phi_0 - \bar \theta) - \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)^2} H(\phi - 4\pi - \phi_0 - \bar \theta - \bar \alpha),
\end{align*}
which becomes for $\phi \geq \phi_0 + \bar \theta + 4\pi + \bar \alpha$
\begin{equation*}
\frac{d}{dt} \delta \tilde L(\phi) = \cot(\bar \alpha) \delta \tilde L(\phi) - \frac{\delta \tilde L(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} + S_L,
\end{equation*}
\begin{align*}
S_L &= \frac{1}{\sin(\bar \alpha)} {\color{red}\text{questo termine non ci vuole}}\bigg[ \cot(\bar \alpha) \frac{1 - \cos(\theta)}{\sin(\bar \alpha)} - 1 + \bigg( 1 - \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} + \cot(\bar \alpha) \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} \bigg) - \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)^2} \bigg] \\
&= - \frac{1 - \cos(\bar \alpha)}{\sin(\bar \alpha)^3} \big( (1 - \cos(\bar \alpha)) (1 - \cos(\theta) + \sin(\bar \alpha) \sin(\theta) \big) < 0.
\end{align*}
In particular we have for the same range of angles
\begin{align*}
\frac{d}{d\phi} \big( \delta \tilde r(\phi) - 2.08 \delta \tilde L(\phi) \big) &= \cot(\bar \alpha) \big( \delta \tilde r(\phi) - 2.08 \delta \tilde L(\phi) \big) - \frac{\delta \tilde r(\phi - 2\pi - \bar \alpha ) - 2.08 \delta \tilde L(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} - S_L \\
&\geq \cot(\bar \alpha) \big( \delta \tilde r(\phi) - 2.08 \delta \tilde L(\phi) \big) - \frac{\delta \tilde r(\phi - 2\pi - \bar \alpha ) - 2.08 \delta \tilde L(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)}.
\end{align*}

\begin{figure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\includegraphics{Lpert_segm1.png}}
\end{subfigure} \hfill
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\includegraphics{Lsegm_pert3.png}}
\end{subfigure} \hfill
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\includegraphics{Lpert_segm2.png}}
\end{subfigure}
\caption{Numerical plot of the function \eqref{Equa:Lpert_segm} rescaled by $e^{-\bar c \phi}$ and using the variable $\tau$ and divided by $\theta^2$: the first 4 rounds, the derivative for the round $\tau \in [4,5]$ and the minimal value.}
\label{Fig:Lpert_segm}
\end{figure}

In Fig. \ref{Fig:Lpert_segm} the numerical plot of the function \eqref{Equa:Lpert_segm} shows that it is positive, increasing after $\tau = 4$ and thus by Lemma \ref{lem:key} and Remark \ref{rmk:exponentially:explod} {\color{red} qual e' questo remark?} it holds

\begin{proposition}
\label{Prop:lemgth_segm_pert}
It holds for the perturbation in the segment case
\begin{equation*}
\rho(\tau) - 2.08 e^{- \bar c(2\pi + \bar \alpha) \tau} \delta \tilde L(\tau) \geq 0.117 \theta, \quad \tau \geq 1. %\phi \geq \phi_0 + \bar \theta + 2\pi.
\end{equation*}
\end{proposition}
{\color{red} E' $\rho$ o $\delta\rho$?}
{\color{red}Magari un commento per cosa useremo questo risultato?}
%{\color{blue} DA RIMUOVERE
%
%In this section we give some estimate needed to proved the structure of the optimal solution constructed in the next section.
%
%First, we write the variation of length of the perturbation of a spiral: since for $\phi \geq \phi_0 + \bar \theta - \bar \alpha$ the spiral $\tilde r$ is saturated, then the radius of curvature is
%\begin{equation*}
%R(\phi') = \frac{\tilde r(\phi)}{\sin(\bar \alpha)},
%\end{equation*}
%because we are in the saturated part of $\tilde r$, and thus the same formula holds for the perturbation $\delta \tilde r$: if we denote %\newglossaryentry{Gcal}{name=\ensuremath{\mathcal G(\phi)},description={primitive of the kernel G}} \newglossaryentry{Heavyside}{name=\ensuremath{H(\phi)},description={Heavyside function}}
%\begin{equation*}
%\gls{Gcal} = \int_{\infty}^\phi \frac{G(\phi')}{\sin(\bar \alpha)} d\phi' = \int_0^{\tau} g(\tau') e^{\bar c(2\pi + \bar \alpha) (\tau' + 1)} d\tau', \quad \phi = (2\pi + \bar \alpha) \tau,
%\end{equation*}
%\begin{equation*}
%\frac{d}{dt} \mathcal G(\phi) = \cot(\bar \alpha) \mathcal G(\phi) - \frac{\mathcal G(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} + \frac{H(\phi)}{\sin(\bar \alpha)},
%\end{equation*}
%where \gls{Heavyside} is the Heavyside function
%\begin{equation*}
%H(\phi) = \begin{cases}
%0 & x < 0, \\
%1 & x \geq 0,
%\end{cases}
%\end{equation*}
%then by \eqref{Equa:evolv_r_after_phi_2} we obtain the formula for the variation $\delta L(\phi)$ of $L(\phi)$ for $\phi \geq \phi_0 + \bar \theta - \theta$
%\begin{equation}
%\label{Equa:delta_L}
%\begin{split}
%\delta L(\phi) &= \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} + \cot(\bar \alpha) \frac{1 - \cos(\theta)}{\sin(\bar \alpha)} \big( \mathcal G(\phi + \hat \theta - \phi_0 - \bar \theta - 2\pi) - \mathcal G(\phi - \phi_0 - \bar \theta - 2\pi) \big) \\
%& \quad - \big( \mathcal G(\phi + \hat \theta - \phi_0 - \bar \theta + \theta - 4\pi - \bar \alpha) - \mathcal G(\phi - \phi_0 - \bar \theta + \theta - 4\pi - \bar \alpha) \big) \\
%& \quad + \bigg( 1 - \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} + \cot(\bar \alpha) \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} \bigg) \big( \mathcal G(\phi + \hat \theta - \phi_0 - \bar \theta - 4\pi - \bar \alpha) - \mathcal G(\phi - \phi_0 - \bar \theta - 4\pi - \bar \alpha) \big) \\
%& \quad + \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)^2} \chi_{[\phi_0 + \bar \theta + 4\pi + \bar \alpha - \hat \theta,\phi_0 + \bar \theta + 4\pi + \bar \alpha)}(\phi) \\
%& \quad - \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)^2} \big( \mathcal G(\phi + \hat \theta - \phi_0 - \bar \theta - 6\pi - 2 \bar \alpha) -  \mathcal G(\phi - \phi_0 - \bar \theta - 6\pi - 2 \bar \alpha) \big).
%\end{split}
%\end{equation}
%The first term $\frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2}$ comes from the perturbation to the initial segment $[P_1,P_2]$ and that the initial angle $\phi_2$ moves of $\delta \theta$, which gives
%\begin{equation*}
%\delta s_0 + \delta |P_2 - P_1| - \frac{\tilde r(\phi_2)}{\sin(\bar \alpha)} \delta \theta = \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2}.
%\end{equation*}
%This can be easily explained also by computing the variation of length for small angles:
%\begin{align*}
%\delta s_0 + \delta |P-2 - P_1| + \delta \bigg( \int_{\phi_2}^\phi \frac{\tilde r(\phi';s_0)}{\sin(\bar \alpha)} d\phi' \bigg) = \delta s_0 + \delta |P_2 - P_1| - \frac{\tilde r(\phi_2)}{\sin(\bar \alpha} \delta \phi_2 + \int_{\phi_2}^\phi \frac{\delta \tilde r(\phi';s_0)}{\sin(\bar \alpha)} d\phi'.
%\end{align*}
%
%In terms of the solution $\rho$ (Equation \eqref{Equa:rho_segm_r}), the above formula becomes
%\begin{align*}
%\delta L(\phi) &= \frac{1-\cos(\theta)}{\sin(\bar \alpha)^2} + \int_0^{\phi} \frac{\rho(\frac{\phi'}{2\pi + \bar \alpha})}{\sin(\bar \alpha)} e^{\bar c \phi'} d\phi' \\
%&= \frac{1-\cos(\theta)}{\sin(\bar \alpha)^2} + \int_0^{\tau} \frac{2\pi + \bar \alpha}{\sin(\bar \alpha)} \rho(\tau') e^{\bar c (2\pi + \bar \alpha) \tau'} d\tau' \\
%&= \frac{1-\cos(\theta)}{\sin(\bar \alpha)^2} + \int_0^{\tau} \rho(\tau') e^{\bar c (2\pi + \bar \alpha) (\tau' + 1)} d\tau',
%\end{align*}
%where we have used $\frac{2\pi + \bar \alpha}{\sin(\bar \alpha)} = e^{\bar c (2\pi + \bar \alpha)}$ by \eqref{Equa:c_gene_defi},\eqref{eq:for:c}.
%
%Define the functional\newglossaryentry{ATphi}{name=\ensuremath{AT(\phi)},description={functional to check the admissibility of the tent, also written depending on $\tau$}}
%\begin{align*}
%\gls{ATphi} &= \frac{\sin(\bar \alpha) (\sin(\bar \alpha + \hat \theta) - \sin(\bar \alpha))}{\cos(\hat \theta)(1 - \sin(\bar \alpha))} \delta \tilde r(\phi;s_0) - \big( \delta L(\phi-\pi) - \delta L(\phi^-) \big),
%\end{align*}
%where $\phi^-$ is the angle such that
%\begin{equation*}
%\phi \in \phi^- + 2\pi + [\beta^-(\phi^-),\beta^+(\phi^-)].
%\end{equation*}
%We compute the quantity
%\begin{equation}
%\label{Equa:variation_lenght_base}
%\delta L(\phi-\pi) - \delta L(\phi^-) = \begin{cases}
%0 & \phi < \phi_0 + \pi, \\
%1 & \phi_0 + \pi \leq \phi < \phi + \bar \theta - \bar \alpha + \pi, \\
%\delta L(\phi-\pi) & \phi_0 + \bar \theta - \bar \alpha + \pi \leq \phi < \phi_0 + \bar \theta + 2\pi - \theta, \\
%\delta L(\phi-\pi) - 1 & \phi_0 + \bar \theta + 2\pi - \theta \leq \phi < \phi_0 + \bar \theta + 2\pi, \\
%\delta L(\phi-\pi) - \delta L(\phi - 2\pi - \bar \alpha) & \phi_0 + \bar \theta + 2\pi < \phi.
%\end{cases}
%\end{equation}
%
%Written in terms of $\rho(\tau)$ we obtain \newglossaryentry{Lfrak}{name=\ensuremath{\delta \mathfrak L(\tau)},description={variation of the length for the functional \gls{ATphi}}}
%\begin{equation}
%\label{Equa:AT_tau}
%e^{\bar c (2\pi + \bar \alpha) \tau} AT(\tau) = \frac{\sin(\bar \alpha) (\sin(\bar \alpha + \hat \theta) - \sin(\bar \alpha))}{\cos(\hat \theta)(1 - \sin(\bar \alpha))} \rho(\tau) - e^{- \bar c (2\pi + \bar \alpha) \tau} \gls{Lfrak},
%\end{equation}
%with \gls{Lfrak} given by \eqref{Equa:variation_lenght_base}.
%
%\begin{proposition}
%\label{Prop:function_AT}
%The functional $AT(\tau)$ is positive for $\tau \geq \frac{\pi}{2\pi+\bar \alpha}$.
%\end{proposition}
%
%\begin{proof}
%
%\end{proof}
%
%
%
%
%\newglossaryentry{tauhat}{name=\ensuremath{\hat \tau},description={interval equal to $\frac{\hat \theta}{2\pi + \bar \alpha}$}}
%\begin{equation*}
%\gls{tauhat} = \frac{\hat \theta}{2\pi + \bar \alpha}.
%\end{equation*}
%Hence, defining %\newglossaryentry{gfrak}{name=\ensuremath{\mathfrak g(\tau)},description={primitive of the function $g(\tau) e^{\bar c (2\pi + \bar \alpha)(\tau+1)}$}}
%\begin{equation*}
%\gls{gfrak} = \int_{-\infty}^\tau g(\tau') e^{\bar c (2\pi + \bar \alpha)(\tau'+1)} d\tau',
%\end{equation*}
%we have for $\tau > 1$ from Corollary \ref{Cor:equation}
%\begin{align*}
%\delta L(\tau) &= S_0 \big( \mathfrak g(\tau + \hat \tau - 1) - \mathfrak g(\tau - 1) \big) + S_1 e^{\bar c(2\pi + \bar \alpha) \tau_1} \big( \mathfrak g(\tau + \hat \tau - 1 - \tau_1) - \mathfrak g(\tau - 1 - \tau_1) \big) \\
%& \quad + S_2 e^{\bar c(2\pi + \bar \alpha)} \big( \mathfrak g(\tau + \hat \tau - 2) - \mathfrak g(\tau - 2) \big) + \frac{D e^{\bar c (2\pi + \bar \alpha)}}{\sin(\bar \alpha)} \ind_{[2-\hat \tau,2)}(\tau) \\
%&\quad + S_3 e^{2\bar c(2\pi + \bar \alpha)} \big( \mathfrak g(\tau + \hat \tau - 3) - \mathfrak g(\tau - 3) \big),
%\end{align*}
%where the coefficients $D,S_i$, $i = 0,\dots,3$ are given by \eqref{Equa:source_segmnt_pert}.
%
%
%
%
%For a given angle $\phi \geq \phi_0 + \bar \theta - \bar \alpha$, we consider the following quantities (see Fig. \ref{Fig:additional_etim_segm}):
%\begin{itemize}
%\item the length $\tilde r(\phi;s_0)$,
%\item the length $\tilde r(\phi + 2\pi + \bar \alpha;s_0)$,
%\item the length $L(\phi)$ of the spiral
%$$
%s^-(\phi + \hat \theta) - s^-(\phi),
%$$
%where we recall that \gls{s-phi}, \gls{s+phi} are the length of the spiral up to the initial/end point of the ray $\tilde r(\phi)$, see Theorem \ref{Cor:angle_preprest}.
%\end{itemize}
%
%\begin{figure}
%\resizebox{.75\textwidth}{!}{\input{computation_tent_segm.pdf_t}}
%\caption{The geometry for the computations of Section \ref{Sss:additional_estim_opt_segm}.}
%\label{Fig:additional_etim_segm}
%\end{figure}
%
%If we use the $(\phi,\tilde r(\phi;s_0))$ coordinates, we can write
%\begin{equation*}
%L(\phi) = \int_{\phi^-}^{\phi^+} R(\phi) d\phi, \quad s^-(\phi) = s^+(\phi^-), \ s^-(\phi + \hat \theta) = s^+(\phi^+).
%\end{equation*}
%Being the angle fixed and the formula linear, then same formula is valid for the perturbation $\delta \tilde r(\phi;s_0)$. The functions \newglossaryentry{phi-phi}{name=\ensuremath{\phi^-(\phi)},description={starting angle for the base of the tent}}   \newglossaryentry{phi+phi}{name=\ensuremath{\phi^+(\phi)},description={ending angle for the base of the tent}} \gls{phi-phi}, \gls{phi+phi} can be computed explicitly in the region of interest $\phi > \phi_0 + 2\pi + \beta^-(\phi_0)$:
%\begin{equation*}
%\gls{phi-phi} = \begin{cases}
%\phi_0 & \phi \in [\phi_0 + 2\pi + \beta^-(\phi_0),\phi_0 + \bar \theta + 2\pi), \\
%\phi - 2\pi - \bar \alpha & \phi \geq \phi_0 + \bar \theta + 2\pi,
%\end{cases}
%\end{equation*}
%\begin{equation*}
%\gls{phi+phi} = \begin{cases}
%\phi_0 & \phi \in [\phi_0 + 2\pi + \beta^-(\phi_0),\phi_0 + \bar \theta - \hat \theta + 2\pi), \bar \theta > \hat \theta, \\
%\phi - 2\pi - \bar \alpha + \hat \theta & \phi \geq \phi_0 + \bar \theta - \hat \theta + 2\pi.
%\end{cases}
%\end{equation*}
%
%We will apply the above formulas for $\phi > \phi_0 + \bar \theta + 2\pi$, where
%\begin{equation*}
%\phi^-(\phi) = \phi - 2\pi - \bar \alpha, \quad \phi^+(\phi) = \phi - 2\pi - \bar \alpha + \hat \theta.
%\end{equation*}
%Moreover in this region it holds
%\begin{equation*}
%R(\phi') = \frac{r(\phi)}{\sin(\bar \alpha)},
%\end{equation*}
%because we are in the saturated part of $\tilde r$, and thus the same formula holds for the perturbation $\delta \tilde r$: if we denote %\newglossaryentry{Gcal}{name=\ensuremath{\mathcal G(\phi)},description={primitive of the kernel G}} \newglossaryentry{Heavyside}{name=\ensuremath{H(\phi)},description={Heavyside function}}
%\begin{equation*}
%\gls{Gcal} = \int_{\infty}^\phi \frac{G(\phi')}{\sin(\bar \alpha)} d\phi' = \int_0^{\tau} g(\tau') e^{\bar c(2\pi + \bar \alpha) (\tau' + 1)} d\tau', \quad \phi = (2\pi + \bar \alpha) \tau,
%\end{equation*}
%\begin{equation*}
%\frac{d}{dt} \mathcal G(\phi) = \cot(\bar \alpha) \mathcal G(\phi) - \frac{\mathcal G(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} + \frac{H(\phi)}{\sin(\bar \alpha)},
%\end{equation*}
%where \gls{Heavyside} is the Heavyside function
%\begin{equation*}
%H(\phi) = \begin{cases}
%0 & x < 0, \\
%1 & x \geq 0,
%\end{cases}
%\end{equation*}
%then by \eqref{Equa:evolv_r_after_phi_2} we obtain the formula for the variation $\delta L(\phi)$ of $L(\phi)$ for $\phi \geq \phi_0 + \bar \theta - \theta$
%\begin{equation}
%\label{Equa:delta_L}
%\begin{split}
%\delta L(\phi) &= \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} + \cot(\bar \alpha) \frac{1 - \cos(\theta)}{\sin(\bar \alpha)} \big( \mathcal G(\phi + \hat \theta - \phi_0 - \bar \theta - 2\pi) - \mathcal G(\phi - \phi_0 - \bar \theta - 2\pi) \big) \\
%& \quad - \big( \mathcal G(\phi + \hat \theta - \phi_0 - \bar \theta + \theta - 4\pi - \bar \alpha) - \mathcal G(\phi - \phi_0 - \bar \theta + \theta - 4\pi - \bar \alpha) \big) \\
%& \quad + \bigg( 1 - \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} + \cot(\bar \alpha) \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} \bigg) \big( \mathcal G(\phi + \hat \theta - \phi_0 - \bar \theta - 4\pi - \bar \alpha) - \mathcal G(\phi - \phi_0 - \bar \theta - 4\pi - \bar \alpha) \big) \\
%& \quad + \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)^2} \chi_{[\phi_0 + \bar \theta + 4\pi + \bar \alpha - \hat \theta,\phi_0 + \bar \theta + 4\pi + \bar \alpha)}(\phi) \\
%& \quad - \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)^2} \big( \mathcal G(\phi + \hat \theta - \phi_0 - \bar \theta - 6\pi - 2 \bar \alpha) -  \mathcal G(\phi - \phi_0 - \bar \theta - 6\pi - 2 \bar \alpha) \big).
%\end{split}
%\end{equation}
%The first term $\frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2}$ comes from the perturbation to the initial segment $[P_1,P_2]$ and that the initial angle $\phi_0 + \bar \theta - \theta$ moves of $\delta \theta$, which gives
%\begin{equation*}
%\delta s_0 + \delta |P_2 - P_1| - \frac{\tilde r(\phi_2)}{\sin(\bar \alpha)} \delta \theta = \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2}.
%\end{equation*}
%
%
%In terms of the solution $\rho$ (Equation \eqref{Equa:rho_segm_r}), the above formula becomes
%\begin{align*}
%\delta L(\phi) &= \frac{1-\cos(\theta)}{\sin(\bar \alpha)^2} + \int_0^{\phi} \frac{\rho(\frac{\phi'}{2\pi + \bar \alpha})}{\sin(\bar \alpha)} e^{\bar c \phi'} d\phi' \\
%&= \frac{1-\cos(\theta)}{\sin(\bar \alpha)^2} + \int_0^{\tau} \frac{2\pi + \bar \alpha}{\sin(\bar \alpha)} \rho(\tau') e^{\bar c (2\pi + \bar \alpha) \tau'} d\tau' \\
%&= \frac{1-\cos(\theta)}{\sin(\bar \alpha)^2} + \int_0^{\tau} \rho(\tau') e^{\bar c (2\pi + \bar \alpha) (\tau' + 1)} d\tau',
%\end{align*}
%where we have used $\frac{2\pi + \bar \alpha}{\sin(\bar \alpha)} = e^{\bar c (2\pi + \bar \alpha)}$ by \eqref{Equa:c_gene_defi},\eqref{eq:for:c} and \newglossaryentry{tauhat}{name=\ensuremath{\hat \tau},description={interval equal to $\frac{\hat \theta}{2\pi + \bar \alpha}$}}
%\begin{equation*}
%\gls{tauhat} = \frac{\hat \theta}{2\pi + \bar \alpha}.
%\end{equation*}
%Hence, defining %\newglossaryentry{gfrak}{name=\ensuremath{\mathfrak g(\tau)},description={primitive of the function $g(\tau) e^{\bar c (2\pi + \bar \alpha)(\tau+1)}$}}
%\begin{equation*}
%\gls{gfrak} = \int_{-\infty}^\tau g(\tau') e^{\bar c (2\pi + \bar \alpha)(\tau'+1)} d\tau',
%\end{equation*}
%we have for $\tau > 1$ from Corollary \ref{Cor:equation}
%\begin{align*}
%\delta L(\tau) &= S_0 \big( \mathfrak g(\tau + \hat \tau - 1) - \mathfrak g(\tau - 1) \big) + S_1 e^{\bar c(2\pi + \bar \alpha) \tau_1} \big( \mathfrak g(\tau + \hat \tau - 1 - \tau_1) - \mathfrak g(\tau - 1 - \tau_1) \big) \\
%& \quad + S_2 e^{\bar c(2\pi + \bar \alpha)} \big( \mathfrak g(\tau + \hat \tau - 2) - \mathfrak g(\tau - 2) \big) + \frac{D e^{\bar c (2\pi + \bar \alpha)}}{\sin(\bar \alpha)} \ind_{[2-\hat \tau,2)}(\tau) \\
%&\quad + S_3 e^{2\bar c(2\pi + \bar \alpha)} \big( \mathfrak g(\tau + \hat \tau - 3) - \mathfrak g(\tau - 3) \big),
%\end{align*}
%where the coefficients $D,S_i$, $i = 0,\dots,3$ are given by \eqref{Equa:source_segmnt_pert}.
%}
%
%The two quantities we are interested are \newglossaryentry{PTphi}{name=\ensuremath{PT(\phi)},description={functional to check the positivity of $\delta \hat r$, also written depending on $\tau$}}
%\begin{align*}
%\gls{ATphi} &= \delta \tilde r(\phi;s_0) - \frac{\cos(\hat \theta)(1 - \sin(\bar \alpha))}{\sin(\bar \alpha) (\sin(\bar \alpha + \hat \theta) - \sin(\bar \alpha))} \delta L(\phi), \\
%\gls{PTphi} &= \delta \tilde r(\phi) - \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \delta \tilde r(\phi - 2\pi - \bar \alpha).
%\end{align*}
%Written in terms of $\rho(\tau)$ we obtain
%\begin{equation}
%\label{Equa:AT_tau}
%AT(\tau) = e^{\bar c (2\pi + \bar \alpha) \tau} \bigg( \rho(\tau) - \frac{\cos(\hat \theta)(1 - \sin(\bar \alpha))}{\sin(\bar \alpha) (\sin(\bar \alpha + \hat \theta) - \sin(\bar \alpha))} e^{- \bar c (2\pi + \bar \alpha) \tau} \delta L(\tau) \bigg),
%\end{equation}
%\begin{equation}
%\label{Equa:PT_tau}
%PT(\tau) = e^{\bar c(2\pi + \bar \alpha) \tau} \bigg( \rho(\tau) - \frac{(1 - \cos(\hat \theta)) e^{-\bar c(2\pi + \bar \alpha)}}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \rho(\tau - 1) \bigg).
%\end{equation}
%
%\begin{proposition}
%\label{Prop:estima_radii_segm}
%The functional $AT(\tau)$ is positive for $\tau \geq 1, \theta \in [0,\frac{\pi}{2}]$.
%\end{proposition}
%
%\begin{figure}
%\begin{subfigure}{.475\linewidth}
%\resizebox{\linewidth}{!}{\includegraphics{AT_first_5.1.png}}
%\end{subfigure} \hfill
%\begin{subfigure}{.475\linewidth}
%\resizebox{\linewidth}{!}{\includegraphics{AT_first_5.2.png}}
%\end{subfigure}
%\caption{The first 3 rounds of the function $AT(\tau) e^{-\bar c(2\pi + \bar \alpha) \tau}$, $\tau \geq 1$ (Equation (\ref{Equa:AT_tau}), depending on the parameter $\theta \in (0,\pi]$. Outside the first round, where $AT(\tau) = \delta \tilde r(\tau)$, the functional is positive.}
%\label{Fig:AT_5}
%\end{figure}
%
%\begin{figure}
%\begin{subfigure}{.475\linewidth}
%\resizebox{\linewidth}{!}{\includegraphics{AT_first_56_2.1.png}}
%\end{subfigure} \hfill
%\begin{subfigure}{.475\linewidth}
%\resizebox{\linewidth}{!}{\includegraphics{AT_first_56_1.1.png}}
%\end{subfigure}
%\caption{The fifth rounds of the function \eqref{Equa:simpli_AT} divided by $\theta^2$.}
%\label{Fig:AT_56_2}
%\end{figure}
%
%\begin{proof}
%For the first 4 rounds, we numerically compute the function
%\begin{equation*}
%\frac{AT(\tau) e^{-\bar c (2\pi + \bar \alpha) \tau}}{\theta^2}, \quad \tau \in [0,4], \ \theta \in (0,\pi].
%\end{equation*}
%One then verifies that for $\tau \geq 1$ this is positive, with minimal value 0.1725 in $(\tau,\theta) = (1,\pi)$.
%
%When the function $\delta \tilde r$ is increasing, one can estimate
%\begin{equation*}
%\delta L(\phi) \leq \frac{\hat \theta}{\sin(\bar \alpha)} \delta \tilde r(\phi - 1 + \hat \theta),
%\end{equation*}
%so that it is enough to study the function
%\begin{equation}
%\label{Equa:simpli_AT}
%\begin{split}
%\delta \tilde r(\phi) - \frac{\hat \theta}{\sin(\bar \alpha)} \delta \tilde r(\phi - 1 + \hat \theta) &= e^{\bar c (2\pi + \bar \alpha) \tau} \bigg( \rho(\tau) - \frac{e^{- \bar c (2\pi + \bar \alpha) (1 - \hat \tau)} \hat \theta}{\sin(\bar \alpha)} \rho(\tau - \hat \tau) \bigg) \\
%&= e^{\bar c (2\pi + \bar \alpha) \tau} \big( \rho(\tau) - \hat \tau e^{-\bar c (2\pi + \bar \alpha) \hat \tau} \rho(\tau - 1 + \hat \tau) \big).
%\end{split}
%\end{equation}
%In Fig. \ref{Fig:AT_56_2} it is numerically verified that the previous function is increasing, so that by Lemma \ref{lem:key} we deduce the positive afterwards.
%\end{proof}
%
%\begin{proposition}
%\label{Prop:PT_tau_pos}
%The functional $PT(\tau)$ is positive for $\tau \geq 1$ and $\theta \in (0,\frac{\pi}{2}]$.
%\end{proposition}
%
%\begin{figure}
%\begin{subfigure}{.475\linewidth}
%\resizebox{\linewidth}{!}{\includegraphics{PT_first_5.1.png}}
%\end{subfigure} \hfill
%\begin{subfigure}{.475\linewidth}
%\resizebox{\linewidth}{!}{\includegraphics{PT_first_5.2.png}}
%\end{subfigure}
%\caption{The function $PT(\tau)$ for $\theta = .05$ (blu) to $\theta = \frac{\pi}{2}$ (brown) with .3 steps: it is positive and strictly increasing for $\tau \geq 3$.}
%\label{Fig:PT_first_5}
%\end{figure}
%
%\begin{proof}
%A numerical plot of the function $PT(\tau)$ is in Fig. \ref{Fig:PT_first_5}: it is positive (with minimal value $> .1$ in $(\tau,\theta) \to (1,0)$) for $\tau \geq 1$ and increasing for $\tau \geq 3$, so that we conclude by Lemma \ref{lem:key}.
%\end{proof}
%
%{\bf \color{red} Questa parte devo ancora rivederla!
%
%We repeat the analysis for the functional
%\begin{equation}
%\label{Equa:r2_segment_adm}
%AT2(\tau) := 6 \delta \tilde r(\phi) - \delta L(\phi - 2\pi - \bar \alpha,\phi)
%\end{equation}
%after the first round of the perturbation, i.e. $\phi \geq \phi_0 + \bar \theta + 2\pi$ or equivalently $\tau \geq 1$. As usual, we will write the dependence w.r.t. $\phi$ or $\tau$ indifferently.
%
%\begin{lemma}
%\label{Lem:AT2_pos}
%The functional $AT2(\tau)$ is positive and increasing for $\tau \geq 1$.
%\end{lemma}
%
%\begin{figure}
%\begin{subfigure}{.475\textwidth}
%\resizebox{\textwidth}{!}{\includegraphics{r2_tent_segment_1.1.png}}
%\end{subfigure} \hfill
%\begin{subfigure}{.475\textwidth}
%\resizebox{\textwidth}{!}{\includegraphics{r2_tent_segment_2.1.png}}
%%\caption{Plot of the function \eqref{Equa:r2_segment_adm}.}
%%\label{Fig:r2_segment_adm_2}
%\end{subfigure}
%\caption{Plot of the function \eqref{Equa:r2_segment_adm}.}
%\label{Fig:r2_segment_adm_1}
%\end{figure}
%
%\begin{proof}
%If Fig. \ref{Fig:r2_segment_adm_1} the first 4 rounds of the function $\frac{AT2}{\theta^2}$ are plotted: numerically one verifies that it is positive and increasing for $\tau \in [3,4]$, with minimal value $> .5$, so that we can apply Lemma \ref{lem:key}.
%\end{proof}
%
%Finally we conclude this section with the same analysis of the function %In this section we study the function
%\begin{equation*}
%\mathcal A(\phi) = \delta \tilde r(\phi) - \frac{1}{10} (\delta L(\phi - \pi) - \delta L(\phi - 7\pi/2)).
%\end{equation*}
%%for $\tau \geq 1 - \frac{\frac{\pi}{2} -\bar \alpha}{2\pi + \bar \alpha}$.
%
%\begin{lemma}
%\label{Lem:calA_pos}
%The function $\mathcal A(\phi)$ is strictly positive and increasing for $\tau \geq 1 - \frac{\frac{\pi}{2} -\bar \alpha}{2\pi + \bar \alpha}$.
%\end{lemma}
%
%We perform the computation in the $\tau$ coordinate, then we will convert it in the $\phi$ angle.
%
%For $\tau \in [1,1 + \hat \tau]$, the length is controlled as:
%\begin{enumerate}
%\item for $\tau \leq \tau_1$ then
%\begin{align*}
%\delta L &\leq 1 + \delta P - \frac{r_2 \delta \bar \theta}{\sin(\bar \alpha)} + \int_0^{\pi} \frac{\delta r}{\sin(\bar \alpha)} d\phi \\
%&= \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} e^{\cot(\bar \alpha) \pi},
%\end{align*}
%This function is positive. This solves also the case for $\theta < \hat \theta$.
%
%\item for $\tau > 3/2$ we use the functional
%\begin{equation*}
%\rho(\tau) - (L(\tau-1) - L(\tau-3/2)),
%\end{equation*}
%which is again positive and increasing. Hence we know it is a tent for $\tau \geq 1$.
%\end{enumerate}
%
%
%For the other part, we use instead the comparison of $\hat \rho_0$ and $\hat L$. {\bf The problem is as always the negative part}
%
%\begin{enumerate}
%\item 
%\end{enumerate}
%
%The length of the perturbation is explicitly computed by
%\begin{align*}
%\delta L(\tau) %&= \delta L(\phi_0 + \bar \theta + (2\pi + \bar \alpha) \tau) \\
%%&= \int_{\tau - 1}^{\tau + \hat \tau - 1} \rho(\tau') e^{\bar c (2\pi + \bar \alpha) (\tau' + 1) - 1} d\tau' \\
%&= S_0 \mathfrak g(\tau) + S_1 e^{\bar c(2\pi + \bar \alpha) \tau_1} \mathfrak g(\tau - \tau_1) \\
%& \quad + S_2 e^{\bar c(2\pi + \bar \alpha)} \mathfrak g(\tau - 1) + \frac{D e^{\bar c (2\pi + \bar \alpha)}}{\sin(\bar \alpha)} H(\tau-1) \\
%&\quad + S_3 e^{2\bar c(2\pi + \bar \alpha)} \mathfrak g(\tau - 2),
%\end{align*}
%
%
%
%}


\subsection{Analysis of Perturbations - Arc Case}
\label{S:arc}


In this section we repeat the computations in the case that the fastest saturated solution for $\phi \in \phi_0 + [0,2\pi + \beta^-(\phi_0))$ has the following structure:
\begin{itemize}
\item it is an arc of the level set $\lbrace u=u(\zeta(s_0)\rbrace$, starting in $P_0 = \zeta(\phi_0)$ and ending in \newglossaryentry{Deltaphi}{name=\ensuremath{\Delta \phi},description={opening angle for the arc on the level set}} $P_1 = \zeta(\phi_1) = \zeta(\phi_0 + \gls{Deltaphi})$;
\item a segment $[P_1,P_2]$ tangent to the level set $\lbrace u=u(\zeta(s_0)\rbrace$ in $P_1$ and such that $P_2 = \zeta(\phi_2) = \zeta(\phi_1 + \frac{\pi}{2} -\bar \alpha)$ is saturated;
\item a saturated spiral with $\beta(\phi) = \bar \alpha$ for $\phi \geq \phi_2$.
\end{itemize}
Due to the presence of the initial arc, we call it the \emph{arc case}. The analysis of this section refers to the geometric situation of Figure \ref{fig:enpert:arc}.

We observe that for angles $\phi\geq \phi_1$ the spiral has the same structure of the segment case (Subsection \ref{S:segment}), with $\bar\theta=\frac{\pi}{2}$, though we will show that the analysis of the derivative is different due to the presence of the initial arc: the formulas will coincide when $\bar \theta = \frac{\pi}{2}$ and $\Delta \phi = 0$, yielding as corollary that the derivative $\delta r$ is continuous across $\bar \theta = \frac{\pi}{2}$ (Remark \ref{Rem:same_as_segment}).

\begin{figure}
\centering
\includegraphics[scale=0.6]{perturbationsarc.png}
\caption{Analysis of perturbations of the arc case, Subsection \ref{S:arc}.}
\label{fig:enpert:arc}
\end{figure}


Let us denote as before
\begin{equation*}
\gls{thetapertsegm} = \frac{\pi}{2} - \theta_0
\end{equation*}
We compute now the variations up to second order terms w.r.t. $\delta s_0$:
\begin{equation*}
\delta P_0 = \delta s_0 e^{\i (\phi_0 + \frac{\pi}{2} - \theta)}, \quad \delta \phi_0 = \delta s_0 \frac{\cos(\theta)}{r(\phi_0)},
\end{equation*}
\begin{equation}\label{eq:P:1:arc}
\delta P_1 = \tilde r(\phi_1) \delta \phi_1 e^{\i (\phi_0 + \Delta\phi + \frac{\pi}{2})} + \delta s_0 \sin(\theta) e^{\i (\phi_0 + \Delta \phi)},
\end{equation}
\begin{equation}\label{eq:P:2:arc}
\delta P_2 = \delta P_1 + \delta |P_2 - P_1| e^{\i (\phi_0 + \Delta\phi + \frac{\pi}{2})} - |P_2 - P_1|e^{i\phi_1} \delta \phi_1.
\end{equation}

By the saturation condition on $P_2$ and $P_2'$ we find that
\begin{equation*}
0 = u(P_2') - \cos(\bar \alpha) (\delta s_0 +L(P'_0P'_1) +|P_2' - P_1'|+L(P_0)),
\end{equation*}
where $L(P_0)$ is the length of the spiral up to the angle $\phi_0$ and $L(P'_0P'_1)$ is the length of the arc $P'_0P_1'$, in particular
\begin{align*}
0 = e^{\i (\phi_0 + \Delta\phi+\frac{\pi}{2} - \bar \alpha)} \cdot \delta P_2 - \cos(\bar \alpha) (\delta s_0 + \delta L(P_0P_1)+ \delta |P_2 - P_1|).
\end{align*}
We now notice that
\begin{equation*}
\delta L(P_0P_1) = \delta s_0 \sin(\theta) \Delta \phi + \tilde r(\phi_1) \delta \phi_1 - \delta s_0 \cos(\theta),
\end{equation*}
so that the saturation condition becomes 
\begin{align*}
0 &= \tilde r(\phi_1) \cos(\bar \alpha) \delta \phi_1 + \delta s_0 \sin(\theta) \sin(\bar \alpha) + \delta |P_2 - P_1| \cos(\bar \alpha) - |P_2 - P_1| \delta \phi_1 \sin(\bar \alpha) \\
& \quad - \cos(\bar \alpha) \big( \delta s_0 + \delta s_0 \sin(\theta) \Delta \phi + \tilde r(\phi_1) \delta \phi_1 - \delta s_0 \cos(\theta) + \delta |P_2 - P_1| \big) \\
&= \delta s_0 \big( \cos(\bar \alpha - \theta) - \cos(\bar \alpha) - \cos(\bar \alpha) \sin(\theta) \Delta\phi \big) - |P_2 - P_1| \delta \phi_1 \sin(\bar \alpha),
\end{align*}
in particular
\begin{equation}
\label{Equa:DeltaP_arc}
|P_2 - P_1| \frac{\delta \phi_1}{\delta s_0} = \sin(\theta) - \cot(\bar \alpha) \big( 1 - \cos(\theta) + \Delta \phi \sin(\theta) \big).
\end{equation}
Moreover, from the relations
\begin{equation*}
r(\phi_2) \delta \phi_2 = \delta P_2 \cdot e^{\i (\phi_0 + \Delta \phi + \pi - \bar \alpha)} \quad \text{and} \quad \phi_2 = \phi_1 + \frac{\pi}{2} - \bar \alpha,
\end{equation*}
we obtain $\delta \phi_2 = \delta \phi_1$ and
\begin{equation}
\label{Equa:Deltar_arc}
\begin{split}
\frac{r(\phi_2) \delta \phi_1}{\sin(\bar \alpha)} - \delta |P_2 - P_1| - r(\phi_1) \delta \phi_1 &= \cot(\bar \alpha) |P_2 - P_1| \delta \phi_1 - \cot(\bar \alpha) \sin(\theta) \delta s_0 \\
&= - \cot(\bar \alpha)^2 \big( 1 - \cos(\theta) + \Delta \phi \sin(\theta) \big).
\end{split}
\end{equation}
The variation of the angle $\Delta \phi$ along the arc of the level set is then
\begin{equation}
\label{Equa:delta_Delta_phi}
\begin{split}
\delta \Delta \phi &= \delta\phi_1-\delta\phi_0 \\
&= \frac{\delta s_0}{|P_2-P_1|} \left( \sin(\theta) (1 - \cot(\bar \alpha) \Delta \phi) - \cot(\bar \alpha) (1 - \cos(\theta)) \right) - \frac{\delta s_0}{r(\phi_0)} \cos(\theta).
\end{split}
\end{equation}
The variation $\delta P(\phi)$ along the segment $[P_1,P_2]$ can be computed as 
\begin{align*}
\delta P(\phi) &= \frac{\delta P_1 \cdot e^{\i \phi_1} - |P(\phi) - P_1| e^{i\phi_1} \delta \phi_1}{\cos(\phi - \phi_1)} \\
&= \frac{1}{\cos(\phi - \phi_1)} \bigg( \sin(\theta) \bigg(1 - \frac{|P(\phi) - P_1|}{|P_2 - P_1|} \bigg) + \frac{|P(\phi) - P_1|}{|P_2 - P_1|} \cot(\bar \alpha) \big( 1 - \cos(\theta) + \Delta \phi \sin(\theta) \big) \bigg),
\end{align*}
with $\phi \in (\phi_1,\phi_2)$.

\begin{remark}
\label{rmk:deltaphi:max}
We remark that $\Delta\phi\leq\tan\bar\alpha,$ where the equality corresponds to the situation of the case study of Section \ref{S:case:study}. Indeed for such a choice
\begin{equation*}
|P_2 - P_1| \frac{\delta \Delta \phi}{\delta s_0} = - \cot(\bar \alpha) (1 - \cos(\theta)) - \frac{|P_2 - P_1|}{\tilde r(\phi_0)} \cos(\theta) < 0
\end{equation*}
unless $\theta = 0$ and $|P_2 - P_1| = 0$, i.e. only if the initial burning region is the point $(0,0)$.
\end{remark}

To compute $\delta \tilde r(\phi;s_0)$ for $\phi \geq \phi_2$, we observe that the angle $\beta(\phi)$ is equal to $\bar \alpha$ in this region, so that one obtains

\begin{lemma}
\label{Lem:equation_arc_tilde_r}
The RDE satisfied by $\tilde r$ for $\phi \geq \phi_0 +\Delta\phi+\frac{\pi}{2} - \bar \alpha$ is
\begin{equation}
\label{Equa:arc_equ_tilde_r}
\dot{\tilde r}(\phi;s_0) = \cot(\bar \alpha) \tilde r(\phi;s_0) - \begin{cases}
R(\phi) & \phi_0 +\Delta\phi+\frac{\pi}{2} - \bar \alpha \leq \phi < \phi_0 + 2\pi + \beta^-(\phi_0), \\
0 & \phi_0 + 2\pi + \beta^-(\phi_0) \leq \phi < \phi_0 + 2\pi + \frac{\pi}{2}, \\
\tilde r(\phi-2\pi-\frac{\pi}{2}) & \phi_0 + 2\pi + \frac{\pi}{2}\leq \phi\leq \phi_0 + 2\pi + \frac{\pi}{2}+\Delta\phi, \\
|P_2 - P_1| \Diracd_{\phi_0 + 2\pi + \frac{\pi}{2}+\Delta\phi} + \frac{\tilde r(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} & \phi \geq \phi_0 + 2\pi + \frac{\pi}{2}+\Delta\phi.
\end{cases}
\end{equation}
where $R(\phi)$ is the radius of curvature of $r(\phi)$ (the original spiral).
\end{lemma}

\begin{proof}
We have just to compute the radius of curvature, since $\beta(\phi) = \bar \alpha$ fixed for $\phi \geq \phi_2$. Formula \eqref{Equa:arc_equ_tilde_r} follows easily, observing that if $\beta^-(s_0) < \frac{\pi}{2}$ then there is corner in the spiral $\tilde r(\phi;s_0)$ whose subdifferential is
\begin{equation*}
\partial^- \tilde r(\phi;s_0) = \bigg\{ e^{i\phi}, \phi \in \phi_0 + 2\pi + \bigg[ \beta^-(\phi_0),\frac{\pi}{2} \bigg] \bigg\}.
\end{equation*}
For the angles $\phi_0 + 2\pi + \frac{\pi}{2}\leq \phi\leq \phi_0 + 2\pi + \frac{\pi}{2}+\Delta\phi$ the radius of curvature is precisely the radius of the spiral, computed at the previous angle (Formula \eqref{eq:subs:angle}). The jump at $\phi_0 + 2\pi + \frac{\pi}{2}+\Delta\phi$ is due to the segment $[P_1,P_2]$, corresponding in a jump in $s^-(\phi)$ at that angle.
\end{proof}

Computing the derivative w.r.t. $s_0$ for $\phi > \phi_0 + \Delta\phi+\frac{\pi}{2}- \bar \alpha$ we can prove the following

\begin{proposition}
\label{Prop:equa_delta_tilde_r_arc}
For $\phi >  \phi_0 + \Delta\phi+\frac{\pi}{2}- \bar \alpha$, the derivative
$$
\delta \tilde r(\phi;s_0) = \lim_{\delta s_0 \searrow 0} \frac{\tilde r(\phi;s_0 + \delta s_0) - \tilde r(\phi;s_0)}{\delta s_0}
$$
satisfies the RDE on $\R$
\begin{equation*}
\frac{d}{d\phi} \delta \tilde r(\phi;s_0) = \cot(\bar \alpha) \delta \tilde r(\phi;s_0) - \frac{\delta \tilde r(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} + S(\phi;s_0),
\end{equation*}
with source
\begin{align*}
S(\phi;s_0) &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\theta) + \Delta \phi \sin(\theta) \big) \Diracd_{\phi_0 + \Delta \phi + \frac{\pi}{2} - \bar \alpha} - \Diracd_{\phi_0 + 2\pi + \frac{\pi}{2} - \theta} + \cos(\theta) \Diracd_{\phi_0 + 2\pi + \frac{\pi}{2}} \\
& \quad - \sin(\theta) \ind_{2\pi + \frac{\pi}{2} + [0,\Delta \phi]} - \cot(\bar \alpha)^2 \big( 1 - \cos(\theta) + \Delta \phi \sin(\theta) \big) \Diracd_{\phi_0 + 2\pi + \Delta \phi + \frac{\pi}{2}} \\
& \quad + \big( \sin(\theta) - \cot(\bar \alpha) (1 - \cos(\theta) + \Delta \phi \sin(\theta)) \big) \Diracd'_{\phi_0 + 2\pi + \frac{\pi}{2} + \Delta \phi}.
\end{align*}
\end{proposition}

\begin{proof}
Recall the notation $\phi_1 = \phi_0 + \Delta \phi$, $\phi_2 = \phi_1 + \frac{\pi}{2} -\bar \alpha$.

We compute first the variation of the initial data of \eqref{Equa:arc_equ_tilde_r}: observing that the spiral $\tilde r(\phi;s_0)$ is saturated at $\phi_2$ and hence its tangent vector is $e^{\i (\phi_0 +\Delta\phi+\frac{\pi}{2})}$, one has up to second order terms for $\phi$ close to $\phi_2$
\begin{align*}
\delta \tilde r(\phi_2) &= \frac{\delta P_2 \cdot  e^{i\phi_1}}{\sin(\bar \alpha)} \\
&= \frac{\delta s_0 \sin(\theta) - |P_2 - P_1| \delta \phi_1}{\sin(\bar \alpha)} \\
&= \delta s_0 \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)}(1 - \cos(\theta) + \Delta \phi \sin(\theta)),
\end{align*}
which gives the first jump at $\phi_2$.

Being $R(\phi)$ the same up to $\phi_0 + 2\pi + \theta_0$, the RDE for $\delta \tilde r$ is actually the ODE
\begin{equation*}
\frac{d}{d\phi} \delta \tilde r(\phi) = \cot(\bar \alpha) \delta \tilde r(\phi)
\end{equation*}
for $\phi_0 + \Delta\phi + \frac{\pi}{2} - \bar\alpha \leq \phi < \phi_0 + 2\pi + \theta_0$.

Using $R = Ds^-$ and taking $\delta \phi \ll 1$, the variation at $\phi_0 + 2\pi + \theta_0$ is up to second order terms w.r.t. $\delta \phi$
\begin{align*}
&\tilde r(\phi_0+2\pi+\theta_0 + \delta \phi; s_0 + \delta s_0) - \tilde r(\phi_0+2\pi+\theta_0 + \delta \phi;s_0) \\
\quad &= (1 + \cot(\bar \alpha) \delta \phi) \big( \tilde r(\phi_0+2\pi+\theta_0;s_0 + \delta s_0) - \tilde r(\phi_0+2\pi+\theta_0;s_0) \big) - \big( s^-(\phi_0 + 2\pi + \theta_0 + \delta \phi) - s^-(\phi_0 + 2\pi + \theta_0) \big) \\
\quad &= (1 + \cot(\bar \alpha) \delta \phi) \big( \tilde r(\phi_0 + 2\pi + \theta_0;s_0 + \delta s_0) - \tilde r(\phi_0 + 2\pi + \theta_0;s_0) \big) - \delta s_0.
\end{align*}
Dividing by $\delta s_0$, letting $\delta s_0 \searrow 0$ first and then $\phi \searrow 0$, we conclude that $\delta \tilde r(\phi;s_0)$ has a jump of size $-1$ at the angle $\phi_0 + 2\pi + \theta_0$.

From \eqref{Equa:arc_equ_tilde_r} it follows that
\begin{equation*}
\frac{d}{d\phi} \delta \tilde r(\phi) = \cot(\bar \alpha) \delta \tilde r(\phi)
\end{equation*}
for $\phi \in \phi_0 + 2\pi + [\theta_0,\frac{\pi}{2}]$.

At about the angle $\phi = \phi_0 + 2\pi + \frac{\pi}{2}$, we can repeat the analysis for a small angle as we did at about the angle $\phi_0 + 2\pi + \theta_0$ above,  obtaining that
there is an upward jump of value $\cos(\theta)$, giving the source $\cos(\theta) \Diracd_{\phi_0 + 2\pi + \frac{\pi}{2}}$.

Again, from \eqref{Equa:arc_equ_tilde_r} it follows that
\begin{equation*}
\frac{d}{d\phi} \delta \tilde r(\phi) = \cot(\bar \alpha) \delta \tilde r(\phi) - \sin(\theta),
\end{equation*}
for $\phi_0 + 2\pi + \frac{\pi}{2} < \phi < \phi_0 + 2\pi + \frac{\pi}{2}+\Delta\phi$, because $\delta \tilde r(\phi_0 + \frac{\pi}{2} + [0,\Delta \phi)) = \sin(\theta)$.

At the angle $\phi_0 + 2\pi + \frac{\pi}{2} + \Delta \phi$ the solution has a discontinuity due to the variation of $\delta \phi_1$ and $|P_2 - P_1|$: computing the first order approximations for $0 \leq \delta \phi \ll 1$ one gets
\begin{align*}
&\tilde r \bigg( \phi_0 + 2\pi + \frac{\pi}{2} + \Delta \phi + \delta \phi, s_0 + \delta s_0 \bigg) - \tilde r \bigg( \phi_0 + 2\pi + \frac{\pi}{2} + \Delta\phi +\delta \phi,s_0 \bigg) \\
& \quad = \left[ \tilde r \bigg( \phi_0 + 2\pi + \frac{\pi}{2} + \Delta \phi - \delta \phi, s_0 + \delta s_0 \bigg) - \tilde r \bigg( \phi_0 + 2\pi + \frac{\pi}{2} + \Delta \phi - \delta \phi,s_0 \bigg) \right] (1 + 2 \cot(\bar \alpha) \delta \phi) \\
& \quad \quad - |P'_2 - P'_1| - (\delta \phi + \delta \phi_1) \tilde r(\phi_1,s_0 + \delta s_0) - (\delta \phi - \delta \phi_1) \frac{\tilde r(\phi_2,s_0 + \delta s_0)}{\sin(\bar \alpha)} \\
& \quad \quad + |P_2 - P_1| + \delta \phi \tilde r(\phi_1,s_0) + \delta \phi \frac{\tilde r(\phi_2,s_0)}{\sin(\bar \alpha)}
\end{align*}
Dividing by $\delta s_0$ and passing to the limit $\delta s_0 \searrow 0$ we obtain
\begin{align*}
&\delta \tilde r \bigg( \phi_0 + 2\pi + \frac{\pi}{2} + \Delta \phi + \delta \ell;s_0 \bigg) \\
& \quad = \delta \tilde r \bigg( \phi_0 + 2\pi + \frac{\pi}{2} + \Delta \phi - \delta \ell;s_0 \bigg) \big( 1 + 2 \cot(\bar \alpha) \delta \phi \big) - \frac{\delta \tilde r(\phi_2;s_0)}{\sin(\bar \alpha)} \delta \phi \\
& \quad \quad + |P_2 - P_1| \frac{\delta \phi_1}{\delta s_0} \Diracd_{\phi_0+2\pi + \frac{\pi}{2} + \Delta \phi} + \bigg[ - \frac{\delta |P_2 - P_1|}{\delta s_0} - \frac{\delta \phi_1}{\delta  s_0} \tilde r(\phi_1) + \frac{\delta \phi_1}{\delta {s_0}} \frac{\tilde r(\phi_2)}{\sin(\bar \alpha)} \bigg].
\end{align*}
Hence its derivative w.r.t. $\phi$ satisfies
\begin{align*}
\frac{d}{d\phi} \delta \tilde r(\phi;s_0) &= \cot(\bar \alpha) \delta \tilde r(\phi;s_0) - \frac{\delta \tilde r(\phi - 2\pi - \bar \alpha;s_0)}{\sin(\bar \alpha)} \\
& \quad + \bigg( - \frac{\delta |P_2 - P_1|}{\delta s_0} + \frac{\tilde r(\phi_2;s_0)}{\sin(\bar \alpha)} \frac{\delta \phi_1}{\delta s_0} -\tilde r(\phi_1)\frac{\delta\phi_1}{\delta s_0} \bigg) \Diracd_{\phi_0 + 2\pi + \frac{\pi}{2}+\Delta \phi} + |P_2 - P_1| \frac{\delta \phi_1}{\delta s_0} \Diracd'_{\phi_0 + 2\pi +\frac{\pi}{2}+\Delta\phi},
\end{align*}
where $\Diracd'$ is the derivative of the Dirac's delta:
\begin{equation*}
\langle \Diracd'_x, f \rangle = - \frac{df(x)}{dx}.
\end{equation*}
Using \eqref{Equa:DeltaP_arc} and \eqref{Equa:Deltar_arc} we obtain source in the statement.

For $\phi \geq \phi_2 + 2\pi + \bar \alpha$ the equation is linear, and then the conclusion follows.
\end{proof}

We remark that, since
\begin{equation*}
\frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \left( 1 - \cos(\theta) + \Delta \phi \sin(\theta) \right) \geq 0,
\end{equation*}
being $\Delta\phi\geq 0$,  it follows that the perturbation is positive for $\phi \in [0,\phi_0 + \frac{\pi}{2} + \Delta \phi -\bar\alpha]$, as the optimality of Theorem \ref{Cor:curve_cal_R_sat_spiral} implies.

\begin{remark}
\label{Rem:same_as_segment}
Observe that when $\Delta \phi = 0$ the source becomes
\begin{align*}
S(\phi;s_0) &= \frac{\cos(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta)) \Diracd_{\phi_0 + \frac{\pi}{2} - \bar \alpha} - \Diracd_{\phi_0 + 2\pi + \theta_0} \\
& \quad + \big( \cos(\theta) - \cot(\bar \alpha)^2 (1 - \cos(\theta)) \big) \Diracd_{\phi_0 + 2\pi + \frac{\pi}{2}} + \big( \sin(\theta) - \cos(\bar \alpha) (1 - \cos(\theta)) \big) \Diracd'_{\phi_0 + 2\pi + \frac{\pi}{2}},
\end{align*}
which is the same as the source of the segment case when $\bar \theta = \frac{\pi}{2}$. Hence the derivative $\delta r$ is continuous when passing from the segment case to the arc case.
\end{remark}

Using the kernel $G$ of Remark \ref{Rem:oringal_phi_kernel} we obtain the following explicit representation of the solution $\delta \tilde r$.

\begin{corollary}
\label{Cor:evolv_r_after_phi_2:arc}
The solution $\delta \tilde r(\phi)$ for $\phi \geq \phi_2 = \phi_0 + \frac{\pi}{2} - \bar \alpha + \Delta \phi$ is explicitly given by
\begin{equation}
\label{Equa:evolv_r_after_phi_2:arc}
\begin{split}
\delta \tilde r(\phi;s_0) &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \left( 1 - \cos(\theta) + \Delta \phi \sin(\theta) \right) G \bigg( \phi - \phi_0 - \Delta \phi - \frac{\pi}{2} + \bar \alpha \bigg) - G(\phi - \phi_0 - 2\pi - \theta_0) \\
& \quad + \cos(\theta) G \bigg( \phi - \phi_0 - 2\pi - \frac{\pi}{2} \bigg) - \sin(\theta) M \bigg( \phi; \phi_0 + 2\pi + \frac{\pi}{2}; \phi_0 + 2\pi + \frac{\pi}{2} + \Delta \phi \bigg) \\
& \quad + \bigg( - \cot(\bar \alpha)^2 \big( 1 - \cos(\theta) + \Delta \phi \sin (\theta) \big) + \cot(\bar \alpha) \big( \sin(\theta) - \cot(\bar \alpha) (1 - \cos(\theta) + \Delta \phi \sin(\theta)) \big) \bigg) G \bigg( \phi -\phi_0 - 2\pi - \Delta \phi - \frac{\pi}{2} \bigg) \\
& \quad + \big( \sin(\theta) - \cot(\bar \alpha) (1 - \cos(\theta) + \Delta \phi \sin(\theta)) \big) \Diracd_{\phi_0 + 2\pi + \frac{\pi}{2} + \Delta \phi} \\
& \quad - \frac{1}{\sin(\bar \alpha)} \big( \sin(\theta) - \cot(\bar \alpha) (1 - \cos(\theta) + \Delta \phi \sin(\theta)) \big) G \bigg( \phi - \phi_0 - 2\pi - \Delta \phi - \frac{\pi}{2} - 2\pi  - \bar \alpha \bigg).
\end{split}
\end{equation}
\end{corollary}

We next make the change of variables
\begin{equation*}
\delta \tilde r(\phi_2 + (2\pi + \bar \alpha) \tau;s_0) = \rho(\tau) e^{\bar c (2\pi + \bar \alpha) \tau},
\end{equation*}
obtaining the following corollary.


\begin{corollary}
\label{Cor:arc_rho_eq}
The values of the perturbation depend only on the angles $\theta = \frac{\pi}{2} - \theta_0$ and $\Delta \phi$, and the function $\rho(\tau)$ is given by
\begin{equation*}
\rho(\tau) = S_0 g(\tau) + S_1 g(\tau - \tau_1) + S_2 g(\tau - \tau_2) + S_3 m(\tau,\tau_2,1) + S_4 g(\tau-1) + D \Diracd_1 + S_5 g(\tau-2),
\end{equation*}
where \newglossaryentry{tau2}{name=\ensuremath{\tau_2},description={time of the second discontinuity in the perturbation in the arc case}}
\begin{equation*}
\gls{tau1} = 1 - \frac{\Delta \phi + \theta}{2\pi + \bar \alpha}, \quad \gls{tau2} = 1 - \frac{\Delta \phi}{2\pi + \bar \alpha},
\end{equation*}
and
\begin{subequations}
\label{Equa:sources_rho_arc}
\begin{equation}
\label{Equa:S0_arc}
S_0(\theta,\Delta \phi) = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\theta) + \Delta \phi \sin(\theta) \big),
\end{equation}
\begin{equation}
\label{Equa:S1_arc}
S_1(\theta,\Delta \phi) = - e^{- \bar c(2\pi + \bar \alpha) \tau_1} = - \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} e^{\bar c(\Delta \phi + \theta)},
\end{equation}
\begin{equation}
\label{Equa:S2_arc}
S_2(\theta,\Delta \phi) = \cos(\theta) e^{-\bar c(2\pi + \bar \alpha) \tau_2} = \frac{\sin(\bar \alpha) \cos(\theta)}{2\pi + \bar \alpha} e^{\bar c \Delta \phi},
\end{equation}
\begin{equation}
\label{Equa:S3_arc}
S_3(\theta) = - \sin(\theta), \qquad m(\tau,\tau_2,1) = \int_{\tau_2}^1 g(\tau - \tau') e^{- \bar c(2\pi + \bar \alpha) \tau'} (2\pi + \bar \alpha) d\tau',
\end{equation}
\begin{equation}
\label{Equa:S4_arc}
S_4(\theta,\Delta \phi) = \frac{\cos(\bar \alpha)}{2\pi + \bar \alpha} \Big( - 2 \cot(\bar \alpha) (1 - \cos(\theta) + \Delta \phi \sin(\theta)) + \sin(\theta) \Big)
\end{equation}
\begin{equation}
\label{Equa:D_arc}
D(\theta,\Delta \phi) = \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} \big( \sin(\theta) - \cot(\bar \alpha) (1 - \cos(\theta) + \Delta \phi \sin(\theta)) \big), 
\end{equation}
\begin{equation}
\label{Equa:S5_arc}
S_5(\theta,\Delta \phi) = - \frac{\sin(\bar \alpha)}{(2\pi + \bar \alpha)^2} \Big( \sin(\theta) - \cot(\bar \alpha) (1 - \cos(\theta) + \Delta \phi \sin(\theta)) \Big).
\end{equation}
\end{subequations}
\end{corollary}

The next result is essential for the next analysis.

\begin{proposition}
\label{Prop:neg_region}
The function $\rho = \rho(\tau;\theta,\Delta \phi)$ is strictly positive outside the region \newglossaryentry{h1Deltaphi}{name=\ensuremath{h_1(\Delta \phi)},description={boundary of the first negativity region in the arc case}} \newglossaryentry{h2Deltaphi}{name=\ensuremath{h_2(\Delta \phi)},description={boundary of the first negativity region in the arc case}} \newglossaryentry{h3Deltaphi}{name=\ensuremath{h_3(\Delta \phi)},description={boundary of the first negativity region in the arc case}} \newglossaryentry{tau3thetaDeltaphi}{name=\ensuremath{\tau_3(\theta,\Delta \phi)},description={initial time of the third negativity region in the arc case}} \newglossaryentry{Narc}{name=\ensuremath{N_\mathrm{arc}},description={negative region for the perturbation of the arc case}} \newglossaryentry{Nresarc}{name=\ensuremath{N_\mathrm{res}},description={residual negative region for the arc case}}
\begin{align*}
\gls{Narc} &= \{\theta = 0\} \cup \big\{ \tau_1 \leq \tau < \tau_2, 0 \leq \theta \leq \gls{h1Deltaphi} \big\} \\
&\quad \cup \big\{\tau_2(\Delta \phi) \leq \tau < 1, 0 \leq \theta \leq \gls{h2Deltaphi} \big\} \\
&\quad \cup \big\{ \gls{tau3thetaDeltaphi} \leq \tau < 1, h_2(\Delta \phi) \leq \theta < \gls{h3Deltaphi} \big\} \cup \gls{Nresarc}, %\\
%&\quad \cup \big\{ \tau \geq 3, \theta \in (3.12,\pi], \Delta \phi \in (2.37,\tan(\bar \alpha)] \big\},
\end{align*}
where the functions $\gls{h1Deltaphi},\gls{h2Deltaphi},\gls{h3Deltaphi},\gls{tau3thetaDeltaphi}$ are determined by solving the equations
\begin{itemize}
\item for $\tau_1 \leq \tau \leq \tau_2$, the function $h_1(\Delta \phi)$ is determined implicitly by
\begin{equation}
\label{Equa:theta_Deltaphi_rel}
\frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) + \sin(\theta) \Delta \phi) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta \phi - \theta)} - 1 = 0,
\end{equation}
\item for $\tau_2 \leq \tau \leq 1$, the function $h_2(\Delta \phi)$ is determined by
\begin{equation*}
\frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) + \sin(\theta) \Delta \phi) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta \phi)} - e^{\cot(\bar \alpha) \theta} + \cos(\theta) = 0,
\end{equation*}
\item for $\tau_3 \leq \tau \leq 1$, the function $h_3(\Delta \phi)$ is determined by
\begin{equation*}
\frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) + \sin(\theta) \Delta \phi) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta \phi)} - e^{\cot(\bar \alpha) \theta} + \cos(\theta) - \sin(\theta) \frac{e^{\cot(\bar \alpha) \Delta \phi} - 1}{\cot(\bar \alpha)} = 0,
\end{equation*}
\item the function $\tau_3(\theta,\Delta \phi) = 1 - \frac{\theta_3}{2\pi + \bar \alpha}$ is given by solving in the region $\{h_2(\Delta \phi) \leq \theta \leq h_3(\Delta \phi)\}$
\begin{equation*}
\frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) + \sin(\theta) \Delta \phi) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \theta_3)} - e^{\cot(\bar \alpha) (\Delta \phi + \theta - \theta_3)} + \cos(\theta) e^{\cot(\bar \alpha) (\Delta \phi - \theta_3} - \sin(\theta) M(\Delta \phi - \theta_3;0,\Delta \phi) = 0.
\end{equation*}
\end{itemize}
Finally, the region \gls{Nresarc} is contained in the set
\begin{equation*}
N_\mathrm{res} \subset \big\{ \tau \geq 3, \theta \in (3.12,\pi], \Delta \phi \in (2.37,\tan(\bar \alpha)] \big\}.
\end{equation*}

The asymptotic behavior is given by
\begin{equation}
\label{Equa:asympt_arc_sta}
\lim_{\tau \to \infty} \frac{\rho(\tau) e^{-\bar c \tau}}{\tau \theta(\theta + \Delta \phi)} = \frac{2}{\theta ( \theta+ \Delta \phi)} \bigg( S_0 + S_1 + S_2 + S_3 \frac{e^{-\bar c (2\pi + \bar \alpha) \tau_2} - e^{-\bar c(2\pi + \bar \alpha)}}{\bar c} + S_4 + S_5 \bigg).
\end{equation}
\end{proposition}

The region of negativity for the arc case is depicted in Fig. \ref{Fig:nega_arc_case} in the first 3 rounds: the last region is due to the fact that the sum of the sources in \eqref{Equa:asympt_arc_sta} is negative in some region, see Fig. \ref{Fig:asympt_arc} below. We will not use this region in our perturbations.

\begin{figure}
\resizebox{.75\textwidth}{!}{\input{negat_regio_arc.pdf_t}}
\caption{The region where $\delta \tilde r \leq 0$ in the arc case: in addition to the plane $\{\theta = 0\}$, it contains the cyan region $\{0 \leq \theta \leq h_1(\Delta \phi), \tau_1 \leq \tau \leq \tau_2\}$ and the trapezoidal blue region for $\{\tau_2 \leq \tau \leq 1\}$.}
\label{Fig:nega_arc_case}
\end{figure}

\begin{proof}
The proof will be given in several steps.


\medskip

{\it Case 0: $\theta = 0$.}

\noindent It is easy to see that in this case $\rho(\tau) = 0$, so that $\{\theta = 0\} \subset N_{\mathrm{arc}}$.

\medskip

{\it Case 1: $\tau \in [0,\tau_1)$.}

\noindent Being $S_0 > 0$ for $\theta > 0$, it follows that $\rho(\tau) > 0$ in this region.


\medskip

{\it Case 2: $\tau \in [\tau_1,\tau_2)$.}

\noindent The solution $\delta r(\phi;s_0)$ is written explicitly as
\begin{align*}
\delta r(\phi;s_0) &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) + \sin(\theta) \Delta \phi) e^{\cot(\bar \alpha) (\phi - \phi_2)} - e^{\cot(\bar \alpha) (\phi - \phi_2 - 2\pi - \bar \alpha + \Delta \phi + \theta} \\
&= e^{\cot(\bar \alpha)(\phi - \phi_2 - 2\pi - \bar \alpha + \Delta \phi + \theta} \bigg( \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) + \sin(\theta) \Delta \phi) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta \phi - \theta)} - 1 \bigg). 
\end{align*}
The study of the above equation is done in the following lemma.

\begin{lemma}
\label{Lem:study_g_1_arc}
The equation
\begin{equation}
\label{Equa:thetaDeltaphi_def}
\frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) + \sin(\theta) \Delta \phi) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta \phi - \theta)} - 1 = 0
\end{equation}
determines implicitly a function \gls{h1Deltaphi} such that
\begin{equation*}
h_1(\Delta \phi) < \hat \theta \quad \text{unless} \ \Delta \phi = 0,
\end{equation*}
and moreover
\begin{equation*}
\Delta \phi \mapsto \hat \theta(\Delta \phi) := \Delta \phi + h_1(\Delta \phi)
\end{equation*}
is strictly increasing unless $\Delta \phi = 0$ and has derivative $<1$.
\end{lemma}

\begin{figure}
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{h1_plot_arc1.png}
\caption{Plot of the function $h_1(\Delta \phi)$ of Lemma \ref{Lem:study_g_1_arc}.}
\label{Fig:h1_plot}
\end{subfigure}
\hfill
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{h1Deltaphi_plot_arc1.png}
\caption{Plot of the function $h_1(\Delta \phi) + \Delta \phi$ of Lemma \ref{Lem:study_g_1_arc}.}
\label{Fig:h1Deltaphi_plot}
\end{subfigure}
\end{figure}

A numerical plot of $h_1(\Delta \phi)$ is in Fig. \ref{Fig:h1_plot}, while in Fig. \ref{Fig:h1Deltaphi_plot} it is plotted the function $h_1(\Delta \phi) + \Delta \phi$.

\begin{proof}
Let
\begin{equation}
\label{Equa:f_1_arc_first_neg}
f_1(\theta,\Delta \phi) = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) + \sin(\theta) \Delta \phi) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta \phi - \theta)} - 1.
\end{equation}
Taking the derivative w.r.t. $\theta$ we obtain
\begin{equation}
\label{Equa:partialf_1_arc_first_neg}
\begin{split}
\partial_\theta f_1 &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( \sin(\theta) + \cos(\theta) \Delta \phi - \cot(\bar \alpha) (1 - \cos(\theta) + \sin(\theta) \Delta \phi) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta \phi - \theta)} \\
&= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)^2} \big( \cos(\bar \alpha - \theta) - \cos(\bar \alpha) + \sin(\bar \alpha - \theta) \Delta \phi \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta \phi - \theta)}.
\end{split}
\end{equation}
Since numerically one observes that (see Fig. \ref{Fig:partialf_1_arc_first_neg})
\begin{equation*}
f_1 \bigg( \bigg[ \frac{\pi}{4}, \pi \bigg] \times [0,\tan(\bar \alpha)] \bigg) \geq f_1(\pi,\tan(\bar \alpha)) = 0.971097,
\end{equation*}
\begin{equation*}
\partial_\theta f_1 \bigg( \bigg[0,\frac{\pi}{4} \bigg],\Delta \phi \bigg) \geq \partial_\theta f_1 \bigg( \frac{\pi}{4},0 \bigg) \geq 1.29579 (\theta + \Delta \phi),
\end{equation*}
then $\partial_\theta f_1 > 0$ in the region $(0,\frac{\pi}{4}) \times [0,\tan(\bar \alpha)]$ (observe that $f1(0,\Delta \phi) = -1$). We deduce that the equation $f_1(\theta,\Delta \phi) = 0$ defines an implicit function $h_1(\Delta \phi)$, such that
\begin{equation*}
h_1(\Delta \phi) < \hat \theta \quad \text{unless} \ \Delta \phi = 0.
\end{equation*}

\begin{figure}
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{f1_arc_first_neg1.png}
\caption{Plot of the function $f_1(\theta,\Delta \phi)$ (\ref{Equa:f_1_arc_first_neg}).}
\label{Fig:f_1_arc_first_neg}
\end{subfigure}\hfill
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{partialf1_arc_first_neg1.png}
\caption{Plot of the function $\partial_\theta f_1(\theta,\Delta \phi)$ (\ref{Equa:partialf_1_arc_first_neg}).}
\label{Fig:partialf_1_arc_first_neg}
\end{subfigure}
\medskip
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{derivative_h_1_arc.png}
\caption{Plot of the function (\ref{Equa:dh1_dDeltaphi}).}
\label{Fig:dh1_dDeltaphi}
\end{subfigure}\hfill
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{d2h1_arc.png}
\caption{Plot of the function (\ref{Equa:d2h1_dDeltaphi}).}
\label{Fig:d2h1_dDeltaphi}
\end{subfigure}
\end{figure}

By the Implicit Function Theorem we obtain
\begin{equation}
\label{Equa:dh1_dDeltaphi}
\begin{split}
\frac{dh_1}{d\Delta \phi} &= - \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha) - \cos(\bar \alpha) \sin(\theta) \Delta \phi}{\cos(\bar \alpha - \theta) - \cos(\bar \alpha) + \sin(\bar \alpha - \theta) \Delta \phi} \\
&= - 1 + \frac{\sin(\bar \alpha) \cos(\theta) \Delta \phi}{\cos(\bar \alpha - \theta) - \cos(\bar \alpha) + \sin(\bar \alpha - \theta) \Delta \phi}.
\end{split}
\end{equation}
so that in the region of interest one can check numerically that (see Fig. \ref{Fig:dh1_dDeltaphi})
\begin{equation*}
-1 \leq \frac{dh_1(\Delta \phi)}{d\Delta \phi} < - 1 + \frac{\sin(\bar \alpha) \cos(\hat \theta) \tan(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha) + \sin(\bar \alpha - \hat \theta) \tan(\bar \alpha)} = 0.0251844.
\end{equation*}
Differentiating w.r.t $\Delta \phi$ one obtains
\begin{equation}
\label{Equa:d2h1_dDeltaphi}
\begin{split}
\frac{d^2h_1}{d\Delta \phi^2} &= \partial_{\Delta \phi} \frac{dh_1}{d\Delta \phi} + \partial_{\theta} \frac{dh_1}{d\Delta \phi} \frac{dh_1}{d\Delta \phi} \\
&= \frac{\sin(\bar \alpha) \cos(\theta) (\cos(\bar \alpha - \theta) - \cos(\bar \alpha))}{(\cos(\bar \alpha - \theta) - \cos(\bar \alpha) + \sin(\bar \alpha - \theta) \Delta \phi)^2} \\
& \quad + \frac{\sin(\bar \alpha) \Delta \phi (- \sin(\bar \alpha) - \cos(\bar \alpha) \sin(\theta) + \cos(\bar \alpha) \Delta \phi)}{(\cos(\bar \alpha - \theta) - \cos(\bar \alpha) + \sin(\bar \alpha - \theta) \Delta \phi)^2} \bigg( - 1 + \frac{\sin(\bar \alpha) \cos(\theta) \Delta \phi}{\cos(\bar \alpha - \theta) - \cos(\bar \alpha) + \sin(\bar \alpha - \theta) \Delta \phi} \bigg),
\end{split}
\end{equation}
and numerically one sees that (see Fig. \ref{Fig:d2h1_dDeltaphi})
\begin{equation*}
\frac{d^2 h_1}{d\Delta \phi^2} > 0.0168525,
\end{equation*}
so that the function is convex, with a minimum near $\Delta \phi = 2.35681$.

Finally, the only case for which $\frac{dh_1}{d\Delta \phi} = -1$ is for $\Delta \phi = 0$, $g_3(\Delta \phi) = \hat \theta$. This means that the function
\begin{equation*}
\delta \phi \mapsto \hat \theta(\Delta \phi) = \Delta \phi + h_1(\Delta \phi)
\end{equation*}
is strictly increasing, convex and has derivative $0$ for $\Delta \phi = 0$, see Fig. \ref{Fig:h1Deltaphi_plot}.
\end{proof}

\medskip

{\it Case 3: $\tau \in [\tau_2,1)$.}

\noindent The solution to be studied is
\begin{align*}
\delta \tilde r(\phi;s_0) &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) + \sin(\theta) \Delta \phi) e^{\cot(\bar \alpha) (\phi - \phi_2)} - e^{\cot(\bar \alpha) (\phi - \phi_2 - 2\pi - \bar \alpha + \Delta \phi + \theta)} \\
&\quad + \cos(\theta) e^{\cot(\bar \alpha) (\phi - \phi_2 - 2\pi - \bar \alpha + \Delta \phi)} - \sin(\theta) \int_{\phi_2 + 2\pi + \bar \alpha + \Delta \phi}^\phi e^{\cot(\bar \alpha) (\phi - \phi')} d\phi' \\
&= e^{\cot(\bar \alpha)(\phi - \phi_2 - 2\pi - \bar \alpha + \theta)} \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) + \sin(\theta) \Delta \phi) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \theta)} - e^{\cot(\bar \alpha) \theta} + \cos(\theta) \bigg] \\
& \quad - \sin(\theta) \tan(\bar \alpha) \big( e^{\cot(\bar \alpha) (\phi - \phi_2 - 2\pi - \bar \alpha + \theta)} - 1 \big).
\end{align*}
At the initial angle $\phi = \phi_2 + 2\pi + \bar \alpha - \Delta \phi$ we have
\begin{equation}
\label{Equa:f2_arc}
f_2(\theta,\Delta \phi) = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) + \sin(\theta) \Delta \phi) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta \phi)} - e^{\cot(\bar \alpha) \theta} + \cos(\theta) = f_1(\theta,\Delta \phi) e^{\cot(\bar \alpha) \theta} + \cos(\theta).
\end{equation}
Numerical plots (see Fig. \ref{Fig:f_2_arc}) show that $f_2 < 0$ is a triangular shaped region $N_2$ with corners
\begin{equation*}
(0,0), \quad (0.0956622,0), \quad (0,0.0428438).
\end{equation*}

\begin{figure}%[hbt!]
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{f2_initial.png}
\caption{Plot of the function $f_2(\theta,\Delta \phi)$ (\ref{Equa:f2_arc}).}
\label{Fig:f_2_arc}
\end{subfigure}\hfill
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{f3_initial.png}
\caption{Plot of the function $f_3(\theta,\Delta \phi)$ (\ref{Equa:f3_arc}).}
\label{Fig:f_3_arc}
\end{subfigure}
\medskip
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{f4_initial.png}
\caption{Plot of the function (\ref{Equa:f4_arc}).}
\label{Fig:f_4_arc}
\end{subfigure}\hfill
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{f234together.png}
\caption{Plot of $f_2(\cdot/3) = 0$ (blue), $f_3 = 0$ (orange), $f_4(\cdot/3) = 0$ (green). We have rescaled the first and the third for clarity.}
\label{Fig:f234}
\end{subfigure}
\end{figure}

Next, we take the derivative of $\delta \tilde r(\phi;s_0)$ w.r.t. $\phi$, obtaining
\begin{equation}
\label{Equa:f3_arc}
\begin{split}
\partial_\phi \delta \tilde r(\phi;s_0) &= e^{\cot(\bar \alpha)(\phi - \phi_2 - 2\pi - \bar \alpha + \Delta \phi)} \cot(\bar \alpha) \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) + \sin(\theta) \Delta \phi) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta \phi)} - e^{\cot(\bar \alpha) \theta} + \cos(\theta) - \sin(\theta) \tan(\bar \alpha) \bigg] \\
&= e^{\cot(\bar \alpha)(\phi - \phi_2 - 2\pi - \bar \alpha + \Delta \phi)} \cot(\bar \alpha) f_3(\theta,\Delta \phi).
\end{split}
\end{equation}
%Again, the derivative w.r.t. $\theta$ at $\theta = 0$ gives
%\begin{equation*}
%    \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \Delta \phi e^{\cot(\bar \alpha) (2\pi + \bar \alpha)} - \cot(\bar \alpha) - 1,
%\end{equation*}
%which is negative for
%\begin{equation*}
%    \Delta \phi < \sin(\bar \alpha) e^{\cot(\bar \alpha) (2\pi + \bar \alpha)} (1 + \tan(\bar \alpha)) \simeq 0.2877.
%\end{equation*}
Numerically (see Fig. \ref{Fig:f_3_arc}), the negativity region is a triangular shaped region $N_3$ with corners
\begin{equation*}
    (0,0), \quad (0.639078,0), \quad (0,0.329784).
\end{equation*}
Being this region larger than the negativity region for $f_2$, it follows that
\begin{equation*}
    \big\{ \tau \in [\tau_2,1], (\theta,\Delta \phi) \in N_2 \big\} \subset N_{\mathrm{arc}},
\end{equation*}
and
\begin{equation*}
    \big\{ \tau \in [\tau_2,1], (\theta,\Delta \phi) \notin N_3 \big\} \cap N_\mathrm{arc} = \emptyset. 
\end{equation*}
In particular the derivative of $\delta \tilde r(\phi;s_0)$ is strictly negative in the region of interest, and thus this determines a function $\tau_2(\theta,\Delta \phi)$ whose graph is the boundary of the region of negativity.

The maximal region is computed by considering
\begin{equation}
\label{Equa:f4_arc}
\begin{split}
\delta \tilde r(\phi_2 + 2\pi + \bar \alpha -;s_0) &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) + \sin(\theta) \Delta \phi) e^{\cot(\bar \alpha) (2\pi + \bar \alpha)} - e^{\cot(\bar \alpha) (\theta + \Delta \phi)} \\
& \quad + \cos(\theta) e^{\cot(\bar \alpha) \Delta \phi} - \sin(\theta) \tan(\bar \alpha) \big( e^{\cot(\bar \alpha) \Delta \phi} - 1 \big) \\
&= f_4(\theta,\Delta \phi).
\end{split}
\end{equation}
Numerically (see Fig. \ref{Fig:f_4_arc}) the negativity region is triangular shaped with corners
\begin{equation*}
    (0,0), \quad (0,0.0478458), \quad (0.0956622,0).
\end{equation*}

The contours of the three regions of negativity are in Fig. \ref{Fig:f234}.

\medskip

{\it Case 4: $\tau \in [1,1+\tau_1)$} 

\noindent The solution $\rho$ is
\begin{align*}
\rho(\tau) &= S_0 (e^{\tau} - e^{\tau - 1} (\tau - 1)) + S_1 e^{\tau - \tau_1} + S_2 e^{\tau - \tau_2} + S_3 e^{- \bar c (2\pi + \bar \alpha)} \frac{e^{\cot(\bar \alpha) \Delta \phi} - 1}{\cot(\bar \alpha)} e^{\tau - 1} + S_4 e^{\tau - 1} \\
&= e^{\tau - 1} \bigg[ S_0 (e - (\tau - 1)) + S_1 e^{1 - \tau_1} + S_2 e^{1 - \tau_2} + S_3 e^{-\bar c(2\pi + \bar \alpha)} \frac{e^{\cot(\bar \alpha) \Delta \phi} - 1}{\cot(\bar \alpha)} + S_4 \bigg].
\end{align*}
The worst case is for $\tau = 1 + \tau_1$, so that we have to study the function
\begin{align*}
f(\theta,\Delta \phi) &= S_0 (e - \tau_1) + S_1 e^{1 - \tau_1} + S_2 e^{1 - \tau_2} + S_3 \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} \frac{e^{\cot(\bar \alpha) \Delta \phi} - 1}{\cot(\bar \alpha)} + S_4.
\end{align*}
%The expansion at $\theta = 0$ gives
%\begin{align*}
%f(\theta,\Delta \phi) &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \theta \Delta \phi \bigg( e - 1 + \frac{\Delta \phi}{2\pi + \bar \alpha} \bigg) - \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} e^{\cot(\bar \alpha) \Delta \phi} (1 + \cot(\bar \alpha) \theta) \\
%&\quad + \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} e^{\cot(\bar \alpha \Delta \phi} - \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} \theta \frac{e^{ \cot(\bar \alpha) \Delta \phi}-1}{\cot(\bar \alpha)} + \frac{\cos(\bar \alpha)}{2\pi + \bar \alpha} \big( - 2 \cot(\bar \alpha) \theta \Delta \phi + \theta \big) + \mathcal O(\theta^2) \\
%&= \theta \Delta \phi \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \bigg( e - 1 + \frac{\Delta \phi}{2\pi + \bar \alpha} \bigg) - 2 \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} \frac{e^{ \cot(\bar \alpha) \Delta \phi}-1}{\cot(\bar \alpha) \Delta \phi} - \frac{2 \cot(\bar \alpha) \cos(\bar \alpha)}{2\pi + \bar \alpha} \bigg] + \mathcal O(\theta^2).
%\end{align*}
One observes numerically that the quantity inside the bracket is strictly positive ($> 0.44$), and also numerically one obtains that
\begin{equation*}
\frac{f(\theta,\Delta \phi)}{\theta(\theta + \Delta \phi)} \geq \frac{f(\pi,\tan(\bar \alpha))}{\pi(\pi + \tan(\bar \alpha)} = 0.031,
\end{equation*}
and that (see Fig. \ref{Fig:second_round_arc_1})
\begin{equation*}
\frac{\rho([1,1+\tau_1),\theta,\Delta \phi)}{\theta(\theta + \Delta \phi)} \geq \frac{\rho(1+\tau_1,\pi,\tan(\bar \alpha))}{\pi(\pi+\tan(\bar \alpha)} > 0.04.
\end{equation*}

\begin{figure}
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{second_round_arc_1.1.png}
\caption{Plot of the function $\frac{\rho(1 + s \tau_1,\theta,\Delta \phi)}{\theta (\theta + \Delta \phi)}$ for $s \in \{0,.2,.4,.6,.8,1\}$ (monotonically bottom to top graph).}
\label{Fig:rho_first_1_arc}
\end{subfigure}\hfill
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{second_round_arc_1_worst1.png}
\caption{Plot of the worst case $\frac{\rho(\tau,\pi,\tan(\bar \alpha))}{\pi(\pi + \tan(\bar \alpha))}$, $\tau \in [1,1+\tau_1)$.}
\label{Fig:rho_first_1_arc_worst}
\end{subfigure}
\caption{Study of $\rho$ for $\tau \in [1,1+\tau_1)$.}
\label{Fig:second_round_arc_1}
\end{figure}

\medskip

{\it Case 5: $\tau \in 1 + [\tau_1,\tau_2)$.}

\noindent The solution is given by
\begin{align*}
\rho(\tau) &= S_0 (e^{\tau} - e^{\tau - 1} (\tau - 1)) + S_1 \big( e^{\tau - \tau_1} - e^{\tau - \tau_1 - 1} (\tau - \tau_1 -1) \big) + S_2 e^{\tau - \tau_2} + S_3 e^{- \bar c(2\pi + \bar \alpha)} \frac{e^{\cot(\bar \alpha) \Delta \phi} - 1}{\cot(\bar \alpha)} e^{\tau - 1} + S_4 e^{\tau - 1} \\
&= e^{\tau - 1} \bigg[ S_0 (e - (\tau - 1)) + S_1 (e^{1 - \tau_1} - e^{-\tau_1} (\tau - \tau_1 - 1)) + S_2 e^{1 - \tau_2} + S_3 e^{-\bar c(2\pi + \bar \alpha)} \frac{e^{\cot(\bar \alpha) \Delta \phi} - 1}{\cot(\bar \alpha)} + S_4 \bigg].
\end{align*}
%The term inside the bracket is linear in $\tau$, so that extreme values are taken for $\tau - 1 = \tau_1,\tau_2$: the first case has been studied in the previous point, so that we are left with the study of
%\begin{equation*}
%f(\theta,\Delta \phi) = S_0 (e - \tau_2) + S_1 (e^{1 - \tau_1} - e^{-\tau_1} (\tau_2 - \tau_1)) + S_2 e^{1 - \tau_2} + S_3 e^{-\bar c(2\pi + \bar \alpha)} \frac{e^{\cot(\bar \alpha) \Delta \phi} - 1}{\cot(\bar \alpha)} + S_4.
%\end{equation*}
%Expanding the solution about $\theta = 0$ one obtains
%\begin{align*}
%    f(\theta,\Delta \phi) &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \theta \Delta \phi \bigg( e - 1 + \frac{\Delta \phi}{2\pi + \bar \alpha} \bigg) - \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} e^{\cot(\bar \alpha) \Delta \phi} (1 + \bar c \theta) \\
%    &\quad + \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} e^{\cot(\bar \alpha \Delta \phi} - \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} \theta \frac{e^{ \cot(\bar \alpha) \Delta \phi}-1}{\cot(\bar \alpha)} + \frac{\cos(\bar \alpha)}{2\pi + \bar \alpha} \big( - 2 \cot(\bar \alpha) \theta \Delta \phi + \theta \big) + \mathcal O(\theta^2) \\
%&= \theta \Delta \phi \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \bigg( e - 1 + \frac{\Delta \phi}{2\pi + \bar \alpha} \bigg) - (1 + \bar c) \frac{\sin(\bar \alpha)}{2\pi + \bar \alpha} \frac{e^{ \cot(\bar \alpha) \Delta \phi} - 1}{\cot(\bar \alpha) \Delta \phi}- \frac{2 \cot(\bar \alpha) \cos(\bar \alpha)}{2\pi + \bar \alpha} \bigg] + \mathcal O(\theta^2).
%\end{align*}
%Hence the same considerations above applies: the quantity inside brackets is $\geq 0.568922$ (the last value is evaluate at $\Delta \phi = 0$), and in the remaining region $f$ is strictly positive.
%
A numerical evaluation shows that (see Fig. \ref{Fig:second_round_arc_2})
\begin{equation*}
\frac{\rho([1+\tau_1,1+\tau_2),\theta,\Delta \phi)}{\theta(\theta + \Delta \phi)} \geq \frac{\rho(\tau_1,\pi,\tan(\bar \alpha))}{\pi(\pi + \tan(\bar \alpha))} > 0.04.
\end{equation*}

\begin{figure}
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{second_round_arc_2.1.png}
\caption{Plot of the function $\frac{\rho(1 + (1-s) \tau_1 + s \tau_2,\theta,\Delta \phi)}{\theta (\theta + \Delta \phi)}$ for $s \in \{0,.2,.4,.6,.8,1\}$ (monotonically bottom to top graph). {\color{red} perche' e' cosi' strano sto plot?}}
\label{Fig:rho_first_2_arc}
\end{subfigure}\hfill
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{second_round_arc_2_worst1.png}
\caption{Plot of the worst case $\frac{\rho(\tau,\frac{\pi}{2},\tan(\bar \alpha))}{\frac{\pi}{2}(\frac{\pi}{2} +\tan(\bar \alpha))}$, $\tau \in [1+\tau_1,1+\tau_2)$.}
\label{Fig:rho_first_2_arc_worst}
\end{subfigure}
\caption{Study of $\rho$ for $\tau \in [1+\tau_1,1+\tau_2)$.}
\label{Fig:second_round_arc_2}
\end{figure}

\medskip

{\it Case 6: $\tau \in [1+\tau_2,2]$.}

\noindent The solution is given by 
\begin{align*}
\rho(\tau) &= S_0 (e^{\tau} - e^{\tau - 1} (\tau - 1)) + S_1 \big( e^{\tau - \tau_1} - e^{\tau - \tau_1 - 1} (\tau - \tau_1 -1) \big) + S_2 \big( e^{\tau - \tau_2} - e^{\tau - \tau_2 - 1} (\tau - \tau_2 - 1) \big) \\
& \quad + S_3 e^{- \bar c(2\pi + \bar \alpha)} \bigg( \frac{e^{\cot(\bar \alpha) \Delta \phi} - 1}{\cot(\bar \alpha)} e^{\tau - 1} - \frac{e^{\cot(\bar \alpha) \Delta \phi} \cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - 2 + \frac{\Delta \phi}{2\pi + \bar \alpha}) - e^{\cot(\bar \alpha) \Delta \phi} + e^{- \cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - 2)}}{(2\pi + \bar \alpha) \cot(\bar \alpha)^2} e^{\tau - 2} \bigg) + S_4 e^{\tau - 1}.
\end{align*}
Numerically one observes that (see Fig. \ref{Fig:second_round_arc_3})
\begin{equation*}
\frac{\rho([1+\tau_2,2),\theta,\Delta \phi)}{\theta(\theta + \Delta \phi)} \geq \frac{\rho(1+\tau_2,\pi,\tan(\bar \alpha))}{\pi(\pi + \tan(\bar \alpha))} > 0.04.
\end{equation*}

\begin{figure}
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{second_round_arc_3.1.png}
\caption{Plot of the function $\frac{\rho(1 + (1-s) \tau_2 + s,\theta,\Delta \phi)}{\theta (\theta + \Delta \phi)}$ for $s \in \{0,.2,.4,.6,.8,1\}$ (monotonically bottom to top graph).}
\label{Fig:rho_first_3_arc}
\end{subfigure}\hfill
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{second_round_arc_3_worst1.png}
\caption{Plot of the worst case $\frac{\rho(\tau,\pi,\tan(\bar \alpha))}{\pi(\pi + \tan(\bar \alpha))}$, $\tau \in [1+\tau_2,2)$.}
\label{Fig:rho_first_3_arc_worst}
\end{subfigure}
\caption{Study of $\rho$ for $\tau \in [1+\tau_2,2)$.}
\label{Fig:second_round_arc_3}
\end{figure}

\medskip

{\it Case 7: $\tau \in [2,2+\tau_1]$.}

\noindent The explicit form of the solution is
\begin{align*}
\rho(\tau) &= S_0 \bigg( e^{\tau} - e^{\tau - 1} (\tau - 1) + e^{\tau-2}\frac{(\tau - 2)^2}{2} \bigg) + S_1 \big( e^{\tau - \tau_1} - e^{\tau - \tau_1 - 1} (\tau - \tau_1 -1) \big) + S_2 \big( e^{\tau - \tau_2} - e^{\tau - \tau_2 - 1} (\tau - \tau_2 - 1) \big) \\
& \quad + S_3 \bigg[ \frac{e^{- \bar c \tau}}{\cot(\bar \alpha)} \big( e^{\cot(\bar \alpha)(2\pi + \bar \alpha) (\tau - \tau_2)} - e^{\cot(\bar \alpha) (2\pi + \bar \alpha) (\tau-1)} \big) + \frac{e^{\bar c(2\pi + \bar \alpha)(\tau-1)}}{\cot(\bar \alpha)^2 (2\pi + \bar \alpha)} \bigg( - e^{-\cot(\bar \alpha) (\tau - \tau_2 - 1)} \cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - \tau_2 - 1) \\
& \quad \qquad \qquad + e^{-\cot(\bar \alpha) (\tau - 2)} \cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - 2) + e^{\cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - \tau_2 - 1} - e^{\cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - 2)} \bigg) \bigg] \\
& \quad + S_4 \big( e^{\tau - 1} - e^{\tau-2} (\tau -2) \big) + S_5 e^{\tau-2}.
\end{align*}
Numerical evaluations show that (see Fig. \ref{Fig:third_round_arc_1})
\begin{equation*}
\frac{\rho([2,2+\tau_1),\theta,\Delta \phi)}{\theta(\theta+\Delta \phi)} \geq \frac{\rho(2,\pi,\tan(\bar \alpha))}{\pi(\pi + \tan(\bar \alpha))} > 0.04,
\end{equation*}
so that the function is positive.

\begin{figure}
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{third_round_arc_1.1.png}
\caption{Plot of the function $\frac{\rho(2 + s \tau_1,\theta,\Delta \phi)}{\theta (\theta + \Delta \phi)}$ for $s \in \{0,.2,.4,.6,.8,1\}$ (monotonically bottom to top graph).}
\label{Fig:rho_third_1_arc}
\end{subfigure}\hfill
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{third_round_arc_1_worst1.png}
\caption{Plot of the worst case $\frac{\rho(\tau,\pi,0)}{\pi(\pi + \tan(\bar \alpha))}$, $\tau \in [2,2+\tau_1)$.}
\label{Fig:rho_third_1_arc_worst}
\end{subfigure}
\caption{Study of $\rho$ for $\tau \in [2,2+\tau_1)$.}
\label{Fig:third_round_arc_1}
\end{figure}

\medskip

{\it Case 8: $\tau \in [2+\tau_1,2+\tau_2]$.}

\noindent The explicit form of the solution is
\begin{align*}
\rho(\tau) &= S_0 \bigg( e^{\tau} - e^{\tau - 1} (\tau - 1) + e^{\tau-2}\frac{(\tau - 2)^2}{2} \bigg) + S_1 \bigg( e^{\tau - \tau_1} - e^{\tau - \tau_1 - 1} (\tau - \tau_1 -1) + e^{\tau - \tau_1 - 2} \frac{(\tau - 2 - \tau_1)^2}{2} \bigg) + S_2 \big( e^{\tau - \tau_2} - e^{\tau - \tau_2 - 1} (\tau - \tau_2 - 1) \big) \\
& \quad + S_3 \bigg[ \frac{e^{- \bar c \tau}}{\cot(\bar \alpha)} \big( e^{\cot(\bar \alpha)(2\pi + \bar \alpha) (\tau - \tau_2)} - e^{\cot(\bar \alpha) (2\pi + \bar \alpha) (\tau-1)} \big) + \frac{e^{\bar c(2\pi + \bar \alpha)(\tau-1)}}{\cot(\bar \alpha)^2 (2\pi + \bar \alpha)} \bigg( - e^{-\cot(\bar \alpha) (\tau - \tau_2 - 1)} \cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - \tau_2 - 1) \\
& \quad \qquad \qquad + e^{-\cot(\bar \alpha) (\tau - 2)} \cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - 2) + e^{\cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - \tau_2 - 1} - e^{\cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - 2)} \bigg) \bigg] \\
& \quad + S_4 \big( e^{\tau - 1} - e^{\tau-2} (\tau -2) \big) + S_5 e^{\tau-2}.
\end{align*}
Numerical evaluations show that (see Fig. \ref{Fig:third_round_arc_2})
\begin{equation*}
\frac{\rho([2+\tau_1,2+\tau_2),\theta,\Delta \phi)}{\theta(\theta+\Delta \phi)} \geq \frac{\rho(2+\tau_1,\pi,\tan(\bar \alpha))}{\pi(\pi + \tan(\bar \alpha))} > 0.04,
\end{equation*}
so that the function is positive.

\begin{figure}
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{third_round_arc_2.1.png}
\caption{Plot of the function $\frac{\rho(2 + (1-s) \tau_1 + s \tau_2,\theta,\Delta \phi)}{\theta (\theta + \Delta \phi)}$ for $s \in \{0,.2,.4,.6,.8,1\}$ (monotonically bottom to top graph).}
\label{Fig:rho_third_2_arc}
\end{subfigure}\hfill
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{third_round_arc_2_worst1.png}
\caption{Plot of the worst case $\frac{\rho(\tau,\frac{\pi}{2},\tan(\bar \alpha))}{\frac{\pi}{2}(\frac{\pi}{2} + \tan(\bar \alpha))}$, $\tau \in [2+\tau_1,2+\tau_2)$.}
\label{Fig:rho_third_2_arc_worst}
\end{subfigure}
\caption{Study of $\rho$ for $\tau \in [2+\tau_1,2+\tau_2)$.}
\label{Fig:third_round_arc_2}
\end{figure}

\medskip

{\it Case 9: $\tau \in [2+\tau_2,3)$.}

\noindent The explicit form of the solution is
\begin{align*}
\rho(\tau) &= S_0 \bigg( e^{\tau} - e^{\tau - 1} (\tau - 1) + e^{\tau-2}\frac{(\tau - 2)^2}{2} \bigg) + S_1 \bigg( e^{\tau - \tau_1} - e^{\tau - \tau_1 - 1} (\tau - \tau_1 -1) + e^{\tau - \tau_1 - 2} \frac{(\tau - 2 - \tau_1)^2}{2} \bigg) \\
& \quad + S_2 \bigg( e^{\tau - \tau_2} - e^{\tau - \tau_2 - 1} (\tau - \tau_2 - 1) + e^{\tau - \tau_2 -2} \frac{(\tau - \tau_2 -2)^2}{2} \bigg) \\
& \quad + S_3 \bigg[ \frac{e^{- \bar c \tau}}{\cot(\bar \alpha)} \big( e^{\cot(\bar \alpha)(2\pi + \bar \alpha) (\tau - \tau_2)} - e^{\cot(\bar \alpha) (2\pi + \bar \alpha) (\tau-1)} \big) \\
& \quad \qquad + \frac{e^{\bar c(2\pi + \bar \alpha)(\tau-1)}}{\cot(\bar \alpha)^2 (2\pi + \bar \alpha)} \bigg( - e^{-\cot(\bar \alpha) (\tau - \tau_2 - 1)} \cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - \tau_2 - 1) + e^{-\cot(\bar \alpha) (\tau - 2)} \cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - 2) \\\
& \quad \qquad \qquad + e^{\cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - \tau_2 - 1} - e^{\cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - 2)} \bigg) \\
& \quad \qquad + \frac{e^{\bar c(2\pi + \bar \alpha)(\tau-2)}}{\cot(\bar \alpha)^3 (2\pi + \bar \alpha)^2} \bigg( e^{-\cot(\bar \alpha) (\tau - \tau_2 - 2)} \frac{(\cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - \tau_2 - 2))^2}{2} - e^{-\cot(\bar \alpha) (\tau - \tau_2 - 2)} (\cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - \tau_2 - 2)) \\
& \quad \qquad \qquad + e^{\cot(\bar \alpha) (2\pi + \bar \alpha) (\tau - \tau_2 - 2)} - 1 \bigg) \bigg] \\
& \quad + S_4 \big( e^{\tau - 1} - e^{\tau-2} (\tau -2) \big) + S_5 e^{\tau-2}.
\end{align*}
Numerical evaluations show that (see Fig. \ref{Fig:third_round_arc_3})
\begin{equation*}
\frac{\rho([2+\tau_2,3),\theta,\Delta \phi)}{\theta(\theta+\Delta \phi)} \geq \frac{\rho(3,\pi,\tan(\bar \alpha))}{\pi(\pi+ \tan(\bar \alpha))} > 0.04,
\end{equation*}
so that the function is positive.

\begin{figure}
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{third_round_arc_3.1.png}
\caption{Plot of the function $\frac{\rho(2 + (1-s) \tau_2 + s,\theta,\Delta \phi)}{\theta (\theta + \Delta \phi)}$ for $s \in \{0,.2,.4,.6,.8,1\}$ (monotonically bottom to top graph).}
\label{Fig:rho_third_3_arc}
\end{subfigure}\hfill
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{third_round_arc_3_worst1.png}
\caption{Plot of the worst case $\frac{\rho(\tau,\frac{\pi}{2},\tan(\bar \alpha))}{\frac{\pi}{2}(\frac{\pi}{2} + \tan(\bar \alpha))}$, $\tau \in [2+\tau_2,3)$.}
\label{Fig:rho_third_3_arc_worst}
\end{subfigure}
\caption{Study of $\rho$ for $\tau \in [2+\tau_2,3)$.}
\label{Fig:third_round_arc_3}
\end{figure}

\medskip

{\it Case 10: $\tau \geq 3$.}

It is enough to find the region where 
\begin{equation*}
\rho(\tau) - \rho(\tau-1) \geq 0
\end{equation*}
and apply Lemma \ref{lem:key}. Numerically it can be shown that (see Fig. \ref{Fig:fourth_round_arc})
\begin{equation*}
\frac{\rho(\tau,\theta,\Delta \phi) - \rho(\tau,\theta,\Delta \phi)}{\theta(\theta + \Delta \phi)} \geq 10^{-4}
\end{equation*}
for
\begin{equation*}
(\theta,\Delta \phi) \in (0,\pi] \times [0,\tan(\bar \alpha)] \setminus (3.12,\pi) \times (2.37,\tan(\bar \alpha)).
\end{equation*}

\begin{figure}
\begin{subfigure}{.32\linewidth}
\includegraphics[width=\linewidth]{fourth_round_arc_variation1.png}
\caption{Plot of the function $\frac{\rho(\tau,\theta,\Delta \phi)-\rho(\tau-1,\theta,\Delta \phi)}{\theta (\theta + \Delta \phi)}$ for $\tau \in \{3,3.2,3.4,3.6,3.8,4\}$.}
\label{Fig:rho_fourth_1_arc}
\end{subfigure}\hfill
\begin{subfigure}{.32\linewidth}
\includegraphics[width=\linewidth]{fourth_round_arc_variation_2.1.png}
\caption{Close-in of the previous graph near the negativity region $(\theta,\Delta \phi) \in (\pi,\tan(\bar \alpha)) + (-.4,0) \times (-4,0)$.}
\label{Fig:rho_fourth_2_arc}
\end{subfigure} \hfill
\begin{subfigure}{.32\linewidth}
\includegraphics[width=\linewidth]{fourth_round_arc_variation_3.1.png}
\caption{Plot of the worst case $\frac{\rho(3,\theta,\Delta \phi)}{\theta(\theta + \Delta \phi)}$ near the negativity region.}
\label{Fig:rho_fourth_3_arc}
\end{subfigure}
\caption{Study of $\rho$ for $\tau \in [3,4)$.}
\label{Fig:fourth_round_arc}
\end{figure}
The application of Lemma \ref{lem:key} concludes the proof.

\medskip

{\it Asymptotic behavior.}

\begin{figure}
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{asympt_arc1.png}
%\caption{Plot of the function $\frac{\rho(2 + (1-s) \tau_2 + s,\theta,\Delta \phi)}{\theta (\theta + \Delta \phi)}$ for $s \in \{0,.2,.4,.6,.8,1\}$ (monotonically bottom to top graph).}
%\label{Fig:asympt_arc1}
\end{subfigure}\hfill
\begin{subfigure}{.475\linewidth}
\includegraphics[width=\linewidth]{asympt_arc2.1.png}
%\caption{Plot of the worst case $\frac{\rho(\tau,\frac{\pi}{2},\tan(\bar \alpha))}{\frac{\pi}{2}(\frac{\pi}{2} + \tan(\bar \alpha))}$, $\tau \in [2+\tau_2,3)$.}
%\label{Fig:asympt_arc2}
\end{subfigure}
\caption{Plot of the function \ref{Equa:asympt_arc}, and a blowup about the negativity region.}
\label{Fig:asympt_arc}
\end{figure}

Using Lemmata \ref{Lem:aympt_g} and \ref{Lem:m_aymptotic} we obtain
\begin{equation}
\label{Equa:asympt_arc}
\lim_{\tau \to \infty} \frac{\rho(\tau) e^{-\bar c \tau}}{\tau \theta(\theta + \Delta \phi)} = \frac{2}{\theta ( \theta+ \Delta \phi)} \bigg( S_0 + S_1 + S_2 + S_3 \frac{e^{-\bar c (2\pi + \bar \alpha) \tau_2} - e^{-\bar c(2\pi + \bar \alpha)}}{\bar c} + S_4 + S_5 \bigg).
\end{equation}
A plot of this function is in Fig. \ref{Fig:asympt_arc}.
\end{proof}

%\begin{remark}
%\label{Rem:study_f1_over}
%When studying the perturbations of the optimal solutions in the next section, it will be necessary to study the function $f_1(\theta,\Delta \phi)$ for angles up to $\hat  \theta + \frac{\pi}{2}$: numerically one see that in the additional strip $[\frac{\pi}{2},\frac{\pi}{2} + \hat \theta] \times [0,\tan(\bar \alpha)]$ the function is strictly positive, with minimal value $> 4$, see Fig. \ref{Fig:f1_funct_over}.
%
%\begin{figure}
%\resizebox{.75\textwidth}{!}{\includegraphics{f1_funct_over.png}}
%\caption{The additional strip for the function $f_1(\theta,\Delta \phi)$, Remark \ref{Rem:study_f1_over}.}
%\label{Fig:f1_funct_over}
%\end{figure}
%\end{remark}



\subsubsection{Estimate on the length for the fastest saturated spiral $\delta r(\phi;s_0)$, arc case}
\label{Sss:additional_estim_opt_arc}


We will repeat some of the estimates for the functional 
\begin{equation*}
\delta \tilde r(\phi;s_0) - 2.08 \delta \tilde L(\phi;s_0), \quad \phi \geq \phi_0 + \Delta \phi + \frac{\pi}{2} + 2\pi.
\end{equation*}
Using computations similar to Section \ref{Sss:additional_estim_opt_segm} we obtain
\begin{equation}
\label{Equa:length_arc}
\begin{split}
\delta \tilde L(\phi;s_0) &= \frac{1 - \cos(\theta) + \sin(\theta) \Delta \phi}{\sin(\bar \alpha)^2} \\
& \quad + \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \left( 1 - \cos(\theta) + \Delta \phi \sin(\theta) \right) \mathcal G \bigg( \phi - \phi_0 - \Delta \phi - \frac{\pi}{2} + \bar \alpha \bigg) - \mathcal G(\phi - \phi_0 - 2\pi - \theta_0) \\
& \quad + \cos(\theta) \mathcal G \bigg( \phi - \phi_0 - 2\pi - \frac{\pi}{2} \bigg) - \sin(\theta) (2\pi+\bar \alpha) \bigg( \mathfrak G \bigg( \phi - \phi_0 - 2\pi - \frac{\pi}{2} \bigg) - \mathfrak G \bigg( \phi - \phi_0 - 2\pi - \frac{\pi}{2} - \Delta \phi \bigg) \bigg)  \\
& \quad + \bigg( - \cot(\bar \alpha)^2 \big( 1 - \cos(\theta) + \Delta \phi \sin (\theta) \big) + \cot(\bar \alpha) \big( \sin(\theta) - \cot(\bar \alpha) (1 - \cos(\theta) + \Delta \phi \sin(\theta)) \big) \bigg) \mathcal G \bigg( \phi -\phi_0 - 2\pi - \Delta \phi - \frac{\pi}{2} \bigg) \\
& \quad + \big( \sin(\theta) - \cot(\bar \alpha) (1 - \cos(\theta) + \Delta \phi \sin(\theta)) \big) H(\phi - \phi_0 + 2\pi + \frac{\pi}{2} + \Delta \phi) \\
& \quad - \frac{1}{\sin(\bar \alpha)} \big( \sin(\theta) - \cot(\bar \alpha) (1 - \cos(\theta) + \Delta \phi \sin(\theta)) \big) \mathcal G \bigg( \phi - \phi_0 - 2\pi - \Delta \phi - \frac{\pi}{2} - 2\pi  - \bar \alpha \bigg),
\end{split}
\end{equation}
where we have used \eqref{Equa:Mint_frakG} and \eqref{Equa:Deltar_arc} for the first term
\begin{equation*}
1 - \cos(\theta) + \sin(\theta) \Delta \phi + r(\phi_1) \delta \phi_1 + \delta |P_2 - P_1| - \frac{r(\phi_2) \delta \phi_2}{\sin(\bar \alpha)} = \frac{1 - \cos(\theta) + \sin(\theta) \Delta \phi}{\sin(\bar \alpha)^2}.
\end{equation*}

For $\phi \geq \phi_0 + 2\pi + \Delta \phi + \frac{\pi}{2} + 2\pi + \bar \alpha$, the RDE satisfied by $\delta \tilde L$ is
\begin{align*}
\frac{d}{d\phi} \delta \tilde L(\phi) &= \cot(\bar \alpha) \delta \tilde L(\phi) - \frac{\delta \tilde L(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} + S_L,
\end{align*}
with
\begin{align*}
S_L &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)^2} \left( 1 - \cos(\theta) + \Delta \phi \sin(\theta) \right) - \frac{1}{\sin(\bar \alpha)} + \frac{\cos(\theta)}{\sin(\bar \alpha)} - \frac{\sin(\theta) \Delta \phi}{\sin(\bar \alpha)} \\
& \quad + \frac{1}{\sin(\bar \alpha)} \bigg( - \cot(\bar \alpha)^2 \big( 1 - \cos(\theta) + \Delta \phi \sin (\theta) \big) + \cot(\bar \alpha) \big( \sin(\theta) - \cot(\bar \alpha) (1 - \cos(\theta) + \Delta \phi \sin(\theta)) \big) \bigg) \\
& \quad - \frac{1}{\sin(\bar \alpha)^2} \big( \sin(\theta) - \cot(\bar \alpha) (1 - \cos(\theta) + \Delta \phi \sin(\theta)) \big) \\
&= - (1 - \cos(\theta) + \sin(\theta) \Delta \phi) \frac{(1 - \cos(\bar \alpha))^2}{\sin(\bar \alpha)^3} + \sin(\theta) \frac{\cos(\bar \alpha) - 1}{\sin(\bar \alpha)^2} < 0.
\end{align*}
Hence the RDE for $\delta \tilde r - 2.08 \delta \tilde L$ is
\begin{equation*}
\frac{d}{d\phi} (\delta \tilde r(\phi) - 2.08 \delta \tilde L(\phi)) > \cot(\bar \alpha) (\delta \tilde r(\phi) - 2.08 \delta \tilde L(\phi)) - \frac{\delta \tilde r(\phi - 2\pi - \bar \alpha) - 2.08 \delta \tilde L(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)}
\end{equation*}
for $\phi \geq \phi_0 + 2\pi + \Delta \phi + \frac{\pi}{2} + 2\pi + \bar \alpha$. We can thus apply Lemma \ref{lem:key} and Remark \ref{rmk:exponentially:explod} {\color{red} ancora questo remark} if we can show numerically that the function is positive and strictly increasing for $\tau \in [4,5]$.

\begin{figure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\includegraphics{Lpert_arc1.png}}
\end{subfigure} \hfill
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\includegraphics{Lpert_arc2.png}}
\end{subfigure} \hfill
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\includegraphics{Lpert_arc3.png}}
\end{subfigure}
\caption{Numerical plots of the function $\frac{\rho(\tau) - e^{-\bar c (2\pi + \bar \alpha) \tau} \delta \tilde L(\tau)}{\theta(\theta + \Delta \phi)}$: the fist 5 rounds, the minimal values for $\theta = \frac{\pi}{2}, \Delta \phi = 0$, and its derivative for $\tau \in [4,5]$.}
\label{Fig:Lpert_arc}
\end{figure}

A numerical plot of the function $\rho(\tau) - 2.08 e^{-\bar c (2\pi + \bar \alpha) \tau} \delta L(\tau)$, $\phi = \phi_0 + \Delta \phi + \frac{\pi}{2} - \bar \alpha$, is in Fig. \ref{Fig:Lpert_arc}: it is shown that the function is positive, increasing for $\tau \in [4,5]$ and its minimal value {\color{red} che vuoi dire qua?}: by Lemma \ref{lem:key} we conclude that

\begin{proposition}
\label{Prop:lemgth_arc_pert}
It holds for the perturbation in the arc case
\begin{equation*}
{\color{red}\delta?}\rho(\tau) - 2.08 e^{-\bar c (2\pi + \bar \alpha) \tau} \delta \tilde L(\tau) \geq 0.27 e^{\bar c (2\pi + \bar \alpha) \tau} \theta(\theta + \Delta \phi), \quad \tau \geq 1.
\end{equation*}
\end{proposition}


\subsection{A bound for the length of a spiral}
\label{Ss:bound_lenth}


We can put Propositions \ref{Prop:lemgth_segm_pert} and \ref{Prop:lemgth_arc_pert} together, obtaining the following

\begin{corollary}
\label{Cor:bound_length_gen}
Consider the spiral $\tilde r(\phi;\phi_0)$: if
$$
\phi \geq \begin{cases}
\phi_0 + \bar \theta + 2\pi & \text{segment case}, \\
\phi_0 + \Delta \phi + \frac{\pi}{2} + 2\pi & \text{arc case},
\end{cases}
$$
then
\begin{equation*}
\tilde r(\phi) - 2.08 \tilde L(\phi - 2\pi - \bar \alpha) \geq r(\phi) - 2.08 L(\phi - 2\pi - \bar \alpha) > 0.67 e^{\bar c(\phi - \tan(\bar \alpha) - \frac{\pi}{2} + \bar \alpha)},
\end{equation*}
\end{corollary}

\begin{proof}
We can write
\begin{align*}
\tilde r(\phi) - 2.08 \tilde L(\phi - 2\pi - \bar \alpha) &= r(\phi) - 2.08 L(\phi - 2\pi - \bar \alpha) + \int_0^{\phi_0} \delta \tilde r(\phi;s_0) - 2.08 \delta \tilde L(\phi - 2\pi - \bar \alpha;s_0) ds_0 \\
&\geq r(\phi) - 2.08 L(\phi - 2\pi - \bar \alpha). \qedhere
\end{align*}
\end{proof}


%
%{\color{blue} QUESTO FORSE NON SERVE}
%
%$PT(\tau)$ in the arc case: recall that
%\begin{equation*}
%%\label{Equa:PT_tau}
%PT(\tau) = e^{\bar c(2\pi + \bar \alpha) \tau} \bigg( \rho(\tau) - \frac{(1 - \cos(\hat \theta)) e^{-\bar c(2\pi + \bar \alpha)}}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \rho(\tau - 1) \bigg).
%\end{equation*}
%Numerically one observes that for $\tau \in [1,4]$ (see Fig. \ref{Fig:PTarc_1}) %the minimal value is
%\begin{equation}
%\label{Equa:PTarc_1}
%\frac{PT(\tau)}{\theta(\theta + \Delta \phi)} \geq \frac{PT(1)}{\frac{\pi}{2}(\frac{\pi}{2} + \tan(\bar \alpha)} > 0.39.
%\end{equation}
%
%\begin{figure}
%\begin{subfigure}{.475\textwidth}
%\resizebox{\textwidth}{!}{\includegraphics{PTarc_1.1.png}}
%\end{subfigure} \hfill
%\begin{subfigure}{.475\textwidth}
%\resizebox{\textwidth}{!}{\includegraphics{PTarc_1.2.png}}
%\end{subfigure}
%\caption{Plot of the function \eqref{Equa:PTarc_1} and of its worst case $\theta = \frac{\pi}{2}$.}
%\label{Fig:PTarc_1}
%\end{figure}
%
%Moreover it is increasing for $[\tau \in [3,4]$ (see Fig. \ref{Fig:PTarc_2}),
%\begin{equation}
%\label{Equa:PTarc_2}
%\frac{PT(4) - PT(\tau)}{\theta (\theta + \Delta \phi) (4 - \tau)} > 0.19.
%\end{equation}
%
%\begin{figure}
%\begin{subfigure}{.475\textwidth}
%\resizebox{\textwidth}{!}{\includegraphics{PTarc_2.1.png}}
%\end{subfigure} \hfill
%\begin{subfigure}{.475\textwidth}
%\resizebox{\textwidth}{!}{\includegraphics{PTarc_2.2.png}}
%\end{subfigure}
%\caption{Plot of the function \eqref{Equa:PTarc_2} and its worst case $\theta = \frac{\pi}{2}$.}
%\label{Fig:PTarc_2}
%\end{figure}
%
%We thus conclude that
%
%\begin{proposition}
%\label{Prop:PT_pso_arc_case}
%The function $PT(\tau)$ is positive for all $\tau \geq 1$ for the arc case, with $\theta \in [0,\frac{\pi}{2}]$ and $\Delta \phi \in [0,\tan(\bar \alpha)]$.
%\end{proposition}
%
%{\color{red} FORSE NON SERVE
%
%
%
%The length can be thus computed by
%\begin{equation}
%\label{Equa:Lenght_arc}
%\begin{split}
%\delta L(\tau) &= S_0 \big( \mathfrak g(\tau + \hat \tau - 1) - \mathfrak g(\tau - 1) \big) + S_1 e^{\bar c (2\pi + \bar \alpha) \tau_1} \big( \mathfrak g(\tau + \hat \tau - 1 - \tau_1) - \mathfrak g(\tau - 1 - \tau_1) \big) \\
%& \quad + S_2 e^{\bar c (2\pi + \bar \alpha) \tau_2} \big( \mathfrak g(\tau + \hat \tau - 1 - \tau_2) - \mathfrak g(\tau - 1 - \tau_2) \big) + S_3 (2\pi + \bar \alpha) \big( \mathfrak G(\tau - 1 - \tau_2) - \mathfrak G(\tau - 2) \big) \\
%& \quad + S_4 e^{\bar c (2\pi + \bar \alpha)} \big( \mathfrak g(\tau + \hat \tau - 2) - \mathfrak g(\tau - 2) \big) + \frac{D e^{\bar c (2\pi + \bar \alpha)}}{\sin(\bar \alpha)} \ind_{[2-\hat \tau,2)}(\tau) \\
%& \quad + S_5 e^{2 \bar c (2\pi + \bar \alpha)} \big( \mathfrak g(\tau + \hat \tau - 3) - \mathfrak g(\tau - 3) \big).
%\end{split}
%\end{equation}
%
%}

==> intro.tex <==
\section{Introduction}
\label{S:intro}


We study a dynamic blocking problem first proposed by A. Bressan in \cite{Bressan_2007}. The problem is concerned with the model of wild fire spreading in a region of the plane $\R^2$ and the possibility to block it by constructing \emph{barriers}, i.e. rectifiable curves which cannot be crossed by the fire. The local fire spreading is described by giving a set valued function
$$
F : \R^2 \to \big\{ K \subset \R^2 \ \text{compact, closed} \big\}.
$$
such that
\begin{enumerate}
\item there exists $r>0$ such that $B_r(0)\subset F(x)\quad\forall x\in\R^2$;
%\item $F(x)$ is compact and convex $\forall x   \in\R^2$;
\item $x\rightarrow F(x)$ is Lipschitz-continuous in the Hausdorff topology.
\end{enumerate}
This function represents the infinitesimal fire evolution when barriers are not present, i.e. $x + \delta t F(x)$ are the points reached by the fire in the infinitesimal time $\delta t$. In other words, if barriers are not present, the \emph{reachable set $R(t)$} is the solution to the differential inclusion
\begin{equation*}
R(t) = \Big\lbrace x(t), \quad x(\cdot) \text{ abs. cont.},\ x(0) \in R_0,\ \dot x(\tau)\in F(x(\tau))\text{ for a.e. }\tau\in[0,t] \Big\rbrace,
\end{equation*}
where the set $R_0\subset\R^2$ is the open region burnt by the fire at the initial time $t=0$.

%
%
%representing the local speed of the fire at the point $x$
%
%If we denote by $R(t)\subset\R^2$ the region burned by the fire at time $t$, then we can describe it as the reachable set for a differential inclusion. More precisely, one considers the Cauchy Problem
%\begin{equation*}
%    \dot{x}\in F(x),\qquad x(0)\in R_0,
%\end{equation*}
%, while the function $F$ describes the speed of spreading of the fire. The set $R_0\subset\R^2$ is assumed to be open, bounded, non-empty and connected with Lipschitz boundary, whereas the standard assumptions on $F:\R^2\rightarrow \R^2$, which is a Lipschitz-continuous multifunction, are:
%\begin{enumerate}
%    \item there exists $r>0$ such that $B_r(0)\subset F(x)\quad\forall x\in\R^2$;
%    \item $F(x)$ is compact and convex $\forall x   \in\R^2$;
%    \item $x\rightarrow F(x)$ is Lipschitz-continuous in the Hausdorff topology. 
%\end{enumerate}
%\noindent If no barriers are present 

When the fire starts spreading, a fireman can construct some barriers, modeled by a one-dimensional rectifiable set $\zeta\subset\R^2$, in order to block the fire. More in detail, we consider a continuous function $\psi: \R^2 \rightarrow \R^+$ together with a positive constant $\psi_0>0$ such that $\psi\geq\psi_0$. If we denote by $\zeta(t)\subset\R^2$ the portion of the barrier constructed within the time $t\geq 0$, we say that  $\zeta$ is an admissible barrier (or admissible strategy) if
\begin{enumerate}
\item{(H1)}\label{admissibility:con:1} $\zeta(t_1)\subset \zeta(t_2)$, $\forall  t_1\leq t_2$;
\item{(H2)}\label{admissibility:con:2} $\int_{\zeta(t)}\psi d\H^1\leq t,\quad \forall t\geq 0$,
\end{enumerate}
where $\H^1$ denotes the one-dimensional Hausdorff measure. Once we have an admissible strategy $\zeta$, then we define the reachable set for $\zeta$ at time $t$ the set
\begin{equation}\label{def:reach:set}
R^\zeta(t) = \Big\lbrace x(t): x\text{ abs. cont.},\ x(0) \in R_0, \ \dot x(\tau)\in F(x(\tau))\text{ for a.e. } \tau\in[0,t],\ x(\tau)\not\in\zeta(\tau) \ \forall\tau\in[0,t] \Big\rbrace.
\end{equation}

\begin{definition}
Let $t\rightarrow\zeta(t)$ be an admissible strategy. We say that it is a \emph{blocking} strategy if
\begin{equation*}
R^\zeta_\infty\doteq\bigcup_{t\geq 0} R^\zeta(t)
\end{equation*}
is a bounded set.
\end{definition}

We call \emph{isotropic} the case in which the fire is assumed to propagate with unit speed in all directions, while the barrier is constructed at a constant speed $\sigma>0$, namely
\begin{equation}
\label{isotropic case}
F \equiv \overline{B_1(0)},\quad R_0=B_1(0), \quad \psi\equiv\frac{1}{\sigma},
\end{equation}
where $\overline{B_1(0)}$ denotes the closure of the unit ball of the plane centered at the origin. We remark that in \cite{Bressan_friends} there are comparison results between more general choices of the data $R_0$ and $F$ and the isotropic problem for the study of the fire problem in a more general setting. 

The existence of admissible blocking (or winning) strategies for the isotropic blocking problem is a very challenging open problem and it has been addressed mainly in \cite{Bressan_2007},\cite{Bressan_friends}.\footnote{One can prove that the existence of blocking strategy does not depend on the starting set $R_0$ but only on the speed $\sigma$ \cite{Bressan_survey}.} In particular, the following theorems hold:

\begin{theorem}
\label{thm:existence:2}
Assume that \eqref{isotropic case} hold. Then if $\sigma>2$ there exists an admissible blocking strategy.
\end{theorem}

\begin{theorem}
\label{thm:nonexistence:1}
Assume that \eqref{isotropic case} hold. Then if $\sigma\leq 1$ no admissible blocking strategy exists.
\end{theorem}

\noindent The two theorems are proved in  \cite{Bressan_2007} and they motivate the following Fire Conjecture \cite{Bressan_conj}:
\begin{conjecture}
\label{conj:bressan}
Let \eqref{isotropic case} hold. Then if $\sigma\leq 2$ no admissible blocking strategy exists.
\end{conjecture}
\noindent For a survey of results related to the previous conjecture, see \cite{Bressan_survey}.

\medskip

\noindent \textbf{Equivalent formulation.} Throughout the paper we will use the following equivalent formulation of the dynamic blocking problem for the isotropic case (for a proof of the equivalence, see \cite{Bressan_equivalent}): let $Z\subset\R^2$ be a rectifiable set. We denote by
\begin{equation}
\label{eq:burned:region_intro}
R^Z(t) = \Big\lbrace  x(t): x\text{ abs. cont.},\ \dot x(\tau) \in \overline{B_1(0)} \text{ for a.e. } \tau \in [0,t],\ x(\tau)\not\in Z \ \forall \tau \in[0,t] \Big\rbrace.
\end{equation}
We say that the strategy $Z$ is \emph{admissible} if $\forall t\geq 0$
\begin{equation}
\H^1(Z\cap\overline{R^Z(t)})\leq\sigma t.
\end{equation}
Similarly to the previous formulation we denote by
\begin{equation}
\label{eq:burned:region}
R^Z_\infty = \bigcup_{t\geq 0} R^Z(t)
\end{equation}
the burned region and we say that $Z$ is an admissible blocking strategy if $R^Z_\infty$ is bounded. The advantage of this description is that the barrier is fixed and it does not grow while the time evolves. Here we can interpret $Z \cap \overline{R^Z(t)}$ as the amount of barrier $Z$ burned by the fire within the time $t$.

\medskip

\noindent \textbf{Minimum time function and Hamilton-Jacobi formulation.} The propagation of fire can be described also in terms of the minimum time function
\begin{equation}\label{eq:min:time:function}
u(x) \doteq \inf \big\lbrace t \geq 0:\ x \in \overline{R^Z(t)} \big\rbrace.
\end{equation}
The function $u$ is the time needed for the fire to reach the point $x$ in the burned region, without crossing the barrier. The minimum time function can be computed by solving an Hamilton-Jacobi equation with obstacles, namely
\begin{equation}
\label{eq:hamilton:jacobi}
\begin{cases}
|\nabla u(x)|\leq 1 \qquad x\not\in Z, \\
u(x)=0 \qquad x\in R_0.
\end{cases}
\end{equation}
For the properties of the solution of \eqref{eq:hamilton:jacobi} we refer to \cite{delellisrobyr}. We conjecture that $|\nabla u(x)|=1$ for every $x\not\in Z$ as in the classic case of Eikonal equation without obstacle. Given the minimum time function $u$, and an admissible barrier $Z$, one defines the following \emph{Admissibility Functional}
\begin{equation*}
\mathcal A(x) = u(x) - \frac{1}{\sigma} \H^1 \big( Z\cap\overline{R^Z(u(x))} \big) \geq 0, \quad \forall x \in Z.
\end{equation*}
The inequality follows by the admissibility of the barrier $Z$.
In particular, one defines the \emph{saturated set} as
\begin{equation*}
\mathcal{S} = \big\lbrace x \in Z:\ \mathcal A(x) = 0 \big\rbrace,
\end{equation*}
corresponding to those points on the barrier where the firefighters are using all the barrier available in order to block the fire.

One can easily prove that if the strategy $Z$ consists of a simple closed curve, then it is not admissible for $\sigma\leq 2$ \cite{Bressan_2007} (the key idea is taking the last point $P$ on the curve reached by the fire and observing that $\mathcal{A}(P)<0$), but only partial results are present in the literature if the strategy has more complicated structures, as for example the presence of internal barriers that slow down the fire.
\medskip

%One possible idea to prove the conjecture would be to investigate the shape of a strategy which is \emph{optimal} among admissible strategies, allowing for the presence of some internal barriers. 

\noindent \textbf{Optimization problem}. An optimization problem among blocking barriers can be given as follows: one introduces the following cost functional
\begin{equation}\label{eq:opt:problem}
    J(Z)=\int_{R^Z_\infty} \kappa_1 d\mathcal{L}^2 +\int_{Z}\kappa_2 d\H^1,
\end{equation}
among all possible admissible blocking strategies, where $\kappa_1,\kappa_2:\R^2\rightarrow \R^+$ are two non-negative continuous functions. In \cite{Bressan_deLellis} it is proved that, if the class of admissible blocking strategies is non-empty, then there exists an optimal strategy. Moreover, there exists an optimal strategy $Z^*$ which is \emph{complete}:
\begin{definition}
Let $Z\subset\R^2$ be a rectifiable set. $Z$ is complete if it contains all its points of positive upper density,  that is, let $x\in\R^2$ such that
\begin{equation*}
\limsup_{r\to 0^+} \frac{\H^1(Z\cap B_r(x))}{2r}>0 \Longrightarrow x\in Z.
\end{equation*}
\end{definition}
 The following corollary also holds \cite{Bressan_equivalent}:
\begin{corollary}
If there exists an admissible blocking strategy $Z$ with $\H^1(Z)<\infty$, then there exists an optimal blocking strategy $Z^*$ such that
\begin{equation*}
Z^* = \bigg( \bigcup_i Z_i \bigg) \cup \mathcal{N},
\end{equation*}
where $Z_i$ are countably many compact rectifiable connected components and $\H^1(\mathcal{N})=0$.
\end{corollary}
We mention also the recent result in \cite{Bressan_Chiri} where it is proved that the optimal strategy is nowhere dense. What really maked the optimization problem hard is that the class of admissible strategy could be empty (and it is conjectured to be empty if $\sigma\leq 2$ \ref{conj:bressan}).

Giving necessary conditions for optimality is a hard open problem. Some necessary optimality conditions are derived in \cite{Bressan_optnec} assuming further regularity on the optimal strategy. In \cite{FireSegment} there are given some necessary optimality condition that characterize the boundary $\partial R^Z_\infty$ in the case $Z$ is an optimal strategy (for the problem $\kappa_1=0$, $\kappa_2=1$) without assuming any regularity assumption on the barrier. There, some properties of the optimal barrier are derived, as the connectedness in the case the $Z=Z^2\cup Z^1$ where $Z^2=\partial R^Z_\infty$ and $Z^1$ is a single internal curve, and some concrete cases are analyzed. The major issue, however, remains deriving necessary conditions for internal barriers.


\subsection{Non admissibility of spiral-like strategies}
\label{Ss:spiral_intro}


In this paper we study spiral-like strategies: namely, admissible barriers that are constructed putting all the effort on a single curve. The study of spiraling strategies is of key importance in the  complete solution of Bressan's Fire conjecture, indeed there is a strongly belief that these strategies are the "best" possible barriers that can be constructed when $\sigma\leq 2$. The heuristic reason is that, if $\sigma\leq 2$, then we can not have two firefighters (constructing therefore two branches of a strategy) with speed strictly greater than the speed of the fire so that they will be engulfed by the fire: thus the best strategy should be a single curve. The case $\sigma>2$ is different, indeed we expect that the optimal strategies in this case are simple closed curves. In \cite{Bressan_isotropic} the authors construct the best strategy for the optimization problem \ref{eq:opt:problem} among simple closed curves.

We start giving the definition of spiral strategies.

\begin{definition}[Spiral strategies]
\label{Def:spiral_barrier_intro}
Let $Z = \zeta([0,S]) \subset \R^2$ be a strategy, where $\zeta$ is a Lipschitz curve parametrized by arc-length. We say that it is a \emph{spiral strategy} if it satisfies:
\begin{enumerate}
\item $\zeta(0) = (1,0)$ and $\zeta \rest_{[0,S)}$ is simple,
\item $s \mapsto u(\zeta(s))$ is increasing,
\item $\zeta$ is locally convex, i.e. locally it is the graph of a convex function,
\item \label{Point:4_intro_def_spiral} it holds
\begin{equation*}
%\text {(A1)} \qquad 
0 \leq \angle (\textbf{t}^+(0),\textbf{e}_2)\leq \frac{\pi}{2},
\end{equation*}
\end{enumerate}
The spiral $\zeta$ is \emph{admissible} if it is also an admissible barrier.
\end{definition}

The assumptions that $\zeta$ is locally convex yields a direction of rotation to the curve, and then Point \eqref{Point:4_intro_def_spiral} above implies that $\zeta$ is rotating counterclockwise about $0$, at least for some interval $s \in [0,\bar s_2]$ (see Proposition \ref{thm:param_1} for the precise definition of the values $\bar s_2$).

%
%Finally, we say that $Z$ is an admissible spiral if it is a spiral-like strategy,   the curve is locally convex, in the sense of Definition \ref{def:convexity:spiral} and moreover it satisfies the following assumption
%
%where $\textbf{e}_2$ is the vertical vector of the canonical base  $\mathbf t(0)$ is the tangent vector of the spiral in the starting point (commonly $(1,0)$) and $\angle$ denotes the angle between the two vectors. 

A deeper discussion is needed for the assumption %requirement
\begin{equation*}
s \rightarrow u\circ\zeta(s) \quad \text{ is increasing},
\end{equation*}
which corresponds to the fact that either a portion of the barrier lies on the level set $\lbrace u=t\rbrace$ (so that the previous function is constant), or the fire can not burn two portions of the barrier simultaneously. This means that the barrier $\zeta(\{s \geq \bar s\})$ depends only on the time function $u$ constructed with $\zeta([0,\bar s])$ is place, and we do not need to compensate part of $\zeta([0,\bar s])$ which will be reached by fire at a later time: in particular, given the barrier up to time $\bar t$ (or equivalently length $\bar s$), we can ask which is the optimal barrier for a given optimization problem with the same freedom as for the initial problem. This final observation will be fundamental in our homotopy argument.


%We believe instead that the hypothesis of local convexity and the assumption $(A1)$ are automatically satisfied by \emph{optimal} spiral-like strategies, which is an open question. 
%\medskip
%
%In addition to the parametrization by arc-length, it is possible to parametrize any admissible spiral by $(r(\phi),\phi)$, where $\phi$ denotes the angle of rotation on the spiral, which is defined in Lemma \ref{lem:ODE:spiral}, while $r(\phi)$ represents the length of the final segment of the fire ray reaching the point $(r(\phi),\phi)$, as explained in Figure \ref{fig:param:spiral} (see Theorem \ref{thm:param}).

\medskip

The only results known on this family of barriers can be found in \cite{Bressan_friends} and \cite{firefighter}. In the two papers it is proved independently and with different techniques the following result:

\begin{theorem}
\label{bressan,klein}
Let $\sigma > 2.6144..$ (critical speed). Then there exists a spiral-like strategy which confines the fire.
\end{theorem}

The proof of this result is obtained by the study of a particular spiral, that we will call \emph{saturated spiral}. Let $S$ be an admissible spiral. We say that $Z$ is a saturated spiral if
\begin{equation}
\label{eq:sat:spir:def}
\mathcal{S}(Z) = \big\lbrace t \in[0,T]:\ \H^1 \big( Z \cap \overline{R^S(t)} \big) = \sigma t \big\rbrace = [0,T].
\end{equation}
In terms of the admissibility functional previously defined, every point $P$ on a saturated spiral is \emph{saturated}, that is $\mathcal{A}(P)=0$.

Saturated spirals (or portions of it) are thought to be building blocks for optimal strategies. Indeed, it has been proved in \cite{Bressan_isotropic} that, if $\sigma>2$, the optimal strategy (that minimizes the cost functional \eqref{eq:opt:problem}) among simple closed curves is made by an arc of circle and two branches of saturated logarithmic spirals in polar coordinates. As we will see, there are intimate relations between logarithmic spirals and saturated spirals. Also, in \cite{FireSegment}, it is proved that for $\sigma<2$, if a strategy $Z$ is optimal ($\kappa_1=0,\kappa_2=1$) and its internal barrier is a segment, then the boundary $\partial R^Z_\infty$ is the union of a segment and a branch of logarithmic spiral.

The proof of Theorem \ref{bressan,klein} relies on the following fact: a saturated spiral $Z$ can be represented by means of polar like coordinates $(\phi,r(\phi)) \in [0,+\infty) \times \R^+$ (see Theorem \ref{Cor:angle_preprest}), and moreover $r(\phi)$ solves the following \emph{Retarded Differential Equation (RDE)} %satisfies the following Cauchy Problem
\begin{equation}
\label{eq:ODE:saturated:1}
\frac{d}{d\phi} r(\phi) = \cot(\alpha) r(\phi) - \frac{r(\phi - (2\pi+\alpha))}{\sin(\alpha)}
\end{equation}
with initial data
\begin{equation}
\label{Equa:init_satur}
r(\phi) = \begin{cases}
e^{\cot\alpha\phi} & \forall\phi\in[0,2\pi), \\
(e^{2\pi\cot\alpha}-1) e^{\cot\alpha(\phi-2\pi)} & \forall \phi \in [2\pi,2\pi+\alpha].
\end{cases}
\end{equation}
The angle $\alpha \in [0,\frac{\pi}{2})$ is given by
\begin{equation}\label{eq:alpha}
\alpha = \arccos \left( \frac{1}{\sigma} \right),
\end{equation}
(this is the analysis followed by \cite{firefighter} translated into thee language of RDE). Here the initial fire is the set $R_0 = B_1(0)$ and the spiral starts in a point $P=(1,0)$. Observe that for $\phi<2\pi$ the solution is an arc of the logarithmic spiral in polar coordinates $r(\phi) = e^{\cot\alpha\phi}$.

A study of the eigenvalues of the operator associated to the previous RDE gives the proof of Theorem \ref{bressan,klein}: there is a critical value ($\bar \sigma = 2.6144...$, solution to a transcendent equation) such that if $\sigma > \bar \sigma$ then all eigenvalues of the associated linear operator are complex conjugate: in particular the solution oscillates, and thus there is some first angle $\bar \phi$ such that $r(\bar \phi) = 0$. This corresponds exactly to the fact that $Z$ blocks the fire.

%(see also Subsection \ref{ss:dde}). Actually, if a player constructs any admissible spiral and at some point it decides to construct a saturated spiral, that is a branch that satisfies the length constraint of Definition \ref{eq:sat:spir:def}, then for $\sigma>2.6144$ it manages to block the fire. This is the content of Proposition \ref{prop:at:crit:speed:fire:dies} and is due to the pure complex spectrum of the operator associated to \eqref{eq:ODE:saturated:1}. 

{\color{blue} In \cite{Bressan_friends} it is not proved that, instead, for $\sigma \leq \bar \sigma$ the saturated spiral does not confine the fire, that is $r(\phi) > 0$ for every angle $\phi$: this fact can be deduce from \cite[Theorem 3]{firefighter}, which gives the estimate
\begin{equation*}
\text{minimal closing angle} \sim \big( \text{imaginary part of the largest eigenvalues} \big)^{-1}.
\end{equation*}
For general spiral, we give the following}

\begin{conjecture}
\label{conj:spiral}
If $\sigma \leq \bar \sigma$ then no spiral-like strategy is blocking the fire.
\end{conjecture}

We remark here that due to the constraints on the barrier, this critical speed is larger than the critical speed $2$ for the original conjecture \ref{conj:bressan}.

%
%
%
%
%The proof of this result is based on the following idea: we consider the following \textbf{change of variables}
%         \begin{equation}\label{eq:change:var:1}
%       \rho(t)=r((2\pi+\bar\alpha)t)e^{-\bar c(2\pi+\bar\alpha)t},\qquad  \bar c=\cot\bar\alpha-\frac{1}{2\pi+\bar\alpha}.
%   \end{equation}
%   Then the function $\rho$ satisfies the following RDE
%   \begin{equation*}
%       \dot\rho(t)=\rho(t)-\rho(t-1).
%   \end{equation*}
%   Then we prove that $\rho(2)>\rho(t)>0$ for every $t\in [1,2)$, and since $\rho:[1,+\infty)\rightarrow\mathbb R$ is continuous, then $\rho$ is \textbf{monotonically increasing} in $[2,+\infty)$. In particular $r(\phi)>0$, for every $\phi$ (this is better explained in Proposition \ref{prop:saturated:not:closed}). This is the key idea that we will use in the later proofs: in order to show that a solution to the RDE \eqref{eq:ODE:saturated:1} is strictly positive, we need to study the monotonicity of the function $\rho$. 
%
%\medskip This collection of results inspires therefore the following 


A partial answer to this conjecture has been given in \cite{firefighter} where the authors use a geometric argument to  prove the following result:

\begin{theorem}
\label{thm:klein}
If $\sigma\leq\frac{1+\sqrt{5}}{2}$ then no spiral-like strategy is admissible. 
\end{theorem}

This bound is obtained in the assumption that only some points on the spiral are admissible, while assuming the admissibility of the whole barrier requires more effort.

The aim of this paper is to prove the following result: %extend Theorem \ref{thm:klein} to higher values of $\sigma$ and to provide a general framework for the study of spirals or more complicated strategies. We will prove the following

\begin{theorem}
\label{thm:main}
No admissible spiral-like strategy confines the fire if $\sigma \leq \bar \sigma$.
\end{theorem}

%The bound $2.3$ is not sharp, since it is obtained by purely numerical computations. It could be an interesting question to investigate the numerical optimization of the parameter $\sigma$ accordingly to the method we will propose for the solution of this problem. But unfortunately, even if the speed $\sigma$ could be optimized, the critical case $\sigma=2.6144..$ at the present time  seems out of reach and very delicate. We remark that Theorem \ref{thm:main} proves Bressan's Fire Conjecture in the case of spiral strategies.

\medskip

We conclude this first part of the introduction by giving a very much simplified idea of our approach. We will neglect some technical issue, which will be further addresses in the section below.

\begin{figure}
\resizebox{.75\textwidth}{!}{\input{angle_spiral_intro.pdf_t}}
\caption{The angle-ray parametrization $(\phi,r(\phi))$ of a spiral barrier: it is also represented an admissible ray for computing the time function $u$.}
\label{Fig:angle_spiral_intro}
\end{figure}

First, a spiral strategy admits a polar-like representation $(\phi,r(\phi) \in [0,+\infty) \times \R^+$ as in Fig. \ref{Fig:angle_spiral_intro} (we will call this representation the \emph{angle-ray coordinates}):
\begin{itemize}
\item $r$ is the length of the segment starting from one point of $\zeta$ and with direction $\dot \zeta$ and ending in the next round of $\zeta$,
\item $\phi$ is the rotation angle of $r$,
\item $\beta(\phi)$ is the angle between $\dot \zeta$ and the direction of $r(\phi)$.
\end{itemize}
We can also think $r(\phi)$ as the last part of the optimal ray used by the time function $u$ in the point $\zeta(\phi)$, where we used $\phi$ as parametrization instead of $s$.

The parameter $\beta(\phi)$ is our control parameter: once it is chosen, the RDE satisfied by $r(\phi)$ is
\begin{equation*}
\frac{d}{d\phi} r(\phi) = \cot(\beta(\phi)) r(\phi) - \frac{r(\phi^-)}{\sin(\beta(\phi^-)},
\end{equation*}
where the angle $\phi^-$ is given by (see Fig. \ref{Fig:angle_spiral_intro})
\begin{equation*}
\phi = \phi^- + 2\pi + \beta(\phi^-).
\end{equation*}
Using this representation, and recalling that $r(\bar \phi) = 0$ means that the spiral closes into itself and thus blocks the fire, we replace the closure problem with the following minimum problem:
\begin{equation}
\label{Equa:minimum_rphi_intro}
\text{{\bf Optimization Problem}: given a rotation angle $\bar \phi$, choose $\phi \mapsto \beta(\phi)$ in order to minimize $r(\bar \phi)$.}
\end{equation}
Differently from the original problem (where we have to show that the set is empty), we prove that the one above has an optimal solution.

We observe that while the RDE for $r$ is linear, the choice of the control parameter affects the RDE by changing the coefficients at the next round and also by varying the delay interval $2\pi + \beta(\phi^-)$: hence it seems quite difficult to find a positive lower bound for the optimization problem \eqref{Equa:minimum_rphi_intro}, or even more to prove that a choice of the control $\beta(\phi)$ is optimal. Notice also that $\beta$ depends on the angle $\bar \phi$, i.e. the optimal spiral is not the same for all angles (and in particular is not the saturated spiral).

In order to overcome these difficulties, we use a homotopy approach as follows. Let $\bar \zeta(\phi)$ be a given spiral strategy, parametrized by the rotation angle: for every $\phi_0$, we construct a new spiral $\hat \zeta(\phi;\bar \zeta([0,\phi_0]))$ with the following properties:
\begin{enumerate}
\item $\hat \zeta(\phi;\bar \zeta([0,\phi_0])) = \bar \zeta(\phi)$ for all $\phi \in [0,\phi_0]$;
\item \label{Point:hat_spiral_2_intro} if $\hat r(\phi;\bar \zeta([0,\phi_0]))$ is the representation of the spiral in the rotation angle coordinates, the final value $\phi_0 \mapsto \hat r(\bar \phi;\bar \zeta([0,\phi_0]))$ is differentiable and has positive derivative;
\item \label{Point:hat_spiral_3_intro} the spiral $\hat \zeta = \hat \zeta(\cdot;\bar \zeta(\{0\}))$ is such that $\hat r(\bar \phi) > 0$.
\end{enumerate}
Since the spiral $\bar \zeta$ is fixed during the homotopy argument, we shorten the notation to $\hat r(\cdot,\phi_0)$ or also $\hat r(\cdot;s_0)$ when using the length parametrization for $\bar \zeta$.

The existence of such a family for every spiral $\zeta$ gives thus the expanded version of the main Theorem \ref{thm:main} (which now becomes a corollary):

\begin{theorem}
\label{Theo:main_extended}
For each spiral strategy $\bar \zeta$ and rotation angle $\bar \phi_0$, the spiral $\hat \zeta(\cdot;\phi_0)$ is the optimal solution to the minimization problem \eqref{Equa:minimum_rphi_intro} given the initial spiral arc $\bar \zeta([0,\phi_0])$. In particular, $\hat \zeta(\cdot;0)$ is optimal among all spirals.
\end{theorem}

Point \eqref{Point:hat_spiral_3_intro} above implies that
\begin{equation*}
0 < \hat r(\bar \phi;0) \leq \hat r(\bar \phi;s_0) + \int_0^{\phi_0} \frac{d}{d\phi_0} \hat r(\bar \phi;\phi_0) d\phi_0 = \hat r(\bar \phi;\phi_0) \leq \bar r(\bar \phi),
\end{equation*}
where $\bar r$ is the spiral representation by the rotation angle. In particular Theorem \ref{thm:main} holds.

We will also prove that the only case when the derivative $\frac{d}{d\phi_0} \hat r(\bar \phi;s_0)$ is $0$ is by following exactly the spiral $\hat r(\cdot;\phi_0)$, so that the above chain of inequalities become strict as soon as we perturb the spiral $\hat r$. Hence we have the following

\begin{corollary}
\label{Cor:uniqueness}
The optimal spiral strategy for the angle $\bar \phi$ is $\hat r(\cdot;0) = \hat r(\cdot)$.
\end{corollary}

We remark that by changing the angle $\bar \phi$, the optimal spiral changes. We also remark that the optimal spiral is not regular, but only Lipschitz at the last round. This can be heuristically explained by observing that the last round is not having influence on the next evolution (being the last one!), so that the regularizing effect of the RDE is not acting.

Being able to describe the optimal spiral, it is possible to give estimates, in particular one can prove the asymptotic divergence of the optimal spiral:

\begin{corollary}
\label{Cor:divergence}
The spiral $\hat \zeta$, optimal at the angle $\bar \phi$, satisfies
\begin{equation*}
\hat r(\bar \phi) \simeq \phi e^{\bar c \phi},
\end{equation*}
where $\bar c$ is the only positive eigenvalue of the RDE.
\end{corollary}

We are also able to give a precise value to the constant in front of $\phi e^{\bar c \phi}$, as we will point out in the extended introduction below.


\subsection{Extended introduction and collection of all principal results}
\label{Ss:extend_more_intro}


In this section we present an extended introduction to the proof of Theorem \ref{Theo:main_extended}, and all the steps required to construct the family $\hat r(\cdot;\phi_0)$. Many of the results obtained along the proof are interesting on their own, and we will report their statement.


\subsubsection{Section \ref{s:admissible:barriers}}
\label{Sss:admiss_barr_intro}


This section introduces the basic objects considered in this paper: the most important ones are the set of admissible curves \gls{Gamma}, Equation \eqref{eq:admissible:curves} (recall also \eqref{eq:burned:region_intro}), the minimum time function \gls{utimefunct}, Equation \ref{eq:solution:HJ} (recall \eqref{eq:min:time:function}), the admissibility functional \gls{Acaladmisx}, Equation \ref{eq:admiss:funct}, and the saturated set \gls{Scal}, Equation \eqref{eq:sat:set}. The limit of a minimizing sequence of admissible curves in $\Gamma$ are the \emph{optimal rays}, Definition \ref{def:optimal:ray}. These Lipschitz curves are not admissible in general, but are the ones needed to compute the value of the time function $u(x)$.

The first result is in Section \ref{Ss:prelimnaries}, where the existence of a closing barrier for every initial burning set $R_0$ is reduced to the study when $R_0 = \{0\}$ and the barrier is constructed outside the unit ball $B_1(0)$, Proposition \ref{Prop:limit_speed}. The equivalence is not exact as stated in the proposition, but since for $\sigma \leq \bar \sigma$ we show that it is not possible to block the fire even in this situation, we conclude that in our case the equivalence is complete.

Section \ref{Ss:spiral_barrier_intro} can be though as a thoughtful description of the notion of spiral barrier of Definition \ref{Def:spiral_barrier_intro}: in particular Remark \ref{Rem:comment_single_curve} explains the importance of the monotonicity of $u(\zeta(s))$. Some notation for convex barriers are also introduce, like th left and right tangent vectors \gls{t-t+} , the local radius of curvature \gls{Rcurva}, the subdifferential \gls{subdiffzeta} (Definition \ref{Def:supporting_direction}). \\
The most important result of this section is that for spiral barrier one can use the angle-ray representation as considered below Theorem \ref{thm:main}. This result is obtained in two steps. First, Proposition \ref{thm:param_1} constructs this representation round-by-round, starting with the initial round about the origin $(0,0) \in \R^2$ (where it corresponds to polar coordinates), and the recursively constructing the angle at the next round. The idea is that the directions of $r(\phi)$ is determined by the previous round, and then the angle $\beta(\phi)$ is deduced by knowing the tangent $\mathbf t = \dot \zeta$ at that point: a look at Fig. \ref{fig:param:spiral} is probably better than any explanation. \\
A version of Proposition \ref{thm:param_1} avoiding the explicit reference to round is Theorem \ref{Cor:angle_preprest}. Together with the function \gls{rphi}, we also introduce the functions \gls{s-phi}, \gls{s+phi}, which are the length parametrization of the starting/ending point of the segment $r(\phi)$. Their regularity properties ($s^-(\phi)$ BV, $s^+(\phi)$ Lipschitz) are also proved. We conclude this section by using the angle-ray representation to rewrite the convexity of $\zeta$ in terms of the angle \gls{beta}, the admissibility functional $\mathcal A = \mathcal A(\phi)$ and the burning rate \gls{b(t)} of the barrier $\zeta$, Proposition \ref{Lem:burnign_rate}.

As a warning, because of Theorem \ref{Cor:angle_preprest} we can use indifferently the length $s$ or the angle $\phi$ as parameter for the a spiral barrier: in the following we will often choose the most convenient one, without underlining it, in order to simplify notation and shorten the analysis. We also note that in the case of $\beta$ constant the RDE for $r$ has been already obtained by \cite{Bressan_friends} and \cite{RDE}.


\subsubsection{Section \ref{S:ODE}}
\label{Sss:ODE_intro}


The first part of the section is devoted to obtain the RDE satisfied by a spiral barrier: Lemma \ref{lem:ODE:spiral} offers some differential relations among the various quantities introduced in the angle-ray description of a spiral. Equation \eqref{eq:spiral:angle} is the distributional RDE for the spiral barrier: it is nothing else than the relation
\begin{equation*}
\big\{ \text{variation of $r$} \big\} \ = \ \big\{ \text{increase due to $\beta$ at the end point} \big\} \ - \ \big\{ \text{decrease due to curvature at the base point} \big\}.
\end{equation*}
Proposition \ref{Prop:construct_spiral} is the inverse statement: assume that $r(\phi),\beta(\phi)$ satisfies the differential relations of Lemma \ref{lem:ODE:spiral}, then, up to fixing the initial point, there is a unique spiral barrier such that its angle-ray coordinates are the given ones. The proof is based on the round decomposition.

In Section \ref{Sss:equation_satur} we prove that the equation of he saturated spiral is \eqref{eq:ODE:saturated:1} with initial data \eqref{Equa:init_satur}.

The next section contains the analysis of the linear RDE
\begin{equation}
\label{Equa:satur_spiral_intro}
\frac{d}{d\phi} r(\phi) = \cot(\alpha) r(\phi) - \frac{r(\phi - 2\pi - \alpha)}{\sin(\bar \alpha)}
\end{equation}
with $\alpha$ constant. This section contains many results which have already been proved in \cite{firefighter}: we present them for completeness. The main one is that there is a critical angle $\bar \alpha$ such that for $\alpha < \bar \alpha$ the characteristic equation of the above RDE has two distinct positive real eigenvalues, for $\alpha = \bar \alpha$ the two eigenvalues coincide and the geometric multiplicity is $1$, for $\alpha > \bar \alpha$ all eigenvalues are complex conjugate, Corollary \ref{Cor:eigen_angle}. This gives in particular that for $\alpha > \bar \alpha$ the saturated spiral confines the fire, Proposition \ref{prop:at:crit:speed:fire:dies}.

Section \ref{ss:subset:saturated} is concerned with the converse result for the saturated spiral. Observe that even if there are positive real eigenvalues, if the initial data is $0$ when projected on the corresponding eigenspace then the solution oscillates and thus the fire is blocked: thus the idea is to give a condition assuring the exponential blow-up of the solution and checking that the saturated spiral satisfies this condition. \\
The starting point is to rescale the variables \newglossaryentry{rhotau}{name=\ensuremath{\rho(\tau)},description={rescaled variable $\rho$ with $\phi = (2\pi + \alpha) \tau$}}
\begin{equation*}
\gls{rhotau} = r((2\pi+\bar \alpha) \tau) e^{-\bar c (2\pi + \bar \alpha) \tau},
\end{equation*}
with $\bar c$ equal to the only real eigenvalue (see Corollary \ref{Cor:divergence}), and rewrite the RDE in the critical case as
\begin{equation}
\label{Equa:retarde_intro}
\dot \rho(\tau) = \rho(\tau) - \rho(\tau-1).
\end{equation}
Lemma \ref{lem:key} gives a simple-to-check criterion to verify if the solution diverges:

\begin{lemma}[Second part of Lemma \ref{lem:key}]
\label{lem:key_intro}
%If $\frac{a}{b} > e$ and $\rho(1) \geq \rho(\tau) > 0$ for every $\tau \in [0,1]$, then $\rho(\tau)$ diverges exponentially. 
%
If $\frac{a}{b} = e$ and $\rho(1) > \rho(\tau) > 0$, $\tau \in [0,1)$, then the solution $\rho(\tau)$ diverges linearly.
%
%If $0 < \frac{a}{b} < e$, the solution $\rho(\tau)$ oscillates.
\end{lemma} %if $\rho$ is increasing in $[0,1]$ then it remains increasing.

Even if it seems trivial, it gives immediately that the saturated spiral is diverging:

\begin{proposition}[Proposition \ref{prop:saturated:not:closed_1}]
\label{prop:not_closed_intro}
Let $Z$ be the saturated spiral. Then it does not confine the fire for $\sigma\leq \bar \sigma$. 
\end{proposition}

The optimal solution $\hat r(\cdot;\phi_0)$ and its derivatives have a more complicated structure than the saturated spiral: hence Section \ref{Sss:green_kernels} introduces the Green kernel \gls{gkernel} for the RDE \eqref{Equa:retarde_intro} (Lemma \ref{Lem:explic_kernel_RDE}), and study its asymptotic behavior (Lemma \ref{Lem:aympt_g}). It is essentially standard analysis for a linear functional equation, and for completeness we write also the explicit forms of the kernel \gls{Gkernel} for the RDE of the saturated spiral \eqref{Equa:satur_spiral_intro}.

Since it will be useful to study also the evolution of the length of a spiral barrier, this section ends with some useful estimates for the primitives of $G(\phi)$ (Section \ref{Sss:length_saturated}).


\subsubsection{Section \ref{S:exist_opti_traj}}
\label{Sss:exists_opti_intro}


In this section we prove that the optimization problem \eqref{Equa:minimum_rphi_intro} has a solution in the domain of admissible spiral barriers with bounded length $L$, Theorem \ref{Theo:exists_min}:

\begin{theorem}[Theorem \ref{Theo:exists_min}]
\label{Theo:exists_min_intro}
Fix a rotation angle ${\bar \phi} \geq {\phi_0}$. Then either there exists an admissible spiral in $\mathcal A_S(Z,{\phi_0})$ with $\bar L \gg 1$ blocking the fire before or at ${\bar \phi}$ or there exists an admissible spiral $\zeta$ such that $r({\bar \phi})$ is minimal among all admissible spirals of length bounded by $\bar L$.
\end{theorem}

Note that in the above statement we consider the more general case where a first arc of $r(\phi)$, $\phi \leq \phi_0$, is fixed, and we are allowed to choose the remaining part. This is perfectly in line with the statement of Theorem \ref{Theo:main_extended}, where the optimality is proved given the initial arc $\bar \zeta([0,\phi_0])$.

A solution means that either there is an admissible spiral blocking the fire before the angle $\bar \phi$, or there is a minimizing one, and the length $L$ is chosen sufficiently large in order to have at least a spiral arriving at the angle $\bar \phi$. The approach is the standard one: first one proves the compactness of the set of admissible spirals, Proposition \ref{Prop:compact_curves} and Corollary \ref{Cor:convergs}, and then passes to the limit to a minimizing sequence, being the functional $\zeta \mapsto r(\bar \phi)$ continuous. We just remark that as a corollary we have that the admissibility functional is u.s.c. for Hasdorff convergence, hence giving the closure of the family of admissible spirals, and also observe that a key ingredient is the decomposition by rounds of Proposition \ref{thm:param_1}. \\
The parameter $L$ will not play any role in the future: indeed once we show that the spiral $\hat r$ is optimal, we have an estimate for all spirals. It is just to assures that the curves $\zeta$ lives in a compact set of $\R^2$.

When studying the derivative $\frac{d}{ds_0} \hat r(\cdot;s_0)$ of $\hat r(\phi;s_0)$ (see the discussion at the end of Section \ref{Sss:admiss_barr_intro} for the equivalence of $\phi$ and $s$), it is important to know the structure of the minimal time function $u$ generated by $\bar \zeta([0,s_0])$. Lemma \ref{Lem:convexity} and Corollary \ref{lem:C:1:1} give explicit computations of the first and second derivatives of $u$: roughly speaking, we are solving the Eikonal equation, because of the assumptions on the fire spreading speed $F(x) = B_1(0)$, and thus $\nabla u$ is BV and the level sets of $u$ are $C^{1,1}$-curves.

\begin{figure}
\resizebox{.75\textwidth}{!}{\input{spiral_first_round_intro.pdf_t}}
\caption{The solution to the optimization problem at the last round. The gray region is the region which cannot be reached by any admissible spiral.}
\label{Fig:optimal_last_intro}
\end{figure}

The first glimpse on the structure of the optimal solution $\hat r$ is given in Section \ref{Ss:minimal_reach}: if we restrict the optimality to just one round after $\phi_0$, then $\hat r$ can be explicitly constructed without further analysis. \\
To describe the structure of such a solution, we refer to Fig. \ref{Fig:optimal_last_intro}. Starting from the angle $\phi_0$, the solution is made by three components.
\begin{enumerate}
\item We follow the level set of the minimal time function $u$ until the point $\zeta(\phi_1)$, which is saturated. At this point it is not possible to proceed along this level set, because the spiral would not be admissible. This arc (the magenta one between the points $\zeta(\phi_0)$ and $\zeta(\phi_1)$ in the picture) is the optimal solution for angles $\bar \phi \in [\phi_0,\phi_1]$, since the monotonicity of $s \mapsto u(\zeta(s))$ gives that we cannot cross the level set of $u(\zeta(\phi_0))$. In the case $\zeta(\bar \phi_0)$ is saturated, then this regions reduces to a point.

The optimal spiral barrier coincides with the are of level set.

\item If $\bar \phi > \phi_1$, then we consider the spirals made by a portion of the magenta arc and a segment: the segment ends in the first point it is saturated. We show that such a construction defines a convex curve (the blue one in Fig. \ref{Fig:optimal_last_intro}) starting orthogonally to the level set of $u$ and ending in a saturated point $\zeta(\phi_2)$ such that the angle formed with the direction of the optimal ray is exactly $\bar \alpha$. Also in this case, if the initial point is saturated, it holds $\phi_2 = \phi_0$.

The optimal spiral barrier is an arc of the level set and a segment ending in the blue curve.

\item For angles $\bar \phi > \phi_2$ one follows the saturated spiral starting from $\zeta(\phi_2)$ (green spiral in the picture). The optimal spiral barrier is an arc of the level set, the segment arriving in $\zeta(\phi_2)$ and an arc of a saturated spiral.
\end{enumerate}

\begin{figure}
\resizebox{\textwidth}{!}{\input{three_cases.pdf_t}}
\caption{The three cases of Theorem \ref{Cor:curve_cal_R_sat_spiral_intro}: in the first picture all level set $\xi$ is admissible, and then for every angle $\geq {\phi_0}$ the optimal solution is an arc of the level set; in the second case all curve $\mathtt R$ is admissible, and then the optimal solutions for point on $\mathtt R$ is an arc of $\xi$ and a segment; in the third case for large angles the minimal point lies on a saturated spiral, and the optimal solution is an arc of $\xi$, a segment and an arc of saturated spiral.}
\label{Fi:three_cases_intro}
\end{figure}

It is important to observe that the curve formed by the magenta arc up to $\phi_1$, the blue convex curve and the green saturated spiral is not a spiral barrier: indeed it is not convex. It gives the optimal solution for $\phi_0 \leq \bar \phi \leq \phi_0 + 2\pi + \beta^-(\phi_0)$, where $\beta^-(\phi_0) = \lim_{\phi \nearrow \phi_0} \mathbf t(\phi)$, i.e. the left tangent vector: for every angle $\bar \phi$ there exists an explicit spiral barrier ending in the corresponding point of the curve constructed above. The three situations above are drawn in Fig. \ref{Fi:three_cases_intro}. The main result is then the following

\begin{theorem}(Theorem \ref{Cor:curve_cal_R_sat_spiral})
\label{Cor:curve_cal_R_sat_spiral_intro}
The curves constructed above are the unique solution to the minimum problem considered in Theorem \ref{Theo:main_extended} for ${\bar \phi} \in [{\phi_0},{\phi_0} + 2\pi + \beta^-({\phi_0}))$.
\end{theorem}

A question which arises naturally is the following: if we proceed the saturated spirals also for angles larger that $\phi_0 + 2\pi + \beta^-(\phi_0)$, is this spiral barrier optimal? The short answer is no, but the proof of this fact and the construction of the correct optimal spiral requires much more analysis and it is the central part of this work. Due to its importance, we will refer the spiral constructed by the procedure above and prolonging the saturated spiral after the angle $\phi_ 0 + 2\pi + \beta^-(\phi_0)$ as the \emph{fastest saturated spiral}.


\subsubsection{Section \ref{S:case:study}}
\label{Sss:case_study_intro}


The construction above when $\phi_0 = 0$ is a particular spiral which is important for the next analysis, since the optimal one will be obtained as a perturbation of this spiral: the study of its properties is in Section \ref{S:case:study}. For the seek of generality, we consider the case where $R_0 = B_{\mathtt a}(0)$, and show explicitly the form of the fastest saturated spiral: depending on the radius $\mathtt a$, it is either a an arc + segment + saturated spiral (if $\mathtt a \in (0,\sin(\bar \alpha))$), a segment + saturated spiral (if $\mathtt a \in [\sin(\bar \alpha),1)$) or just the saturated spiral when $\mathtt a = 1$. We will use the denomination
\begin{description}
\item[Arc case] the fastest saturated spiral starts with a non-trivial arc of the level set, i.e. this arc is not just a point;
\item[Segment case] The fastest saturated spiral starts with a segment, possibly made of just a point, i.e. the initial point is saturated and the spiral coincides with the saturated one.
\end{description}
These various cases will be also encountered when considering as a starting point the spiral arc $\zeta([0,s_0])$, so that they are worth studying in this setting where the functions are explicit.

The study of the behavior of this spiral gives the following

\begin{theorem}[Theorem \ref{thm:case:a}]
\label{thm:case:a_intro}
For any value of $\mathtt a \in (0,1]$, the fastest saturated spiral $S_{\mathtt a}$ with initial burning region $B_\mathtt a(0)$ does not confine the fire: more precisely, the spiral diverges exponentially as $r(\phi) \sim \phi e^{\bar c \phi}$,
%$$
%r(\phi) \sim 2 \phi e^{\bar c \phi} \begin{cases}
%\frac{e^{-\bar c(\Delta \phi_{\mathtt a} + \frac{\pi}{2} - \bar \alpha)}}{\sin(\bar \alpha)} - e^{-\bar c(2\pi)} - \frac{e^{-\bar c(2\pi + \frac{\pi}{2})} - e^{- \bar c (2\pi + \frac{\pi}{2} + \Delta \phi_\mathtt a)}}{\bar c} - \cot(\bar \alpha) e^{-\bar c(2\pi + \frac{\pi}{2} + \Delta \phi_\mathtt a)} & 0 \leq \mathtt a < \sin(\bar \alpha), \\
%\frac{\sin(\theta_\mathtt a + \bar \alpha) e^{-\bar c \theta_\mathtt a}}{\sin(\bar \alpha)} - e^{-\bar c(2\pi)} - \frac{\sin(\theta_\mathtt a) e^{-\bar c(2\pi + \theta_\mathtt a + \bar \alpha)}}{\sin(\bar \alpha)} & \sin(\bar \alpha) \leq \mathtt a \leq 1,
%\end{cases}
%$$
being $\bar c = \ln(\frac{2\pi+\bar \alpha}{\sin(\bar \alpha)})$ the only real eigenvalue for the characteristic equation of the RDE for saturated spirals.
\end{theorem}

The proof is also interesting, because it is the prototype of the line of proof of many of the subsequence statement. The explicit form of the spiral barrier in the angle-ray coordinates can be given explicitly using the kernel \gls{Gkernel}: in the segment case, where the explicit forms are simpler, the solution takes the form (see Equation \ref{Equa:expl_sol_sat})
\begin{equation*}
r(\phi) = \frac{\sin(\bar \theta_{\mathtt a})}{\sin(\bar \alpha)} G \big( \phi - \bar \phi_0(\mathtt a) \big) - G(\phi - 2\pi) - \frac{\sin(\bar \theta_{\mathtt a} - \bar \alpha)}{\sin(\bar \alpha)} G \big( \phi - \bar \phi_0(\mathtt a) - 2\pi - \bar \alpha \big),
\end{equation*}
with
\begin{equation*}
\bar \phi_0 = \bar \theta_{\mathtt a} - \bar \alpha, \quad \bar \theta_a = \arccos(\mathtt a) + \bar \alpha.
\end{equation*}
By studying the derivative w.r.t. $\mathtt a$ (Step 2 of the proof of Theorem \ref{thm:case:a}, pag. \pageref{Page:step_2_case_study_segment}), one proves that $r(\phi) = r(\phi,\mathtt a)$ is monotonically increasing w.r.t. $\mathtt a$ increases, and then that the worst case happens for $\mathtt a = \sin(\bar \alpha)$, which means $\bar \theta_a = \frac{\pi}{2}$, $\bar \phi_0 = \frac{\pi}{2} - \bar \alpha$. Then one plots numerically the rescaled function
$$
\rho(\tau) = r(\bar \phi_0 + (2\pi + \bar \alpha) \tau) e^{-\bar c (2\pi + \bar \alpha) \tau}
$$
which is explicitly given by
\begin{equation}
\label{Equa:base_sol_intro}
\rho(\tau) = \frac{1}{\sin(\bar \alpha)} g(\tau) - e^{-\bar c(2\pi + \bar \alpha - \frac{\pi}{2})} g \bigg( \tau - \frac{\frac{\pi}{2}}{2\pi + \bar \alpha} \bigg) - \cot(\bar \alpha) e^{-\bar c (2\pi + \bar \alpha)} g(\tau - 1).
\end{equation}

\begin{figure}
\resizebox{.75\textwidth}{!}{\includegraphics{base_sol_intro.png}}
\caption{Plot of the first 5 rounds of the function \eqref{Equa:base_sol_intro}.}
\label{Fig:base_sol_intro}
\end{figure}

A numerical plot of the function above is in Fig. \ref{Fig:base_sol_intro}: one observes that the function is positive, and its derivative can be numerically computed to be strictly positive for $\tau \in [4,5]$ (which corresponds to the fifth round). Then one can apply Lemma \ref{lem:key_intro} to deduce that $r(\phi)$ is positive, and actually exponentially increasing as $\phi \to \infty$. The asymptotic behavior is a consequence of the asymptotic expansion of the kernel $G(\tau)$ as $\tau \to \infty$.

The last result is this section is a estimate on the ratio between $r(\phi)$ and the length $L(\phi)$ of the spiral:

\begin{proposition}[Proposition \ref{Prop:length_compar}]
\label{Prop:length_compar_intro}
It holds for $\phi \geq \tan(\bar \alpha) + \frac{\pi}{2} - \bar \alpha$
\begin{equation*}
r(\phi) - 2.08 L(\phi - 2\pi - \bar \alpha) \geq 0.67 e^{\bar c(\phi - \tan(\bar \alpha) - \frac{\pi}{2} + \bar \alpha)}.
\end{equation*}
\end{proposition}

Besides having an interest on its own, this estimate is fundamental to show that the optimal spiral $\hat r(\phi;\phi_0)$ may have an arc only for angles $\phi$ close to $\phi_0$: this mans that there is a regularizing effect in the evolution of $\hat r$, because it can be proved that one can choose the control parameter $\beta$ in order to have an arbitrarily number of arcs at arbitrarily large angles, see Remark \ref{Rem:inital_tent}. The constant $2.08$ is almost optimal, see Remark \ref{Rem:asymtp_consta_for_comp}.


\subsubsection{Section \ref{S:family}}
\label{Sss:family_intro}


This section is the core of the paper: we construct a differentiable path from the fastest saturated spiral of Section \ref{S:case:study} (Section \ref{Sss:case_study_intro}) to any admissible spiral. The construction is based on the results of Theorem \ref{Cor:curve_cal_R_sat_spiral_intro} which gives an explicit construction for the first round starting from $\zeta([0,s_0])$, and this construction is then extended to every angle by prolonging as a saturated spiral. We denote this barrier as $\tilde r(\phi) = \tilde r(\phi;s_0)$.

As we said the fastest saturated spiral $\tilde r$ is not the optimal spiral after the first round starting in $\phi_0$, and indeed the derivative w.r.t. $s_0$ will be a function with some negative regions. There re however two main advantages in studying this one-parameter family of spirals.
\begin{enumerate}
\item There are only two main cases to be considered (for the optimal case we need to work on about 20 cases): we can start with a segment or with an arc+segment. It is actually possible to reduce the analysis of the derivative $\delta \tilde r = \frac{d\tilde r}{ds_0}$ to a single case (the segment is the arc when the latter reduces to a single point, Remark \ref{Rem:same_as_segment}, yielding as a consequence that the family is actually $C^1$ in a suitable topology), but since the segment case is much easier we prefer to keep it. In Fig. \ref{Fig:segment_intro_1} the geometric situation to compute the derivative $\delta \tilde r(\phi;s_0)$ is represented.

\item The optimal solution $\hat r$ will be a perturbation of the spiral $\tilde r$: this perturbation will be added to the solution computed in this section, and it will be shown that the analysis is fundamentally different only in the first round, more precisely in the regions where the derivative $\delta \tilde r$ is negative. In the other region a simple adaptation of the estimates obtained in this section is sufficient to prove the positivity of the derivative $\delta \hat r = \frac{d\hat r}{ds_0}$.
\end{enumerate}

The main results of this section are:
\begin{itemize}
\item Propositions \ref{Prop:equa_delta_tilde_r_segm} and \ref{Prop:equa_delta_tilde_r_arc}, which compute the RDE satisfied be the derivative $\delta \tilde r(\phi)$: for example, in the segment case this derivative satisfies

\begin{proposition}(Proposition \ref{Prop:equa_delta_tilde_r_segm})
\label{Prop:equa_delta_tilde_r_segm_intro}
For $\phi > \phi_0 + \bar \theta - \bar \alpha$, the derivative 
$$
\delta \tilde r(\phi;s_0) = \lim_{\delta s_0 \searrow 0} \frac{\tilde r(\phi;s_0 + \delta s_0) - \tilde r(\phi;s_0)}{\delta s_0}
$$
satisfies the RDE on $\R$
\begin{equation*}
\frac{d}{d\phi} \delta \tilde r(\phi;s_0) = \cot(\bar \alpha) \delta \tilde r(\phi;s_0) - \frac{\delta \tilde r(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)} + S(\phi;s_0),
\end{equation*}
with source
\begin{align*}
S(\phi;s_0) &= \cot(\bar \alpha) \frac{1 - \cos(\theta)}{\sin(\bar \alpha)} \Diracd_{\phi_0 + \bar \theta - \bar \alpha} - \Diracd_{\phi_0 + 2\pi + \theta_0} \\
& \quad + \frac{\cos(\theta) - \cos(\bar \alpha)^2}{\sin(\bar \alpha)^2} \Diracd_{\phi_0 + 2\pi + \bar \theta} + \frac{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}{\sin(\bar \alpha)} \Diracd'_{\phi_0 + 2\pi + \bar \theta},
\end{align*}
where $\Diracd_0$ is the Dirac-delta measure in $0$, and $\Diracd_0'$ its distributional derivative.
\end{proposition}
The angle $\theta$ is the angle formed by the tangent to the spiral $\zeta$ and the initial segment of $\tilde r$ at the angle $\phi_0$. Note the similarity with the fastest saturated spiral studied in the previous section.

\item Corollaries \ref{Cor:evolv_r_after_phi_2} and \ref{Cor:evolv_r_after_phi_2:arc}, which gives the explicit solution in terms of the kernel $G$;

\item Propositions \ref{Prop:regions_pos_neg_segm} and \ref{Prop:neg_region}, where the positivity properties and asymptotic behavior of $\delta \tilde r$ is analyzed. We present here the segment case, where we use the change of variable $\phi = \phi_0 + \bar \theta - \bar \alpha + (2\pi + \bar \alpha) \tau$, $\bar \theta$ being the angle of the ray $r(\phi_0)$ and the initial segment starting at $\zeta(\phi_0)$: using the rescaled function
\begin{equation*}
\rho(\tau) = \delta \tilde r \big( \phi_0 + \bar \theta - \bar \alpha + (2\pi + \bar \alpha) \tau \big) e^{-\bar c (2 \pi + \bar \alpha) \tau}
\end{equation*}

\begin{proposition}(Proposition \ref{Prop:regions_pos_neg_segm})
\label{Prop:regions_pos_neg_segm_intro}
The function $\rho(\tau) = \rho(\tau,\theta)$ is strictly positive outside the region
\begin{equation}
\label{Equa:neg_segmnt_666_intro}
\gls{Nsegm} := \bigg\{ 1 - \frac{\theta}{2\pi + \bar \alpha} \leq \tau \leq 1, 0 \leq \theta \leq \hat \theta \bigg\} \cup \big\{ \theta = 0 \} \cup \{ \tau = 1, \theta \in [2\bar \alpha,\pi] \big\} \subset \R \times [0,\pi],
\end{equation}
where the angle \gls{thetahat} is determined by the unique solution to
\begin{equation}
\label{Equa:hat_theta_det_666_intro}
\cot(\bar \alpha) \frac{1 - \cos(\hat \theta)}{\sin(\bar \alpha)} -  e^{- \cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} = 0, \qquad \hat \theta \in [0,\pi].
\end{equation}
Moreover, as $\tau \to \infty$, the function $\rho(\tau)$ diverges like
\begin{equation*}
\lim_{\tau \to \infty} \frac{\rho(\tau) e^{-\bar c \tau}}{\tau} = 2 (S_0 + S_1 + S_2 + S_3), \quad 2 (S_0 + S_1 + S_2 + S_3) \in \theta^2 (0.08,028).
\end{equation*}
\end{proposition}

The arc case is more complicated, we refer the reader to Proposition \ref{Prop:neg_region}. In Fig. \ref{Fig:segment_intro_2} we plot numerically the solution of Proposition \ref{Prop:equa_delta_tilde_r_segm_intro} with $\theta = .3$ for the first 3 rounds. Observe that there is a negative region $\tau \in [1 - \frac{\theta}{2\pi + \bar \alpha},1]$ in the first rounds, then the solution become positive. Note that the derivative is not smooth, and this force us to study numerically the first 5 rounds in order to apply Lemma \ref{lem:key_intro}. \\
A final observation here is that we allot $\theta$ the go beyond $\frac{\pi}{2}$, which is not possible under our definition of spiral strategy because of convexity. However we expect that our results can be used to address the general case where the strategy is a generic curve of finite length, in which case the change of direction is not restricted by convexity.
\end{itemize}

\begin{figure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{segment_intro.pdf_t}}
\caption{Geometric structure of the spiral $\tilde r$ and its perturbation.}
\label{Fig:segment_intro_1} \hfill
\end{subfigure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\includegraphics{rhosegm_intro_first3.png}}
\caption{Numerical plot of the function $\rho(\tau)$ for the first 3 rounds.}
\label{Fig:segment_intro_2}
\end{subfigure}
\caption{The segment case of Section \ref{Sss:family_intro}}
\label{Fig:segment_intro}
\end{figure}

The fact that there is a negative region at about the end of the first round for some angles $\theta$ means in particular that the saturated spiral is \emph{not optimal}: indeed, at the angle $\bar \phi - 2\pi - \bar \alpha$ by moving the barrier $\zeta$ along the direction $\bar \phi$ instead of following the spiral one obtains that $r(\bar \phi)$ is decreasing (it has negative derivative by Proposition \ref{Prop:regions_pos_neg_segm_intro}. However, since this negative region is for a relatively short interval of angles, the correction to the fastest saturated spiral $\tilde r$ will be localized only at the last round. Thus we have another argument to affirm that the fastest saturated spiral is in some sense the building block for the optimal spiral $\hat r$.

For the proof of the above propositions, the approach is similar to the one used for Theorem \ref{thm:case:a_intro}: the only difference is that since the structure of the derivative is more complicate, we split the first rounds into pieces in order to avoid discontinuities. After $3$ rounds the regularizing effect of the RDE has smoothen the solution, so that we can prove the monotonicity of the solution. Numerically, we plot the function
\begin{equation*}
\frac{\delta \tilde r(\phi)}{\theta (\theta + \Delta \phi)}, \quad \Delta \phi \ \text{being the opening of the initial arc and $\theta$ as above}, 
\end{equation*}
and observe the uniform positivity or monotonicity. As observed before, we require the computer only computations on explicit functions (polynomials, exponential, trigonometric functions and their combinations), we never ask to solve a differential equation.


The fact that the negativity region is limited to the first round gives that we can extended the length estimate of Proposition \ref{Prop:length_compar_intro} to a general spiral:

\begin{proposition}(Corollary \ref{Cor:bound_length_gen})
\label{Cor:bound_length_gen_intro}
Consider the spiral $\tilde r(\phi;\phi_0)$: if
$$
\phi \geq \begin{cases}
\phi_0 + \bar \theta + 2\pi & \text{segment case}, \\
\phi_0 + \Delta \phi + \frac{\pi}{2} + 2\pi & \text{arc case},
\end{cases}
$$
then
\begin{equation*}
\tilde r(\phi) - 2.08 \tilde L(\phi - 2\pi - \bar \alpha) \geq r(\phi) - 2.08 L(\phi - 2\pi - \bar \alpha) > 0.67 e^{\bar c (\phi - \tan(\bar \alpha) - \frac{\pi}{2} + \bar \alpha)},
\end{equation*}
\end{proposition}

This is a regularity result: after one round the spirals $\tilde r$ starts to be similar to the fastest saturated spiral of the previous section. It will be used to simplify the expression of the optimal spiral $\hat r(\cdot;s_0)$.


\subsubsection{Section \ref{S:optimal_solut}}
\label{Sss:optimal_solut_intro}


In this section we construct the optimal solution candidate $\hat r(\cdot;s_0)$, when the spiral $\zeta([0,s_0])$ is fixed. The construct is based on the observation that in the first round there is a region where the derivative $\delta \tilde r(\cdot;s_0)$ is negative. We explain the construction in the simple case of the saturated spiral, in order to avoid additional technicalities. We refer to Fig. \ref{Fig:optimal_intro}.

\begin{figure}
\resizebox{.75\textwidth}{!}{\input{optimal_intro.pdf_t}}
\caption{The construction of the optimal solution for the saturated spiral.}
\label{Fig:optimal_intro}
\end{figure}

We are thus given the angle $\bar \phi$, and the question is if by changing the spiral at and angle $\phi_0$ the ray $r(\bar \phi)$ becomes smaller. \\
If $\phi_0 + 2\pi + \bar \alpha < \bar \phi$, Proposition \ref{Prop:regions_pos_neg_segm_intro} yields that any perturbation to $\zeta$ at $\phi_0$ has a positive derivative, and then the ray $r$ increases. \\
If $\phi_0 + 2\pi + \bar \alpha = \bar \phi$, i.e. at the point $P_0$ of Fig. \ref{Fig:optimal_intro}, we are entering in the negativity region: indeed $\tau = 1$ is the boundary of the $N_\mathrm{segm}$ for $\theta = 0$: this last condition on the angle $\theta$ formed by $\bar \phi$ and the segment of the spiral means that at that angle the perturbation is tangent to the saturated spiral. If the point $P_1$ thus follows the direction $\bar \phi$, it follows from the computation of Section \ref{S:family} that $\theta$ is increasing, and then it is convenient to construct this segment up to the point where $\theta = \hat \theta$ (the angle constructed in Proposition \ref{Prop:regions_pos_neg_segm_intro}), i.e. we are exiting the negativity region $N_\mathrm{segm}$. \\
From this point onward we can apply Theorem \ref{Cor:curve_cal_R_sat_spiral_intro} to specify the remaining part of the last round: it is the fastest saturated starting from the point $P_1$ such that the segment originating in $P_1$ form the critical angle $\hat \theta$ with the direction $\bar \phi$.

%
%Let $s_0 = s(\phi_0)$ be the initial point of the construction corresponding to a rotation angle $\phi_0$, i.e. the initial spiral is given for $s \in [0,s_0]$, and consider a final angle $\bar \phi$. If $\bar \phi \in \phi_0 + [0,2\pi + \beta^-(\phi_0))$, Theorem \ref{prop:best:first:Enclosure} implies that the solution $\tilde r(\phi;s_0)$ of the previous section is optimal. \\
%For $\phi \geq \phi_0 + 2\pi + \beta^-(\phi_0)$, one first follow the solution $\tilde r(\phi;s_0)$ up to an angle $\check \phi_0$ determined by $\bar \phi \in \check \phi_0 + \partial \tilde \zeta(\check \phi_0) + 2\pi$: $\tilde \zeta(s;s_0)$ is the spiral corresponding to $\tilde r(\phi;s_0)$. This angle can be either the initial angle $\phi_0$, or along the level set arc (and in this case $\bar \phi = \check \phi_0 + \frac{5}{3}\pi$) or a prolongation of the final segment $[P_1,P_2]$ ($\bar \phi = \phi_0 + \frac{\pi}{2} + \Delta \phi + 2\pi$), or in the saturated region ($\bar \phi = \check \phi_0 + 2\pi + \bar \alpha$). Let $s_1$ be the corresponding length at the angle $\check \phi_0$, $s_1 = s(\check \phi_0)$. \\
%If we repeat the construction of the previous section stating from $s_1$, and denote with $\tilde r'(\phi;s_1)$ the new fastest saturated spiral, it follows that $\tilde r'(\phi;s_1) = \tilde r(\phi;s_0)$ because both are the fastest saturated spiral. However the derivative $\delta \tilde r'$ could be negative at $\bar \phi$: indeed this happens if we are in the negativity region of the segment or the arc case. It is thus convenient for the spiral to follow a segment with direction $\bar \phi$ until the derivative $\delta \tilde r'$ becomes $0$, and at this point one closes with the fastest closing spiral. \\
%Depending on the structure of the spiral up to $s_1 = s(\check \phi)$, the segment in the direction $\bar \phi$ ends with a level set arc or with a segment: in both cases we are on the boundary of the negativity region, i.e. in the arc case the angle between the tangent to the level set and $\bar \phi$ is given by $h_1(\Delta \phi)$ (Equation \eqref{Equa:theta_Deltaphi_rel}), while in the segment case the angle between $\bar \phi$ and the segment for the fastest closing spiral is $\check \theta_0$ (Equation \eqref{Equa:hat_theta_det_666}). The various cases in the segment case are presented in Fig. \ref{fig:tent:solution}, while Fig. \ref{Fig:checkr_notation} is the most general case, and will serve as a reference for notations.
%

The first main result of this section is the definition of the optimal closing spiral $\check r(\phi;s_0)$ given the spiral arc $\zeta([0,s_0])$ and the final angle $\bar \phi$. This is the done in the first part of Section \ref{Ss:optimal_sol_def}, which contains also the proof that such a definition yields a unique spiral $\hat r(\cdot;s_0)$ (Proposition \ref{Prop:unique_optimal_guess}:

\begin{proposition}(Proposition \ref{Prop:unique_optimal_guess})
\label{Prop:unique_optimal_guess_intro}
Given $s_0 = s(\phi_0) \geq 0$ and an angle $\bar \phi \geq \phi_0$, there exists a unique optimal spiral candidate $\check r(\phi;s_0)$.
\end{proposition}

Such a statement is not elementary, indeed one has to rule out the possibility that when $P_1$ moves along the direction $\bar \phi$ is may reenter the negativity region. In the segment case this is easy, but in the arc case (i.e. when in the point $P_1$ the fastest saturated spiral starts with an arc) it is not, due to the more complicated structure of the negativity region \gls{Narc} for the arc perturbation.

The most common geometric situation for the perturbation is as in Fig. \ref{Fig:optimal_intro}: the last round starts with a segment in the direction $\bar \phi$ followed by the fastest saturated spiral starting again with a segment. We say it is the most common because the other case (i.e. the fastest saturated spiral starts with an arc in $P_1$) requires that the point $P_0$ is close to the last point of the given spiral arc $\zeta(s_0)$: roughly speaking, this is a regularity property of the fastest saturated spiral $\tilde r(\cdot;s_0)$, i.e. after less than 1 round after $s_0$ the spiral is already close to the saturated spiral. \\
We call \emph{tent} this two consecutive segments configuration. In Section \ref{Ss:comput_tent_new} we study the equations describing a spiral with a tent, obtaining the formulas which allows to compute how much the final tent in $\hat r(\cdot;s_0)$ is going to perturb the fastest saturated spiral $\tilde r(\cdot;s_0)$ in the last round. Lemma \ref{Lem:relation_admissibility_tent} explicitly computes these formulas, and being linear relations the same formulas holds for the perturbation (Corollary \ref{Cor:tent_corol_for_pert}. \\
Next, with these relations, we can check which condition are required in order to be not the admissible solution: in other words, the tent is not an admissible spiral, which in this particular case means that $s \mapsto u(\zeta(s))$ is not monotone (and then we are forced to follow an arc of the level set of $u$). It turns out that, if the the initial point $P_0$ of the tent is saturated, a necessary condition is that the length of the spiral at the previous round is much larger than the estimate of Proposition \ref{Cor:bound_length_gen_intro} (Lemma \ref{Lem:when_tent}). One thus concludes that it $P_0$ is saturated, then the optimal spiral has a tent:

\begin{proposition}(Proposition \ref{Prop:tent_admissible})
\label{Prop:tent_admissible_intro}
The tent is admissible (and then is the optimal candidate) in the saturated part of $\tilde r(\cdot;s_0)$.
%\begin{equation*}
%\tau \geq 1 - \hat \tau - \frac{\tan(\bar \alpha)}{2\pi + \bar \alpha} \ln \bigg( \frac{2.08}{\frac{e^{\cot(\bar \alpha) \hat \theta}}{K_\mathrm{tent}} - 1} \bigg) = 0.277638.
%\end{equation*}
\end{proposition}

We remark that in the non saturated part of $\tilde r(\cdot;s_0)$, i.e. when $\phi$ is close to $\phi_0$, the tent is in general not the admissible spiral solution, see the example of Remark \ref{Rem:inital_tent}.

The last result of this section is a formula based on a simple observation, Lemma \ref{Lem:final_value_satu}, which allows to prove that the derivative $\delta \check r(\bar \phi;s_0) = \frac{d}{ds_0} \check r(\bar \phi;s_0)$ is positive if $\delta \tilde r(\bar \phi;s_0) = \frac{d}{ds_0} \tilde r(\bar \phi;s_0)$ is. This formula can be applied only after 2 rounds, so that in the following we have to address what happens in these initial part of $\check r$ when $\bar \phi$ is close to $\phi_0$. One can rightly suspect that the non smoothness of $\delta \tilde r$ is the problem.


\bigskip


The last three sections address the homotopy argument starting from the optimal solution candidate and proving that the derivative $\delta \check r(\bar \phi;s_0)$ is increasing.


\subsubsection{Section \ref{S:optimal_sol_candidate}}
\label{Sss:optimal_sol_cand_intro}


This section is devoted to the construction of the optimal solution candidate for any given $\bar \phi$. The solution \gls{roptim} will depends on the angle $\bar \phi$, and thus its structure is more articulate than the fastest saturated spiral of Section \ref{Sss:case_study_intro}. We refer to Fig. \ref{Fig:opt_spiral_intro} for the description of the solution $r_\mathrm{opt}$.

\begin{figure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{spiral_opt_first_intro.pdf_t}}
\caption{The optimal solution for $\bar \phi \in [0,2\pi + \frac{\pi}{2} - h_1]$.}
\label{Fig:spiral_opt_first}
\end{subfigure} \hfill
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{opt_sol_1.pdf_t}}
\caption{The optimal solution for $\bar \phi \in 2\pi + \frac{\pi}{2} + [- h_1,0]$.}
\label{Fig:spiral_opt_first_2}
\end{subfigure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{opt_sol_2.pdf_t}}
\caption{The optimal solution for $\bar \phi \in 2\pi + \frac{\pi}{2} + [0,h_2]$.}
\label{Fig:spiral_opt_first_3}
\end{subfigure} \hfill
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{opt_sol_2_tent.pdf_t}}
\caption{The optimal solution for $\bar \phi \in 2\pi + \frac{\pi}{2} + [h_2,\tan(\bar \alpha)]$.}
\label{Fig:spiral_opt_first_4}
\end{subfigure}
\caption{The optimal solution depending on the final angle $\bar \phi$ for the first round.}
\label{Fig:opt_spiral_intro}
\end{figure}

The first situation is the $\bar \phi$ is the first round, more precisely $\bar \phi \in [0,2\pi + \frac{\pi}{2} - h_1]$, where the constant $h_1$ is computed explicitly by the results of Section \ref{S:family}: it is $\theta$ coordinates of the unique point on the border of the negativity region \gls{Narc} for $\Delta \phi = \tan(\bar \alpha)$. In this case the optimal solution coincides with the fastest saturated spiral of Section \ref{Sss:case_study_intro}: see Fig. \ref{Fig:spiral_opt_first}.

After the angle $2\pi + \frac{\pi}{2} - h_1$, the derivative $\delta \tilde r(\bar \phi;0)$ is negative: hence the optimal solution has a initial segment of length $h$ in the direction $\bar \phi$, then it is the fastest saturated solution starting with an arc of the level set, Fig. \ref{Fig:spiral_opt_first_2}.

For $\bar \phi \in 2\pi + \frac{\pi}{2} + [0,h_2]$, the optimal solution candidate starts with an arc of the level set $\partial B_1(0)$, then a segment in the direction $\bar \phi$ and next the last round is the fastest saturated spiral, Fig. \ref{Fig:spiral_opt_first_3}. The value $h_2$ is computed explicitly in Section \ref{Ss:optimal_cand_3}, and corresponds to the transition from the arc case to the segment case for the fastest saturated spiral of the last round, Fig. \ref{Fig:spiral_opt_first_4}.

\begin{figure}
\resizebox{.75\textwidth}{!}{\input{opt_sol_3_tent.pdf_t}}
\caption{The optimal candidate $r_\mathrm{opt}(\phi)$ for $\bar \phi \geq 2\pi + \tan(\bar \alpha) + \frac{\pi}{2}$.}
\label{Fig:opt_sol_3_tent_intro}
\end{figure}

Finally, for $\bar \tau > 2\pi + \tan(\bar \alpha) + \frac{\pi}{2}$, the solution is the fastest saturated spiral up to the angle $\bar \phi - 2\pi - \bar \alpha$, followed by the tent case as described in Section \ref{Sss:optimal_solut_intro}, see Fig. \ref{Fig:opt_sol_3_tent_intro}.

The main result of this section is that this construction yields a unique spiral barrier which is positive:


\begin{proposition}[Propositions \ref{Prop:e_opt_large_phi} and \ref{Prop:postiv_aympt}]
\label{Prop:e_opt_large_phi_intro}
The optimal solution $r_\mathrm{opt}$ is positive for all $\bar \phi$ and for large angles can be estimated as %growth exponentially as
\begin{equation*}
r_\mathrm{opt}(\bar \phi) = 0.976359 r(\bar \phi) + \mathcal O(1)
\end{equation*}
where $r(\bar \phi)$ is the fastest saturated spiral
\end{proposition}

A remark is natural here: the gain of optimality is about 2.25\% w.r.t. the fastest saturated spiral, so one may suspect that there are some simpler proof of this result. Besides the fact that knowing the optimal solution is not a trivial fact, the difficulty in obtaining estimates is due to the RDE satisfied by $r(\phi)$, which makes comparisons difficult. One the other hand this method can be applied also for speeds which are not the critical one, and also to other geometric situations.


\subsubsection{Sections \ref{S:segment_case} and \ref{S:arc_1}}
\label{Sss:final_case_opt_intro}


At this point, having proved that for any given spiral barrier $\zeta$ the one can construct the one parameter family of spirals $\check r(\cdot;s_0)$ starting from $r_\mathrm{opt}$ and ending in $\zeta$, we are left to prove that $s_0 \mapsto \check r(\bar \phi;s_0)$ is increasing for all $\bar \phi$, thus effectively removing the negative regions of Proposition \ref{Prop:regions_pos_neg_segm_intro} (and Proposition \ref{Prop:neg_region} in the arc case) because of the additional perturbation to $\tilde r(\cdot;s_0)$. Since the structure of $\check r(\cdot;s_0)$ is more complicated, we have to consider several geometric situations, depending on the relative distance of $\bar \phi$ from $\phi_0$ and the structure of $\tilde r(\cdot;s_0)$.

\begin{figure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{segm_segm_sat_6.pdf_t}}
\caption{Segment-segment case.}
\label{Fig:deltacheckr_1}
\end{subfigure} \hfill
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_2.pdf_t}}
\caption{Segment-arc case.}
\label{Fig:deltacheckr_2}
\end{subfigure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{arc_segm_1.pdf_t}}
\caption{Arc-segment case.}
\label{Fig:deltacheckr_3}
\end{subfigure} \hfill
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_3_bis.pdf_t}}
\caption{Arc-arc case..}
\label{Fig:deltacheckr_4}
\end{subfigure}
\caption{The 4 main geometric situations for the optimal solution $\check r$.}
\label{Fig:deltacheckr}
\end{figure}

There are 4 main cases, each one with several subcases:
\begin{enumerate}
\item $\tilde r(\cdot;s_0)$ starts with a segment and its perturbation $\check r(\cdot;s_0)$ has an additional tent, Fig. \ref{Fig:deltacheckr_1}: we call it the \emph{segment-segment case};
\item $\tilde r(\cdot;s_0)$ starts with a segment and its perturbation $\check r(\cdot;s_0)$ end with an arc, Fig. \ref{Fig:deltacheckr_2}: we call it the \emph{segment-arc case};
\item $\tilde r(\cdot;s_0)$ starts with an arc and its perturbation $\check r(\cdot;s_0)$ has an additional tent, Fig. \ref{Fig:deltacheckr_3}: we call it the \emph{arc-segment case};
\item $\tilde r(\cdot;s_0)$ starts with an arc and its perturbation $\check r(\cdot;s_0)$ ends with an arc, Fig. \ref{Fig:deltacheckr_4}: we call it the \emph{arc-arc case}.
\end{enumerate}

The almost 20 subscases are due to the relative position of the final segment-arc and the initial segment-arc: referring for example to Fig. \ref{Fig:deltacheckr_1}, the tent may start inside the cone of opening $\theta$, instead that afterwards as depicted. Since this region is exactly when $\tilde r$ is discontinuous (it has also a Dirac-delta!), we did not find a general way of reducing these cases to a general situation, and we analyze them one by one.

It is important to notice that, because of Proposition \ref{Prop:tent_admissible_intro}, the segment-segment or arc-segment case are the only possibilities after some small initial angle of rotation, and this fact greatly simplify the analysis: for example, we do not need to study the arc-arc case for large angles.

The main result are a series of lemmata, which state that the derivative $\delta \check r(\bar \phi;s_0)$ is positive: we collect their statements into the following:

\begin{proposition}
\label{Prop:deltacheckr_intro}
For a.e. every choice of $0 \leq \phi_0 < \bar \phi$ it holds $\delta \check r(\bar \phi;\phi_0) \geq 0$, with the equality only if $\dot \zeta(\phi_0+)$ is tangent to the optimal spiral $\check \zeta(\phi_0+;\phi_0)$.
\end{proposition}

This gives the proof of Theorem \ref{Theo:main_extended}, and concludes the paper.











%
%discuss here the general idea of our approach: let $Z=\zeta([0,S])$  be an admissible spiral-like strategy and let $(r(\phi),\phi)$ be its parametrization by radius (see again Theorem \ref{thm:param}). 
%Assume that for every point $\zeta(s)$ of the barrier you can assign a \emph{generalized} spiral $Z_s$ coinciding with $Z$ up to the point $\zeta(s)$ and parametrized by $(f_s(\phi),\phi)$, that is
%\begin{definition}[Family of Generalized Barriers]\label{def:fam:pert}
% We say that $f_{s}\in\text{SBV}([0,+\infty);\R)$, with $s\in[0,S]$, is an element of the family of generalized barriers $\mathcal F_Z$ if:
% \begin{itemize}
%     \item $f_0(\phi)> 0$ for $\phi\in[0,+\infty)$;
%     \item $f_s(\phi)=r(\phi)$ for every $\phi\leq\bar\phi$ whenever $\zeta(s)=(r(\bar\phi),\bar\phi)$.
%      \end{itemize}
%     Moreover, we say that it is a \emph{diverging family} if, calling \begin{equation}\label{eq:derivative:family}
%         \bar f_s(\phi)=\lim_{h\to 0}\frac{ f_{s+h}(\phi)-f_s(\phi)}{h},
%     \end{equation}
%     then $\bar f_s(\phi)\geq 0$ for every $\phi\in[0,\infty)$.
%
% \end{definition}
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{familyofspirals.png}
%     \caption{At every point an element of the family of generalized barriers is assigned.}
%     \label{fig:fam:of:spirals}
% \end{figure}
% See Figure \ref{fig:fam:of:spirals}.
%We remark that the parametrization of the optimal barrier $Z$ chosen at the beginning is an element of any family of generalized barriers, since it is $f_{S}$ accordingly to the previous notation. 
%We remark that a family of generalized barriers is NOT in general a family of admissible barriers, but it is a family of functions parametrized by the length parameter $s$. Indeed, it is not required that $Z_s$ are admissible or even that $(f_s(\phi),\phi)$ is a parametrization by angle as in the case of spirals. The family has only to satisfy all the assumptions in Definition \ref{def:fam:pert}.
%
%If a diverging family of generalized barriers exists, then no spiral-like strategy confines the fire, indeed:
%\begin{theorem}\label{thm:adm:diverg:family}
%Let $Z$ be as before and assume that there exists a family of generalized barriers $\lbrace f_s\rbrace=\mathcal F_Z$ which is diverging. Then $Z$ does not confine the fire.
%\end{theorem}
%The proof of this fact is very easy and relies on the following observation:
%by the fundamental theorem of calculus we have that
%\begin{equation*}
%    f_s(\phi)=f_0(\phi)+\int_0^s \bar f_{\eta}(\phi)d\eta.
%\end{equation*}
%By the diverging condition on the family $\mathcal F_Z$ it holds then that
%\begin{equation*}
%    f_s(\phi)\geq f_0(\phi),\quad\forall \phi\geq 0,\forall s\in[0,S], 
%\end{equation*}
%therefore
%\begin{equation*}
%    f_S(\phi)\geq f_0(\phi)> 0,
%\end{equation*}
%by the first assumption on the family. But since $f_S(\phi)$ is $r(\phi)$ one concludes that the radius of $Z$ is always positive. This also proves that $f_0(\phi)$ is the \emph{best} strategy we can do, since $r(\phi)\geq f_0(\phi)$ for every $\phi$. Here best refers to another optimization problem that we will discuss in a while (see Proposition \ref{Prop:opt:problem}).
%
%\medskip 
%Setting the framework of generalized barriers for the study of spirals has been extremely hard. One of the main issues of this procedure is that,
%in general, finding a diverging family of generalized barriers is a really difficult task. We did many attempts in order to exhibit an example of such a family, since the most reasonable failed to be correct (here the need to introduce the concept of \emph{generalized} barriers). Another important issue is that the proofs of these results are based on  numerical computations, so that it is extremely hard to take under control how the strategies evolve. The possibility to perform an analytical proof of these results is currently under investigation, but we strongly believe that the use of machine-based computations is always needed. 
%
%On the other side, we are strongly convinced that this new method to prove the non-admissibility of strategies could be promising in the study of the fire problem and could be adapted to more general cases involving internal barriers, therefore towards a proof of Bressan's Fire Conjecture in full generality.
%
%\subsection{Construction of the family of generalized barriers.}
%Summarizing, in order to prove the non-admissibility of spiral-like strategies, we need to find a diverging family of generalized barriers $\lbrace f_s\rbrace$. Let $Z$ be an admissible spiral, then for every $P\in Z$ the Admissibility Functional $\mathcal{A}$ reads as
%\begin{equation*}
%    \mathcal{A}(P)=u(P)-\frac{1}{\sigma}L(P)\geq 0,
%\end{equation*}
%where $L(P)$ is the length of the spiral from the starting point until the point $P$.
%
%We consider then the following \textbf{Optimization Problem}: fix any $\bar\phi$ angle, then the minimization problem is
%\begin{equation}\label{eq:mim:probl}
%    \min_{\tilde Z\in \mathcal A_S(Z,\bar\phi)} r_{\tilde Z}(\phi),\quad\text{ for some } \phi\geq\bar\phi,
%\end{equation}
%where $\mathcal{A}_S(Z,\bar\phi)$ denotes the class of admissible spirals (not necessarily blocking) that coincide with $Z$ up to the angle $\bar\phi$, with length uniformly bounded by a constant $N>>1$, and if $\tilde Z\in\mathcal{A}_S(Z,\bar\phi)$, then $(r_{\tilde Z}(\phi),\phi)$ will denote its parametrization by angle.
%Differently from what stated for the optimization problem \eqref{eq:opt:problem}, for which it has been proved that the minimum exists among admissible blocking strategies (therefore in a class that could be empty) \cite{Bressan_deLellis}, here the class of strategies is non-empty, since we are not assuming that they confine the fire in general. 
%
%
%
%Then we have the following geometric result (which is the content of Section \ref{S:exist_opti_traj}), that gives the minimum of the previous problem in the assumption $\phi\in[\bar\phi,\bar\phi+2\pi]$: 
%
%\begin{proposition}\label{prop:best:first:Enclosure}
%    Let $Z$ be an admissible spiral-like strategy and let $(r(\phi),\phi)$ be its parametrization by angle. Fix any $\bar\phi$ and consider the following strategy $\hat Z$ parametrized by $(\hat r(\phi),\phi)$ such that:
%    \begin{itemize}
%        \item $\hat r(\phi)=r(\phi)$ for every $\phi\leq\bar \phi$;
%        \item  $(r(\phi),\phi)\subset\lbrace u=u((r(\bar\phi),\bar\phi)\rbrace$ for $\phi\in[\bar\phi,\bar\phi+\Delta\bar\phi]$ (it is a subset of the level set of the minimum time function $u$);
%        \item $(r(\phi),\phi))$ for $\phi\in[\bar\phi+\Delta\bar\phi=\phi_1,\phi_2]$ is a segment of endpoints $P_1,P_2$ such that $P_1\in \lbrace u=u((r(\bar\phi),\bar\phi)\rbrace$ and $P_2$ is saturated, that is $\mathcal{A}(P_2)=0$. Moreover the segment $P_1P_2$ is tangent to $\lbrace u=u((r(\bar\phi),\bar\phi)\rbrace$ in $P_1$.
%        \item for every $\phi\geq \phi_2$ $\hat Z$ is a saturated spiral, that is $\mathcal{A}(r(\phi),\phi)=0$.
%    \end{itemize} Then we have that, for $\phi\in [\bar\phi,\bar\phi+2\pi]$ it holds
%    \begin{equation*}
%        r(\phi)\geq \hat r(\phi).
%    \end{equation*}
%\end{proposition}
%In Section \ref{S:exist_opti_traj} we prove that a minimizer for the problem \eqref{eq:mim:probl} always exists, but determining its exact shape for angles $\phi>>\bar\phi$ is an open problem.
%
%Since by the definition of diverging family of generalized barriers one naturally gets $r(\phi)\geq f_0(\phi)$ for every $\phi$ (so that $f_0$ is a minimizer!) we expected that the correct guess for the family was precisely the one suggested by the previous proposition. 
%
%\medskip
%At each point $P=\zeta(s)$ of the spiral the element of the family $f_s(\phi)$ is the length of the radius of a spiral-like strategy $Z_s$ (not necessarily admissible), with parametrization by angle given by $(f_s(\phi),\phi)$ with the following properties: it is a subset of the level set $\lbrace u=u(P)\rbrace$, then it continues as a segment whose last endpoint is saturated (in the sense the admissibility functional is zero at that point) and then it is a saturated spiral, in the sense that every point on the spiral is saturated. This is precisely the optimal found in Proposition \ref{prop:best:first:Enclosure}.
%
%
%
%Actually, it turned out that this construction did not produce a diverging family of generalized barriers since there was always a tiny region of parameters in which $\bar f_{s}<0$. Inspired by this (negative) result, after many attempts, we found out instead that the best strategy a player can do in order to confine the fire is to speed up the construction up to the critical value $2.144..$ (which is the maximum amount of speed we have for spirals not confining the fire, as conjectured in \ref{conj:spiral}), more precisely: from the point $\zeta(s)$, the strategy $Z_s$ is an an arc (subset of the level set of $u$), a segment (whose last point is saturated for the admissibility functional defined in \eqref{eq:sat:family}) and then it is a saturated spiral, but this time for the critical value $\sigma=2.6144...$. We underline that this is not a family of admissible barriers, since we are using a construction speed which is higher than the one available ($\leq 2.3$ in this case), but every element is a \emph{generalized} barrier. Computations show that in this case $\bar f_s>0$, therefore this family is diverging and it is the right one to consider for proving Theorem \ref{thm:main}. We remark that the value $2.3$ is 'sharp' up to numerical computations, indeed this procedure does not work for the value $2.4$. 
%
%The construction of this family gives the proof for the following 
%\begin{theorem}
%    If $\sigma\leq 2.3$ there exists a diverging family $\lbrace f_s\rbrace=\mathcal F_Z$ of generalized barriers.
%\end{theorem}
%This is the content of the last section. The main observation to carry out the proof is that, given two elements of the family $f_s$ and $f_{s+\delta s}$, then 
%$f_{s+\delta s}$ and $f_s$ for $\phi>>\bar\phi$ are the radii of saturated spirals, that is they satisfy the RDE \eqref{eq:ODE:saturated:1} for the critical speed. By linearity of the problem,  the derivative
%\begin{equation*}
%    \bar f_s(\phi)=\lim_{\delta s\to 0} \frac{f_{s+\delta s}(\phi)-f_s(\phi)}{\delta s}\qquad\text{ a.e } s,
%\end{equation*}
%satisfies the same RDE. To prove then its positivity, we need to use the \textbf{change of variables} \eqref{eq:change:var:1}. Therefore the study of the derivative $\bar f_s$ relies on a careful study of the solution of the same RDE.
%
%We conclude remarking that, even if a probably different proof is required in order to deal with the critical case $\sigma=2.6144..$, one could investigate extension of this procedure (weakening the diverging hypothesis of the family) in order to reach at least the values $2.4\sim 2.5$. We want also to underline that in this approach the presence of internal barriers seems to have no concrete role: it is a current object of investigation possible extension of the approach of generalized barriers to more general cases. 
%\subsubsection{Plan of the discussion.}
%In Section \ref{s:admissible:barriers} we give some notations and we define spiral-like strategies Definition \ref{def:adm:spirals}. We define the parametrization by angle $(r(\phi),\phi)$ Theorem \ref{thm:param}, which is motivated by the geometry of fire rays (Lemma \ref{lem:fire:rays}. In Section \ref{S:ODE} we derive the retarded differential equation associated to any admissible spiral (Lemma \ref{lem:ODE:spiral}). We study then in detail the RDE for a saturated spiral \eqref{eq:ODE:saturated} and we compute its spectrum in Subsection \ref{ss:dde}, Lemma \ref{lem:real:Eigenvalues} and Lemma \ref{lem:complex:eigenvalues}. In Subsection \ref{sss:subset:saturated} we prove that starting from any admissible spiral, if the player start constructing with speed $>2.6144..$ then it manages to confine the fire. In Subsection \ref{sss:important} we study the change of variable \eqref{eq:change:var:1} which will be of key importance for all the following results and we prove that the saturated spiral does not confine the fire for $\sigma\leq 2.6144..$ (Proposition \ref{prop:saturated:not:closed}). In Section \ref{S:exist_opti_traj} we study the optimization problem \ref{eq:mim:probl} and some properties of the minimum time function, previously defined. the results lead to the construction of the minimizer (at least for small angles) In Subsection \ref{Ss:minimal_reach}. In Section \ref{S:case:study} we focus on the first element of a family of generalized barrier $Z_0$ accordingly to the definition \ref{def:fam:pert} and we prove that $f_0(\phi)>0$ for every $\phi$, thus verifying the first condition on the family of generalized barriers. Finally, in Section \ref{c:family} we exhibit an example of a diverging family $\lbrace f_s\rbrace$ of generalized barriers and we compute the derivative $\lbrace \bar f_s\rbrace$. Here we distinguish between two cases: the first one in the assumption that the portion of strategy constructed on a level set of the minimum time function is not a single point (arc case, Subsection \ref{S:arc}), and the second one in the assumption it is a single point (segment case, Subsection \ref{S:segment}). In the Appendix \ref{S:appendix: fire} we give the numerical evaluations of functions needed for the proof of our results. 
%
%
%{\color{blue} {\bf DA SPOSTARE NELL'INTRODUZIONE} In this section we start with the construction of an optimal solution for the problem of Theorem \ref{Theo:exists_min}.
%
%More precisely, we will prove the following: given an admissible spiral $r(\phi)$, $0 \leq \phi \leq \bar \phi$, and an angle $\phi_0$, we prolong this spiral for $\phi > \phi_0$ as an admissible spiral $r(\phi;s_0)$, $s_0 = s^+(\phi_0)$, by assigning the angle of $\beta(\phi)$ for $\phi > \phi_0$. Let $\bar r(\phi) = r(\phi;0)$, which is independent of the spiral $r(\phi)$: it is indeed the unique spiral of the family starting from the point $(1,0)$.
%
%In this way we construct a continuous path
%\begin{equation*}
%    s_0 \mapsto r(\phi;s_0),
%\end{equation*}
%with the properties that
%$$
%r(\phi,0) = \bar r(\phi), \quad r(\phi;\bar \phi) = r(\phi).
%$$
%Next, we will show that for almost every $\phi$ there exists the limit
%\begin{equation*}
%    \lim_{\delta s_0 \to 0} \frac{r(\phi,s_0 + \delta s_0) - r(\phi,s_0)}{\delta s_0} = \delta r(\phi;s_0),
%\end{equation*}
%and the function $\phi \mapsto \delta r(\phi;s_0)$ satisfies an explicit RDE. In particular, we can compare the given spiral $r(\phi)$ with the spiral $\bar r(\phi)$ by
%\begin{equation}
%\label{Equa:deriv_integr_r}
%    r(\phi) = \bar r(\phi) + \int_0^{s^+(\phi)} \delta r(\phi;s) ds.
%\end{equation}
%
%The key point of the proof is the following
%
%\begin{theorem}
%    \label{Theo:optimality_check}
%    Assume that for every admissible spiral $r(\phi)$ the family $\{r(\phi;s_0)\}_{s_0 \in [0,S]}$ is a family of admissible spirals (Definition \ref{def:adm:spirals}) and for a.e. angle $\phi$ the map
%    \begin{equation*}
%        s_0 \mapsto r(\phi,s_0)
%    \end{equation*} 
%    is Lipschitz. If
%    \begin{equation*}
%        \delta r(\phi;s_0) := \lim_{\delta s \searrow 0} \frac{r(\phi,s_0 + \delta s_0) - r(\phi,s_0)}{\delta s_0} \geq 0,
%    \end{equation*}
%    for all $\phi$, then the following hold:
%    \begin{enumerate}
%        \item the spiral $r(\phi;s_0)$ is a minimum for Theorem \ref{Theo:exists_min} in the set of spirals $r'(\phi)$ such that
%        \begin{equation*}
%            r'(\phi) = r(\phi) \quad \forall \phi \leq \phi_0;
%        \end{equation*}
%        \item the base spiral $\bar r(\phi) = r(\phi;0)$ is an optimal solution of Theorem \ref{Theo:exists_min};
%        \item if moreover $\delta r(\phi;s_0) > 0$ for all $\phi >\phi(s_0)$, $s_0=s^+(\phi(s_0))$, unless
%        \begin{equation*}
%            \frac{d^+r}{ds} \rest_{s = s_0} = \frac{d^+r(s;s_0)}{ds} \rest_{s_0}, 
%        \end{equation*}
%        then $r(\phi;s_0)$ is the unique optimal solution for the closing problem starting at $\phi_0$ with a given admissible spiral $r(\phi)$ $\phi \in [0,\phi_0]$, and $\bar r(\phi)$ is the unique optimal solution for the closing problem.
%    \end{enumerate}
%\end{theorem}
%
%\begin{proof}
%    Formula \eqref{Equa:deriv_integr_r} gives the first two points. For the last one, since $s_0 \mapsto \frac{d^+r(s;s_0)}{ds} \rest_{s_0}$ is a given function, it follows that every optimal spiral has $\frac{dr}{d\phi}$ determined a.e.. In particular, being the discontinuous part only due to the curvature of the previous round, the function is uniquely determined by the construction of Theorem \ref{Prop:construct_spiral}. 
%\end{proof}
%
%Note that the uniqueness of the third point implies that if $r'(\phi;s_0')$ is the optimal spiral starting at $s_0' \geq s_0$ for the spiral $r(\phi;s_0)$, then $r'(\phi;s_0') = r(\phi;s_0)$.
%
%In order to construct the family $r(\phi;s_0)$ as required in the theorem, we need some preliminary analysis of an almost optimal candidate $\tilde r(\phi;s_0)$: the analysis of this family is the base for the construction of the optimal family $r(\phi;s_0)$. We will call this family \emph{the saturated family}, emphasizing the idea of being the fastest admissible spiral becoming saturated and remaining so.
%
%The family $\tilde r(\phi;s_0)$ is constructed in this section, while the construction of $r(\phi;s_0)$ will be studied in the next one.
%%{\color{blue} qui dobbiamo giustificare la scelta di $r$? Nono qui, metterei dopo, ma tanto lo rileggiamo}
%\begin{remark}
%    \label{Rem:more_than_one_round}
%    Note that we can assume that the optimal closing spiral is not closing for at least one round: indeed by Theorem \ref{Cor:curve_cal_R_sat_spiral} the structure of the last round is already known.
%\end{remark}
%
%\begin{comment}
%{\color{gray}
%In this section we will exhibit an example of a diverging family of generalized barriers. The computations that the construction requires rely on the evaluation of some trascendental functions, in the spirit of what has been done in Theorem \ref{thm:case:a} of the previous section, where we have analyzed concrete examples of admissible barriers and we have proved that they do not confine the fire. Here, we fix $\hat \sigma = 2.3$ and
%\begin{equation*}
%    \hat \alpha = \arccos \left( \frac{1}{\hat\sigma} \right),
%\end{equation*}
%while $\bar \sigma=2.6144..$ is the critical speed and $\bar \alpha$ denotes the corresponding angle. We consider also $Z = \zeta([0,S]) \in \mathcal{A}_S$ an admissible spiral, where $(r(\phi),\phi)$ denotes its parametrization by angle (Theorem \ref{thm:param_1}). For every point $\zeta(s)$ of the barrier we can assign an element of a family of generalized barriers, according to the following definition. (DA RIVEDERE L'INTRODUZIONE)
%
%Let $Z$ be an admissible spiral, and fix a length $\bar s$: this spiral is the one we have to evaluate, and sometimes will be referred as \emph{base spiral}.
%
%\begin{definition}[Family of Generalized spirals]
%\label{Def:fami_gene_barri_6}
%A spiral $Z_{\bar s} = \zeta_{\bar s}([0,+\infty))$ is a \emph{generalized spiral originating at $\zeta(\bar s)$} if, when represented in the fire coordinates $r_{\bar s}(\phi)$, it holds
%\begin{itemize}
%    \item $r_{\bar s}(\phi) > 0$ for $\phi \in [0,+\infty)$;
%    \item $r_{\bar s}(\phi) = r(\phi)$ for every $\phi \leq \bar \phi$, where $\bar \phi$ is the rotation angle corresponding to the length $\bar s$ for the base spiral, and $r(\phi)$ is the representation of $Z$ according to the fire coordinates (Theorem \ref{thm:param_1}). % whenever $\zeta(s)=(r(\bar\phi),\bar\phi)$.
%\end{itemize}
%
%A \emph{family of generalized spirals $\{Z_s\}_{s \in [0,S]}$} is a set of generalized spirals originating at every $s \in [0,S]$ of the domain of $\zeta$.
%
%The family of generalized spirals is a \emph{diverging family} if it is monotone w.r.t. $s$, i.e.
%\begin{equation*}
%    s \mapsto r_{s}(\phi) \quad \text{is monotone for all $\phi \in [0,\infty)$.}
%\end{equation*}
%\end{definition}
%
%The essential difference w.r.t. admissible spirals is that we do not require $\zeta_{\bar s}$ to be admissible. Looking into the proof of Theorem \ref{thm:adm:diverg:family}, one sees that this is not necessary, even if the speed of exponential growth is affected by the particular family we consider: indeed, since we will prolong $Z$ (constructed with speed $\hat \sigma = 2.3$) with spirals which are admissible for the faster speed $\bar \sigma = 2.61...$, we will obtain an exponential growth as for the critical case, which is lower than the exponential growth for the family of Section \ref{S:case:study}.
%
%In the following we will construct a family of generalized spirals which is differentiable w.r.t. $s$, and thus we will study the positivity of its derivative w.r.t. the starting point $\bar s$:
%\begin{equation}
%\label{eq:derivative:family}
%    \bar r_s(\phi) = \lim_{h \to 0} \frac{r_{s+h}(\phi) - r_s(\phi)}{h}.
%\end{equation}
%(MA SERVE QUESTA FORMULA QUI?) No però lasciamola, meglio una cosa in più
%
%%The construction of a diverging family of generalized spirals is necessary for the proof of Theorem \ref{thm:main}, whose proof follows by Theorem \ref{thm:adm:diverg:family}.
%
%The main result of this section is the following
%
%\begin{theorem}
%\label{thm:main:2}
%    If $\hat \sigma \leq 2.3$ there exists a diverging family $\lbrace r_s \rbrace_{s \in [0,S]} = \mathcal F_Z$ of generalized barriers, exponentially growing as in Theorem \ref{thm:case:a}.
%\end{theorem}
%
%Before diving into the proof, which requires several steps and some numerical evaluation of trascendental functions and it is the content of the next sections, we give a geometric intuition of the construction done below.
%
%The fundamental idea is to prolong the explicit solution for the optimal closing spiral. \\
%More precisely, for fixed angle $\bar \phi$, corresponding to a spiral length $\bar s$ for the base spiral $\zeta$, Theorem \ref{Cor:curve_cal_R_sat_spiral} gives the optimal closing barrier $\zeta_{\bar s}$ for angles $\phi \in [\bar \phi,\bar \phi + 2\pi + \beta^-(\bar \phi)]$. A first attempt is thus to continue $\zeta_{\bar s}$ as a saturated spiral for angles $\phi \geq \bar \phi + 2\pi + \beta^-(\bar \phi)$.
%%A possible candidate for the family is given following the geometric intuition of Section \ref{S:exist_opti_traj}. We recall that we have proved that, fixed any angle $\bar\phi$, the best strategy we can construct for $\phi\in[\bar\phi,\bar\phi+2\pi+\theta_0]$ where $\beta(\bar\phi)=\theta_0$ (Corollary \ref{Cor:curve_cal_R_sat_spiral}) is the one given by the union of a subset of the level set $u^{-1}(u(r(\bar\phi),\bar\phi))$, a segment tangent to it whose last point is saturated and then a saturated spiral. In Chapter  \ref{S:case:study} we have then proved that the strategy made by a circle, a segment tangent to it and a saturated spiral, does not confine the fire, which gives precisely the proof that $f_0$, which is the first element of the family of generalized barriers, is always strictly positive. 
%Even if perfectly reasonable, this family $f_s$ turned out to be non-diverging (see Definition \ref{def:fam:pert}), since in some cases $\bar r_s \leq 0$: the wrong sign of the derivative $\bar r_s$ happens already for the speed $\hat \sigma = \frac{1 + \sqrt{5}}{2}$ of Theorem \ref{thm:klein}. The explanation of this is that the continuation of the optimal closing solution of Theorem \ref{Cor:curve_cal_R_sat_spiral} as a saturated spiral is not the optimal closing solution for angles $> \bar \phi + 2\pi + \beta^-(\bar \phi)$: the idea behind this fact is that if we increase the length of a spiral of $\delta L$ about the angle $\bar \phi$, then the time function $u$ increases of $\delta L$ about the angle $\bar \phi + 2\pi + \beta^-(\bar \phi)$, and then we can build an admissible barrier of length $\hat \sigma \delta L > \delta L$, in particular a barrier which is closer that the original one.
%
%The idea to overcome this issue is to change the barrier speed $\hat \sigma \to \bar \sigma$ after the point $\bar s$: in other words, after the point $\bar s$ we construct the barrier as in the previous paragraph (i.e. the optimal closing barrier of Theorem \ref{Cor:curve_cal_R_sat_spiral} prolonged as a saturated spiral) with the critical speed $\bar \sigma$. Roughly speaking, after the time $u(\zeta(\bar s))$, the firefighters are allowed to build the barrier at a faster rate. Hence, even if these generalized spirals are not optimal for the speed $\bar \sigma$, they still form a diverging family. \\
%The new admissibility (functional which makes them admissible) is given by
%\begin{equation}
%\label{eq:new:Adm:funct}
%    \mathcal A_{\bar \sigma,\hat \sigma}(\zeta_{\bar s}(s)) = u(\zeta_{\bar s}(s)) - \frac{1}{\hat \sigma} \min\{\bar s,s\} - \frac{1}{\bar \sigma} [s - \bar s]^+ \geq 0,
%\end{equation}
%i.e. the length of the spiral is weighted by $\frac{1}{\hat \sigma}$ up to the point $\zeta(\bar s)$, then the by the smaller coefficient $\frac{1}{\bar \sigma}$ later on. This is the analytic expression of the fact that we allow a faster construction of the barrier after the base point $\zeta(\bar s)$.
%
%The exponential growth will be thus the one of the critical speed, given by Theorem \ref{thm:case:a}: indeed, Theorem \ref{thm:adm:diverg:family} yields the inequality
%\begin{equation*}
%    r(\phi) \geq r_0(\phi), \quad \forall \phi \geq 0,
%\end{equation*}
%in other words $r_0$ is the best strategy a firefighter can follow: construct a sub-optimal barrier with a faster speed. %it can decide to put some barrier on a level set, continue as a segment tangent to the level set and then it can construct a saturated spiral for the maximum speed available: the critical speed. This strategy is clearly not admissible, and this is the reason for considering \emph{generalized} barriers.
%
%The sub-optimality of $r_0$ is compensated if the speed difference is sufficiently large: this is the reason of the choice $\hat \sigma = 2.3$.
%%The idea here is that at any point $\zeta(s)=(r(\bar\phi),\bar\phi)$ of the spiral the strategy that confines better the fire is the union of a subset of the level set $u^{-1}(\zeta(s))$, a segment tangent to it and a saturated spiral for the critical speed $\bar\sigma=2.6144..$. In some sense it corresponds to slowing down the fire at the speed $\frac{\hat\sigma}{\bar\sigma}$ and then having at our disposal the construction speed $\hat \sigma\left(\frac{\bar\sigma}{\hat\sigma}\right)=\bar\sigma$. We will prove that this new family is diverging, and its explicit construction will give the proof of Theorem \ref{thm:main:2}. The heuristic motivations behind this choice of the family is not satisfactory: it is not clear while this method stops working with higher values of the speed $\hat\sigma$. Moreover, e
%Even if we strongly believe that variations of this procedure can be explored in order to increase the value of $\hat\sigma$ ($\sim 2.4-2.5$), the critical case seems to us very difficult to solve with such techniques. If we interpret our construction as the assignment of the control parameter $\beta_s(\phi)$ for each element of the generalized family $r_s$, the critical case requires a more careful choice of $\beta_s$, and probably an almost optimal choice, since every small perturbation can lead to a non diverging spiral due to the critical choice of the speed.
%
%The proof is organized as follows. In the first subsection we show that the first element $r_0$ of the family is always strictly positive and exponentially growing (Section \ref{Ss:r_0}). Then, we construct a generic element of the family $\mathcal F_Z$. As in the proof of Theorem \ref{thm:case:a}, we will consider separately the elements $r_s$ of the family made by an arc (a subset of the level set of the minimum time function $u$), a segment whose endpoint is saturated and a saturated spiral for the critical speed $\bar\sigma$ (\textbf{arc case}, Section \ref{S:arc}), and the elements $r_s$ made by a segment plus a saturated spiral (\textbf{segment case}, Section \ref{S:segment}). 
%
%The idea of the proof is very similar to the proof of Theorem \ref{thm:case:a}, when we optimize w.r.t. the parameter $a$. The derivative $\bar r_s(\phi)$ will satisfy the saturated Delay DE for angles $\phi \geq \bar \phi + 4\pi$ (the exact angle depends on the situation), so that one has to show that the initial data for this RDE verifies the condition of Lemma \ref{lem:key}: the proof of this fact is made by numerical evaluation of trascendental functions (all the plots are available in the Appendix \ref{S:appendix: fire}, done using Mathematica).% We use the software Mathematica to simply verify that all the quantities we are interested in are positive.
%
%}
%\end{comment}
%
%}


==> optimal_family__edited_.tex <==

\section{The optimal solution}
\label{S:optimal_solut}



In this section we construct the optimal candidate spiral for the minimization problem \eqref{Equa:minimum_rphi_intro}, \eqref{eq:min:probl_pert}. The previous section showed that the fastest saturated spiral $\tilde \zeta(\phi;s_0)$ is optimal outside a small interval of rotation angle in the first round after $\phi_0$ (for $\theta \in [0,\frac{\pi}{2}]$): we thus construct a new family of spirals $\check r$ whose structure takes into account that for some angles $\phi$ it is better not to follow the fastest saturated spiral $\tilde r$.


\subsection{Definition and construction of the optimal solution candidate}
\label{Ss:optimal_sol_def}


To describe the possible situations which can occur, depending on the relative position of $\phi_0, \bar \phi$ and the quantities \gls{thetatildeseg}, \gls{Deltaphi} {\color{red}(recall the definitions of the two quantities from Section \ref{S:family})}, we define the quantity \newglossaryentry{omegaopt}{name=\ensuremath{\omega},description={rotation angle for the unsaturated part of the fastest saturated spiral $\tilde r$}}
\begin{equation}
\label{Eq:def:omega:bar:theta}
\gls{omegaopt} = \begin{cases}
\bar \theta & \text{segment case}, \\
\frac{\pi}{2} + \Delta \phi & \text{arc case},
\end{cases} \qquad \text{so that} \ \bar \theta = \min \bigg\{ \omega, \frac{\pi}{2} \bigg\},
\end{equation}
and consider the following cases:
\begin{description}
\item[$\bar \phi -\phi_0 \in [0,2\pi +\beta^-(\phi_0))$] in this case we define
$$
\hat r(\phi;s_0) = \tilde r(\phi;s_0), \quad \phi \in [\phi_0,\bar \phi],
$$
i.e. we follow the fastest saturated spiral, which we already know it is the optimal solution for the first round by Theorem \ref{Cor:curve_cal_R_sat_spiral}.
{\color{red}Va messo come Point (2) perche' nello step successivo si fa riferimento a Point (2). }
\item[$\bar \phi - \phi_0 - 2\pi \in [\beta^-(\phi_0),\bar \theta)$] the solution $\hat r(\phi;s_0)$ will be a segment $[\check P_0,\check P^-]$ in the direction $\bar \phi - 2\pi$. We stop at a length $\ell_0 = |\check P^- - \check P_0|$ such that the fastest saturated spiral starting at the end point $\check P^-$ forms an initial angle whose value is on the boundary of the negativity region (it may happen that $\ell_0 = 0$). From this point onward, the solution is the fastest saturated spiral, which can start either with a segment or with a level set arc.

%    in the segment case, we follow the segment of direction $\bar \phi - 2\pi$ for a length $\ell_0$: this length is determined by the last point for which $\tilde r$ with perturbation in the direction $\bar \phi - 2\pi$ is in the negative region. Then we consider the almost optimal spiral $\tilde r$. 

\item[$\bar \phi - \phi_0 - 2\pi \in [\frac{\pi}{2},\omega)$] here we are in the arc case, and we follow the fastest saturated solution $\tilde r(\phi;s_0)$ in the interval
\begin{equation*}
\phi \in \bigg[ \phi_0,\bar \phi - 2\pi - \frac{\pi}{2} \bigg),
\end{equation*}
then we repeat the construction of the previous point: follow the direction $\bar \phi - 2\pi$ until we remain in the negativity region. Also in this case, after reaching the boundary of the negativity region, we close the last round starting either with a segment or with a level set arc.
%    we follow a segment of length $\ell_0$ in the direction $\bar \phi - 2\pi$ and then the fastest saturated solution $\tilde r$.

\item[$\bar \phi - \phi_0 - 2\pi - \omega \geq 0$] we follow the fastest saturated solution $\tilde \zeta$ up to the angle $\bar \phi - 2\pi - \bar \alpha$, then we repeat Point (2) above starting from a saturated point $\bar \phi - 2\pi - \bar \alpha$. Note that when $\bar \phi = \phi_0 + \omega + 2\pi$, then
\begin{equation*}
P_2 = \tilde \zeta \bigg( \phi_0 + \Delta \phi + \frac{\pi}{2} - \bar \alpha \bigg), \quad P_1 = \tilde \zeta(\phi_0 + \Delta \phi),
\end{equation*}
and then $\bar \phi - 2\pi \in \partial^- \tilde \zeta(\phi_1) \cap \partial^- \tilde \zeta(\phi_2)$, so that the two constructions above are the same. Here, we have indicated by $\phi_1=\phi_0+\Delta\phi$ and by $\phi_2=\phi_0+\Delta\phi+\frac{\pi}{2}-\bar\alpha$ as in Section \ref{S:arc}.
\end{description}

We can summarize the construction as follows, Fig. \ref{Fig:checkr_notation}: we follow the fastest saturated solution $\tilde r$ up to the angle $\check \phi_0$ such that
\begin{equation}
\label{Equa:barphi_checkphi_rel}
\bar \phi \in \check \phi_0 + 2\pi + [\beta^-(\check \phi_0),\beta^+(\check \phi_0)],
\end{equation}
then a segment of length $\ell_0 = |\check P^- - \check P_0|$ determined by requiring that it is the last point such that the derivative of the fastest saturated spiral $\tilde r'$ starting from that point satisfies $\delta \tilde r' \leq 0$, and then the fastest saturated solution for the last round.

\begin{figure}
\resizebox{.75\textwidth}{!}{\input{checkr_notation_2.pdf_t}}
\caption{The construction of the optimal closing solution: the starting spiral is $\zeta$ (black) up to the angle $\phi_0$. Then we follow the fastest saturated spiral $\tilde \zeta$ (blue) up to the angle $\check \phi_0$, determined by \eqref{Equa:barphi_checkphi_rel}. At this point we follow the segment with direction $\bar \phi$ until the angle between $\bar \phi$ and the new fastest saturated spiral $\check \zeta$ (red) is on the boundary of the negativity region. Note that while the blue spiral is inside the red one, the ray $\check r(\bar \phi;s_0)$ is smaller than $\tilde r(\bar \phi;s_0)$.}
\label{Fig:checkr_notation}
\end{figure}

Apriori, the perturbation of $\tilde r$ in the last case (i.e. on the saturated part of $\tilde r$) can be either a segment of an arc, i.e. we are exiting the negativity region in the arc or segment case. This may only happen in the first round, because afterwards the last round corresponds to the segment case (Proposition \ref{Prop:tent_admissible}): due to the particular form of the solution in this case (two consecutive segments followed by a saturated spiral), we will call this construction a \emph{tent}. In particular, Fig. \ref{Fig:checkr_notation} is correct when $\check P_1 = \check P^-$, but its purpose was just for notation.

We next fix the notation for the optimal candidate solution, see Fig. \ref{Fig:checkr_notation}.
\begin{itemize}
\item \gls{phibar} is the final angle, where we want to minimize $r(\bar \phi)$;
\item \gls{phi0} is the starting angle, with $\phi_0 \leq \bar\phi$, from which the arc/segment of the fastest saturated spiral \gls{rtildefam} starts;
\item the point \newglossaryentry{P0check}{name=\ensuremath{\check P_0},description={initial point of the segment of length $\ell_0$ in the direction $\bar \phi$}} \gls{P0check} is the point of the spiral $\tilde r(\phi;s_0)$ where a segment of length $\ell_0$ starts with direction $\bar \phi$; the corresponding angle is \newglossaryentry{phi0check}{name=\ensuremath{\check \phi_0},description={angle of the point $\check P_0$}} \gls{phi0check};
\item the segment of length \newglossaryentry{ell0}{name=\ensuremath{\ell_0},description={length of the segment $[\check P_0,P^-]$ of direction $\bar \phi$}} \gls{ell0} has endpoints \newglossaryentry{P-check}{name=\ensuremath{\check P^-},description={final point of the segment of length $\ell_0$ and direction $\bar \phi$}} $\check P_0,\gls{P-check}$, and its direction belongs to the subdifferential to the fastest saturated spiral $\tilde r(\phi;s_0),\phi)$ in the point $\check P_0$;
\item in the point $\check P^{-}$ we compute the fastest saturated spiral%, which we call \newglossaryentry{rcheck}{name=\ensuremath{\check r(\phi;s0)},description={last round of the oprimal spiral}} \gls{rcheck}
: two cases again can occur (arc and segment, see however Proposition \ref{Prop:tent_admissible});
\item if the segment case occurs in the point $\check P^{-}$ we will denote it by \newglossaryentry{P1check}{name=\ensuremath{\check P_1},description={initial point of the last segment of the fastest saturated spiral}} $\gls{P1check} = \check P^{-}$;
\item if the arc case occurs in the point $\check P^{-}$ we will denote by \gls{P1check} the second endpoint of the arc of the level set of $u$, with opening \newglossaryentry{Deltaphicheck}{name=\ensuremath{\Delta \check \phi},description={angle of the level set for the last round of the optimal solution $\check r(\bar \phi;s_0)$}} \gls{Deltaphicheck};
\item from the point $\check P_1$ the spiral is a segment of length \newglossaryentry{ell1}{name=\ensuremath{\ell_1},description={length of the last segment $[\check P_1,\check P_2]$ of the fastest saturated spiral}} \gls{ell1} and endpoints \newglossaryentry{P2check}{name=\ensuremath{\check P_2},description={final point of the last segment $[\check P_1,\check P_2]$ in the fastest saturated spiral}} $\check P_1,\gls{P2check}$;
\item the point $\check P_2$ is saturated;
\item the exterior angle between the segments $[\check P_0,\check P_1]$ and $[\check P_1,\check P_2]$ is the critical angle \gls{thetahat} in the segment case, while in the arc case the angle between $[\check P_0,\check P^-]$ and the level set arc is $\gls{h1Deltaphi} \leq \hat \theta$.
\end{itemize}

\begin{figure}
\centering
\includegraphics[scale=0.6]{tentspirals.png}
\caption{The three possible situations occurring in the construction of an element of the family, in the segment case ($\omega<\frac{\pi}{2}$). The blue curve represents the strategy $\tilde r(\phi,s_0)$ constructed in the previous section. In red the angle $\hat\theta$. {\color{blue} NON SO SE QUESTA FIGURA E' NECESSARIA}{\color{red} non perche' l'ho fatta io, ma secondo me e' piu' chiara perche' riassume punto 1,2,3. Io la terrei. Meglio una figura in piu' che una in meno}}
\label{fig:tent:solution}
\end{figure}

The first result of this section is that the above {\color{red}construction} defines a unique spiral \newglossaryentry{rcheckphis0}{name=\ensuremath{\check r(\phi;s_0)},description={optimal spiral at the angle $\bar \phi$}} \gls{rcheckphis0}.

\begin{proposition}
\label{Prop:unique_optimal_guess}
Given $s_0 = s(\phi_0) \geq 0$ and an angle $\bar \phi \geq \phi_0$, there exists a unique spiral $\check r(\phi;s_0)$ with the properties above.
\end{proposition}

We observe here that the Dirac delta part at $\tau = 1$ of $\delta \tilde r$ can be neglected having $0$ contribution to the integral {\color{red} la $\delta\tilde r$ e' calcolata in $\phi$ invece che in $\tau$, quindi secondo me scritto cosi', senza riferimenti, questo commento e' oscuro}
\begin{equation*}
\int \delta \tilde r(\bar \phi;s_0) ds_0.
\end{equation*}

\begin{proof}
The spiral $\check r(\phi;s_0)$ is defined once we know at what length $\ell_0$ of the segment starting in $\check P_0$ and pointing in the direction $\bar \phi$ has to stop, and the spiral becomes the fastest saturated afterward. This point is when the derivative $\delta \tilde r(\phi;\ell_0)$ of the fastest saturated spiral $\tilde r(\phi;\ell_0)$ starting from $\check P^-$, $|\check P^- - \check P_0| = \ell_0$, is $0$. Recall the definition of $\omega,\bar\theta$ in \eqref{Eq:def:omega:bar:theta}.

\begin{figure}
\resizebox{.75\textwidth}{!}{\input{nu_funct.pdf_t}}
\caption{The curves $\nu(\ell_0)$ of Proposition \ref{Prop:unique_optimal_guess} in blue, and the boundary of the negativity region in red.}
\label{Fig:nu_funct}
\end{figure}

If we define $\omega(\ell_0), \theta(\ell_0)$ as the values of the angles $\omega$, $\theta$ formed by the fastest saturated spiral along the segment $\ell_0 e^{\i \bar \phi}$ (recall that \gls{thetapertsegm} is the angle $\gls{thetatildeseg} -\theta_0$, where $\theta_0 = \beta^-(\check P_0)$ is the direction of the perturbation), we have defined a curve \newglossaryentry{nuell0}{name=\ensuremath{\nu(\ell_0)},description={curve representinvg the variation of the angles for the fastest saturated spiral w.r.t. the length $\ell_0$ of the segment $[\check P_0.\check P^-]$}}
\begin{equation*}
\R^+ \ni \ell_0 \mapsto \gls{nuell0} = (\theta(\ell_0),\omega(\ell_0)) \in \R^2.
\end{equation*}
The statement is proved if we show that this curve crosses the boundary of the negativity region $N = N_\mathrm{segm} \cup N_\mathrm{arc}$ (Propositions \ref{Prop:neg_region} and \ref{Prop:regions_pos_neg_segm}) only in one point: if this happens, the crossing point is a minimum for the quantity $\tilde r(\bar \phi;\ell_0)$, see Fig. \ref{Fig:nu_funct}. In the case the initial value is already outside the negativity region (i.e. $\theta > h_1(\Delta \phi)$), then we deduce that $\ell_0 = 0$. We observe that after the point $P_0$, the segment $[\check P_0,\check P^-]$ starts tangent to the spiral $\tilde \zeta$, i.e. $\theta = 0$ at the beginning $P_0$: thus we always start in the negativity region of $\delta \tilde r(\bar \phi)$ (i.e. $\ell_0 > 0$) apart from the case where $\check P_0 = P_0$. {\color{red}Cosa vuol dire questa frase? Non e' chiara}

%{\color{red} mi è venuto un dubbio: se per caso in $\bar\phi-2\pi$ sono nella regione di positività, allora $\ell_0=0$? Se sì forse vale la pena scriverlo. } {\color{blue} Si}

We can compute the derivative of the curve $\nu(\ell_0)$ by using the formulas of the previous section.

\begin{description}
\item[Segment case] we have form {\color{red}from} \eqref{Equa:delta_theta_segm_1}
\begin{equation*}
\frac{d\bar \theta}{d\ell_0} = \frac{1}{|\check P_2 - \check P_1|} \big( \sin(\theta) - \cot(\bar \alpha) \big( 1 - \cos(\theta)) \big) - \frac{\sin(\check \theta_1)}{\check r(\check \phi_1)},
\end{equation*}
\begin{equation*}
\frac{d\theta}{d\ell_0} = \frac{1}{|\check P_2 - \check P_1|} \big( \sin(\theta) - \cot(\bar \alpha) \big( 1 - \cos(\theta) \big),
\end{equation*}
where we have used Equation \eqref{Equa:delta_theta_segm_1} and where $\check r(\check \phi_1)$ is the length of the segment part of the optimal ray ending in the initial point $\check P_1$ and $\check \theta_1 = \beta^+(\check \phi_1) - \check \phi_1$. {\color{red}non ho capito che angolo e' $\check\theta_1$. Altra questione: questa derivata e' calcolata nel punto $\hat P_1$? Se si'  forse vale la pena scriverlo? Non so mi e' un po' oscuro}

 Hence, since $\frac{d\theta}{d\ell_0} > 0$ unless $\theta = 0$, the curve $\nu(\ell_0)$ {\color{red} which in the segment case is $(\theta(\ell_0),\bar\theta(\ell_0))$} can be represented as the graph of a differentiable function $\bar \theta(\theta)$, parameterized with $\theta$ increasing. Since in the segment case the boundary of the negativity region is $\theta = \hat \theta$, this curve exits the negativity region only in one point, corresponding to a unique value $\ell_0$.
 {\color{red}Altra domanda: il punto $\check P_1$ non puo' essere saturato? Il mio dubbio e' se l'espressione sopra con $\check P_2=\check P_1$ come si possa definire quella derivata? }

%{\color{red} scusa qui non mi trovo, ok la formula $\frac{d\theta}{d\ell_0}$ pero` non capisco la $\frac{d\theta_0}{d\ell_0}$... non dovrebbe essere $\delta\phi_0=-\delta\theta_0$?} {\color{blue} fissiamo l'angolo iniziale $\bar \theta_0$:  $\bar \theta$ e' l'angolo del segmento con la direzione $\theta_0$. Siccome nella nostra derivavazione noi calcoliamo la variatione $\delta \bar \theta$ di $\bar \theta$ rispetto alla direzione $\bar \theta_0$, allora il nuovo $\bar \theta$ e' $\bar \theta + \delta \bar \theta - \delta \theta_0$.}
% \medskip
% 
% {\color{red} il fatto e` che quella che scrivi tu e` vera se $\bar\theta=\frac{\pi}{2}$, in cui appunto verrebbe $\sin\theta_0$, ma cosi` onestamente non capisco.}
%
% \medskip
% {\color{red} altra domanda: perche` non basta dire che $\ell_0\rightarrow\theta({\ell_0})$ e` crescente?} {\color{blue} basta si, volevo mostrare che sappiamo calcolarlo in maniera bizantina}

\item[Arc case] here using \eqref{Equa:delta_Delta_phi} and the fact that the angle of the level set with the ray is $\frac{\pi}{2}$ to write
\begin{equation*}
\frac{d\omega}{d\ell_0} = \frac{d\Delta \check \phi}{d\ell_0} = \frac{1}{|P_2 - P_1|} \big( \sin(\theta) - \cot(\bar \alpha) (1 - \cot(\theta)) + {\color{red}\cot\bar\alpha}\sin(\theta) \Delta \check \phi \big) - \frac{\cos(\theta)}{\check r(\check \phi^-)},
\end{equation*}
{\color{red} ok ma ci ho messo un'ora per capire sto conto... forse vale la pena scrivere qualcosa in piu' o e' che sono troppo arrugginita?}
\begin{equation*}
\frac{d\theta}{d\ell_0} = \frac{\cos(\theta)}{\check r(\check \phi^-)},
\end{equation*}
with $\check r(\check \phi^-)$ the segment part of the optimal ray ending in $\check P^-$. Hence the curve can be represented again as the graph of a function $\Delta \check \phi(\theta)$, oriented along the increasing $\theta$ axis, and such that
\begin{equation*}
\frac{d\Delta \check \phi}{d\theta} = \frac{\check r(\check \phi^-)}{|P_2 - P_1|} \frac{\sin(\theta) - \cot(\bar \alpha) (1 - \cot(\theta) + \sin(\theta) \Delta \phi)}{\cos(\theta)} - 1.
\end{equation*}
The computation of Lemma \ref{Lem:study_g_1_arc} gives that the derivative of the boundary curve $h_1(\Delta \check \phi)$ is (see Equation \eqref{Equa:dh1_dDeltaphi})
\begin{equation*}
\frac{d\Delta \check \phi}{d\theta} = \bigg( \frac{dh_1}{d\Delta \check \phi} \bigg)^{-1} = - 1 - \frac{\cos(\theta) \Delta \check \phi}{\sin(\theta) - \cot(\bar \alpha) (1 - \cos(\theta) + \sin(\theta) \Delta \check \phi)},
\end{equation*}
Hence it follows that the curves are not transversal only if
\begin{equation*}
\frac{\check r(\check \phi^-)}{|P_2 - P_1|} = - \frac{\cos(\theta)^2 \Delta \check \phi}{(\sin(\theta) - \cot(\bar \alpha) (1 - \cot(\theta) + \sin(\theta) \Delta \check \phi))^2} \leq 0,
\end{equation*}
which is impossible, because the l.h.s. is strictly positive. {\color{red}Assolutamente non chiaro}
\end{description}
Thus the curves are transversal, and the crossing occurs from the negative to the positive: indeed this is clear in the segment case, while in the arc case
$$
\text{if} \quad \sin(\theta) - \cot(\bar \alpha)(1 - \cos(\theta) + \sin(\theta) \Delta \check \phi) < 0 \quad \text{then} \quad \frac{d\Delta \check \phi}{d\theta} < - 1 < \bigg( \frac{dh_1}{d\Delta \check \phi} \bigg)^{-1},
$$
$$
\text{if} \quad \sin(\theta) - \cot(\bar \alpha)(1 - \cos(\theta) + \sin(\theta) \Delta \check \phi) > 0 \quad \text{then} \quad \frac{d\Delta \check \phi}{d\theta} > -1 > \bigg( \frac{dh_1}{d\Delta \check \phi} \bigg)^{-1}. 
$$
The above inequalities yield the statement.
\end{proof}

\begin{figure}
\resizebox{.75\textwidth}{!}{\includegraphics{cross_segm_arc.png}}
\caption{Plot of the function of Remark \ref{Rem:trans_segm_arc}.}
\label{Fig:cross_segm_arc}
\end{figure}

\begin{remark}
\label{Rem:trans_segm_arc}
Observe that along the line $\Delta \check \phi = 0$, i.e. $\bar \theta = \frac{\pi}{2}$ and $\check \theta_1 = \frac{\pi}{2} - \theta$, we have
\begin{equation*}
\frac{d\omega}{d\theta} = \frac{d\bar \theta}{d\theta} = 1 - \frac{\ell_0}{\check r(\check \phi_1)} \frac{\sin(\bar \alpha) \sin(\theta)}{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)}.
\end{equation*}
{\color{red}Ecco qua non si capisce. Penso che tu voglia fare separatamente il caso in cui $\hat P_0$ sia saturato, cosi' risponderesti alla mia domanda di prima, pero' va messo negli statement. E comunque non e' chiaro }
By observing that the spirals are convex and the angle at the top of the segment $\ell_0$ with the optimal ray is $\bar \alpha$, by elementary geometrical reasons we must have {\color{red}So elementary che sto qui da mezzora e ancora non ho capito come l'hai ottenuta}
\begin{equation*}
\ell_0 \leq \check r(\check \phi_1) \cot(\bar \alpha),
\end{equation*}
so that we obtain (see Fig. \ref{Fig:cross_segm_arc})
\begin{equation*}
\frac{d\omega}{d\theta} > 1 - \frac{\cos(\bar \alpha) \sin(\theta)}{\cos(\bar \alpha - \theta) - \cos(\bar \alpha)} \geq 1 - \frac{\cos(\bar \alpha)}{\sin(\bar \alpha) - \cos(\bar \alpha)} > 0.293599 > 0.
\end{equation*}
Hence, when increasing the length $\ell_0$, we always pass from the segment case to the arc case.
\end{remark}

The previous proposition proves that construction of the spiral $\check r(\phi;s_0)$ at the beginning of the section is well defined. To prove that it is the minimizer for the minimization problem \eqref{eq:min:probl_pert}, we need to study the positivity of $\check r(\bar \phi;s_0)$ w.r.t. to perturbations. More precisely, we want to compute the derivative \newglossaryentry{deltarcheck}{name=\ensuremath{\delta \check r(\phi;s_0)},description={derivative of the candidate optimal slosing spiral w.r.t. the starting position $s_0$}}
\begin{equation}
\label{Equa:deltacheckr_def}
\gls{deltarcheck} = \frac{d}{ds_0} \check r(\phi;s_0).
\end{equation}
Similarly to the computation of $\delta \tilde r(\phi;s_0)$, depending on the structure of the solution $\check r$ several cases are possible: the initial fastest saturated part of $\check r(\phi;s_0)$ can be a segment or a level-set arc, and the segment starting in $\check P_0$ with length $\ell_0$ may be followed by a segment (tent case) or an arc.

The most important case is when the last round starts with segment (tent case), which we analyze in the next section.

%{\color{red} DA RIVEDERE
%
%
%We list the cases to be studied in the two following grids.
%
%\medskip
%First, we consider the case where at $\phi_0$ the solution $\tilde r(\phi;s_0)$ starts with a segment (Subsection \ref{S:segment}).
%
%\medskip
%
%\textbf{ The fastest saturated spiral $\tilde r(\phi;s_0)$ starts with a segment in $\phi_0$ (Segment Case), that is $\omega=\bar\theta$.}
%
%\begin{center}
%\begin{tabular}{ | m{4cm} | m{3.5cm}| m{3.5cm} | m{3.1cm}|} 
%\hline
%&$\bar \phi -\phi_0 \in [0,2\pi +\beta^-(\phi_0))$&$\bar \phi - \phi_0 - 2\pi \in [\beta^-(\phi_0),\bar \theta)$&$\bar \phi - \phi_0 - 2\pi - \omega \geq 0$\\
%  \hline
%  Tent& Content of Section \ref{S:exist_opti_traj} & Section \ref{Ss:init_segment}&Section \ref{Ss:init_segment}\\ 
%  \hline
%  Segment of length $\ell_0$+Arc & Content of Section \ref{S:exist_opti_traj} & Proposition \ref{Prop:tent_worst} &Proposition \ref{Prop:tent_worst}\\ 
%  \hline
%  
%\end{tabular}
%\end{center}
%
%We point out that the case $\bar\phi-\phi_0\in[0,2\pi+\beta^-(\phi_0))$ is the one considered in Section \ref{S:exist_opti_traj}, where the positivity is already proved. Moreover, the case where the closure is given by a segment of length $\ell_0$ and an arc can be reduced to the study of the case of the tent (two segments of lengths $\ell_0, \ell_1$ respectively) via Proposition \ref{Prop:tent_worst}, which we will prove in this subsection.
%\medskip
%
%Secondly, we consider the case where at $\phi_0$ the solution $\tilde r(\phi;s_0)$ starts with an arc (Subsection \ref{S:arc}).
%
%\medskip 
%
%\textbf{ The fastest saturated spiral $\tilde r(\phi;s_0)$ starts with an arc in $\phi_0$, that is $\omega=\frac{\pi}{2}+\Delta\phi$.}
%
%\begin{center}
%\begin{tabular}{ | m{2.5cm}| m{3.3 cm} | m{3.4cm}| m{2.9cm} | m{2.5cm}|} 
%\hline
%&$\bar \phi -\phi_0 \in [0,2\pi +\beta^-(\phi_0))$&$\bar\phi-\phi_0-2\pi\in[\beta^{-}(\phi_0),\frac{\pi}{2})$&$\bar \phi - \phi_0 - 2\pi \in [\frac{\pi}{2},\omega)$&$\bar \phi - \phi_0 - 2\pi - \omega \geq 0$\\
%  \hline
%  Tent & Content of Section \ref{S:exist_opti_traj}  & Subsection \ref{Ss:init_segment}& Subsection \ref{Ss:arc_to_segment} &\\ 
%  \hline
%  Segment $P_0P_1$+Arc & Content of Section \ref{S:exist_opti_traj} & Proposition \ref{Prop:tent_worst} &Proposition \ref{Prop:tent_worst}&Proposition \ref{Prop:tent_worst}\\ 
%  \hline
%  
%\end{tabular}
%\end{center}
%
%Again, the case $\bar\phi-\phi_0\in[0,2\pi+\beta^-(\phi_0))$ is the one considered in Section \ref{S:exist_opti_traj}, where the positivity is already proved. Moreover, the case where the closure is given by a segment of length $\ell_0$ and an arc can be reduced also in this case to the study of the tent (two segments of lengths $\ell_0$,$\ell_1$ respectively) via Proposition \ref{Prop:tent_worst}.
%}


\subsection{Formulas for the tent case}
\label{Ss:comput_tent_new}


\begin{figure}
\resizebox{.5\textwidth}{!}{\input{tent_compu.pdf_t}}
\caption{The geometry used to obtain the formulas for the tent case, Section \ref{Ss:comput_tent_new}.}
\label{Fig:tent_comput_geo}
\end{figure}

In order to study the correction to the fastest saturated spiral $\tilde r$ after the angle $\check \phi_0$, we need to study some geometric relations among the length $\ell_0$ of this segment and the underlying spiral $\tilde r$. This section is thus devoted to obtain these formulas, depending on the following quantities, which in order to distinguish from the previous ones are denoted with a hat, see Fig. \ref{Fig:tent_comput_geo}:
\begin{itemize}
\item the entrance ray \newglossaryentry{rhat0}{name=\ensuremath{\hat r_0},description={entry ray for the formulas for tent or arc perturbation}} \gls{rhat0} at angle $0$ initial position \newglossaryentry{Qhat0tent}{name=\ensuremath{\hat Q_0},description={base point for $\hat r_0$ in the tent or arc perturbation}} \gls{Qhat0tent}, the end point \newglossaryentry{Phat0}{name=\ensuremath{\hat P_0},description={initial point of the tent or arc perturbation}} \gls{Phat0} of $\hat r_0$ is saturated;
\item the exit ray \newglossaryentry{rhat2}{name=\ensuremath{\hat r_2},description={exit ray for the tent or arc computations}} \gls{rhat2} at angle $\hat \theta$ with initial position \newglossaryentry{Qhat2tent}{name=\ensuremath{\hat Q_2},description={base point for $\hat r_2$ in the tent or arc perturbation}} \gls{Qhat2tent}, the end point of $\hat r_2$ is saturated;
\item the length of segments \newglossaryentry{ellhat0}{name=\ensuremath{\hat \ell_0},description={length of the first segment in the tent or arc computations}} \newglossaryentry{ellhat1}{name=\ensuremath{\hat \ell_1},description={length of the second segment in the tent or arc computations}} \gls{ellhat0}, \gls{ellhat1};
\item the length \newglossaryentry{Lhattent}{name=\ensuremath{\hat L},description={length of the spiral between $Q_0,\hat Q_2$ in the tent or arc computations}} \gls{Lhattent} of the spiral at the base between the points $\hat Q_0, \hat Q_2$ (angle opening $[0,\hat \theta]$).
\end{itemize}
We will also give conditions to verify that it is admissible, which is equivalent to check that the angle formed by segment \newglossaryentry{Qhat1tent}{name=\ensuremath{\hat Q_1},description={point of the curve $\zeta$ where the optimal ray ending in the tip $\hat P_1$ of the ten or arc is detaching}} \newglossaryentry{Phat1tent}{name=\ensuremath{\hat P_1},description={tip of the tent or arc}} $[\gls{Qhat1tent},\gls{Phat1tent}]$ and \newglossaryentry{Phat2tent}{name=\ensuremath{\hat P_2},description={saturated final point of the tent or arc}} the second segment $[\gls{Phat1tent},\gls{Phat2tent}]$ is $\leq \frac{\pi}{2}$. %The input quantities are $\hat r_0$, $\hat Q_2 - \hat Q_0$, $\hat L$. 
{\color{red} Io scriverei che $\angle \hat Q_1\hat P_1\hat P_2\geq\frac{\pi}{2}$}

Since $\hat P_0$ is saturated, the saturation condition at the end point of the segment $\ell_1$ reads as
\begin{equation}
\label{Equa:saturation_tent}
\hat r_2 + \hat L - \hat r_0 - \cos(\bar \alpha) (\hat \ell_0 + \hat \ell_1) = 0,
\end{equation}
and the vector relation among the various points is
\begin{equation}
\label{Equa:vector_Q_1_Q_2}
\hat Q_0 + \hat r_0 (1,0) + \hat \ell_0 e^{\i \bar \alpha} + \hat \ell_1 e^{\i (\bar \alpha + \hat \theta)} = \hat Q_2 + \hat r_2 e^{\i \hat \theta}.
\end{equation}

Projecting the second equation in the direction $e^{\i \hat \theta}$ we obtain
\begin{equation*}
(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} + \hat r_2 - \hat \ell_1 \cos(\bar \alpha) - \hat \ell_0 \cos(\bar \alpha - \hat \theta) - \hat r_0 \cos(\hat \theta) = 0,
\end{equation*}
and then using the saturation condition
\begin{equation*}
(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - \hat \ell_0 \cos(\bar \alpha - \hat \theta) - \hat r_0 \cos(\hat \theta) = \hat L - \hat r_0 - \cos(\bar \alpha) \hat \ell_0,
\end{equation*}
\begin{equation*}
\begin{split}
\hat \ell_0 &= \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - {\color{red}\hat L} + \hat r_0 (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}. %\\
%&= 2.50013((\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - L) + 0.313453 \hat r_0.
\end{split}
\end{equation*}
Projecting again \eqref{Equa:vector_Q_1_Q_2} on the direction $e^{\i (\alpha + \hat \theta - \frac{\pi}{2})}$
\begin{equation*}
(\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})} + \hat r_2 \sin(\bar \alpha) - \hat \ell_0 \sin(\hat \theta) - \hat r_0 \sin(\bar \alpha + \hat \theta) = 0,
\end{equation*}
which gives
\begin{equation*}
\hat r_2 = \frac{\hat r_0 \sin(\bar \alpha + \hat \theta) + \hat \ell_0 \sin(\hat \theta) - (\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha)}.
\end{equation*}
%and using \eqref{Equa:ell_0_tent_general}
%\begin{align*}
%\hat r_2 &= \frac{\hat r_0}{\sin(\bar \alpha)} \bigg( \sin(\bar \alpha + \hat \theta) + \frac{\sin(\hat \theta) (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg) - \frac{L}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
%&\quad + \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta}}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha)} \\
%&= \hat r_0 \frac{\cos(\bar \alpha) - \cos(\bar \alpha + \hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - L}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha)}. %\\
%&= 1.23979 \hat r_0 + 1.31181 ((\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - L) - 1.0823 (\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}.
%\end{align*}
We can now compute $\hat \ell_1$ from \eqref{Equa:saturation_tent} as
\begin{equation*}
\hat \ell_1 = \frac{\hat r_2 + {\color{red}\hat L}  -\hat r_0 - \cos(\bar \alpha) \hat \ell_0}{\cos(\bar \alpha)}.
\end{equation*}
%and using \eqref{Equa:vector_Q_1_Q_2}, \eqref{Equa:r_2_tent_general}
%\begin{align*}
%\hat \ell_1 &= \frac{\hat r_0}{\cos(\bar \alpha)} \bigg[ \frac{1}{\sin(\bar \alpha)} \bigg( \sin(\bar \alpha + \hat \theta) + \frac{\sin(\hat \theta) (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg) - 1 - \cos(\bar \alpha) \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] \\
%&\quad + \frac{L}{\cos(\bar \alpha)} \bigg[ - \frac{L}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + 1 + \frac{\cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] \\
%&\quad + \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta}}{\cos(\bar \alpha)} \bigg[ \frac{1}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - \frac{\cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] - \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha) \cos(\bar \alpha)} \\
%&= \hat r_0 \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} + \frac{L}{\cos(\bar \alpha)} \\
%&\quad +  \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - L}{\cos(\bar \alpha)} \bigg[ \frac{1}{\sin(\bar \alpha)} \frac{\sin(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} -\frac{\cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \bigg] - \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha) \cos(\bar \alpha)}. %\\
%&= 0.313453 \hat r_0 + 2.61433 L +  0.929517 ((\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - L) - 2.8296 (\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}.
%\end{align*}
Finally, the relation between $\hat L$ and $\hat Q_2 - \hat Q_0$ is given by integrating the curve \newglossaryentry{zetahattent}{name=\ensuremath{\hat \zeta},description={convex curve for computing the formulas for the tent or arc case}} \gls{zetahattent}: 
\begin{equation*}
\frac{d\hat \zeta}{d\theta} = e^{\i \theta} \hat R(\theta), \quad \hat \zeta(\theta) - \hat \zeta(\theta_0) = \int_{\theta_0}^{\theta} e^{\i \omega} \hat R(\omega) d\omega,
\end{equation*}
where \newglossaryentry{Rhatcurvsegm}{name=\ensuremath{\hat R},description={curvature of the convex curve $\hat \zeta$ for the computations of the tent or arc formulas}} \gls{Rhatcurvsegm} is the radius of curvature of $\hat \zeta$. The above formula holds also when the curvature is $\infty$, by considering $ds = \hat R d\theta$ as a measure.

We summarize the results obtained in the following lemma.

\begin{lemma}
\label{Lem:relation_admissibility_tent}
Consider the geometric configuration as in Fig. \ref{Fig:tent_comput_geo}, with $\hat P_0,\hat P_2$ saturated. Then the following geometric relations hold:
\begin{equation}
\label{Equa:DeltahatQ_tent}
\hat Q_2 - \hat Q_0 = \int_0^{\hat \theta} e^{\i \omega} \hat R(\omega) d\omega, \quad \hat R(\theta) \ \text{curvature of } \ \hat \zeta,
\end{equation}
\begin{equation*}
\hat L = \int_0^{\hat \theta} \hat R(\theta) d\theta,
\end{equation*}
\begin{equation}
\label{Equa:ell_0_tent_general}
\hat \ell_0 = \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - {\color{red}\hat L} + \hat r_0 (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation}
\begin{equation}
\label{Equa:r_2_tent_general}
\hat r_2 = \frac{\hat r_0 \sin(\bar \alpha + \hat \theta) + \hat \ell_0 \sin(\hat \theta) - (\hat Q_2 - \hat Q_0) \cdot e^{\i (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{\sin(\bar \alpha)},
\end{equation}
\begin{equation*}
\hat \ell_1 = \frac{\hat r_2 + {\color{red}\hat L} -\hat r_0 - \cos(\bar \alpha) \hat \ell_0}{\cos(\bar \alpha)}.
\end{equation*}
\end{lemma}

Since all formulas are linear, we obtain the following corollary.

\begin{corollary}
\label{Cor:tent_corol_for_pert}
The same formula{\color{red}s} of Lemma \ref{Lem:relation_admissibility_tent} holds {\color{red}hold} for the perturbation $\delta \check r(\phi;s_0)$.
\end{corollary}

For future use, define the angle shift $\hat \theta$ in the $\tau$  ${\color{red}\hat\tau}$ variable: \newglossaryentry{tauhat}{name=\ensuremath{\hat \tau},description={angle shift \gls{thetahat} in the $\tau$ coordinates}}
\begin{equation}
\label{Equa:hattau_def}
\hat \tau = \frac{\hat \theta}{2\pi + \bar \alpha}.
\end{equation}

\subsubsection{Estimates for the admissibility of the tent}
\label{Sss:having_tent_check}


 The next series of lemmas give sufficient conditions which assure {\color{red}ensure} that the construction above is admissible, i.e. the angle between the segments $[\hat Q_1,\hat P_1]$ and $[\hat P_1,\hat P_2]$ is $\leq \frac{\pi}{2}$. If \newglossaryentry{phihat}{name=\ensuremath{\hat \phi},description={angular coordinate correponding to $\hat Q_1 = \hat \zeta(\hat \phi)$ for the tent or arc case}} $\hat Q_1 = \zeta(\gls{phihat})$, then we must require {\color{red}Questa $\zeta$ e' ausiliaria per indicare quel tratto li'. Non e' $\hat\zeta?$..?}
\begin{equation*}
\bar \alpha + \hat \theta - \hat \phi < \frac{\pi}{2}, \quad \hat \phi \geq 0,113642.
\end{equation*}

\begin{lemma}
\label{Lem:when_tent}
Assume that we are in the configuration of Fig. \ref{Fig:tent_comput_geo}: if \newglossaryentry{Kadmis}{name=\ensuremath{K_\mathrm{tent}},description={constant for verifying whether the tent is admissible}}
\begin{equation*}
\frac{\hat L}{\hat r_0} \leq \gls{Kadmis} = \frac{\sin(\bar \alpha) (\sin(\bar \alpha + \hat \theta) - \sin(\bar \alpha))}{\cos(\hat \theta) (1 - \sin(\bar \alpha))} < 0.966795,
\end{equation*}
then the tent is admissible.
\end{lemma}

%Observe that this is exactly the functional $AT(\tau)$ defined in \eqref{Equa:AT_tau}.

\begin{proof}
One sees geometrically that the worst case is when $\hat L = |\hat Q_2 - \hat Q_0|$ and $\hat Q_2 - \hat Q_1 {\color{red}\hat Q_0 } = \hat L e^{\i \hat \phi}$: indeed, from \eqref{Equa:ell_0_tent_general} one sees that by increasing $\hat L$ and keeping $\hat Q_0,\hat Q_1,\hat Q_2$ fixed, then length $\hat \ell_0$ increases {\color{red}decreases}, so that the worst situation is when $\hat \zeta$ is made of 2 segments, namely
\begin{equation*}
\hat \zeta = [\hat Q_0,\hat Q_1] e^{\i \bar \phi} \cup [\hat Q_1,\hat Q_2] e^{\i \hat \theta}.
\end{equation*}
{\color{red}Non e' $\bar\phi$.. a che angolo ti riferisci? }
At this point, the length of the segment $[\hat Q_1,\hat Q_2]$ does not enter into the computation of $\hat \ell_0$, while the first segment $[\hat Q_0,\hat Q_1]$ enters with the factor
\begin{equation*}
(\hat Q_1 - \hat Q_0) \cdot e^{\i \hat \theta} - |\hat Q_1 - \hat Q_0| = (\cos(\hat \theta - \hat \phi) - 1) |\hat Q_1 - \hat Q_0|.
\end{equation*}
Hence the worst case is when $\hat Q_2 = \hat Q_1$ (Fig. \ref{Fig:worst_tent_case}), maximizing the above negative term.

%if $Q$ is the point with the direction of $P_1$ in the subdifferential
%\begin{enumerate}
%    \item by taking the segment $Q - Q_0$ the angle of the optimal ray at $P_1$ increases,
%    \item by taking the largest $L$ after $Q$ the length of $\ell_0$ decreases, so that the angle increases.
%\end{enumerate}
%and the angle is $\phi$ where
%\begin{equation*}
%    \frac{\hat \ell_0}{\sin(\phi)} = \frac{\hat r_0}{\sin(\bar \alpha - \phi)},
%\end{equation*}
%i.e. the ray for the end point of $\hat r_0$ starts in the initial point of $\hat r_0$, and $Q_2$ is on the segment connecting these two points.
%
%This is because for $L$ and $Q_2 - Q_0$ fixed, the angle increases by packing the curve an close to $Q_ - Q_0$ as possible, and then increasing $L$ as much as we can so that $\hat \ell_0$ decreases.

\begin{figure}
\begin{subfigure}{.32\textwidth}
\resizebox{\linewidth}{!}{\input{worst_case_tent.pdf_t}}
\caption{The worst scenario of Lemma \ref{Lem:when_tent}.}
\label{Fig:worst_tent_case}
\end{subfigure}
\hfill
\begin{subfigure}{.32\linewidth}
\includegraphics[width=\linewidth]{admissi_tent_cond1.png}
\caption{Plot of the function (\ref{Equa:Loverr0_tent}) in blue, in orange the value of $\frac{\hat L}{\hat r_0}$ for the critical angle $\hat \phi = \bar \alpha + \hat \theta - \frac{\pi}{2}$.}
\label{Fig:Loverr0_tent}
\end{subfigure}
\hfill
\begin{subfigure}{.32\linewidth}
\resizebox{\linewidth}{!}{\input{worst_case_tent_L.pdf_t}}
\caption{The geometric situation to estimate the tent.}
\label{Fig:worst_case_tent_L}
\end{subfigure}
\caption{Analysis of Lemma \ref{Lem:when_tent}.}
\label{Fig:tent_2_case}
\end{figure}

For this configuration, elementary geometry gives %At this point the relation ($\hat \phi$ is the direction of the ray at $\hat P_1$)
\begin{equation*}
\hat r_0 \frac{\sin(\hat \phi)}{\sin(\bar \alpha - \hat \phi)} = \hat \ell_0 = \frac{\hat r_0 (1 - \cos(\hat \theta)) - \hat L (1 - \cos(\hat \theta - \hat \phi))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
{\color{red}where we have used Equation \eqref{Equa:ell_0_tent_general}},
i.e.
\begin{equation*}
\frac{{\color{red}{\hat L}}}{\hat r_0} = \frac{\sin(\bar \alpha - \hat \phi)(1 - \cos(\hat \theta)) - \sin(\hat \phi) (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha))}{\sin(\bar \alpha - \hat \phi)(1 - \cos(\hat \theta - \hat \phi))} = \frac{\sin(\bar \alpha) (\cos(\hat \phi) - \cos(\hat \theta - \hat \phi))}{\sin(\bar \alpha - \hat \phi) (1 - \cos(\hat \theta - \hat \phi))}.
\end{equation*}
The function
\begin{equation}
\label{Equa:Loverr0_tent}
\hat \phi \mapsto \frac{\sin(\bar \alpha) (\cos(\hat \phi) - \cos(\hat \theta - \hat \phi))}{\sin(\bar \alpha - \hat \phi) (1 - \cos(\hat \theta - \hat \phi))}
\end{equation}
is decreasing after $\bar \alpha + \hat \theta - \frac{\pi}{2}$, and its value at that angle is $0.966795$, see Fig. \ref{Fig:Loverr0_tent}: hence only for $\hat L \geq 0.966795 \hat r_0$ the tent may not be admissible.
\end{proof}

Consider finally the spiral $\tilde r(\phi;\phi_0)$, and let $\hat \phi_0$ {\color{red}be} the initial angle for the tent and $\hat \phi_2 = \hat \phi_0 + \hat \theta$ the final angle, and let \newglossaryentry{phihat3}{name=\ensuremath{\hat \phi_3},description={maximal angle for using the length bound as admissibility criterion for the tent}} $\gls{phihat3} \geq \hat \phi_0$. By considering the fastest growing spiral
\begin{equation*}
\dot r = \cot(\bar \alpha) r,
\end{equation*}
and observing that the worst situation is the one of the previous lemma (because it is the minimal length needed and applied at the last possible time), we obtain that if the tent is not admissible
\begin{equation}
\label{Equa:eastima_hat_r_2}
\begin{split}
\tilde r(\hat \phi_3) &\leq \tilde r(\hat \phi_0) e^{\cot(\bar \alpha)(\hat \phi_3 - \hat \phi_0)} - (\tilde L(\hat \phi_0 + \hat \theta) - \tilde L(\hat \phi_0)) e^{\cot(\bar \alpha)(\hat \phi_3 - \hat \phi_0 + \frac{\pi}{2} - \bar \alpha - \hat \theta)} \\
&\leq (\tilde L(\hat \phi_0 + \hat \theta) - \tilde L(\hat \phi_0)) \bigg( \frac{e^{\cot(\bar \alpha) (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{K_\mathrm{tent}} - 1 \bigg) e^{\cot(\bar \alpha) (\hat \phi_3 - \hat \phi_0 + \frac{\pi}{2} - \bar \alpha - \hat \theta)} \\
&\leq \tilde L(\hat \phi_3) \bigg( \frac{e^{\cot(\bar \alpha) (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{K_\mathrm{tent}} - 1 \bigg) e^{\cot(\bar \alpha) (\hat \phi_3 - \hat \phi_0 + \frac{\pi}{2} - \bar \alpha - \hat \theta)}.
\end{split}
\end{equation}
Hence by Corollary \ref{Cor:bound_length_gen} if
\begin{equation*}
\hat \phi_3 > \phi_0 + \omega \quad \text{and} \quad \bigg( \frac{e^{\cot(\bar \alpha) (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{K_\mathrm{tent}} - 1 \bigg) e^{\cot(\bar \alpha) (\hat \phi_3 - \hat \phi_0 + \frac{\pi}{2} - \bar \alpha - \hat \theta))} \leq 2.08
\end{equation*}
the tent is admissible. Numerically one obtains
\begin{equation*}
\hat \phi_3 - \hat \phi_0 \leq \bar \alpha + \hat \theta - \frac{\pi}{2} + \tan(\bar \alpha) \ln \bigg( \frac{2.08}{\frac{e^{\cot(\bar \alpha) (\bar \alpha + \hat \theta - \frac{\pi}{2})}}{K_\mathrm{tent}} - 1} \bigg) = 7.86127,
\end{equation*}
which in the $\tau$ coordinates corresponds to
\begin{equation}
\label{Equa:hattau3_cond}
\hat \tau_3 - \hat \tau_0 \leq 1.05358.
\end{equation}
We thus have the following

\begin{proposition}
\label{Prop:tent_admissible}
The tent is admissible for $\tau \geq 0$.
%\begin{equation*}
%\tau \geq 1 - \hat \tau - \frac{\tan(\bar \alpha)}{2\pi + \bar \alpha} \ln \bigg( \frac{2.08}{\frac{e^{\cot(\bar \alpha) \hat \theta}}{K_\mathrm{tent}} - 1} \bigg) = 0.277638.
%\end{equation*}
\end{proposition}

\begin{proof}
The estimate \eqref{Equa:hattau3_cond} gives that if the tent starting in $\tau > 0$ is not admissible, then at $\tau + 1.05258 > 1$ the length $\tilde L$ does not satisfy Corollary \ref{Cor:bound_length_gen}, which is a contradiction.
\end{proof}

\begin{remark}
\label{Rem:inital_tent}
%Note that we cannot deduce that the tent is always admissible for $\tau \geq 0$ (i.e. in the saturated part) as we will see in the next section: we have only proved that after $\frac{1}{4}$ round the spiral $\tilde r$ has settled enough so that the tent become admissible.
%
It is easy to see that the tent is not always admissible: if we assume that the spiral $\zeta$ has a very long segment, $\zeta$ asymptotically becomes by scaling
\begin{equation*}
\Omega_0 = B_{\cos(\bar \alpha)}(0), \quad \zeta = [0,1],
\end{equation*}
for which the fastest saturated is an arc. Indeed, in this situation the saturation condition for the tent reads as
\begin{align*}
0 &= \hat \ell_1 \cos(\bar \alpha) + \hat \ell_0 \cos(\bar \alpha - \hat \theta) + \cos(\hat \theta) - \cos(\bar \alpha) - \cos(\bar \alpha) (1 + \hat \ell_0 + \hat \ell_1) \\
&= \hat \ell_0 (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)) - 2 \cos(\bar \alpha) + \cos(\hat \theta).
\end{align*}
Being
\begin{equation*}
2 \cos(\bar \alpha) - \cos(\hat \theta) = - 0.10964 < 0,
\end{equation*}
the tent is not admissible.
\end{remark}

\begin{remark}
\label{Rem:tent_admis_optim}
We end this section with the observation that if the tent is admissible it is the optimal solution. This fact is clearly implied by the uniqueness of Proposition \ref{Prop:unique_optimal_guess}, and moreover by Remark \ref{Rem:trans_segm_arc} we can only transition from the segment case to the arc case, not the opposite.
\end{remark}


\subsubsection{An estimate on the final value $\hat r(\bar \phi)$}
\label{Sss:estima_final_value}


To conclude this section, we give a simplified formula for estimating the final value of $\hat r$ and the angle $\bar \phi = \hat \phi_0 + 2\pi + \bar \alpha$.

\begin{lemma}
\label{Lem:final_value_satu}
Assume that base of the tent is a convex curve, $\hat r_0$ is saturated and that $\tilde r$ is the saturated spiral starting from $\hat \phi_0$. Then it holds
\begin{equation*}
\hat r(\bar \phi) \geq \tilde r(\bar \phi) - \hat \ell_0 \geq \tilde r(\bar \phi) - \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \hat r_0.
\end{equation*}
\end{lemma}

\begin{proof}
Since the base of the spiral is a convex curve, then
\begin{equation*}
|\hat Q_2 - \hat Q_0| \leq \hat L,
\end{equation*}
and then
\begin{equation*}
\hat \ell_0 \leq \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \hat r_0.
\end{equation*}
By Theorem \ref{Cor:curve_cal_R_sat_spiral} it holds also
\begin{equation*}
\hat r_2 \geq \tilde r(\hat \phi_2) = \tilde r(\hat \phi_0 + \hat \theta).
\end{equation*}
Hence we conclude that
\begin{align*}
\hat r(\bar \phi) &= (\hat r_2 - \tilde r(\hat \phi_2)) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} + \tilde r(\bar \phi) - \hat \ell_0 \\
&\geq \tilde r(\bar \phi) - \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \hat r_0. \qedhere
\end{align*}
\end{proof}


%
%{\color{blue} NON SERVE?
%
%\begin{corollary}
%\label{Cor:r_2tent_criterion}
%Let $\gls{phihat3} > \phi_0$: then if the solution of the saturated spiral satisfies
%$$
%r(\hat \phi_3) \geq \hat L (\frac{e^{\cot(\bar \alpha)\hat \theta}}{K_\mathrm{tent}} - e^{\cot(\bar \alpha)(\frac{\pi}{2} - \bar \alpha)}) = 0.0990184 \hat L,
%$$
%then the tent is admissible.
%\end{corollary}
%
%\begin{proof}
%The worst configuration is again the one in the previous lemma: indeed it is convenient to have the initial ray starting from $0$, and in order to maximize $\hat r_2$ one does not take additional base length. Then we compute for the saturated spiral
%\begin{align*}
%\hat r_2 &\leq \hat r_0 e^{\cot(\bar \alpha) \hat \theta} - \hat L e^{\cot(\bar \alpha)(\frac{\pi}{2} - \bar \alpha)} \\
%&\leq \hat L \bigg( \frac{e^{\cot(\bar \alpha) \hat \theta}}{K_\mathrm{tent}} - e^{\cot(\bar \alpha)(\frac{\pi}{2} - \bar \alpha)} \bigg) = 0.0990184 \hat L. \qedhere
%\end{align*}
%\end{proof}
%
%
%
%
%
%\newglossaryentry{phihat00}{name=\ensuremath{\hat \phi_{00}},description={maximal angle for using the length bound as admissibility criterion for the tent}}
%\begin{align*}
%\tilde r(\hat \phi_2) - \hat L \bigg( \frac{e^{\cot(\bar \alpha)\hat \theta}}{K_\mathrm{tent}} - e^{\cot(\bar \alpha)(\frac{\pi}{2} - \bar \alpha)} \bigg) &\geq \tilde r(\hat \phi_2) - \tilde L(\hat \phi_2 - 2\pi - \bar \alpha) \bigg( \frac{e^{\cot(\bar \alpha)\hat \theta}}{K_\mathrm{tent}} - e^{\cot(\bar \alpha)(\frac{\pi}{2} - \bar \alpha)} \bigg) \\
%&\geq \tilde L(\hat \phi_2 - \gls{phihat00}) \bigg( \frac{e^{\cot(\bar \alpha)\hat \theta}}{K_\mathrm{tent}} - e^{\cot(\bar \alpha)(\frac{\pi}{2} - \bar \alpha)} \bigg)
%\end{align*}
%if $\hat \phi_{00} \geq \hat \phi_2 - 2\pi - \bar \alpha$.
%
%
%
%If we let the the evolution run up tp the angle such that we are outside the non saturated zone + one rotation this angle is such that the final point is at most
%\begin{equation*}
%\tan(\bar \alpha) + \frac{\pi}{2} - \bar \alpha = 2.80812,
%\end{equation*}
%so that its final value is at most
%\begin{equation*}
%e^{\cot(\bar \alpha)(\tan(\bar \alpha) + \frac{\pi}{2} - \bar  \alpha)} r_2 \leq \hat L e^{\cot(\bar \alpha)(\tan(\bar \alpha) + \frac{\pi}{2} - \bar  \alpha)} \bigg( \frac{e^{\cot(\bar \alpha)\hat \theta}}{K_\mathrm{tent}} - e^{\cot(\bar \alpha)(\frac{\pi}{2} - \bar \alpha)} \bigg) = 0.316647.
%\end{equation*}
%
%
%
%
%
%{\bf DA VEDERE DOPO LE STIME}
%
%We will now give a second functional whose positivity implies the positivity of $K_\mathrm{tent} \hat r_0 - \hat L$. The idea is to allow the base of the tent to be convex but not necessarily part of an admissible spiral.
%
%Assume that the base of the spiral $\hat Q$ is saturated in $\hat Q_0$. The best perturbation in order to have that the length $\hat L$ is maximal and $\hat r_0$ is minimal is in Fig. \ref{Fig:Loverr0_tent}. Indeed, by convexity the maximal length is when the base is a tent, and the angle $\hat \theta$ at $\hat Q_1$ is the critical angle for which $\hat r_0$ is minimal when the spiral after $\hat Q_1$ is the fastest saturated spiral of Section \ref{S:segment}.
%
%Since the derivative $\delta \tilde r$ of Proposition \ref{Prop:regions_pos_neg_segm} is independent on the admissibility, the above analysis holds also for the non-admissible spiral, and as observed before the formulas of Lemma \ref{Lem:relation_admissibility_tent} are linear so that they holds also for the non-admissible spiral.
%
%For a more precise definition, let $\zeta$ be a spiral and an angle $\phi_{00}$ such that $\phi_0 \in \phi_{00} + 2\pi + [\beta^-(\phi_{00},\beta^+(\phi_{00}]$, and let $\hat r$ be the convex spiral defined by:
%\begin{itemize}
%\item a segment $[\hat Q_0,\hat Q_1]$ with direction $\phi_0$ of length $\hat \ell_0'$,
%\item a segment $[\hat Q_1,\hat Q_2]$ with direction $\phi_0 + \hat \theta$ of length $\hat \ell'_1$, and such that $\hat Q_2$ is saturated,
%\item the saturated spiral from $\hat Q_2$ (corresponding angle $\phi_{00} + \hat \theta$)
%\end{itemize}
%
%Define thus
%\begin{equation}
%\label{Equa:AT2_def}
%AT2(\phi_0) = K_\mathrm{tent} \hat r_0 - (\hat \ell_0' + \hat \ell_1').
%\end{equation}
%Clearly
%\begin{equation*}
%AT2(\phi_0) \leq AT(\phi_0),
%\end{equation*}
%so that the positivity of the $AT2$ is sufficient. We will thus proceed as follows: we will analyze the positivity of $r(\bar \phi)$ together with the positivity of
%\begin{equation*}
%K_\mathrm{tent} \hat r(\bar \phi) - (\hat \ell_0 + \hat \ell_1).
%\end{equation*}
%Actually we will work with the perturbations,
%\begin{equation*}
%K_\mathrm{tent} \delta \hat r(\bar \phi) - (\delta \hat \ell_0 + \delta \hat \ell_1).
%\end{equation*}
%
%
%%
%%procedure to have an upper estimate on the length of the base of the spiral: by geometric consideration the worst case is when the base is a tent itself, indeed it is the longest convex curve with slopes $0,\hat \theta$ at the boundary. Moreover, $r_0$ is minimal, so that
%%\begin{equation}
%%\label{Equa:simply_tent_verification}
%%\frac{\sin(\bar \alpha) (\sin(\bar \alpha + \hat \theta) - \sin(\bar \alpha))}{\cos(\hat \theta) (1 - \sin(\bar \alpha))} \hat r_0 - \hat L \geq \frac{\sin(\bar \alpha) (\sin(\bar \alpha + \hat \theta) - \sin(\bar \alpha))}{\cos(\hat \theta) (1 - \sin(\bar \alpha))} \hat r_0 - (\hat \ell_0' + \hat \ell_1'),
%%\end{equation}
%%see Fig. \ref{Fig:worst_case_tent_L}. We will show that the above functional is positive for the base solution and remains positive for the perturbation.
%%
%%\begin{remark}
%%\label{Rem:non_admis}
%%We note that here we do not require to be admissible, in the sense that the angle made by the optimal ray ending at the tip $\hat Q_1$ with the segment $[\hat P_1,\hat P_2]$ is larger than $\frac{\pi}{2}$: however the formula of Lemma \ref{Lem:relation_admissibility_tent} holds independently from the admissibility, and thus we will use these formulas.
%%\end{remark}
%%
%%
%
%
%
%
%\subsubsection{Estimates of $\hat r_2$}
%\label{Sss:estima_hat_r_2}
%
%
%{\color{red} DA AGGIUNGERE QUALCOSA}
%
%
%In this final section we give a condition which implies immediately that the perturbation $\delta \check r(\bar \phi;s_0)$ is positive. This condition, as well as the condition above, yields that after 1 rounds the positivity of $\delta \check r$ is assured, so that we are left to study only the first rounds for $\delta \check r$.
%
%The idea is to compare $\delta \check r$ with $\delta \tilde r$: indeed, if $\check \phi_2$ is the rotation angle of $\check P_2$ (the last point of the tent, see Fig. \ref{Fig:checkr_notation}) and %$\check \phi_0 + \hat \theta$ is the rotation angle correspondin
%\begin{equation*}
%\delta \tilde r(\check \phi_2;s_0) \leq \delta \check r(\check \phi_2,s_0),
%\end{equation*}
%being the RDE linear and since we do only a partial rotation $\bar \phi = \check \phi_2 + 2\pi + \bar \alpha - \hat \theta$, we have (see Fig. \ref{fig:comparison:saturated})
%\begin{equation}
%\label{eq:comp:sat}
%\check r(\bar \phi;s_0) - \tilde r(\bar \phi;s_0) = e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} \big( \check r(\check \phi_2;s_0) - \tilde r(\check \phi_2,s_0) \big) - \check \ell_0.
%\end{equation}
%The above formula is written for the derivative, but being linear holds also for the original solution, i.e
%\begin{equation*}
%\delta \check r(\bar \phi;s_0) - \delta \tilde r(\bar \phi;s_0) = e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} \big( \delta \check r(\check \phi_2;s_0) - \delta \tilde r(\check \phi_2,s_0) \big) - \delta \check \ell_0.
%\end{equation*}
%
%\begin{figure}
%\centering\includegraphics[scale=0.5]{comparisonwithsaturated.png}
%\caption{To quantify the quantity $\hat r(\bar\phi;s_0)$ we compare the black spiral with the saturated spiral (red curve). This motivates Equation \eqref{eq:comp:sat}, where the length $\overline{AB}=\hat r(\bar\phi-2\pi-\bar\theta)-\bar r(\bar\phi-2\pi-\bar\theta)$ is propagated in the angle $\bar\phi$ via the RDE of Saturated Spirals.}
%\label{fig:comparison:saturated}
%\end{figure}
%
%\begin{lemma}
%\label{Lem:estima_tent}
%Assume that the base of the tent $\hat \zeta$ of Fig. \ref{Fig:tent_comput_geo} is in the region where $\tilde r$ is saturated. Then
%\begin{equation*}
%\tilde r(\check \phi_2;s_0) < \hat r(\check \phi_2;s_0), \quad \hat \ell_0 \leq \hat r(\check \phi_0;s_0) \frac{1- \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} < 0.313454 \hat r(\check \phi_0;s_0).
%\end{equation*}
%The same holds for the perturbation $\delta r$, i.e.
%\begin{equation*}
%\delta \tilde r(\check \phi_2;s_0) < \delta \hat r(\check \phi_2;s_0), \quad \delta \hat \ell_0 \leq \hat r(\check \phi_0;s_0) \frac{1- \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} < 0.313454 \delta \hat r(\check \phi_0;s_0).
%\end{equation*}
%\end{lemma}
%
%\begin{proof}
%We use the saturation condition for the solution $\tilde r$,
%\begin{equation*}
%\tilde r(\check \phi_2;s_0) + L - \tilde r(\check \phi_0;s_0) + \cos(\bar\alpha)) \int \frac{\tilde r(\phi;s_0)}{\sin(\bar \alpha)} d\phi = 0,
%\end{equation*}
%and the same for the tent,
%\begin{equation*}
%\hat r(\check \phi_2;s_0) + L - \tilde r(\check \phi_0;s_0) + \cos(\bar\alpha)) (\ell_0 + \ell_1) = 0.
%\end{equation*}
%Since by convexity
%\begin{equation*}
%\int \frac{\tilde r(\phi;s_0)}{\sin(\bar \alpha)} d\phi < \ell_0 + \ell_1,
%\end{equation*}
%unless $\tilde r = 0$, we obtain the first inequality
%\begin{equation*}
%\tilde r(\check \phi_2;s_0) \leq \hat r_2(\phi;s_0).
%\end{equation*}
%The second follows from the formula \eqref{Equa:ell_0_tent_general}, 
%\begin{equation*}
%\begin{split}
%\hat \ell_0 &= \frac{(\hat Q_2 - \hat Q_0) \cdot e^{\i \hat \theta} - L + \hat r_0 (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
%\big[ |\hat Q2 - \hat Q_0| \leq L \big] \quad &\leq \frac{\hat r_0 (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}.
%\end{split}
%\end{equation*}
%We used that for continuous curves
%\begin{equation*}
%|\hat Q2 - \hat Q_0| \leq L.
%\end{equation*}
%
%The same formulas holds for the perturbations $\delta r_2,\hat r_2$, provided that
%\begin{equation*}
%\int \frac{\delta \tilde r(\phi;s_0)}{\sin(\bar \alpha)} d\phi \leq \delta \ell_0 + \delta \ell_1,
%\end{equation*}
%The picture of Fig. \ref{Fig:tent_comput_geo} is the same for the perturbation $\delta \tilde r,\delta \hat r$ provided that the base $\check \zeta$ is a convex spiral. Using \eqref{Equa:DeltahatQ_tent}, this occurs when $\tilde r \geq 0$ in the region at the base of the tent, i.e. for the angles $[\hat \phi_0,\hat \phi_2] - 2 \pi - \bar \alpha$ (recall that we are in the saturated region).
%%
%%
%%Observe that by
%%\begin{equation*}
%%L \geq |\Delta Q|,
%%\end{equation*}
%%it follows immediately
%%\begin{equation*}
%%\hat \ell_0 \leq \hat r_0 \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}.
%%\end{equation*}
%%Considering now the curve with radius of curvature given by $\tilde r$: then this curve is saturated, and thus it is impossible that $\hat r_2 = r_2$ is some point for any admissible curve, because the length of the tent is larger than the one of the saturated spiral.
%\end{proof}
%
%
%
%\subsubsection{A comparison for the tent case and the arc case}
%\label{Sss:comparison_tent_arc}
%
%
%In order to simplify the verification that the optimal solution is a generically a tent, we compare the arc case with a non admissible tent: this means that the angle \gls{thetatildeseg} (made by the optimal ray $r(\phi_0)$ and the segment $[P_1,P_2]$) is greater than $\frac{\pi}{2}$. For a given angle $\bar \phi$, let $r(\bar \phi)$ be the solution obtained by closing the last round with an arc (i.e. the arc is the only admissible solution here), and let $r_\mathrm{tent,n.a.}(\bar \phi)$ the solution obtained by closing with a segment even if $\bar \theta > \frac{\pi}{2}$ (i.e. it is not admissible (n.a.)).
%
%\begin{proposition}
%\label{Prop:tent_worst}
%It holds $r_\mathrm{tent,n.a.}(\bar \phi) < r(\bar \phi)$.
%\end{proposition}
%
%\begin{proof}
%First observe that we can reconstruct the arc solution by considering the non admissible segment solution and following the arc, i.e.
%\begin{equation*}
%r(\bar \phi) = \int \delta r_\mathrm{tent}(\bar \phi;s_0) ds_0.
%\end{equation*}
%It is thus enough to show that the derivative is $0$ in the arc region, because after it coincides with the segment solution.
%
%In this region for the non admissible tent the angles are as follows:
%\begin{equation*}
%\theta = \bar \theta - \frac{\pi}{2} > 0,
%\end{equation*}
%and since the derivative in the segment case depends only on $\theta$, if follows that the integral is strictly positive.
%\end{proof}
%
%
%
%
%
%%
%%In order to estimate the value $\hat r(\bar \phi;s_0)$, the idea will be to compare $\hat r_2(\bar \phi - 2\pi + \hat \theta;s_0)$ with $\tilde r_2(\bar \phi - 2\pi + \hat \theta;s_0)$, and then write
%%\begin{align}\label{eq:comp:sat}
%%    \notag\hat r(\bar \phi;s_0) &= e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} \big( \hat r_2(\bar \phi - 2\pi + \hat \theta;s_0) - \tilde r_2(\bar \phi - 2\pi + \hat \theta;s_0) \big) \\
%%    & \quad + \tilde r_2(\bar \phi;s_0) - \hat \ell_0.
%%\end{align}
%%{\color{red} non ho capito perchè hai messo il pedice $2$, non sono le soluzioni della spirale saturata $\bar r(\phi,s_0)$ della sezione $6$? No, lo so la notazione fa schifo}
%%
%%We next give some condition on $\hat r_0,L,Q_2-Q_1$ which assures that the above quantity is positive. The statements are based on the RDE, so that they hold also in the case of the perturbation.
%%
%%
%%
%%
%%\subsection{Formulas for the arc case}
%%\label{Ss:formulas_arc}
%%
%%
%%The geometric situation is in Fig. \ref{Fig:arc_comnpu}.
%%
%%\begin{figure}
%%\resizebox{.75\textwidth}{!}{\input{arc_compu.pdf_t}}
%%\caption{Geometric setting for the arc perturbation.}
%%\label{Fig:arc_comnpu}
%%\end{figure}
%%
%%The relations among points are \newglossaryentry{Phat-}{name=\ensuremath{\hat P^-},description={beginning of the arc in the arc perturbation}} \newglossaryentry{Qhat-}{name=\ensuremath{\hat Q^-},description={initial point of the optimal ray ending in $\hat P^-$ in the arc perturbation}} \newglossaryentry{rhat-}{name=\ensuremath{\hat r^-},description={optamal ray ening in $\hat P^-$ for the arc perturbation}} \newglossaryentry{rhat1}{name=\ensuremath{\hat r_1},description={optamal ray ening in $\hat P_1$ for the tent or arc perturbation}} \newglossaryentry{Deltaphicheck}{name=\ensuremath{\Delta \check \phi},description={opening angle of the arc for the arc perturbation}} \newglossaryentry{omegacheck}{name=\ensuremath{\check \omega},description={angle given by $\check \omega = \check \theta + \Delta \check \phi$ for the arc perturbation}} \newglossaryentry{thetacheck}{name=\ensuremath{\check \theta},description={angle formed by the arc and the segment $\hat \ell_0$ for the arc perturbation}} \newglossaryentry{Lhat1}{name=\ensuremath{\hat L_1},description={length of the arc $\overset{\frown}{\hat Q^- \hat Q_1}$ for the arc perturbation}}
%%\begin{equation}
%%\label{Equa:hatP0P-_arc}
%%\gls{Phat0} = \gls{Qhat0tent} + \gls{rhat0} e^{\i 0}, \quad \ \gls{Phat-} = \hat P_0 + \gls{ellhat0} e^{\i \bar \alpha} = \gls{Qhat-} + \gls{rhat-} e^{i (\bar \alpha + \gls{thetacheck} - \frac{\pi}{2})},
%%\end{equation}
%%\begin{equation}
%%\label{Equa:hatP1_arc}
%%\gls{Phat1tent} = \gls{Qhat1tent} + \gls{rhat1} e^{\i (\bar \alpha + \gls{omegacheck} - \frac{\pi}{2})}, \quad \gls{omegacheck} = \gls{thetacheck} + \gls{Deltaphicheck}, \quad \gls{rhat1} + \gls{Lhat1} = \check r^-,
%%\end{equation}
%%\begin{equation}
%%\label{Equa:hatP2_arc}
%%\gls{Phat2tent} = \gls{Phat1tent} + \gls{ellhat1} e^{\i (\bar \alpha + \gls{omegacheck})} = \gls{Qhat1tent} + \gls{rhat1} e^{i (\gls{omegacheck} + \bar \alpha - \frac{\pi}{2})} + \gls{ellhat1} e^{\i (\bar \alpha + \gls{omegacheck})} = \gls{Qhat2tent} + \gls{rhat2} e^{\i \gls{omegacheck}}.
%%\end{equation}
%%The relation among the angles is by
%%\begin{equation*}
%%\check \theta = h_1(\Delta \check \phi),
%%\end{equation*}
%%where $h_1$ is given by Lemma \ref{Lem:study_g_1_arc}, and the saturation condition is \newglossaryentry{Lcheckprime}{name=\ensuremath{\check L'},description={length of the arc $\overset{\frown}{\hat P^- \hat P_1}$ for the arc perturbation}}
%%\begin{equation*}
%%\hat r_2 + \gls{Lhattent} - \hat r_0 - \cos(\bar \alpha) \big( \hat \ell_0 + \gls{Lcheckprime} + \hat \ell_1 \big) = 0,
%%\end{equation*}
%%where $\check L'$ is the arc length $\overset{\frown}{\check P^- \check P_1}$. 
%%
%%We are interested in the perturbation of the above equation: we thus have
%%\begin{equation}
%%\label{Equa:saturation_arc_gen}
%%\begin{split}
%%0 &= \delta \hat r_2 + \delta \hat L - \delta \hat r_0 - \cos(\bar \alpha) \big( \delta \hat \ell_0 + \delta \check L' + \delta \ell_1 \big) \\
%%\big[(\ref{Equa:hatP2_arc})\big] \quad &= (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i \check \omega} + (\delta \hat r_1 - \hat \ell_1 \delta \check \omega) \sin(\bar \alpha) + \delta \hat L - \delta \hat r_0- \cos(\bar \alpha) \bigg( \delta \hat \ell_0 - \hat r^- \delta \check \theta + \int_{\check \theta}^{\check \omega} \delta \hat r(\phi) d\phi \bigg),
%%%\big[(\ref{Equa:hatP1_arc})\big] \quad &= (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i \check \omega} + \delta \hat r_1 \sin(\bar \alpha) + \hat r_1 \delta \check \omega \cos(\bar \alpha) - \hat \ell_1  \delta \check \omega \sin(\bar \alpha) + \delta \hat L - \delta \hat r(\check \phi_0) - \cos(\bar \alpha) \Bigg[ \delta \hat \ell_0 - \hat r^- \delta \check \theta + \int_{\check \theta}^{\check \omega} \delta r(\phi) d\phi + \hat r_1 \delta \check \omega \Bigg] \\
%%\end{split}
%%\end{equation}
%%where we have used
%%\begin{equation*}
%%\delta \hat r_2 = (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i \check \omega} + (\delta \hat r_1 - \hat \ell_1 \delta \check \omega) \sin(\bar \alpha) + (\hat r_1 \delta \check \omega + \delta \ell_1) \cos(\bar \alpha), \quad \delta \check L' = - \hat r^- \delta \check \theta + \int_{\check \theta}^{\check \omega} \delta \hat r(\phi) d\phi + \hat r_1 \delta \check \omega.
%%\end{equation*}
%%
%%Since the perturbation has initial data
%%\begin{equation}
%%\label{Equa:delta_hatr2}
%%\hat r(\check \omega + \phi) = \hat r_2 (1 + \cot(\bar \alpha) (\phi - \check \omega)) - L(\phi) + L(\check \omega), \quad \delta \hat r(\check \omega) = \delta \hat r_2 - \hat r_2 \cot(\bar \alpha) \delta \check \omega - \hat R_2 \delta \check \omega,
%%\end{equation}
%%where $R_2$ is the radius of curvature at $\hat Q_2$, by \eqref{Equa:hatP2_arc} we have
%%\begin{equation*}
%%\delta \hat r_2 - \cot(\bar \alpha) \hat r_2 \delta \check \omega = \frac{1}{\sin(\bar \alpha)} \big[ (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i (\check \omega + \bar \alpha - \frac{\pi}{2})} + (\delta \hat r_1 - \hat \ell_1 \delta \check \omega) \big],
%%\end{equation*}
%%and we rewrite \eqref{Equa:saturation_arc_gen} as
%%\begin{equation}
%%\label{Equa:initla_arc_gen}
%%\begin{split}
%%\delta \hat r_2 - \cot(\bar \alpha) \hat r_2 &= \frac{1}{\sin(\bar \alpha)^2} \bigg[ (\delta \hat Q_1 - \delta \hat Q_2) \cdot \big( \sin(\bar \alpha) e^{\i (\check \omega + \bar \alpha - \frac{\pi}{2})} - e^{\i \check \omega} \big) - \delta \hat L + \delta \hat r_0 + \cos(\bar \alpha) \bigg( \delta \hat \ell_0 - \hat r^- \delta \check \theta + \int_{\check \theta}^{\check \omega} \delta \hat r(\phi) d\phi \bigg) \bigg] \\
%%&= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \bigg[ - (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i (\check \omega + \bar \alpha)} + \delta \hat \ell_0 - \hat r^- \delta \check \theta + \int_{\check \theta}^{\check \omega} \delta \hat r(\phi) d\phi \bigg] + \frac{- \delta \hat L + \delta \hat r_0}{\sin(\bar \alpha)^2}.
%%\end{split}
%%\end{equation}
%%Using \eqref{Equa:hatP0P-_arc} we can write
%%\begin{equation*}
%%\hat r^- \delta \check \theta = (\delta \hat Q_0 - \delta \hat Q_1) \cdot e^{i(\check \theta + \bar \alpha)} + \delta \hat r_0 \cos(\bar \alpha + \check \theta) + \delta \hat \ell_0 \cos(\check \theta),
%%\end{equation*}
%%\begin{equation*}
%%\delta r^- = (\delta \hat Q_0 - \delta \hat Q^-) \cdot e^{i(\bar \alpha + \check \theta - \frac{\pi}{2})} + \delta \hat r_0 \sin(\bar \alpha + \check \theta) + \delta \hat \ell_0 \sin(\check \theta).
%%\end{equation*}
%%and since for $\phi \in [\check \theta,\check \omega]$
%%\begin{equation*}
%%\hat r(\phi) = \hat r^- - \hat L(\phi) + \hat L(\check \theta),
%%\end{equation*}
%%we also have
%%\begin{equation*}
%%\delta \hat r(\phi) = \delta \hat r^- - \delta \hat L(\phi) + \delta \hat L(\check \theta),
%%\end{equation*}
%%\begin{align*}
%%\int_{\check \theta}^{\check \omega} \delta \hat r &= \delta \hat r^- \Delta \check \phi - \int_{\check \theta}^{\check \omega} ( \delta \hat L(\phi) - \delta \hat L(\check \theta) ) d\phi \\
%%&= \Big[ (\delta \hat Q_0 - \delta \hat Q^-) \cdot e^{i(\bar \alpha + \check \theta - \frac{\pi}{2})} + \delta \hat r_0 \sin(\bar \alpha + \check \theta) + \delta \hat \ell_0 \sin(\check \theta) \Big] \Delta \check \phi - \int_{\check \theta}^{\check \omega} ( \delta \hat L(\phi) - \delta \hat L(\check \theta) ) d\phi.
%%\end{align*}
%%Substituting into \eqref{Equa:initla_arc_gen} we obtain
%%\begin{equation}
%%\label{Equa:2_initla_arc_gen}
%%\begin{split}
%%\delta \hat r_2 - \cot(\bar \alpha) \hat r_2 &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \bigg[ - (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i (\check \omega + \bar \alpha)} - (\delta \hat Q_0 - \delta \hat Q_1) \cdot e^{i(\check \theta + \bar \alpha)} + (\delta \hat Q_0 - \delta \hat Q^-) \cdot e^{i(\bar \alpha + \check \theta - \frac{\pi}{2})} \Delta \check \phi \bigg] \\
%%& \quad - \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \int_{\check \theta}^{\check \omega} ( \delta \hat L(\phi) - \delta \hat L(\check \theta) ) d\phi - \frac{\delta \hat L(\check \omega)}{\sin(\bar \alpha)^2} \\
%%&\quad + \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \bigg( \frac{1}{\cos(\bar \alpha)} - \cos(\bar \alpha + \check \theta) + \sin(\bar \alpha + \check \theta) \Delta \check \phi \bigg) \bigg] \delta \hat r_0 \\
%%& \quad + \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\check \theta) + \sin(\check \theta) \delta \Delta \check \phi) \bigg] \delta \hat \ell_0.
%%\end{split}
%%\end{equation}
%%The final value is then computed by
%%\begin{equation}
%%\label{Equa:final_arc_gen}
%%\begin{split}
%%\delta \hat r(\bar \phi) &= \bigg[ \delta \hat r_2 - \cot(\bar \alpha) \hat r_2 \delta \check \omega - \delta \tilde r_2 \bigg] e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \check \theta - \Delta \check \phi)} + \delta \tilde r(\bar \phi) - \delta \check \ell_0 \\
%%[(\ref{Equa:thetaDeltaphi_def}] \quad &= \Bigg\{ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \bigg[ - (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i (\check \omega + \bar \alpha)} - (\delta \hat Q_0 - \delta \hat Q_1) \cdot e^{i(\check \theta + \bar \alpha)} + (\delta \hat Q_0 - \delta \hat Q^-) \cdot e^{i(\bar \alpha + \check \theta - \frac{\pi}{2})} \Delta \check \phi \bigg] \\
%%& \qquad - \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \int_{\check \theta}^{\check \omega} ( \delta \hat L(\phi) - \delta \hat L(\check \theta) ) d\phi - \frac{\delta \hat L(\check \omega)}{\sin(\bar \alpha)^2} \\
%%& \qquad + \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \bigg[ \frac{1}{\cos(\bar \alpha)} - \cos(\bar \alpha + \check \theta) + \sin(\bar \alpha + \check \theta) \Delta \check \phi \bigg] \delta \hat r_0 - \delta \tilde r_2 \Bigg\} e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \check \theta - \Delta \check \phi)} + \delta \tilde r(\bar \phi) \\
%%&= \frac{\cot(\bar \alpha) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \check \theta - \Delta \check \phi)}}{\sin(\bar \alpha)} \\
%%& \quad \cdot \Bigg\{ \bigg[ - (\delta \hat Q_1 - \delta \hat Q_2) \cdot e^{\i (\check \omega + \bar \alpha)} - (\delta \hat Q_0 - \delta \hat Q_1) \cdot e^{i(\check \theta + \bar \alpha)} + (\delta \hat Q_0 - \delta \hat Q^-) \cdot e^{i(\bar \alpha + \check \theta - \frac{\pi}{2})} \Delta \check \phi \bigg] \\
%%& \qquad - \int_{\check \theta}^{\check \omega} ( \delta \hat L(\phi) - \delta \hat L(\check \theta) ) d\phi - \frac{\delta \hat L(\check \omega)}{\cos(\bar \alpha)} \\
%%& \qquad + \bigg[ \frac{1}{\cos(\bar \alpha)} - \cos(\bar \alpha + \check \theta) + \sin(\bar \alpha + \check \theta) \Delta \check \phi \bigg] \delta \hat r_0 - \frac{\sin(\bar \alpha)}{\cot(\bar \alpha)} \delta \tilde r_2 + \big( 1 - \cos(\check \theta) + \sin(\check \theta) \Delta \check \phi \big) \delta \tilde r(\bar \phi) \Bigg\},
%%\end{split}
%%\end{equation}
%%where $\delta \tilde r$ is the evolution for the perturbation of the saturated spiral. We remark that the critical relation $\check \theta = h_1(\Delta \check \phi)$ gives that $\delta \hat \ell_0$ disappears in the above formula.
%%
%%\begin{remark}
%%\label{Rem:different_der}
%%Note that the derivative is different, perhaps due to the fact that the angle for the segment case are fixed, while here they may change because we are on the critical curve $\check \theta = h_1(\Delta \check \phi)$.
%%\end{remark}
%}


==> partitoltearco.tex <==
\begin{itemize}
    \item $r_{\phi_0}(\phi) = r(\phi)$ for every $\phi \leq \phi_0$: set $P_0 = \zeta(s^+(\phi_0))$;
    \item $r_{\phi_0}(\phi) \subset \lbrace u = u(P_0) \rbrace$ for $\phi \in [\phi_0, \phi_0 + \Delta \phi = \phi_1]$;
    \item for $\phi \in [\phi_1,\phi_2]$, $r_{\phi_0}(\phi)$ corresponds to a segment of endpoints $P_1,P_2$ such that %$P_1 \in \lbrace u = u((r(\bar\phi),\bar\phi) \rbrace$ and 
    $P_2$ is saturated for the admissibility functional \eqref{eq:new:Adm:funct}: in this setting this takes the form
        \begin{equation}
        \label{eq:sat:family}
             \mathcal A_{\bar\sigma,\hat\sigma}(P_2) = u(P_2) - \frac{1}{\bar \sigma} |P_2 - P_1| - \frac{1}{\bar \sigma} L(P_0 P_1) - \frac{s^+(\phi_0)}{\hat \sigma}=0,
        \end{equation}
        where $u$ is the minimum time function and $L(P_0 P_1)$ denotes the length of the level set from the starting point $P_0$ until the point $P_1$, and $s^+(\phi_0)$ is the length of the spiral up to the point $P_0$. Moreover, by admissibility for the functional \eqref{eq:new:Adm:funct} and convexity as in Section \ref{S:case:study}, we must require that the segment $P_1P_2$ is tangent to $\lbrace u = u(P_0) \rbrace$ in $P_1$ and tangent to the saturated spiral with speed $\bar \sigma$ in $P_2$; %. Here we use the new functional \eqref{eq:sat:family} because in the case $P_2\equiv P_1\equiv P_0$ it is the admissibility functional \eqref{eq:admissibility:functional} for $\hat\sigma$, that is the point $P_0$ must be admissible for the functional \eqref{eq:admissibility:functional}. 
    \item $r_{\phi_0}(\phi)$ is a saturated spiral for every $\phi \geq \phi_2$ for the critical speed $\bar \sigma$, that is, if we denote by $\beta_{\phi_0}$ the function describing the angle that a fire ray does with the generalized spiral, then $\beta_{\phi_0}(\phi) = \bar \alpha = \arccos(\frac{1}{\bar \sigma})$ for every $\phi \geq \phi_2$. 
\end{itemize}
   % \begin{remark}\label{rmk:angle:length}
    %    We have denoted the family as $f_{\phi_0}$ instead of $f_s$ with $s$ length parameter since the computations $f_{\phi_0+\delta\phi_0}-f_{\phi_0}$ with the angle parameter are easier to handle. Only later we change back to the length parameter. 
    %\end{remark}

The above construction assigns the choice of $\beta(\phi)$ for all angles $\phi \geq \bar \phi_0$.

The next step is to write the equation satisfied by the derivative $\bar r_s$ of \eqref{eq:derivative:family}. For this computation, we refer to Fig. \ref{fig:enpert:arc}. We list below the points and quantities which we will use, as well as some notation for convenience: %for an infinitesimal perturbation of the initial position:

\begin{itemize}
    \item $P_0 = \zeta(\bar s) = \zeta(\phi_0)$, the base point of the generalized barrier $\zeta_{\bar s}$, and we call $O_0 \in Z$ the base point of the optimal ray arriving in $P_0$ (Definition \ref{def:starting:point};
%    \medskip
    
    \item $P_1$, the starting point of the tangent segment point on the same level set as $P_0$, and we call $O_1 \in Z$ the base point of the optimal ray arriving in $P_1$. 
%    \medskip
    
    \item $\Delta \phi$ is the angle covered by the arc $P_0P_1$ along the level set: if $\phi_i$ is the angle of $P_i$, $i=1,2,3$, then $\Delta \phi = \phi_1 - \phi_0$;
%    \medskip
    
    \item $P_2$, the end point of the segment, from which a saturated spiral starts, tangent to the segment, and we call $O_2 \in Z$ the base point of the optimal ray arriving in $P_2$;
    
    \item $\theta_0 = \beta^+(\phi_0) \in [0,\frac{\pi}{2}]$;
    
    \item the local fire frames, given by the unit vectors
    $$
    \textbf{n}(P_1) = \frac{\nabla u(P_1)}{|\nabla u(P_1)|}, \qquad \textbf{n}(P_2) = \frac{\nabla u(P_2)}{|\nabla u(P_2)|}, \qquad \textbf{t}(P_1) = \frac{P_2-P_1}{|P_2-P_1|}.
    $$
    
%    \item $\delta s = \overline{P_0\tilde P_0}$, with $\delta s<<1$, and 
%    \begin{equation}
%        h=\delta s\cos\theta_0.
%    \end{equation}
%    \medskip
    
    \item the infinitesimal perturbation of all points will be denoted by $\delta P_i$, $i=0,1,2$.
%    \medskip
%    
%    \item Call $\phi_0$ the angle corresponding to the point $P_0$ and $\phi_1$ the angle corresponding to $P_1$, that is $\Delta\phi=\phi_1-\phi_0$.
%    \medskip

    \item We will use the notation $f_{\phi_0}(P_2)$, $f_{\phi_0}(P_1)$ to denote $f_{\phi_0}(\phi_2)$ and $f_{\phi_0}(\phi_1)$. We remark that for every point $Q$ in the level set of endpoints $P_0,P_1$ it holds $f_{\phi_0}(Q)=r(P_0)=f_{\phi_0}(P_1).$
\end{itemize}

%, and hence we compute $\tilde r_{\bar s} = r_{\bar s + \delta \bar s}$ (for shortness we will now write the dependence w.r.t. $\delta \bar s$): the perturbed starting point is $\tilde P_0$ given by %, that is
%\begin{equation*}
%    \tilde P_0 = P_0 + \delta \bar s e^{i \theta_0}, \quad \theta_0 = \beta^+(\bar s_0)
%\end{equation*}
%where $\theta_0$ is the angle with respect to the direction of fire rays at $P_0$ (see Figure \ref{fig:enpert:arc}) (it is $\beta^+(\phi_0)$ according to the notations of Section \ref{s:admissible:barriers}). Here and in the following we will denote by $\textbf{n}(P)$ the unit vector in the direction of the fire rays at a point $P$ (thus $\nabla u$, where $u$ is the minimum time function) and $\textbf{t}(P)$ will denote the tangent at the level sets.
%This means that we follow the level set for a positive angle $\Delta\phi$ up to a point $P_1$, and then a segment with direction $\textbf{t}(P_1)$, up to a point $P_2$. The point $P_2$ is saturated (in the sense of equation \eqref{eq:sat:family}) and it holds $\angle \textbf{n}(P_2),\textbf{t}(P_1)=\bar\alpha$. More precisely, we have:
%
%\begin{remark}
%    We remark that the starting point on the spiral of the rays for $P_i$ and $\tilde P_i$ is the same: indeed, if the ray $\bar\gamma_{P_i}$ is not tangent to the curve, it is clearly true. If it is tangent, then if $P_i\tilde P_i=\mathcal{O}(\delta s)$, if we call the two starting points $O_i,\tilde O_i$ then $O_i\tilde O_i= o(\delta s)$, therefore we can assume that the starting point is the same.
%\end{remark}

% We underline that here the computations are performed with the parameter $h$ instead of the parameter $s$ of the family, since it is the difference in time for the fire to reach $\tilde P_0$, $P_0$. We chose this description to make the computations more direct. In the following we will change back all the formulas in order to deal directly with $\bar f_s$ with the length parameter.
\noindent \textbf{Relations at point $P_0$:} the point $P_0 = \zeta(\bar s)$ is moved to the point $\zeta(\bar s + \delta \bar s)$, so that
\begin{equation*}
    \delta P_0 = \delta \bar s e^{i\beta^+(\phi_0)},
\end{equation*}
We will use for shortness the notation
\begin{equation}
\label{Equa:theta_0_def}
    \theta_0 = \beta^+(\phi_+0).
\end{equation}
The variation of the time function and of the spiral length are respectively
\begin{equation*}
    u(P_0 + \delta P_0) = u(P_0) + \delta \bar s \cos(\theta_0),
\end{equation*}
and $\delta s$.
%\begin{equation}
%    s^+(P_0 + \delta P_0) = L(P_0)+\frac{h}{\cos\theta_0},
%\end{equation}
%where $L(P)$ is the length of the spiral up to the point $P$.
The variation of the angle $\phi_0$ is %reads as
\begin{equation}
\label{eq:delta:phi:0}
    r(P_0) \delta \phi_0 = \delta \bar s \sin(\theta_0),
\end{equation}
%(recall $r$ is the radius of the original spiral $Z$ fixed at the very beginning), therefore 
and the position of the new point $\tilde P_0$ is
\begin{equation*}
    P_0 + \delta P_0 = P_0 + \delta \bar s \cos(\theta_0) \textbf{n}(P_0) + r(P_0) \delta \phi_0 \textbf{t}(P_1).
\end{equation*}
\medskip

\noindent \textbf{Relations at point $P_1$:} using that the point $P_1$ is on the same level set as $P_0$, we obtain
\begin{equation*}
    u(P_1 + \delta P_1) = u(P_0 + \delta P_0) = u(P_0) + \delta \bar s \cos(\theta_0).% =u(P_1)+h.
\end{equation*}
The position of the perturbed point is
\begin{equation*}
    P_1 + \delta P_1 = P_1 + \delta \bar s \textbf{n}(P_1) + r_{\phi_0}(P_1) \delta \phi_1 \textbf{t}(P_1).
\end{equation*}
The slope of the perturbed segment $[P_1 + \delta P_1,P_2 + \delta P_2]$ can be now computed because of its tangency with the level set, obtaining its unit direction to be $e^{i(\phi_1 + \delta \phi_1 + \frac{\pi}{2})}$.% Indeed here we cannot a priori assume that the fire rays arrive parallel at the points $P_1,\tilde P_1$.

\medskip 

\noindent\textbf{Relations at point $P_2$:} here we use the tangency with the saturated spiral. The slope of the segment arriving at $P_2 + \delta P_2$ is $e^{i(\phi_1 + \delta \phi_1 + \frac{\pi}{2})}$, and the slope of the starting spiral is $e^{i(\phi_2 + \delta \phi_2 + \bar\alpha)}$: the tangency requirement implies
%Therefore, since we require them to be parallel, the condition on the angles reads as
\begin{equation*}
    \phi_1 + \delta \phi_1 + \frac{\pi}{2} = \phi_2 + \delta \phi_2 + \bar \alpha \quad \Rightarrow \quad \delta \phi_1 = \delta \phi_2.
\end{equation*}
%The difference in slope between the two vectors 
%$$\frac{\tilde P_2-\tilde P_1}{|\tilde P_2-\tilde P_1|}\text{ and } \frac{P_2- P_1}{| P_2- P_1|}$$
%is $\delta\phi_1=\delta\phi_2$, 
Therefore the position of the perturbed point $P_2 + \delta {P}_2$ can be computed as
\begin{equation*}
    \delta P_2 = \big( \delta \bar s \cos(\theta_0) - |P_2 -P_1| \delta \phi_1 \big) \mathbf{n}(P_1) + \left( \big( \delta \bar s \cos(\theta_0) - |P_2 -P_1| \delta \phi_1 \big) \cot(\bar \alpha) + \frac{r_{\phi_0}(P_2)}{\sin(\bar \alpha)} \delta \phi_1 \right) \mathbf{t}(P_1).
\end{equation*}

\medskip

\noindent \textbf{Saturation:} we use the saturation condition, i.e. $P_2 + \delta {P_2}$ is a saturated point as well as $P_2$: for the point $P_2$ this reads as
    \begin{equation}
    \label{eq:sat:1}
        u(O_2) + |P_2-O_2| = \cos(\bar \alpha) |P_2 - P_1| + \cos(\bar \alpha) \widearc{P_0 P_1} + \cos(\hat \alpha) \bar s,
    \end{equation}
and for $P_2 + \delta P_2$
%We write the same equation for the perturbed point. 
%
%\medskip
%
%\textbf{Saturation  perturbed}: $\tilde P_2$ is a saturated point:
    \begin{equation}
    \label{eq:sat:2}
\begin{split}
u(O_2) + |P_2 + \delta P_2 - O_2| &= \cos(\bar \alpha) |P_2 + \delta P_2 - P_1 - \delta P_1| \\
& \quad + \cos(\bar \alpha) \widearc{(P_0 + \delta P_0)(P_1 + \delta P_1)} + \cos(\hat \alpha) (\bar s + \delta \bar s).
\end{split}
    \end{equation}
%where in the last we used that the arc and the segment are tangent.
By elementary computations
%    We compute all the quantities of the previous equations. We have that: 
%    
    \begin{align*}
        \widearc{(P_0 + \delta P_0)(P_1 + \delta P_1)} = %\tilde P_1\tilde P_0 &=\int_{\phi_0+\delta\phi_0}^{\phi_1+\delta\phi_1} (f_{\phi_0}(\eta)+h)d\eta \\ &= P_0P_1+h\Delta\phi-\int_{\phi_0}^{\phi_0+\delta\phi_0}(f_{\phi_0}(\eta)+h)d\eta+\int_{\phi_1}^{\phi_1+\delta\phi_1}(f_{\phi_0}(\eta)+h)d\eta \\ &= 
        \widearc{P_0 P_1} + \delta \bar s \cos(\theta_0) \Delta \phi -\delta \bar s \sin(\theta_0) + r_{\bar s}(P_1) \delta \phi_1,
    \end{align*}
where we have used \eqref{eq:delta:phi:0}, %Moreover, 

    \begin{align*}
       \big| P_2 + \delta P_2 - (\tilde P_1 + \delta P_1) \big| &= |P_2 - P_1| - r_{\bar s}(P_1) \delta \phi_1 + \big( \delta \bar s \cos(\theta_0) - |P_2 -P_1| \delta \phi_1 \big) \cot(\bar \alpha) + \frac{r_{\bar s}(P_2)}{\sin(\bar \alpha)} \delta \phi_1 \\
       &= |P_2 - P_1| + \delta \bar s \cos(\theta_0) \cot(\bar \alpha) + \left( \frac{r_{\bar s}(P_2)}{\sin(\bar \alpha)} - r_{\bar s}(P_1) - |P_2 - P_1| \cot(\bar \alpha) \right) \delta \phi_1, 
    \end{align*}
%and 
    \begin{align*}
        |P_2 + \delta P_2 - O_2| &= |P_2 - O_2| + \frac{\delta \bar s \cos(\theta_0) - |P_2 - P_1| \delta \phi_1}{\sin(\bar \alpha)} + r_{\phi_0}(P_2) \delta \phi_1 \cot(\bar \alpha).
    \end{align*}
Subtracting equation \eqref{eq:sat:1} to equation \eqref{eq:sat:2} we get
    \begin{align*}
        &\frac{\delta \bar s - |P_2 - P_1| \delta \phi_1}{\sin(\bar \alpha)} + r_{\phi_0}(P_2) \delta \phi_1 \cot(\bar \alpha) - \cos(\bar \alpha) \big( \delta \bar s \cos(\theta_0) \Delta \phi - \delta \bar s \sin(\theta_0) + r_{\phi_0}(P_1) \delta \phi_1 \big) \\
        & \qquad - \cos(\bar \alpha) \left( - r_{\phi_0}(P_1) \delta \phi_1 + \big( \delta \bar s \cos(\theta_0) - |P_2 - P_1| \delta \phi_1 \big) \cot(\bar \alpha) + \frac{r_{\phi_0}(P_2)}{\sin(\bar \alpha)} \delta \phi_1 \right) - \cos(\hat \alpha) \delta \bar s = 0,
    \end{align*}
obtaining %    that is, expliciting $\delta\phi_1$ we obtain
    \begin{align}
    \label{eq:delta:phi:1}
        \delta \phi_1 %&= \frac{\delta \bar s \cos(\theta_0)}{|P_2 - P_1|} \left( 1 - \cot(\bar \alpha) \Delta \phi + \cot(\bar \alpha) \tan \theta_0 - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \frac{1}{\cos(\theta_0)} \right) \\
        &= \frac{\delta \bar s}{|P_2-P_1|} \left( \cos(\theta_0) - \cot(\bar \alpha) \Delta \phi \cos(\theta_0) + \cot(\bar \alpha) \sin(\theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \right).
    \end{align}
    Moreover, 
\begin{equation}
\label{Equa:delta|P2-P1|}
\begin{split}
\delta \big| P_2 - P_1| &= \left( \frac{r(\phi_2)}{\sin(\bar \alpha)} - r(\phi_1) + \cot(\bar \alpha) |P_2 - P_1|  \right) \delta \phi_1 + \big( \delta s_0 \cos(\theta_0) - 2 |P_2 - P_1| \delta \phi_1) \cot(\bar \alpha) \\%\bigg( \cos(\theta_0) - \cot(\bar \alpha) \Delta \phi \cos(\theta_0) + \cot(\bar \alpha) \sin(\theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \bigg) \right) \cot(\bar \alpha) \\
&= \bigg( \frac{r(\phi_2)}{\sin(\bar \alpha)} - r(\phi_1) + |P_2 - P_1| \cot(\bar \alpha) \bigg) \delta \phi_1 \\
& \quad +  \delta s_0  \left( \big( 2 \Delta \phi \cot(\bar \alpha) - 1 \big) \cos(\theta_0) + 2 \cot(\alpha)  \left( \frac{\cos(\hat \alpha)}{\cos(\bar \alpha)} - \sin(\theta_0) \right) \right) \cot(\bar \alpha),
\end{split}
\end{equation}
and the variation of the angle of the level set arc is then 
       \begin{equation}
\label{Equa:delta_Delta_phi}
\begin{split}
\delta \Delta \phi &= \delta\phi_1-\delta\phi_0 \\
&= \frac{\delta \bar s}{|P_2-P_1|} \left( \cos(\theta_0) - \cot(\bar \alpha) \Delta \phi \cos(\theta_0) + \cot(\bar \alpha) \sin(\theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} - \frac{|P_2-P_1|}{r(P_0)} \sin(\theta_0) \right).
\end{split}
       \end{equation}
The variation $\delta P(\phi)$ along the segment $[P_1,P_2]$ can be computed as %Call $P(\phi)$ any point on the segment, with $P(\phi_1)=P_1$ and $P(\phi_2)=P_2$. Then we recover that, for any $\phi$, $\phi+t=\phi_1+\frac{\pi}{2}$.
   \begin{align*}
       \delta P(\phi) &= \big( \delta \bar s \cos(\theta_0) - |P(\phi)-P_1| \delta \phi_1 \big) \mathbf{n}(P_1) \\ &+ \left( \big( \delta \bar s \cos(\theta_0) -|P(\phi) - P_1| \delta \phi_1 \big) \tan(\phi - \phi_1) + \frac{r_{\phi_0}(P(\phi))}{\cos(\phi - \phi_1)} \delta \phi_1 \right) \mathbf{t}(P_1),
   \end{align*}
with $\phi \in (\phi_1,\phi_2)$.
%   and recall that
%   \begin{equation}
%       \textbf{n}(P(\phi))=\cos(\phi-\phi_1)\textbf{n}(P_1)+\sin(\phi-\phi_1)\textbf{t}(P_1).
%   \end{equation}
Finally, we obtain an initial data for the perturbation $\delta r_{\bar s}$ given by %if we call $\tilde f_{\phi_0}$ the element of the family of generalized barrier which is a perturbation of $f_{\phi_0}$ we find that:  $\tilde{f}_{\phi_0}-f_{\phi_0}(\phi)=\delta r (\phi)$ with 
  \begin{equation*}
      \delta r(\phi) = \begin{cases}
      0 & \phi < \phi_0, \\
          \frac{\delta \bar s \cos(\theta_0)}{\delta \phi_0}(\phi-\phi_0) & \phi_0 \leq \phi < \phi_0 + \delta \phi_0, \\
          \delta \bar s \cos(\theta_0) & \phi_0 + \delta \phi_0 \leq \phi < \phi_1 + \delta \phi_1, \\
          \frac{\delta \bar s \cos(\theta_0) - |P(\phi) - P_1| \delta \phi_1}{\cos(\phi - \phi_1)} & \phi_1 + \delta \phi_1 \leq \phi < \phi_2 + \delta \phi_2.
      \end{cases}
  \end{equation*}
The derivative $\bar r_{\bar s}$ has the initial data below 
  \begin{equation}\label{eq:initial:data}
     \bar r_{\bar s}(\phi) = \begin{cases}
     0 & \phi < \phi_0, \\
     \cos(\theta_0) & \phi_0 \leq \phi < \phi_0 + \Delta \phi = \phi_1, \\
    \frac{\cos(\theta_0) - \frac{|P(\phi) - P_1|}{|P_2 - P_1|} \left( \cos(\theta_0) - \cot(\bar \alpha) \Delta \phi \cos(\theta_0) + \cot(\bar \alpha) \sin(\theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \right)}{\cos(\phi - \phi_1)}, & \phi_1 \leq \phi < \phi_2 = \phi_1 + \frac{\pi}{2} - \bar \alpha.
      \end{cases}
  \end{equation}
%In particular to get $\bar f_{\phi_0}$ we need simply to multiply $\cos\theta_0 \bar g_{\phi_0}(\phi).$

\begin{remark}
    With reference to Remark \ref{rmk:cases:1:2}, formula \eqref{eq:initial:data} tells us that for $\phi \in [\phi_0,\phi_2]$ the derivative $\bar r_{\bar s}$ is positive. The only computation to check is indeed
    \begin{equation*}
        \frac{1 - \frac{|P(\phi) - P_1|}{|P_2 - P_1|} \left(1 - \cot(\bar \alpha) \Delta \phi + \cot(\bar \alpha) \tan(\theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \frac{1}{\cos(\theta_0)} \right)}{\cos(\phi - \phi_1)} \geq 0, \qquad \phi_1 \leq \phi < \phi_2 = \phi_1 + \frac{\pi}{2} - \bar \alpha.
    \end{equation*}
    This follows by observing that
    \begin{align*}
        &\frac{1 - \frac{|P(\phi) - P_1|}{|P_2 - P_1|} \left( 1 - \cot(\bar \alpha) \Delta \phi + \cot(\bar \alpha) \tan(\theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \frac{1}{\cos(\theta_0)} \right)}{\cos(\phi - \phi_1)} \\
        & \qquad \geq \frac{1 - \frac{|P_2-P_1|}{|P_2-P_1|} \left( 1 - \cot(\bar \alpha) \Delta \phi + \cot(\bar \alpha) \tan(\theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \frac{1}{\cos(\theta_0)} \right)}{\cos(\phi - \phi_1)} \\ 
        & \qquad = \frac{\cot(\bar \alpha) \Delta \phi - \cot(\bar \alpha) \tan(\theta_0) + \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \frac{1}{\cos(\theta_0)}}{\cos(\phi - \phi_1)} \\
        & \qquad \geq \frac{\cot(\bar \alpha) \Delta \phi - \cot(\bar \alpha) \tan(\theta_0) + \cot(\bar \alpha) \frac{1}{\cos(\theta_0)}}{\cos(\phi - \phi_1)} \\
        & \qquad \geq \cot(\bar \alpha) \Delta \phi \geq 0,
    \end{align*}
    where we have used the inequality
    \begin{equation*}
        \cos(\hat \alpha) \geq \cos(\bar \alpha).
    \end{equation*}
\end{remark}
The variation $\delta P(\phi)$ along the segment $[P_1,P_2]$ can be computed as %Call $P(\phi)$ any point on the segment, with $P(\phi_1)=P_1$ and $P(\phi_2)=P_2$. Then we recover that, for any $\phi$, $\phi+t=\phi_1+\frac{\pi}{2}$.
   \begin{align*}
       \delta P(\phi) &= \big( \delta \bar s \cos(\theta_0) - |P(\phi)-P_1| \delta \phi_1 \big) \mathbf{n}(P_1) \\ &+ \left( \big( \delta \bar s \cos(\theta_0) -|P(\phi) - P_1| \delta \phi_1 \big) \tan(\phi - \phi_1) + \frac{r_{\phi_0}(P(\phi))}{\cos(\phi - \phi_1)} \delta \phi_1 \right) \mathbf{t}(P_1),
   \end{align*}
with $\phi \in (\phi_1,\phi_2)$.
%   and recall that
%   \begin{equation}
%       \textbf{n}(P(\phi))=\cos(\phi-\phi_1)\textbf{n}(P_1)+\sin(\phi-\phi_1)\textbf{t}(P_1).
%   \end{equation}
Finally, we obtain an initial data for the perturbation $\delta r_{\bar s}$ given by %if we call $\tilde f_{\phi_0}$ the element of the family of generalized barrier which is a perturbation of $f_{\phi_0}$ we find that:  $\tilde{f}_{\phi_0}-f_{\phi_0}(\phi)=\delta r (\phi)$ with 
  \begin{equation*}
      \delta r(\phi) = \begin{cases}
      0 & \phi < \phi_0, \\
          \frac{\delta \bar s \cos(\theta_0)}{\delta \phi_0}(\phi-\phi_0) & \phi_0 \leq \phi < \phi_0 + \delta \phi_0, \\
          \delta \bar s \cos(\theta_0) & \phi_0 + \delta \phi_0 \leq \phi < \phi_1 + \delta \phi_1, \\
          \frac{\delta \bar s \cos(\theta_0) - |P(\phi) - P_1| \delta \phi_1}{\cos(\phi - \phi_1)} & \phi_1 + \delta \phi_1 \leq \phi < \phi_2 + \delta \phi_2.
      \end{cases}
  \end{equation*}
The derivative $\bar r_{\bar s}$ has the initial data below 
  \begin{equation}\label{eq:initial:data}
     \bar r_{\bar s}(\phi) = \begin{cases}
     0 & \phi < \phi_0, \\
     \cos(\theta_0) & \phi_0 \leq \phi < \phi_0 + \Delta \phi = \phi_1, \\
    \frac{\cos(\theta_0) - \frac{|P(\phi) - P_1|}{|P_2 - P_1|} \left( \cos(\theta_0) - \cot(\bar \alpha) \Delta \phi \cos(\theta_0) + \cot(\bar \alpha) \sin(\theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \right)}{\cos(\phi - \phi_1)}, & \phi_1 \leq \phi < \phi_2 = \phi_1 + \frac{\pi}{2} - \bar \alpha.
      \end{cases}
  \end{equation}
%In particular to get $\bar f_{\phi_0}$ we need simply to multiply $\cos\theta_0 \bar g_{\phi_0}(\phi).$

\begin{remark}
    With reference to Remark \ref{rmk:cases:1:2}, formula \eqref{eq:initial:data} tells us that for $\phi \in [\phi_0,\phi_2]$ the derivative $\bar r_{\bar s}$ is positive. The only computation to check is indeed
    \begin{equation*}
        \frac{1 - \frac{|P(\phi) - P_1|}{|P_2 - P_1|} \left(1 - \cot(\bar \alpha) \Delta \phi + \cot(\bar \alpha) \tan(\theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \frac{1}{\cos(\theta_0)} \right)}{\cos(\phi - \phi_1)} \geq 0, \qquad \phi_1 \leq \phi < \phi_2 = \phi_1 + \frac{\pi}{2} - \bar \alpha.
    \end{equation*}
    This follows by observing that
    \begin{align*}
        &\frac{1 - \frac{|P(\phi) - P_1|}{|P_2 - P_1|} \left( 1 - \cot(\bar \alpha) \Delta \phi + \cot(\bar \alpha) \tan(\theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \frac{1}{\cos(\theta_0)} \right)}{\cos(\phi - \phi_1)} \\
        & \qquad \geq \frac{1 - \frac{|P_2-P_1|}{|P_2-P_1|} \left( 1 - \cot(\bar \alpha) \Delta \phi + \cot(\bar \alpha) \tan(\theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \frac{1}{\cos(\theta_0)} \right)}{\cos(\phi - \phi_1)} \\ 
        & \qquad = \frac{\cot(\bar \alpha) \Delta \phi - \cot(\bar \alpha) \tan(\theta_0) + \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \frac{1}{\cos(\theta_0)}}{\cos(\phi - \phi_1)} \\
        & \qquad \geq \frac{\cot(\bar \alpha) \Delta \phi - \cot(\bar \alpha) \tan(\theta_0) + \cot(\bar \alpha) \frac{1}{\cos(\theta_0)}}{\cos(\phi - \phi_1)} \\
        & \qquad \geq \cot(\bar \alpha) \Delta \phi \geq 0,
    \end{align*}
    where we have used the inequality
    \begin{equation*}
        \cos(\hat \alpha) \geq \cos(\bar \alpha).
    \end{equation*}
\end{remark}
Finally, we obtain an initial data for the perturbation $\delta r_{\bar s}$ given by %if we call $\tilde f_{\phi_0}$ the element of the family of generalized barrier which is a perturbation of $f_{\phi_0}$ we find that:  $\tilde{f}_{\phi_0}-f_{\phi_0}(\phi)=\delta r (\phi)$ with 
  \begin{equation*}
      \delta r(\phi) = \begin{cases}
      0 & \phi < \phi_0, \\
          \frac{\delta \bar s \cos(\theta_0)}{\delta \phi_0}(\phi-\phi_0) & \phi_0 \leq \phi < \phi_0 + \delta \phi_0, \\
          \delta \bar s \cos(\theta_0) & \phi_0 + \delta \phi_0 \leq \phi < \phi_1 + \delta \phi_1, \\
          \frac{\delta \bar s \cos(\theta_0) - |P(\phi) - P_1| \delta \phi_1}{\cos(\phi - \phi_1)} & \phi_1 + \delta \phi_1 \leq \phi < \phi_2 + \delta \phi_2.
      \end{cases}
  \end{equation*}
The derivative $\bar r_{\bar s}$ has the initial data below 
  \begin{equation}\label{eq:initial:data}
     \bar r_{\bar s}(\phi) = \begin{cases}
     0 & \phi < \phi_0, \\
     \cos(\theta_0) & \phi_0 \leq \phi < \phi_0 + \Delta \phi = \phi_1, \\
    \frac{\cos(\theta_0) - \frac{|P(\phi) - P_1|}{|P_2 - P_1|} \left( \cos(\theta_0) - \cot(\bar \alpha) \Delta \phi \cos(\theta_0) + \cot(\bar \alpha) \sin(\theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \right)}{\cos(\phi - \phi_1)}, & \phi_1 \leq \phi < \phi_2 = \phi_1 + \frac{\pi}{2} - \bar \alpha.
      \end{cases}
  \end{equation}
%In particular to get $\bar f_{\phi_0}$ we need simply to multiply $\cos\theta_0 \bar g_{\phi_0}(\phi).$
\subsubsection{Analysis of the derivative (arc case)}
\label{ss:analysis:arc}


In this subsection we analyze the initial data obtained in the previous section. The initial data is given by \eqref{eq:initial:data}, namely
\begin{equation*}
    \bar r_{\bar s}(\phi) = \begin{cases}
    0 & \phi \leq \phi_0, \\
    \cos(\theta_0) & \phi_0 \leq \phi < \phi_0 + \Delta\phi = \phi_1, \\
    \frac{\cos(\theta_0) - \frac{|P(\phi) - P_1|}{|P_2 - P_1|} ( \cos(\theta_0) - \cot(\bar \alpha) \Delta \phi \cos(\theta_0) + \cot(\bar \alpha) \sin(\theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} )}{\cos(\phi - \phi_1)} & \phi_1 \leq \phi < \phi_2 = \phi_1 + \frac{\pi}{2} -\bar \alpha.
\end{cases}
\end{equation*}
After the angle $\phi_2$, the generalized spiral satisfies the RDE of the saturated spirals with critical speed, namely $\beta(\phi) = \bar \alpha$. However we have still to compute the derivative of the curvature term $D s^-(\phi)$ for the second round, after which the RDE of the saturated spiral becomes linear with constant coefficients. We will also compute the solution, which will be needed for evaluating Lemma \ref{lem:key}.

%      Since after the point $P_2$ it is a saturated spiral, by linearity we can compute the RDE that the derivative $\bar g_{\phi_0}$ satisfies.
%      In this subsection we study precisely the RDE satisfied by the derivative $\bar g_{\phi_0}$ in the arc case. 
%
%      \medskip
%      
      %It holds:
      \begin{comment}

\subsubsection{Origin case.}\label{sss:origin}
   In the case of the fire burning from $B_1(0)$ and the spiral starting at $(r,0)$ (corresponding to the element $f_0$ of the family) (no barrier from which the fire rays $\bar\gamma_{P_i}$ depart) the relation for $\Delta\phi$ is
   \begin{equation}
       \Delta\phi=\tan{\alpha}-\frac{1}{r\cos\alpha}\leq\tan\alpha,
   \end{equation}
   where $r$ is the distance of the spiral from the fire. Indeed here the admissibility at the saturated point (endpoint of the segment) reads as
   \begin{equation*}
       r\Delta\phi+r\cot\alpha=\sigma\left(\frac{r}{\sin\alpha}-1\right).
   \end{equation*}
   By the theorem of sines one can also compute
   \begin{equation*}
       \frac{|P(\phi)-P_1|}{|P_2-P_1|}=\tan\alpha\tan(\phi-\phi_1),
   \end{equation*}
   In particular in this case we have
   \begin{equation}
      \bar f_0(\phi)=\begin{cases}
          1 \qquad 0\leq\phi<\Delta\phi=\phi_1, \\
          \\
          \frac{1-\tan(\phi-\phi_1)\left(\frac{1}{r\cos\alpha}-\frac{1-\sin\theta_0}{\cos\theta_0}\right)}{\cos(\phi-\phi_1)},\qquad \phi_1\leq\phi<\phi_2=\phi_1+\frac{\pi}{2}-\alpha.
      \end{cases}
      \end{equation}
      \begin{remark}
      We remark that also in the general case with barriers we can do the assumption
          $\Delta\phi\leq\tan\alpha$, which represents the maximum amount of barrier one can put on a level set. 
      \end{remark}
\end{comment}

\begin{description}
    \item[$\phi \in [\phi_1+\frac{\pi}{2}-\bar\alpha, \phi_0
+2\pi+\theta_0)$] in this interval the function $s^-(\phi)$ is the one of the base spiral, so that it is canceled out when taking the derivative: hence %it holds
\begin{equation*}
    \frac{d \bar r_{\bar s}(\phi)}{d\phi} = \bar r_{\bar s}(\phi) \cot(\bar \alpha).
\end{equation*}
    In particular the solution is computed as
    \begin{equation}
    \label{eq:initial:data_equ}
        \bar r_{\bar s}(\phi) = \bar r_{\bar s}(\phi_2) %\left( \Delta \phi + \phi_0 + \frac{\pi}{2} - \bar\alpha \right)
        e^{\cot(\bar \alpha) (\phi - \phi_2)}, %(\Delta \phi+\phi_0+\frac{\pi}{2}-\bar\alpha))}.
    \end{equation}
%   We remark that $\bar g_{\phi_0}\left(\Delta\phi+\phi_0+\frac{\pi}{2}-\bar\alpha\right)$ can be easily computed: indeed it is
with
\begin{equation}
\label{eq:initial:data:Arc}
\bar r_{\bar s}(\phi_2) %= \left(\Delta\phi+\phi_0+\frac{\pi}{2}-\bar\alpha\right)
= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \left( \big( \Delta \phi \cos(\theta_0) - \sin(\theta_0) \big) + \frac{\cos(\hat \alpha)}{\cos(\bar \alpha)} \right). %\frac{1}{\cos\theta_0},
   \end{equation}
%   in particular we want to underline that there is no need for the  computation of the formula $|P(\phi)-P_1|$ here.
%   \medskip
   
\item[$\phi = \phi_0 + 2\pi + \theta_0$] the derivative $\bar r_{\bar s}$ has a downward jump, due to the fact that we are prolonging the base spiral of $\delta \bar s e^{i\theta_0}$, obtaining
   \begin{equation*}
       \bar r_{\bar s}(\phi_0 + 2\pi + \theta_0) - \bar r_{\bar s}(\phi_0 + 2\pi + \theta_0-) = - 1.
   \end{equation*}
   
\item[$\phi\in [\phi_0+2\pi+\theta_0,\phi_0+2\pi+\frac{\pi}{2})$] for these angles the base point of the optimal ray is the point $\zeta(\bar s)$, and then it holds
    \begin{equation*}
        \frac{d\bar r_{\bar s}(\phi)}{d\phi} = \bar r_{\bar s}(\phi) \cot(\bar \alpha).
    \end{equation*}
We compute the solution to be
%    In particular the solution reads as
    \begin{equation*}
        \bar r_{\bar s}(\phi) = \left( \bar r_{\bar s}(\phi_2) %\left(\Delta\phi+\phi_0+\frac{\pi}{2}-\bar\alpha\right)
        e^{\cot(\bar \alpha)(2\pi + \theta_0 - (\phi_2 - \phi_0)} - 1 \right) e^{\cot(\bar \alpha)(\phi - (\phi_0 + 2\pi + \theta_0))}.
    \end{equation*}
%    \medskip
    
\item[$\phi = \phi_0 + 2\pi + \frac{\pi}{2}$] there is an upward jump, due to the fact that the optimal ray ending in $r_{\bar s + \delta \bar s}(\phi)$ is still in the base point $\zeta(\bar s + \delta \bar s)$ while $r_{\bar s}$ has the term $- Ds^-$ in its RDE. The amount of length subtracted by this last term is
\begin{equation*}
    r(\phi_0) \delta \phi_0 = \delta \bar s \sin(\theta_0),
\end{equation*}
%$r_{\bar s + \delta \bar s}$ jump downward of a smaller amount than $r_{\bar s}$, because the segment $[P_1,P_2]$ becomes shorter: explicit computation gives
%   \begin{equation*}
%       \tilde r_{\bar_0} \left( 2\pi + \frac{\pi}{2} + \delta \phi_0 \right)=\tilde f_{\phi_0}\left(2\pi+\frac{\pi}{2}\right)\left(1+\frac{h\tan\theta_0}{r(P_0)}\cot\bar\alpha\right)+o(h).
%   \end{equation*}
%$$
%r_{\bar s} \left( 2\pi + \frac{\pi}{2} + \delta \phi_0 \right) - r_{\bar s} \left( 2\pi + \frac{\pi}{2} \right) + \frac{h\tan\theta_0}{r(P_0)}\left(f_{\phi_0}\left(2\pi+\frac{\pi}{2}\right)\cot\bar\alpha-r(P_0)\right)+o(h),$$ while
% and the that is
and then
   \begin{equation}
   \label{Equa:jump_init_cirle}
       \bar r_{\bar s} \bigg( \phi_0 + 2\pi + \frac{\pi}{2} \bigg) - \bar r_{\bar s} \bigg( \phi_0 + 2\pi + \frac{\pi}{2} - \bigg) = \sin(\theta_0).
   \end{equation}
%   Indeed
%      \medskip
   
\item[$\phi \in [\phi_0 + 2\pi + \frac{\pi}{2}, \phi_0 + 2\pi + \frac{\pi}{2} +\Delta \phi)$] the difference $Ds^-(\phi)$ in this interval is $\delta \bar s \cos(\theta_0)$ by \eqref{eq:initial:data}, and then
%
%it holds
    \begin{equation*}
        \frac{d\bar r_{\bar s}(\phi)}{d\phi} = \bar r_{\bar s}(\phi) \cot(\bar \alpha) - \cos(\theta_0).
    \end{equation*}
We compute the solution as
    \begin{align*}
        \bar r_{\bar s}(\phi) &= \left[ \left( \bar r_{\phi_0}(\phi_2) %\left( \Delta \phi + \phi_0 + \frac{\pi}{2} - \bar \alpha \right) 
        e^{\cot(\bar \alpha) (2\pi + \theta_0 - (\phi_2 - \phi_0))} - 1 \right) e^{\cot(\bar \alpha) (\frac{\pi}{2} - \theta_0)} + \sin(\theta_0) \right] e^{\cot(\bar \alpha) (\phi - (\phi_0 + 2\pi + \frac{\pi}{2}))} \\
        & \quad - \tan(\bar \alpha) \big( e^{\cot(\bar \alpha) (\phi - (\phi_0 +2\pi + \frac{\pi}{2}))} - 1 \big).
    \end{align*}
%    \medskip
    
\item[$\phi = \phi_0 + 2\pi + \frac{\pi}{2} + \Delta \phi$] there is a downward jump, due to the difference in size of the downward jumps of $r_{\bar s}$ and $r_{\bar s + \delta \bar s}$ and the different angles to which this jump happens. We compute up to higher order infinitesimal: for $\epsilon \ll 1$ we can approximate the solutions as
   \begin{align*}
      r_{\bar s} \left( \phi_0 + \Delta \phi + \frac{\pi}{2} + 2\pi + \epsilon \right) &= \left( r_{\bar s} \left( \phi_0 + \Delta \phi + \frac{\pi}{2} + 2\pi - \epsilon \right)(1 + \cot(\bar \alpha) \epsilon) - r_{\bar s}(P_1) \epsilon - |P_2 - P_1| \right) (1 + \cot(\bar \alpha) \epsilon) %\\
      %& \quad %+ \left( r_{\bar s} \left( \phi_0 + \Delta \phi + \frac{\pi}{2} + 2\pi - \right) - |P_2 - P_1| \right) \cot(\bar \alpha) \delta \phi_1 
      - \frac{r_{\bar s}(\phi_2)}{\sin(\bar \alpha)} \epsilon,
   \end{align*}

%while 
    \begin{align*}
       r_{\bar s + \delta \bar s}& \left( \phi_0 + \Delta \phi + \frac{\pi}{2} + 2 \pi + \epsilon \right) \\
       &= \left[ r_{\bar s + \delta \bar s} \left( \phi_0 + \Delta \phi + \frac{\pi}{2} + 2 \pi - \epsilon \right) \big( 1 + \cot(\bar \alpha) (\epsilon + \delta \phi_1) \big) - r_{\bar s + \delta \bar s}(P_1) (\epsilon + \delta \phi_1) - |\tilde P_2 - \tilde P_1| \right] \big( 1 + \cot(\bar \alpha) (\epsilon - \delta \phi_1) \big) \\
       & \quad %+ \left( \tilde f_{\phi_0}\left(\Delta\phi+\frac{\pi}{2}+2\pi\right)-|\tilde P_2-\tilde P_1|\right)\cot\bar\alpha\delta\phi_1 
       - \frac{r_{\bar s + \delta \bar s}(P_2)}{\sin(\bar \alpha)} (\epsilon - \delta \phi_1).  %- |P_2 + \delta P_2 - P_1 - \delta P_1|,
   \end{align*}
Taking the difference and passing to the limit we obtain up to second order terms
%that is
   \begin{align*}
       \bar r_{\bar s} \left( \phi_0 + 2\pi + \frac{\pi}{2} + \Delta \phi + \epsilon \right) &= \bar r_{\bar s} \left( \phi_0 + 2\pi + \frac{\pi}{2} + \Delta \phi - \epsilon \right) (1 + 2 \cot(\bar \alpha) \epsilon) - \bar r_{\bar s}(P_1) \epsilon (1 + \cot(\bar \alpha) \epsilon) - r_{\bar s}(P_1) \delta \phi_1 (1 + \cot(\bar \alpha) \epsilon) \\
       & \quad - \delta |P_2 - P_1| (1 + \cot(\bar \alpha) \epsilon) + |P_2 - P_1| \cot(\bar \alpha) \delta \phi_1 - \frac{\bar r_{\bar s}(P_2)}{\sin(\bar \alpha)} \epsilon + \frac{r_{\bar s}(P_2)}{\sin(\bar \alpha)} \delta \phi_1.
   \end{align*}
The jump is then by \eqref{Equa:delta|P2-P1|}
\begin{equation}
\label{Equa:J_jump_speriamo_bene}
    \begin{split}
        &\left( \frac{r_{\bar s}(P_2)}{\sin(\bar \alpha)} - r_{\bar s}(P_1) + \cot(\bar \alpha) |P_2 - P_1|  \right) \delta \phi_1 - \delta |P_2 - P_1| \\
        & \qquad = - \left( \big( 2 \Delta \phi \cot(\bar \alpha) - 1 \big) \cos(\theta_0) + 2 \cot(\bar \alpha) \left( \frac{\cos(\hat \alpha)}{\cos(\bar \alpha)} - \sin(\theta_0) \right) \right) \cot(\bar \alpha) = \hat r_{\bar s}.
    \end{split}
\end{equation}


%   \medskip
   
\item[$\phi \geq \phi_0 + \Delta \phi + 2\pi + \frac{\pi}{2}$] the function $\bar r_{\bar s}$ satisfies:
    \begin{equation*}
        \frac{d\bar r_{\bar s}}{d\phi} = \cot(\bar \alpha) \bar r_{\bar s}(\phi) - \frac{\bar r_{\bar s}(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)}.
    \end{equation*}
\end{description}

%We compute then the same quantities for $\bar f_{\phi_0}=\cos\theta_0\bar g_{\phi_0}$ (the derivative with respect to the length parameter $s$).


==> segment.tex <==

\subsection{Segment-segment case}
\label{Ss:segment_case}


In the following subsections, we analyze the cases of the first grid {\color{red} non so come mettere il label alla griglia}, where the assumption is that in the point $\phi_0$ the fastest saturated spiral starts with a tent, and that at the end point $\check P^-$ of the segment $\check P_0 + \ell_0 e^{\i \bar \phi}$ the fastest closing spiral is a segment. Depending on the relative position of $\phi_0$ and $\bar \phi$, $e$ cases can happen: we will study them in the next subsections.

We recall that the angle $\bar \theta$ is the angle formed by the initial segment $[P_1,P_2]$ of the fastest saturated spiral.


\subsubsection{Segment-segment with $\bar \phi \in \phi_0 + [\beta^-(\phi_0),2\pi + \bar \theta - \hat \theta]$}
\label{Sss:segm-segm_low}


In this case $\hat r(\phi;s_0) = \tilde r(\phi;s_0)$, because the derivative $\delta r(\phi;s_0) \geq 0$: indeed $\bar \phi$ is outside the region of negativity $\gls{Nsegm}$. This fact gives then

\begin{lemma}
\label{Lem:segm_segm_1_case}
If $\bar \phi \in \phi_0 + [\beta^-(\phi_0),2\pi + \bar \theta - \hat \theta]$ and $\tilde r = \check r$ is in the segment case, any non-null perturbation of the optimal solution is strictly positive at $\bar \phi$.
\end{lemma}

For a drawing of the geometric situation see Fig. \ref{Fig:segm_arc_1}.

\begin{figure}
%\begin{subfigure}{.475\textwidth}
\resizebox{.75\textwidth}{!}{\input{segm_arc_1.pdf_t}}
\caption{The geometric situation of Section \ref{Sss:segm_arc_1}: being $\bar \phi - 2\pi - \phi_0 - \bar \theta > \hat \theta$, $\hat r = \tilde r$ and the derivative is $\leq 0$.}
%\end{subfigure}
%\hfill
%\begin{subfigure}{.475\textwidth}
%\resizebox{\textwidth}{!}{\input{segm_arc_2.pdf_t}}
%\caption{The geometric situation of Section \ref{Sss:segm_arc_2}.}
%\label{Fig:segm_arc_2}
%\end{subfigure}
%\resizebox{.75\textwidth}{!}{\input{segm_arc_1.pdf_t}}
%\caption{The geometric situation of Section \ref{Sss:segm_arc_1}: being $\bar \phi - 2\pi - \phi_0 - \bar \theta > \hat \theta$, $\hat r = \tilde r$ and the derivative is $\leq 0$.}
\label{Fig:segm_arc_1}
\end{figure}


\subsubsection{Segment-segment with $\bar \phi \in \phi_0 + 2\pi + (\bar \theta-\hat \theta,\bar \theta)$}
\label{Sss:segm_semg_neg}


This situation occurs when $\bar \phi$ is inside the negative region $\gls{Nsegm}$: it is thus more convenient to take an initial segment in the direction $\bar \phi$, because the derivative is negative.

The spiral $\check \zeta$, corresponding to $\check r(\phi;s_0)$, is thus made of a segment $[P_0 = P_1 = \check P_0, \check P^- = \check P_1]$ and a second segment $[\check P_1,\check P_2]$, forming an angle equal to the critical value $\hat \theta$. The assumptions enter here because the second segment corresponds to the fastest saturated spiral starting in $\check P_1$.

In order to prove that this is the optimal solution, we compute the derivative w.r.t. an initial perturbation.

First of all, if $\phi_0 + \beta^+(\phi_0) + 2\pi > \bar \phi$, we are not in the optimal solution: indeed this would imply that $\delta r(\phi;s_0) > 0$. Hence the situation of the perturbation $\delta \check r(\phi;s_0)$ is in Fig. \ref{Fig:segm_segm_2_case}.

\begin{figure}
\resizebox{.75\textwidth}{!}{\input{segm_segm_2_case.pdf_t}}
\caption{The perturbation of the optimal solution $\check r$ for the case of Section \ref{Sss:segm_semg_neg}. In blue the fastest saturated solution $\tilde r$ is represented, while $\check r$ is in red. While $\delta \tilde r(\bar \phi;s_0) < 0$ (variation of the distance of the final point from $P_0$), it holds $\delta \check r(\phi;s_0) \geq 0$ (variation of the distance from $\check P^-$), giving the optimality in this case. It is also represented the angle $\theta$ (magenta), formed by the direction of the perturbation and $\bar \phi$.}
\label{Fig:segm_segm_2_case}
\end{figure}

%In the reference frame where $e^{\i \bar \phi} = (1,0)$, t
The variations are
\begin{equation*}
\delta \check P_0 = \delta s_0 e^{\i (\bar \phi - \theta)}, \quad \theta = \bar \phi - 2\pi - \theta_0,
\end{equation*}
\begin{equation*}
\delta \check P_1 = \delta \check P_0 + \delta \ell_0 e^{\i \bar \phi} = \delta s_0 e^{\i (\bar \phi - \theta)} + \delta \ell_0 e^{\i \bar \phi},
\end{equation*}
\begin{equation*}
\delta \check P_2 = \delta \check P_1 + \delta \ell_1 e^{\i (\bar \phi + \hat \theta)} = \delta s_0 e^{\i (\bar \phi - \theta)} + \delta \ell_0 e^{\i \bar \phi} + \delta \ell_1 e^{\i (\bar \phi + \hat \theta)},
\end{equation*}
where we recall that %have denoted by
\begin{equation*}
\ell_0 = |\check P_1 - \check P_0|, \quad \ell_1 = |\check P_2 - \check P_1|.
\end{equation*}
%(see Equation \eqref{eq:sec6:imp} and hereafter).
The vector relation among the above quantities is
\begin{equation*}
\delta \check r_2(\bar \phi - 2\pi - \bar \alpha + \hat \theta) e^{\i (\hat \theta - \bar \alpha)} = \delta \check P_2,
\end{equation*}
because the angle of the optimal ray with $\check \zeta$ at $\check P_2$ is constant to $\alpha$ by construction, see Fig. \ref{Fig:segm_segm_2_case}).

Projecting the above equation one obtains
\begin{align*}
0 &= e^{\i (\bar \phi + \frac{\pi}{2} + \hat \theta - \bar \alpha)} \cdot \delta \check P_2 \\
&= \delta s_0 \sin(\bar \alpha - \hat \theta - \theta) + \delta \ell_0 \sin(\bar \alpha - \hat \theta) + \delta \ell_1 \sin(\bar \alpha), 
\end{align*}
\begin{align*}
\delta \check r_2 = \delta \check P_2 \cdot e^{\i (\hat \theta - \bar \alpha)} &= \delta s_0 \cos(\bar \alpha - \hat \theta - \theta) + \delta \ell_0 \cos(\bar \alpha - \hat \theta) + \delta \ell_1 \cos(\bar \alpha) \\
&= \delta s_0 \frac{\sin(\hat \theta + \theta)}{\sin(\bar \alpha)} + \delta \ell_0 \frac{\sin(\hat \theta)}{\sin(\bar \alpha)},
\end{align*}
where we have used the first projection to replace $\delta \ell_1$.

The saturation condition at the point $\check P_2 + \delta \check P_2$ gives
\begin{align*}
0 &= \delta \check r_2 - \cos(\bar \alpha) \big( \delta s_0 + \delta \ell_0 + \delta \ell_1 \big) \\
&= \delta s_0 \big( \cos(\bar \alpha - \hat \theta - \theta) - \cos(\bar \alpha) \big) + \delta \ell_0 ( \cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)),
\end{align*}
so that
\begin{equation*}
\delta \ell_0 = - \delta s_0 \frac{\cos(\bar \alpha - \hat \theta - \theta) - \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
\begin{align*}
\delta \check r_2 &= \delta s_0 \frac{\sin(\hat \theta + \theta) (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)) - \sin(\hat \theta) (\cos(\bar \alpha - \hat \theta - \theta) - \cos(\bar \alpha))}{\sin(\bar \alpha) (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha))} \\
&= \delta s_0 \frac{\cot(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \big( \sin(\theta) (1 - \cos(\hat \theta)) + (1 - \cos(\theta)) \sin(\hat \theta) \big).
\end{align*}

As in Corollary \ref{Cor:equation}, the ODE for the perturbation gives where divided by $\delta s_0$
\begin{equation*}
\delta r(\bar \phi - \theta -) = e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta - \theta)} \delta \check r_2,
\end{equation*}
\begin{equation*}
\delta \check r(\bar \phi -) = e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} \delta \check r_2 - e^{\cot(\bar \alpha) \theta},
\end{equation*}
and then the final value is computed as
\begin{align*}
\delta \check r(\bar \phi) &= \delta \check r_2 e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} - e^{\cot(\bar \alpha) \theta} - \delta \ell_0 \\
&= \frac{\cot(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \big( \sin(\theta) (1 - \cos(\hat \theta)) + (1 - \cos(\theta)) \sin(\hat \theta) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} - e^{\cot(\bar \alpha) \theta} + \frac{\cos(\bar \alpha - \hat \theta - \theta) - \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
&= \frac{1 - \cos(\hat \theta + \theta)}{1 - \cos(\hat \theta)} - e^{\cot(\bar \alpha) \theta},
\end{align*}
where we have used the definition of \gls{thetahat},
$$
\frac{\cot(\bar \alpha)}{\sin(\bar \alpha)}(1 - \cos(\hat \theta)) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} = 1.
$$

%{\color{red} come hai ottenuto l'ultima uguaglianza? non me la trovo proprio!}
%{\color{blue}
%$$
%\frac{\cot(\bar \alpha)}{\sin(\bar \alpha)}(1 - \cos(\hat \theta)) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} = 1?
%$$
%\begin{align*}
%    &\frac{\cot(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \big( \sin(\theta) (1 - \cos(\hat \theta)) + (1 - \cos(\theta)) \sin(\hat \theta) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} - e^{\cot(\bar \alpha) \theta} + \frac{\cos(\bar \alpha - \hat \theta - \theta) - \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
%    &= \frac{\sin(\bar \alpha) \sin(\theta) + \sin(\bar \alpha) \sin(\hat \theta) \frac{1 - \cos(\theta)}{1 - \cos(\hat \theta)} + \cos(\bar \alpha - \hat \theta - \theta) - \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - e^{\cot(\bar \alpha) \theta},
%\end{align*}
%e per il numeratore
%\begin{align*}
%    & \sin(\bar \alpha) \sin(\theta) (1 - \cos(\hat \theta) + \sin(\bar \alpha) \sin(\hat \theta) (1 - \cos(\theta)) + (1 - \cos(\hat \theta)) (\cos(\bar \alpha - \hat \theta - \theta) - \cos(\bar \alpha)) \\
%    &= \sin(\bar \alpha) (\sin(\theta) + \sin(\hat \theta)) - \sin(\bar \alpha) \sin(\theta + \hat \theta) + (1 - \cos(\hat \theta)) [\cos(\bar \alpha) \cos(\hat \theta + \theta) + \sin(\bar \alpha) \sin(\theta + \hat \theta) - \cos(\bar \alpha)] \\
%    &= \sin(\bar \alpha) (\sin(\theta) + \sin(\hat \theta)) + (1 - \cos(\hat \theta)) \cos(\bar \alpha) [\cos(\hat \theta + \theta) - 1] - \cos(\hat \theta) \sin(\bar \alpha) \sin(\theta + \hat \theta) \\
%    &= \sin(\bar \alpha) (\sin(\theta) + \sin(\hat \theta)) + (1 - \cos(\hat \theta)) \cos(\bar \alpha) [\cos(\hat \theta + \theta) - 1] - \cos(\hat \theta) \sin(\bar \alpha) [ \sin(\theta) \cos(\hat \theta) + \sin(\hat \theta) \cos(\theta) ] \\
%    &= \sin(\bar \alpha) (\sin(\theta) \sin(\hat \theta)^2 + \sin(\hat \theta) (1 - \cos(\theta) \cos(\hat \theta)) ) + (1 - \cos(\hat \theta)) \cos(\bar \alpha) [\cos(\hat \theta + \theta) - 1] \\
%    &= \sin(\bar \alpha) \sin(\hat \theta) (1 - \cos(\theta + \hat \theta)) + (1 - \cos(\hat \theta)) \cos(\bar \alpha) [\cos(\hat \theta + \theta) - 1] \\
%    &= (\sin(\bar \alpha) \sin(\hat \theta) - (1 - \cos(\hat \theta)) \cos(\bar \alpha)) [\cos(\hat \theta + \theta) - 1] \\
%    &= (1 - \cos(\hat \theta + \theta)) (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha))
%\end{align*}
%}

A numerical plot of
\begin{equation}
\label{Equa:segm_segm_2_final}
\theta \mapsto \frac{\delta \check r_2(\bar \phi)}{\theta} = \frac{1}{\theta} \bigg( \frac{1 - \cos(\hat \theta + \theta)}{1 - \cos(\hat \theta)} - e^{\cot(\bar \alpha) \theta} \bigg)
\end{equation}
is in Fig. \ref{Fig:segm_segm_case_2_final}: the function is strictly positive.

\begin{figure}
\resizebox{.75\textwidth}{!}{\includegraphics{segm_segm_case_2_final.png}}
\caption{Plot of the function (\ref{Equa:segm_segm_2_final}), whose minimal value is $3.45283$.}
\label{Fig:segm_segm_case_2_final}
\end{figure}

%At the first order near $\theta = 0$ this function is
%\begin{equation*}
%\frac{d\delta r(\bar \phi)}{d\theta} = \theta \bigg( \frac{\sin(\hat \theta)}{1 - \cos(\hat \theta)} - \cot(\bar \alpha) \bigg) + \mathcal O(\theta^2),
%\end{equation*}
%which is positive, and numerically $\frac{\delta r(\bar \phi)}{\theta}$ is positive increasing in the remaining part of the interval, remaining above $3.45283$.

We have proved the following result.

\begin{lemma}
\label{Lem:segm_segm_2_case}
If $\bar \phi \in \phi_0 + 2\pi + (\bar \theta-\hat \theta,\bar \theta)$, any non-null perturbation of the optimal solution is strictly positive at $\bar \phi$.
\end{lemma}

%The fact that $\delta \check r(\bar \phi) = 0$ only when $\theta = \hat \theta$ means exactly that the optimal solution si to follow the segment $\ell_0$, until we end in the situation of Section \ref{Sss:segm-segm_low}.

\begin{figure}
\begin{subfigure}{.475\textwidth}
\resizebox{\linewidth}{!}{\input{segm_segm_sat_1.pdf_t}}
\caption{The geometric situation of Section \ref{Sss:segm_semg_after_neg}.}
\label{Fig:segm_segm_sat_1}
\end{subfigure}
\hfill
\begin{subfigure}{.475\linewidth}
\resizebox{\linewidth}{!}{\input{segm_segm_sat_2.pdf_t}}
\caption{The geometric situation of Section \ref{Sss:segm_semg_after_neg_2}.}
\label{Fig:segm_segm_sat_2}
\end{subfigure}
\begin{subfigure}{.475\textwidth}
\resizebox{\linewidth}{!}{\input{segm_segm_sat_3.pdf_t}}
\caption{The geometric situation of Section \ref{Sss:segm_semg_after_neg_3}.}
\label{Fig:segm_segm_sat_3}
\end{subfigure}
\hfill
\begin{subfigure}{.475\linewidth}
\resizebox{\linewidth}{!}{\input{segm_segm_sat_4.pdf_t}}
\caption{The geometric situation of Section \ref{Sss:segm_semg_after_neg_4}.}
\label{Fig:segm_segm_sat_4}
\end{subfigure}
\begin{subfigure}{.475\textwidth}
\resizebox{\linewidth}{!}{\input{segm_segm_sat_5.pdf_t}}
\caption{The geometric situation of Section \ref{Sss:segm_semg_after_neg_5}.}
\label{Fig:segm_segm_sat_5}
\end{subfigure}
\hfill
\begin{subfigure}{.475\linewidth}
\resizebox{\linewidth}{!}{\input{segm_segm_sat_6.pdf_t}}
\caption{The geometric situation of Section \ref{Sss:segm_semg_after_neg_6}.}
\label{Fig:segm_segm_sat_6}
\end{subfigure}
\end{figure}


\subsubsection{Segment-segment with $\bar \phi \in \phi_0 + 2\pi + [\bar \theta,2\pi + \bar \alpha + \bar \theta - \hat \theta$: see Fig. \ref{Fig:segm_segm_sat_1}}
\label{Sss:segm_semg_after_neg}


In this case the full tent is constructed, so that we can use the formulas of Lemma \ref{Lem:relation_admissibility_tent} to compute the perturbation $\check r(\phi;s_0)$. In this case, we have that the base of the tent is not perturbed, so that we are in the situation of Fig. \ref{Fig:tent_comput_geo} with
\begin{equation*}
\hat \zeta = 0 \quad \text{because} \quad \check \phi_0 = \bar \theta - 2\pi - \bar \alpha \geq \bar \phi_0 + \bar \theta - \bar \alpha, \ \check \phi_1 = \check \phi_0 + \hat \theta \leq \phi_0 + 2\pi - \bar \theta - \theta.
\end{equation*}
The computations are thus explicit: from Lemma \ref{Lem:relation_admissibility_tent}
\begin{equation*}
\hat r_0 = \delta \tilde r(\check \phi_0;s_0),
\end{equation*}
\begin{equation*}
\hat \ell_0 = \frac{\hat r_0 (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
\begin{equation*}
\hat r_2 = \frac{\hat r_0 \sin(\bar \alpha + \hat \theta) + \hat \ell_0 \sin(\hat \theta)}{\sin(\bar \alpha)} \geq \delta \tilde r_2(\check \phi_1;s_0),
\end{equation*}
where in the last inequality we observe that the curve $\delta \hat \zeta = 0$ for the perturbations.

Thus, using the explicit expression of $\delta \tilde r$,
\begin{align*}
\delta \check r(\bar \phi;s_0) &= (\hat r_2 - \delta \tilde r(\check \phi_2;s_0)) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} + \delta \tilde r(\bar \phi;s_0) - \hat \ell_0 \\
&\geq \delta \tilde r(\bar \phi;s_0) - \delta \tilde r(\bar \phi - 2\pi - \bar \alpha;s_0) \frac{1 - \cos(\hat \theta)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)}.
\end{align*}
The above quantity is equal to $PT(\tau)$ of Equation \eqref{Equa:PT_tau} for $\tau \in [1,1+\tau1(\theta))$, which is positive by Proposition \ref{Prop:PT_tau_pos}.

We have proved the following result.

\begin{lemma}
\label{Lem:segm_segm_3_case}
If $\bar \phi \in \phi_0 + 2\pi + [\bar \theta,2\pi + \bar \alpha + \bar \theta - \hat \theta)$, any non-null perturbation of the optimal solution is strictly positive at $\bar \phi$.
\end{lemma}


\subsubsection{Segment-segment with $\check \phi_0 \leq \phi_0 + 2\pi + \bar \theta - \theta, \check \phi_1 \in \phi_0 + 2\pi + [\bar \theta - \theta,\bar \theta)$: see Fig. \ref{Fig:segm_segm_sat_2}}
\label{Sss:segm_semg_after_neg_2}


For these angles we have to use the formulas of Lemma \ref{Lem:relation_admissibility_tent}: %changing coordinates $\check \phi_0 \to 0$,
\begin{equation*}
\delta \hat Q_2 - \delta \hat Q_0 = e^{\i (\phi_0 + 2\pi + \bar \theta - \theta)} = e^{\i (\bar \phi - (2\pi + \bar \alpha))} e^{\i (\phi_0 + \bar \theta - \bar \alpha - \theta + 2 (2 \pi + \bar \alpha) - \bar \phi)} = e^{\i (\bar \phi - (2\pi + \bar \alpha))} e^{\i ((2 \pi + \bar \alpha)(2 - \bar \tau) - \theta)},
\end{equation*}
\begin{equation*}
\delta \hat L = 1, \quad \delta \hat r_0 = \delta \tilde r(\check \phi_0) = \rho(\check \tau_0) e^{\bar c (2\pi + \bar \alpha) \check \tau_0}.
\end{equation*}
In terms of $\check \tau_0$ the interval of interest is
\begin{equation*}
1 - \frac{\theta + \hat \theta}{2\pi + \bar \alpha} \leq \check \tau_0 < 1 - \frac{\max\{\theta,\hat \theta\}}{2\pi + \bar \alpha}.
\end{equation*}
In Fig. \ref{Fig:segm_tent_1} we numerically plot the function
\begin{equation}
\label{Equa:segm_tent_1}
\frac{1}{\theta^2} \delta \hat r(\bar \phi) e^{- \bar c (2\pi + \bar \alpha) \bar \tau} = \frac{e^{- \bar c (2\pi + \bar \alpha) \bar \tau}}{\theta^2} \big[ e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} (\delta \hat r(\check \phi_2) - \delta \tilde r(\check \phi_2)) + \delta \tilde r(\bar \phi) - \delta \hat \ell_0 \big],
\end{equation}
as a function of \newglossaryentry{taubar}{name=\ensuremath{\bar \tau},description={the value of $\tau$ corresponding to $\bar \phi$, $\bar \tau = \frac{\bar \phi - \phi_0 - \bar \theta + \bar \alpha}{2\pi + \bar \alpha}$}} $\gls{taubar} = \frac{\bar \phi - \phi_0 - \bar \theta + \bar \alpha}{2\pi + \bar \alpha}$. The function is strictly positive, with minimal value equal to $0.5466$ in $\theta = \frac{\pi}{2}, \tau = 2 - \frac{\frac{\pi}{2} + \hat \theta}{2\pi + \bar \alpha}$.

\begin{figure}
\resizebox{.75\textwidth}{!}{\includegraphics{segm_tent_1.png}}
\caption{Plot of the function \eqref{Equa:segm_tent_1}.}
\label{Fig:segm_tent_1}
\end{figure}

We thus have proved the following lemma.

\begin{lemma}
\label{Lem:segm_tent_1}
If $\check \phi_0 \leq \phi_0 + 2\pi + \bar \theta - \theta, \check \phi_2 \in \phi_0 + 2\pi + [\bar \theta - \theta,\bar \theta)$, then $\delta \hat r(\bar \phi) \geq 0$.
\end{lemma}

\begin{remark}
\label{Rem:more_regu}
Note that the asymptotic behavior $\delta \tilde r(\bar \phi) \simeq \theta$ as $\theta \to 0$ for these angles (see Fig. \ref{Fig:segm_round_2}) becomes now $\delta \hat r(\bar \phi) \simeq \theta^2$, showing that the tent has a regularizing effect on the dependence w.r.t. $\theta$.
\end{remark}


\subsubsection{Segment-segment with $\check \phi_0 \leq \phi_0 + 2\pi + \bar \theta - \theta, \check \phi_1 \geq \phi_0 + 2\pi + \bar \theta]$: see Fig. \ref{Fig:segm_segm_sat_3}}
\label{Sss:segm_semg_after_neg_3}


We have in this case
\begin{equation*}
\delta \hat Q_2 - \delta \hat Q_0 = \delta \tilde r(\check \phi_2 - 2\pi - \bar \alpha) e^{\i (\phi_0 + \bar \theta - \bar \alpha + (2\pi + \bar \alpha) (\tau - 2 + \hat \tau))} = \rho(\bar \tau - 2 + \hat \tau) e^{\bar c (2\pi + \bar \alpha) (\bar \tau - 2 + \hat \tau)} e^{\i(\phi_0 + \bar \theta - \bar \alpha + (2\pi + \bar \alpha) (\tau - 1))} e^{\i (\hat \theta - \bar \alpha)},
\end{equation*}
\begin{align*}
\delta \hat L %&= \delta s_0 + \Delta P' + \int_{\delta \phi_2}^\phi \frac{r'}{\sin(\bar \alpha)} - \Delta P - \int_0^\phi \frac{r}{\sin(\bar \alpha)} \\
&= 1 + \delta \Delta P - \frac{r(\phi_2)}{\sin(\bar \alpha)} \delta \phi_2 + \int_0^{(2\pi + \bar \alpha)(\tau - 2 + \hat \tau)} \frac{\delta \tilde r(\phi)}{\sin(\bar \alpha)} d\phi \\
\big[ (\ref{Equa:delta_P_2P_1_segm}) \big] \quad &= \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} + \int_0^{(2\pi + \bar \alpha)(\tau - 2 + \hat \tau)} \frac{\delta \tilde r(\phi)}{\sin(\bar \alpha)} d\phi,
\end{align*}
\begin{equation*}
\delta \hat r_0 = \rho(\bar \tau - 1) e^{\bar c (2\pi + \bar \alpha) (\bar \tau - 1)}.
\end{equation*}
In terms of $\check \tau_0$ the interval of interest is
\begin{equation*}
2 - \frac{\hat \theta}{2\pi + \bar \alpha} \leq \bar \tau < 2 - \frac{\theta}{2\pi + \bar \alpha}, \quad \theta < \hat \theta.
\end{equation*}
In Fig. \ref{Fig:segm_tent_2} we numerically plot the function
\begin{equation}
\label{Equa:segm_tent_2}
%\frac{\delta \hat r_2 - \delta \tilde r(\check \phi_2)}{\theta^2} % 
\delta \hat r(\bar \phi) e^{- \bar c (2\pi + \bar \alpha) \bar \tau} = \frac{e^{- \bar c (2\pi + \bar \alpha) \bar \tau}}{\theta^2} \big[ e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} (\delta \hat r(\check \phi_2) - \delta \tilde r(\check \phi_2)) + \delta \tilde r(\bar \phi) - \delta \hat \ell_0 \big],
\end{equation}
as a function of $\bar \tau$. The function is strictly positive $\geq 0.19$. %, and then we can use Proposition \ref{Prop:PT_tau_pos} to deduce that
%\begin{equation*}
%\delta \hat r(\bar \phi) \geq \delta \tilde r(\bar \phi) - \delta \hat \ell_0 \geq 0.
%\end{equation*}

\begin{figure}
\resizebox{.75\textwidth}{!}{\includegraphics{segm_tent_2.png}}
\caption{Plot of the function \eqref{Equa:segm_tent_2}.}
\label{Fig:segm_tent_2}
\end{figure}

We thus have proved the following lemma.

\begin{lemma}
\label{Lem:segm_tent_2}
If $\check \phi_0 \leq \phi_0 + 2\pi + \bar \theta - \theta, \check \phi_2 \geq \phi_0 + 2\pi + \bar \theta$, then $\delta \hat r(\bar \phi) \geq 0$.
\end{lemma}


\subsubsection{Segment-segment with $\check \phi_0 \geq \phi_0 + 2\pi + \bar \theta - \theta, \check \phi_1 \leq \phi_0 + 2\pi + \bar \theta$: see Fig. \ref{Fig:segm_segm_sat_4}}
\label{Sss:segm_semg_after_neg_4}


We compute in this case
\begin{equation*}
\delta \hat Q_2 - \delta \hat Q_0 = 0, \quad \delta \hat L = 0
\end{equation*}
\begin{equation*}
\delta \hat r_0 = \rho(\bar \tau - 1) e^{\bar c (2\pi + \bar \alpha) (\bar \tau - 1)}.
\end{equation*}
In terms of $\check \tau_0$ the interval of interest is
\begin{equation*}
2 - \frac{\theta}{2\pi + \bar \alpha} \leq \bar \tau < 2 - \hat \tau, \quad \theta > \hat \theta.
\end{equation*}

The computations of Lemma \ref{Lem:relation_admissibility_tent} gives
\begin{equation*}
\hat r_0 = \delta \tilde r(\check \phi_0;s_0),
\end{equation*}
\begin{equation*}
\hat \ell_0 = \frac{\hat r_0 (1 - \cos(\hat \theta))}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
\begin{equation*}
\hat r_2 = \frac{\hat r_0 \sin(\bar \alpha + \hat \theta) + \hat \ell_0 \sin(\hat \theta)}{\sin(\bar \alpha)} \geq \delta \tilde r_2(\check \phi_2),
\end{equation*}
where in the last inequality we observe that $\theta > \hat \theta$ and thus $\delta \tilde r > 0$.

Using Proposition \ref{Prop:PT_tau_pos} we conclude that $\delta \hat r(\bar \phi) > 0$.

\begin{lemma}
\label{Lem:segm_tent_3}
If $2 - \frac{\theta}{2\pi + \bar \alpha} \leq \tau < 2 - \frac{\hat \theta}{2\pi + \bar \alpha}$, then $\delta \hat r(\bar \phi) > 0$.
\end{lemma}



\subsubsection{Segment-segment with $\check \phi_0 \geq \phi_0 + 2\pi + \bar \theta - \theta, \check \phi_1 \geq \phi_0 + 2\pi + \bar \theta$: see Fig. \ref{Fig:segm_segm_sat_5}}
\label{Sss:segm_semg_after_neg_5}


In this case we have
\begin{align*}
\delta \hat Q_2 - \delta \hat Q_0 &= \delta \tilde r(\check \phi_2 - 2\pi - \bar \alpha) e^{\i (\phi_0 + \bar \theta -\bar \alpha + (2\pi + \bar \alpha) (\tau - 2 + \hat \tau))} - e^{\i (\phi_0 + \bar \theta - \theta - (\phi_0 + \bar \theta - \bar \alpha + (2\pi + \bar \alpha) (\tau - 1)))} \\
&= \rho(\bar \tau - 2 + \hat \tau) e^{\bar c (2\pi + \bar \alpha) (\bar \tau - 2 + \hat \tau)} e^{\i (\phi_0 + \bar \theta + (2\pi + \bar \alpha) (\tau - 1 + \hat \tau))} e^{\i (\hat \theta - \bar \alpha)} \\
& \quad - e^{\i (\phi_0 + \bar \theta - \bar \alpha + (2\pi + \bar \alpha) (\tau - 1))} e^{\i (- \theta - (2\pi + \bar \alpha) (\tau - 2)))},
\end{align*}
\begin{align*}
\delta \hat L %&= \delta s_0 + \Delta P' + \int_{\delta \phi_2}^\phi \frac{r'}{\sin(\bar \alpha)} - \Delta P - \int_0^\phi \frac{r}{\sin(\bar \alpha)} \\
&= \delta \Delta P - \frac{r(\phi_2)}{\sin(\bar \alpha)} \delta \phi_2 + \int_0^{(2\pi + \bar \alpha)(\tau - 2 + \hat \tau)} \frac{\delta \tilde r(\phi)}{\sin(\bar \alpha)} d\phi \\
\big[ (\ref{Equa:delta_P_2P_1_segm}) \big] \quad &= - 1 + \frac{1 - \cos(\theta)}{\sin(\bar \alpha)^2} + \int_0^{(2\pi + \bar \alpha)(\tau - 2 + \hat \tau)} \frac{\delta \tilde r(\phi)}{\sin(\bar \alpha)} d\phi,
\end{align*}
\begin{equation*}
\delta \hat r_0 = \rho(\bar \tau - 1) e^{\bar c (2\pi + \bar \alpha) (\bar \tau - 1)}.
\end{equation*}
In terms of $\check \tau_0$ the interval of interest is
\begin{equation*}
2 - \frac{\hat \theta}{2\pi + \bar \alpha} \leq \bar \tau < 2, \quad \theta > (2\pi + \bar \alpha)(2 - \tau).
\end{equation*}
In Fig. \ref{Fig:segm_tent_3} we numerically plot the function
\begin{equation}
\label{Equa:segm_tent_3}
\frac{\delta \hat r_2 - \delta \tilde r(\check \phi_2)}{\theta^2} % \delta \hat r(\bar \phi) e^{- \bar c (2\pi + \bar \alpha) \bar \tau} = \frac{e^{- \bar c (2\pi + \bar \alpha) \bar \tau}}{\theta^2} \big[ e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} (\delta \hat r(\check \phi_2) - \delta \tilde r(\check \phi_2)) + \delta \tilde r(\bar \phi) - \delta \hat \ell_0 \big],
\end{equation}
as a function of $\bar \tau$. The function is strictly positive $\geq 1$, and then we can use Proposition \ref{Prop:PT_tau_pos} to deduce that
\begin{equation*}
\delta \hat r(\bar \phi) \geq \delta \tilde r(\bar \phi) - \delta \hat \ell_0 \geq 0.
\end{equation*}

\begin{figure}
\resizebox{.75\textwidth}{!}{\includegraphics{segm_tent_3.png}}
\caption{Plot of the function \eqref{Equa:segm_tent_3}.}
\label{Fig:segm_tent_3}
\end{figure}

We thus have proved the following lemma.

\begin{lemma}
\label{Lem:segm_tent_5}
If $\check \phi_0 \geq \phi_0 + 2\pi + \bar \theta - \theta, \check \phi_2 \geq \phi_0 + 2\pi + \bar \theta$, then $\delta \hat r(\bar \phi) \geq 0$.
\end{lemma}


\subsubsection{Segment-segment with $\tau - 2 \geq 0$: see Fig. \ref{Fig:segm_segm_sat_6}}
\label{Sss:segm_semg_after_neg_6}


This interval of values is when both functional $AT(\tau), PT(\tau)$, Equations \eqref{Equa:AT_tau}, \eqref{Equa:PT_tau}, are positive by Propositions \ref{Prop:estima_radii_segm} and \ref{Prop:PT_tau_pos}, so that the tent is the admissible solution and moreover, being $\delta \tilde r$ positive, we can apply Lemma \ref{Lem:estima_tent} to deduce that
\begin{equation*}
\delta \hat r(\bar \phi) \geq \tilde \rho(\bar \phi) - \hat \ell_0 \geq 0.
\end{equation*}
We thus conclude that

\begin{lemma}
\label{Lem:segm_tent_6}
If $\tau \geq 2$, then $\delta \hat r(\bar \phi) \geq 0$.
\end{lemma}


\begin{remark}
\label{Rem:tent_optimal}
Observe that the positivity of $AT(\tau)$ implies that we do not need to study the arc case for $\bar \tau \geq 2$, because the perturbation $\hat r$ is a tent after this point.
\end{remark}



\subsection{Segment-arc case}
\label{Ss:segm_arc_1}


Because of the previous remark, we need to study this case only for $\bar \phi \leq \phi_0 + \bar \theta + 4\pi + \bar \alpha$, i.e. $\bar \tau < 2$.


\subsubsection{Segment-arc with $\bar \phi < \phi_0 + \bar \theta + 2\pi - \hat \theta$: see Fig. \ref{Fig:segm_arc_1}}
\label{Sss:segm_arc_1}


In this case $\check r = \tilde r$, and the optimality follows from the fact that we are outside the region $N_\mathrm{segm}$, as in the segment-segment case of Section \ref{Sss:segm-segm_low}.

\begin{lemma}
\label{Lem:segm_arc_1}
If $\bar \phi \in \phi_0 + [\beta^-(\phi_0),\bar \theta + 2\pi - \hat \theta)$, then $\delta \check r(\bar \phi) \geq 0$.
\end{lemma}

Note that the angle between the level set and the direction $e^{\i \bar \phi}$ is increasing when we move from $P_0$ towards $\check \phi$, and then the arc case cannot be optimal here: indeed by Proposition \ref{Prop:unique_optimal_guess} the we are in the negativity zone for the derivative $\delta \tilde r(\bar \phi;s_0)$.


\subsubsection{Segment-arc with $\bar \phi \in \phi_0 + 2\pi + [\bar \theta - \theta,\bar \theta)$: see Fig. \ref{Fig:segm_arc_2}}
\label{Sss:segm_arc_2}


\begin{figure}
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_2.pdf_t}}
\caption{The geometric situation of Section \ref{Sss:segm_arc_2}.}
\label{Fig:segm_arc_2}
\end{subfigure}
\hfill
\begin{subfigure}{.475\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_2_2.pdf_t}}
\caption{The geometry to compute the variations of the points in the arc case.}
\label{Fig:segm_arc_2_2}
\end{subfigure}
\end{figure}

Setting for simplicity $\bar \phi = 0$ and with $\theta$ the angle of the perturbation of the point $P_0$, the  variations of the positions of the points is (see Fig. \ref{Fig:segm_arc_2_2}):
\begin{equation*}
\delta P_0 = e^{- \i \theta}, \quad \delta \check P^- = \delta P_0 + \delta \check \ell_0 e^{\i 0}, \quad \delta \check \phi^- = \frac{\delta \check P^- \cdot e^{\i \check \theta}}{\check r(\check \phi^-)},
\end{equation*}
\begin{equation*}
\delta \check P_1 = \big[ \delta \check P^- \cdot e^{\i (\check \theta - \frac{\pi}{2})} \big] e^{\i (\check \theta + \Delta \check \phi - \frac{\pi}{2})} + \check r(\check \phi_1) \delta \check \phi_1 e^{\i (\check \theta + \Delta \check \phi)}, \quad \delta \check \phi_1 = \frac{\delta \check P^- \cdot e^{\i \check \theta}}{\check r(\check \phi^-)} + \delta \Delta \check \phi,
\end{equation*}
where the first term is the variation of the level set and the second is the variation of the angle along the level set,
\begin{equation*}
\delta \check P_2 = \delta \check P_1 + \delta \check \ell_1 e^{\i (\check \theta + \Delta \check \phi)} + \delta \check \phi_1 \check \ell_1 e^{i (\check \theta + \Delta \check \phi + \frac{\pi}{2})}.
\end{equation*}
The optimality condition requires by Lemma \ref{Lem:study_g_1_arc} that
\begin{equation*}
\check \theta = h_1(\Delta \check \phi), \quad \delta \check \theta = \delta \check \phi^- = \frac{dh_1(\Delta \check \phi)}{d\Delta \phi} \delta \Delta \check \phi,
\end{equation*}
and the saturation condition reads are
\begin{equation}
\label{Equa:segm_arc_2_satu}
\begin{split}
\delta \check P_2 \cdot e^{\i (\check \theta + \Delta \check \phi - \bar \alpha)} - \cos(\bar \alpha) \bigg( 1 + \delta \check \ell_0 - \check r(\check \phi^-) \delta \check \phi^- + \Delta \check \phi \big( \delta \check P^- \cdot e^{\i (\check \theta - \frac{\pi}{2})} \big) + \check r(\check \phi_1) \delta \check \phi_1 + \delta \check \ell_1 \bigg) & \\
\delta \check P_2 \cdot e^{\i (\check \theta + \Delta \check \phi - \frac{\pi}{2})} \sin(\bar \alpha) - \cos(\bar \alpha) \bigg( 1 + \delta \check \ell_0 - \check r(\check \phi^-) \delta \check \phi^- + \Delta \check \phi \big( \delta \check P^- \cdot e^{\i (\check \theta - \frac{\pi}{2})} \big) \bigg) &= 0.
\end{split}
\end{equation}
The final values is computed by
\begin{equation}
\label{Equa:segm_arc_2_final}
\begin{split}
\delta \hat r(\bar \phi) &= \frac{\delta \check P_2 \cdot e^{\i (\check \theta + \Delta \check \phi - \frac{\pi}{2})}}{\sin(\bar \alpha)} e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \check \theta - \Delta \check \phi)} - e^{\cot(\bar \alpha) \theta} - \delta \ell_0 \\
&= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \bigg( 1 + \delta \check \ell_0 - \big( \cos(\theta + \check \theta) + \delta \check \ell_0 \cos(\check \theta) \big) + \Delta \check \phi \big( \sin(\theta + \check \theta) + \delta \check \ell_0 \sin(\check \theta) \big) \bigg) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \check \theta - \Delta \check \phi)} - e^{\cot(\bar \alpha) \theta} - \delta \ell_0.
\end{split}
\end{equation}
Using \eqref{Equa:theta_Deltaphi_rel} we simplify into
\begin{equation*}
\begin{split}
\delta \hat r(\bar \phi) &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\theta + \check \theta) + \Delta \check \phi  \sin(\theta + \check \theta) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \check \theta - \Delta \check \phi)} - e^{\cot(\bar \alpha) \theta} \\
&= e^{\cot(\bar \alpha) \theta} \bigg( \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\theta + \check \theta) + \Delta \check \phi \sin(\theta + \check \theta) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - (\check \theta + \theta) - \Delta \check \phi)} - 1 \bigg),
\end{split}
\end{equation*}
which is $\geq 0$ unless $\theta = 0$ by Lemma \ref{Lem:study_g_1_arc}.

We thus have the following result.

\begin{lemma}
\label{Lem:segm_arc_2}
If $\bar \phi \in \phi_0 + 2\pi + [\bar \theta - \theta,\bar \theta)$, then $\delta \check r(\bar \phi) \geq 0$.
\end{lemma}


\subsubsection{Segment-arc with $\bar \phi \geq \phi_0 + 4\pi + \bar \alpha + \bar \theta, \bar \phi + \hat \theta + \Delta \phi \leq \phi_0 + 4\pi + \bar \alpha + \bar \theta - \theta$: see Fig. \ref{Fig:segm_arc_3}}
\label{Sss:segm_arc_3}


\begin{figure}
\resizebox{.75\textwidth}{!}{\input{segm_arc_3.pdf_t}}
\caption{The geometric situation of Section \ref{Sss:segm_arc_3}.}
\label{Fig:segm_arc_3}
\end{figure}

Following the same simplification of \eqref{Equa:segm_arc_2_final} by means of \eqref{Equa:theta_Deltaphi_rel} and observing that the angle of the perturbation entering in $\check P_0$ forms an angle of $\frac{\pi}{2}$, it follows that
\begin{equation*}
\begin{split}
\delta \hat r(\bar \phi) &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\theta + \check \theta) + \Delta \check \phi  \sin(\theta + \check \theta) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \check \theta - \Delta \check \phi)} - e^{\cot(\bar \alpha) \theta} \bigg|_{\theta = \frac{\pi}{2}} \cdot \delta \tilde r(\bar \phi - 2\pi - \bar \alpha) \\
&= e^{\cot(\bar \alpha) \frac{\pi}{2}} \delta \tilde r(\bar \phi - 2\pi - \bar \alpha) \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 + \sin(\check \theta) + \Delta \check \phi \cos(\check \theta) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - (\check \theta + \frac{\pi}{2}) - \Delta \check \phi)} - 1 \bigg].
\end{split}
\end{equation*}
The quantity inside bracket is strictly positive because of Remark \ref{Rem:study_f1_over}.

\begin{lemma}
\label{Lem:segm_arc_3}
If $\bar \phi \geq \phi_0 + 4\pi + \bar \alpha + \bar \theta, \bar \phi + \hat \theta + \Delta \phi \leq \phi_0 + 4\pi + \bar \alpha + \bar \theta - \theta$, then $\delta \check r(\bar \phi) \geq 0$.
\end{lemma}


\begin{figure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_4.pdf_t}}
\caption{Section \ref{Sss:segm_arc_4}.}
\label{Fig:segm_arc_4}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_5.pdf_t}}
\caption{Section \ref{Sss:segm_arc_5}.}
\label{Fig:segm_arc_5}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_6.pdf_t}}
\caption{Section \ref{Sss:segm_arc_6}.}
\label{Fig:segm_arc_6}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_7.pdf_t}}
\caption{Section \ref{Sss:segm_arc_7}.}
\label{Fig:segm_arc_7}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_8.pdf_t}}
\caption{Section \ref{Sss:segm_arc_8}.}
\label{Fig:segm_arc_8}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_10.pdf_t}}
\caption{Section \ref{Sss:segm_arc_9}.}
\label{Fig:segm_arc_9}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_9.pdf_t}}
\caption{Section \ref{Sss:segm_arc_10}.}
\label{Fig:segm_arc_10}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_11.pdf_t}}
\caption{Section \ref{Sss:segm_arc_11}.}
\label{Fig:segm_arc_11}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_12.pdf_t}}
\caption{Section \ref{Sss:segm_arc_12}.}
\label{Fig:segm_arc_12}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_13.pdf_t}}
\caption{Section \ref{Sss:segm_arc_13}.}
\label{Fig:segm_arc_13}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_14.pdf_t}}
\caption{Section \ref{Sss:segm_arc_14}.}
\label{Fig:segm_arc_14}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
\resizebox{\textwidth}{!}{\input{segm_arc_15.pdf_t}}
\caption{Section \ref{Sss:segm_arc_15}.}
\label{Fig:segm_arc_15}
\end{subfigure}
%\begin{subfigure}{.33\textwidth}
%\resizebox{\textwidth}{!}{\input{segm_arc_16.pdf_t}}
%\end{subfigure}
%\begin{subfigure}{.33\textwidth}
%\resizebox{\textwidth}{!}{\input{segm_arc_17.pdf_t}}
%\end{subfigure} \hfill
\end{figure}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_4}}
\label{Sss:segm_arc_4}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_5}}
\label{Sss:segm_arc_5}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_6}}
\label{Sss:segm_arc_6}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_7}}
\label{Sss:segm_arc_7}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_8}}
\label{Sss:segm_arc_8}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_9}}
\label{Sss:segm_arc_9}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_10}}
\label{Sss:segm_arc_10}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_11}}
\label{Sss:segm_arc_11}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_12}}
\label{Sss:segm_arc_12}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_13}}
\label{Sss:segm_arc_13}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_14}}
\label{Sss:segm_arc_14}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_15}}
\label{Sss:segm_arc_15}


\subsubsection{Segment-arc of Fig. \ref{Fig:segm_arc_16}}
\label{Sss:segm_arc_16}



\begin{figure}
\resizebox{.5\textwidth}{!}{\input{segm_arc_17.pdf_t}}
\caption{Section \ref{Sss:segm_arc_16}.}
\label{Fig:segm_arc_16}
\end{figure}



\newpage










{\color{red} non capisco questa frase} {\color{blue} confesso anche io, secondo me era solo per dire che dobbiamo osservare che potrebbero esserci angolo $\theta > \pi/2$} In the last case, we need to study how the perturbation of the fastest saturated spiral enters into the final tent/arc (final angle $>< \pi/2$ and computed its positivity.

\medskip

We stress that apriori we do not know if the last construction tent/arc is a tent or an arc. It is possible to prove that if $\bar \phi \geq \phi_0 + (2\pi+\bar \alpha) + (2\pi + \omega)$, then it is a tent, but for smaller angle the minimal solution could be given by the arc construction (meaning a segment of length $\ell_0$ together with an arc). We believe that this holds for any angle, but this requires additional computations. Therefore, instead of proving that the last construction is an arc, in the next proposition we show that the closure with the tent (even if not admissible) is positive and smaller than the true admissible perturbation. This reduces the study to the tent case. 
\begin{proposition}
    \label{Prop:tent_worst}
    The tent closure is the minimal solution.{\color{red} non lo scriverei così perchè potrebbe essere l'arco. Qui tenda potrebbe anche non essere ammissibile.} {\color{blue} Beh comunque hai capito che vuole dire che quando prendi il segmento chiude prima di tutti, se lo permettiamo non ammissibile.}
\end{proposition}

\begin{proof}
With reference to Figure \ref{fig:prop72}, we assume to be in the case where the tent/arc is in the saturated region, {\color{red} in the sense that $\bar\phi-\phi_0-2\pi\geq \omega$ ?}. {\color{red}We assume that the minimal solution in the point $P^{-}$ is an arc of endpoints $P^{-}P_1$}.

We construct a path as follows: we connect the initial point $P^-$ of the final arc with another point $Q$ of the arc by a segment, then we follow the level set of the fire (arc) up to $P_1$ and then the segment of endpoints $P_1P_2$: we require that the last point $P_2$ is saturated. Such a solution is not a spiral because the initial segment is inside the level set of the fire, in particular it is not an admissible strategy (Figure \ref{fig:prop72}).
\begin{figure}
    \centering
    \includegraphics[scale=0.45]{prop72.png}
    \caption{In the point $P^{-}$ the arc solution starts. We replace it with the a segment of endpoints $P^{-},Q$ (red segment).}
    \label{fig:prop72}
\end{figure}

We compute now the derivative of this family of solutions as in the previous section. Using Equation \eqref{eq:sec6:imp} as a reference, and {\color{blue} setting $0$ at the angle corresponding to the point $Q$ we have that %setting $0$ at the angle of $Q$
\begin{equation*}
    \delta Q = r_0 \delta \phi_0 e^{\i \frac{\pi}{2}},
\end{equation*}
because $Q$ moves along the level set,
\begin{equation*}
    \delta P_1 = r_1 \delta \phi_1 e^{\i (\delta \phi + \frac{\pi}{2})}
\end{equation*}
\begin{equation*}
    \delta P_2 = \delta P_1 + \delta \Delta P e^{\i (\phi_1 + \frac{\pi}{2})} - \Delta P \delta \phi_1 e^{\i \phi_1}.
\end{equation*}
If $h > 0$ is the gain in length by moving the segment, the saturation condition is perturbed to
\begin{align*}
    0 &= \delta P_2 \cdot e^{\i (\phi_1 + \frac{\pi}{2} - \bar \alpha)} - \cos(\bar \alpha) \big( \delta \Delta P + r_1 \delta \phi_1 - h \big) \\
    &= (r_1 \delta \phi_1 + \delta \Delta P) \cos(\bar \alpha) - \Delta P \delta \phi_1 \sin(\bar \alpha) - \cos(\bar \alpha) \big( \delta \Delta P + r_1 \delta \phi_1 - h \big) \\
    &= - \Delta P \delta \phi_1 \sin(\bar \alpha) + \cos(\bar \alpha) h.
\end{align*}
This gives
\begin{equation*}
    \Delta P \delta \phi_1 = \cot(\bar \alpha) h,
\end{equation*}
and using the relation. $\delta r_2 = - \Delta P \delta \phi_1/\sin(\bar \alpha)$ gives
\begin{equation*}
    \delta r_2 = - \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} h.
\end{equation*}
This perturbation is transported by the ODE $\dot r = \cot(\bar \alpha) r$, since it circles and angle ending before it feels itself, so that
he variation at the final angle is hence
\begin{equation*}
    \delta r(\bar \phi) = \delta r_2 e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \theta)} < 0.
\end{equation*}
Hence also for the derivative the relation is negative, so that by increasing the segment the length $\delta r(\bar \phi)$ decreases.

This shows that we can proceed in this way up to the end point of the arc, i.e. the closing solution is made by two segments, and the last segment is admissible.

The same computations holds when moving the point $Q$ (now the initial point of the second segment) towards the end point, and the spirals shrink because the saturation condition improves (we are shortening the length).

If the final segment has an angle which is not $\hat \theta$, we know that moving the point $P^-$ towards the angle $\hat \theta$ makes the solution at $\bar \phi$ to decrease. We have thus shown that there is a continuous path among spirals connecting the arc to the (non admissible) segment such that the fainal $r(\bar \phi)$ is decreasing. This concludes the proof.

}
{\color{red} onestamente non sto capendo i tuoi conti, ti chiedo da vicino, ci rinuncio.}


\medskip



%The final length is
%\begin{equation*}
%    \delta r_2 = - \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} h.
%\end{equation*}
%The variation at the final angle is hence (some geometric relations)
%\begin{equation*}
%    \delta r(\bar \phi) = \delta r_2 e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \theta)}, \quad h = 1 - \cos(\theta')....
%\end{equation*}
%The relation is linear and negative. Hence also for the derivative the relation is negative, so that by increasing the segment the length $\delta r(\bar \phi)$ decreases.
%
%Hence we can prolong the segment up to the point that the arc disappears. In this case, we move the initial point up towards the angle $\hat \theta$: we have already proved that in this case the solution decreases.

{\color{red} altra cosa: all'inizio dici che $P_0$ è saturato, ma in che punto usi questa condizione?}{\color{blue} mai}
\end{proof}

{\color{red} The previous proposition reduces the study to the case in the point $P_0$ a tent starts. We thus have to study only the tent in the next cases. Recall the reparametrization used in the previous section $\bar\tau=\frac{\bar\phi}{2\pi+\bar\alpha}$. If we assume $\phi_0=0$, then }
the case $\bar \tau \in [0,1]$ (the tent is at $0$) is in the next section, the case $\bar \tau \in [1,2]$ (the tent is in $[0,1]$ and the base is at $0$) is in Section \ref{Ss:small_bar_phi}, the case $\bar \tau \geq 2$ is in Section \ref{Ss:phi_large_optimal}. For $\bar \phi \geq 3$ we can use the Lemma {\color{red} which Lemma?}{\color{blue} credo sia il fatto che la soluzione cresce e quindi hai la tenda e non si chiude}.


\newpage




%\subsubsection{The segment starts at $\phi_0$ and closes with a segment {\color{red} meglio dare come nome l'intervallo in cui c'è la tenda}}
%\label{Sss:init_segment}
%
%
%In this case we assume that the angle $\bar \phi$ lies in
%\begin{equation*}
%    \bar \theta - \hat \theta \leq \bar \phi{\color{red}-2\pi-\phi_0} \leq \bar \theta,
%\end{equation*}
%{\color{blue} perche` non hai messo come estremo $\beta^-(\phi_0)$?}
%and that the curve $\check r$ is the segment along $\bar \phi$ until the final angle is $\hat \theta$, where the fastest closing spiral is in the segment case {\color{red}(this is indeed justified by Proposition \ref{Prop:tent_worst})}.
%
%We repeat the same perturbation analysis as before (Section \ref{c:family}), noticing here that the angles at the final corner are fixed (Figure \ref{fig:parallel:tent}).
%
%\medskip
%
%{\it Case 1.} 
%
%\smallskip
%
%\noindent {\color{red} non chiaro a cosa corrisponde il caso 1! Secondo me intendevi il caso $<\beta^-(\phi_0)$ della Sezione 4}{\color{blue} hai ragione penso} If we perturb with an angle $\theta_0$ larger than $\bar \phi - 2\pi - \phi_0$, then the fastest saturated spiral is the optimal solution in the last round by the results of the previous section, and we already know that moving along the segment generates a smaller solution, because we are in the negativity region of the derivative $\delta \tilde r$.
%\begin{figure}
%    \centering
%\includegraphics[scale=0.6]{paralleltent.png}
%    \caption{The figure represents the situation of Subsection \ref{Ss:init_segment}, where the perturbations are parallel. Moreover, the angle of the tent is fixed to be $\hat\theta$.}
%    \label{fig:parallel:tent}
%\end{figure}
%
%\medskip
%
%{\it Case 2.}
%
%\smallskip
%
%\noindent Since the angles are fixed (see Fig. \ref{fig:parallel:tent}), we can assume $\bar \phi = 2\pi{\color{red}-\phi_0}$, {\color{blue} questo $\theta$ si confonde con quello della sezione 6!!!} and the variations are
%\begin{equation*}
%    \delta P_0 = \delta s_0 e^{-i \theta}, \quad \theta = \bar \phi - 2\pi - \theta_0,
%\end{equation*}
%\begin{equation*}
%    \delta P_1 = \delta P_0 + \delta \ell_0 e^{\i (\bar \phi - 2\pi)},
%\end{equation*}
%\begin{equation*}
%    \delta P_2 = \delta P_1 + \delta \ell_1 e^{\i \hat \theta},
%\end{equation*}
%where we have denoted by
%\begin{equation*}
%    \ell_0 = |P_1 - P_0|, \quad \ell_1 = |P_2 - P_1|,
%\end{equation*}
%(see Equation \eqref{eq:sec6:imp} and hereafter).
%The vector relation among the above quantities is
%\begin{equation*}
%    \delta r_2 e^{\i (\hat \theta - \bar \alpha)} = \delta P_2,
%\end{equation*}
%
%where $r_2 = r(\bar \phi - 2\pi{\color{red}-\phi_0} + \hat \theta - \bar \alpha)$: projecting the above equation one obtains
%\begin{align*}
%    0 &= e^{\i (\frac{\pi}{2} + \hat \theta - \bar \alpha)} \cdot \delta P_2 \\
%    &= \delta s_0 \sin(\bar \alpha - \hat \theta - \theta) + \delta \ell_0 \sin(\bar \alpha - \hat \theta) + \delta \ell_1 \sin(\bar \alpha), 
%\end{align*}
%\begin{align*}
%    \delta r_2 = \delta P_2 \cdot e^{\i (\hat \theta - \bar \alpha)} &= \delta s_0 \cos(\bar \alpha - \hat \theta - \theta) + \delta \ell_0 \cos(\bar \alpha - \hat \theta) + \delta \ell_1 \cos(\bar \alpha) \\
%    &= \delta s_0 \frac{\sin(\hat \theta + \theta)}{\sin(\bar \alpha)} + \delta \ell_0 \frac{\sin(\hat \theta)}{\sin(\bar \alpha)},
%\end{align*}
%where we have used the first projection to replace $\delta \ell_1$.
%
%The saturation condition at the point $P_2 + \delta P_2$ gives
%\begin{align*}
%    0 &= \delta r_2 - \cos(\bar \alpha) \big( \delta s_0 + \delta \ell_0 + \delta \ell_1 \big) \\
%    &= \delta s_0 \big( \cos(\bar \alpha - \hat \theta - \theta) - \cos(\bar \alpha) \big) + \delta \ell_0 ( \cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)),
%\end{align*}
%so that
%\begin{equation*}
%    \delta \ell_0 = - \delta s_0 \frac{\cos(\bar \alpha - \hat \theta - \theta) - \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
%\end{equation*}
%\begin{align*}
%    \delta r_2 &= \delta s_0 \frac{\sin(\hat \theta + \theta) (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)) - \sin(\hat \theta) (\cos(\bar \alpha - \hat \theta - \theta) - \cos(\bar \alpha))}{\sin(\bar \alpha) (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha))} \\
%    &= \frac{\cot(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \big( \sin(\theta) (1 - \cos(\hat \theta)) + (1 - \cos(\theta)) \sin(\hat \theta) \big).
%\end{align*}
%
%As in Corollary \ref{Cor:equation}, the ODE for the perturbation gives
%\begin{equation*}
%    \delta r(\bar \phi - \theta -) = e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta - \theta)} \delta r_2,
%\end{equation*}
%\begin{equation*}
%    \delta r(\bar \phi -) = e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} \delta r_2 - e^{\cot(\bar \alpha) \theta},
%\end{equation*}
%and then the final value is computed as
%\begin{align*}
%    &\delta r_2 e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} - e^{\cot(\bar \alpha) \theta} - \delta \ell_0 \\
%    &= \frac{\cot(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \big( \sin(\theta) (1 - \cos(\hat \theta)) + (1 - \cos(\theta)) \sin(\hat \theta) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} - e^{\cot(\bar \alpha) \theta} + \frac{\cos(\bar \alpha - \hat \theta - \theta) - \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
%    &= \frac{1 - \cos(\hat \theta + \theta)}{1 - \cos(\hat \theta)} - e^{\cot(\bar \alpha) \theta}.
%\end{align*}
%{\color{red} come hai ottenuto l'ultima uguaglianza? non me la trovo proprio!}
%{\color{blue}
%$$
%\frac{\cot(\bar \alpha)}{\sin(\bar \alpha)}(1 - \cos(\hat \theta)) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} = 1?
%$$
%\begin{align*}
%    &\frac{\cot(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \big( \sin(\theta) (1 - \cos(\hat \theta)) + (1 - \cos(\theta)) \sin(\hat \theta) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \hat \theta)} - e^{\cot(\bar \alpha) \theta} + \frac{\cos(\bar \alpha - \hat \theta - \theta) - \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} \\
%    &= \frac{\sin(\bar \alpha) \sin(\theta) + \sin(\bar \alpha) \sin(\hat \theta) \frac{1 - \cos(\theta)}{1 - \cos(\hat \theta)} + \cos(\bar \alpha - \hat \theta - \theta) - \cos(\bar \alpha)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)} - e^{\cot(\bar \alpha) \theta},
%\end{align*}
%e per il numeratore
%\begin{align*}
%    & \sin(\bar \alpha) \sin(\theta) (1 - \cos(\hat \theta) + \sin(\bar \alpha) \sin(\hat \theta) (1 - \cos(\theta)) + (1 - \cos(\hat \theta)) (\cos(\bar \alpha - \hat \theta - \theta) - \cos(\bar \alpha)) \\
%    &= \sin(\bar \alpha) (\sin(\theta) + \sin(\hat \theta)) - \sin(\bar \alpha) \sin(\theta + \hat \theta) + (1 - \cos(\hat \theta)) [\cos(\bar \alpha) \cos(\hat \theta + \theta) + \sin(\bar \alpha) \sin(\theta + \hat \theta) - \cos(\bar \alpha)] \\
%    &= \sin(\bar \alpha) (\sin(\theta) + \sin(\hat \theta)) + (1 - \cos(\hat \theta)) \cos(\bar \alpha) [\cos(\hat \theta + \theta) - 1] - \cos(\hat \theta) \sin(\bar \alpha) \sin(\theta + \hat \theta) \\
%    &= \sin(\bar \alpha) (\sin(\theta) + \sin(\hat \theta)) + (1 - \cos(\hat \theta)) \cos(\bar \alpha) [\cos(\hat \theta + \theta) - 1] - \cos(\hat \theta) \sin(\bar \alpha) [ \sin(\theta) \cos(\hat \theta) + \sin(\hat \theta) \cos(\theta) ] \\
%    &= \sin(\bar \alpha) (\sin(\theta) \sin(\hat \theta)^2 + \sin(\hat \theta) (1 - \cos(\theta) \cos(\hat \theta)) ) + (1 - \cos(\hat \theta)) \cos(\bar \alpha) [\cos(\hat \theta + \theta) - 1] \\
%    &= \sin(\bar \alpha) \sin(\hat \theta) (1 - \cos(\theta + \hat \theta)) + (1 - \cos(\hat \theta)) \cos(\bar \alpha) [\cos(\hat \theta + \theta) - 1] \\
%    &= (\sin(\bar \alpha) \sin(\hat \theta) - (1 - \cos(\hat \theta)) \cos(\bar \alpha)) [\cos(\hat \theta + \theta) - 1] \\
%    &= (1 - \cos(\hat \theta + \theta)) (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha))
%\end{align*}
%}
%
%
%At the first order near $\theta = 0$ this function is
%\begin{equation*}
%    \frac{d\delta r(\bar \phi)}{d\theta} = \theta \bigg( \frac{\sin(\hat \theta)}{1 - \cos(\hat \theta)} - \cot(\bar \alpha) \bigg) + \mathcal O(\theta^2),
%\end{equation*}
%which is positive, and numerically $\frac{\delta r(\bar \phi)}{\theta}$ is positive increasing in the remaining part of the interval, remaining above $3.45283$.
%
%We have proved the following result.
%
%\begin{lemma}
%    \label{Lem:segm_segm_optimal}
%    Under assumptions at the beginning of this section, any non-null perturbation of the optimal solution is strictly positive at $\bar \phi$.
%\end{lemma}




\newpage



\subsection{The segment starts at $\phi_0$ and closes with an arc}
\label{Ss:tent_arc}

{\color{red} questa sezione non sparisce quindi?}{\color{blue} si dovrebbe sparire ora}
This case can happen when $\bar \theta$ of the segment case is close to $\frac{\pi}{2}$, so that by prolonging the segment the angle $\bar \theta$ overtakes $\frac{\pi}{2}$. We set as before $\bar \phi = 2\pi$. The length $\ell_0$ of the initial segment is chosen according to Proposition \ref{Prop:unique_optimal_guess}.

The case where the angle $\theta_0 > \bar \phi - 2\pi$ is as before.

Using Figure ?? as reference and recalling that $\hat \theta = \hat \theta(\Delta \phi)$, the perturbation of the points are
\begin{equation*}
    \delta P^- = \delta s_0 e^{-i \theta},
\end{equation*}
\begin{equation*}
    \delta P_0 = \delta P_0 + \delta \ell_0 e^{\i 0},
\end{equation*}
%and denoting with $\theta$ the angle between the segment $\ell_0$ and the starting of the arc
\begin{equation*}
    \delta P_1 = (\delta P_0 \cdot e^{\i (\hat \theta - \frac{\pi}{2})}) e^{\i (\Delta \phi + \hat \theta - \frac{\pi}{2})} + r_1 \delta \phi_1 e^{\i (\Delta \phi + \hat \theta)},
\end{equation*}
\begin{equation*}
    \delta P_2 = \delta P_1 + \delta \ell_1 e^{\i (\Delta \phi + \hat \theta)} - \Delta P \delta \phi_1 e^{\i (\Delta \phi + \hat \theta - \frac{\pi}{2})}.
\end{equation*}
Observing that at $P_2$ the spiral is saturated, the vector relation at the point $P_2$ gives
\begin{equation*}
    r_2 \delta \phi_1 e^{\i (\Delta \phi + \hat \theta - \bar \alpha + \frac{\pi}{2})} + \delta r_2 e^{\i (\Delta \phi + \hat \theta - \bar \alpha)} = \delta P_2,
\end{equation*}
and the saturation at $P_2$ yields
\begin{equation*}
    \delta r_2 - \cos(\bar \alpha) \big( \delta s_0 + \delta \ell_0 + r_1 \delta \phi_1 - r_0 \delta \phi_0 + (\delta P_0 \cdot e^{\i (\Delta \phi + \hat \theta - \frac{\pi}{2})}) \Delta \phi + \delta \ell_1 \big) = 0.
\end{equation*}
We have also the request that $\hat \theta = \hat \theta(\Delta \phi)$, i.e. on the null curve, and observe that $\phi_0 + \frac{\pi}{2} = \hat \theta$, so that $\delta \phi_0 = \delta \hat \theta$.

Projecting the vector relation on $e^{\i (\Delta \phi + \hat \theta - \bar \alpha)}$
\begin{align*}
    \delta r_2 = \delta \ell_1 \cos(\bar \alpha) - \Delta P \delta \phi_1 \sin(\bar \alpha) + r_1 \delta \phi_1 \cos(\bar \alpha) + (\delta P_0 \cdot e^{\i (\hat \theta - \frac{\pi}{2})}) \sin(\bar \alpha), 
\end{align*}
which gives together with the saturation
\begin{equation*}
     - \Delta P \delta \phi_1 \sin(\bar \alpha) + (\delta P_0 \cdot e^{\i (\hat \theta - \frac{\pi}{2})}) \sin(\bar \alpha) = \cos(\bar \alpha) \big( \delta s_0 + \delta \ell_0 - r_0 \delta \hat \theta + (\delta P_0 \cdot e^{\i (\Delta \phi + \hat \theta - \frac{\pi}{2})}) \Delta \phi \big),
\end{equation*}
i.e.
\begin{equation*}
    \Delta P \delta \phi_1 = (1 - \cot(\bar \alpha) \Delta \phi) (\delta P_0 \cdot e^{\i (\hat \theta - \frac{\pi}{2})}) - \cot(\bar \alpha) \big( \delta s_0 + \delta \ell_0 - r_0 \delta \hat \theta \big).
\end{equation*}

Projecting along $e^{\i (\Delta \phi + \hat \theta + \frac{\pi}{2} - \bar \alpha)}$
\begin{equation*}
    r_2 \delta \phi_1 = \delta \ell_1 \sin(\bar \alpha) + \Delta P \delta \phi_1 \cos(\bar \alpha) + r_1 \delta \phi_1 \sin(\bar \alpha) - (\delta P_0 \cdot e^{\i (\hat \theta - \frac{\pi}{2})}) \cos(\bar \alpha),
\end{equation*}
and finally the perturbation of the initial data is
\begin{align*}
    \delta r_2 - \cot(\bar \alpha) r_2 \delta \phi_1 &= \frac{(\delta P_0 \cdot e^{\i (\hat \theta - \frac{\pi}{2})}) - \Delta P \delta \phi_1}{\sin(\bar \alpha)} \\
    &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( \delta s_0 + \delta \ell_0 - r_0 \delta \hat \theta + \Delta \phi (\delta P_0 \cdot e^{\i (\hat \theta - \frac{\pi}{2})} \big) \\
    &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( \delta s_0 + \delta \ell_0 - (\delta s_0 \cos(\hat \theta + \theta) + \delta \ell_0 \cos(\hat \theta)) + \Delta \phi (\delta s_0 \sin(\theta + \hat \theta) + \delta \ell_0 \sin(\hat \theta) \big). 
\end{align*}
The solution at $\bar \phi$ is then
\begin{align*}
    \delta r(\bar \phi) &= (\delta r_2 - \cot(\bar \alpha) r_2 \delta \phi_1) e^{\cot(\bar \alpha)(2 \pi + \bar \alpha - \Delta \phi - \hat \theta)} - \delta s_0 e^{\cot(\bar \alpha) \theta)} - \delta \ell_0 \\
    &= \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( \delta s_0 + \delta \ell_0 - (\delta s_0 \cos(\hat \theta + \theta) + \delta \ell_0 \cos(\hat \theta)) + \Delta \phi (\delta s_0 \sin(\theta + \hat \theta) + \delta \ell_0 \sin(\hat \theta) \big) \bigg] e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta \phi - \hat \theta)} - \delta s_0 e^{\cot(\bar \alpha) \theta} - \delta \ell_0.
\end{align*}

We next use the choice of $\hat \theta$: if $\theta = 0$ we obtain
\begin{align*}
    \delta r(\bar \phi) &= \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 -  \cos(\hat \theta) + \Delta \phi \sin(\hat \theta) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta \phi - \hat \theta)} - 1 \bigg] (\delta s_0 + \delta \ell_0) = 0
\end{align*}
by the null condition, so that we simplify
\begin{align*}
    \frac{\delta r(\bar \phi)}{\delta s_0} &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big(  \cos(\hat \theta) - \cos(\hat \theta + \theta) + \Delta \phi (\sin(\theta + \hat \theta) - \sin(\hat \theta)) \big) e^{\cot(\bar \alpha) (2\pi + \bar \alpha - \Delta \phi - \hat \theta)} - (e^{\cot(\bar \alpha) \theta} - 1) \\
    &= \frac{1 - \cos(\hat \theta + \theta) + \Delta \phi \sin(\hat \theta + \theta)}{1 - \cos(\hat \theta) + \Delta \phi \sin(\hat \theta)} - e^{\cot(\bar \alpha) \theta}.
\end{align*}
%Since
%\begin{equation*}
%    \frac{1 - \cos(\hat \theta + \theta) + \Delta \phi \sin(\hat \theta + \theta)}{1 - \cos(\hat \theta) + \Delta \phi \sin(\hat \theta)} \geq \frac{1 - \cos(\hat \theta + \theta)}{1 - \cos(\hat \theta)}, \quad \hat \theta = 0.50...
%\end{equation*}
Numerical analysis shows that the above function is $\geq 0.546759 \theta$.

\begin{lemma}
\label{Lem:segment_arc_optimal}
    Under the assumptions above, it holds $\delta r(\bar \phi) \geq 0$.
\end{lemma}
{\color{blue} qui secondo me è più chiaro prima fare tutti i casi del segmento, poi tutti quelli dell'arco, seguendo la suddivisione delle griglie}
\subsection{{\color{red} Arc Case}}
{\color{red}In the following subsections, we analyze the cases of the second grid, where the assumption is that in the point $\phi_0$ the optimal spiral is an arc, namely a subset of the level set of the fire.}

\subsection{The arc starts at $\phi_0$ and ends with a segment, {\color{red}$\bar\phi-\phi_0-2\pi\in[\frac{\pi}{2},\omega)$.}}
\label{Ss:arc_to_segment}

{\it This should be the most general case {\color{red} che intendi qui?}{\color{blue} che non dobbiamo considerare la chiusura con un arco: quindi parti con un arco (prop 7.2), e chiudi con un segmento}
\begin{figure}
    \centering
  \includegraphics[scale=0.5]{proparcsegment.png}
  \caption{The case of Subsection \ref{Ss:arc_to_segment}. The red region indicates $\bar\phi-\phi_0-2\pi\in[\frac{\pi}{2},\omega)$. The blue curve is the one constructed in Section \ref{S:segment}, while the black one indicates the optimal strategy.}
  \label{fig:proparc:segment:1}
  \end{figure}
  
     \begin{figure}
  \centering
  \includegraphics[scale=0.7]{perturbationtent1.png}
  \caption{Study of the perturbations for the case of Subsection \ref{Ss:arc_to_segment}.}
 \label{fig:proparc:segment:2}

    
\end{figure}
In this case, the segment with direction $\bar \phi - 2\pi$ starts along the arc of the level set of the fastest saturated spiral $\tilde r(\phi;s_0)$: hence we have that the closing solution is made of a level set arc of opening $\Delta \phi^-$, a segment of length $\ell_0$, a final segment of length $\ell_1$ and a saturated spiral (see \ref{fig:proparc:segment:1}).

The perturbations are (see Fig. ??)
\begin{equation*}
    \delta P^{--} = \delta s e^{\i (\frac{\pi}{2} - \theta^-)},
\end{equation*}
\begin{equation*}
    \delta P^- = \delta s \sin(\theta^-) e^{\i \Delta \phi^-} = h_0 e^{\i \Delta \phi^-}, \quad h_0 = \delta s \sin(\theta^-),
\end{equation*}
\begin{equation*}
    \delta P_0 = h_0 e^{\i \Delta \phi^-} + \delta \ell_0 e^{\i (\Delta \phi^- + \frac{\pi}{2})},
\end{equation*}
\begin{equation*}
    \delta P_1 = \delta P_0 + \delta \ell_1 e^{\i (\Delta \phi^- + \frac{\pi}{2} + \hat \theta)}. %(\delta \ell_0 \sin(\theta) + h_0 \cos(\theta)) e^{\i (\frac{\pi}{2} + \Delta \phi^- + \hat \theta} + r_1 \delta \phi_1 e^{\i (\phi_1 + \frac{\pi}{2})} = h_1 e^{\i \phi_1} + r_1 \delta \phi_1 e^{\i (\phi_1 + \frac{\pi}{2})},
\end{equation*}

The vector constraint is that
\begin{equation*}
    \delta r_2 e^{\i (\Delta \phi^- + \frac{\pi}{2} + \hat \theta - \bar \alpha)} = \delta P_2,
\end{equation*}
and projecting on $e^{\i (\Delta \phi^- + \frac{\pi}{2} + \hat \theta - \bar \alpha)}, e^{\i (\Delta \phi^- + \hat \theta - \bar \alpha)}$ we obtain
\begin{equation*}
    \delta r_2 = h_0 \sin(\bar \alpha - \hat \theta) + \delta \ell_0 \cos(\bar \alpha - \hat \theta) + \delta \ell_! \cos(\bar \alpha), 
\end{equation*}
\begin{equation*}
    0 = h_0 \cos(\bar \alpha - \hat \theta) - \delta \ell_0 \sin(\bar \alpha - \hat \theta) - \delta \ell_1 \sin(\bar \alpha).
\end{equation*}

The saturation condition is
\begin{align*}
    0 &= \delta r_2 - \cos(\bar \alpha) \big( \delta s_0 (1 - \cos(\theta) + \sin(\theta) \Delta \phi^-) + \delta \ell_0 + \delta \ell_1 \big) \\
    &= \delta s_0 (\sin(\theta) \sin(\bar \alpha - \hat \theta) - \cos(\bar \alpha) ((1 - \cos(\theta) + \sin(\theta) \Delta \phi^-) + \delta \ell_0 (\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)),
\end{align*}
where we have used the first projection of the vector relation, and then we get
\begin{equation*}
    \delta \ell_0 = - \delta s_0 \frac{\sin(\theta) \sin(\bar \alpha - \hat \theta) - \cos(\bar \alpha) (1 - \cos(\theta) + \sin(\theta) \Delta \phi^-)}{\cos(\bar \alpha - \hat \theta) - \cos(\bar \alpha)},
\end{equation*}
\begin{equation*}
    \delta r_2 = h_0 \frac{\cos(\hat \theta)}{\sin(\bar \alpha)} + \delta \ell_0 \frac{\sin(\hat \theta)}{\sin(\bar \alpha)}.
\end{equation*}

Using the same approach as in the arc case, the solution is written as
\begin{align*}
    \delta r(\bar \phi + 2\pi) &= \delta r_2 e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} - e^{\cot(\bar \alpha) (\Delta \phi^- + \theta)} + \cos(\theta) e^{\cot(\bar \alpha) \Delta \phi^-} - \sin(\theta) \int_0^{\Delta \phi^-} e^{\cot(\bar \alpha)(\Delta \phi^- - \phi)} d\phi - \delta \ell_0 \\
    &= \bigg( h_0 \frac{\cos(\hat \theta)}{\sin(\bar \alpha)} + \delta \ell_0 \frac{\sin(\hat \theta)}{\sin(\bar \alpha)} \bigg) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \theta)} - e^{\cot(\bar \alpha)(\Delta \phi^- + \theta)} \\
    & \quad + \cos(\theta) e^{\cot(\bar \alpha) \Delta \phi^-} - \sin(\theta) \frac{e^{\cot(\bar \alpha) \Delta \phi^-} - 1}{\cos(\bar \alpha)} - \delta \ell_0. %\\
%    &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big[ \sin(\theta^-) \Delta \phi^- + \delta \ell_0 - (\delta \ell_0 \cos(\theta) - \sin(\theta^-) \sin(\theta))  + \big( \delta \ell_0 \sin(\theta) + \sin(\theta^-) \cos(\theta) \big) \Delta \phi \big] e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \theta)} \\
%    &\quad - e^{\cot(\bar \alpha)(\Delta \phi^- + \theta^-)} + \cos(\theta^-) e^{\cot(\bar \alpha) \Delta \phi^-} - \sin(\theta^-) \tan(\bar \alpha) (e^{\cot(\bar \alpha) \Delta \phi^-} - 1) - \delta \ell_0 \\
%    &= \delta \ell_0 \bigg[ \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} (1 - \cos(\theta) + \Delta \phi \sin(\theta)) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \theta)} - 1 \bigg] \\
%    &\quad + \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \sin(\theta^-) \big[ \Delta \phi^- + \sin(\theta) + \cos(\theta) \Delta \phi \big] e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \Delta \phi - \theta)} \\
%    &\quad - e^{\cot(\bar \alpha)(\Delta \phi^- + \theta^-)} + \cos(\theta^-) e^{\cot(\bar \alpha) \Delta \phi^-} - \sin(\theta^-) \tan(\bar \alpha) (e^{\cot(\bar \alpha) \Delta \phi^-} - 1). 
\end{align*}
Recall that %$\theta,\Delta \phi$ are related by being on the critical curve,
\begin{align*}
\frac{\cot(\bar \alpha)}{\sin(\bar \alpha)} \big( 1 - \cos(\hat \theta)\big) e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} - 1 = 0,
\end{align*}
so that the perturbation becomes
\begin{align*}
    \delta r(\bar \phi + 2\pi)
    &= \frac{h_0 \cos(\hat \theta) + \delta \ell_0 \sin(\hat \theta) - \delta \ell_0 \cot(\bar \alpha) (1 - \cos(\hat \theta)) + \cos(\theta) \cot(\bar \alpha) (1 - \cos(\hat \theta))}{\sin(\bar \alpha)} e^{\cot(\bar \alpha)(2\pi + \bar \alpha - \hat \theta)} \\
    & \quad - e^{\cot(\bar \alpha)(\Delta \phi^- + \theta)} + \cos(\theta) (e^{\cot(\bar \alpha) \Delta \phi^-} - 1) - \sin(\theta) \frac{e^{\cot(\bar \alpha) \Delta \phi^-} - 1}{\sin(\bar \alpha)}. %\\
%    &= \cot(\bar \alpha) \big( 1 - \cos(\theta) - \cos(\hat \theta + \theta) + \sin(\theta) \Delta \phi^-\big) 
\end{align*}
%with $\theta = \hat \theta(\Delta \phi)$ the null curve.

The minimal value of $\frac{\rho}{\theta}$ happens for $\Delta \phi = 0, \theta = 0$, and numerically its value is $1.9$.

\begin{lemma}
    \label{Lem:positive_deriva_arc_arc}
    Under the assumptions above, the perturbation is positive unless we follow the optimal solution.
\end{lemma}


\end{comment}



==> segmentcasepartitolte.tex <==
\noindent\textbf{Relations at the point $P_1$:} {\color{red} define the quantity
\begin{equation}
\label{eq:var:length}
    h = \frac{\delta \bar s \sin(\bar \theta - \theta_0)}{\sin(\bar \theta)}
\end{equation}
representing the variation of $r(\phi_0)$, where $\delta \bar s = |\tilde P_1 - P_1|$ is the variation of the base point for the generalized barrier}.
In particular, the time difference for reaching the points $\tilde P_1$ and $P_1$ is computed as:
\begin{equation*}
    u(\tilde P_1) = u(P_1) + h.
\end{equation*}
Moreover, we have that (see Figure \ref{segm:per})
\begin{equation}
\label{Equa:angle_delta_phi_0_segment}
r(P_1) \delta \phi_0 = h \frac{\sin\theta_0\sin\bar\theta}{\sin(\bar\theta-\theta_0)} {\color{red} \delta \bar s \sin(\theta_0)},
\end{equation}
where we recall that $(r(\phi),\phi)$ is the parametrization for the original spiral $Z$. 

Call $\textbf{n}(P_1)$ the direction orthogonal to the segment $P_1P_2$ and $\textbf{t}(P_1)$ the tangent such that $(\textbf{t}(P_1),\textbf{n}(P_1)) =(-e_1,e_2)$ {\color{red} $(\textbf{n}(P_1),\textbf{t}(P_1))$ is an orthogonal base}. We have that
\begin{equation}
    \tilde P_1 = P_1 + h \sin\bar\theta \textbf{n}(P_1) + h \sin\bar\theta \cot(\bar\theta-\theta_0) \textbf{t}(P_1) = {\color{red} P_1 + \delta \bar s \sin(\bar \theta - \theta_0) \mathbf t(P_1) + \delta \bar s \cos(\bar \theta - \theta_0) \mathbf n(P_1).}
\end{equation}

\medskip

\noindent\textbf{Relations at the point $P_2$:} the new angle is computed as
$$
{\color{red} \angle(e^{i\phi_0},[\tilde P_1,\tilde P_2])} \quad 
\angle O_0\tilde P_1\tilde P_2=\pi-\bar\theta-\delta\bar\theta
$$
and{\color{red}, due to the tangency with the saturated spiral in $P_2$,} the following relation holds:
   \begin{equation}
       \phi_0 + \bar\theta + \delta \bar \theta = \phi_2 + \delta \phi_2 + \bar \alpha.
   \end{equation}
%holds. 
Hence we obtain %We observe that since $\phi_0+\bar\theta=\phi_2+\bar\alpha$ we have that 
$$
\delta \bar \theta = \delta \phi_2.
$$
The position of the perturbed point $\tilde P_2$ is computed as
\begin{equation}
    \tilde P_2 = P_2+\left(h\sin\bar\theta-|P_2-P_1|\delta\phi_1\right)\textbf{n}(P_1)+\left(\left(h\sin\bar\theta-|P_2-P_1|\delta\bar\theta\right)\cot\bar\alpha+\frac{f_{\phi_0}(P_2)\delta\bar\theta}{\sin\bar\alpha}\right)\textbf{t}(P_1).
   \end{equation}
{\color{red} \begin{equation}
    \tilde P_2 = P_2 + \big( \delta \bar s \sin(\bar \theta - \theta_0) - |P_2 - P_1| \delta \phi_1 \big) \textbf{n}(P_1) + \left( \big( \delta \bar s \sin(\bar \theta - \theta_0) - |P_2 - P_1| \delta \bar \theta \big) \cot(\bar \alpha) + \frac{r_{\phi_0}(P_2) \delta(\bar \theta)}{\sin(\bar \alpha)} \right) \textbf{t}(P_1).
\end{equation}}
In particular, the variation of the length of the segment $[P_1,P_2] = |\tilde P_2 - \tilde P_1| - |P_2 - P_1|$ is computed as follows:
   \begin{equation}
   \label{eq:difference:length}
       \delta |P_2 - P_1| = (h \sin\bar\theta-|P_2-P_1|\delta\bar\theta)\cot\bar\alpha-h\sin\bar\theta\cot(\bar\theta-\theta_0)+\frac{f_{\phi_0}(P_2)\delta\phi_2}{\sin\bar\alpha}.
   \end{equation}
{\color{red} \begin{equation}
   \label{eq:difference:length}
       \delta |P_2 - P_1| = \big( \delta \bar s \sin(\bar \theta - \theta_0) - |P_2 - P_1| \delta \bar \theta \big) \cot(\bar \alpha) - \delta \bar s \cos(\bar \theta - \theta_0) + \frac{r_{\phi_0}(P_2) \delta \phi_2}{\sin(\bar \alpha)}.
\end{equation}}
The time difference is
\begin{equation*}
   \tilde u(\tilde P_2)-u(P_2)= {f_{\phi_0}(P_2)}\delta\bar\theta\cot\bar\alpha+(h\sin\bar\theta-|P_2-P_1|\delta\bar\theta)\frac{1}{\sin\bar\alpha}.
\end{equation*}
{\color{red} \begin{equation*}
   u(\tilde P_2) - u(P_2) = r_{\phi_0}(P_2) \delta \bar \theta \cot(\bar \alpha) + \big( \delta \bar s \sin(\bar \theta - \theta_0) - |P_2 - P_1| \delta \bar \theta \big) \frac{1}{\sin(\bar \alpha)}.
\end{equation*}}
{\color{red} and we can write the admissibility condition as} Finally the admissibility condition reads as
   \begin{align*}
       &\left({h\sin\bar\theta}-|P_2-P_1|\delta\bar\theta\right)\frac{1}{\sin\bar\alpha}+f_{\phi_0}(P_2)\delta\bar\theta\cot\bar\alpha \\ & -\cos\bar\alpha\left(\left(h\sin\bar\theta-|P_2-P_1|\delta\bar\theta\right)\cot\bar\alpha+\frac{f_{\phi_0}(P_2)\delta\bar\theta}{\sin\bar\alpha}-h\sin\bar\theta\cot(\bar\theta-\theta_0)\right) -\cos\hat\alpha{h}\frac{\sin(\bar\theta)}{\sin(\bar\theta-\theta_0)}\\ &
       =\left({h\sin\bar\theta}-|P_2-P_1|\delta\bar\theta\right)\sin\bar\alpha+\cos\bar\alpha\sin\bar\theta\cot(\bar\theta-\theta_0)-\cos\hat\alpha\frac{\sin\bar\theta}{\sin(\bar\theta-\theta_0)}=0.
       %\\ &=\left({h\sin\bar\theta}-|P_2-P_1|\delta\bar\theta\right)\sin\alpha-\cos\alpha h\frac{\sin\bar\theta-\sin\theta_0}{\sin(\bar\theta-\theta_0)}+h\cos\alpha\cos\bar\theta=0.
   \end{align*}
{\color{red} \begin{align*}
    &r_{\phi_0}(P_2) \delta \bar \theta \cot(\bar \alpha) + \big( \delta \bar s \sin(\bar \theta - \theta_0) - |P_2 - P_1| \delta \bar \theta \big) \frac{1}{\sin(\bar \alpha)} \\
    & \quad \quad - \cos(\bar \alpha) \left( \big( \delta \bar s \sin(\bar \theta - \theta_0) - |P_2 - P_1| \delta \bar \theta \big) \cot(\bar \alpha) - \delta \bar s \cos(\bar \theta - \theta_0) + \frac{r_{\phi_0}(P_2) \delta \phi_2}{\sin(\bar \alpha)} \right) - \cos(\hat \alpha) \\
    & \quad = \big( \delta \bar s \sin(\bar \theta - \theta_0) - |P_2 - P_1| \delta \bar \theta \big) \sin(\bar \alpha) + \cos(\bar \alpha) \delta \bar s \cos(\bar \theta - \theta_0) -\cos(\hat \alpha) = 0.
    %\\ &=\left({h\sin\bar\theta}-|P_2-P_1|\delta\bar\theta\right)\sin\alpha-\cos\alpha h\frac{\sin\bar\theta-\sin\theta_0}{\sin(\bar\theta-\theta_0)}+h\cos\alpha\cos\bar\theta=0.
\end{align*}}
The above computations lead to the following formula for $\delta \bar \theta$:
\begin{equation*}
    \delta \bar \theta = \frac{h}{|P_2-P_1|}\left(\sin\bar\theta+\cot\bar\alpha\sin\bar\theta\cot(\bar\theta-\theta_0)-\frac{\cos\hat\alpha}{\sin\bar\alpha}\frac{\sin\bar\theta}{\sin(\bar\theta-\theta_0)}\right),
\end{equation*}
{\color{red} \begin{equation}
\label{Equa:delta_bar_theta_segment}
    \delta \bar \theta = \frac{\delta \bar s}{|P_2 - P_1|} \left( \sin(\bar \theta - \theta_0) + \cot(\bar \alpha) \cos(\bar \theta - \theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \right).
\end{equation}}
%that should be compared with the previous case with $\bar\theta=\frac{\pi}{2}$ and $\Delta\phi=0$. 
In this case the initial data (where we are deriving w.r.t. the parameter $h$) is the following:
{\color{red} We thus compute the value of the initial data $\bar r_{\bar s}(\phi)$ as  
\begin{equation*}
    \bar r_{\bar s}(\phi) = \begin{cases}
        0 & \phi \leq \phi_0, \\
        \frac{1}{\sin(\bar\theta-\phi+\phi_0)} \left( \sin(\bar \theta - \theta_0) - \frac{|P(\phi) - P_1|}{|P_2 - P_1|} \left( \sin(\bar\theta - \theta_0) + \cot(\bar \alpha) \cos(\bar \theta - \theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \right) \right) & \phi_0 \leq \phi < \phi_2.
    \end{cases}
\end{equation*}}
\begin{align*}\label{eq:initial:segment}
   \bar g_{\phi_0}(\phi)&=\frac{\sin\bar\theta}{\sin(\bar\theta-\phi+\phi_0)}-\frac{|P(\phi)-P_1|\frac{\delta\bar\theta}{h}}{\sin(\bar\theta-\phi+\phi_0)}\\&=\frac{1}{\sin(\bar\theta-\phi+\phi_0)}\left(\sin\bar\theta-\frac{|P(\phi)-P_1|}{|P_2-P_1|}\left(\sin\bar\theta+\cot\bar\alpha\sin\bar\theta\cot(\bar\theta-\theta_0)-\frac{\cos\hat\alpha}{\sin\bar\alpha}\frac{\sin\bar\theta}{\sin(\bar\theta-\theta_0)}\right)\right).
  \end{align*}
As before we are interested in the final point, i.e. for $\phi = \phi_2 = \phi_0 + \bar \theta - \bar \alpha$: %We find that the derivative in the parameter $h$ is
  \begin{equation}
  \label{eq:initial:point:segment}
  \bar r_{\phi_0}(\phi_0+\bar\theta-\bar\alpha)=\left(\frac{\cos\hat\alpha-\cos\bar\alpha\cos(\bar\theta-\theta_0)}{\sin\bar\alpha^2}\right)\frac{\sin\bar\theta}{\sin(\bar\theta-\theta_0)},
  \end{equation}
{\color{red} \begin{equation}
  \label{eq:initial:point:segment}
  \bar r_{\phi_0}(\phi_2) = \frac{\cos(\hat \alpha) - \cos(\bar \alpha) \cos(\bar \theta - \theta_0)}{\sin(\bar \alpha)^2}.
\end{equation}}
%  (compare again with the computations for the segment case, that is $\Delta\phi=0$ and $\bar\theta=\frac{\pi}{2}$). We recall again that to get $\bar f_{\phi_0}$ we need simply to multiply $\bar f_{\phi_0}=\frac{\sin(\bar\theta-\theta_0)}{\sin\bar\theta}\bar g_{\phi_0}$.

\begin{remark}
    \label{Rem:comparison_segment_arc}
    If $\bar \theta = \frac{\pi}{2}$, then the initial data becomes
    \begin{equation*}
        \bar r_{\phi_0}(\phi_2) = \frac{\cos(\hat \alpha) - \cos(\bar \alpha) \sin(\theta_0)}{\sin(\bar \alpha)^2},
    \end{equation*}
    which coincides with \eqref{eq:initial:data:Arc} for $\Delta \phi = 0$. Similarly
    \begin{equation*}
        \delta \theta \rest_{\bar \theta = \frac{\pi}{2}} = \frac{\delta \bar s}{|P_2 - P_1|} \left( \cos(\theta_0) + \cot(\bar \alpha) \sin(\theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \right)
    \end{equation*}
    coincides with $\delta \phi_1 \rest{\Delta \phi = 0}$ given by \eqref{eq:delta:phi:1}.
\end{remark}


\subsubsection{Analysis of the derivative $\bar r_{\phi_0}$ (segment case)}
\label{Sss:deriv_ana_segment_case}


In this subsection we study the RDE satisfied by the derivative $\bar r_{\phi_0}$.

\begin{description}
    \item[$\phi\in [\phi_0+\bar\theta-\bar\alpha,\phi_0+2\pi+\theta_0)$] being $s^-(\phi)$ the same for both solutions, it holds
        \begin{equation*}
            \frac{d\bar r_{\phi_0}(\phi)}{d\phi} = \bar r_{\phi_0}(\phi) \cot(\bar \alpha).
        \end{equation*}
    In particular the solution is computed as
    \begin{equation*}
        \bar{g}_{\phi_0}(\phi)=\bar{g}_{\phi_0}\left(\phi_0+\bar\theta-\bar\alpha\right)e^{\cot\bar\alpha(\phi-(\phi_0+\bar\theta-\bar\alpha))}.
    \end{equation*}
    {\color{red}    \begin{equation*}
        \bar r_{\phi_0}(\phi) = \bar r_{\phi_0}(\phi_2) e^{\cot(\bar \alpha) (\phi - (\phi_0 + \bar \theta - \bar \alpha))},
    \end{equation*}}
   where  $\bar r_{\phi_0}(\phi_2)$ is given by the formula \eqref{eq:initial:point:segment}.
 
   \item[$\phi=\phi_0+2\pi+\theta_0$]the derivative $\bar r_{\bar s}$ has a downward jump due to the segment $\delta \bar s e^{i \theta_0}$, that is
   \begin{equation}
       \bar g_{\phi_0}(\phi_0+2\pi+\theta_0)- \bar g_{\phi_0}(\phi_0+2\pi+\theta_0-)=-\frac{\sin\bar\theta}{\sin(\bar\theta-\theta_0)},
   \end{equation}
{\color{red}   \begin{equation}
       \bar r_{\phi_0}(\phi_0 + 2\pi + \theta_0) - \bar r_{\phi_0}(\phi_0 + 2\pi + \theta_0-) = - 1.
   \end{equation}}
   %which is computed by subtracting the length $\frac{|P_1-\tilde P_1|}{h}$.

\item[$\phi \in [\phi_0 + 2\pi + \theta_0, \phi_0 + 2\pi +\bar \theta)$] here the base point for the optimal ray is $P_1$, so that it holds
    \begin{equation*}
        \frac{d\bar g_{\phi_0}(\phi)}{d\phi}=\bar g_{\phi_0}(\phi)\cot\bar\alpha.
        \end{equation*}
{\color{red} \begin{equation*}
        \frac{d\bar r_{\phi_0}(\phi)}{d\phi} = \bar r_{\phi_0}(\phi) \cot(\bar \alpha).
        \end{equation*}}
    
\item[$\phi = \phi_0 + 2\pi + \bar\theta$] there is a jump, due to the fact that the segment $[P_1,P_2]$ changes length and direction. {\color{red} Computing the variation for small angles and assuming $\delta \bar \theta > 0$ (the other case being completely similar)
    \begin{equation*}
        r_{\phi_0}(\phi_0 + 2\pi + \bar\theta + \delta \bar \theta) = \big( r_{\phi_0}(2\pi + \bar \theta + \phi_0) - |P_2-P_1| \big)\big( 1 + \cot(\bar \alpha) \delta \bar \theta \big) -\frac{r_{\phi_0}(P_2) \delta \bar \theta}{\sin(\bar \alpha)};
    \end{equation*}
     \begin{equation*}
        \tilde f_{\phi_0}(\phi_0+2\pi+\bar\theta+\delta\bar\theta)=\tilde f_{\phi_0}(2\pi+\bar\theta+\phi_0)+\delta\bar\theta \tilde f_{\phi_0}(2\pi+\bar\theta+\phi_0)\cot\bar\alpha-|\tilde P_2-\tilde P_1|.
    \end{equation*}
Hence, by \eqref{eq:difference:length} and \eqref{Equa:delta_bar_theta_segment}, the jump is
\begin{align*}
       \bar r_{\phi_0}(\phi_0 + 2\pi + \bar \theta) - \bar r_{\phi_0}(\phi_0 + 2\pi + \bar \theta-) &= \frac{1}{\delta \bar s} \left( - \delta |P_2 - P_1| + |P_2 - P_1| \cot(\bar \alpha) \delta \bar \theta + \frac{r_{\phi_0}(P_2)}{\sin(\bar \alpha)} \delta \bar \theta \right) \\
       &= - \sin(\bar \theta - \theta_0) \cot(\bar \alpha) + 2 |P_2 - P_1| \cot(\bar \alpha) \frac{\delta \bar \theta}{\delta \bar s} + \cos(\bar \theta - \theta_0) \\
       &= \sin(\bar \theta - \theta_0) \cot(\bar \alpha) + \cos(\bar\theta - \theta_0) \frac{1 + \cos(\bar \alpha)^2}{\sin^2(\bar \alpha)} - 2 \cot(\bar \alpha)^2 \frac{\cos(\hat \alpha)}{\cos(\bar \alpha)}.
\end{align*}
}

that is
    \begin{align*}
       &\bar g_{\phi_0}(\phi_0+2\pi+\bar\theta)- \bar g_{\phi_0}(\phi_0+2\pi+\bar\theta-)=\\ & =-\delta|P_2-P_1|+\frac{f_{\phi_0}(P_2)}{\sin\bar\alpha}\delta\bar\theta\\ & =\frac{\cot(\bar\theta-\theta_0)\sin\bar\theta}{\sin^2\bar\alpha}-\cot^2\bar\alpha\frac{\sin\bar\theta}{\sin(\bar\theta-\theta_0)},
   \end{align*}
   which is computed as follows:
    \begin{equation*}
        f_{\phi_0}(\phi_0+2\pi+\bar\theta+\delta\bar\theta)=f_{\phi_0}(2\pi+\bar\theta+\phi_0)+\delta\bar\theta f_{\phi_0}(2\pi+\bar\theta+\phi_0)\cot\bar\alpha-\frac{f_{\phi_0}(P_2)\delta\bar\theta}{\sin\bar\alpha}-|P_2-P_1|;
    \end{equation*}
     \begin{equation*}
        \tilde f_{\phi_0}(\phi_0+2\pi+\bar\theta+\delta\bar\theta)=\tilde f_{\phi_0}(2\pi+\bar\theta+\phi_0)+\delta\bar\theta \tilde f_{\phi_0}(2\pi+\bar\theta+\phi_0)\cot\bar\alpha-|\tilde P_2-\tilde P_1|.
    \end{equation*}
    The computation of the jump then follows by applying  \eqref{eq:difference:length}.
   
\item[$\phi \geq \phi_0 + 2\pi + \bar \theta$] the function $\bar r_{\phi_0}$ satisfies
    \begin{equation*}
        \frac{d\bar r_{\phi_0}}{d\phi} = \cot(\bar \alpha) \bar r_{\phi_0}(\phi) - \frac{\bar r_{\phi_0}(\phi - 2\pi - \bar \alpha)}{\sin(\bar \alpha)}.
    \end{equation*}
\end{description}

{\color{red} \begin{remark}
    \label{Rem:comaris_ODE_segment_arc}
    Observe that when $\bar \theta = \frac{\pi}{2}$ the last jump becomes
    \begin{equation*}
        \cos(\theta_0) \cot(\bar \alpha) + \sin(\theta_0) \frac{1 + \cos(\bar \alpha)^2}{\sin(\bar \alpha)^2} - 2 \cot(\bar \alpha)^2 \frac{\cos(\hat \alpha)}{\cos(\bar \alpha)}, 
    \end{equation*}
    which is equal to the sum of the jumps \eqref{Equa:jump_init_cirle} and \eqref{Equa:J_jump_speriamo_bene} for $\Delta \phi = 0$. This proves that $\bar r_{\phi_0}$ depends continuously on the parameter {\color{blue} cos'è $\beta$?}$\bar \theta,\Delta \phi$ across the point $\bar \theta = \frac{\pi}{2}, \Delta \phi = 0$.
\end{remark}}

%We have then that $$\bar f_{\phi_0}=\frac{\sin(\bar\theta-\theta_0)}{\sin\bar\theta}\bar g_{\phi_0},$$ so the values of the two jumps are computed as
%\begin{description}
%    \item In the point $\phi=\phi_0+2\pi+\theta_0$ the downward jump is
%   \begin{equation}
%       \bar f_{\phi_0}(\phi_0+2\pi+\theta_0)- \bar f_{\phi_0}(\phi_0+2\pi+\theta_0-)=-1;
%   \end{equation}
%   \item In the point $\phi=\phi_0+2\pi+\bar\theta$ the jump is 
%   \begin{align*}
%&\bar f_{\phi_0}(\phi_0+2\pi+\bar\theta)- \bar f_{\phi_0}(\phi_0+2\pi+\bar\theta-) =\frac{\cos(\bar\theta-\theta_0)}{\sin^2\bar\alpha}-\cot^2\bar\alpha.
%   \end{align*}
%
%\begin{align*}
%    r_{\bar + \delta \bar s}(+\epsilon) &= \Big[ r_{\bar + \delta \bar s}(-\epsilon) \big( 1 + \cot(\bar \alpha)(\epsilon + \delta \phi) \big) - |\tilde P_2 - \tilde P_1| \Big] \big( 1 + \cot(\bar \alpha) (\epsilon - \delta \phi) \big) - \frac{r_{\bar + \delta \bar s}(\phi_2)}{\sin(\bar \alpha)} (\epsilon - \delta \phi) \\
%    &= r_{\bar + \delta \bar s}(-\epsilon) \big( 1 + 2 \cot(\bar \alpha) \epsilon \big) - |\tilde P_2 - \tilde P_1| \big( 1 + \cot(\bar \alpha) (\epsilon - \delta) \big) - \frac{r_{\bar + \delta \bar s}(\phi_2)}{\sin(\bar \alpha)} (\epsilon - \delta \phi),
%\end{align*}
%\begin{align*}
%    \bar r_{\bar s}(+\epsilon) &= \bar r_{\bar s}(-\epsilon) \big( 1 + 2\cot(\bar \alpha) \epsilon \big) - \delta |P_2 - P_1| (1 + \cot(\bar \alpha) \epsilon) + |P_2 - P_1| \cot(\alpha) \frac{d\phi}{d\bar s} - \frac{\bar r_{\bar s}(\phi_2)}{\sin(\bar \alpha)} \epsilon + \frac{r_{\bar s}(\phi_2)}{\sin(\bar \alpha)} \frac{d\delta \phi}{d\bar s},
%\end{align*}
%\begin{align*}
%    \bar r(+) &= \bar r(-) - \delta |P_2 - P_1| + |P_2 - P_1| \cot(\bar \alpha) \delta \phi + \frac{r(\phi_2)}{\sin(\bar \alpha)} \delta \phi \\
%    &= - (h \sin\bar\theta-2|P_2-P_1|\delta\bar\theta)\cot\bar\alpha + h \sin(\bar \theta) \cot(\bar \theta - \theta_0) \\
%    &= - \left( h \sin(\bar \theta) - 2 \left[ h \left( \sin(\bar \theta) + \cot(\bar \alpha) \sin(\bar \theta) \cot(\bar \theta - \theta_0) - \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \frac{\sin(\bar \theta)}{\sin(\bar \theta - \theta_0)} \right) \right] \right) \cot(\bar \alpha) + h \sin(\bar \theta) \cot(\bar \theta - \theta_0) \\
%    &= h \left[ \sin(\bar \theta) \cot(\bar \alpha) + \sin(\bar \theta) \cot(\bar \theta - \theta_0) \big( 1 + 2 \cot(\bar \alpha)^2 \big) - 2 \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \frac{\sin(\bar \theta)}{\sin(\bar \theta - \theta_0)} \cot(\bar \alpha) \right].
%\end{align*}
%For $\bar \theta = \frac{\pi}{2}$, $h = \delta \bar s \cos(\theta_0)$
%\begin{align*}
%    & \cos(\theta_0) \left[ \cot(\bar \alpha) + \tan(\theta_0) \big( 1 + 2 \cot(\bar \alpha)^2 \big) - 2 \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \frac{1}{\cos(\theta_0)} \cot(\bar \alpha) \right] \\
%    &= \left[ \cot(\bar \alpha) \cos(\theta_0) + \sin(\theta_0) \big( 1 + 2 \cot(\bar \alpha)^2 \big) - 2 \frac{\cos(\hat \alpha)}{\sin(\bar \alpha)} \cot(\bar \alpha) \right]
%\end{align*}
%
%
%\end{description}


{\color{red}
As a function of $\tau$, the data are
\begin{equation*}
    \rho_0 = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)}(1 - \cos(\bar \theta - \theta_0)) e^{-\bar c(2\pi + \bar \alpha) \tau_0}, \quad \tau_0 = \frac{\bar \theta - \bar \alpha}{2\pi + \bar \alpha},
\end{equation*}
\begin{equation*}
    \rho_1 = - e^{-\bar c (2\pi + \bar \alpha) \tau_1}, \quad \tau_1 = \frac{2\pi + \theta_0}{2\pi + \bar \alpha},
\end{equation*}
\begin{equation*}
    \rho_2 = \big( \cot(\bar \alpha) \sin(\bar \theta - \theta_0) + \cos(\theta - \theta_0) - 2 \cot(\bar \alpha)^2 (1 - \cos(\bar \theta - \theta_0) \big) e^{-\bar c (2\pi + \bar \alpha) \tau_2}, \quad \tau_2 = 1 + \tau_0,
\end{equation*}
\begin{equation*}
    \rho(\tau) = \rho_0 g(\tau - \tau_0) + \rho_1 g(\tau - \tau_1) + \rho_2 g(\tau - \tau_2).
\end{equation*}
In this case we can get rid of one parameter by translating to $\tau_0 \to 0$ and collecting $e^{-\bar c(2\pi + \bar \alpha) \tau_0}$: setting $\theta = \bar \theta - \theta_0$
\begin{equation*}
    \rho_0 = \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)}(1 - \cos(\theta)), \quad \tau_0 = 0,
\end{equation*}
\begin{equation*}
    \rho_1 = - e^{-\bar c (2\pi + \bar \alpha) \tau_1}, \quad \tau_1 = 1 - \frac{\theta}{2\pi + \bar \alpha},
\end{equation*}
\begin{equation*}
    \rho_2 = \big( \cot(\bar \alpha) \sin(\theta) + \cos(\theta) - 2 \cot(\bar \alpha)^2 (1 - \cos(\theta) \big) e^{-\bar c (2\pi + \bar \alpha) \tau_2}, \quad \tau_2 = 1,
\end{equation*}
\begin{equation*}
    \rho(\tau) = \rho_0 g(\tau) + \rho_1 g(\tau - \tau_1) + \rho_2 g(\tau - 1).
\end{equation*}
The new parameter $\theta$ takes values in $[0,\frac{\pi}{2}]$.

{\bf \color{blue} ADD A JUMP AT $2\pi + \bar \alpha + 2\pi + \bar \theta \sim 2 + \tau_0$ OF SIZE $\frac{\delta r(\phi - 2\pi-\bar \alpha)}{\sin(\bar \alpha)}$: in the $\rho$ coordinates it corresponds to a multiplication by $(2\pi+\bar \alpha)^{-1}$, so that
\begin{equation*}
    \frac{|P_2 - P_1| \delta \theta}{\sin(\bar \alpha)} e^{-\bar c(2\pi+\bar \alpha)(2+\tau_0)} \delta_{\tau = 2 + \tau_0} = \big( \sin(\bar \theta - \theta_0) - \cot(\bar \alpha) (1 - \cos(\theta - \theta_0)) \big) e^{-\bar c(2\pi+\bar \alpha)(2+\tau_0)} \delta_{\tau = 2 + \tau_0}.
\end{equation*}

}

It is then particularly easy to compute the derivative: using the previous formulas
\begin{align*}
    \partial_\theta \rho(\tau) &= \frac{\cot(\bar \alpha)}{\sin(\bar \alpha)}(2 - \cos(\theta)) g(\tau) - \cot(\bar \alpha) e^{-\bar c (2\pi + \bar \alpha) \tau_1} g(\tau - \tau_1) + \frac{e^{-\bar c (2\pi + \bar \alpha) \tau_1}}{2\pi + \bar \alpha} g(\tau - \tau_1 - 1) \\
    & \quad + \big( \cot(\bar \alpha) \cos(\theta) - (1 + 2 \cot(\bar \alpha)^2) \sin(\theta) \big) e^{-\bar c(2\pi + \bar \alpha)} g(\tau - 1).
\end{align*}
Again numerically the derivative is $\geq .01$ for $\tau \geq 2$, and numerically the solution is positive for $\tau \in [1,2]$.

The only case to consider is the negative region obtained by
\begin{align*}
    \rho(\tau_1) &= \rho_0 e^{\tau_1} + \rho_1 \\
    &= \frac{\cot(\bar \alpha)}{
    \sin(\bar \alpha)}(1 - \cos(\theta)) e^{\tau_1} - e^{-\bar c (2\pi + \bar \alpha) \tau_1} \\
    &= e^{-\bar c (2\pi + \bar \alpha) \tau_1} \bigg( \frac{\cot(\bar \alpha)}{
    \sin(\bar \alpha)}(1 - \cos(\theta)) e^{\cot(\bar \alpha) (2\pi + \bar \alpha) \tau_1} - 1 \bigg).
\end{align*}
It is negative in the interval $\theta \in [0,.608463]$, otherwise positive for larger angles. After $\tau = 1$ it is always positive.
}
\subsection{Diverging family: segment case}
\label{Ss:devirg_segment}


In this subsection we will prove that also in the segment case the derivative $\bar r_{\phi_0}(\phi) \geq 0$ for every $\phi$, verifying the divergence condition on the family of generalized barriers of Lemma \ref{lem:key}. As in the previous section, we will need to evaluate the relevant quantities numerically: the numerical plots of these functions can be found in the Appendix, Section \ref{s:appendix:segm}.

\begin{theorem}
\label{thm:div:segm}
    Let $\hat \sigma \leq 2.3$ and let $r_{\phi_0}$ be an element of the family made by a segment and a saturated spiral. Then its derivative $\bar r_{\phi_0}(\phi)$ w.r.t. the initial position $\bar s$ is positive for every angle $\phi$.
\end{theorem}

\begin{proof}
{\color{red} By a translation we will assume that $\phi_0 = 0$, in order to shorten the notation.}
Without loss of generality we can assume $\phi_0=0$.

We compute the solution $\bar r_{\phi_0}$ by means of Lemma \ref{lem:conti:uguali}.
Call 
 $$\bar{f}_{\phi_0}\left(\phi_0+\bar\theta-\bar\alpha\right)=\kappa_1(\bar\theta,\theta_0)=\frac{\cos\hat\alpha-\cos\bar\alpha\cos(\bar\theta-\theta_0)}{\sin\bar\alpha^2},$$
 \medskip
 
 $$\bar f_{\phi_0}(2\pi+\theta_0)=\kappa_2(\bar\theta,\theta_0)=\kappa_1(\bar\theta,\theta_0)e^{\cot\bar\alpha(2\pi+\theta_0-\bar\theta+\bar\alpha)}-1,$$
 \medskip

  $$\bar f_{\phi_0}(2\pi+\bar\theta)=\kappa_3(\bar\theta,\theta_0)=\kappa_2(\bar\theta,\theta_0)e^{\cot\bar\alpha(\bar\theta-\theta_0)}+\frac{\cos(\bar\theta-\theta_0)}{\sin\bar\alpha^2}-\cot^2\bar\alpha.$$
 \medskip
 
So by Lemma \ref{lem:conti:uguali} we have that the solution reads as
   \begin{itemize}
   
   \item for $\phi\in[2\pi+\bar\theta,4\pi+\theta_0+\bar\alpha)$
   \begin{equation}\label{eq:sol:up:4pithetaalpha}
       \bar f_{\phi_0}(\phi)=\left(\kappa_3(\bar\theta,\theta_0)-\frac{\kappa_1(\bar\theta,\theta_0)}{\sin\bar\alpha}(\phi-2\pi-\bar\theta)\right)e^{\cot\bar\alpha(\phi-2\pi-\bar\theta)}.
   \end{equation}
  Call
  \begin{equation*}
      \bar f_{\phi_0}(4\pi+\theta_0+\bar\alpha)=\kappa_4(\bar\theta,\theta_0).
  \end{equation*}
  \item For $\phi\in[4\pi+\theta_0+\bar\alpha,4\pi+\bar\theta+\bar\alpha]$ the solution reads as
  \begin{equation}
  \label{eq:sol:up:4pitheta:bar:alpha}
      \bar f_{\phi_0}(\phi)=\left(\kappa_4(\bar\theta,\theta_0)-\frac{\kappa_2(\bar\theta,\theta_0)}{\sin\bar\alpha}(\phi-4\pi-\theta_0-\bar\alpha)\right)e^{\cot\bar\alpha(\phi-4\pi-\theta_0-\bar\alpha)},
  \end{equation}
  and so on.
  \end{itemize}
  Again, to apply Lemma \ref{lem:conti:uguali:2:che:palle}, we need to verify that $\kappa_i(\bar\theta,\theta_0)\geq 0$, for every $i=1,2,3,4$. We evaluate numerically these quantities and we find that $\kappa_i\geq 0$ for $i=1,2,3,4$, corresponding to Figures \ref{fig:seg:k:1},\ref{fig:seg:k:2},\ref{fig:seg:k:3},\ref{fig:seg:k:4} in the Appendix. The proof proceeds exactly in the same way as the one of the arc case (see Theorem \ref{thm:div:arc}). Indeed it is enough to show, by Lemma \ref{lem:conti:uguali:2:che:palle}, that the two following quantities are positive (see Appendix \ref{S:appendix: fire}, Section \ref{s:appendix:segm}).
  \begin{equation*}
         -\frac{\kappa_1}{\sin\bar\alpha}\left(4\pi+\theta_0+2\bar\alpha-\bar\theta\right)+\kappa_3\geq 0
    \end{equation*}
    and
    \begin{equation*}
        -\frac{\kappa_2}{\sin\bar\alpha}\left(2\pi+\bar\alpha+\bar\theta-\theta_0\right)+\kappa_4\geq 0.
    \end{equation*}

\end{proof}
Again the numerical evaluations can be found in Figures \ref{fig:seg:Q:1},\ref{fig:seg:Q:2}.
\begin{remark}
    We remark that the previous computations are compatible with the ones done for the arc case in the case $\Delta\phi=0$ and $\bar\theta=\frac{\pi}{2}$.
\end{remark}
%\begin{remark}
 %   It would be interesting to investigate the optimization w.r.t. $\bar\theta$ and $\theta_0$. 
%\end{remark}

